Automation and Taxation

Decomposing taxes by source (labor, capital, sales), we analyze the impact of automation on tax revenues and the structure of taxation in 19 EU countries during 1995-2016. Pre-2008, robot diffusion lead to decreasing factor and tax income, and a shift from taxes on capital to goods. ICTs changed the structure of taxation from capital to labor, with decreasing employment, but increasing wages and labor income. Post-2008, we find an ICT-induced increase in capital income and services, but no effect on taxation from ICT/robots. Overall, automation goes through various phases with heterogeneous economic effects which impact the amount and structure of taxes. Whether automation erodes taxation depends on the technology and stage of diffusion, and thus concerns about public budgets might be myopic when focusing on the short-run and ignoring relevant technological trends.

==> inputs/all_95_16/Results1RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.026$^{\ast}$        &      -0.051$^{\ast\ast}$    &       0.005                 &      -0.021                 &       0.093                 &      -0.292                 &       0.358                 &       0.026                 &      -0.955                 &       0.758                 &      -0.092                 \\
            &     (0.014)                 &     (0.022)                 &     (0.042)                 &     (0.020)                 &     (0.467)                 &     (0.233)                 &     (0.363)                 &     (0.199)                 &     (0.635)                 &     (0.898)                 &     (0.621)                 \\\addlinespace
$ICT_{c,t}$&      -0.042$^{\ast\ast\ast}$&      -0.081                 &      -0.101$^{\ast\ast\ast}$&      -0.024                 &      -1.359$^{\ast\ast}$    &       0.225                 &      -1.499$^{\ast\ast}$    &      -0.085                 &       1.689                 &      -2.103$^{\ast}$        &       0.596                 \\
            &     (0.013)                 &     (0.107)                 &     (0.033)                 &     (0.022)                 &     (0.529)                 &     (0.383)                 &     (0.602)                 &     (0.196)                 &     (1.001)                 &     (1.110)                 &     (0.694)                 \\\addlinespace
$R*ICT_{c,t}$&       0.018$^{\ast\ast}$    &       0.023                 &       0.044$^{\ast\ast}$    &       0.027$^{\ast\ast}$    &       0.405                 &      -0.262                 &       0.492$^{\ast}$        &       0.176                 &      -1.068$^{\ast\ast\ast}$&       0.812$^{\ast}$        &       0.201                 \\
            &     (0.007)                 &     (0.039)                 &     (0.016)                 &     (0.012)                 &     (0.257)                 &     (0.161)                 &     (0.248)                 &     (0.131)                 &     (0.292)                 &     (0.451)                 &     (0.407)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .998                 &        .999                 &        .966                 &        .984                 &        .974                 &        .904                 &        .982                 &        .971                 &        .939                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/all_95_16/Results2RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.019$^{\ast}$        &      -0.039$^{\ast}$        &       0.013                 &      -0.014                 &      -0.056                 &      -0.323                 &       0.322                 &      -0.055                 &      -0.922                 &       0.801                 &      -0.202                 \\
            &     (0.010)                 &     (0.019)                 &     (0.040)                 &     (0.021)                 &     (0.421)                 &     (0.226)                 &     (0.357)                 &     (0.127)                 &     (0.598)                 &     (0.905)                 &     (0.515)                 \\\addlinespace
$ICT_{c,t}$&      -0.061$^{\ast\ast\ast}$&      -0.093                 &      -0.122$^{\ast\ast\ast}$&      -0.047$^{\ast}$        &      -1.620$^{\ast\ast\ast}$&       0.022                 &      -1.794$^{\ast\ast}$    &       0.152                 &       1.291                 &      -2.695$^{\ast\ast}$    &       1.457$^{\ast\ast}$    \\
            &     (0.011)                 &     (0.095)                 &     (0.038)                 &     (0.024)                 &     (0.544)                 &     (0.353)                 &     (0.641)                 &     (0.165)                 &     (0.903)                 &     (1.118)                 &     (0.608)                 \\\addlinespace
$R*ICT_{c,t}$&       0.022$^{\ast\ast\ast}$&       0.022                 &       0.048$^{\ast\ast}$    &       0.031$^{\ast\ast}$    &       0.429                 &      -0.199                 &       0.589$^{\ast\ast}$    &       0.040                 &      -0.893$^{\ast\ast}$    &       1.067$^{\ast\ast}$    &      -0.196                 \\
            &     (0.005)                 &     (0.034)                 &     (0.017)                 &     (0.012)                 &     (0.290)                 &     (0.153)                 &     (0.269)                 &     (0.077)                 &     (0.363)                 &     (0.429)                 &     (0.291)                 \\\addlinespace
$wL_{c,t}$&       0.593$^{\ast\ast\ast}$&       0.721$^{\ast}$        &       0.661$^{\ast\ast}$    &       0.626$^{\ast\ast\ast}$&      -0.457$^{\ast\ast\ast}$&       0.051                 &       0.122                 &      -0.630$^{\ast\ast\ast}$&       0.560$^{\ast\ast}$    &       0.799$^{\ast\ast}$    &      -1.392$^{\ast\ast\ast}$\\
            &     (0.164)                 &     (0.345)                 &     (0.280)                 &     (0.150)                 &     (0.156)                 &     (0.111)                 &     (0.133)                 &     (0.094)                 &     (0.245)                 &     (0.377)                 &     (0.253)                 \\\addlinespace
$rK_{c,t}$&       0.097                 &       0.260                 &       0.119                 &       0.069                 &      -0.656$^{\ast\ast\ast}$&      -0.022                 &       0.025                 &      -0.659$^{\ast\ast\ast}$&       0.508$^{\ast\ast}$    &       0.715$^{\ast\ast}$    &      -1.315$^{\ast\ast\ast}$\\
            &     (0.090)                 &     (0.256)                 &     (0.162)                 &     (0.091)                 &     (0.135)                 &     (0.088)                 &     (0.105)                 &     (0.073)                 &     (0.178)                 &     (0.262)                 &     (0.216)                 \\\addlinespace
$pQ_{c,t}$&       0.205                 &      -0.066                 &       0.128                 &       0.238                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.246)                 &     (0.561)                 &     (0.378)                 &     (0.220)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.003                 &       0.005                 &      -0.002                 &       0.004                 &      -0.031                 &       0.039                 &      -0.004                 &      -0.109                 &       0.135                 &      -0.004                 \\
            &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.002)                 &     (0.039)                 &     (0.026)                 &     (0.027)                 &     (0.016)                 &     (0.076)                 &     (0.086)                 &     (0.040)                 \\\addlinespace
$Services_{c,t}$&      -0.003                 &       0.011                 &      -0.014                 &      -0.015$^{\ast\ast}$    &      -0.026                 &       0.151$^{\ast}$        &      -0.129                 &      -0.047                 &       0.513$^{\ast\ast}$    &      -0.371                 &      -0.169                 \\
            &     (0.004)                 &     (0.013)                 &     (0.010)                 &     (0.007)                 &     (0.091)                 &     (0.080)                 &     (0.099)                 &     (0.042)                 &     (0.235)                 &     (0.273)                 &     (0.111)                 \\\addlinespace
$HHI_{c,t}$&      -0.886                 &       2.203                 &      -3.399                 &      -2.793$^{\ast\ast\ast}$&     -13.553                 &      24.999$^{\ast}$        &     -27.689                 &     -10.863                 &      90.046$^{\ast\ast}$    &     -73.312                 &     -16.057                 \\
            &     (0.575)                 &     (1.771)                 &     (2.073)                 &     (0.840)                 &    (17.702)                 &    (13.563)                 &    (18.820)                 &     (7.968)                 &    (42.454)                 &    (58.541)                 &    (24.486)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.002$^{\ast\ast\ast}$&       0.000                 &       0.004$^{\ast\ast}$    &       0.002$^{\ast\ast\ast}$&       0.051$^{\ast\ast\ast}$&      -0.005                 &       0.038$^{\ast\ast\ast}$&       0.018$^{\ast\ast\ast}$&      -0.062$^{\ast\ast}$    &       0.061                 &      -0.007                 \\
            &     (0.000)                 &     (0.001)                 &     (0.001)                 &     (0.001)                 &     (0.012)                 &     (0.007)                 &     (0.013)                 &     (0.004)                 &     (0.024)                 &     (0.036)                 &     (0.012)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.008                 &       0.004                 &      -0.021                 &      -0.012$^{\ast}$        &      -0.324                 &      -0.050                 &      -0.171                 &      -0.103$^{\ast\ast}$    &       0.298                 &      -0.266                 &       0.211                 \\
            &     (0.007)                 &     (0.008)                 &     (0.015)                 &     (0.006)                 &     (0.191)                 &     (0.091)                 &     (0.155)                 &     (0.044)                 &     (0.257)                 &     (0.391)                 &     (0.156)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.005$^{\ast\ast\ast}$&      -0.002                 &       0.004                 &       0.006$^{\ast\ast}$    &       0.116$^{\ast\ast\ast}$&       0.012                 &       0.071$^{\ast}$        &       0.033$^{\ast\ast\ast}$&      -0.029                 &       0.047                 &      -0.032                 \\
            &     (0.001)                 &     (0.004)                 &     (0.004)                 &     (0.002)                 &     (0.028)                 &     (0.019)                 &     (0.036)                 &     (0.011)                 &     (0.065)                 &     (0.084)                 &     (0.040)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.007                 &       0.009                 &       0.004                 &      -0.003                 &      -0.001                 &       0.020                 &       0.039                 &      -0.060                 &       0.055                 &      -0.021                 &      -0.182                 \\
            &     (0.006)                 &     (0.009)                 &     (0.015)                 &     (0.006)                 &     (0.193)                 &     (0.106)                 &     (0.154)                 &     (0.062)                 &     (0.274)                 &     (0.333)                 &     (0.221)                 \\\addlinespace
$XRate_{c,t}$&      -0.004$^{\ast\ast\ast}$&      -0.004                 &      -0.004                 &      -0.008$^{\ast\ast\ast}$&      -0.089$^{\ast\ast}$    &      -0.002                 &      -0.075$^{\ast}$        &      -0.012                 &       0.101                 &      -0.090                 &       0.042                 \\
            &     (0.001)                 &     (0.006)                 &     (0.003)                 &     (0.002)                 &     (0.036)                 &     (0.028)                 &     (0.038)                 &     (0.011)                 &     (0.067)                 &     (0.081)                 &     (0.034)                 \\\midrule
%$R^{2}$  &          0.999                &        .998                 &        .999                 &        .999                 &        .973                 &        .985                 &        .975                 &         .96                 &        .983                 &        .972                 &        .956                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/all_95_16/Results2shortEXCGDPV1_RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{8}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.019$^{\ast}$        &      -0.039$^{\ast}$        &       0.013                 &      -0.014                 &      -0.922                 &       0.801                 &      -0.202                 \\
            &     (0.010)                 &     (0.019)                 &     (0.040)                 &     (0.021)                 &     (0.598)                 &     (0.905)                 &     (0.515)                 \\\addlinespace
$ICT_{c,t}$&      -0.061$^{\ast\ast\ast}$&      -0.093                 &      -0.122$^{\ast\ast\ast}$&      -0.047$^{\ast}$        &       1.291                 &      -2.695$^{\ast\ast}$    &       1.457$^{\ast\ast}$    \\
            &     (0.011)                 &     (0.095)                 &     (0.038)                 &     (0.024)                 &     (0.903)                 &     (1.118)                 &     (0.608)                 \\\addlinespace
$R*ICT_{c,t}$&       0.022$^{\ast\ast\ast}$&       0.022                 &       0.048$^{\ast\ast}$    &       0.031$^{\ast\ast}$    &      -0.893$^{\ast\ast}$    &       1.067$^{\ast\ast}$    &      -0.196                 \\
            &     (0.005)                 &     (0.034)                 &     (0.017)                 &     (0.012)                 &     (0.363)                 &     (0.429)                 &     (0.291)                 \\\addlinespace
$wL_{c,t}$&       0.593$^{\ast\ast\ast}$&       0.721$^{\ast}$        &       0.661$^{\ast\ast}$    &       0.626$^{\ast\ast\ast}$&       0.560$^{\ast\ast}$    &       0.799$^{\ast\ast}$    &      -1.392$^{\ast\ast\ast}$\\
            &     (0.164)                 &     (0.345)                 &     (0.280)                 &     (0.150)                 &     (0.245)                 &     (0.377)                 &     (0.253)                 \\\addlinespace
$rK_{c,t}$&       0.097                 &       0.260                 &       0.119                 &       0.069                 &       0.508$^{\ast\ast}$    &       0.715$^{\ast\ast}$    &      -1.315$^{\ast\ast\ast}$\\
            &     (0.090)                 &     (0.256)                 &     (0.162)                 &     (0.091)                 &     (0.178)                 &     (0.262)                 &     (0.216)                 \\\addlinespace
$pQ_{c,t}$&       0.205                 &      -0.066                 &       0.128                 &       0.238                 &                             &                             &                             \\
            &     (0.246)                 &     (0.561)                 &     (0.378)                 &     (0.220)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &        .999                 &        .983                 &        .972                 &        .956                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/all_95_16/Results2shortEXCGDPV2_RICTint_ct_All_95t16.tex <==
& $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{4}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.922                 &       0.801                 &      -0.202                 \\
            &     (0.598)                 &     (0.905)                 &     (0.515)                 \\\addlinespace
$ICT_{c,t}$&       1.291                 &      -2.695$^{\ast\ast}$    &       1.457$^{\ast\ast}$    \\
            &     (0.903)                 &     (1.118)                 &     (0.608)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.893$^{\ast\ast}$    &       1.067$^{\ast\ast}$    &      -0.196                 \\
            &     (0.363)                 &     (0.429)                 &     (0.291)                 \\\addlinespace
$wL_{c,t}$&       0.560$^{\ast\ast}$    &       0.799$^{\ast\ast}$    &      -1.392$^{\ast\ast\ast}$\\
            &     (0.245)                 &     (0.377)                 &     (0.253)                 \\\addlinespace
$rK_{c,t}$&       0.508$^{\ast\ast}$    &       0.715$^{\ast\ast}$    &      -1.315$^{\ast\ast\ast}$\\
            &     (0.178)                 &     (0.262)                 &     (0.216)                 \\\midrule
$R^{2}$  &        .983                 &        .972                 &        .956                 \\
$N$      &         395                 &         395                 &         395                 \\


==> inputs/all_95_16/Results2shortV1_RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\cmidrule(l){2-5} \cmidrule(l){6-9} \cmidrule(l){10-12} & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule
\multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016 (N = 395)}}} \\\midrule
$R_{c,t}$ &      -0.019$^{\ast}$        &      -0.039$^{\ast}$        &       0.013                 &      -0.014                 &      -0.056                 &      -0.323                 &       0.322                 &      -0.055                 &      -0.922                 &       0.801                 &      -0.202                 \\
            &     (0.010)                 &     (0.019)                 &     (0.040)                 &     (0.021)                 &     (0.421)                 &     (0.226)                 &     (0.357)                 &     (0.127)                 &     (0.598)                 &     (0.905)                 &     (0.515)                 \\\addlinespace
$ICT_{c,t}$&      -0.061$^{\ast\ast\ast}$&      -0.093                 &      -0.122$^{\ast\ast\ast}$&      -0.047$^{\ast}$        &      -1.620$^{\ast\ast\ast}$&       0.022                 &      -1.794$^{\ast\ast}$    &       0.152                 &       1.291                 &      -2.695$^{\ast\ast}$    &       1.457$^{\ast\ast}$    \\
            &     (0.011)                 &     (0.095)                 &     (0.038)                 &     (0.024)                 &     (0.544)                 &     (0.353)                 &     (0.641)                 &     (0.165)                 &     (0.903)                 &     (1.118)                 &     (0.608)                 \\\addlinespace
$R*ICT_{c,t}$&       0.022$^{\ast\ast\ast}$&       0.022                 &       0.048$^{\ast\ast}$    &       0.031$^{\ast\ast}$    &       0.429                 &      -0.199                 &       0.589$^{\ast\ast}$    &       0.040                 &      -0.893$^{\ast\ast}$    &       1.067$^{\ast\ast}$    &      -0.196                 \\
            &     (0.005)                 &     (0.034)                 &     (0.017)                 &     (0.012)                 &     (0.290)                 &     (0.153)                 &     (0.269)                 &     (0.077)                 &     (0.363)                 &     (0.429)                 &     (0.291)                 \\\addlinespace
$wL_{c,t}$&       0.593$^{\ast\ast\ast}$&       0.721$^{\ast}$        &       0.661$^{\ast\ast}$    &       0.626$^{\ast\ast\ast}$&      -0.457$^{\ast\ast\ast}$&       0.051                 &       0.122                 &      -0.630$^{\ast\ast\ast}$&       0.560$^{\ast\ast}$    &       0.799$^{\ast\ast}$    &      -1.392$^{\ast\ast\ast}$\\
            &     (0.164)                 &     (0.345)                 &     (0.280)                 &     (0.150)                 &     (0.156)                 &     (0.111)                 &     (0.133)                 &     (0.094)                 &     (0.245)                 &     (0.377)                 &     (0.253)                 \\\addlinespace
$rK_{c,t}$&       0.097                 &       0.260                 &       0.119                 &       0.069                 &      -0.656$^{\ast\ast\ast}$&      -0.022                 &       0.025                 &      -0.659$^{\ast\ast\ast}$&       0.508$^{\ast\ast}$    &       0.715$^{\ast\ast}$    &      -1.315$^{\ast\ast\ast}$\\
            &     (0.090)                 &     (0.256)                 &     (0.162)                 &     (0.091)                 &     (0.135)                 &     (0.088)                 &     (0.105)                 &     (0.073)                 &     (0.178)                 &     (0.262)                 &     (0.216)                 \\\addlinespace
$pQ_{c,t}$&       0.205                 &      -0.066                 &       0.128                 &       0.238                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.246)                 &     (0.561)                 &     (0.378)                 &     (0.220)                 &                             &                             &                             &                             &                             &                             &                             \\%\midrule
%$R^{2}$  &          0.999                &        .998                 &        .999                 &        .999                 &        .973                 &        .985                 &        .975                 &         .96                 &        .983                 &        .972                 &        .956                 \\
%$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/all_95_16/Results2shortV2_RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{8}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.056                 &      -0.323                 &       0.322                 &      -0.055                 &      -0.922                 &       0.801                 &      -0.202                 \\
            &     (0.421)                 &     (0.226)                 &     (0.357)                 &     (0.127)                 &     (0.598)                 &     (0.905)                 &     (0.515)                 \\\addlinespace
$ICT_{c,t}$&      -1.620$^{\ast\ast\ast}$&       0.022                 &      -1.794$^{\ast\ast}$    &       0.152                 &       1.291                 &      -2.695$^{\ast\ast}$    &       1.457$^{\ast\ast}$    \\
            &     (0.544)                 &     (0.353)                 &     (0.641)                 &     (0.165)                 &     (0.903)                 &     (1.118)                 &     (0.608)                 \\\addlinespace
$R*ICT_{c,t}$&       0.429                 &      -0.199                 &       0.589$^{\ast\ast}$    &       0.040                 &      -0.893$^{\ast\ast}$    &       1.067$^{\ast\ast}$    &      -0.196                 \\
            &     (0.290)                 &     (0.153)                 &     (0.269)                 &     (0.077)                 &     (0.363)                 &     (0.429)                 &     (0.291)                 \\\addlinespace
$wL_{c,t}$&      -0.457$^{\ast\ast\ast}$&       0.051                 &       0.122                 &      -0.630$^{\ast\ast\ast}$&       0.560$^{\ast\ast}$    &       0.799$^{\ast\ast}$    &      -1.392$^{\ast\ast\ast}$\\
            &     (0.156)                 &     (0.111)                 &     (0.133)                 &     (0.094)                 &     (0.245)                 &     (0.377)                 &     (0.253)                 \\\addlinespace
$rK_{c,t}$&      -0.656$^{\ast\ast\ast}$&      -0.022                 &       0.025                 &      -0.659$^{\ast\ast\ast}$&       0.508$^{\ast\ast}$    &       0.715$^{\ast\ast}$    &      -1.315$^{\ast\ast\ast}$\\
            &     (0.135)                 &     (0.088)                 &     (0.105)                 &     (0.073)                 &     (0.178)                 &     (0.262)                 &     (0.216)                 \\\midrule
$R^{2}$  &        .973                 &        .985                 &        .975                 &         .96                 &        .983                 &        .972                 &        .956                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/all_95_16/Results3RICTint_cit_All_95t16.tex <==
& ln $wL_{i,c,t}$ & ln $w_{i,c,t}$ & ln $L_{i,c,t}$ & ln $rK_{i,c,t}$ & ln $r_{i,c,t}$ & ln $K_{i,c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{i,c,t}$&      -0.031                 &       0.026$^{\ast\ast}$    &      -0.057$^{\ast\ast}$    &      -0.053                 &      -0.011                 &       0.008                 \\
            &     (0.031)                 &     (0.010)                 &     (0.027)                 &     (0.036)                 &     (0.007)                 &     (0.027)                 \\\addlinespace
$ICT_{i,c,t}$&       0.020                 &       0.005                 &       0.015                 &       0.026                 &      -0.001                 &       0.028                 \\
            &     (0.012)                 &     (0.005)                 &     (0.013)                 &     (0.026)                 &     (0.010)                 &     (0.023)                 \\\addlinespace
$R*ICT_{i,c,t}$&      -0.007                 &       0.005$^{\ast\ast}$    &      -0.012$^{\ast\ast}$    &       0.003                 &      -0.004                 &       0.006                 \\
            &     (0.005)                 &     (0.002)                 &     (0.005)                 &     (0.009)                 &     (0.002)                 &     (0.007)                 \\\midrule
%$R^{2}$  &        .997                 &        .996                 &        .994                 &        .972                 &        .927                 &        .996                 \\
$N$      &        4898                 &        4898                 &        4898                 &        4843                 &        4803                 &        4803                 \\


==> inputs/all_95_16/Results4RICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.128$^{\ast\ast\ast}$&      -0.006                 &      -0.088$^{\ast\ast\ast}$&      -0.056$^{\ast\ast}$    &       0.003                 &      -0.941$^{\ast\ast\ast}$&       0.002                 &       0.032$^{\ast\ast\ast}$\\
            &     (0.032)                 &     (0.016)                 &     (0.031)                 &     (0.026)                 &     (0.003)                 &     (0.269)                 &     (0.004)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t}$&       0.168$^{\ast\ast\ast}$&      -0.092$^{\ast\ast}$    &       0.077                 &      -0.006                 &      -0.001                 &       0.527                 &      -0.004                 &       0.038$^{\ast\ast\ast}$\\
            &     (0.049)                 &     (0.040)                 &     (0.047)                 &     (0.069)                 &     (0.004)                 &     (1.008)                 &     (0.009)                 &     (0.013)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.075$^{\ast\ast\ast}$&       0.035$^{\ast\ast}$    &      -0.032                 &      -0.004                 &       0.000                 &       0.212                 &       0.003                 &      -0.008                 \\
            &     (0.023)                 &     (0.016)                 &     (0.022)                 &     (0.037)                 &     (0.003)                 &     (0.464)                 &     (0.005)                 &     (0.006)                 \\\midrule
$R^{2}$  &        .995                 &        .999                 &        .907                 &        .999                 &        .918                 &        .973                 &        .713                 &        .762                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/all_95_16/Results4shortRICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $Services_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016 (N=395)}}} \\\midrule
$R_{c,t}$ &      -0.128$^{\ast\ast\ast}$&      -0.006                 &      -0.088$^{\ast\ast\ast}$&      -0.056$^{\ast\ast}$    &      -0.941$^{\ast\ast\ast}$&       0.032$^{\ast\ast\ast}$\\
            &     (0.032)                 &     (0.016)                 &     (0.031)                 &     (0.026)                 &     (0.269)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t}$&       0.168$^{\ast\ast\ast}$&      -0.092$^{\ast\ast}$    &       0.077                 &      -0.006                 &       0.527                 &       0.038$^{\ast\ast\ast}$\\
            &     (0.049)                 &     (0.040)                 &     (0.047)                 &     (0.069)                 &     (1.008)                 &     (0.013)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.075$^{\ast\ast\ast}$&       0.035$^{\ast\ast}$    &      -0.032                 &      -0.004                 &       0.212                 &      -0.008                 \\
            &     (0.023)                 &     (0.016)                 &     (0.022)                 &     (0.037)                 &     (0.464)                 &     (0.006)                 \\%\midrule
%$R^{2}$  &        .995                 &        .999                 &        .907                 &        .999                 &        .973                 &        .762                 \\
%$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/all_95_16/Results5RICTint_ct_All_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.131$^{\ast\ast\ast}$&      -0.133$^{\ast\ast}$    &      -0.139$^{\ast\ast\ast}$&      -0.113$^{\ast\ast}$    &       0.009                 &      -0.099$^{\ast\ast\ast}$&      -0.006                 &      -0.004                 \\
            &     (0.039)                 &     (0.047)                 &     (0.042)                 &     (0.040)                 &     (0.029)                 &     (0.029)                 &     (0.019)                 &     (0.014)                 \\\addlinespace
$ICT_{c,t}$&       0.068                 &      -0.062                 &       0.015                 &       0.017                 &       0.026                 &      -0.019                 &       0.093$^{\ast\ast}$    &      -0.046                 \\
            &     (0.057)                 &     (0.058)                 &     (0.055)                 &     (0.049)                 &     (0.032)                 &     (0.044)                 &     (0.033)                 &     (0.030)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.033                 &       0.005                 &      -0.019                 &      -0.026                 &      -0.016                 &       0.016                 &      -0.049$^{\ast\ast}$    &       0.027$^{\ast\ast}$    \\
            &     (0.036)                 &     (0.035)                 &     (0.036)                 &     (0.035)                 &     (0.026)                 &     (0.021)                 &     (0.022)                 &     (0.012)                 \\\midrule
%$R^{2}$  &        .997                 &        .996                 &        .997                 &        .997                 &        .999                 &        .916                 &        .998                 &        .869                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         309                 &         309                 &         309                 &         309                 \\


==> inputs/all_subperiod/Results1RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.004                 &       0.012                 &       0.028                 &      -0.022                 &       0.520                 &       0.300                 &       0.262                 &      -0.041                 &       0.301                 &       0.426                 &      -0.699                 \\
            &     (0.020)                 &     (0.023)                 &     (0.059)                 &     (0.027)                 &     (0.807)                 &     (0.362)                 &     (0.540)                 &     (0.338)                 &     (0.787)                 &     (1.210)                 &     (0.940)                 \\\addlinespace
$ICT_{c,t}$&      -0.016                 &      -0.005                 &      -0.012                 &      -0.041                 &      -0.971                 &      -0.196                 &       0.112                 &      -0.886                 &      -0.205                 &       1.693$^{\ast}$        &      -1.520                 \\
            &     (0.034)                 &     (0.045)                 &     (0.028)                 &     (0.061)                 &     (0.838)                 &     (0.520)                 &     (0.235)                 &     (0.610)                 &     (0.911)                 &     (0.790)                 &     (0.887)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.006                 &       0.004                 &      -0.001                 &      -0.012                 &       0.112                 &      -0.099                 &       0.122                 &       0.089                 &       0.204                 &      -0.459                 &       0.221                 \\
            &     (0.023)                 &     (0.022)                 &     (0.039)                 &     (0.035)                 &     (0.857)                 &     (0.343)                 &     (0.573)                 &     (0.365)                 &     (0.530)                 &     (0.626)                 &     (0.415)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .983                 &        .994                 &        .989                 &        .949                 &        .991                 &        .987                 &        .966                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/all_subperiod/Results1RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.064$^{\ast\ast}$    &      -0.145$^{\ast}$        &      -0.121$^{\ast\ast\ast}$&      -0.010                 &      -0.916                 &      -0.294                 &      -0.872$^{\ast\ast}$    &       0.250                 &      -0.122                 &      -1.903$^{\ast\ast}$    &       1.189$^{\ast\ast}$    \\
            &     (0.022)                 &     (0.073)                 &     (0.034)                 &     (0.031)                 &     (0.635)                 &     (0.263)                 &     (0.380)                 &     (0.247)                 &     (0.507)                 &     (0.637)                 &     (0.536)                 \\\addlinespace
$ICT_{c,t}$&      -0.005                 &      -0.132                 &      -0.069                 &      -0.001                 &       0.804                 &       0.909$^{\ast\ast}$    &      -0.573                 &       0.468$^{\ast\ast}$    &       1.671$^{\ast}$        &      -2.274$^{\ast}$        &       0.250                 \\
            &     (0.025)                 &     (0.158)                 &     (0.052)                 &     (0.024)                 &     (0.709)                 &     (0.331)                 &     (0.633)                 &     (0.208)                 &     (0.800)                 &     (1.184)                 &     (0.569)                 \\\addlinespace
$R*ICT_{c,t}$&       0.003                 &       0.047                 &       0.010                 &       0.007                 &      -0.602                 &      -0.178                 &      -0.216                 &      -0.208$^{\ast}$        &       0.101                 &       0.250                 &      -0.002                 \\
            &     (0.019)                 &     (0.056)                 &     (0.033)                 &     (0.014)                 &     (0.638)                 &     (0.259)                 &     (0.424)                 &     (0.115)                 &     (0.327)                 &     (0.633)                 &     (0.536)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .975                 &        .986                 &        .983                 &        .943                 &         .99                 &        .985                 &        .964                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/all_subperiod/Results2RICTint_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.012                 &       0.015                 &       0.016                 &      -0.058                 &       0.210                 &       0.233                 &       0.196                 &      -0.220                 &       0.479                 &       0.439                 &      -0.901                 \\
            &     (0.023)                 &     (0.025)                 &     (0.059)                 &     (0.034)                 &     (0.758)                 &     (0.405)                 &     (0.539)                 &     (0.238)                 &     (0.925)                 &     (0.956)                 &     (0.776)                 \\\addlinespace
$ICT_{c,t}$&       0.019                 &      -0.007                 &       0.017                 &       0.026                 &       0.280                 &      -0.118                 &       0.137                 &       0.261$^{\ast\ast\ast}$&      -1.274                 &       0.519                 &       0.731                 \\
            &     (0.036)                 &     (0.050)                 &     (0.034)                 &     (0.056)                 &     (0.466)                 &     (0.623)                 &     (0.318)                 &     (0.058)                 &     (1.056)                 &     (0.753)                 &     (0.657)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.020                 &      -0.000                 &      -0.016                 &      -0.035                 &      -0.149                 &      -0.131                 &       0.098                 &      -0.117                 &       0.399                 &      -0.302                 &      -0.135                 \\
            &     (0.024)                 &     (0.031)                 &     (0.039)                 &     (0.033)                 &     (0.647)                 &     (0.376)                 &     (0.605)                 &     (0.095)                 &     (0.595)                 &     (0.736)                 &     (0.535)                 \\\addlinespace
$wL_{c,t}$&       0.403$^{\ast\ast\ast}$&       0.339                 &       0.539$^{\ast}$        &       0.375$^{\ast\ast\ast}$&      -0.662$^{\ast\ast\ast}$&       0.039                 &       0.087                 &      -0.788$^{\ast\ast\ast}$&       0.715$^{\ast}$        &       1.091$^{\ast}$        &      -1.795$^{\ast\ast\ast}$\\
            &     (0.075)                 &     (0.193)                 &     (0.284)                 &     (0.094)                 &     (0.182)                 &     (0.070)                 &     (0.232)                 &     (0.085)                 &     (0.342)                 &     (0.572)                 &     (0.343)                 \\\addlinespace
$rK_{c,t}$&       0.017                 &       0.235                 &       0.146                 &      -0.242$^{\ast\ast}$    &      -0.718$^{\ast\ast\ast}$&       0.013                 &       0.058                 &      -0.789$^{\ast\ast\ast}$&       0.722$^{\ast\ast}$    &       1.013$^{\ast\ast}$    &      -1.728$^{\ast\ast\ast}$\\
            &     (0.064)                 &     (0.130)                 &     (0.151)                 &     (0.075)                 &     (0.146)                 &     (0.032)                 &     (0.181)                 &     (0.089)                 &     (0.253)                 &     (0.412)                 &     (0.306)                 \\\addlinespace
$pQ_{c,t}$&       0.204                 &       0.099                 &       0.202                 &       0.248$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.122)                 &     (0.351)                 &     (0.327)                 &     (0.128)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.000                 &      -0.003                 &       0.000                 &       0.004$^{\ast\ast}$    &      -0.084                 &      -0.048                 &      -0.024                 &      -0.012                 &      -0.077                 &       0.041                 &       0.031                 \\
            &     (0.002)                 &     (0.003)                 &     (0.004)                 &     (0.002)                 &     (0.059)                 &     (0.032)                 &     (0.031)                 &     (0.007)                 &     (0.063)                 &     (0.082)                 &     (0.049)                 \\\addlinespace
$Services_{c,t}$&      -0.000                 &       0.019$^{\ast\ast}$    &       0.009                 &      -0.021$^{\ast\ast}$    &       0.219                 &       0.127$^{\ast}$        &       0.112                 &      -0.020                 &       0.200                 &       0.037                 &      -0.252                 \\
            &     (0.005)                 &     (0.007)                 &     (0.013)                 &     (0.008)                 &     (0.188)                 &     (0.066)                 &     (0.153)                 &     (0.047)                 &     (0.234)                 &     (0.294)                 &     (0.161)                 \\\addlinespace
$HHI_{c,t}$&      -0.850                 &       1.508                 &      -0.386                 &      -3.682$^{\ast\ast}$    &      16.968                 &      14.520                 &      -2.496                 &       4.943                 &      16.206                 &     -22.266                 &       3.475                 \\
            &     (0.705)                 &     (1.067)                 &     (2.189)                 &     (1.346)                 &    (22.773)                 &    (13.039)                 &    (17.292)                 &     (9.459)                 &    (36.421)                 &    (49.622)                 &    (34.892)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast}$        &       0.001                 &      -0.001                 &       0.045$^{\ast\ast}$    &      -0.003                 &       0.022                 &       0.026$^{\ast\ast\ast}$&      -0.042                 &       0.023                 &       0.022                 \\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.001)                 &     (0.014)                 &     (0.008)                 &     (0.013)                 &     (0.007)                 &     (0.027)                 &     (0.032)                 &     (0.015)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.012                 &       0.020$^{\ast}$        &      -0.036                 &       0.041$^{\ast\ast\ast}$&      -0.797$^{\ast\ast}$    &      -0.051                 &      -0.409$^{\ast\ast}$    &      -0.336$^{\ast\ast}$    &       0.644$^{\ast\ast}$    &      -0.561                 &      -0.133                 \\
            &     (0.008)                 &     (0.010)                 &     (0.036)                 &     (0.011)                 &     (0.274)                 &     (0.075)                 &     (0.161)                 &     (0.130)                 &     (0.231)                 &     (0.371)                 &     (0.325)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003$^{\ast\ast}$    &       0.001                 &       0.008$^{\ast\ast}$    &       0.001                 &       0.092$^{\ast}$        &       0.011                 &       0.074$^{\ast\ast}$    &       0.007                 &      -0.050                 &       0.130$^{\ast\ast}$    &      -0.088$^{\ast}$        \\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.002)                 &     (0.042)                 &     (0.013)                 &     (0.030)                 &     (0.012)                 &     (0.030)                 &     (0.046)                 &     (0.041)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.004                 &       0.023$^{\ast}$        &      -0.003                 &      -0.004                 &       0.132                 &       0.111                 &       0.086                 &      -0.064                 &       0.366                 &      -0.074                 &      -0.280                 \\
            &     (0.005)                 &     (0.012)                 &     (0.016)                 &     (0.009)                 &     (0.193)                 &     (0.092)                 &     (0.153)                 &     (0.045)                 &     (0.224)                 &     (0.255)                 &     (0.258)                 \\\addlinespace
$XRate_{c,t}$&       0.008                 &      -0.004                 &       0.014                 &       0.020$^{\ast\ast}$    &       0.027                 &      -0.042                 &       0.052                 &       0.017                 &      -0.247                 &       0.292                 &      -0.046                 \\
            &     (0.007)                 &     (0.011)                 &     (0.013)                 &     (0.008)                 &     (0.246)                 &     (0.108)                 &     (0.227)                 &     (0.050)                 &     (0.205)                 &     (0.302)                 &     (0.197)                 \\\midrule
%$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .986                 &        .994                 &        .989                 &        .984                 &        .992                 &        .989                 &        .982                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/all_subperiod/Results2RICTint_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.040$^{\ast}$        &      -0.078                 &      -0.108$^{\ast\ast\ast}$&       0.020                 &      -0.683$^{\ast}$        &      -0.223                 &      -0.830$^{\ast\ast}$    &       0.370$^{\ast\ast}$    &      -0.104                 &      -1.984$^{\ast\ast}$    &       1.315$^{\ast\ast}$    \\
            &     (0.021)                 &     (0.049)                 &     (0.031)                 &     (0.032)                 &     (0.382)                 &     (0.185)                 &     (0.377)                 &     (0.132)                 &     (0.480)                 &     (0.730)                 &     (0.459)                 \\\addlinespace
$ICT_{c,t}$&      -0.042                 &      -0.163                 &      -0.110$^{\ast}$        &      -0.008                 &      -0.856                 &       0.275                 &      -1.269                 &       0.138                 &       0.967                 &      -2.616                 &       0.873                 \\
            &     (0.027)                 &     (0.123)                 &     (0.057)                 &     (0.028)                 &     (0.701)                 &     (0.468)                 &     (0.760)                 &     (0.187)                 &     (1.024)                 &     (1.510)                 &     (0.997)                 \\\addlinespace
$R*ICT_{c,t}$&       0.008                 &       0.036                 &       0.019                 &       0.000                 &       0.083                 &       0.053                 &      -0.025                 &       0.054                 &       0.254                 &       0.170                 &       0.107                 \\
            &     (0.017)                 &     (0.045)                 &     (0.031)                 &     (0.016)                 &     (0.567)                 &     (0.267)                 &     (0.415)                 &     (0.092)                 &     (0.423)                 &     (0.681)                 &     (0.624)                 \\\addlinespace
$wL_{c,t}$&       0.540$^{\ast\ast}$    &       1.383$^{\ast\ast}$    &       0.331                 &       0.593$^{\ast\ast\ast}$&      -0.588$^{\ast\ast}$    &      -0.129                 &       0.058                 &      -0.517$^{\ast\ast\ast}$&       0.187                 &       0.578$^{\ast}$        &      -0.940$^{\ast\ast\ast}$\\
            &     (0.213)                 &     (0.495)                 &     (0.302)                 &     (0.137)                 &     (0.223)                 &     (0.138)                 &     (0.165)                 &     (0.088)                 &     (0.262)                 &     (0.314)                 &     (0.287)                 \\\addlinespace
$rK_{c,t}$&      -0.032                 &       0.288                 &      -0.120                 &       0.162                 &      -0.887$^{\ast\ast\ast}$&      -0.249$^{\ast}$        &      -0.086                 &      -0.552$^{\ast\ast\ast}$&       0.033                 &       0.474$^{\ast}$        &      -0.757$^{\ast\ast}$    \\
            &     (0.129)                 &     (0.343)                 &     (0.158)                 &     (0.110)                 &     (0.232)                 &     (0.138)                 &     (0.153)                 &     (0.070)                 &     (0.258)                 &     (0.262)                 &     (0.286)                 \\\addlinespace
$pQ_{c,t}$&       0.485                 &      -0.671                 &       0.726$^{\ast}$        &       0.290                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.304)                 &     (0.801)                 &     (0.385)                 &     (0.213)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.007                 &      -0.002                 &       0.004                 &       0.001                 &      -0.063                 &       0.008                 &       0.056$^{\ast}$        &      -0.155                 &      -0.049                 &       0.180$^{\ast}$        \\
            &     (0.002)                 &     (0.004)                 &     (0.003)                 &     (0.003)                 &     (0.049)                 &     (0.038)                 &     (0.033)                 &     (0.027)                 &     (0.092)                 &     (0.078)                 &     (0.089)                 \\\addlinespace
$Services_{c,t}$&       0.001                 &      -0.024                 &      -0.014                 &      -0.001                 &      -0.088                 &       0.146                 &      -0.231$^{\ast}$        &      -0.002                 &       0.574$^{\ast\ast}$    &      -0.594$^{\ast\ast}$    &      -0.016                 \\
            &     (0.004)                 &     (0.028)                 &     (0.009)                 &     (0.005)                 &     (0.142)                 &     (0.104)                 &     (0.119)                 &     (0.028)                 &     (0.200)                 &     (0.254)                 &     (0.140)                 \\\addlinespace
$HHI_{c,t}$&      -1.002                 &      -1.847                 &      -2.840$^{\ast\ast\ast}$&      -1.663                 &     -46.114                 &      14.996                 &     -44.451$^{\ast\ast}$    &     -16.658$^{\ast}$        &      90.039$^{\ast\ast}$    &     -69.920$^{\ast\ast}$    &      -5.931                 \\
            &     (0.694)                 &     (2.807)                 &     (0.842)                 &     (0.960)                 &    (31.257)                 &    (20.870)                 &    (14.942)                 &     (7.923)                 &    (33.816)                 &    (23.348)                 &    (39.046)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001                 &       0.004$^{\ast}$        &       0.002                 &      -0.000                 &       0.035$^{\ast}$        &       0.015                 &       0.015                 &       0.006                 &       0.008                 &       0.009                 &      -0.029                 \\
            &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.001)                 &     (0.018)                 &     (0.011)                 &     (0.015)                 &     (0.008)                 &     (0.025)                 &     (0.033)                 &     (0.031)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.004                 &      -0.006                 &       0.002                 &      -0.007$^{\ast}$        &       0.154                 &      -0.077                 &       0.199                 &       0.032                 &      -0.152                 &       0.464                 &       0.250                 \\
            &     (0.007)                 &     (0.012)                 &     (0.010)                 &     (0.004)                 &     (0.179)                 &     (0.134)                 &     (0.114)                 &     (0.066)                 &     (0.308)                 &     (0.290)                 &     (0.279)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.004                 &      -0.005                 &       0.007                 &       0.000                 &       0.136                 &       0.020                 &       0.099                 &       0.017                 &      -0.026                 &       0.094                 &      -0.081                 \\
            &     (0.003)                 &     (0.006)                 &     (0.006)                 &     (0.002)                 &     (0.079)                 &     (0.033)                 &     (0.072)                 &     (0.012)                 &     (0.081)                 &     (0.123)                 &     (0.068)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.005                 &      -0.019                 &       0.014                 &      -0.018$^{\ast}$        &      -0.063                 &       0.039                 &      -0.002                 &      -0.100                 &      -0.080                 &       0.245                 &      -0.330                 \\
            &     (0.008)                 &     (0.011)                 &     (0.012)                 &     (0.009)                 &     (0.201)                 &     (0.125)                 &     (0.161)                 &     (0.069)                 &     (0.261)                 &     (0.316)                 &     (0.300)                 \\\addlinespace
$XRate_{c,t}$&      -0.005$^{\ast\ast\ast}$&      -0.007                 &      -0.010$^{\ast\ast}$    &      -0.005$^{\ast\ast}$    &      -0.121$^{\ast\ast}$    &       0.003                 &      -0.117$^{\ast\ast}$    &      -0.008                 &       0.156$^{\ast}$        &      -0.207$^{\ast\ast}$    &       0.095$^{\ast\ast}$    \\
            &     (0.001)                 &     (0.006)                 &     (0.003)                 &     (0.002)                 &     (0.048)                 &     (0.033)                 &     (0.045)                 &     (0.011)                 &     (0.080)                 &     (0.083)                 &     (0.037)                 \\\midrule
%$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .982                 &        .988                 &        .984                 &        .972                 &         .99                 &        .986                 &        .969                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/all_subperiod/Results2shortEXCGDPV1_RICTint_ct_All_08t16.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.012                 &       0.015                 &       0.016                 &      -0.058                 &       0.479                 &       0.439                 &      -0.901                 \\
            &     (0.023)                 &     (0.025)                 &     (0.059)                 &     (0.034)                 &     (0.925)                 &     (0.956)                 &     (0.776)                 \\\addlinespace
$ICT_{c,t}$&       0.019                 &      -0.007                 &       0.017                 &       0.026                 &      -1.274                 &       0.519                 &       0.731                 \\
            &     (0.036)                 &     (0.050)                 &     (0.034)                 &     (0.056)                 &     (1.056)                 &     (0.753)                 &     (0.657)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.020                 &      -0.000                 &      -0.016                 &      -0.035                 &       0.399                 &      -0.302                 &      -0.135                 \\
            &     (0.024)                 &     (0.031)                 &     (0.039)                 &     (0.033)                 &     (0.595)                 &     (0.736)                 &     (0.535)                 \\\addlinespace
$wL_{c,t}$&       0.403$^{\ast\ast\ast}$&       0.339                 &       0.539$^{\ast}$        &       0.375$^{\ast\ast\ast}$&       0.715$^{\ast}$        &       1.091$^{\ast}$        &      -1.795$^{\ast\ast\ast}$\\
            &     (0.075)                 &     (0.193)                 &     (0.284)                 &     (0.094)                 &     (0.342)                 &     (0.572)                 &     (0.343)                 \\\addlinespace
$rK_{c,t}$&       0.017                 &       0.235                 &       0.146                 &      -0.242$^{\ast\ast}$    &       0.722$^{\ast\ast}$    &       1.013$^{\ast\ast}$    &      -1.728$^{\ast\ast\ast}$\\
            &     (0.064)                 &     (0.130)                 &     (0.151)                 &     (0.075)                 &     (0.253)                 &     (0.412)                 &     (0.306)                 \\\addlinespace
$pQ_{c,t}$&       0.204                 &       0.099                 &       0.202                 &       0.248$^{\ast}$        &                             &                             &                             \\
            &     (0.122)                 &     (0.351)                 &     (0.327)                 &     (0.128)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .992                 &        .989                 &        .982                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/all_subperiod/Results2shortEXCGDPV1_RICTint_ct_All_95t07.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.040$^{\ast}$        &      -0.078                 &      -0.108$^{\ast\ast\ast}$&       0.020                 &      -0.104                 &      -1.984$^{\ast\ast}$    &       1.315$^{\ast\ast}$    \\
            &     (0.021)                 &     (0.049)                 &     (0.031)                 &     (0.032)                 &     (0.480)                 &     (0.730)                 &     (0.459)                 \\\addlinespace
$ICT_{c,t}$&      -0.042                 &      -0.163                 &      -0.110$^{\ast}$        &      -0.008                 &       0.967                 &      -2.616                 &       0.873                 \\
            &     (0.027)                 &     (0.123)                 &     (0.057)                 &     (0.028)                 &     (1.024)                 &     (1.510)                 &     (0.997)                 \\\addlinespace
$R*ICT_{c,t}$&       0.008                 &       0.036                 &       0.019                 &       0.000                 &       0.254                 &       0.170                 &       0.107                 \\
            &     (0.017)                 &     (0.045)                 &     (0.031)                 &     (0.016)                 &     (0.423)                 &     (0.681)                 &     (0.624)                 \\\addlinespace
$wL_{c,t}$&       0.540$^{\ast\ast}$    &       1.383$^{\ast\ast}$    &       0.331                 &       0.593$^{\ast\ast\ast}$&       0.187                 &       0.578$^{\ast}$        &      -0.940$^{\ast\ast\ast}$\\
            &     (0.213)                 &     (0.495)                 &     (0.302)                 &     (0.137)                 &     (0.262)                 &     (0.314)                 &     (0.287)                 \\\addlinespace
$rK_{c,t}$&      -0.032                 &       0.288                 &      -0.120                 &       0.162                 &       0.033                 &       0.474$^{\ast}$        &      -0.757$^{\ast\ast}$    \\
            &     (0.129)                 &     (0.343)                 &     (0.158)                 &     (0.110)                 &     (0.258)                 &     (0.262)                 &     (0.286)                 \\\addlinespace
$pQ_{c,t}$&       0.485                 &      -0.671                 &       0.726$^{\ast}$        &       0.290                 &                             &                             &                             \\
            &     (0.304)                 &     (0.801)                 &     (0.385)                 &     (0.213)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &         .99                 &        .986                 &        .969                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/all_subperiod/Results2shortEXCGDPV2_RICTint_ct_All_08t16.tex <==
\multicolumn{4}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.479                 &       0.439                 &      -0.901                 \\
            &     (0.925)                 &     (0.956)                 &     (0.776)                 \\\addlinespace
$ICT_{c,t}$&      -1.274                 &       0.519                 &       0.731                 \\
            &     (1.056)                 &     (0.753)                 &     (0.657)                 \\\addlinespace
$R*ICT_{c,t}$&       0.399                 &      -0.302                 &      -0.135                 \\
            &     (0.595)                 &     (0.736)                 &     (0.535)                 \\\addlinespace
$wL_{c,t}$&       0.715$^{\ast}$        &       1.091$^{\ast}$        &      -1.795$^{\ast\ast\ast}$\\
            &     (0.342)                 &     (0.572)                 &     (0.343)                 \\\addlinespace
$rK_{c,t}$&       0.722$^{\ast\ast}$    &       1.013$^{\ast\ast}$    &      -1.728$^{\ast\ast\ast}$\\
            &     (0.253)                 &     (0.412)                 &     (0.306)                 \\\midrule
$R^{2}$  &        .992                 &        .989                 &        .982                 \\
$N$      &         171                 &         171                 &         171                 \\


==> inputs/all_subperiod/Results2shortEXCGDPV2_RICTint_ct_All_95t07.tex <==
\multicolumn{4}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.104                 &      -1.984$^{\ast\ast}$    &       1.315$^{\ast\ast}$    \\
            &     (0.480)                 &     (0.730)                 &     (0.459)                 \\\addlinespace
$ICT_{c,t}$&       0.967                 &      -2.616                 &       0.873                 \\
            &     (1.024)                 &     (1.510)                 &     (0.997)                 \\\addlinespace
$R*ICT_{c,t}$&       0.254                 &       0.170                 &       0.107                 \\
            &     (0.423)                 &     (0.681)                 &     (0.624)                 \\\addlinespace
$wL_{c,t}$&       0.187                 &       0.578$^{\ast}$        &      -0.940$^{\ast\ast\ast}$\\
            &     (0.262)                 &     (0.314)                 &     (0.287)                 \\\addlinespace
$rK_{c,t}$&       0.033                 &       0.474$^{\ast}$        &      -0.757$^{\ast\ast}$    \\
            &     (0.258)                 &     (0.262)                 &     (0.286)                 \\\midrule
$R^{2}$  &         .99                 &        .986                 &        .969                 \\
$N$      &         224                 &         224                 &         224                 \\


==> inputs/all_subperiod/Results2shortV1_RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016 (N = 171)}}} \\\midrule
$R_{c,t}$ &      -0.012                 &       0.015                 &       0.016                 &      -0.058                 &       0.210                 &       0.233                 &       0.196                 &      -0.220                 &       0.479                 &       0.439                 &      -0.901                 \\
            &     (0.023)                 &     (0.025)                 &     (0.059)                 &     (0.034)                 &     (0.758)                 &     (0.405)                 &     (0.539)                 &     (0.238)                 &     (0.925)                 &     (0.956)                 &     (0.776)                 \\\addlinespace
$ICT_{c,t}$&       0.019                 &      -0.007                 &       0.017                 &       0.026                 &       0.280                 &      -0.118                 &       0.137                 &       0.261$^{\ast\ast\ast}$&      -1.274                 &       0.519                 &       0.731                 \\
            &     (0.036)                 &     (0.050)                 &     (0.034)                 &     (0.056)                 &     (0.466)                 &     (0.623)                 &     (0.318)                 &     (0.058)                 &     (1.056)                 &     (0.753)                 &     (0.657)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.020                 &      -0.000                 &      -0.016                 &      -0.035                 &      -0.149                 &      -0.131                 &       0.098                 &      -0.117                 &       0.399                 &      -0.302                 &      -0.135                 \\
            &     (0.024)                 &     (0.031)                 &     (0.039)                 &     (0.033)                 &     (0.647)                 &     (0.376)                 &     (0.605)                 &     (0.095)                 &     (0.595)                 &     (0.736)                 &     (0.535)                 \\\addlinespace
$wL_{c,t}$&       0.403$^{\ast\ast\ast}$&       0.339                 &       0.539$^{\ast}$        &       0.375$^{\ast\ast\ast}$&      -0.662$^{\ast\ast\ast}$&       0.039                 &       0.087                 &      -0.788$^{\ast\ast\ast}$&       0.715$^{\ast}$        &       1.091$^{\ast}$        &      -1.795$^{\ast\ast\ast}$\\
            &     (0.075)                 &     (0.193)                 &     (0.284)                 &     (0.094)                 &     (0.182)                 &     (0.070)                 &     (0.232)                 &     (0.085)                 &     (0.342)                 &     (0.572)                 &     (0.343)                 \\\addlinespace
$rK_{c,t}$&       0.017                 &       0.235                 &       0.146                 &      -0.242$^{\ast\ast}$    &      -0.718$^{\ast\ast\ast}$&       0.013                 &       0.058                 &      -0.789$^{\ast\ast\ast}$&       0.722$^{\ast\ast}$    &       1.013$^{\ast\ast}$    &      -1.728$^{\ast\ast\ast}$\\
            &     (0.064)                 &     (0.130)                 &     (0.151)                 &     (0.075)                 &     (0.146)                 &     (0.032)                 &     (0.181)                 &     (0.089)                 &     (0.253)                 &     (0.412)                 &     (0.306)                 \\\addlinespace
$pQ_{c,t}$&       0.204                 &       0.099                 &       0.202                 &       0.248$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.122)                 &     (0.351)                 &     (0.327)                 &     (0.128)                 &                             &                             &                             &                             &                             &                             &                             \\%\midrule
%$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .986                 &        .994                 &        .989                 &        .984                 &        .992                 &        .989                 &        .982                 \\
%$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/all_subperiod/Results2shortV1_RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007 (N = 224)}}} \\\midrule
$R_{c,t}$ &      -0.040$^{\ast}$        &      -0.078                 &      -0.108$^{\ast\ast\ast}$&       0.020                 &      -0.683$^{\ast}$        &      -0.223                 &      -0.830$^{\ast\ast}$    &       0.370$^{\ast\ast}$    &      -0.104                 &      -1.984$^{\ast\ast}$    &       1.315$^{\ast\ast}$    \\
            &     (0.021)                 &     (0.049)                 &     (0.031)                 &     (0.032)                 &     (0.382)                 &     (0.185)                 &     (0.377)                 &     (0.132)                 &     (0.480)                 &     (0.730)                 &     (0.459)                 \\\addlinespace
$ICT_{c,t}$&      -0.042                 &      -0.163                 &      -0.110$^{\ast}$        &      -0.008                 &      -0.856                 &       0.275                 &      -1.269                 &       0.138                 &       0.967                 &      -2.616                 &       0.873                 \\
            &     (0.027)                 &     (0.123)                 &     (0.057)                 &     (0.028)                 &     (0.701)                 &     (0.468)                 &     (0.760)                 &     (0.187)                 &     (1.024)                 &     (1.510)                 &     (0.997)                 \\\addlinespace
$R*ICT_{c,t}$&       0.008                 &       0.036                 &       0.019                 &       0.000                 &       0.083                 &       0.053                 &      -0.025                 &       0.054                 &       0.254                 &       0.170                 &       0.107                 \\
            &     (0.017)                 &     (0.045)                 &     (0.031)                 &     (0.016)                 &     (0.567)                 &     (0.267)                 &     (0.415)                 &     (0.092)                 &     (0.423)                 &     (0.681)                 &     (0.624)                 \\\addlinespace
$wL_{c,t}$&       0.540$^{\ast\ast}$    &       1.383$^{\ast\ast}$    &       0.331                 &       0.593$^{\ast\ast\ast}$&      -0.588$^{\ast\ast}$    &      -0.129                 &       0.058                 &      -0.517$^{\ast\ast\ast}$&       0.187                 &       0.578$^{\ast}$        &      -0.940$^{\ast\ast\ast}$\\
            &     (0.213)                 &     (0.495)                 &     (0.302)                 &     (0.137)                 &     (0.223)                 &     (0.138)                 &     (0.165)                 &     (0.088)                 &     (0.262)                 &     (0.314)                 &     (0.287)                 \\\addlinespace
$rK_{c,t}$&      -0.032                 &       0.288                 &      -0.120                 &       0.162                 &      -0.887$^{\ast\ast\ast}$&      -0.249$^{\ast}$        &      -0.086                 &      -0.552$^{\ast\ast\ast}$&       0.033                 &       0.474$^{\ast}$        &      -0.757$^{\ast\ast}$    \\
            &     (0.129)                 &     (0.343)                 &     (0.158)                 &     (0.110)                 &     (0.232)                 &     (0.138)                 &     (0.153)                 &     (0.070)                 &     (0.258)                 &     (0.262)                 &     (0.286)                 \\\addlinespace
$pQ_{c,t}$&       0.485                 &      -0.671                 &       0.726$^{\ast}$        &       0.290                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.304)                 &     (0.801)                 &     (0.385)                 &     (0.213)                 &                             &                             &                             &                             &                             &                             &                             \\%\midrule
%$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .982                 &        .988                 &        .984                 &        .972                 &         .99                 &        .986                 &        .969                 \\
%$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/all_subperiod/Results2shortV2_RICTint_ct_All_08t16.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.210                 &       0.233                 &       0.196                 &      -0.220                 &       0.479                 &       0.439                 &      -0.901                 \\
            &     (0.758)                 &     (0.405)                 &     (0.539)                 &     (0.238)                 &     (0.925)                 &     (0.956)                 &     (0.776)                 \\\addlinespace
$ICT_{c,t}$&       0.280                 &      -0.118                 &       0.137                 &       0.261$^{\ast\ast\ast}$&      -1.274                 &       0.519                 &       0.731                 \\
            &     (0.466)                 &     (0.623)                 &     (0.318)                 &     (0.058)                 &     (1.056)                 &     (0.753)                 &     (0.657)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.149                 &      -0.131                 &       0.098                 &      -0.117                 &       0.399                 &      -0.302                 &      -0.135                 \\
            &     (0.647)                 &     (0.376)                 &     (0.605)                 &     (0.095)                 &     (0.595)                 &     (0.736)                 &     (0.535)                 \\\addlinespace
$wL_{c,t}$&      -0.662$^{\ast\ast\ast}$&       0.039                 &       0.087                 &      -0.788$^{\ast\ast\ast}$&       0.715$^{\ast}$        &       1.091$^{\ast}$        &      -1.795$^{\ast\ast\ast}$\\
            &     (0.182)                 &     (0.070)                 &     (0.232)                 &     (0.085)                 &     (0.342)                 &     (0.572)                 &     (0.343)                 \\\addlinespace
$rK_{c,t}$&      -0.718$^{\ast\ast\ast}$&       0.013                 &       0.058                 &      -0.789$^{\ast\ast\ast}$&       0.722$^{\ast\ast}$    &       1.013$^{\ast\ast}$    &      -1.728$^{\ast\ast\ast}$\\
            &     (0.146)                 &     (0.032)                 &     (0.181)                 &     (0.089)                 &     (0.253)                 &     (0.412)                 &     (0.306)                 \\\midrule
$R^{2}$  &        .986                 &        .994                 &        .989                 &        .984                 &        .992                 &        .989                 &        .982                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/all_subperiod/Results2shortV2_RICTint_ct_All_95t07.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.683$^{\ast}$        &      -0.223                 &      -0.830$^{\ast\ast}$    &       0.370$^{\ast\ast}$    &      -0.104                 &      -1.984$^{\ast\ast}$    &       1.315$^{\ast\ast}$    \\
            &     (0.382)                 &     (0.185)                 &     (0.377)                 &     (0.132)                 &     (0.480)                 &     (0.730)                 &     (0.459)                 \\\addlinespace
$ICT_{c,t}$&      -0.856                 &       0.275                 &      -1.269                 &       0.138                 &       0.967                 &      -2.616                 &       0.873                 \\
            &     (0.701)                 &     (0.468)                 &     (0.760)                 &     (0.187)                 &     (1.024)                 &     (1.510)                 &     (0.997)                 \\\addlinespace
$R*ICT_{c,t}$&       0.083                 &       0.053                 &      -0.025                 &       0.054                 &       0.254                 &       0.170                 &       0.107                 \\
            &     (0.567)                 &     (0.267)                 &     (0.415)                 &     (0.092)                 &     (0.423)                 &     (0.681)                 &     (0.624)                 \\\addlinespace
$wL_{c,t}$&      -0.588$^{\ast\ast}$    &      -0.129                 &       0.058                 &      -0.517$^{\ast\ast\ast}$&       0.187                 &       0.578$^{\ast}$        &      -0.940$^{\ast\ast\ast}$\\
            &     (0.223)                 &     (0.138)                 &     (0.165)                 &     (0.088)                 &     (0.262)                 &     (0.314)                 &     (0.287)                 \\\addlinespace
$rK_{c,t}$&      -0.887$^{\ast\ast\ast}$&      -0.249$^{\ast}$        &      -0.086                 &      -0.552$^{\ast\ast\ast}$&       0.033                 &       0.474$^{\ast}$        &      -0.757$^{\ast\ast}$    \\
            &     (0.232)                 &     (0.138)                 &     (0.153)                 &     (0.070)                 &     (0.258)                 &     (0.262)                 &     (0.286)                 \\\midrule
$R^{2}$  &        .982                 &        .988                 &        .984                 &        .972                 &         .99                 &        .986                 &        .969                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/all_subperiod/Results3RICTint_cit_All_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{i,c,t}$&      -0.034                 &       0.013                 &      -0.047$^{\ast}$        &      -0.021                 &      -0.004                 &      -0.021                 \\
            &     (0.027)                 &     (0.012)                 &     (0.023)                 &     (0.043)                 &     (0.004)                 &     (0.020)                 \\\addlinespace
$ICT_{i,c,t}$&      -0.033                 &       0.016                 &      -0.049                 &      -0.100                 &      -0.006                 &      -0.036                 \\
            &     (0.027)                 &     (0.010)                 &     (0.027)                 &     (0.095)                 &     (0.005)                 &     (0.053)                 \\\addlinespace
$R*ICT_{i,c,t}$&      -0.012                 &       0.000                 &      -0.012                 &       0.028                 &      -0.003$^{\ast}$        &       0.011                 \\
            &     (0.010)                 &     (0.004)                 &     (0.009)                 &     (0.020)                 &     (0.002)                 &     (0.009)                 \\\midrule
%$R^{2}$  &        .999                 &        .998                 &        .998                 &        .985                 &        .918                 &        .999                 \\
$N$      &        2070                 &        2070                 &        2070                 &        2052                 &        2025                 &        2025                 \\


==> inputs/all_subperiod/Results3RICTint_cit_All_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{i,c,t}$&      -0.006                 &       0.016$^{\ast}$        &      -0.022                 &       0.005                 &      -0.002                 &       0.020                 \\
            &     (0.028)                 &     (0.008)                 &     (0.027)                 &     (0.050)                 &     (0.005)                 &     (0.021)                 \\\addlinespace
$ICT_{i,c,t}$&       0.026$^{\ast\ast}$    &       0.005                 &       0.021$^{\ast}$        &       0.001                 &       0.001                 &       0.029                 \\
            &     (0.010)                 &     (0.005)                 &     (0.010)                 &     (0.027)                 &     (0.010)                 &     (0.017)                 \\\addlinespace
$R*ICT_{i,c,t}$&       0.002                 &       0.001                 &       0.001                 &      -0.003                 &      -0.000                 &       0.008                 \\
            &     (0.005)                 &     (0.002)                 &     (0.005)                 &     (0.015)                 &     (0.003)                 &     (0.008)                 \\\midrule
%$R^{2}$  &        .998                 &        .997                 &        .996                 &        .975                 &         .94                 &        .998                 \\
$N$      &        2827                 &        2827                 &        2827                 &        2790                 &        2777                 &        2777                 \\


==> inputs/all_subperiod/Results4RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.034                 &       0.018                 &      -0.039                 &      -0.004                 &       0.014$^{\ast\ast}$    &      -1.635$^{\ast\ast}$    &       0.004                 &       0.009$^{\ast}$        \\
            &     (0.027)                 &     (0.019)                 &     (0.028)                 &     (0.023)                 &     (0.005)                 &     (0.562)                 &     (0.005)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.011                 &       0.008                 &       0.046                 &       0.100$^{\ast}$        &      -0.011$^{\ast\ast}$    &       2.054                 &      -0.000                 &       0.006                 \\
            &     (0.018)                 &     (0.035)                 &     (0.036)                 &     (0.047)                 &     (0.004)                 &     (1.161)                 &     (0.006)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.032$^{\ast\ast}$    &       0.002                 &      -0.036                 &      -0.038                 &       0.004                 &      -0.467                 &      -0.001                 &       0.008                 \\
            &     (0.013)                 &     (0.021)                 &     (0.024)                 &     (0.034)                 &     (0.003)                 &     (0.726)                 &     (0.003)                 &     (0.005)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .822                 &          0.999                &        .967                 &        .988                 &        .936                 &        .948                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/all_subperiod/Results4RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.145$^{\ast\ast\ast}$&      -0.040                 &      -0.084$^{\ast\ast}$    &      -0.065$^{\ast\ast}$    &       0.002                 &      -1.539$^{\ast\ast\ast}$&      -0.010                 &       0.011                 \\
            &     (0.040)                 &     (0.023)                 &     (0.029)                 &     (0.026)                 &     (0.005)                 &     (0.497)                 &     (0.007)                 &     (0.011)                 \\\addlinespace
$ICT_{c,t}$&       0.301$^{\ast\ast\ast}$&      -0.142$^{\ast\ast\ast}$&       0.141$^{\ast\ast\ast}$&      -0.049$^{\ast}$        &       0.016$^{\ast\ast\ast}$&      -2.427$^{\ast\ast}$    &      -0.007                 &       0.018                 \\
            &     (0.052)                 &     (0.023)                 &     (0.040)                 &     (0.024)                 &     (0.005)                 &     (1.107)                 &     (0.013)                 &     (0.017)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.141$^{\ast\ast\ast}$&       0.040$^{\ast\ast\ast}$&      -0.065$^{\ast\ast}$    &       0.017                 &      -0.009$^{\ast\ast}$    &       1.215$^{\ast}$        &      -0.001                 &      -0.006                 \\
            &     (0.032)                 &     (0.011)                 &     (0.023)                 &     (0.015)                 &     (0.003)                 &     (0.607)                 &     (0.006)                 &     (0.010)                 \\\midrule
$R^{2}$  &        .998                 &        .999                 &        .923                 &          0.999                &        .958                 &         .98                 &        .781                 &        .878                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/all_subperiod/Results4shortRICTint_ct_All_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016 (N=171)}}} \\\midrule
$R_{c,t}$ &      -0.034                 &       0.018                 &      -0.039                 &      -0.004                 &      -1.635$^{\ast\ast}$    &       0.009$^{\ast}$        \\
            &     (0.027)                 &     (0.019)                 &     (0.028)                 &     (0.023)                 &     (0.562)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.011                 &       0.008                 &       0.046                 &       0.100$^{\ast}$        &       2.054                 &       0.006                 \\
            &     (0.018)                 &     (0.035)                 &     (0.036)                 &     (0.047)                 &     (1.161)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.032$^{\ast\ast}$    &       0.002                 &      -0.036                 &      -0.038                 &      -0.467                 &       0.008                 \\
            &     (0.013)                 &     (0.021)                 &     (0.024)                 &     (0.034)                 &     (0.726)                 &     (0.005)                 \\%\midrule
%$R^{2}$  &        .999                 &          0.999                &        .822                 &          0.999                &        .988                 &        .948                 \\
%$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/all_subperiod/Results4shortRICTint_ct_All_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007 (N=224)}}} \\\midrule
$R_{c,t}$ &      -0.145$^{\ast\ast\ast}$&      -0.040                 &      -0.084$^{\ast\ast}$    &      -0.065$^{\ast\ast}$    &      -1.539$^{\ast\ast\ast}$&       0.011                 \\
            &     (0.040)                 &     (0.023)                 &     (0.029)                 &     (0.026)                 &     (0.497)                 &     (0.011)                 \\\addlinespace
$ICT_{c,t}$&       0.301$^{\ast\ast\ast}$&      -0.142$^{\ast\ast\ast}$&       0.141$^{\ast\ast\ast}$&      -0.049$^{\ast}$        &      -2.427$^{\ast\ast}$    &       0.018                 \\
            &     (0.052)                 &     (0.023)                 &     (0.040)                 &     (0.024)                 &     (1.107)                 &     (0.017)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.141$^{\ast\ast\ast}$&       0.040$^{\ast\ast\ast}$&      -0.065$^{\ast\ast}$    &       0.017                 &       1.215$^{\ast}$        &      -0.006                 \\
            &     (0.032)                 &     (0.011)                 &     (0.023)                 &     (0.015)                 &     (0.607)                 &     (0.010)                 \\%\midrule
%$R^{2}$  &        .998                 &        .999                 &        .923                 &          0.999                &         .98                 &        .878                 \\
%$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/all_subperiod/Results5RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.008                 &      -0.035                 &      -0.025                 &      -0.006                 &       0.066$^{\ast\ast}$    &      -0.033$^{\ast\ast}$    &       0.028                 &      -0.003                 \\
            &     (0.030)                 &     (0.039)                 &     (0.024)                 &     (0.025)                 &     (0.026)                 &     (0.014)                 &     (0.026)                 &     (0.010)                 \\\addlinespace
$ICT_{c,t}$&       0.047                 &       0.127$^{\ast}$        &       0.083$^{\ast}$        &       0.069                 &       0.039                 &       0.029                 &       0.013                 &       0.020$^{\ast\ast\ast}$\\
            &     (0.034)                 &     (0.061)                 &     (0.037)                 &     (0.054)                 &     (0.029)                 &     (0.020)                 &     (0.022)                 &     (0.002)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.029                 &      -0.063                 &      -0.048                 &      -0.049                 &      -0.018                 &      -0.026$^{\ast}$        &      -0.016                 &      -0.002                 \\
            &     (0.030)                 &     (0.040)                 &     (0.029)                 &     (0.035)                 &     (0.026)                 &     (0.013)                 &     (0.019)                 &     (0.009)                 \\\midrule
%$R^{2}$  &        .999                 &        .999                 &          0.999                &          0.999                &          0.999                &        .875                 &          0.999                &        .978                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         135                 &         135                 &         135                 &         135                 \\


==> inputs/all_subperiod/Results5RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.193$^{\ast\ast\ast}$&      -0.147$^{\ast\ast\ast}$&      -0.180$^{\ast\ast\ast}$&      -0.133$^{\ast\ast\ast}$&      -0.060$^{\ast\ast\ast}$&      -0.114$^{\ast\ast\ast}$&      -0.017                 &       0.009                 \\
            &     (0.038)                 &     (0.041)                 &     (0.037)                 &     (0.038)                 &     (0.015)                 &     (0.023)                 &     (0.011)                 &     (0.011)                 \\\addlinespace
$ICT_{c,t}$&       0.126$^{\ast\ast\ast}$&      -0.034                 &       0.059                 &       0.096$^{\ast}$        &       0.015                 &       0.014                 &       0.142$^{\ast\ast\ast}$&      -0.091$^{\ast\ast\ast}$\\
            &     (0.040)                 &     (0.066)                 &     (0.049)                 &     (0.054)                 &     (0.018)                 &     (0.047)                 &     (0.031)                 &     (0.028)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.074$^{\ast\ast}$    &      -0.048                 &      -0.060$^{\ast}$        &      -0.085$^{\ast\ast}$    &      -0.010                 &      -0.015                 &      -0.061$^{\ast\ast}$    &       0.058$^{\ast\ast\ast}$\\
            &     (0.028)                 &     (0.038)                 &     (0.032)                 &     (0.035)                 &     (0.015)                 &     (0.027)                 &     (0.020)                 &     (0.015)                 \\\midrule
%$R^{2}$  &        .999                 &        .998                 &        .999                 &        .999                 &          0.999                &        .946                 &        .999                 &        .929                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         174                 &         174                 &         174                 &         174                 \\


==> inputs/coverage/Coverage_sample_firm_L.tex <==
 & (1) & (2) & (3) & (4) & (5) \\                                  
 Country &\multicolumn{3}{c}{Total employment} & \multicolumn{2}{c}{Employment share \%} \\\cmidrule(r){2-4} \cmidrule(r){5-6}                                                  & EUKLEMS & $R$-sample & $ICT$-sample & $R$-sample & $ICT$-sample \\\midrule
AT          &   1,254,090&     932,795&     932,795&       74.38&       74.38\\
BE          &   1,130,893&     784,687&     784,687&       69.39&       69.39\\
CZ          &   2,080,420&   1,283,846&   1,283,846&       61.71&       61.71\\
DE          &  12,381,000&   8,997,709&   8,997,709&       72.67&       72.67\\
DK          &     733,000&     297,891&     297,891&       40.64&       40.64\\
EE          &     241,000&      57,452&      10,524&       23.84&        4.37\\
ES          &   4,787,000&   1,572,781&   1,572,781&       32.86&       32.86\\
FI          &     705,900&     824,132&     824,132&      116.75&      116.75\\
FR          &   6,386,000&   1,508,347&   1,508,347&       23.62&       23.62\\
GR          &     777,160&      49,835&      49,835&        6.41&        6.41\\
HR          &     545,340&     291,881&          N/A&       53.52&          N/A\\
HU          &   1,495,220&     536,044&          N/A&       35.85&          N/A\\
IE          &     472,790&     677,391&          N/A&      143.28&          N/A\\
IT          &   6,534,000&   4,614,803&   4,614,803&       70.63&       70.63\\
LT          &     495,570&     482,602&     294,167&       97.38&       59.36\\
LV          &     291,860&     113,203&     113,203&       38.79&       38.79\\
NL          &   1,654,000&   1,610,159&   1,610,159&       97.35&       97.35\\
PL          &   5,863,800&   1,313,027&          N/A&       22.39&          N/A\\
PT          &   1,389,160&     598,185&          N/A&       43.06&          N/A\\
RO          &   2,907,400&   1,470,350&          N/A&       50.57&          N/A\\
SE          &   1,489,000&   1,352,279&   1,352,279&       90.82&       90.82\\
SI          &     325,680&     155,516&      53,275&       47.75&       16.36\\
SK          &     821,310&     436,482&     436,482&       53.14&       53.14\\
UK          &   6,433,010&   4,806,876&   4,806,876&       74.72&       74.72\\\midrule
Mean        &   2,549,775&   1,448,678&   1,641,322&       60.06&       55.78\\


==> inputs/coverage/Coverage_sample_firm_T.tex <==
 & (1) & (2) & (3) & (4) & (5) \\                                  Country &\multicolumn{3}{c}{Aggregate Tax} & \multicolumn{2}{c}{Tax share (Sample Tax/$T^{k,corp}_{c}$)\%} \\\cmidrule(r){2-4} \cmidrule(r){5-6}                                                  & $T^{k}_{c}$ & $T^{k,corp}_{c}$ & $T^{k}_{c} / T^{k,corp}_{c}$ & $R$-sample & $ICT$-sample \\\midrule
AT          &          44&           8&       19.18&          N/A&          N/A\\
BE          &          81&          15&       18.03&       39.61&       39.61\\
CZ          &         385&         179&       46.40&        0.16&        0.16\\
DE          &         410&          62&       15.23&          N/A&          N/A\\
DK          &         641&          60&        9.32&        7.62&        7.62\\
EE          &           2&           0&       21.88&        4.37&        4.12\\
ES          &         133&          25&       18.97&       35.34&       35.34\\
FI          &          36&           5&       13.33&       30.52&       30.52\\
FR          &         331&          45&       13.70&       19.10&       19.10\\
GR          &          21&           4&       20.43&        3.16&        3.16\\
HU          &       3,076&         831&       27.02&        0.10&          N/A\\
IE          &          31&           7&       23.56&        1.06&          N/A\\
IT          &         275&          36&       13.19&       27.11&       27.11\\
LT          &           2&           1&       27.26&        3.90&          N/A\\
LV          &           2&           0&       18.61&          N/A&          N/A\\
NL          &          85&          24&       27.96&        7.32&        7.32\\
PL          &         150&          34&       22.81&        6.84&          N/A\\
PT          &          21&           6&       27.49&       35.85&          N/A\\
SE          &         744&         121&       16.20&        1.36&        1.36\\
SI          &           3&           1&       21.35&        1.31&          N/A\\
SK          &           6&           3&       46.77&       31.92&       31.92\\
UK          &         311&          53&       17.12&       56.61&       56.61\\\midrule
Mean        &         309&          69&       22.08&       16.49&       20.30\\


==> inputs/descriptives/Coverage_sample_cit.tex <==
\begin{tabular}{lccccccccccccccc} \toprule

&\multicolumn{15}{c}{Industry groups based on ISIC Rev.4 (NACE Rev.2) 2-digit codes used in the industry-level sample} \\ \cmidrule(l){2-16}
Country & 01t03 & 05t09 & 10t12 & 13t15 & 16t18 & 19t21 & 22t23 & 24t25 & 26t27 & 28 & 29t30 & 31t33 & 35t39 & 41t43 & 85 \\ \midrule
AT & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
BE & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
CZ & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
DE & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
DK & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
EE & 2000-2016 & 2000-2016 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 2000-2016 & 2000-2016 & 2000-2016 \\
ES & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
FI & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
FR & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
GR & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
IT & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
LT & 1995-2016 & 1995-2016 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1995-2016 & 1995-2016 & 1995-2016 \\
LV & 1995-2016 & 2000-2016 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 2000-2016 & 1995-2016 & 2000-2016 \\
NL & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
SE & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\
SI & 2000-2016 & 2000-2016 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 2000-2016 & 2000-2016 & 2000-2016 \\
SK & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 & 2000-2016 \\
 UK & 2007-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 & 1995-2016 \\ \bottomrule
\end{tabular}


==> inputs/descriptives/Industry_codes_IFR_EUKLEMS.tex <==
\begin{tabular}{ccl} \toprule
\multicolumn{2}{c}{Industry aggregation:} & \\ \cmidrule(l){1-2}
EUKLEMS & IFR  & Description of industries in IFR dataset \\ \midrule
01t03 & 01t03 & A-B-Agriculture, forestry, fishing \\
05t09 & 05t09 & C-Mining and quarrying \\
10t12 & 10t12 & 10-12-Food and beverages \\
13t15 & 13t15 & 13-15-Textiles \\
16t18 & 16 & 16-Wood and furniture \\
16t18 & 17t18 & 17-18-Paper \\
19t21 & 19t20 & 20-21-other chemical products n.e.c. \\
19t21 & 21 & 19-Pharmaceuticals, cosmetics \\
22t23 & 22 & 22-Rubber and plastic products (non-automotive) \\
22t23 & 23 & 23-Glass, ceramics, stone, mineral products (non-auto \\
24t25 & 24 & 24-Basic metals \\
24t25 & 25 & 25-Metal products (non-automotive) \\
26t27 & 26t27 & 26-27-Electrical/electronics \\
28 & 28 & 28-Industrial machinery \\
29t30 & 29 & 29-Automotive \\
29t30 & 30 & 30-Other vehicles \\
31t33 & 32 & 91-All other manufacturing branches \\
35t39 & 35t39 & E-Electricity, gas, water supply \\
41t43 & 41t43 & F-Construction \\
85 & 85 & P-Education/research/development \\
 Rest & Rest & 90-All other non-manufacturing branches \\ \bottomrule
\end{tabular}

==> inputs/descriptives/Sumstat_controls_ct_AT.tex <==
\multicolumn{20}{l}{AT} \\\midrule
Mean        &          42&          17&          13&          12&          40&          30&          28&         154&          79&         470&         1.8&          56&         .12&          72&         3.1&        -2.7&           3&         .16&         .51\\
St.Dev.     &           1&         .44&         .61&         .37&         .86&           1&         .56&          29&          21&         122&         1.6&         .92&       .0029&           8&         .51&         1.4&         .37&       .0037&        .007\\
Min         &          40&          16&          11&          11&          39&          28&          27&         112&          46&         290&        -3.8&          54&         .11&          64&         2.1&        -6.1&         2.4&         .15&          .5\\
Median      &          42&          17&          13&          12&          40&          30&          29&         150&          83&         471&           2&          57&         .12&          68&         3.1&        -2.5&           3&         .16&         .51\\
Max         &          43&          18&          14&          13&          43&          32&          29&         206&         112&         646&         3.7&          58&         .13&          85&           4&         -.7&         3.9&         .16&         .52\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_All.tex <==
%\multicolumn{20}{l}{All} \\\midrule
Mean        &          36&          12&          13&          12&          32&          35&          32&         530&         330&        1830&         2.3&          57&         .13&          63&         2.8&          -3&         3.5&         .16&         .51\\
St.Dev.     &         5.8&         4.2&         5.2&         1.5&          10&          10&         5.2&         578&         414&        2212&         3.5&         6.8&        .026&          34&         1.8&         3.7&           1&        .049&        .029\\
Min         &          23&         .29&         4.6&         6.9&          .6&          17&          23&         2.5&         1.7&         8.7&         -15&          41&        .082&         8.5&          .4&         -32&         1.5&        .081&         .41\\
Median      &          35&          12&          12&          11&          33&          32&          31&         209&         120&         715&         2.3&          57&         .13&          58&         2.6&        -2.6&         3.6&         .15&         .51\\
Max         &          49&          19&          33&          16&          45&          69&          44&        2307&        1978&       10831&          25&          71&         .19&         181&          11&         6.9&         7.7&          .4&          .6\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_BE.tex <==
\multicolumn{20}{l}{BE} \\\midrule
Mean        &          43&          14&          19&          11&          32&          43&          25&         177&         106&         649&         1.9&          60&         .13&         106&         5.1&        -2.1&         2.2&         .21&         .56\\
St.Dev.     &         .76&         .35&         .59&         .18&         .71&          .8&         .53&          37&          24&         149&         1.4&         1.9&         .01&          12&         1.9&         1.8&         .19&        .054&       .0088\\
Min         &          42&          13&          17&          10&          31&          41&          24&         121&          70&         417&          -2&          56&         .12&          87&         2.7&        -5.4&         1.9&         .15&         .55\\
Median      &          43&          14&          19&          11&          32&          43&          25&         174&         111&         651&         1.8&          60&         .13&         105&         4.3&        -2.3&         2.1&          .2&         .56\\
Max         &          45&          14&          20&          11&          33&          44&          26&         232&         147&         868&         3.8&          63&         .15&         131&           9&          .2&         2.6&         .31&         .57\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_CZ.tex <==
\multicolumn{20}{l}{CZ} \\\midrule
Mean        &          33&          15&         8.1&          11&          44&          24&          32&        1590&        1357&        7499&         2.7&          46&         .17&          28&         1.1&        -3.6&         4.8&         .15&         .53\\
St.Dev.     &         .75&         .21&         .67&          .5&         .75&         1.7&         1.5&         484&         384&        2403&         2.8&         1.1&        .012&          11&         .16&         2.7&         .94&       .0064&       .0046\\
Min         &          32&          14&           7&         9.9&          41&          21&          30&         737&         703&        3451&        -4.7&          44&         .15&          12&          .8&         -12&         3.2&         .14&         .52\\
Median      &          33&          15&           8&          11&          44&          24&          32&        1668&        1403&        7916&         2.6&          46&         .17&          28&         1.1&          -3&         4.7&         .15&         .54\\
Max         &          35&          15&         9.2&          12&          45&          27&          34&        2307&        1978&       10831&         6.8&          49&         .19&          44&         1.4&          .7&         7.7&         .16&         .54\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_DE.tex <==
\multicolumn{20}{l}{DE} \\\midrule
Mean        &          35&          14&          11&          10&          39&          32&          29&        1452&         726&        4339&         1.4&          57&         .15&          67&         2.7&        -2.1&         2.2&         .12&         .53\\
St.Dev.     &         .98&         .43&         .78&         .25&         1.3&         1.4&         .72&         196&         139&         780&           2&           1&       .0063&         8.5&         .66&         2.4&         .18&       .0037&       .0036\\
Min         &          34&          13&          10&         9.7&          36&          30&          27&        1192&         528&        3185&        -5.7&          55&         .14&          55&         1.2&        -9.4&         1.9&         .12&         .52\\
Median      &          35&          14&          11&          10&          39&          32&          28&        1385&         712&        4284&         1.6&          56&         .15&          65&         2.8&        -2.1&         2.2&         .12&         .53\\
Max         &          37&          15&          13&          11&          41&          35&          30&        1864&         984&        5657&         4.2&          59&         .16&          82&         3.5&         1.2&         2.6&         .13&         .53\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_DK.tex <==
\multicolumn{20}{l}{DK} \\\midrule
Mean        &          46&         .39&          30&          15&         .85&          66&          33&         972&         505&        2970&         1.3&          66&        .096&          42&         2.1&         .64&         3.2&        .094&         .52\\
St.Dev.     &         1.1&         .17&         1.1&         .51&         .37&         1.3&         1.2&         136&          82&         469&           2&           2&       .0033&         6.7&         .75&         2.8&         .44&         .01&       .0052\\
Min         &          45&         .29&          29&          15&          .6&          64&          30&         738&         405&        2206&        -4.9&          63&         .09&          27&         1.1&        -3.5&         2.6&        .081&         .51\\
Median      &          46&         .33&          30&          15&         .73&          65&          33&        1030&         493&        3093&         1.3&          65&        .096&          44&         1.9&          .1&           3&        .091&         .51\\
Max         &          48&         .88&          33&          16&         1.9&          69&          35&        1174&         648&        3610&         3.9&          68&          .1&          52&         3.7&           5&         3.9&         .12&         .53\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_ES.tex <==
\multicolumn{20}{l}{ES} \\\midrule
Mean        &          33&          12&          12&         9.3&          35&          36&          28&         506&         283&        1650&         2.2&          53&         .13&          63&         2.9&        -3.9&         3.8&         .15&         .49\\
St.Dev.     &         1.6&          .2&         1.1&         .78&         1.7&         1.8&         1.8&         129&          86&         482&         2.5&         3.3&         .01&          21&         1.1&         4.1&         .89&       .0074&        .017\\
Min         &          30&          11&          11&         6.9&          32&          34&          23&         286&         139&         811&        -3.8&          49&         .11&          36&         1.6&         -11&           2&         .14&         .46\\
Median      &          33&          12&          12&         9.5&          35&          36&          29&         553&         314&        1890&           3&          51&         .13&          61&         2.9&        -4.1&         3.9&         .15&          .5\\
Max         &          36&          12&          15&          10&          40&          42&          31&         664&         387&        2253&         5.2&          59&         .14&         101&           5&         2.1&         5.2&         .16&         .51\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_East.tex <==
\multicolumn{20}{l}{East} \\\midrule
Mean        &          32&          12&         7.8&          12&          38&          25&          37&         369&         314&        1733&         3.5&          50&         .15&          32&         1.4&        -3.5&           4&         .18&         .53\\
St.Dev.     &         3.2&         2.6&         1.2&         1.2&         5.7&           4&         3.5&         698&         592&        3313&         4.4&         5.8&        .027&          16&         .71&           3&         1.1&        .065&        .037\\
Min         &          27&         7.7&         4.6&         9.9&          26&          17&          30&         2.5&         1.7&         8.7&         -15&          41&        .093&         8.5&          .4&         -15&         1.5&         .11&         .41\\
Median      &          31&          13&           8&          11&          40&          24&          37&          18&          10&          67&         3.6&          50&         .15&          28&         1.3&        -2.8&           4&         .16&         .53\\
Max         &          38&          16&         9.8&          15&          45&          34&          44&        2307&        1978&       10831&          12&          63&         .19&          83&           4&         1.4&         7.7&          .4&          .6\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_FI.tex <==
\multicolumn{20}{l}{FI} \\\midrule
Mean        &          43&          12&          17&          14&          28&          40&          31&          95&          48&         307&         2.3&          53&         .15&          47&         2.1&         .54&         3.8&         .11&         .51\\
St.Dev.     &         1.5&         .66&         1.3&         .61&         1.3&         2.2&         1.2&          21&          11&          74&         3.2&         3.2&         .02&         8.9&           1&         3.5&         .29&        .015&        .013\\
Min         &          41&          11&          16&          12&          25&          37&          29&          59&          27&         178&        -8.1&          48&         .12&          33&         1.1&        -5.9&         3.3&        .096&          .5\\
Median      &          43&          12&          17&          14&          28&          41&          32&          95&          51&         320&         2.8&          52&         .16&          45&         1.6&          .3&         3.9&         .11&         .51\\
Max         &          46&          14&          21&          14&          31&          46&          33&         123&          63&         396&         6.3&          59&         .18&          64&         4.1&         6.9&         4.4&         .14&         .53\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_FR.tex <==
\multicolumn{20}{l}{FR} \\\midrule
Mean        &          42&          18&          13&          11&          40&          31&          25&        1077&         505&        3095&         1.6&          64&         .11&          73&         2.8&        -3.7&         3.9&         .16&         .49\\
St.Dev.     &         1.3&         .86&         1.4&         .51&         1.9&         2.8&         1.2&         210&          92&         623&         1.4&         2.2&       .0081&          15&         .46&         1.5&         .22&        .017&       .0051\\
Min         &          40&          17&         9.8&          10&          38&          23&          24&         754&         337&        2061&        -2.9&          61&        .095&          56&         1.8&        -7.2&         3.4&         .14&         .49\\
Median      &          42&          17&          14&          11&          40&          32&          25&        1088&         533&        3197&         1.8&          64&         .11&          65&         2.8&        -3.6&         3.9&         .16&         .49\\
Max         &          44&          19&          15&          12&          45&          33&          28&        1381&         611&        3895&         3.9&          68&         .12&          98&         3.6&        -1.3&         4.3&          .2&         .51\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_GR.tex <==
\multicolumn{20}{l}{GR} \\\midrule
Mean        &          32&          10&         9.8&          12&          32&          30&          38&          94&          62&         282&         .84&          66&         .09&         126&         5.9&        -7.5&         4.5&         .17&         .48\\
St.Dev.     &         2.7&         .65&         1.2&         1.3&         1.9&           2&         2.1&          25&          13&          68&         4.4&         3.2&       .0034&          33&         2.1&         3.4&         1.1&        .023&       .0097\\
Min         &          28&           9&         7.5&          11&          28&          26&          35&          49&          36&         157&         -10&          60&        .084&          97&         3.2&         -15&         2.5&         .14&         .46\\
Median      &          32&          11&         9.7&          12&          32&          31&          37&          95&          63&         288&         2.5&          66&        .091&         106&         5.2&        -6.5&         4.7&         .17&         .48\\
Max         &          39&          11&          12&          15&          35&          35&          41&         131&          85&         386&         5.8&          70&        .098&         181&          11&          .5&         5.9&         .24&         .49\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_IE.tex <==
\multicolumn{20}{l}{IE} \\\midrule
Mean        &          29&         4.4&          14&          11&          15&          47&          37&          73&          64&         318&         5.7&          58&         .14&          61&         2.5&        -3.2&         3.1&         .18&          .5\\
St.Dev.     &         2.4&         .59&         1.2&         1.4&         2.6&         1.8&         2.3&          24&          34&         123&         6.2&         5.1&        .017&          32&         1.3&         8.2&         .97&        .035&        .017\\
Min         &          23&         3.7&          11&         7.5&          12&          44&          33&          30&          19&         114&        -5.1&          51&         .12&          24&           1&         -32&         1.8&         .13&         .47\\
Median      &          28&         4.1&          14&          11&          14&          48&          37&          84&          63&         342&         5.5&          55&         .14&          57&         2.4&        -.35&         3.3&         .18&          .5\\
Max         &          32&         5.5&          15&          13&          20&          50&          40&         103&         152&         561&          25&          67&         .18&         120&         5.1&         4.9&         5.3&         .28&         .53\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_IT.tex <==
\multicolumn{20}{l}{IT} \\\midrule
Mean        &          39&          13&          16&          11&          30&          38&          27&         826&         459&        2747&         .66&          56&         .14&         116&         5.8&        -3.4&         2.9&         .14&         .48\\
St.Dev.     &         1.7&         .74&         .75&         .53&         1.5&           1&         .91&         134&          72&         469&           2&           2&         .01&          11&         2.1&         1.4&         .36&       .0077&        .015\\
Min         &          37&          11&          14&          10&          29&          37&          25&         582&         308&        1838&        -5.3&          52&         .12&         104&         3.9&        -7.2&         2.3&         .12&         .46\\
Median      &          39&          13&          16&          11&          30&          39&          26&         872&         487&        2941&         1.3&          56&         .14&         115&         4.8&          -3&         2.9&         .14&         .48\\
Max         &          42&          14&          17&          12&          34&          41&          28&         969&         549&        3267&         3.8&          59&         .16&         135&          11&        -1.3&         3.7&         .15&          .5\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_LT.tex <==
\multicolumn{20}{l}{LT} \\\midrule
Mean        &          29&          10&         7.6&          12&          35&          26&          39&          11&         9.9&          41&         4.3&          51&         .14&          26&         1.3&        -3.2&         3.6&         .18&         .53\\
St.Dev.     &         1.7&         1.3&         1.9&         .79&           5&         5.5&         1.7&         4.5&         4.5&          17&         5.3&         2.8&        .011&          10&         .43&         3.3&           1&        .049&        .016\\
Min         &          27&         7.7&         4.6&          11&          28&          17&          36&         4.8&         3.9&          19&         -15&          44&         .12&          14&          .7&         -12&         2.3&         .12&          .5\\
Median      &          29&          10&         8.3&          11&          32&          28&          40&          12&         9.4&          42&         5.2&          51&         .14&          23&         1.3&        -2.8&         3.6&         .17&         .54\\
Max         &          33&          13&         9.8&          13&          42&          33&          42&          19&          16&          66&          11&          56&         .16&          43&           2&          .2&         5.4&         .27&         .55\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_LV.tex <==
\multicolumn{20}{l}{LV} \\\midrule
Mean        &          29&         8.9&         8.4&          12&          31&          29&          40&         7.4&           6&          30&         4.2&          59&          .1&          23&           1&        -2.2&         3.7&         .25&          .5\\
St.Dev.     &         1.1&         .81&         .46&         .86&         2.5&         1.8&           2&         3.9&         2.8&          15&           6&         1.8&       .0095&          15&         .46&         2.7&         1.5&        .098&        .064\\
Min         &          27&         7.9&         7.6&          10&          26&          26&          37&         2.5&         1.7&         8.7&         -14&          55&        .093&         8.5&          .4&        -9.6&         1.5&         .13&         .41\\
Median      &          29&         8.7&         8.4&          12&          30&          29&          40&         8.1&         6.9&          35&         5.7&          59&          .1&          14&          .9&        -1.4&         3.7&         .22&         .48\\
Max         &          31&          10&         9.6&          14&          35&          34&          44&          13&         9.4&          49&          12&          63&         .13&          48&         1.8&         1.4&           6&          .4&          .6\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_NL.tex <==
\multicolumn{20}{l}{NL} \\\midrule
Mean        &          36&          14&          11&          11&          38&          31&          30&         333&         158&        1026&           2&          63&         .11&          58&         2.6&        -2.1&         3.8&         .12&         .54\\
St.Dev.     &           1&         .88&         .56&         .21&         1.8&         1.3&         .94&          71&          38&         245&         2.1&         1.6&       .0035&         8.8&         1.2&         2.3&         .24&       .0088&       .0046\\
Min         &          34&          12&          10&          10&          35&          28&          29&         209&          90&         594&        -3.7&          60&        .099&          43&         1.2&        -8.7&         3.5&         .11&         .53\\
Median      &          36&          14&          11&          11&          38&          32&          30&         333&         170&        1045&         2.1&          63&         .11&          59&         2.1&        -1.8&         3.8&         .12&         .54\\
Max         &          38&          15&          12&          11&          41&          33&          32&         430&         205&        1360&           5&          66&         .11&          73&         5.1&         1.2&         4.3&         .14&         .55\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_North.tex <==
\multicolumn{20}{l}{North} \\\midrule
Mean        &          39&          12&          16&          12&          29&          40&          30&         656&         379&        2078&         2.3&          60&         .12&          64&         2.8&        -1.9&         3.2&         .15&         .52\\
St.Dev.     &         5.8&         5.3&         5.1&         1.6&          12&          10&         3.7&         567&         371&        1849&           3&         5.1&        .023&          23&         1.4&         3.7&         .84&        .042&         .02\\
Min         &          23&         .29&         9.8&         7.5&          .6&          23&          24&          30&          19&         114&        -8.1&          48&        .082&          24&          .5&         -32&         1.6&        .081&         .47\\
Median      &          41&          14&          15&          11&          32&          39&          29&         410&         195&        1294&         2.2&          60&         .12&          62&         2.7&        -1.9&         3.3&         .14&         .52\\
Max         &          49&          19&          33&          16&          45&          69&          40&        2166&        1710&        7618&          25&          71&         .18&         131&           9&         6.9&         5.3&         .31&         .57\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_PT.tex <==
\multicolumn{20}{l}{PT} \\\midrule
Mean        &          31&         8.5&          10&          13&          27&          31&          41&          93&          51&         302&         .54&          58&         .11&          91&         3.5&        -5.5&         3.6&         .21&         .52\\
St.Dev.     &         1.5&         .38&           1&         .54&         .86&         1.9&         1.9&         6.7&         9.8&          28&         2.1&         2.2&       .0067&          30&         .89&         2.5&         1.1&        .011&        .017\\
Min         &          29&         7.9&         8.8&          12&          25&          29&          37&          78&          34&         245&        -4.1&          54&        .097&          54&         2.6&         -11&         1.5&         .19&          .5\\
Median      &          31&         8.5&         9.8&          13&          27&          32&          41&          93&          54&         309&         .79&          58&         .11&          76&           3&        -5.1&         3.7&         .22&         .52\\
Max         &          34&         9.1&          12&          14&          29&          35&          44&         102&          66&         338&         3.8&          61&         .13&         133&         4.9&        -1.9&         5.3&         .23&         .55\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_SE.tex <==
\multicolumn{20}{l}{SE} \\\midrule
Mean        &          45&          15&          18&          12&          32&          40&          27&        1480&        1179&        5397&         2.6&          61&         .13&          49&         2.3&        -.12&         4.3&         .11&         .53\\
St.Dev.     &         2.1&         .48&           2&         .25&         1.2&         2.5&         1.5&         389&         285&        1346&         2.3&         2.5&        .012&          11&         1.5&         2.2&         .27&       .0049&       .0089\\
Min         &          42&          14&          16&          12&          30&          36&          25&         901&         746&        3334&        -4.3&          58&          .1&          37&          .5&          -7&         3.9&        .096&         .51\\
Median      &          45&          15&          18&          12&          33&          40&          27&        1440&        1193&        5448&           3&          60&         .13&          47&         1.7&           0&         4.3&         .11&         .53\\
Max         &          49&          16&          22&          13&          34&          44&          29&        2166&        1710&        7618&           6&          66&         .15&          69&         5.2&         3.3&         5.1&         .12&         .54\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_SK.tex <==
\multicolumn{20}{l}{SK} \\\midrule
Mean        &          31&          13&         6.7&          11&          42&          22&          36&          27&          27&         137&         3.9&          44&         .18&          44&         2.1&        -4.7&         3.7&         .19&         .51\\
St.Dev.     &         1.9&         .98&         .61&         .73&         1.6&           1&         1.8&         7.9&         7.2&          39&         3.6&         1.5&        .012&         8.8&          .9&         2.9&         .77&        .017&       .0091\\
Min         &          28&          11&         5.7&         9.9&          39&          20&          33&          15&          13&          73&        -5.5&          41&         .15&          29&         1.3&         -13&         2.9&         .16&         .48\\
Median      &          31&          13&         6.5&          11&          43&          22&          36&          30&          29&         143&         4.5&          44&         .18&          43&         1.8&        -3.1&         3.6&         .19&         .51\\
Max         &          34&          14&         7.5&          12&          44&          23&          39&          39&          35&         193&          11&          46&         .19&          55&           4&        -2.1&         6.4&         .21&         .52\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_South.tex <==
\multicolumn{20}{l}{South} \\\midrule
Mean        &          34&          11&          12&          11&          31&          34&          33&         397&         223&        1302&         1.1&          58&         .12&     1.0e+02&         4.6&        -5.1&         3.7&         .16&         .49\\
St.Dev.     &         3.7&         1.6&         2.7&         1.6&         3.4&         3.8&         6.2&         325&         180&        1094&           3&         5.6&        .019&          35&         2.1&         3.4&         1.1&         .03&        .023\\
Min         &          28&         7.9&         7.5&         6.9&          25&          26&          23&          49&          34&         157&         -10&          49&        .084&          36&         1.6&         -15&         1.5&         .12&         .46\\
Median      &          33&          11&          11&          11&          31&          35&          30&         318&         157&         927&         1.6&          57&         .12&         104&         4.4&        -4.6&         3.7&         .15&         .49\\
Max         &          42&          14&          17&          15&          40&          42&          44&         969&         549&        3267&         5.8&          70&         .16&         181&          11&         2.1&         5.9&         .24&         .55\\\bottomrule


==> inputs/descriptives/Sumstat_controls_ct_UK.tex <==
\multicolumn{20}{l}{UK} \\\midrule
Mean        &          32&         5.8&          16&          10&          18&          49&          32&         825&         448&        2429&         2.2&          68&        .089&          55&         2.4&        -3.8&         2.4&         .18&          .5\\
St.Dev.     &         .96&         .35&         .86&         .46&         .84&         1.6&         1.8&         203&          89&         573&         1.8&         2.6&       .0083&          21&         .48&         3.1&         .52&        .016&       .0087\\
Min         &          29&         5.1&          14&         9.1&          17&          47&          29&         485&         335&        1527&        -4.1&          62&        .082&          34&         1.8&         -10&         1.6&         .15&         .49\\
Median      &          32&           6&          16&          10&          19&          49&          32&         858&         463&        2508&         2.4&          69&        .085&          43&         2.4&        -3.1&         2.5&         .18&          .5\\
Max         &          33&         6.2&          17&          11&          20&          52&          36&        1147&         609&        3329&           5&          71&         .11&          87&         3.1&         1.4&         3.3&          .2&         .52\\\bottomrule


==> inputs/descriptives/Sumstat_firm.tex <==
&\multicolumn{2}{c}{$R$-sample}
&
\multicolumn{2}{c}{$ICT$-sample}
\\\cmidrule(r){2-3}
\cmidrule(r){4-5}
&
$L_{f,i,t}$
&
$T_{f,i,t}^\dagger$
&
$L_{f,i,t}$
&
$T_{f,i,t}^\dagger$
\\\midrule
Mean        &          23&         321&          26&         409\\
St.Dev.     &         838&      30,453&         985&      35,244\\
Min         &           1&        .001&           1&        .001\\
Median      &           4&         5.2&           3&           8\\
Max         &     855,492&  24,474,986&     855,492&  24,474,986\\


==> inputs/descriptives/Sumstat_firm_more.tex <==
 \# Observations&  16,261,216&   8,095,653&  11,391,818&   6,019,433\\
 \# Firms &   4,385,360&   1,964,694&   3,245,827&   1,478,475\\
 \# Countries&          24&          24&          18&          18\\
 \# NUTS2 regions&         273&         273&         227&         227\\
 \# NUTS3 regions&       1,310&       1,314&       1,119&       1,123\\\bottomrule


==> inputs/east_95_16/Results1RICTint_ct_East_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.030                 &      -0.042$^{\ast\ast}$    &       0.037                 &      -0.062$^{\ast}$        &      -0.294                 &      -0.220                 &       0.468                 &      -0.542$^{\ast\ast}$    &      -0.568                 &       2.044$^{\ast}$        &      -1.416$^{\ast\ast}$    \\
            &     (0.029)                 &     (0.012)                 &     (0.056)                 &     (0.029)                 &     (0.553)                 &     (0.218)                 &     (0.404)                 &     (0.181)                 &     (0.807)                 &     (0.924)                 &     (0.457)                 \\\addlinespace
$ICT_{c,t}$&       0.024                 &       0.096$^{\ast}$        &      -0.063                 &      -0.001                 &       2.337                 &       1.701$^{\ast}$        &       0.154                 &       0.482                 &       2.672                 &      -1.343                 &      -1.310                 \\
            &     (0.048)                 &     (0.040)                 &     (0.083)                 &     (0.075)                 &     (1.205)                 &     (0.793)                 &     (0.479)                 &     (0.442)                 &     (1.634)                 &     (0.913)                 &     (1.443)                 \\\addlinespace
$R*ICT_{c,t}$&       0.009                 &      -0.019                 &       0.024                 &       0.033                 &      -0.100                 &      -0.405$^{\ast}$        &       0.081                 &       0.224                 &      -1.171$^{\ast\ast}$    &       0.368                 &       0.807                 \\
            &     (0.009)                 &     (0.010)                 &     (0.014)                 &     (0.018)                 &     (0.278)                 &     (0.178)                 &     (0.106)                 &     (0.114)                 &     (0.380)                 &     (0.179)                 &     (0.395)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .948                 &        .977                 &        .845                 &        .901                 &        .962                 &        .917                 &        .909                 \\
$N$      &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 \\


==> inputs/east_95_16/Results2RICTint_ct_East_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.017                 &      -0.036$^{\ast}$        &       0.054                 &      -0.047                 &       0.100                 &      -0.285                 &       0.570                 &      -0.185$^{\ast\ast\ast}$&      -1.207                 &       2.046$^{\ast}$        &      -0.763                 \\
            &     (0.021)                 &     (0.014)                 &     (0.052)                 &     (0.029)                 &     (0.471)                 &     (0.206)                 &     (0.362)                 &     (0.038)                 &     (0.583)                 &     (0.817)                 &     (0.473)                 \\\addlinespace
$ICT_{c,t}$&      -0.008                 &       0.120                 &      -0.173                 &      -0.035                 &       1.197                 &       1.918                 &      -0.509                 &      -0.211                 &       4.590$^{\ast}$        &      -2.596                 &      -1.982                 \\
            &     (0.049)                 &     (0.076)                 &     (0.108)                 &     (0.057)                 &     (1.598)                 &     (0.998)                 &     (0.793)                 &     (0.316)                 &     (1.737)                 &     (1.548)                 &     (1.592)                 \\\addlinespace
$R*ICT_{c,t}$&       0.011                 &      -0.024                 &       0.033                 &       0.034$^{\ast\ast}$    &      -0.164                 &      -0.402$^{\ast}$        &       0.153                 &       0.085                 &      -1.084$^{\ast\ast}$    &       0.666$^{\ast}$        &       0.411                 \\
            &     (0.008)                 &     (0.014)                 &     (0.017)                 &     (0.012)                 &     (0.276)                 &     (0.164)                 &     (0.125)                 &     (0.049)                 &     (0.286)                 &     (0.257)                 &     (0.221)                 \\\addlinespace
$wL_{c,t}$&       0.421$^{\ast}$        &       0.266                 &       0.454                 &       0.486$^{\ast}$        &      -0.645$^{\ast}$        &       0.085                 &       0.098                 &      -0.828$^{\ast\ast\ast}$&       0.995$^{\ast\ast}$    &       0.891$^{\ast}$        &      -1.936$^{\ast\ast\ast}$\\
            &     (0.162)                 &     (0.148)                 &     (0.351)                 &     (0.201)                 &     (0.243)                 &     (0.096)                 &     (0.177)                 &     (0.053)                 &     (0.296)                 &     (0.361)                 &     (0.271)                 \\\addlinespace
$rK_{c,t}$&      -0.053                 &       0.210                 &      -0.466$^{\ast}$        &      -0.047                 &      -0.765$^{\ast\ast}$    &       0.112                 &      -0.034                 &      -0.843$^{\ast\ast\ast}$&       1.208$^{\ast\ast}$    &       0.548                 &      -1.801$^{\ast\ast\ast}$\\
            &     (0.128)                 &     (0.228)                 &     (0.173)                 &     (0.144)                 &     (0.265)                 &     (0.144)                 &     (0.157)                 &     (0.046)                 &     (0.312)                 &     (0.277)                 &     (0.291)                 \\\addlinespace
$pQ_{c,t}$&       0.557                 &       0.557                 &       0.574                 &       0.587$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.267)                 &     (0.323)                 &     (0.533)                 &     (0.255)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.000                 &      -0.005                 &      -0.006                 &       0.008$^{\ast}$        &      -0.143                 &      -0.100$^{\ast}$        &      -0.036                 &      -0.007                 &      -0.116                 &      -0.014                 &       0.118                 \\
            &     (0.003)                 &     (0.004)                 &     (0.007)                 &     (0.003)                 &     (0.070)                 &     (0.040)                 &     (0.038)                 &     (0.015)                 &     (0.066)                 &     (0.061)                 &     (0.074)                 \\\addlinespace
$Services_{c,t}$&       0.010                 &       0.050$^{\ast\ast}$    &      -0.044                 &       0.010                 &       0.178$^{\ast}$        &       0.393$^{\ast\ast\ast}$&      -0.229$^{\ast\ast}$    &       0.014                 &       1.149$^{\ast\ast\ast}$&      -0.938$^{\ast\ast}$    &      -0.229                 \\
            &     (0.009)                 &     (0.011)                 &     (0.022)                 &     (0.013)                 &     (0.065)                 &     (0.054)                 &     (0.079)                 &     (0.024)                 &     (0.193)                 &     (0.213)                 &     (0.126)                 \\\addlinespace
$HHI_{c,t}$&      -0.181                 &       7.356$^{\ast\ast\ast}$&      -9.693$^{\ast\ast\ast}$&      -0.809                 &       3.429                 &      58.719$^{\ast\ast}$    &     -56.126$^{\ast\ast\ast}$&       0.836                 &     203.464$^{\ast\ast\ast}$&    -203.918$^{\ast\ast\ast}$&      -1.281                 \\
            &     (0.969)                 &     (1.417)                 &     (1.936)                 &     (1.831)                 &    (21.374)                 &    (13.088)                 &    (11.241)                 &     (3.604)                 &    (26.785)                 &    (20.504)                 &    (25.856)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001                 &      -0.002                 &      -0.001                 &       0.006                 &      -0.039                 &      -0.056                 &       0.010                 &       0.007                 &      -0.117$^{\ast\ast}$    &       0.066                 &       0.054                 \\
            &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.004)                 &     (0.066)                 &     (0.028)                 &     (0.041)                 &     (0.006)                 &     (0.041)                 &     (0.083)                 &     (0.074)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.000                 &       0.048                 &      -0.026                 &      -0.037                 &       0.596                 &       0.866$^{\ast}$        &      -0.339                 &       0.068                 &       1.894$^{\ast\ast}$    &      -1.557                 &      -0.345                 \\
            &     (0.009)                 &     (0.027)                 &     (0.047)                 &     (0.055)                 &     (0.901)                 &     (0.338)                 &     (0.576)                 &     (0.111)                 &     (0.496)                 &     (1.200)                 &     (0.965)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003                 &       0.002                 &       0.010$^{\ast}$        &       0.000                 &       0.048                 &      -0.004                 &       0.064                 &      -0.012                 &      -0.066                 &       0.173                 &      -0.102                 \\
            &     (0.002)                 &     (0.003)                 &     (0.005)                 &     (0.003)                 &     (0.069)                 &     (0.052)                 &     (0.042)                 &     (0.014)                 &     (0.082)                 &     (0.105)                 &     (0.096)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.013                 &       0.015                 &       0.031                 &      -0.001                 &       0.413                 &       0.227                 &       0.180                 &       0.006                 &       0.180                 &       0.241                 &      -0.403                 \\
            &     (0.012)                 &     (0.015)                 &     (0.022)                 &     (0.016)                 &     (0.199)                 &     (0.160)                 &     (0.100)                 &     (0.053)                 &     (0.294)                 &     (0.264)                 &     (0.368)                 \\\addlinespace
$XRate_{c,t}$&      -0.001                 &       0.004$^{\ast}$        &      -0.004                 &      -0.004                 &      -0.016                 &       0.036                 &      -0.033                 &      -0.019                 &       0.154$^{\ast\ast}$    &      -0.106                 &      -0.054                 \\
            &     (0.003)                 &     (0.002)                 &     (0.005)                 &     (0.004)                 &     (0.085)                 &     (0.029)                 &     (0.043)                 &     (0.028)                 &     (0.051)                 &     (0.083)                 &     (0.036)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .962                 &        .978                 &        .867                 &        .986                 &        .973                 &        .931                 &        .958                 \\
$N$      &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 \\


==> inputs/east_95_16/Results2shortEXCGDPV1_RICTint_ct_East_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{8}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.017                 &      -0.036$^{\ast}$        &       0.054                 &      -0.047                 &      -1.207                 &       2.046$^{\ast}$        &      -0.763                 \\
            &     (0.021)                 &     (0.014)                 &     (0.052)                 &     (0.029)                 &     (0.583)                 &     (0.817)                 &     (0.473)                 \\\addlinespace
$ICT_{c,t}$&      -0.008                 &       0.120                 &      -0.173                 &      -0.035                 &       4.590$^{\ast}$        &      -2.596                 &      -1.982                 \\
            &     (0.049)                 &     (0.076)                 &     (0.108)                 &     (0.057)                 &     (1.737)                 &     (1.548)                 &     (1.592)                 \\\addlinespace
$R*ICT_{c,t}$&       0.011                 &      -0.024                 &       0.033                 &       0.034$^{\ast\ast}$    &      -1.084$^{\ast\ast}$    &       0.666$^{\ast}$        &       0.411                 \\
            &     (0.008)                 &     (0.014)                 &     (0.017)                 &     (0.012)                 &     (0.286)                 &     (0.257)                 &     (0.221)                 \\\addlinespace
$wL_{c,t}$&       0.421$^{\ast}$        &       0.266                 &       0.454                 &       0.486$^{\ast}$        &       0.995$^{\ast\ast}$    &       0.891$^{\ast}$        &      -1.936$^{\ast\ast\ast}$\\
            &     (0.162)                 &     (0.148)                 &     (0.351)                 &     (0.201)                 &     (0.296)                 &     (0.361)                 &     (0.271)                 \\\addlinespace
$rK_{c,t}$&      -0.053                 &       0.210                 &      -0.466$^{\ast}$        &      -0.047                 &       1.208$^{\ast\ast}$    &       0.548                 &      -1.801$^{\ast\ast\ast}$\\
            &     (0.128)                 &     (0.228)                 &     (0.173)                 &     (0.144)                 &     (0.312)                 &     (0.277)                 &     (0.291)                 \\\addlinespace
$pQ_{c,t}$&       0.557                 &       0.557                 &       0.574                 &       0.587$^{\ast}$        &                             &                             &                             \\
            &     (0.267)                 &     (0.323)                 &     (0.533)                 &     (0.255)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .973                 &        .931                 &        .958                 \\
$N$      &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 \\


==> inputs/east_95_16/Results2shortEXCGDPV2_RICTint_ct_East_95t16.tex <==
& $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{4}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -1.207                 &       2.046$^{\ast}$        &      -0.763                 \\
            &     (0.583)                 &     (0.817)                 &     (0.473)                 \\\addlinespace
$ICT_{c,t}$&       4.590$^{\ast}$        &      -2.596                 &      -1.982                 \\
            &     (1.737)                 &     (1.548)                 &     (1.592)                 \\\addlinespace
$R*ICT_{c,t}$&      -1.084$^{\ast\ast}$    &       0.666$^{\ast}$        &       0.411                 \\
            &     (0.286)                 &     (0.257)                 &     (0.221)                 \\\addlinespace
$wL_{c,t}$&       0.995$^{\ast\ast}$    &       0.891$^{\ast}$        &      -1.936$^{\ast\ast\ast}$\\
            &     (0.296)                 &     (0.361)                 &     (0.271)                 \\\addlinespace
$rK_{c,t}$&       1.208$^{\ast\ast}$    &       0.548                 &      -1.801$^{\ast\ast\ast}$\\
            &     (0.312)                 &     (0.277)                 &     (0.291)                 \\\midrule
$R^{2}$  &        .973                 &        .931                 &        .958                 \\
$N$      &          97                 &          97                 &          97                 \\


==> inputs/east_95_16/Results2shortV1_RICTint_ct_East_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.017                 &      -0.036$^{\ast}$        &       0.054                 &      -0.047                 &       0.100                 &      -0.285                 &       0.570                 &      -0.185$^{\ast\ast\ast}$&      -1.207                 &       2.046$^{\ast}$        &      -0.763                 \\
            &     (0.021)                 &     (0.014)                 &     (0.052)                 &     (0.029)                 &     (0.471)                 &     (0.206)                 &     (0.362)                 &     (0.038)                 &     (0.583)                 &     (0.817)                 &     (0.473)                 \\\addlinespace
$ICT_{c,t}$&      -0.008                 &       0.120                 &      -0.173                 &      -0.035                 &       1.197                 &       1.918                 &      -0.509                 &      -0.211                 &       4.590$^{\ast}$        &      -2.596                 &      -1.982                 \\
            &     (0.049)                 &     (0.076)                 &     (0.108)                 &     (0.057)                 &     (1.598)                 &     (0.998)                 &     (0.793)                 &     (0.316)                 &     (1.737)                 &     (1.548)                 &     (1.592)                 \\\addlinespace
$R*ICT_{c,t}$&       0.011                 &      -0.024                 &       0.033                 &       0.034$^{\ast\ast}$    &      -0.164                 &      -0.402$^{\ast}$        &       0.153                 &       0.085                 &      -1.084$^{\ast\ast}$    &       0.666$^{\ast}$        &       0.411                 \\
            &     (0.008)                 &     (0.014)                 &     (0.017)                 &     (0.012)                 &     (0.276)                 &     (0.164)                 &     (0.125)                 &     (0.049)                 &     (0.286)                 &     (0.257)                 &     (0.221)                 \\\addlinespace
$wL_{c,t}$&       0.421$^{\ast}$        &       0.266                 &       0.454                 &       0.486$^{\ast}$        &      -0.645$^{\ast}$        &       0.085                 &       0.098                 &      -0.828$^{\ast\ast\ast}$&       0.995$^{\ast\ast}$    &       0.891$^{\ast}$        &      -1.936$^{\ast\ast\ast}$\\
            &     (0.162)                 &     (0.148)                 &     (0.351)                 &     (0.201)                 &     (0.243)                 &     (0.096)                 &     (0.177)                 &     (0.053)                 &     (0.296)                 &     (0.361)                 &     (0.271)                 \\\addlinespace
$rK_{c,t}$&      -0.053                 &       0.210                 &      -0.466$^{\ast}$        &      -0.047                 &      -0.765$^{\ast\ast}$    &       0.112                 &      -0.034                 &      -0.843$^{\ast\ast\ast}$&       1.208$^{\ast\ast}$    &       0.548                 &      -1.801$^{\ast\ast\ast}$\\
            &     (0.128)                 &     (0.228)                 &     (0.173)                 &     (0.144)                 &     (0.265)                 &     (0.144)                 &     (0.157)                 &     (0.046)                 &     (0.312)                 &     (0.277)                 &     (0.291)                 \\\addlinespace
$pQ_{c,t}$&       0.557                 &       0.557                 &       0.574                 &       0.587$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.267)                 &     (0.323)                 &     (0.533)                 &     (0.255)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .962                 &        .978                 &        .867                 &        .986                 &        .973                 &        .931                 &        .958                 \\
$N$      &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 \\


==> inputs/east_95_16/Results2shortV2_RICTint_ct_East_95t16.tex <==
&\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{8}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &       0.100                 &      -0.285                 &       0.570                 &      -0.185$^{\ast\ast\ast}$&      -1.207                 &       2.046$^{\ast}$        &      -0.763                 \\
            &     (0.471)                 &     (0.206)                 &     (0.362)                 &     (0.038)                 &     (0.583)                 &     (0.817)                 &     (0.473)                 \\\addlinespace
$ICT_{c,t}$&       1.197                 &       1.918                 &      -0.509                 &      -0.211                 &       4.590$^{\ast}$        &      -2.596                 &      -1.982                 \\
            &     (1.598)                 &     (0.998)                 &     (0.793)                 &     (0.316)                 &     (1.737)                 &     (1.548)                 &     (1.592)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.164                 &      -0.402$^{\ast}$        &       0.153                 &       0.085                 &      -1.084$^{\ast\ast}$    &       0.666$^{\ast}$        &       0.411                 \\
            &     (0.276)                 &     (0.164)                 &     (0.125)                 &     (0.049)                 &     (0.286)                 &     (0.257)                 &     (0.221)                 \\\addlinespace
$wL_{c,t}$&      -0.645$^{\ast}$        &       0.085                 &       0.098                 &      -0.828$^{\ast\ast\ast}$&       0.995$^{\ast\ast}$    &       0.891$^{\ast}$        &      -1.936$^{\ast\ast\ast}$\\
            &     (0.243)                 &     (0.096)                 &     (0.177)                 &     (0.053)                 &     (0.296)                 &     (0.361)                 &     (0.271)                 \\\addlinespace
$rK_{c,t}$&      -0.765$^{\ast\ast}$    &       0.112                 &      -0.034                 &      -0.843$^{\ast\ast\ast}$&       1.208$^{\ast\ast}$    &       0.548                 &      -1.801$^{\ast\ast\ast}$\\
            &     (0.265)                 &     (0.144)                 &     (0.157)                 &     (0.046)                 &     (0.312)                 &     (0.277)                 &     (0.291)                 \\\midrule
$R^{2}$  &        .962                 &        .978                 &        .867                 &        .986                 &        .973                 &        .931                 &        .958                 \\
$N$      &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 \\


==> inputs/east_95_16/Results3RICTint_cit_East_95t16.tex <==
& ln $wL_{i,c,t}$ & ln $w_{i,c,t}$ & ln $L_{i,c,t}$ & ln $rK_{i,c,t}$ & ln $r_{i,c,t}$ & ln $K_{i,c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{i,c,t}$&      -0.012                 &       0.031                 &      -0.043$^{\ast\ast\ast}$&       0.036                 &       0.002                 &      -0.029                 \\
            &     (0.022)                 &     (0.019)                 &     (0.014)                 &     (0.023)                 &     (0.003)                 &     (0.031)                 \\\addlinespace
$ICT_{i,c,t}$&       0.014                 &      -0.006                 &       0.021                 &       0.021                 &      -0.012$^{\ast\ast\ast}$&       0.043$^{\ast}$        \\
            &     (0.020)                 &     (0.021)                 &     (0.013)                 &     (0.023)                 &     (0.002)                 &     (0.022)                 \\\addlinespace
$R*ICT_{i,c,t}$&      -0.009                 &       0.010                 &      -0.019$^{\ast\ast\ast}$&       0.004                 &       0.002$^{\ast\ast}$    &      -0.016                 \\
            &     (0.007)                 &     (0.007)                 &     (0.004)                 &     (0.007)                 &     (0.001)                 &     (0.009)                 \\\midrule
$R^{2}$  &        .998                 &        .997                 &        .992                 &        .985                 &         .99                 &        .998                 \\
$N$      &         909                 &         909                 &         909                 &         909                 &         814                 &         814                 \\


==> inputs/east_95_16/Results4RICTint_ct_East_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.145$^{\ast\ast\ast}$&       0.053$^{\ast\ast}$    &      -0.113$^{\ast\ast\ast}$&       0.023                 &       0.003                 &       0.216                 &       0.027                 &       0.057$^{\ast}$        \\
            &     (0.018)                 &     (0.015)                 &     (0.022)                 &     (0.017)                 &     (0.002)                 &     (0.394)                 &     (0.016)                 &     (0.026)                 \\\addlinespace
$ICT_{c,t}$&       0.274$^{\ast\ast}$    &      -0.064                 &       0.232$^{\ast\ast}$    &      -0.023                 &       0.009                 &      -5.645$^{\ast\ast}$    &      -0.018                 &       0.008                 \\
            &     (0.090)                 &     (0.040)                 &     (0.068)                 &     (0.034)                 &     (0.009)                 &     (1.662)                 &     (0.038)                 &     (0.058)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.030$^{\ast}$        &       0.005                 &      -0.013                 &      -0.012$^{\ast}$        &      -0.002                 &       0.522                 &       0.002                 &      -0.011                 \\
            &     (0.013)                 &     (0.008)                 &     (0.009)                 &     (0.005)                 &     (0.002)                 &     (0.317)                 &     (0.005)                 &     (0.011)                 \\\midrule
$R^{2}$  &        .999                 &        .998                 &        .948                 &          0.999                &        .945                 &        .978                 &        .767                 &        .825                 \\
$N$      &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 \\


==> inputs/east_95_16/Results4shortRICTint_ct_East_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $Services_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.145$^{\ast\ast\ast}$&       0.053$^{\ast\ast}$    &      -0.113$^{\ast\ast\ast}$&       0.023                 &       0.216                 &       0.057$^{\ast}$        \\
            &     (0.018)                 &     (0.015)                 &     (0.022)                 &     (0.017)                 &     (0.394)                 &     (0.026)                 \\\addlinespace
$ICT_{c,t}$&       0.274$^{\ast\ast}$    &      -0.064                 &       0.232$^{\ast\ast}$    &      -0.023                 &      -5.645$^{\ast\ast}$    &       0.008                 \\
            &     (0.090)                 &     (0.040)                 &     (0.068)                 &     (0.034)                 &     (1.662)                 &     (0.058)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.030$^{\ast}$        &       0.005                 &      -0.013                 &      -0.012$^{\ast}$        &       0.522                 &      -0.011                 \\
            &     (0.013)                 &     (0.008)                 &     (0.009)                 &     (0.005)                 &     (0.317)                 &     (0.011)                 \\\midrule
$R^{2}$  &        .999                 &        .998                 &        .948                 &          0.999                &        .978                 &        .825                 \\
$N$      &          97                 &          97                 &          97                 &          97                 &          97                 &          97                 \\


==> inputs/east_95_16/Results5RICTint_ct_East_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.106$^{\ast\ast\ast}$&      -0.059                 &      -0.086$^{\ast\ast}$    &      -0.084                 &       0.059$^{\ast\ast}$    &      -0.090$^{\ast\ast\ast}$&      -0.009                 &      -0.002                 \\
            &     (0.021)                 &     (0.044)                 &     (0.029)                 &     (0.041)                 &     (0.018)                 &     (0.013)                 &     (0.019)                 &     (0.011)                 \\\addlinespace
$ICT_{c,t}$&      -0.016                 &      -0.186                 &      -0.098                 &      -0.026                 &      -0.007                 &      -0.198$^{\ast\ast}$    &       0.049                 &      -0.185$^{\ast\ast}$    \\
            &     (0.061)                 &     (0.113)                 &     (0.067)                 &     (0.102)                 &     (0.038)                 &     (0.050)                 &     (0.035)                 &     (0.048)                 \\\addlinespace
$R*ICT_{c,t}$&       0.010                 &       0.022                 &       0.016                 &       0.008                 &      -0.016                 &       0.036$^{\ast}$        &      -0.024                 &       0.026$^{\ast}$        \\
            &     (0.014)                 &     (0.028)                 &     (0.018)                 &     (0.025)                 &     (0.009)                 &     (0.014)                 &     (0.011)                 &     (0.011)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &        .999                 &        .999                 &          0.999                &        .983                 &          0.999                &        .933                 \\
$N$      &          97                 &          97                 &          97                 &          97                 &          76                 &          76                 &          76                 &          76                 \\


==> inputs/east_subperiod/Results1RICTint_ct_East_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.008                 &       0.018                 &       0.076                 &      -0.047                 &       1.161                 &       0.526                 &       0.733                 &      -0.099                 &       0.048                 &       1.712                 &      -1.633                 \\
            &     (0.013)                 &     (0.039)                 &     (0.056)                 &     (0.023)                 &     (0.969)                 &     (0.408)                 &     (0.528)                 &     (1.063)                 &     (1.804)                 &     (1.217)                 &     (1.768)                 \\\addlinespace
$ICT_{c,t}$&       0.143                 &       0.036                 &       0.285$^{\ast}$        &       0.184$^{\ast}$        &       1.163                 &      -0.387                 &       1.146$^{\ast\ast\ast}$&       0.404                 &      -3.195                 &       3.875$^{\ast}$        &      -0.952                 \\
            &     (0.078)                 &     (0.122)                 &     (0.105)                 &     (0.077)                 &     (3.117)                 &     (1.413)                 &     (0.150)                 &     (1.616)                 &     (5.180)                 &     (1.700)                 &     (2.422)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.011                 &       0.028                 &      -0.018                 &      -0.036                 &       0.960                 &       0.316                 &       0.152                 &       0.492                 &      -0.167                 &      -0.307                 &       0.526                 \\
            &     (0.018)                 &     (0.030)                 &     (0.052)                 &     (0.033)                 &     (0.565)                 &     (0.200)                 &     (0.190)                 &     (0.434)                 &     (0.349)                 &     (0.672)                 &     (0.507)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .977                 &        .982                 &        .932                 &        .936                 &        .959                 &        .949                 &        .944                 \\
$N$      &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 \\


==> inputs/east_subperiod/Results1RICTint_ct_East_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.022                 &      -0.037                 &      -0.014                 &       0.000                 &      -0.524                 &      -0.123                 &       0.115                 &      -0.516                 &       0.291                 &       0.541                 &      -0.861$^{\ast\ast}$    \\
            &     (0.022)                 &     (0.032)                 &     (0.030)                 &     (0.021)                 &     (0.504)                 &     (0.153)                 &     (0.102)                 &     (0.270)                 &     (0.245)                 &     (0.278)                 &     (0.198)                 \\\addlinespace
$ICT_{c,t}$&       0.031                 &       0.030                 &      -0.044                 &       0.060                 &       3.108                 &       1.105                 &       0.295                 &       1.709                 &       0.068                 &      -1.872                 &       1.833                 \\
            &     (0.115)                 &     (0.139)                 &     (0.085)                 &     (0.152)                 &     (1.653)                 &     (1.233)                 &     (0.779)                 &     (1.208)                 &     (2.888)                 &     (2.125)                 &     (3.833)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.002                 &       0.013                 &      -0.029                 &      -0.002                 &      -0.432                 &       0.073                 &      -0.346$^{\ast}$        &      -0.159                 &       0.679                 &      -0.599                 &      -0.031                 \\
            &     (0.018)                 &     (0.022)                 &     (0.020)                 &     (0.024)                 &     (0.232)                 &     (0.172)                 &     (0.132)                 &     (0.204)                 &     (0.508)                 &     (0.363)                 &     (0.725)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .973                 &        .991                 &          .9                 &        .913                 &         .99                 &        .962                 &        .932                 \\
$N$      &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 \\


==> inputs/east_subperiod/Results2RICTint_ct_East_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &       0.007                 &       0.025                 &       0.038                 &      -0.041                 &       1.096$^{\ast}$        &       0.497                 &       0.731                 &      -0.131$^{\ast\ast}$    &       0.037                 &       1.763                 &      -1.672$^{\ast\ast}$    \\
            &     (0.014)                 &     (0.036)                 &     (0.051)                 &     (0.027)                 &     (0.471)                 &     (0.254)                 &     (0.438)                 &     (0.046)                 &     (0.710)                 &     (1.210)                 &     (0.566)                 \\\addlinespace
$ICT_{c,t}$&       0.114                 &       0.086                 &       0.310$^{\ast\ast\ast}$&       0.094                 &       1.952                 &       1.232                 &       0.648                 &       0.072                 &       0.726                 &       1.541$^{\ast\ast}$    &      -2.565$^{\ast\ast}$    \\
            &     (0.074)                 &     (0.093)                 &     (0.053)                 &     (0.092)                 &     (2.608)                 &     (0.839)                 &     (0.689)                 &     (0.694)                 &     (0.834)                 &     (0.379)                 &     (0.674)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.012                 &       0.034                 &      -0.046                 &      -0.034                 &       0.396                 &       0.417$^{\ast\ast}$    &      -0.020                 &      -0.001                 &       0.800                 &      -0.350                 &      -0.408                 \\
            &     (0.014)                 &     (0.021)                 &     (0.037)                 &     (0.026)                 &     (0.266)                 &     (0.106)                 &     (0.201)                 &     (0.104)                 &     (0.395)                 &     (0.622)                 &     (0.346)                 \\\addlinespace
$wL_{c,t}$&       0.099                 &      -0.107                 &      -0.515                 &       0.393                 &      -1.203$^{\ast\ast}$    &       0.182$^{\ast\ast}$    &      -0.354                 &      -1.032$^{\ast\ast\ast}$&       1.966$^{\ast\ast}$    &      -0.048                 &      -1.939$^{\ast\ast\ast}$\\
            &     (0.059)                 &     (0.121)                 &     (0.377)                 &     (0.189)                 &     (0.282)                 &     (0.043)                 &     (0.273)                 &     (0.088)                 &     (0.536)                 &     (0.635)                 &     (0.143)                 \\\addlinespace
$rK_{c,t}$&      -0.188                 &       0.609                 &      -1.684$^{\ast}$        &      -0.218                 &      -1.076$^{\ast\ast}$    &       0.430$^{\ast\ast\ast}$&      -0.428                 &      -1.078$^{\ast\ast\ast}$&       2.558$^{\ast\ast}$    &      -0.406                 &      -2.177$^{\ast\ast\ast}$\\
            &     (0.173)                 &     (0.354)                 &     (0.750)                 &     (0.351)                 &     (0.308)                 &     (0.042)                 &     (0.304)                 &     (0.098)                 &     (0.595)                 &     (0.727)                 &     (0.211)                 \\\addlinespace
$pQ_{c,t}$&       0.572                 &       0.567                 &       2.668$^{\ast}$        &      -0.217                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.303)                 &     (0.397)                 &     (1.032)                 &     (0.576)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.002                 &      -0.008                 &       0.013                 &       0.006                 &      -0.171$^{\ast}$        &      -0.127$^{\ast}$        &      -0.032                 &      -0.012                 &      -0.159                 &       0.021                 &       0.130                 \\
            &     (0.003)                 &     (0.006)                 &     (0.009)                 &     (0.006)                 &     (0.068)                 &     (0.058)                 &     (0.065)                 &     (0.009)                 &     (0.143)                 &     (0.181)                 &     (0.073)                 \\\addlinespace
$Services_{c,t}$&       0.015$^{\ast}$        &       0.064$^{\ast\ast\ast}$&       0.012                 &      -0.019                 &       0.472                 &       0.608$^{\ast\ast\ast}$&      -0.152                 &       0.016                 &       1.360$^{\ast\ast}$    &      -0.748                 &      -0.624                 \\
            &     (0.006)                 &     (0.010)                 &     (0.032)                 &     (0.020)                 &     (0.316)                 &     (0.040)                 &     (0.277)                 &     (0.052)                 &     (0.367)                 &     (0.658)                 &     (0.313)                 \\\addlinespace
$HHI_{c,t}$&      -0.116                 &       4.020$^{\ast\ast\ast}$&      -1.969                 &      -2.229                 &      16.404                 &      22.740$^{\ast}$        &     -20.945                 &      14.609                 &      68.966$^{\ast\ast}$    &     -98.584$^{\ast}$        &      28.860                 \\
            &     (0.582)                 &     (0.838)                 &     (2.267)                 &     (1.604)                 &    (26.332)                 &     (9.184)                 &    (16.827)                 &     (8.089)                 &    (23.681)                 &    (44.890)                 &    (20.729)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.006$^{\ast}$        &       0.007                 &      -0.001                 &      -0.080                 &      -0.087$^{\ast}$        &       0.014                 &      -0.006                 &      -0.167$^{\ast}$        &       0.111                 &       0.047                 \\
            &     (0.001)                 &     (0.003)                 &     (0.005)                 &     (0.003)                 &     (0.038)                 &     (0.037)                 &     (0.037)                 &     (0.011)                 &     (0.065)                 &     (0.107)                 &     (0.047)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.025                 &       0.087                 &      -0.183                 &      -0.021                 &       0.309                 &       1.023                 &      -1.076                 &       0.362                 &       2.743$^{\ast}$        &      -3.513                 &       0.976                 \\
            &     (0.027)                 &     (0.065)                 &     (0.131)                 &     (0.048)                 &     (0.670)                 &     (0.642)                 &     (0.627)                 &     (0.183)                 &     (1.138)                 &     (1.756)                 &     (0.790)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.004                 &      -0.003                 &       0.019$^{\ast\ast}$    &       0.002                 &       0.054                 &      -0.041                 &       0.102$^{\ast}$        &      -0.007                 &      -0.193                 &       0.290$^{\ast}$        &      -0.097                 \\
            &     (0.002)                 &     (0.005)                 &     (0.006)                 &     (0.002)                 &     (0.042)                 &     (0.051)                 &     (0.041)                 &     (0.012)                 &     (0.148)                 &     (0.122)                 &     (0.053)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.020$^{\ast}$        &       0.016                 &       0.019                 &       0.015                 &       0.669$^{\ast\ast\ast}$&       0.342$^{\ast\ast}$    &       0.382$^{\ast\ast}$    &      -0.055                 &       0.156                 &       0.833$^{\ast}$        &      -0.936$^{\ast\ast}$    \\
            &     (0.008)                 &     (0.013)                 &     (0.028)                 &     (0.019)                 &     (0.112)                 &     (0.098)                 &     (0.115)                 &     (0.080)                 &     (0.454)                 &     (0.362)                 &     (0.272)                 \\\addlinespace
$XRate_{c,t}$&      -0.001                 &      -0.036$^{\ast\ast}$    &       0.034                 &       0.012                 &      -0.572$^{\ast\ast}$    &      -0.515$^{\ast\ast}$    &      -0.017                 &      -0.039                 &      -0.874$^{\ast\ast}$    &       0.409                 &       0.439$^{\ast\ast}$    \\
            &     (0.006)                 &     (0.013)                 &     (0.027)                 &     (0.014)                 &     (0.131)                 &     (0.144)                 &     (0.126)                 &     (0.059)                 &     (0.310)                 &     (0.390)                 &     (0.124)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .989                 &        .992                 &        .946                 &        .995                 &        .987                 &        .956                 &        .987                 \\
$N$      &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 \\


==> inputs/east_subperiod/Results2RICTint_ct_East_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &       0.028                 &       0.027                 &       0.030                 &       0.041                 &       0.636                 &       0.319                 &       0.512$^{\ast\ast}$    &      -0.194                 &       0.526                 &       0.849$^{\ast}$        &      -1.412$^{\ast\ast}$    \\
            &     (0.014)                 &     (0.020)                 &     (0.031)                 &     (0.028)                 &     (0.305)                 &     (0.169)                 &     (0.136)                 &     (0.157)                 &     (0.309)                 &     (0.316)                 &     (0.351)                 \\\addlinespace
$ICT_{c,t}$&      -0.115                 &      -0.126                 &      -0.345$^{\ast\ast}$    &       0.058                 &      -3.927$^{\ast}$        &      -1.601                 &      -2.148                 &      -0.178                 &      -1.438                 &      -3.874                 &       5.382                 \\
            &     (0.094)                 &     (0.095)                 &     (0.111)                 &     (0.069)                 &     (1.804)                 &     (1.014)                 &     (1.122)                 &     (0.556)                 &     (2.688)                 &     (2.122)                 &     (2.791)                 \\\addlinespace
$R*ICT_{c,t}$&       0.019                 &       0.037$^{\ast}$        &       0.012                 &       0.001                 &       0.519$^{\ast}$        &       0.465$^{\ast\ast}$    &       0.023                 &       0.031                 &       0.960$^{\ast}$        &      -0.196                 &      -0.722                 \\
            &     (0.012)                 &     (0.017)                 &     (0.016)                 &     (0.014)                 &     (0.205)                 &     (0.134)                 &     (0.158)                 &     (0.075)                 &     (0.425)                 &     (0.370)                 &     (0.342)                 \\\addlinespace
$wL_{c,t}$&       0.967$^{\ast\ast\ast}$&       1.277$^{\ast\ast\ast}$&       0.543$^{\ast\ast}$    &       1.008$^{\ast\ast}$    &       0.095                 &       0.312$^{\ast}$        &       0.444$^{\ast\ast\ast}$&      -0.661$^{\ast\ast\ast}$&       0.830$^{\ast}$        &       1.407$^{\ast\ast\ast}$&      -2.253$^{\ast\ast\ast}$\\
            &     (0.167)                 &     (0.164)                 &     (0.142)                 &     (0.276)                 &     (0.188)                 &     (0.144)                 &     (0.084)                 &     (0.062)                 &     (0.342)                 &     (0.186)                 &     (0.193)                 \\\addlinespace
$rK_{c,t}$&       0.240                 &       0.382                 &      -0.256                 &       0.516$^{\ast\ast\ast}$&      -0.277                 &       0.146                 &       0.280$^{\ast\ast\ast}$&      -0.703$^{\ast\ast\ast}$&       0.683$^{\ast}$        &       1.185$^{\ast\ast\ast}$&      -1.880$^{\ast\ast\ast}$\\
            &     (0.115)                 &     (0.215)                 &     (0.154)                 &     (0.082)                 &     (0.178)                 &     (0.129)                 &     (0.054)                 &     (0.053)                 &     (0.311)                 &     (0.135)                 &     (0.181)                 \\\addlinespace
$pQ_{c,t}$&      -0.111                 &      -0.819$^{\ast}$        &       0.508$^{\ast}$        &       0.016                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.242)                 &     (0.335)                 &     (0.227)                 &     (0.266)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.004                 &       0.004                 &      -0.002                 &       0.010$^{\ast\ast}$    &       0.080                 &       0.043                 &       0.009                 &       0.028                 &       0.053                 &      -0.039                 &      -0.018                 \\
            &     (0.003)                 &     (0.003)                 &     (0.006)                 &     (0.003)                 &     (0.080)                 &     (0.025)                 &     (0.038)                 &     (0.030)                 &     (0.053)                 &     (0.071)                 &     (0.048)                 \\\addlinespace
$Services_{c,t}$&       0.006                 &       0.011                 &      -0.018                 &       0.022                 &       0.171                 &       0.317$^{\ast\ast\ast}$&      -0.144                 &      -0.002                 &       0.930$^{\ast\ast\ast}$&      -0.712$^{\ast\ast}$    &      -0.200                 \\
            &     (0.006)                 &     (0.007)                 &     (0.020)                 &     (0.016)                 &     (0.088)                 &     (0.037)                 &     (0.083)                 &     (0.039)                 &     (0.120)                 &     (0.185)                 &     (0.102)                 \\\addlinespace
$HHI_{c,t}$&      -0.522                 &       0.092                 &      -3.379                 &       1.359                 &     -23.448                 &      25.836                 &     -36.984$^{\ast\ast\ast}$&     -12.300$^{\ast}$        &     128.158$^{\ast}$        &    -109.586$^{\ast\ast\ast}$&     -21.499                 \\
            &     (1.423)                 &     (2.304)                 &     (1.994)                 &     (1.762)                 &    (21.753)                 &    (22.306)                 &     (3.717)                 &     (4.547)                 &    (50.501)                 &    (16.102)                 &    (30.946)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.009                 &       0.008                 &       0.017$^{\ast\ast}$    &       0.006                 &       0.286$^{\ast\ast}$    &       0.111$^{\ast}$        &       0.150$^{\ast\ast}$    &       0.024                 &       0.054                 &       0.222$^{\ast}$        &      -0.267$^{\ast}$        \\
            &     (0.005)                 &     (0.005)                 &     (0.006)                 &     (0.006)                 &     (0.082)                 &     (0.051)                 &     (0.042)                 &     (0.018)                 &     (0.102)                 &     (0.092)                 &     (0.110)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.042                 &      -0.013                 &      -0.045                 &      -0.072                 &      -1.060                 &      -0.202                 &      -0.619                 &      -0.239                 &       0.204                 &      -0.820                 &       0.503                 \\
            &     (0.027)                 &     (0.037)                 &     (0.064)                 &     (0.064)                 &     (0.562)                 &     (0.298)                 &     (0.346)                 &     (0.132)                 &     (0.569)                 &     (0.750)                 &     (0.650)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.001                 &       0.002                 &      -0.003                 &       0.003                 &       0.019                 &       0.021                 &      -0.013                 &       0.010                 &       0.042                 &      -0.065                 &       0.027                 \\
            &     (0.002)                 &     (0.004)                 &     (0.004)                 &     (0.005)                 &     (0.047)                 &     (0.044)                 &     (0.026)                 &     (0.014)                 &     (0.126)                 &     (0.080)                 &     (0.091)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.008                 &      -0.003                 &      -0.017                 &      -0.009                 &      -0.244$^{\ast\ast}$    &      -0.052                 &      -0.176$^{\ast\ast\ast}$&      -0.016                 &       0.053                 &      -0.372$^{\ast\ast}$    &       0.308                 \\
            &     (0.005)                 &     (0.004)                 &     (0.010)                 &     (0.010)                 &     (0.080)                 &     (0.087)                 &     (0.037)                 &     (0.041)                 &     (0.263)                 &     (0.132)                 &     (0.183)                 \\\addlinespace
$XRate_{c,t}$&      -0.001                 &       0.004                 &      -0.002                 &      -0.005                 &       0.004                 &       0.071$^{\ast\ast\ast}$&      -0.036                 &      -0.032$^{\ast}$        &       0.251$^{\ast\ast}$    &      -0.126$^{\ast\ast}$    &      -0.121$^{\ast\ast\ast}$\\
            &     (0.002)                 &     (0.002)                 &     (0.004)                 &     (0.006)                 &     (0.046)                 &     (0.013)                 &     (0.021)                 &     (0.014)                 &     (0.059)                 &     (0.040)                 &     (0.024)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .985                 &        .994                 &        .947                 &        .992                 &        .993                 &        .986                 &        .989                 \\
$N$      &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 \\


==> inputs/east_subperiod/Results2shortEXCGDPV1_RICTint_ct_East_08t16.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.007                 &       0.025                 &       0.038                 &      -0.041                 &       0.037                 &       1.763                 &      -1.672$^{\ast\ast}$    \\
            &     (0.014)                 &     (0.036)                 &     (0.051)                 &     (0.027)                 &     (0.710)                 &     (1.210)                 &     (0.566)                 \\\addlinespace
$ICT_{c,t}$&       0.114                 &       0.086                 &       0.310$^{\ast\ast\ast}$&       0.094                 &       0.726                 &       1.541$^{\ast\ast}$    &      -2.565$^{\ast\ast}$    \\
            &     (0.074)                 &     (0.093)                 &     (0.053)                 &     (0.092)                 &     (0.834)                 &     (0.379)                 &     (0.674)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.012                 &       0.034                 &      -0.046                 &      -0.034                 &       0.800                 &      -0.350                 &      -0.408                 \\
            &     (0.014)                 &     (0.021)                 &     (0.037)                 &     (0.026)                 &     (0.395)                 &     (0.622)                 &     (0.346)                 \\\addlinespace
$wL_{c,t}$&       0.099                 &      -0.107                 &      -0.515                 &       0.393                 &       1.966$^{\ast\ast}$    &      -0.048                 &      -1.939$^{\ast\ast\ast}$\\
            &     (0.059)                 &     (0.121)                 &     (0.377)                 &     (0.189)                 &     (0.536)                 &     (0.635)                 &     (0.143)                 \\\addlinespace
$rK_{c,t}$&      -0.188                 &       0.609                 &      -1.684$^{\ast}$        &      -0.218                 &       2.558$^{\ast\ast}$    &      -0.406                 &      -2.177$^{\ast\ast\ast}$\\
            &     (0.173)                 &     (0.354)                 &     (0.750)                 &     (0.351)                 &     (0.595)                 &     (0.727)                 &     (0.211)                 \\\addlinespace
$pQ_{c,t}$&       0.572                 &       0.567                 &       2.668$^{\ast}$        &      -0.217                 &                             &                             &                             \\
            &     (0.303)                 &     (0.397)                 &     (1.032)                 &     (0.576)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .987                 &        .956                 &        .987                 \\
$N$      &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 \\


==> inputs/east_subperiod/Results2shortEXCGDPV1_RICTint_ct_East_95t07.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &       0.028                 &       0.027                 &       0.030                 &       0.041                 &       0.526                 &       0.849$^{\ast}$        &      -1.412$^{\ast\ast}$    \\
            &     (0.014)                 &     (0.020)                 &     (0.031)                 &     (0.028)                 &     (0.309)                 &     (0.316)                 &     (0.351)                 \\\addlinespace
$ICT_{c,t}$&      -0.115                 &      -0.126                 &      -0.345$^{\ast\ast}$    &       0.058                 &      -1.438                 &      -3.874                 &       5.382                 \\
            &     (0.094)                 &     (0.095)                 &     (0.111)                 &     (0.069)                 &     (2.688)                 &     (2.122)                 &     (2.791)                 \\\addlinespace
$R*ICT_{c,t}$&       0.019                 &       0.037$^{\ast}$        &       0.012                 &       0.001                 &       0.960$^{\ast}$        &      -0.196                 &      -0.722                 \\
            &     (0.012)                 &     (0.017)                 &     (0.016)                 &     (0.014)                 &     (0.425)                 &     (0.370)                 &     (0.342)                 \\\addlinespace
$wL_{c,t}$&       0.967$^{\ast\ast\ast}$&       1.277$^{\ast\ast\ast}$&       0.543$^{\ast\ast}$    &       1.008$^{\ast\ast}$    &       0.830$^{\ast}$        &       1.407$^{\ast\ast\ast}$&      -2.253$^{\ast\ast\ast}$\\
            &     (0.167)                 &     (0.164)                 &     (0.142)                 &     (0.276)                 &     (0.342)                 &     (0.186)                 &     (0.193)                 \\\addlinespace
$rK_{c,t}$&       0.240                 &       0.382                 &      -0.256                 &       0.516$^{\ast\ast\ast}$&       0.683$^{\ast}$        &       1.185$^{\ast\ast\ast}$&      -1.880$^{\ast\ast\ast}$\\
            &     (0.115)                 &     (0.215)                 &     (0.154)                 &     (0.082)                 &     (0.311)                 &     (0.135)                 &     (0.181)                 \\\addlinespace
$pQ_{c,t}$&      -0.111                 &      -0.819$^{\ast}$        &       0.508$^{\ast}$        &       0.016                 &                             &                             &                             \\
            &     (0.242)                 &     (0.335)                 &     (0.227)                 &     (0.266)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .993                 &        .986                 &        .989                 \\
$N$      &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 \\


==> inputs/east_subperiod/Results2shortEXCGDPV2_RICTint_ct_East_08t16.tex <==
\multicolumn{4}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.037                 &       1.763                 &      -1.672$^{\ast\ast}$    \\
            &     (0.710)                 &     (1.210)                 &     (0.566)                 \\\addlinespace
$ICT_{c,t}$&       0.726                 &       1.541$^{\ast\ast}$    &      -2.565$^{\ast\ast}$    \\
            &     (0.834)                 &     (0.379)                 &     (0.674)                 \\\addlinespace
$R*ICT_{c,t}$&       0.800                 &      -0.350                 &      -0.408                 \\
            &     (0.395)                 &     (0.622)                 &     (0.346)                 \\\addlinespace
$wL_{c,t}$&       1.966$^{\ast\ast}$    &      -0.048                 &      -1.939$^{\ast\ast\ast}$\\
            &     (0.536)                 &     (0.635)                 &     (0.143)                 \\\addlinespace
$rK_{c,t}$&       2.558$^{\ast\ast}$    &      -0.406                 &      -2.177$^{\ast\ast\ast}$\\
            &     (0.595)                 &     (0.727)                 &     (0.211)                 \\\midrule
$R^{2}$  &        .987                 &        .956                 &        .987                 \\
$N$      &          45                 &          45                 &          45                 \\


==> inputs/east_subperiod/Results2shortEXCGDPV2_RICTint_ct_East_95t07.tex <==
\multicolumn{4}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &       0.526                 &       0.849$^{\ast}$        &      -1.412$^{\ast\ast}$    \\
            &     (0.309)                 &     (0.316)                 &     (0.351)                 \\\addlinespace
$ICT_{c,t}$&      -1.438                 &      -3.874                 &       5.382                 \\
            &     (2.688)                 &     (2.122)                 &     (2.791)                 \\\addlinespace
$R*ICT_{c,t}$&       0.960$^{\ast}$        &      -0.196                 &      -0.722                 \\
            &     (0.425)                 &     (0.370)                 &     (0.342)                 \\\addlinespace
$wL_{c,t}$&       0.830$^{\ast}$        &       1.407$^{\ast\ast\ast}$&      -2.253$^{\ast\ast\ast}$\\
            &     (0.342)                 &     (0.186)                 &     (0.193)                 \\\addlinespace
$rK_{c,t}$&       0.683$^{\ast}$        &       1.185$^{\ast\ast\ast}$&      -1.880$^{\ast\ast\ast}$\\
            &     (0.311)                 &     (0.135)                 &     (0.181)                 \\\midrule
$R^{2}$  &        .993                 &        .986                 &        .989                 \\
$N$      &          52                 &          52                 &          52                 \\


==> inputs/east_subperiod/Results2shortV1_RICTint_ct_East_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.007                 &       0.025                 &       0.038                 &      -0.041                 &       1.096$^{\ast}$        &       0.497                 &       0.731                 &      -0.131$^{\ast\ast}$    &       0.037                 &       1.763                 &      -1.672$^{\ast\ast}$    \\
            &     (0.014)                 &     (0.036)                 &     (0.051)                 &     (0.027)                 &     (0.471)                 &     (0.254)                 &     (0.438)                 &     (0.046)                 &     (0.710)                 &     (1.210)                 &     (0.566)                 \\\addlinespace
$ICT_{c,t}$&       0.114                 &       0.086                 &       0.310$^{\ast\ast\ast}$&       0.094                 &       1.952                 &       1.232                 &       0.648                 &       0.072                 &       0.726                 &       1.541$^{\ast\ast}$    &      -2.565$^{\ast\ast}$    \\
            &     (0.074)                 &     (0.093)                 &     (0.053)                 &     (0.092)                 &     (2.608)                 &     (0.839)                 &     (0.689)                 &     (0.694)                 &     (0.834)                 &     (0.379)                 &     (0.674)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.012                 &       0.034                 &      -0.046                 &      -0.034                 &       0.396                 &       0.417$^{\ast\ast}$    &      -0.020                 &      -0.001                 &       0.800                 &      -0.350                 &      -0.408                 \\
            &     (0.014)                 &     (0.021)                 &     (0.037)                 &     (0.026)                 &     (0.266)                 &     (0.106)                 &     (0.201)                 &     (0.104)                 &     (0.395)                 &     (0.622)                 &     (0.346)                 \\\addlinespace
$wL_{c,t}$&       0.099                 &      -0.107                 &      -0.515                 &       0.393                 &      -1.203$^{\ast\ast}$    &       0.182$^{\ast\ast}$    &      -0.354                 &      -1.032$^{\ast\ast\ast}$&       1.966$^{\ast\ast}$    &      -0.048                 &      -1.939$^{\ast\ast\ast}$\\
            &     (0.059)                 &     (0.121)                 &     (0.377)                 &     (0.189)                 &     (0.282)                 &     (0.043)                 &     (0.273)                 &     (0.088)                 &     (0.536)                 &     (0.635)                 &     (0.143)                 \\\addlinespace
$rK_{c,t}$&      -0.188                 &       0.609                 &      -1.684$^{\ast}$        &      -0.218                 &      -1.076$^{\ast\ast}$    &       0.430$^{\ast\ast\ast}$&      -0.428                 &      -1.078$^{\ast\ast\ast}$&       2.558$^{\ast\ast}$    &      -0.406                 &      -2.177$^{\ast\ast\ast}$\\
            &     (0.173)                 &     (0.354)                 &     (0.750)                 &     (0.351)                 &     (0.308)                 &     (0.042)                 &     (0.304)                 &     (0.098)                 &     (0.595)                 &     (0.727)                 &     (0.211)                 \\\addlinespace
$pQ_{c,t}$&       0.572                 &       0.567                 &       2.668$^{\ast}$        &      -0.217                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.303)                 &     (0.397)                 &     (1.032)                 &     (0.576)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .989                 &        .992                 &        .946                 &        .995                 &        .987                 &        .956                 &        .987                 \\
$N$      &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 \\


==> inputs/east_subperiod/Results2shortV1_RICTint_ct_East_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &       0.028                 &       0.027                 &       0.030                 &       0.041                 &       0.636                 &       0.319                 &       0.512$^{\ast\ast}$    &      -0.194                 &       0.526                 &       0.849$^{\ast}$        &      -1.412$^{\ast\ast}$    \\
            &     (0.014)                 &     (0.020)                 &     (0.031)                 &     (0.028)                 &     (0.305)                 &     (0.169)                 &     (0.136)                 &     (0.157)                 &     (0.309)                 &     (0.316)                 &     (0.351)                 \\\addlinespace
$ICT_{c,t}$&      -0.115                 &      -0.126                 &      -0.345$^{\ast\ast}$    &       0.058                 &      -3.927$^{\ast}$        &      -1.601                 &      -2.148                 &      -0.178                 &      -1.438                 &      -3.874                 &       5.382                 \\
            &     (0.094)                 &     (0.095)                 &     (0.111)                 &     (0.069)                 &     (1.804)                 &     (1.014)                 &     (1.122)                 &     (0.556)                 &     (2.688)                 &     (2.122)                 &     (2.791)                 \\\addlinespace
$R*ICT_{c,t}$&       0.019                 &       0.037$^{\ast}$        &       0.012                 &       0.001                 &       0.519$^{\ast}$        &       0.465$^{\ast\ast}$    &       0.023                 &       0.031                 &       0.960$^{\ast}$        &      -0.196                 &      -0.722                 \\
            &     (0.012)                 &     (0.017)                 &     (0.016)                 &     (0.014)                 &     (0.205)                 &     (0.134)                 &     (0.158)                 &     (0.075)                 &     (0.425)                 &     (0.370)                 &     (0.342)                 \\\addlinespace
$wL_{c,t}$&       0.967$^{\ast\ast\ast}$&       1.277$^{\ast\ast\ast}$&       0.543$^{\ast\ast}$    &       1.008$^{\ast\ast}$    &       0.095                 &       0.312$^{\ast}$        &       0.444$^{\ast\ast\ast}$&      -0.661$^{\ast\ast\ast}$&       0.830$^{\ast}$        &       1.407$^{\ast\ast\ast}$&      -2.253$^{\ast\ast\ast}$\\
            &     (0.167)                 &     (0.164)                 &     (0.142)                 &     (0.276)                 &     (0.188)                 &     (0.144)                 &     (0.084)                 &     (0.062)                 &     (0.342)                 &     (0.186)                 &     (0.193)                 \\\addlinespace
$rK_{c,t}$&       0.240                 &       0.382                 &      -0.256                 &       0.516$^{\ast\ast\ast}$&      -0.277                 &       0.146                 &       0.280$^{\ast\ast\ast}$&      -0.703$^{\ast\ast\ast}$&       0.683$^{\ast}$        &       1.185$^{\ast\ast\ast}$&      -1.880$^{\ast\ast\ast}$\\
            &     (0.115)                 &     (0.215)                 &     (0.154)                 &     (0.082)                 &     (0.178)                 &     (0.129)                 &     (0.054)                 &     (0.053)                 &     (0.311)                 &     (0.135)                 &     (0.181)                 \\\addlinespace
$pQ_{c,t}$&      -0.111                 &      -0.819$^{\ast}$        &       0.508$^{\ast}$        &       0.016                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.242)                 &     (0.335)                 &     (0.227)                 &     (0.266)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .985                 &        .994                 &        .947                 &        .992                 &        .993                 &        .986                 &        .989                 \\
$N$      &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 \\


==> inputs/east_subperiod/Results2shortV2_RICTint_ct_East_08t16.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       1.096$^{\ast}$        &       0.497                 &       0.731                 &      -0.131$^{\ast\ast}$    &       0.037                 &       1.763                 &      -1.672$^{\ast\ast}$    \\
            &     (0.471)                 &     (0.254)                 &     (0.438)                 &     (0.046)                 &     (0.710)                 &     (1.210)                 &     (0.566)                 \\\addlinespace
$ICT_{c,t}$&       1.952                 &       1.232                 &       0.648                 &       0.072                 &       0.726                 &       1.541$^{\ast\ast}$    &      -2.565$^{\ast\ast}$    \\
            &     (2.608)                 &     (0.839)                 &     (0.689)                 &     (0.694)                 &     (0.834)                 &     (0.379)                 &     (0.674)                 \\\addlinespace
$R*ICT_{c,t}$&       0.396                 &       0.417$^{\ast\ast}$    &      -0.020                 &      -0.001                 &       0.800                 &      -0.350                 &      -0.408                 \\
            &     (0.266)                 &     (0.106)                 &     (0.201)                 &     (0.104)                 &     (0.395)                 &     (0.622)                 &     (0.346)                 \\\addlinespace
$wL_{c,t}$&      -1.203$^{\ast\ast}$    &       0.182$^{\ast\ast}$    &      -0.354                 &      -1.032$^{\ast\ast\ast}$&       1.966$^{\ast\ast}$    &      -0.048                 &      -1.939$^{\ast\ast\ast}$\\
            &     (0.282)                 &     (0.043)                 &     (0.273)                 &     (0.088)                 &     (0.536)                 &     (0.635)                 &     (0.143)                 \\\addlinespace
$rK_{c,t}$&      -1.076$^{\ast\ast}$    &       0.430$^{\ast\ast\ast}$&      -0.428                 &      -1.078$^{\ast\ast\ast}$&       2.558$^{\ast\ast}$    &      -0.406                 &      -2.177$^{\ast\ast\ast}$\\
            &     (0.308)                 &     (0.042)                 &     (0.304)                 &     (0.098)                 &     (0.595)                 &     (0.727)                 &     (0.211)                 \\\midrule
$R^{2}$  &        .989                 &        .992                 &        .946                 &        .995                 &        .987                 &        .956                 &        .987                 \\
$N$      &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 \\


==> inputs/east_subperiod/Results2shortV2_RICTint_ct_East_95t07.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &       0.636                 &       0.319                 &       0.512$^{\ast\ast}$    &      -0.194                 &       0.526                 &       0.849$^{\ast}$        &      -1.412$^{\ast\ast}$    \\
            &     (0.305)                 &     (0.169)                 &     (0.136)                 &     (0.157)                 &     (0.309)                 &     (0.316)                 &     (0.351)                 \\\addlinespace
$ICT_{c,t}$&      -3.927$^{\ast}$        &      -1.601                 &      -2.148                 &      -0.178                 &      -1.438                 &      -3.874                 &       5.382                 \\
            &     (1.804)                 &     (1.014)                 &     (1.122)                 &     (0.556)                 &     (2.688)                 &     (2.122)                 &     (2.791)                 \\\addlinespace
$R*ICT_{c,t}$&       0.519$^{\ast}$        &       0.465$^{\ast\ast}$    &       0.023                 &       0.031                 &       0.960$^{\ast}$        &      -0.196                 &      -0.722                 \\
            &     (0.205)                 &     (0.134)                 &     (0.158)                 &     (0.075)                 &     (0.425)                 &     (0.370)                 &     (0.342)                 \\\addlinespace
$wL_{c,t}$&       0.095                 &       0.312$^{\ast}$        &       0.444$^{\ast\ast\ast}$&      -0.661$^{\ast\ast\ast}$&       0.830$^{\ast}$        &       1.407$^{\ast\ast\ast}$&      -2.253$^{\ast\ast\ast}$\\
            &     (0.188)                 &     (0.144)                 &     (0.084)                 &     (0.062)                 &     (0.342)                 &     (0.186)                 &     (0.193)                 \\\addlinespace
$rK_{c,t}$&      -0.277                 &       0.146                 &       0.280$^{\ast\ast\ast}$&      -0.703$^{\ast\ast\ast}$&       0.683$^{\ast}$        &       1.185$^{\ast\ast\ast}$&      -1.880$^{\ast\ast\ast}$\\
            &     (0.178)                 &     (0.129)                 &     (0.054)                 &     (0.053)                 &     (0.311)                 &     (0.135)                 &     (0.181)                 \\\midrule
$R^{2}$  &        .985                 &        .994                 &        .947                 &        .992                 &        .993                 &        .986                 &        .989                 \\
$N$      &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 \\


==> inputs/east_subperiod/Results3RICTint_cit_East_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{i,c,t}$&       0.010                 &       0.017                 &      -0.007                 &      -0.038                 &       0.005                 &      -0.002                 \\
            &     (0.016)                 &     (0.016)                 &     (0.010)                 &     (0.041)                 &     (0.004)                 &     (0.015)                 \\\addlinespace
$ICT_{i,c,t}$&      -0.013                 &      -0.003                 &      -0.010                 &       0.072                 &       0.001                 &       0.011                 \\
            &     (0.017)                 &     (0.019)                 &     (0.018)                 &     (0.058)                 &     (0.009)                 &     (0.043)                 \\\addlinespace
$R*ICT_{i,c,t}$&       0.001                 &       0.006                 &      -0.005                 &      -0.018                 &       0.004$^{\ast\ast}$    &      -0.007                 \\
            &     (0.007)                 &     (0.007)                 &     (0.003)                 &     (0.016)                 &     (0.002)                 &     (0.009)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &        .997                 &        .992                 &        .976                 &          0.999                \\
$N$      &         450                 &         450                 &         450                 &         450                 &         405                 &         405                 \\


==> inputs/east_subperiod/Results3RICTint_cit_East_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{i,c,t}$&      -0.038                 &      -0.029                 &      -0.009                 &      -0.017                 &      -0.004                 &      -0.009                 \\
            &     (0.043)                 &     (0.037)                 &     (0.029)                 &     (0.053)                 &     (0.002)                 &     (0.022)                 \\\addlinespace
$ICT_{i,c,t}$&       0.008                 &      -0.011                 &       0.019                 &      -0.000                 &      -0.007$^{\ast\ast\ast}$&       0.043$^{\ast\ast\ast}$\\
            &     (0.043)                 &     (0.034)                 &     (0.030)                 &     (0.042)                 &     (0.002)                 &     (0.013)                 \\\addlinespace
$R*ICT_{i,c,t}$&       0.030                 &       0.057                 &      -0.027                 &       0.055                 &       0.009$^{\ast}$        &      -0.004                 \\
            &     (0.056)                 &     (0.045)                 &     (0.035)                 &     (0.069)                 &     (0.004)                 &     (0.043)                 \\\midrule
$R^{2}$  &        .998                 &        .997                 &        .992                 &        .984                 &        .993                 &        .998                 \\
$N$      &         459                 &         459                 &         459                 &         459                 &         409                 &         409                 \\


==> inputs/east_subperiod/Results4RICTint_ct_East_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.057$^{\ast}$        &       0.025                 &      -0.031                 &       0.007                 &       0.006                 &      -1.018                 &       0.004                 &       0.006                 \\
            &     (0.025)                 &     (0.026)                 &     (0.023)                 &     (0.026)                 &     (0.004)                 &     (0.502)                 &     (0.004)                 &     (0.008)                 \\\addlinespace
$ICT_{c,t}$&       0.158                 &       0.182$^{\ast\ast}$    &       0.000                 &       0.112                 &      -0.019                 &      -1.852                 &       0.013                 &      -0.033$^{\ast}$        \\
            &     (0.114)                 &     (0.057)                 &     (0.080)                 &     (0.100)                 &     (0.017)                 &     (1.968)                 &     (0.013)                 &     (0.015)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.031$^{\ast\ast\ast}$&      -0.020                 &      -0.038                 &      -0.022                 &       0.007$^{\ast\ast\ast}$&      -0.810$^{\ast\ast}$    &       0.001                 &       0.007$^{\ast}$        \\
            &     (0.006)                 &     (0.030)                 &     (0.018)                 &     (0.021)                 &     (0.001)                 &     (0.212)                 &     (0.002)                 &     (0.003)                 \\\midrule
$R^{2}$  &          0.999                &        .999                 &        .883                 &          0.999                &        .985                 &        .995                 &        .988                 &        .909                 \\
$N$      &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 \\


==> inputs/east_subperiod/Results4RICTint_ct_East_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.118$^{\ast}$        &      -0.021                 &      -0.039                 &      -0.048$^{\ast\ast}$    &      -0.006$^{\ast}$        &       0.102                 &       0.027                 &       0.055$^{\ast\ast}$    \\
            &     (0.045)                 &     (0.014)                 &     (0.054)                 &     (0.016)                 &     (0.003)                 &     (0.405)                 &     (0.020)                 &     (0.019)                 \\\addlinespace
$ICT_{c,t}$&       0.596$^{\ast\ast\ast}$&      -0.165$^{\ast\ast\ast}$&       0.279                 &      -0.043                 &       0.040$^{\ast\ast}$    &     -10.135$^{\ast\ast\ast}$&       0.021                 &       0.128                 \\
            &     (0.107)                 &     (0.027)                 &     (0.135)                 &     (0.060)                 &     (0.014)                 &     (1.581)                 &     (0.047)                 &     (0.066)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.094$^{\ast\ast}$    &       0.028$^{\ast\ast\ast}$&      -0.035                 &       0.012                 &      -0.005                 &       1.121$^{\ast\ast}$    &      -0.006                 &      -0.024$^{\ast}$        \\
            &     (0.022)                 &     (0.002)                 &     (0.034)                 &     (0.011)                 &     (0.003)                 &     (0.377)                 &     (0.006)                 &     (0.010)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &        .947                 &          0.999                &         .98                 &        .991                 &        .824                 &        .933                 \\
$N$      &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 \\


==> inputs/east_subperiod/Results4shortRICTint_ct_East_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.057$^{\ast}$        &       0.025                 &      -0.031                 &       0.007                 &      -1.018                 &       0.006                 \\
            &     (0.025)                 &     (0.026)                 &     (0.023)                 &     (0.026)                 &     (0.502)                 &     (0.008)                 \\\addlinespace
$ICT_{c,t}$&       0.158                 &       0.182$^{\ast\ast}$    &       0.000                 &       0.112                 &      -1.852                 &      -0.033$^{\ast}$        \\
            &     (0.114)                 &     (0.057)                 &     (0.080)                 &     (0.100)                 &     (1.968)                 &     (0.015)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.031$^{\ast\ast\ast}$&      -0.020                 &      -0.038                 &      -0.022                 &      -0.810$^{\ast\ast}$    &       0.007$^{\ast}$        \\
            &     (0.006)                 &     (0.030)                 &     (0.018)                 &     (0.021)                 &     (0.212)                 &     (0.003)                 \\\midrule
$R^{2}$  &          0.999                &        .999                 &        .883                 &          0.999                &        .995                 &        .909                 \\
$N$      &          45                 &          45                 &          45                 &          45                 &          45                 &          45                 \\


==> inputs/east_subperiod/Results4shortRICTint_ct_East_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.118$^{\ast}$        &      -0.021                 &      -0.039                 &      -0.048$^{\ast\ast}$    &       0.102                 &       0.055$^{\ast\ast}$    \\
            &     (0.045)                 &     (0.014)                 &     (0.054)                 &     (0.016)                 &     (0.405)                 &     (0.019)                 \\\addlinespace
$ICT_{c,t}$&       0.596$^{\ast\ast\ast}$&      -0.165$^{\ast\ast\ast}$&       0.279                 &      -0.043                 &     -10.135$^{\ast\ast\ast}$&       0.128                 \\
            &     (0.107)                 &     (0.027)                 &     (0.135)                 &     (0.060)                 &     (1.581)                 &     (0.066)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.094$^{\ast\ast}$    &       0.028$^{\ast\ast\ast}$&      -0.035                 &       0.012                 &       1.121$^{\ast\ast}$    &      -0.024$^{\ast}$        \\
            &     (0.022)                 &     (0.002)                 &     (0.034)                 &     (0.011)                 &     (0.377)                 &     (0.010)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &        .947                 &          0.999                &        .991                 &        .933                 \\
$N$      &          52                 &          52                 &          52                 &          52                 &          52                 &          52                 \\


==> inputs/east_subperiod/Results5RICTint_ct_East_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.032                 &       0.006                 &      -0.016                 &       0.012                 &       0.072$^{\ast\ast}$    &      -0.022                 &       0.019                 &      -0.018$^{\ast}$        \\
            &     (0.036)                 &     (0.040)                 &     (0.031)                 &     (0.036)                 &     (0.022)                 &     (0.010)                 &     (0.016)                 &     (0.006)                 \\\addlinespace
$ICT_{c,t}$&       0.292                 &       0.093                 &       0.164                 &       0.157                 &       0.089                 &      -0.019                 &      -0.065                 &       0.017                 \\
            &     (0.161)                 &     (0.124)                 &     (0.109)                 &     (0.098)                 &     (0.112)                 &     (0.033)                 &     (0.116)                 &     (0.019)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.080$^{\ast}$        &      -0.062$^{\ast\ast}$    &      -0.069$^{\ast}$        &      -0.057$^{\ast}$        &      -0.021                 &      -0.016                 &      -0.006                 &      -0.013$^{\ast}$        \\
            &     (0.032)                 &     (0.019)                 &     (0.026)                 &     (0.022)                 &     (0.009)                 &     (0.008)                 &     (0.017)                 &     (0.005)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &        .917                 &          0.999                &        .985                 \\
$N$      &          45                 &          45                 &          45                 &          45                 &          36                 &          36                 &          36                 &          36                 \\


==> inputs/east_subperiod/Results5RICTint_ct_East_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.181$^{\ast}$        &      -0.040                 &      -0.130$^{\ast}$        &      -0.106                 &      -0.063$^{\ast}$        &      -0.089                 &      -0.055                 &      -0.032$^{\ast}$        \\
            &     (0.066)                 &     (0.038)                 &     (0.052)                 &     (0.063)                 &     (0.023)                 &     (0.046)                 &     (0.028)                 &     (0.013)                 \\\addlinespace
$ICT_{c,t}$&       0.138                 &      -0.542$^{\ast\ast\ast}$&      -0.126                 &      -0.106                 &      -0.031                 &      -0.151                 &       0.144                 &      -0.241$^{\ast\ast}$    \\
            &     (0.134)                 &     (0.117)                 &     (0.117)                 &     (0.160)                 &     (0.064)                 &     (0.093)                 &     (0.080)                 &     (0.043)                 \\\addlinespace
$R*ICT_{c,t}$&       0.000                 &       0.102$^{\ast\ast}$    &       0.045                 &       0.052                 &       0.013                 &       0.021                 &      -0.020                 &       0.043$^{\ast\ast}$    \\
            &     (0.034)                 &     (0.034)                 &     (0.033)                 &     (0.045)                 &     (0.013)                 &     (0.018)                 &     (0.016)                 &     (0.010)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &        .999                 &        .999                 &          0.999                &         .99                 &          0.999                &        .988                 \\
$N$      &          52                 &          52                 &          52                 &          52                 &          40                 &          40                 &          40                 &          40                 \\


==> inputs/north_95_16/Results1RICTint_ct_North_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.025                 &       0.023                 &      -0.010                 &      -0.020                 &       0.684                 &      -0.368$^{\ast\ast}$    &       0.875$^{\ast}$        &       0.177                 &      -1.376$^{\ast\ast\ast}$&       1.165                 &       0.098                 \\
            &     (0.021)                 &     (0.043)                 &     (0.032)                 &     (0.029)                 &     (0.437)                 &     (0.137)                 &     (0.451)                 &     (0.264)                 &     (0.402)                 &     (0.711)                 &     (0.622)                 \\\addlinespace
$ICT_{c,t}$&      -0.007                 &      -0.255                 &      -0.159$^{\ast\ast}$    &       0.084                 &      -0.254                 &       1.247$^{\ast\ast\ast}$&      -2.716$^{\ast\ast\ast}$&       1.215$^{\ast}$        &       3.084$^{\ast\ast}$    &      -5.947$^{\ast\ast\ast}$&       2.706$^{\ast}$        \\
            &     (0.028)                 &     (0.220)                 &     (0.052)                 &     (0.049)                 &     (1.217)                 &     (0.337)                 &     (0.637)                 &     (0.658)                 &     (0.959)                 &     (1.052)                 &     (1.346)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.012                 &       0.140                 &       0.062                 &      -0.050                 &      -0.603                 &      -0.974$^{\ast\ast\ast}$&       1.139$^{\ast}$        &      -0.768                 &      -1.696$^{\ast\ast\ast}$&       2.971$^{\ast\ast\ast}$&      -1.140                 \\
            &     (0.017)                 &     (0.128)                 &     (0.037)                 &     (0.035)                 &     (0.773)                 &     (0.131)                 &     (0.511)                 &     (0.434)                 &     (0.509)                 &     (0.897)                 &     (0.923)                 \\\midrule
$R^{2}$  &          0.999                &        .997                 &        .998                 &        .999                 &        .974                 &        .995                 &        .974                 &        .956                 &        .994                 &        .984                 &        .942                 \\
$N$      &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 \\


==> inputs/north_95_16/Results2RICTint_ct_North_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.010                 &       0.038                 &       0.003                 &      -0.009                 &       0.520                 &      -0.407$^{\ast\ast}$    &       0.826$^{\ast}$        &       0.101                 &      -1.355$^{\ast\ast}$    &       1.220$^{\ast}$        &       0.024                 \\
            &     (0.015)                 &     (0.029)                 &     (0.031)                 &     (0.022)                 &     (0.344)                 &     (0.134)                 &     (0.392)                 &     (0.136)                 &     (0.428)                 &     (0.620)                 &     (0.449)                 \\\addlinespace
$ICT_{c,t}$&      -0.038                 &      -0.255                 &      -0.178$^{\ast\ast}$    &       0.065                 &      -1.883                 &       0.671$^{\ast\ast}$    &      -3.503$^{\ast\ast\ast}$&       0.949                 &       2.665$^{\ast\ast\ast}$&      -6.157$^{\ast\ast\ast}$&       3.256$^{\ast}$        \\
            &     (0.030)                 &     (0.158)                 &     (0.068)                 &     (0.052)                 &     (1.047)                 &     (0.259)                 &     (0.853)                 &     (0.587)                 &     (0.673)                 &     (1.556)                 &     (1.490)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.007                 &       0.113                 &       0.059                 &      -0.049                 &       0.193                 &      -0.735$^{\ast\ast\ast}$&       1.455$^{\ast\ast}$    &      -0.527                 &      -1.636$^{\ast\ast\ast}$&       2.901$^{\ast\ast}$    &      -1.114                 \\
            &     (0.015)                 &     (0.089)                 &     (0.043)                 &     (0.037)                 &     (0.515)                 &     (0.109)                 &     (0.533)                 &     (0.379)                 &     (0.412)                 &     (1.044)                 &     (0.963)                 \\\addlinespace
$wL_{c,t}$&       0.770$^{\ast\ast\ast}$&       1.435$^{\ast\ast\ast}$&       0.799$^{\ast\ast}$    &       0.637$^{\ast\ast\ast}$&      -0.114                 &       0.155                 &       0.260                 &      -0.530$^{\ast\ast}$    &       0.634                 &       0.778                 &      -1.313$^{\ast\ast}$    \\
            &     (0.162)                 &     (0.257)                 &     (0.345)                 &     (0.169)                 &     (0.234)                 &     (0.142)                 &     (0.243)                 &     (0.198)                 &     (0.358)                 &     (0.496)                 &     (0.515)                 \\\addlinespace
$rK_{c,t}$&       0.114$^{\ast}$        &       0.630                 &       0.214$^{\ast}$        &       0.141                 &      -0.523$^{\ast\ast}$    &       0.004                 &       0.053                 &      -0.579$^{\ast\ast\ast}$&       0.507$^{\ast}$        &       0.699                 &      -1.130$^{\ast\ast}$    \\
            &     (0.056)                 &     (0.448)                 &     (0.111)                 &     (0.093)                 &     (0.197)                 &     (0.114)                 &     (0.206)                 &     (0.176)                 &     (0.274)                 &     (0.403)                 &     (0.445)                 \\\addlinespace
$pQ_{c,t}$&      -0.027                 &      -0.935                 &      -0.288                 &       0.064                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.183)                 &     (0.629)                 &     (0.399)                 &     (0.256)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.001                 &      -0.003                 &       0.002                 &       0.000                 &       0.069                 &      -0.017                 &       0.053                 &       0.032$^{\ast\ast}$    &      -0.095$^{\ast\ast}$    &       0.080                 &       0.008                 \\
            &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.001)                 &     (0.045)                 &     (0.016)                 &     (0.037)                 &     (0.011)                 &     (0.037)                 &     (0.052)                 &     (0.042)                 \\\addlinespace
$Services_{c,t}$&       0.001                 &      -0.001                 &       0.006                 &      -0.013$^{\ast}$        &       0.096                 &       0.074                 &       0.074                 &      -0.053                 &       0.094                 &       0.143                 &      -0.293                 \\
            &     (0.004)                 &     (0.017)                 &     (0.011)                 &     (0.006)                 &     (0.181)                 &     (0.065)                 &     (0.179)                 &     (0.053)                 &     (0.208)                 &     (0.259)                 &     (0.173)                 \\\addlinespace
$HHI_{c,t}$&       0.278                 &      -0.451                 &       1.923                 &      -3.190$^{\ast\ast\ast}$&      27.954                 &      20.964$^{\ast}$        &      25.742                 &     -18.753                 &      20.983                 &      42.126                 &     -69.404$^{\ast\ast}$    \\
            &     (0.734)                 &     (2.704)                 &     (1.870)                 &     (0.831)                 &    (28.332)                 &    (10.884)                 &    (30.160)                 &    (12.425)                 &    (37.826)                 &    (41.410)                 &    (26.447)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.000                 &      -0.000                 &       0.000                 &      -0.000                 &       0.026                 &      -0.006                 &       0.029                 &       0.003                 &      -0.025                 &       0.031                 &       0.001                 \\
            &     (0.001)                 &     (0.002)                 &     (0.002)                 &     (0.001)                 &     (0.028)                 &     (0.010)                 &     (0.022)                 &     (0.006)                 &     (0.015)                 &     (0.035)                 &     (0.029)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.001                 &       0.019                 &       0.006                 &      -0.001                 &      -0.284                 &      -0.044                 &      -0.218                 &      -0.022                 &       0.191                 &      -0.167                 &      -0.014                 \\
            &     (0.011)                 &     (0.020)                 &     (0.024)                 &     (0.008)                 &     (0.418)                 &     (0.133)                 &     (0.345)                 &     (0.081)                 &     (0.259)                 &     (0.396)                 &     (0.331)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.005$^{\ast\ast}$    &      -0.006                 &       0.010$^{\ast\ast}$    &       0.003                 &       0.141$^{\ast}$        &      -0.009                 &       0.144$^{\ast\ast}$    &       0.006                 &      -0.115$^{\ast\ast}$    &       0.239$^{\ast\ast\ast}$&      -0.114$^{\ast}$        \\
            &     (0.002)                 &     (0.004)                 &     (0.004)                 &     (0.002)                 &     (0.064)                 &     (0.018)                 &     (0.059)                 &     (0.009)                 &     (0.039)                 &     (0.071)                 &     (0.052)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.026$^{\ast}$        &      -0.027                 &       0.050$^{\ast}$        &       0.016                 &       0.399                 &      -0.024                 &       0.655                 &      -0.232$^{\ast}$        &      -0.227                 &       1.165$^{\ast}$        &      -0.865$^{\ast\ast}$    \\
            &     (0.013)                 &     (0.020)                 &     (0.025)                 &     (0.015)                 &     (0.527)                 &     (0.090)                 &     (0.525)                 &     (0.110)                 &     (0.259)                 &     (0.623)                 &     (0.380)                 \\\addlinespace
$XRate_{c,t}$&       0.011                 &       0.114                 &      -0.001                 &       0.000                 &       0.410                 &       0.403$^{\ast\ast\ast}$&      -0.040                 &       0.047                 &       0.668$^{\ast}$        &      -0.492                 &      -0.210                 \\
            &     (0.007)                 &     (0.063)                 &     (0.022)                 &     (0.005)                 &     (0.295)                 &     (0.086)                 &     (0.379)                 &     (0.083)                 &     (0.332)                 &     (0.614)                 &     (0.293)                 \\\midrule
$R^{2}$  &          0.999                &        .997                 &        .998                 &        .999                 &        .981                 &        .996                 &        .976                 &        .979                 &        .994                 &        .984                 &        .958                 \\
$N$      &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 \\


==> inputs/north_95_16/Results2shortEXCGDPV1_RICTint_ct_North_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{8}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.010                 &       0.038                 &       0.003                 &      -0.009                 &      -1.355$^{\ast\ast}$    &       1.220$^{\ast}$        &       0.024                 \\
            &     (0.015)                 &     (0.029)                 &     (0.031)                 &     (0.022)                 &     (0.428)                 &     (0.620)                 &     (0.449)                 \\\addlinespace
$ICT_{c,t}$&      -0.038                 &      -0.255                 &      -0.178$^{\ast\ast}$    &       0.065                 &       2.665$^{\ast\ast\ast}$&      -6.157$^{\ast\ast\ast}$&       3.256$^{\ast}$        \\
            &     (0.030)                 &     (0.158)                 &     (0.068)                 &     (0.052)                 &     (0.673)                 &     (1.556)                 &     (1.490)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.007                 &       0.113                 &       0.059                 &      -0.049                 &      -1.636$^{\ast\ast\ast}$&       2.901$^{\ast\ast}$    &      -1.114                 \\
            &     (0.015)                 &     (0.089)                 &     (0.043)                 &     (0.037)                 &     (0.412)                 &     (1.044)                 &     (0.963)                 \\\addlinespace
$wL_{c,t}$&       0.770$^{\ast\ast\ast}$&       1.435$^{\ast\ast\ast}$&       0.799$^{\ast\ast}$    &       0.637$^{\ast\ast\ast}$&       0.634                 &       0.778                 &      -1.313$^{\ast\ast}$    \\
            &     (0.162)                 &     (0.257)                 &     (0.345)                 &     (0.169)                 &     (0.358)                 &     (0.496)                 &     (0.515)                 \\\addlinespace
$rK_{c,t}$&       0.114$^{\ast}$        &       0.630                 &       0.214$^{\ast}$        &       0.141                 &       0.507$^{\ast}$        &       0.699                 &      -1.130$^{\ast\ast}$    \\
            &     (0.056)                 &     (0.448)                 &     (0.111)                 &     (0.093)                 &     (0.274)                 &     (0.403)                 &     (0.445)                 \\\addlinespace
$pQ_{c,t}$&      -0.027                 &      -0.935                 &      -0.288                 &       0.064                 &                             &                             &                             \\
            &     (0.183)                 &     (0.629)                 &     (0.399)                 &     (0.256)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &        .997                 &        .998                 &        .999                 &        .994                 &        .984                 &        .958                 \\
$N$      &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 \\


==> inputs/north_95_16/Results2shortEXCGDPV2_RICTint_ct_North_95t16.tex <==
& $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{4}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -1.355$^{\ast\ast}$    &       1.220$^{\ast}$        &       0.024                 \\
            &     (0.428)                 &     (0.620)                 &     (0.449)                 \\\addlinespace
$ICT_{c,t}$&       2.665$^{\ast\ast\ast}$&      -6.157$^{\ast\ast\ast}$&       3.256$^{\ast}$        \\
            &     (0.673)                 &     (1.556)                 &     (1.490)                 \\\addlinespace
$R*ICT_{c,t}$&      -1.636$^{\ast\ast\ast}$&       2.901$^{\ast\ast}$    &      -1.114                 \\
            &     (0.412)                 &     (1.044)                 &     (0.963)                 \\\addlinespace
$wL_{c,t}$&       0.634                 &       0.778                 &      -1.313$^{\ast\ast}$    \\
            &     (0.358)                 &     (0.496)                 &     (0.515)                 \\\addlinespace
$rK_{c,t}$&       0.507$^{\ast}$        &       0.699                 &      -1.130$^{\ast\ast}$    \\
            &     (0.274)                 &     (0.403)                 &     (0.445)                 \\\midrule
$R^{2}$  &        .994                 &        .984                 &        .958                 \\
$N$      &         214                 &         214                 &         214                 \\


==> inputs/north_95_16/Results2shortV1_RICTint_ct_North_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.010                 &       0.038                 &       0.003                 &      -0.009                 &       0.520                 &      -0.407$^{\ast\ast}$    &       0.826$^{\ast}$        &       0.101                 &      -1.355$^{\ast\ast}$    &       1.220$^{\ast}$        &       0.024                 \\
            &     (0.015)                 &     (0.029)                 &     (0.031)                 &     (0.022)                 &     (0.344)                 &     (0.134)                 &     (0.392)                 &     (0.136)                 &     (0.428)                 &     (0.620)                 &     (0.449)                 \\\addlinespace
$ICT_{c,t}$&      -0.038                 &      -0.255                 &      -0.178$^{\ast\ast}$    &       0.065                 &      -1.883                 &       0.671$^{\ast\ast}$    &      -3.503$^{\ast\ast\ast}$&       0.949                 &       2.665$^{\ast\ast\ast}$&      -6.157$^{\ast\ast\ast}$&       3.256$^{\ast}$        \\
            &     (0.030)                 &     (0.158)                 &     (0.068)                 &     (0.052)                 &     (1.047)                 &     (0.259)                 &     (0.853)                 &     (0.587)                 &     (0.673)                 &     (1.556)                 &     (1.490)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.007                 &       0.113                 &       0.059                 &      -0.049                 &       0.193                 &      -0.735$^{\ast\ast\ast}$&       1.455$^{\ast\ast}$    &      -0.527                 &      -1.636$^{\ast\ast\ast}$&       2.901$^{\ast\ast}$    &      -1.114                 \\
            &     (0.015)                 &     (0.089)                 &     (0.043)                 &     (0.037)                 &     (0.515)                 &     (0.109)                 &     (0.533)                 &     (0.379)                 &     (0.412)                 &     (1.044)                 &     (0.963)                 \\\addlinespace
$wL_{c,t}$&       0.770$^{\ast\ast\ast}$&       1.435$^{\ast\ast\ast}$&       0.799$^{\ast\ast}$    &       0.637$^{\ast\ast\ast}$&      -0.114                 &       0.155                 &       0.260                 &      -0.530$^{\ast\ast}$    &       0.634                 &       0.778                 &      -1.313$^{\ast\ast}$    \\
            &     (0.162)                 &     (0.257)                 &     (0.345)                 &     (0.169)                 &     (0.234)                 &     (0.142)                 &     (0.243)                 &     (0.198)                 &     (0.358)                 &     (0.496)                 &     (0.515)                 \\\addlinespace
$rK_{c,t}$&       0.114$^{\ast}$        &       0.630                 &       0.214$^{\ast}$        &       0.141                 &      -0.523$^{\ast\ast}$    &       0.004                 &       0.053                 &      -0.579$^{\ast\ast\ast}$&       0.507$^{\ast}$        &       0.699                 &      -1.130$^{\ast\ast}$    \\
            &     (0.056)                 &     (0.448)                 &     (0.111)                 &     (0.093)                 &     (0.197)                 &     (0.114)                 &     (0.206)                 &     (0.176)                 &     (0.274)                 &     (0.403)                 &     (0.445)                 \\\addlinespace
$pQ_{c,t}$&      -0.027                 &      -0.935                 &      -0.288                 &       0.064                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.183)                 &     (0.629)                 &     (0.399)                 &     (0.256)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &        .997                 &        .998                 &        .999                 &        .981                 &        .996                 &        .976                 &        .979                 &        .994                 &        .984                 &        .958                 \\
$N$      &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 \\


==> inputs/north_95_16/Results2shortV2_RICTint_ct_North_95t16.tex <==
&\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{8}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &       0.520                 &      -0.407$^{\ast\ast}$    &       0.826$^{\ast}$        &       0.101                 &      -1.355$^{\ast\ast}$    &       1.220$^{\ast}$        &       0.024                 \\
            &     (0.344)                 &     (0.134)                 &     (0.392)                 &     (0.136)                 &     (0.428)                 &     (0.620)                 &     (0.449)                 \\\addlinespace
$ICT_{c,t}$&      -1.883                 &       0.671$^{\ast\ast}$    &      -3.503$^{\ast\ast\ast}$&       0.949                 &       2.665$^{\ast\ast\ast}$&      -6.157$^{\ast\ast\ast}$&       3.256$^{\ast}$        \\
            &     (1.047)                 &     (0.259)                 &     (0.853)                 &     (0.587)                 &     (0.673)                 &     (1.556)                 &     (1.490)                 \\\addlinespace
$R*ICT_{c,t}$&       0.193                 &      -0.735$^{\ast\ast\ast}$&       1.455$^{\ast\ast}$    &      -0.527                 &      -1.636$^{\ast\ast\ast}$&       2.901$^{\ast\ast}$    &      -1.114                 \\
            &     (0.515)                 &     (0.109)                 &     (0.533)                 &     (0.379)                 &     (0.412)                 &     (1.044)                 &     (0.963)                 \\\addlinespace
$wL_{c,t}$&      -0.114                 &       0.155                 &       0.260                 &      -0.530$^{\ast\ast}$    &       0.634                 &       0.778                 &      -1.313$^{\ast\ast}$    \\
            &     (0.234)                 &     (0.142)                 &     (0.243)                 &     (0.198)                 &     (0.358)                 &     (0.496)                 &     (0.515)                 \\\addlinespace
$rK_{c,t}$&      -0.523$^{\ast\ast}$    &       0.004                 &       0.053                 &      -0.579$^{\ast\ast\ast}$&       0.507$^{\ast}$        &       0.699                 &      -1.130$^{\ast\ast}$    \\
            &     (0.197)                 &     (0.114)                 &     (0.206)                 &     (0.176)                 &     (0.274)                 &     (0.403)                 &     (0.445)                 \\\midrule
$R^{2}$  &        .981                 &        .996                 &        .976                 &        .979                 &        .994                 &        .984                 &        .958                 \\
$N$      &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 \\


==> inputs/north_95_16/Results3RICTint_cit_North_95t16.tex <==
& ln $wL_{i,c,t}$ & ln $w_{i,c,t}$ & ln $L_{i,c,t}$ & ln $rK_{i,c,t}$ & ln $r_{i,c,t}$ & ln $K_{i,c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{i,c,t}$&      -0.006                 &       0.007                 &      -0.013                 &      -0.012                 &      -0.010                 &       0.057                 \\
            &     (0.036)                 &     (0.009)                 &     (0.033)                 &     (0.047)                 &     (0.010)                 &     (0.037)                 \\\addlinespace
$ICT_{i,c,t}$&       0.006                 &       0.004                 &       0.002                 &       0.029                 &       0.001                 &       0.007                 \\
            &     (0.013)                 &     (0.004)                 &     (0.013)                 &     (0.020)                 &     (0.013)                 &     (0.015)                 \\\addlinespace
$R*ICT_{i,c,t}$&      -0.002                 &       0.005$^{\ast}$        &      -0.007                 &       0.009                 &      -0.004                 &       0.014$^{\ast}$        \\
            &     (0.008)                 &     (0.002)                 &     (0.008)                 &     (0.012)                 &     (0.003)                 &     (0.008)                 \\\midrule
$R^{2}$  &        .997                 &        .998                 &        .997                 &        .947                 &        .901                 &        .994                 \\
$N$      &        2958                 &        2958                 &        2958                 &        2925                 &        2958                 &        2958                 \\


==> inputs/north_95_16/Results4RICTint_ct_North_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.078$^{\ast\ast\ast}$&      -0.036$^{\ast\ast}$    &      -0.134$^{\ast\ast\ast}$&      -0.034$^{\ast}$        &       0.006                 &      -0.883$^{\ast\ast\ast}$&       0.001                 &      -0.003                 \\
            &     (0.012)                 &     (0.011)                 &     (0.028)                 &     (0.018)                 &     (0.003)                 &     (0.229)                 &     (0.004)                 &     (0.008)                 \\\addlinespace
$ICT_{c,t}$&       0.170$^{\ast\ast}$    &      -0.070                 &       0.034                 &       0.046                 &       0.004                 &       1.564                 &       0.025                 &       0.103$^{\ast\ast}$    \\
            &     (0.061)                 &     (0.040)                 &     (0.116)                 &     (0.073)                 &     (0.009)                 &     (1.811)                 &     (0.014)                 &     (0.034)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.070$^{\ast}$        &       0.036                 &      -0.013                 &       0.004                 &      -0.005                 &       0.289                 &      -0.015                 &      -0.050$^{\ast\ast}$    \\
            &     (0.035)                 &     (0.029)                 &     (0.068)                 &     (0.050)                 &     (0.007)                 &     (0.979)                 &     (0.010)                 &     (0.021)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .945                 &        .999                 &        .919                 &         .96                 &        .935                 &         .92                 \\
$N$      &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 \\


==> inputs/north_95_16/Results4shortRICTint_ct_North_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $Services_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.078$^{\ast\ast\ast}$&      -0.036$^{\ast\ast}$    &      -0.134$^{\ast\ast\ast}$&      -0.034$^{\ast}$        &      -0.883$^{\ast\ast\ast}$&      -0.003                 \\
            &     (0.012)                 &     (0.011)                 &     (0.028)                 &     (0.018)                 &     (0.229)                 &     (0.008)                 \\\addlinespace
$ICT_{c,t}$&       0.170$^{\ast\ast}$    &      -0.070                 &       0.034                 &       0.046                 &       1.564                 &       0.103$^{\ast\ast}$    \\
            &     (0.061)                 &     (0.040)                 &     (0.116)                 &     (0.073)                 &     (1.811)                 &     (0.034)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.070$^{\ast}$        &       0.036                 &      -0.013                 &       0.004                 &       0.289                 &      -0.050$^{\ast\ast}$    \\
            &     (0.035)                 &     (0.029)                 &     (0.068)                 &     (0.050)                 &     (0.979)                 &     (0.021)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .945                 &        .999                 &         .96                 &         .92                 \\
$N$      &         214                 &         214                 &         214                 &         214                 &         214                 &         214                 \\


==> inputs/north_95_16/Results5RICTint_ct_North_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.158$^{\ast\ast\ast}$&      -0.140                 &      -0.166$^{\ast\ast}$    &      -0.141$^{\ast\ast}$    &      -0.029                 &      -0.051$^{\ast\ast\ast}$&      -0.000                 &       0.029$^{\ast\ast}$    \\
            &     (0.038)                 &     (0.078)                 &     (0.058)                 &     (0.052)                 &     (0.019)                 &     (0.006)                 &     (0.015)                 &     (0.011)                 \\\addlinespace
$ICT_{c,t}$&       0.117                 &      -0.038                 &       0.068                 &       0.064                 &      -0.002                 &       0.025$^{\ast\ast}$    &       0.068$^{\ast}$        &      -0.005                 \\
            &     (0.077)                 &     (0.077)                 &     (0.083)                 &     (0.071)                 &     (0.037)                 &     (0.010)                 &     (0.034)                 &     (0.030)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.071                 &      -0.029                 &      -0.066                 &      -0.076                 &      -0.001                 &      -0.022$^{\ast\ast}$    &      -0.043$^{\ast}$        &       0.030                 \\
            &     (0.055)                 &     (0.069)                 &     (0.065)                 &     (0.058)                 &     (0.021)                 &     (0.008)                 &     (0.020)                 &     (0.018)                 \\\midrule
$R^{2}$  &        .998                 &        .993                 &        .997                 &        .997                 &          0.999                &        .992                 &          0.999                &        .885                 \\
$N$      &         214                 &         214                 &         214                 &         214                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/north_subperiod/Results1RICTint_ct_North_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.007                 &      -0.043                 &       0.018                 &      -0.068$^{\ast\ast\ast}$&       0.100                 &       0.186                 &       0.904                 &      -0.989$^{\ast\ast\ast}$&       1.499                 &       0.953                 &      -2.605$^{\ast\ast\ast}$\\
            &     (0.029)                 &     (0.071)                 &     (0.083)                 &     (0.020)                 &     (1.358)                 &     (0.462)                 &     (0.926)                 &     (0.221)                 &     (1.020)                 &     (1.508)                 &     (0.719)                 \\\addlinespace
$ICT_{c,t}$&       0.073                 &       0.381                 &       0.075                 &       0.043                 &      -1.555                 &      -0.462                 &      -0.876                 &      -0.217                 &      -0.792                 &      -0.192                 &       0.506                 \\
            &     (0.063)                 &     (0.250)                 &     (0.157)                 &     (0.033)                 &     (1.830)                 &     (0.545)                 &     (1.597)                 &     (0.275)                 &     (1.947)                 &     (2.511)                 &     (1.597)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.051$^{\ast}$        &      -0.153                 &      -0.082                 &      -0.057$^{\ast\ast\ast}$&      -1.586$^{\ast\ast}$    &      -0.222                 &      -0.434                 &      -0.930$^{\ast\ast\ast}$&       1.782                 &      -0.727                 &      -0.890                 \\
            &     (0.027)                 &     (0.143)                 &     (0.084)                 &     (0.011)                 &     (0.672)                 &     (0.442)                 &     (0.433)                 &     (0.211)                 &     (1.419)                 &     (1.385)                 &     (0.528)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .989                 &        .998                 &        .992                 &        .985                 &        .997                 &        .995                 &        .977                 \\
$N$      &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 \\


==> inputs/north_subperiod/Results1RICTint_ct_North_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.046$^{\ast\ast}$    &       0.103                 &      -0.128$^{\ast\ast\ast}$&      -0.001                 &      -1.067$^{\ast}$        &       0.250                 &      -1.635$^{\ast\ast\ast}$&       0.318                 &       1.408                 &      -3.054$^{\ast\ast}$    &       1.448                 \\
            &     (0.016)                 &     (0.076)                 &     (0.032)                 &     (0.031)                 &     (0.488)                 &     (0.451)                 &     (0.472)                 &     (0.361)                 &     (0.945)                 &     (0.963)                 &     (1.203)                 \\\addlinespace
$ICT_{c,t}$&      -0.012                 &      -0.962$^{\ast}$        &      -0.078                 &       0.027                 &      -0.049                 &       0.428                 &      -1.121                 &       0.644                 &       1.328                 &      -2.963                 &       1.794                 \\
            &     (0.035)                 &     (0.452)                 &     (0.076)                 &     (0.074)                 &     (1.200)                 &     (0.927)                 &     (1.203)                 &     (0.711)                 &     (2.125)                 &     (1.933)                 &     (2.591)                 \\\addlinespace
$R*ICT_{c,t}$&       0.018                 &       0.557$^{\ast\ast}$    &       0.026                 &      -0.015                 &       0.278                 &       0.384                 &       0.200                 &      -0.306                 &       0.707                 &       0.512                 &      -1.251                 \\
            &     (0.023)                 &     (0.238)                 &     (0.046)                 &     (0.046)                 &     (0.790)                 &     (0.585)                 &     (0.739)                 &     (0.485)                 &     (1.334)                 &     (1.190)                 &     (1.659)                 \\\midrule
$R^{2}$  &          0.999                &        .997                 &        .999                 &          0.999                &        .988                 &        .995                 &        .986                 &        .972                 &        .995                 &        .989                 &        .965                 \\
$N$      &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 \\


==> inputs/north_subperiod/Results2RICTint_ct_North_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.040                 &      -0.035                 &      -0.044                 &      -0.113$^{\ast\ast\ast}$&      -0.380                 &      -0.444                 &       0.835                 &      -0.771$^{\ast}$        &       0.308                 &       1.115                 &      -1.714                 \\
            &     (0.035)                 &     (0.070)                 &     (0.093)                 &     (0.016)                 &     (1.170)                 &     (0.532)                 &     (1.209)                 &     (0.381)                 &     (1.779)                 &     (2.310)                 &     (1.162)                 \\\addlinespace
$ICT_{c,t}$&       0.065                 &       0.350                 &       0.049                 &       0.049                 &       0.256                 &       0.198                 &      -0.395                 &       0.454$^{\ast}$        &      -0.410                 &      -1.120                 &       1.275                 \\
            &     (0.065)                 &     (0.213)                 &     (0.140)                 &     (0.045)                 &     (1.942)                 &     (0.955)                 &     (1.562)                 &     (0.207)                 &     (1.832)                 &     (2.363)                 &     (1.669)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.081$^{\ast\ast\ast}$&      -0.141                 &      -0.137$^{\ast\ast}$    &      -0.103$^{\ast\ast\ast}$&      -2.181$^{\ast\ast\ast}$&      -0.736                 &      -0.554                 &      -0.892$^{\ast\ast}$    &       0.944                 &      -0.477                 &      -0.426                 \\
            &     (0.023)                 &     (0.139)                 &     (0.041)                 &     (0.010)                 &     (0.346)                 &     (0.561)                 &     (0.621)                 &     (0.373)                 &     (1.626)                 &     (1.743)                 &     (0.926)                 \\\addlinespace
$wL_{c,t}$&       0.553$^{\ast\ast}$    &      -0.152                 &       1.026                 &       0.779$^{\ast\ast\ast}$&      -0.264                 &       0.295$^{\ast\ast}$    &      -0.120                 &      -0.439$^{\ast}$        &       0.882                 &       0.208                 &      -1.054$^{\ast}$        \\
            &     (0.197)                 &     (0.453)                 &     (0.674)                 &     (0.176)                 &     (0.228)                 &     (0.122)                 &     (0.249)                 &     (0.197)                 &     (0.651)                 &     (0.609)                 &     (0.468)                 \\\addlinespace
$rK_{c,t}$&       0.098                 &       0.234                 &       0.270                 &      -0.005                 &      -0.515$^{\ast\ast}$    &       0.140                 &      -0.179                 &      -0.476$^{\ast\ast}$    &       0.676                 &       0.325                 &      -1.008$^{\ast\ast}$    \\
            &     (0.054)                 &     (0.136)                 &     (0.158)                 &     (0.073)                 &     (0.212)                 &     (0.093)                 &     (0.190)                 &     (0.164)                 &     (0.477)                 &     (0.394)                 &     (0.402)                 \\\addlinespace
$pQ_{c,t}$&      -0.007                 &      -0.632$^{\ast}$        &      -0.382                 &       0.234$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.163)                 &     (0.282)                 &     (0.460)                 &     (0.112)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.000                 &      -0.004$^{\ast}$        &       0.000                 &       0.002                 &      -0.003                 &       0.008                 &      -0.011                 &      -0.000                 &       0.015                 &       0.009                 &      -0.014                 \\
            &     (0.001)                 &     (0.002)                 &     (0.002)                 &     (0.001)                 &     (0.027)                 &     (0.014)                 &     (0.018)                 &     (0.008)                 &     (0.022)                 &     (0.033)                 &     (0.027)                 \\\addlinespace
$Services_{c,t}$&      -0.002                 &      -0.020$^{\ast\ast}$    &       0.028                 &      -0.023                 &       0.565$^{\ast}$        &      -0.018                 &       0.643$^{\ast\ast\ast}$&      -0.060                 &      -0.292                 &       1.005$^{\ast\ast\ast}$&      -0.668$^{\ast\ast}$    \\
            &     (0.006)                 &     (0.008)                 &     (0.020)                 &     (0.013)                 &     (0.253)                 &     (0.057)                 &     (0.185)                 &     (0.088)                 &     (0.222)                 &     (0.222)                 &     (0.267)                 \\\addlinespace
$HHI_{c,t}$&      -0.201                 &      -0.261                 &       4.752                 &      -4.684$^{\ast\ast}$    &      86.496$^{\ast}$        &      -3.083                 &     108.736$^{\ast\ast}$    &     -19.157                 &     -40.405                 &     152.757$^{\ast\ast\ast}$&    -103.938$^{\ast}$        \\
            &     (0.878)                 &     (1.794)                 &     (2.753)                 &     (1.726)                 &    (44.466)                 &    (10.372)                 &    (37.341)                 &    (14.741)                 &    (32.674)                 &    (32.947)                 &    (52.118)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.000                 &      -0.001                 &      -0.001                 &      -0.000                 &       0.002                 &       0.008                 &       0.004                 &      -0.010                 &       0.035$^{\ast}$        &      -0.011                 &      -0.024                 \\
            &     (0.001)                 &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.026)                 &     (0.007)                 &     (0.017)                 &     (0.007)                 &     (0.017)                 &     (0.019)                 &     (0.017)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.020                 &       0.019                 &       0.017                 &       0.060$^{\ast\ast\ast}$&       0.289                 &      -0.177                 &       0.025                 &       0.442$^{\ast\ast}$    &      -0.502                 &      -0.565$^{\ast}$        &       0.955$^{\ast\ast\ast}$\\
            &     (0.012)                 &     (0.019)                 &     (0.019)                 &     (0.015)                 &     (0.324)                 &     (0.139)                 &     (0.099)                 &     (0.159)                 &     (0.469)                 &     (0.259)                 &     (0.255)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003$^{\ast}$        &      -0.002$^{\ast}$        &       0.008$^{\ast\ast}$    &      -0.001                 &       0.097                 &      -0.016                 &       0.120$^{\ast\ast}$    &      -0.006                 &      -0.092$^{\ast}$        &       0.220$^{\ast\ast\ast}$&      -0.118$^{\ast\ast\ast}$\\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.002)                 &     (0.055)                 &     (0.014)                 &     (0.041)                 &     (0.011)                 &     (0.046)                 &     (0.046)                 &     (0.032)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.027$^{\ast}$        &       0.056                 &       0.057$^{\ast}$        &       0.012                 &       1.291$^{\ast}$        &      -0.155                 &       1.368$^{\ast\ast}$    &       0.078                 &      -0.638                 &       1.356$^{\ast}$        &      -0.684                 \\
            &     (0.012)                 &     (0.041)                 &     (0.029)                 &     (0.011)                 &     (0.595)                 &     (0.170)                 &     (0.583)                 &     (0.099)                 &     (0.565)                 &     (0.608)                 &     (0.547)                 \\\addlinespace
$XRate_{c,t}$&       0.025                 &      -0.071                 &       0.064                 &       0.041                 &       1.343                 &       0.349$^{\ast}$        &       0.662                 &       0.332$^{\ast}$        &      -0.482                 &       0.945                 &      -0.347                 \\
            &     (0.026)                 &     (0.042)                 &     (0.054)                 &     (0.027)                 &     (0.975)                 &     (0.164)                 &     (0.899)                 &     (0.150)                 &     (0.525)                 &     (0.918)                 &     (0.629)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .992                 &        .998                 &        .992                 &        .994                 &        .998                 &        .995                 &        .985                 \\
$N$      &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 \\


==> inputs/north_subperiod/Results2RICTint_ct_North_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.029$^{\ast}$        &       0.155                 &      -0.108$^{\ast\ast\ast}$&       0.015                 &      -1.238$^{\ast\ast}$    &       0.168                 &      -1.711$^{\ast\ast\ast}$&       0.305                 &       1.307                 &      -3.084$^{\ast\ast\ast}$&       1.583                 \\
            &     (0.014)                 &     (0.088)                 &     (0.033)                 &     (0.028)                 &     (0.497)                 &     (0.435)                 &     (0.452)                 &     (0.276)                 &     (0.901)                 &     (0.862)                 &     (0.980)                 \\\addlinespace
$ICT_{c,t}$&      -0.029                 &      -0.972$^{\ast\ast}$    &      -0.096                 &       0.028                 &      -0.699                 &       0.181                 &      -1.303                 &       0.423                 &       1.127                 &      -2.800                 &       1.892                 \\
            &     (0.029)                 &     (0.414)                 &     (0.087)                 &     (0.062)                 &     (1.229)                 &     (0.828)                 &     (1.210)                 &     (0.669)                 &     (1.887)                 &     (1.911)                 &     (2.252)                 \\\addlinespace
$R*ICT_{c,t}$&       0.005                 &       0.545$^{\ast}$        &       0.012                 &      -0.016                 &       0.021                 &       0.183                 &      -0.048                 &      -0.115                 &       0.328                 &       0.126                 &      -0.537                 \\
            &     (0.019)                 &     (0.256)                 &     (0.047)                 &     (0.037)                 &     (0.735)                 &     (0.428)                 &     (0.725)                 &     (0.433)                 &     (1.065)                 &     (1.237)                 &     (1.338)                 \\\addlinespace
$wL_{c,t}$&       0.849$^{\ast\ast\ast}$&       1.770$^{\ast\ast\ast}$&       0.958$^{\ast\ast}$    &       0.467$^{\ast\ast}$    &       0.011                 &       0.201                 &       0.340                 &      -0.530$^{\ast}$        &       0.577                 &       0.861                 &      -1.295$^{\ast}$        \\
            &     (0.131)                 &     (0.520)                 &     (0.312)                 &     (0.175)                 &     (0.317)                 &     (0.165)                 &     (0.326)                 &     (0.241)                 &     (0.369)                 &     (0.569)                 &     (0.667)                 \\\addlinespace
$rK_{c,t}$&       0.164$^{\ast\ast}$    &       0.825                 &       0.199                 &       0.289$^{\ast\ast}$    &      -0.307                 &       0.044                 &       0.190                 &      -0.540$^{\ast\ast}$    &       0.374                 &       0.782                 &      -1.009                 \\
            &     (0.066)                 &     (0.480)                 &     (0.127)                 &     (0.097)                 &     (0.277)                 &     (0.157)                 &     (0.292)                 &     (0.229)                 &     (0.349)                 &     (0.507)                 &     (0.635)                 \\\addlinespace
$pQ_{c,t}$&      -0.022                 &      -1.659$^{\ast\ast}$    &       0.032                 &      -0.042                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.155)                 &     (0.641)                 &     (0.285)                 &     (0.316)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.002                 &       0.002                 &       0.009                 &      -0.002                 &       0.069                 &      -0.054                 &       0.052                 &       0.070$^{\ast}$        &      -0.141                 &       0.005                 &       0.097                 \\
            &     (0.003)                 &     (0.007)                 &     (0.007)                 &     (0.005)                 &     (0.092)                 &     (0.075)                 &     (0.072)                 &     (0.032)                 &     (0.132)                 &     (0.108)                 &     (0.143)                 \\\addlinespace
$Services_{c,t}$&       0.012                 &      -0.041                 &       0.012                 &       0.006                 &       0.495                 &       0.157                 &       0.244                 &       0.095                 &       0.028                 &       0.081                 &      -0.145                 \\
            &     (0.007)                 &     (0.028)                 &     (0.017)                 &     (0.007)                 &     (0.271)                 &     (0.122)                 &     (0.231)                 &     (0.052)                 &     (0.281)                 &     (0.325)                 &     (0.215)                 \\\addlinespace
$HHI_{c,t}$&       1.499                 &      -9.179                 &       2.189                 &      -0.169                 &      71.433                 &      27.183                 &      50.057                 &      -5.807                 &      -0.314                 &      61.421                 &     -60.457$^{\ast}$        \\
            &     (1.053)                 &     (5.482)                 &     (2.593)                 &     (1.314)                 &    (45.398)                 &    (15.405)                 &    (39.647)                 &     (9.460)                 &    (37.820)                 &    (46.879)                 &    (32.779)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &       0.000                 &       0.005                 &      -0.005$^{\ast\ast}$    &      -0.001                 &      -0.038                 &       0.026                 &       0.012                 &      -0.094                 &       0.065                 &       0.036                 \\
            &     (0.001)                 &     (0.006)                 &     (0.003)                 &     (0.002)                 &     (0.030)                 &     (0.029)                 &     (0.019)                 &     (0.015)                 &     (0.059)                 &     (0.038)                 &     (0.057)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.016                 &       0.026                 &      -0.010                 &       0.032$^{\ast}$        &       0.428                 &       0.324                 &       0.279                 &      -0.176                 &       0.780                 &       0.153                 &      -0.832                 \\
            &     (0.013)                 &     (0.064)                 &     (0.027)                 &     (0.016)                 &     (0.318)                 &     (0.303)                 &     (0.208)                 &     (0.142)                 &     (0.647)                 &     (0.409)                 &     (0.533)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.005                 &      -0.007                 &       0.008                 &       0.000                 &       0.175                 &      -0.015                 &       0.193                 &      -0.002                 &      -0.105                 &       0.273                 &      -0.139                 \\
            &     (0.004)                 &     (0.008)                 &     (0.010)                 &     (0.002)                 &     (0.144)                 &     (0.041)                 &     (0.138)                 &     (0.022)                 &     (0.090)                 &     (0.207)                 &     (0.135)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.005                 &       0.025                 &      -0.020                 &      -0.001                 &      -0.349                 &       0.052                 &      -0.037                 &      -0.364$^{\ast\ast}$    &       0.520                 &       0.427                 &      -0.742$^{\ast}$        \\
            &     (0.014)                 &     (0.056)                 &     (0.024)                 &     (0.022)                 &     (0.406)                 &     (0.261)                 &     (0.230)                 &     (0.116)                 &     (0.416)                 &     (0.327)                 &     (0.347)                 \\\addlinespace
$XRate_{c,t}$&      -0.001                 &       0.142$^{\ast\ast}$    &      -0.037                 &       0.001                 &       0.006                 &       0.479$^{\ast\ast\ast}$&      -0.489                 &       0.016                 &       1.100$^{\ast\ast\ast}$&      -1.123$^{\ast}$        &       0.021                 \\
            &     (0.005)                 &     (0.061)                 &     (0.021)                 &     (0.007)                 &     (0.185)                 &     (0.118)                 &     (0.278)                 &     (0.057)                 &     (0.334)                 &     (0.519)                 &     (0.226)                 \\\midrule
$R^{2}$  &          0.999                &        .997                 &        .999                 &          0.999                &         .99                 &        .995                 &        .986                 &        .982                 &        .995                 &         .99                 &        .973                 \\
$N$      &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 \\


==> inputs/north_subperiod/Results2shortEXCGDPV1_RICTint_ct_North_08t16.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.040                 &      -0.035                 &      -0.044                 &      -0.113$^{\ast\ast\ast}$&       0.308                 &       1.115                 &      -1.714                 \\
            &     (0.035)                 &     (0.070)                 &     (0.093)                 &     (0.016)                 &     (1.779)                 &     (2.310)                 &     (1.162)                 \\\addlinespace
$ICT_{c,t}$&       0.065                 &       0.350                 &       0.049                 &       0.049                 &      -0.410                 &      -1.120                 &       1.275                 \\
            &     (0.065)                 &     (0.213)                 &     (0.140)                 &     (0.045)                 &     (1.832)                 &     (2.363)                 &     (1.669)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.081$^{\ast\ast\ast}$&      -0.141                 &      -0.137$^{\ast\ast}$    &      -0.103$^{\ast\ast\ast}$&       0.944                 &      -0.477                 &      -0.426                 \\
            &     (0.023)                 &     (0.139)                 &     (0.041)                 &     (0.010)                 &     (1.626)                 &     (1.743)                 &     (0.926)                 \\\addlinespace
$wL_{c,t}$&       0.553$^{\ast\ast}$    &      -0.152                 &       1.026                 &       0.779$^{\ast\ast\ast}$&       0.882                 &       0.208                 &      -1.054$^{\ast}$        \\
            &     (0.197)                 &     (0.453)                 &     (0.674)                 &     (0.176)                 &     (0.651)                 &     (0.609)                 &     (0.468)                 \\\addlinespace
$rK_{c,t}$&       0.098                 &       0.234                 &       0.270                 &      -0.005                 &       0.676                 &       0.325                 &      -1.008$^{\ast\ast}$    \\
            &     (0.054)                 &     (0.136)                 &     (0.158)                 &     (0.073)                 &     (0.477)                 &     (0.394)                 &     (0.402)                 \\\addlinespace
$pQ_{c,t}$&      -0.007                 &      -0.632$^{\ast}$        &      -0.382                 &       0.234$^{\ast}$        &                             &                             &                             \\
            &     (0.163)                 &     (0.282)                 &     (0.460)                 &     (0.112)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .998                 &        .995                 &        .985                 \\
$N$      &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 \\


==> inputs/north_subperiod/Results2shortEXCGDPV1_RICTint_ct_North_95t07.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.029$^{\ast}$        &       0.155                 &      -0.108$^{\ast\ast\ast}$&       0.015                 &       1.307                 &      -3.084$^{\ast\ast\ast}$&       1.583                 \\
            &     (0.014)                 &     (0.088)                 &     (0.033)                 &     (0.028)                 &     (0.901)                 &     (0.862)                 &     (0.980)                 \\\addlinespace
$ICT_{c,t}$&      -0.029                 &      -0.972$^{\ast\ast}$    &      -0.096                 &       0.028                 &       1.127                 &      -2.800                 &       1.892                 \\
            &     (0.029)                 &     (0.414)                 &     (0.087)                 &     (0.062)                 &     (1.887)                 &     (1.911)                 &     (2.252)                 \\\addlinespace
$R*ICT_{c,t}$&       0.005                 &       0.545$^{\ast}$        &       0.012                 &      -0.016                 &       0.328                 &       0.126                 &      -0.537                 \\
            &     (0.019)                 &     (0.256)                 &     (0.047)                 &     (0.037)                 &     (1.065)                 &     (1.237)                 &     (1.338)                 \\\addlinespace
$wL_{c,t}$&       0.849$^{\ast\ast\ast}$&       1.770$^{\ast\ast\ast}$&       0.958$^{\ast\ast}$    &       0.467$^{\ast\ast}$    &       0.577                 &       0.861                 &      -1.295$^{\ast}$        \\
            &     (0.131)                 &     (0.520)                 &     (0.312)                 &     (0.175)                 &     (0.369)                 &     (0.569)                 &     (0.667)                 \\\addlinespace
$rK_{c,t}$&       0.164$^{\ast\ast}$    &       0.825                 &       0.199                 &       0.289$^{\ast\ast}$    &       0.374                 &       0.782                 &      -1.009                 \\
            &     (0.066)                 &     (0.480)                 &     (0.127)                 &     (0.097)                 &     (0.349)                 &     (0.507)                 &     (0.635)                 \\\addlinespace
$pQ_{c,t}$&      -0.022                 &      -1.659$^{\ast\ast}$    &       0.032                 &      -0.042                 &                             &                             &                             \\
            &     (0.155)                 &     (0.641)                 &     (0.285)                 &     (0.316)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &        .997                 &        .999                 &          0.999                &        .995                 &         .99                 &        .973                 \\
$N$      &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 \\


==> inputs/north_subperiod/Results2shortEXCGDPV2_RICTint_ct_North_08t16.tex <==
\multicolumn{4}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.308                 &       1.115                 &      -1.714                 \\
            &     (1.779)                 &     (2.310)                 &     (1.162)                 \\\addlinespace
$ICT_{c,t}$&      -0.410                 &      -1.120                 &       1.275                 \\
            &     (1.832)                 &     (2.363)                 &     (1.669)                 \\\addlinespace
$R*ICT_{c,t}$&       0.944                 &      -0.477                 &      -0.426                 \\
            &     (1.626)                 &     (1.743)                 &     (0.926)                 \\\addlinespace
$wL_{c,t}$&       0.882                 &       0.208                 &      -1.054$^{\ast}$        \\
            &     (0.651)                 &     (0.609)                 &     (0.468)                 \\\addlinespace
$rK_{c,t}$&       0.676                 &       0.325                 &      -1.008$^{\ast\ast}$    \\
            &     (0.477)                 &     (0.394)                 &     (0.402)                 \\\midrule
$R^{2}$  &        .998                 &        .995                 &        .985                 \\
$N$      &          90                 &          90                 &          90                 \\


==> inputs/north_subperiod/Results2shortEXCGDPV2_RICTint_ct_North_95t07.tex <==
\multicolumn{4}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &       1.307                 &      -3.084$^{\ast\ast\ast}$&       1.583                 \\
            &     (0.901)                 &     (0.862)                 &     (0.980)                 \\\addlinespace
$ICT_{c,t}$&       1.127                 &      -2.800                 &       1.892                 \\
            &     (1.887)                 &     (1.911)                 &     (2.252)                 \\\addlinespace
$R*ICT_{c,t}$&       0.328                 &       0.126                 &      -0.537                 \\
            &     (1.065)                 &     (1.237)                 &     (1.338)                 \\\addlinespace
$wL_{c,t}$&       0.577                 &       0.861                 &      -1.295$^{\ast}$        \\
            &     (0.369)                 &     (0.569)                 &     (0.667)                 \\\addlinespace
$rK_{c,t}$&       0.374                 &       0.782                 &      -1.009                 \\
            &     (0.349)                 &     (0.507)                 &     (0.635)                 \\\midrule
$R^{2}$  &        .995                 &         .99                 &        .973                 \\
$N$      &         124                 &         124                 &         124                 \\


==> inputs/north_subperiod/Results2shortV1_RICTint_ct_North_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.040                 &      -0.035                 &      -0.044                 &      -0.113$^{\ast\ast\ast}$&      -0.380                 &      -0.444                 &       0.835                 &      -0.771$^{\ast}$        &       0.308                 &       1.115                 &      -1.714                 \\
            &     (0.035)                 &     (0.070)                 &     (0.093)                 &     (0.016)                 &     (1.170)                 &     (0.532)                 &     (1.209)                 &     (0.381)                 &     (1.779)                 &     (2.310)                 &     (1.162)                 \\\addlinespace
$ICT_{c,t}$&       0.065                 &       0.350                 &       0.049                 &       0.049                 &       0.256                 &       0.198                 &      -0.395                 &       0.454$^{\ast}$        &      -0.410                 &      -1.120                 &       1.275                 \\
            &     (0.065)                 &     (0.213)                 &     (0.140)                 &     (0.045)                 &     (1.942)                 &     (0.955)                 &     (1.562)                 &     (0.207)                 &     (1.832)                 &     (2.363)                 &     (1.669)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.081$^{\ast\ast\ast}$&      -0.141                 &      -0.137$^{\ast\ast}$    &      -0.103$^{\ast\ast\ast}$&      -2.181$^{\ast\ast\ast}$&      -0.736                 &      -0.554                 &      -0.892$^{\ast\ast}$    &       0.944                 &      -0.477                 &      -0.426                 \\
            &     (0.023)                 &     (0.139)                 &     (0.041)                 &     (0.010)                 &     (0.346)                 &     (0.561)                 &     (0.621)                 &     (0.373)                 &     (1.626)                 &     (1.743)                 &     (0.926)                 \\\addlinespace
$wL_{c,t}$&       0.553$^{\ast\ast}$    &      -0.152                 &       1.026                 &       0.779$^{\ast\ast\ast}$&      -0.264                 &       0.295$^{\ast\ast}$    &      -0.120                 &      -0.439$^{\ast}$        &       0.882                 &       0.208                 &      -1.054$^{\ast}$        \\
            &     (0.197)                 &     (0.453)                 &     (0.674)                 &     (0.176)                 &     (0.228)                 &     (0.122)                 &     (0.249)                 &     (0.197)                 &     (0.651)                 &     (0.609)                 &     (0.468)                 \\\addlinespace
$rK_{c,t}$&       0.098                 &       0.234                 &       0.270                 &      -0.005                 &      -0.515$^{\ast\ast}$    &       0.140                 &      -0.179                 &      -0.476$^{\ast\ast}$    &       0.676                 &       0.325                 &      -1.008$^{\ast\ast}$    \\
            &     (0.054)                 &     (0.136)                 &     (0.158)                 &     (0.073)                 &     (0.212)                 &     (0.093)                 &     (0.190)                 &     (0.164)                 &     (0.477)                 &     (0.394)                 &     (0.402)                 \\\addlinespace
$pQ_{c,t}$&      -0.007                 &      -0.632$^{\ast}$        &      -0.382                 &       0.234$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.163)                 &     (0.282)                 &     (0.460)                 &     (0.112)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .992                 &        .998                 &        .992                 &        .994                 &        .998                 &        .995                 &        .985                 \\
$N$      &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 \\


==> inputs/north_subperiod/Results2shortV1_RICTint_ct_North_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.029$^{\ast}$        &       0.155                 &      -0.108$^{\ast\ast\ast}$&       0.015                 &      -1.238$^{\ast\ast}$    &       0.168                 &      -1.711$^{\ast\ast\ast}$&       0.305                 &       1.307                 &      -3.084$^{\ast\ast\ast}$&       1.583                 \\
            &     (0.014)                 &     (0.088)                 &     (0.033)                 &     (0.028)                 &     (0.497)                 &     (0.435)                 &     (0.452)                 &     (0.276)                 &     (0.901)                 &     (0.862)                 &     (0.980)                 \\\addlinespace
$ICT_{c,t}$&      -0.029                 &      -0.972$^{\ast\ast}$    &      -0.096                 &       0.028                 &      -0.699                 &       0.181                 &      -1.303                 &       0.423                 &       1.127                 &      -2.800                 &       1.892                 \\
            &     (0.029)                 &     (0.414)                 &     (0.087)                 &     (0.062)                 &     (1.229)                 &     (0.828)                 &     (1.210)                 &     (0.669)                 &     (1.887)                 &     (1.911)                 &     (2.252)                 \\\addlinespace
$R*ICT_{c,t}$&       0.005                 &       0.545$^{\ast}$        &       0.012                 &      -0.016                 &       0.021                 &       0.183                 &      -0.048                 &      -0.115                 &       0.328                 &       0.126                 &      -0.537                 \\
            &     (0.019)                 &     (0.256)                 &     (0.047)                 &     (0.037)                 &     (0.735)                 &     (0.428)                 &     (0.725)                 &     (0.433)                 &     (1.065)                 &     (1.237)                 &     (1.338)                 \\\addlinespace
$wL_{c,t}$&       0.849$^{\ast\ast\ast}$&       1.770$^{\ast\ast\ast}$&       0.958$^{\ast\ast}$    &       0.467$^{\ast\ast}$    &       0.011                 &       0.201                 &       0.340                 &      -0.530$^{\ast}$        &       0.577                 &       0.861                 &      -1.295$^{\ast}$        \\
            &     (0.131)                 &     (0.520)                 &     (0.312)                 &     (0.175)                 &     (0.317)                 &     (0.165)                 &     (0.326)                 &     (0.241)                 &     (0.369)                 &     (0.569)                 &     (0.667)                 \\\addlinespace
$rK_{c,t}$&       0.164$^{\ast\ast}$    &       0.825                 &       0.199                 &       0.289$^{\ast\ast}$    &      -0.307                 &       0.044                 &       0.190                 &      -0.540$^{\ast\ast}$    &       0.374                 &       0.782                 &      -1.009                 \\
            &     (0.066)                 &     (0.480)                 &     (0.127)                 &     (0.097)                 &     (0.277)                 &     (0.157)                 &     (0.292)                 &     (0.229)                 &     (0.349)                 &     (0.507)                 &     (0.635)                 \\\addlinespace
$pQ_{c,t}$&      -0.022                 &      -1.659$^{\ast\ast}$    &       0.032                 &      -0.042                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.155)                 &     (0.641)                 &     (0.285)                 &     (0.316)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &        .997                 &        .999                 &          0.999                &         .99                 &        .995                 &        .986                 &        .982                 &        .995                 &         .99                 &        .973                 \\
$N$      &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 \\


==> inputs/north_subperiod/Results2shortV2_RICTint_ct_North_08t16.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.380                 &      -0.444                 &       0.835                 &      -0.771$^{\ast}$        &       0.308                 &       1.115                 &      -1.714                 \\
            &     (1.170)                 &     (0.532)                 &     (1.209)                 &     (0.381)                 &     (1.779)                 &     (2.310)                 &     (1.162)                 \\\addlinespace
$ICT_{c,t}$&       0.256                 &       0.198                 &      -0.395                 &       0.454$^{\ast}$        &      -0.410                 &      -1.120                 &       1.275                 \\
            &     (1.942)                 &     (0.955)                 &     (1.562)                 &     (0.207)                 &     (1.832)                 &     (2.363)                 &     (1.669)                 \\\addlinespace
$R*ICT_{c,t}$&      -2.181$^{\ast\ast\ast}$&      -0.736                 &      -0.554                 &      -0.892$^{\ast\ast}$    &       0.944                 &      -0.477                 &      -0.426                 \\
            &     (0.346)                 &     (0.561)                 &     (0.621)                 &     (0.373)                 &     (1.626)                 &     (1.743)                 &     (0.926)                 \\\addlinespace
$wL_{c,t}$&      -0.264                 &       0.295$^{\ast\ast}$    &      -0.120                 &      -0.439$^{\ast}$        &       0.882                 &       0.208                 &      -1.054$^{\ast}$        \\
            &     (0.228)                 &     (0.122)                 &     (0.249)                 &     (0.197)                 &     (0.651)                 &     (0.609)                 &     (0.468)                 \\\addlinespace
$rK_{c,t}$&      -0.515$^{\ast\ast}$    &       0.140                 &      -0.179                 &      -0.476$^{\ast\ast}$    &       0.676                 &       0.325                 &      -1.008$^{\ast\ast}$    \\
            &     (0.212)                 &     (0.093)                 &     (0.190)                 &     (0.164)                 &     (0.477)                 &     (0.394)                 &     (0.402)                 \\\midrule
$R^{2}$  &        .992                 &        .998                 &        .992                 &        .994                 &        .998                 &        .995                 &        .985                 \\
$N$      &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 \\


==> inputs/north_subperiod/Results2shortV2_RICTint_ct_North_95t07.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -1.238$^{\ast\ast}$    &       0.168                 &      -1.711$^{\ast\ast\ast}$&       0.305                 &       1.307                 &      -3.084$^{\ast\ast\ast}$&       1.583                 \\
            &     (0.497)                 &     (0.435)                 &     (0.452)                 &     (0.276)                 &     (0.901)                 &     (0.862)                 &     (0.980)                 \\\addlinespace
$ICT_{c,t}$&      -0.699                 &       0.181                 &      -1.303                 &       0.423                 &       1.127                 &      -2.800                 &       1.892                 \\
            &     (1.229)                 &     (0.828)                 &     (1.210)                 &     (0.669)                 &     (1.887)                 &     (1.911)                 &     (2.252)                 \\\addlinespace
$R*ICT_{c,t}$&       0.021                 &       0.183                 &      -0.048                 &      -0.115                 &       0.328                 &       0.126                 &      -0.537                 \\
            &     (0.735)                 &     (0.428)                 &     (0.725)                 &     (0.433)                 &     (1.065)                 &     (1.237)                 &     (1.338)                 \\\addlinespace
$wL_{c,t}$&       0.011                 &       0.201                 &       0.340                 &      -0.530$^{\ast}$        &       0.577                 &       0.861                 &      -1.295$^{\ast}$        \\
            &     (0.317)                 &     (0.165)                 &     (0.326)                 &     (0.241)                 &     (0.369)                 &     (0.569)                 &     (0.667)                 \\\addlinespace
$rK_{c,t}$&      -0.307                 &       0.044                 &       0.190                 &      -0.540$^{\ast\ast}$    &       0.374                 &       0.782                 &      -1.009                 \\
            &     (0.277)                 &     (0.157)                 &     (0.292)                 &     (0.229)                 &     (0.349)                 &     (0.507)                 &     (0.635)                 \\\midrule
$R^{2}$  &         .99                 &        .995                 &        .986                 &        .982                 &        .995                 &         .99                 &        .973                 \\
$N$      &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 \\


==> inputs/north_subperiod/Results3RICTint_cit_North_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{i,c,t}$&      -0.053$^{\ast\ast}$    &      -0.005                 &      -0.048$^{\ast\ast}$    &       0.003                 &       0.000                 &      -0.023                 \\
            &     (0.022)                 &     (0.012)                 &     (0.020)                 &     (0.074)                 &     (0.004)                 &     (0.023)                 \\\addlinespace
$ICT_{i,c,t}$&      -0.060                 &       0.024                 &      -0.085$^{\ast}$        &      -0.165                 &      -0.011                 &      -0.086                 \\
            &     (0.041)                 &     (0.015)                 &     (0.038)                 &     (0.128)                 &     (0.006)                 &     (0.080)                 \\\addlinespace
$R*ICT_{i,c,t}$&      -0.011                 &      -0.001                 &      -0.010                 &       0.052                 &      -0.002                 &       0.022                 \\
            &     (0.014)                 &     (0.006)                 &     (0.012)                 &     (0.036)                 &     (0.002)                 &     (0.013)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &        .999                 &        .971                 &        .918                 &        .998                 \\
$N$      &        1215                 &        1215                 &        1215                 &        1206                 &        1215                 &        1215                 \\


==> inputs/north_subperiod/Results3RICTint_cit_North_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{i,c,t}$&       0.041                 &       0.010                 &       0.031                 &       0.096                 &       0.002                 &       0.071$^{\ast\ast\ast}$\\
            &     (0.031)                 &     (0.007)                 &     (0.027)                 &     (0.076)                 &     (0.007)                 &     (0.023)                 \\\addlinespace
$ICT_{i,c,t}$&       0.008                 &       0.001                 &       0.007                 &       0.004                 &       0.002                 &       0.019                 \\
            &     (0.009)                 &     (0.005)                 &     (0.011)                 &     (0.034)                 &     (0.015)                 &     (0.017)                 \\\addlinespace
$R*ICT_{i,c,t}$&       0.003                 &      -0.001                 &       0.004                 &      -0.001                 &      -0.001                 &       0.010                 \\
            &     (0.009)                 &     (0.003)                 &     (0.008)                 &     (0.024)                 &     (0.004)                 &     (0.007)                 \\\midrule
$R^{2}$  &        .998                 &        .999                 &        .998                 &        .953                 &         .92                 &        .998                 \\
$N$      &        1742                 &        1742                 &        1742                 &        1718                 &        1742                 &        1742                 \\


==> inputs/north_subperiod/Results4RICTint_ct_North_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.032$^{\ast}$        &      -0.041                 &      -0.017                 &      -0.031                 &       0.007                 &      -0.329                 &       0.010$^{\ast}$        &       0.012$^{\ast\ast}$    \\
            &     (0.017)                 &     (0.041)                 &     (0.041)                 &     (0.021)                 &     (0.005)                 &     (0.721)                 &     (0.005)                 &     (0.005)                 \\\addlinespace
$ICT_{c,t}$&      -0.001                 &       0.038                 &      -0.048                 &       0.068                 &      -0.039$^{\ast\ast}$    &       7.653$^{\ast\ast}$    &      -0.009                 &      -0.013                 \\
            &     (0.010)                 &     (0.052)                 &     (0.074)                 &     (0.052)                 &     (0.013)                 &     (2.442)                 &     (0.006)                 &     (0.010)                 \\\addlinespace
$R*ICT_{c,t}$&       0.015$^{\ast\ast}$    &       0.000                 &       0.033                 &       0.050                 &       0.017$^{\ast\ast\ast}$&      -2.464$^{\ast}$        &      -0.003                 &       0.020$^{\ast}$        \\
            &     (0.006)                 &     (0.035)                 &     (0.058)                 &     (0.030)                 &     (0.005)                 &     (1.164)                 &     (0.005)                 &     (0.009)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .877                 &          0.999                &        .966                 &        .983                 &        .961                 &        .974                 \\
$N$      &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 \\


==> inputs/north_subperiod/Results4RICTint_ct_North_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.037                 &      -0.026                 &      -0.083$^{\ast\ast}$    &       0.023                 &       0.014$^{\ast\ast\ast}$&      -1.947$^{\ast\ast}$    &       0.002                 &      -0.012                 \\
            &     (0.023)                 &     (0.020)                 &     (0.033)                 &     (0.019)                 &     (0.004)                 &     (0.746)                 &     (0.003)                 &     (0.008)                 \\\addlinespace
$ICT_{c,t}$&       0.055                 &      -0.053                 &       0.082                 &      -0.102                 &      -0.010                 &       1.579                 &       0.008                 &       0.099$^{\ast\ast\ast}$\\
            &     (0.053)                 &     (0.037)                 &     (0.097)                 &     (0.072)                 &     (0.008)                 &     (1.827)                 &     (0.009)                 &     (0.023)                 \\\addlinespace
$R*ICT_{c,t}$&       0.022                 &       0.007                 &      -0.006                 &       0.077$^{\ast}$        &       0.006                 &      -1.217                 &      -0.004                 &      -0.034$^{\ast\ast}$    \\
            &     (0.027)                 &     (0.024)                 &     (0.051)                 &     (0.036)                 &     (0.004)                 &     (0.804)                 &     (0.005)                 &     (0.013)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .955                 &          0.999                &        .963                 &        .971                 &        .987                 &        .966                 \\
$N$      &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 \\


==> inputs/north_subperiod/Results4shortRICTint_ct_North_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.032$^{\ast}$        &      -0.041                 &      -0.017                 &      -0.031                 &      -0.329                 &       0.012$^{\ast\ast}$    \\
            &     (0.017)                 &     (0.041)                 &     (0.041)                 &     (0.021)                 &     (0.721)                 &     (0.005)                 \\\addlinespace
$ICT_{c,t}$&      -0.001                 &       0.038                 &      -0.048                 &       0.068                 &       7.653$^{\ast\ast}$    &      -0.013                 \\
            &     (0.010)                 &     (0.052)                 &     (0.074)                 &     (0.052)                 &     (2.442)                 &     (0.010)                 \\\addlinespace
$R*ICT_{c,t}$&       0.015$^{\ast\ast}$    &       0.000                 &       0.033                 &       0.050                 &      -2.464$^{\ast}$        &       0.020$^{\ast}$        \\
            &     (0.006)                 &     (0.035)                 &     (0.058)                 &     (0.030)                 &     (1.164)                 &     (0.009)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .877                 &          0.999                &        .983                 &        .974                 \\
$N$      &          90                 &          90                 &          90                 &          90                 &          90                 &          90                 \\


==> inputs/north_subperiod/Results4shortRICTint_ct_North_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.037                 &      -0.026                 &      -0.083$^{\ast\ast}$    &       0.023                 &      -1.947$^{\ast\ast}$    &      -0.012                 \\
            &     (0.023)                 &     (0.020)                 &     (0.033)                 &     (0.019)                 &     (0.746)                 &     (0.008)                 \\\addlinespace
$ICT_{c,t}$&       0.055                 &      -0.053                 &       0.082                 &      -0.102                 &       1.579                 &       0.099$^{\ast\ast\ast}$\\
            &     (0.053)                 &     (0.037)                 &     (0.097)                 &     (0.072)                 &     (1.827)                 &     (0.023)                 \\\addlinespace
$R*ICT_{c,t}$&       0.022                 &       0.007                 &      -0.006                 &       0.077$^{\ast}$        &      -1.217                 &      -0.034$^{\ast\ast}$    \\
            &     (0.027)                 &     (0.024)                 &     (0.051)                 &     (0.036)                 &     (0.804)                 &     (0.013)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .955                 &          0.999                &        .971                 &        .966                 \\
$N$      &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 \\


==> inputs/north_subperiod/Results5RICTint_ct_North_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.001                 &      -0.082                 &      -0.061                 &      -0.093                 &       0.025                 &      -0.005                 &      -0.003                 &       0.017                 \\
            &     (0.030)                 &     (0.115)                 &     (0.062)                 &     (0.055)                 &     (0.027)                 &     (0.019)                 &     (0.020)                 &     (0.012)                 \\\addlinespace
$ICT_{c,t}$&       0.041                 &      -0.008                 &       0.019                 &       0.018                 &       0.028                 &       0.023                 &      -0.041$^{\ast}$        &       0.038$^{\ast\ast}$    \\
            &     (0.051)                 &     (0.171)                 &     (0.094)                 &     (0.070)                 &     (0.018)                 &     (0.018)                 &     (0.021)                 &     (0.016)                 \\\addlinespace
$R*ICT_{c,t}$&       0.020                 &       0.020                 &       0.014                 &      -0.025                 &       0.030                 &      -0.035$^{\ast\ast}$    &       0.015                 &       0.015                 \\
            &     (0.034)                 &     (0.105)                 &     (0.067)                 &     (0.046)                 &     (0.021)                 &     (0.012)                 &     (0.019)                 &     (0.014)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &          0.999                &        .962                 &          0.999                &        .989                 \\
$N$      &          90                 &          90                 &          90                 &          90                 &          72                 &          72                 &          72                 &          72                 \\


==> inputs/north_subperiod/Results5RICTint_ct_North_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.059$^{\ast}$        &       0.021                 &      -0.025                 &      -0.003                 &      -0.034                 &      -0.045$^{\ast\ast\ast}$&       0.015                 &       0.018                 \\
            &     (0.029)                 &     (0.062)                 &     (0.036)                 &     (0.039)                 &     (0.022)                 &     (0.008)                 &     (0.015)                 &     (0.010)                 \\\addlinespace
$ICT_{c,t}$&      -0.019                 &      -0.189                 &      -0.093                 &      -0.084                 &       0.029                 &       0.019                 &       0.061                 &      -0.025                 \\
            &     (0.094)                 &     (0.168)                 &     (0.116)                 &     (0.114)                 &     (0.056)                 &     (0.013)                 &     (0.045)                 &     (0.016)                 \\\addlinespace
$R*ICT_{c,t}$&       0.038                 &       0.055                 &       0.053                 &       0.045                 &      -0.011                 &      -0.012                 &      -0.007                 &       0.028$^{\ast\ast}$    \\
            &     (0.051)                 &     (0.077)                 &     (0.057)                 &     (0.057)                 &     (0.034)                 &     (0.009)                 &     (0.025)                 &     (0.009)                 \\\midrule
$R^{2}$  &        .999                 &        .997                 &        .999                 &        .999                 &          0.999                &        .992                 &          0.999                &         .92                 \\
$N$      &         124                 &         124                 &         124                 &         124                 &          99                 &          99                 &          99                 &          99                 \\


==> inputs/robustness/CTR_KPMG/Results1RICTint_EUKLEMS_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.000                 &       0.003                 &       0.013                 &      -0.020                 &       0.226                 &       0.246                 &       0.061                 &      -0.082                 &       0.386                 &       0.154                 &      -0.540                 \\
            &     (0.018)                 &     (0.027)                 &     (0.054)                 &     (0.028)                 &     (0.718)                 &     (0.347)                 &     (0.486)                 &     (0.358)                 &     (0.848)                 &     (1.215)                 &     (0.957)                 \\\addlinespace
$ICT_{c,t}$&      -0.015                 &       0.017                 &       0.002                 &      -0.046                 &      -0.849                 &      -0.317                 &       0.431                 &      -0.963                 &      -0.499                 &       2.264                 &      -1.801                 \\
            &     (0.027)                 &     (0.065)                 &     (0.034)                 &     (0.062)                 &     (0.632)                 &     (0.470)                 &     (0.342)                 &     (0.577)                 &     (1.107)                 &     (1.272)                 &     (1.038)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.001                 &      -0.002                 &       0.007                 &      -0.011                 &       0.375                 &       0.056                 &       0.122                 &       0.197                 &       0.340                 &      -0.587                 &       0.249                 \\
            &     (0.019)                 &     (0.032)                 &     (0.030)                 &     (0.034)                 &     (0.690)                 &     (0.313)                 &     (0.461)                 &     (0.345)                 &     (0.641)                 &     (0.715)                 &     (0.464)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .985                 &        .995                 &        .989                 &         .95                 &        .991                 &        .988                 &        .967                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/CTR_KPMG/Results1RICTint_EUKLEMS_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 2003-2007}}} \\\midrule
$R_{c,t}$ &      -0.094$^{\ast\ast}$    &      -0.092                 &      -0.019                 &      -0.030                 &       0.048                 &      -0.302                 &       0.217                 &       0.133                 &      -0.288                 &       0.284                 &       0.196                 \\
            &     (0.026)                 &     (0.046)                 &     (0.035)                 &     (0.056)                 &     (1.239)                 &     (0.847)                 &     (0.672)                 &     (0.801)                 &     (1.713)                 &     (1.306)                 &     (2.275)                 \\\addlinespace
$ICT_{c,t}$&      -0.085                 &      -0.123$^{\ast}$        &      -0.128                 &      -0.135                 &      -2.219                 &       1.194                 &      -2.031                 &      -1.383                 &       4.816                 &      -2.511                 &      -2.036                 \\
            &     (0.093)                 &     (0.054)                 &     (0.174)                 &     (0.134)                 &     (1.824)                 &     (0.918)                 &     (2.233)                 &     (1.101)                 &     (3.653)                 &     (4.524)                 &     (2.757)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.028                 &      -0.010                 &      -0.064                 &       0.037                 &      -1.306                 &      -0.728$^{\ast}$        &      -0.808                 &       0.229                 &      -0.721                 &      -1.151                 &       1.918                 \\
            &     (0.029)                 &     (0.020)                 &     (0.071)                 &     (0.044)                 &     (0.853)                 &     (0.327)                 &     (1.092)                 &     (0.487)                 &     (1.285)                 &     (2.011)                 &     (1.103)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .994                 &        .998                 &        .996                 &        .981                 &        .998                 &        .996                 &        .989                 \\
$N$      &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 \\


==> inputs/robustness/CTR_KPMG/Results1RICTint_EUKLEMS_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 2003-2016}}} \\\midrule
$R_{c,t}$ &      -0.007                 &      -0.038                 &       0.048                 &      -0.019                 &       0.354                 &      -0.257                 &       0.651                 &      -0.040                 &      -1.099                 &       1.630                 &      -0.552                 \\
            &     (0.014)                 &     (0.029)                 &     (0.066)                 &     (0.023)                 &     (0.558)                 &     (0.324)                 &     (0.546)                 &     (0.266)                 &     (0.939)                 &     (1.506)                 &     (1.014)                 \\\addlinespace
$ICT_{c,t}$&      -0.067$^{\ast\ast}$    &      -0.024                 &      -0.026                 &      -0.110                 &      -1.992$^{\ast\ast}$    &      -0.439                 &      -0.423                 &      -1.130                 &      -0.158                 &       1.601                 &      -1.680                 \\
            &     (0.030)                 &     (0.057)                 &     (0.052)                 &     (0.068)                 &     (0.907)                 &     (0.572)                 &     (0.718)                 &     (0.670)                 &     (1.415)                 &     (2.030)                 &     (1.655)                 \\\addlinespace
$R*ICT_{c,t}$&       0.027$^{\ast}$        &       0.005                 &       0.010                 &       0.065$^{\ast}$        &       0.714                 &      -0.085                 &       0.153                 &       0.646$^{\ast}$        &      -0.538                 &      -0.653                 &       1.262                 \\
            &     (0.014)                 &     (0.024)                 &     (0.028)                 &     (0.031)                 &     (0.438)                 &     (0.323)                 &     (0.270)                 &     (0.307)                 &     (0.680)                 &     (0.866)                 &     (0.814)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &        .999                 &        .975                 &        .991                 &        .983                 &        .923                 &        .988                 &        .979                 &        .947                 \\
$N$      &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 \\


==> inputs/robustness/CTR_KPMG/Results1RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.001                 &       0.008                 &       0.018                 &      -0.020                 &       0.253                 &       0.228                 &       0.113                 &      -0.088                 &       0.335                 &       0.241                 &      -0.576                 \\
            &     (0.018)                 &     (0.024)                 &     (0.057)                 &     (0.029)                 &     (0.716)                 &     (0.352)                 &     (0.514)                 &     (0.365)                 &     (0.880)                 &     (1.284)                 &     (0.980)                 \\\addlinespace
$ICT_{c,t}$&      -0.019                 &      -0.010                 &      -0.023                 &      -0.039                 &      -0.988                 &      -0.201                 &       0.102                 &      -0.889                 &      -0.203                 &       1.681                 &      -1.512                 \\
            &     (0.030)                 &     (0.045)                 &     (0.029)                 &     (0.063)                 &     (0.669)                 &     (0.466)                 &     (0.330)                 &     (0.571)                 &     (0.933)                 &     (1.053)                 &     (1.023)                 \\\addlinespace
$R*ICT_{c,t}$&       0.001                 &       0.012                 &       0.021                 &      -0.016                 &       0.435                 &      -0.013                 &       0.302                 &       0.145                 &       0.163                 &      -0.236                 &       0.072                 \\
            &     (0.021)                 &     (0.026)                 &     (0.037)                 &     (0.036)                 &     (0.727)                 &     (0.322)                 &     (0.580)                 &     (0.348)                 &     (0.586)                 &     (0.746)                 &     (0.529)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .985                 &        .994                 &        .989                 &         .95                 &        .991                 &        .988                 &        .966                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/CTR_KPMG/Results1RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 2003-2007}}} \\\midrule
$R_{c,t}$ &      -0.093$^{\ast\ast}$    &      -0.090                 &      -0.018                 &      -0.027                 &      -0.049                 &      -0.322                 &       0.130                 &       0.143                 &      -0.402                 &       0.238                 &       0.343                 \\
            &     (0.026)                 &     (0.044)                 &     (0.040)                 &     (0.056)                 &     (1.179)                 &     (0.859)                 &     (0.619)                 &     (0.775)                 &     (1.749)                 &     (1.316)                 &     (2.180)                 \\\addlinespace
$ICT_{c,t}$&      -0.086                 &      -0.131$^{\ast}$        &      -0.133                 &      -0.154                 &      -1.682                 &       1.421                 &      -1.659                 &      -1.444                 &       5.631                 &      -2.457                 &      -2.845                 \\
            &     (0.088)                 &     (0.058)                 &     (0.152)                 &     (0.136)                 &     (1.625)                 &     (0.812)                 &     (1.821)                 &     (1.090)                 &     (3.356)                 &     (4.002)                 &     (2.591)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.026                 &      -0.008                 &      -0.058                 &       0.042                 &      -1.416                 &      -0.813$^{\ast\ast}$    &      -0.853                 &       0.249                 &      -1.044                 &      -1.044                 &       2.114                 \\
            &     (0.026)                 &     (0.020)                 &     (0.063)                 &     (0.042)                 &     (0.775)                 &     (0.282)                 &     (0.970)                 &     (0.485)                 &     (1.111)                 &     (1.783)                 &     (1.084)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .994                 &        .998                 &        .996                 &        .981                 &        .998                 &        .996                 &        .989                 \\
$N$      &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 \\


==> inputs/robustness/CTR_KPMG/Results1RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 2003-2016}}} \\\midrule
$R_{c,t}$ &      -0.005                 &      -0.036                 &       0.053                 &      -0.018                 &       0.385                 &      -0.282                 &       0.709                 &      -0.041                 &      -1.219                 &       1.776                 &      -0.572                 \\
            &     (0.014)                 &     (0.029)                 &     (0.068)                 &     (0.023)                 &     (0.548)                 &     (0.329)                 &     (0.556)                 &     (0.272)                 &     (0.974)                 &     (1.583)                 &     (1.025)                 \\\addlinespace
$ICT_{c,t}$&      -0.074$^{\ast\ast}$    &      -0.045                 &      -0.069                 &      -0.111                 &      -2.269$^{\ast\ast}$    &      -0.229                 &      -0.934                 &      -1.105                 &       0.847                 &       0.311                 &      -1.458                 \\
            &     (0.033)                 &     (0.041)                 &     (0.046)                 &     (0.070)                 &     (0.891)                 &     (0.612)                 &     (0.607)                 &     (0.678)                 &     (1.323)                 &     (1.885)                 &     (1.667)                 \\\addlinespace
$R*ICT_{c,t}$&       0.029$^{\ast}$        &       0.013                 &       0.028                 &       0.064$^{\ast}$        &       0.788                 &      -0.195                 &       0.367                 &       0.616$^{\ast}$        &      -1.005                 &      -0.050                 &       1.145                 \\
            &     (0.016)                 &     (0.019)                 &     (0.036)                 &     (0.032)                 &     (0.479)                 &     (0.341)                 &     (0.417)                 &     (0.306)                 &     (0.760)                 &     (1.120)                 &     (0.864)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &        .999                 &        .975                 &        .991                 &        .983                 &        .922                 &        .988                 &        .979                 &        .947                 \\
$N$      &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 \\


==> inputs/robustness/CTR_KPMG/Results2RICTint_EUKLEMS_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.018                 &       0.005                 &      -0.003                 &      -0.056                 &      -0.210                 &       0.158                 &      -0.069                 &      -0.299                 &       0.617                 &       0.102                 &      -0.738                 \\
            &     (0.021)                 &     (0.039)                 &     (0.053)                 &     (0.035)                 &     (0.659)                 &     (0.468)                 &     (0.507)                 &     (0.245)                 &     (0.970)                 &     (0.959)                 &     (0.816)                 \\\addlinespace
$ICT_{c,t}$&       0.020                 &       0.015                 &       0.034                 &       0.023                 &       0.654$^{\ast}$        &      -0.211                 &       0.563                 &       0.302                 &      -1.719                 &       1.136                 &       0.568                 \\
            &     (0.029)                 &     (0.057)                 &     (0.044)                 &     (0.057)                 &     (0.325)                 &     (0.571)                 &     (0.384)                 &     (0.187)                 &     (1.343)                 &     (1.252)                 &     (0.554)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.014                 &      -0.004                 &      -0.007                 &      -0.035                 &       0.013                 &       0.016                 &       0.067                 &      -0.070                 &       0.603                 &      -0.413                 &      -0.196                 \\
            &     (0.020)                 &     (0.039)                 &     (0.032)                 &     (0.033)                 &     (0.477)                 &     (0.361)                 &     (0.490)                 &     (0.102)                 &     (0.729)                 &     (0.809)                 &     (0.430)                 \\\addlinespace
$wL_{c,t}$&       0.423$^{\ast\ast\ast}$&       0.367$^{\ast}$        &       0.596$^{\ast}$        &       0.370$^{\ast\ast\ast}$&      -0.639$^{\ast\ast}$    &       0.049                 &       0.094                 &      -0.782$^{\ast\ast\ast}$&       0.720$^{\ast}$        &       1.098$^{\ast}$        &      -1.805$^{\ast\ast\ast}$\\
            &     (0.077)                 &     (0.181)                 &     (0.285)                 &     (0.099)                 &     (0.215)                 &     (0.071)                 &     (0.238)                 &     (0.090)                 &     (0.334)                 &     (0.566)                 &     (0.349)                 \\\addlinespace
$rK_{c,t}$&       0.013                 &       0.225$^{\ast}$        &       0.132                 &      -0.241$^{\ast\ast}$    &      -0.730$^{\ast\ast\ast}$&       0.016                 &       0.045                 &      -0.791$^{\ast\ast\ast}$&       0.738$^{\ast\ast}$    &       0.994$^{\ast\ast}$    &      -1.726$^{\ast\ast\ast}$\\
            &     (0.056)                 &     (0.108)                 &     (0.121)                 &     (0.078)                 &     (0.159)                 &     (0.038)                 &     (0.176)                 &     (0.091)                 &     (0.252)                 &     (0.398)                 &     (0.309)                 \\\addlinespace
$pQ_{c,t}$&       0.233$^{\ast}$        &       0.117                 &       0.270                 &       0.248$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.122)                 &     (0.338)                 &     (0.332)                 &     (0.132)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.001                 &      -0.003                 &       0.001                 &       0.004$^{\ast}$        &      -0.066                 &      -0.043                 &      -0.015                 &      -0.008                 &      -0.079                 &       0.053                 &       0.025                 \\
            &     (0.001)                 &     (0.003)                 &     (0.004)                 &     (0.002)                 &     (0.055)                 &     (0.028)                 &     (0.029)                 &     (0.006)                 &     (0.061)                 &     (0.076)                 &     (0.051)                 \\\addlinespace
$Services_{c,t}$&      -0.005                 &       0.015$^{\ast\ast\ast}$&      -0.003                 &      -0.020$^{\ast\ast}$    &      -0.024                 &       0.066                 &      -0.020                 &      -0.070                 &       0.245                 &      -0.121                 &      -0.162                 \\
            &     (0.004)                 &     (0.002)                 &     (0.010)                 &     (0.008)                 &     (0.136)                 &     (0.040)                 &     (0.134)                 &     (0.048)                 &     (0.176)                 &     (0.258)                 &     (0.172)                 \\\addlinespace
$HHI_{c,t}$&      -1.599$^{\ast\ast}$    &       0.803                 &      -2.327                 &      -3.594$^{\ast\ast}$    &     -19.448                 &       4.374                 &     -21.210                 &      -2.611                 &      20.915                 &     -44.171                 &      17.035                 \\
            &     (0.567)                 &     (0.866)                 &     (1.640)                 &     (1.306)                 &    (13.550)                 &     (9.106)                 &    (13.289)                 &     (8.889)                 &    (24.681)                 &    (41.033)                 &    (32.877)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast}$        &       0.002                 &      -0.001                 &       0.040$^{\ast\ast}$    &      -0.004                 &       0.019                 &       0.025$^{\ast\ast\ast}$&      -0.041                 &       0.020                 &       0.024                 \\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.001)                 &     (0.014)                 &     (0.008)                 &     (0.015)                 &     (0.007)                 &     (0.028)                 &     (0.035)                 &     (0.017)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.019$^{\ast\ast}$    &       0.027                 &      -0.018                 &       0.040$^{\ast\ast}$    &      -0.305                 &       0.083                 &      -0.153                 &      -0.236                 &       0.580                 &      -0.261                 &      -0.319                 \\
            &     (0.006)                 &     (0.025)                 &     (0.035)                 &     (0.013)                 &     (0.256)                 &     (0.112)                 &     (0.189)                 &     (0.137)                 &     (0.397)                 &     (0.504)                 &     (0.349)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.002                 &       0.000                 &       0.005$^{\ast}$        &       0.001                 &       0.041                 &      -0.002                 &       0.046                 &      -0.003                 &      -0.041                 &       0.097$^{\ast}$        &      -0.069                 \\
            &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.002)                 &     (0.034)                 &     (0.012)                 &     (0.026)                 &     (0.008)                 &     (0.031)                 &     (0.046)                 &     (0.043)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.002                 &       0.020                 &      -0.009                 &      -0.004                 &       0.041                 &       0.092                 &       0.033                 &      -0.083                 &       0.395                 &      -0.140                 &      -0.250                 \\
            &     (0.005)                 &     (0.012)                 &     (0.015)                 &     (0.009)                 &     (0.198)                 &     (0.091)                 &     (0.160)                 &     (0.053)                 &     (0.226)                 &     (0.248)                 &     (0.250)                 \\\addlinespace
$CTR_{c,t}$&       0.004$^{\ast\ast}$    &       0.004                 &       0.012$^{\ast}$        &      -0.001                 &       0.231$^{\ast\ast}$    &       0.061                 &       0.123$^{\ast}$        &       0.047$^{\ast\ast}$    &      -0.036                 &       0.146                 &      -0.087                 \\
            &     (0.002)                 &     (0.007)                 &     (0.006)                 &     (0.002)                 &     (0.079)                 &     (0.040)                 &     (0.059)                 &     (0.019)                 &     (0.098)                 &     (0.118)                 &     (0.066)                 \\\addlinespace
$XRate_{c,t}$&       0.007                 &      -0.004                 &       0.012                 &       0.020$^{\ast\ast}$    &      -0.022                 &      -0.071                 &       0.046                 &       0.003                 &      -0.273                 &       0.298                 &      -0.035                 \\
            &     (0.006)                 &     (0.014)                 &     (0.010)                 &     (0.008)                 &     (0.184)                 &     (0.105)                 &     (0.194)                 &     (0.044)                 &     (0.239)                 &     (0.313)                 &     (0.179)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .988                 &        .995                 &        .989                 &        .985                 &        .992                 &        .989                 &        .983                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/CTR_KPMG/Results2RICTint_EUKLEMS_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.053                 &      -0.062                 &       0.001                 &       0.039                 &       0.367                 &      -0.089                 &      -0.371                 &       0.827                 &      -0.452                 &      -1.323                 &       1.845                 \\
            &     (0.031)                 &     (0.038)                 &     (0.056)                 &     (0.061)                 &     (1.289)                 &     (0.878)                 &     (0.587)                 &     (0.591)                 &     (1.624)                 &     (1.083)                 &     (1.398)                 \\\addlinespace
$ICT_{c,t}$&      -0.077                 &      -0.096$^{\ast}$        &      -0.148                 &      -0.119                 &      -2.323                 &       1.303                 &      -2.403                 &      -1.223                 &       4.947                 &      -3.246                 &      -1.583                 \\
            &     (0.070)                 &     (0.043)                 &     (0.185)                 &     (0.104)                 &     (1.891)                 &     (0.986)                 &     (2.519)                 &     (0.752)                 &     (3.997)                 &     (4.966)                 &     (2.388)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.032                 &      -0.022                 &      -0.057                 &       0.028                 &      -1.341                 &      -0.742$^{\ast}$        &      -0.773                 &       0.173                 &      -0.699                 &      -1.041                 &       1.789$^{\ast}$        \\
            &     (0.022)                 &     (0.012)                 &     (0.072)                 &     (0.032)                 &     (1.003)                 &     (0.312)                 &     (1.094)                 &     (0.268)                 &     (1.432)                 &     (1.796)                 &     (0.763)                 \\\addlinespace
$wL_{c,t}$&       0.504$^{\ast}$        &       0.563$^{\ast\ast}$    &       0.029                 &       0.875$^{\ast\ast\ast}$&      -0.516$^{\ast}$        &      -0.080                 &       0.115                 &      -0.551$^{\ast\ast\ast}$&       0.383                 &       0.731$^{\ast\ast}$    &      -1.197$^{\ast\ast\ast}$\\
            &     (0.191)                 &     (0.127)                 &     (0.407)                 &     (0.170)                 &     (0.223)                 &     (0.086)                 &     (0.155)                 &     (0.067)                 &     (0.192)                 &     (0.254)                 &     (0.219)                 \\\addlinespace
$rK_{c,t}$&       0.148                 &      -0.184                 &       0.392$^{\ast}$        &       0.198                 &      -0.479                 &      -0.112                 &       0.226                 &      -0.593$^{\ast\ast\ast}$&       0.339                 &       0.945$^{\ast\ast}$    &      -1.322$^{\ast\ast\ast}$\\
            &     (0.106)                 &     (0.130)                 &     (0.160)                 &     (0.138)                 &     (0.228)                 &     (0.084)                 &     (0.151)                 &     (0.049)                 &     (0.164)                 &     (0.218)                 &     (0.191)                 \\\addlinespace
$pQ_{c,t}$&       0.230                 &       0.250                 &       0.724                 &      -0.095                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.274)                 &     (0.247)                 &     (0.548)                 &     (0.312)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.003                 &      -0.001                 &      -0.013$^{\ast\ast}$    &       0.005                 &      -0.235$^{\ast\ast\ast}$&      -0.075$^{\ast\ast}$    &      -0.143$^{\ast}$        &      -0.016                 &       0.002                 &      -0.227                 &       0.200$^{\ast}$        \\
            &     (0.002)                 &     (0.002)                 &     (0.005)                 &     (0.006)                 &     (0.049)                 &     (0.022)                 &     (0.059)                 &     (0.025)                 &     (0.076)                 &     (0.132)                 &     (0.092)                 \\\addlinespace
$Services_{c,t}$&       0.007                 &      -0.002                 &       0.004                 &       0.013                 &       0.188                 &      -0.040                 &       0.134                 &       0.094                 &      -0.117                 &       0.012                 &       0.085                 \\
            &     (0.007)                 &     (0.009)                 &     (0.013)                 &     (0.009)                 &     (0.260)                 &     (0.105)                 &     (0.123)                 &     (0.082)                 &     (0.185)                 &     (0.188)                 &     (0.105)                 \\\addlinespace
$HHI_{c,t}$&      -1.582                 &      -2.604$^{\ast}$        &      -1.555                 &      -0.759                 &     -39.671                 &     -28.735                 &     -12.046                 &       1.109                 &     -54.308                 &      -6.462                 &      48.037$^{\ast}$        \\
            &     (1.198)                 &     (1.075)                 &     (2.045)                 &     (1.723)                 &    (42.607)                 &    (15.303)                 &    (24.852)                 &    (11.157)                 &    (26.683)                 &    (41.336)                 &    (21.744)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.002                 &      -0.003$^{\ast}$        &      -0.001                 &       0.001                 &      -0.100                 &      -0.036                 &      -0.040                 &      -0.023                 &      -0.041                 &       0.014                 &       0.021                 \\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.002)                 &     (0.050)                 &     (0.023)                 &     (0.039)                 &     (0.015)                 &     (0.039)                 &     (0.076)                 &     (0.048)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.029$^{\ast\ast}$    &       0.063$^{\ast\ast\ast}$&       0.038                 &      -0.048                 &       1.517$^{\ast\ast}$    &       0.783$^{\ast\ast}$    &       0.697                 &       0.038                 &       0.998                 &       0.425                 &      -1.287                 \\
            &     (0.008)                 &     (0.013)                 &     (0.039)                 &     (0.027)                 &     (0.477)                 &     (0.171)                 &     (0.467)                 &     (0.221)                 &     (0.590)                 &     (0.870)                 &     (0.625)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.015$^{\ast\ast}$    &      -0.002                 &       0.024$^{\ast\ast}$    &       0.013$^{\ast}$        &       0.388$^{\ast}$        &      -0.022                 &       0.373$^{\ast\ast}$    &       0.037                 &      -0.334$^{\ast\ast}$    &       0.589$^{\ast\ast}$    &      -0.269                 \\
            &     (0.003)                 &     (0.003)                 &     (0.006)                 &     (0.006)                 &     (0.141)                 &     (0.039)                 &     (0.120)                 &     (0.033)                 &     (0.112)                 &     (0.163)                 &     (0.131)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.012                 &       0.008                 &       0.019                 &      -0.008                 &       0.341                 &      -0.131                 &       0.448                 &       0.024                 &      -0.590                 &       0.815$^{\ast}$        &      -0.263                 \\
            &     (0.011)                 &     (0.011)                 &     (0.017)                 &     (0.018)                 &     (0.252)                 &     (0.104)                 &     (0.220)                 &     (0.092)                 &     (0.405)                 &     (0.347)                 &     (0.251)                 \\\addlinespace
$CTR_{c,t}$&       0.002                 &      -0.001                 &       0.006                 &       0.000                 &       0.120$^{\ast}$        &       0.017                 &       0.079                 &       0.024$^{\ast}$        &      -0.045                 &       0.096                 &      -0.042                 \\
            &     (0.002)                 &     (0.001)                 &     (0.004)                 &     (0.002)                 &     (0.053)                 &     (0.020)                 &     (0.044)                 &     (0.011)                 &     (0.072)                 &     (0.081)                 &     (0.040)                 \\\addlinespace
$XRate_{c,t}$&      -0.009                 &      -0.022$^{\ast\ast}$    &       0.004                 &      -0.008                 &      -0.174                 &       0.003                 &      -0.100                 &      -0.077                 &       0.062                 &       0.013                 &      -0.038                 \\
            &     (0.006)                 &     (0.006)                 &     (0.012)                 &     (0.012)                 &     (0.128)                 &     (0.102)                 &     (0.152)                 &     (0.064)                 &     (0.329)                 &     (0.315)                 &     (0.177)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .995                 &        .998                 &        .996                 &        .992                 &        .998                 &        .996                 &        .994                 \\
$N$      &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 \\


==> inputs/robustness/CTR_KPMG/Results2RICTint_EUKLEMS_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.017                 &      -0.038                 &       0.030                 &      -0.040$^{\ast}$        &       0.069                 &      -0.283                 &       0.598                 &      -0.246                 &      -0.814                 &       1.681                 &      -0.912                 \\
            &     (0.012)                 &     (0.025)                 &     (0.050)                 &     (0.023)                 &     (0.607)                 &     (0.336)                 &     (0.488)                 &     (0.146)                 &     (0.967)                 &     (1.123)                 &     (0.663)                 \\\addlinespace
$ICT_{c,t}$&      -0.036                 &      -0.024                 &       0.026                 &      -0.056                 &      -0.497                 &      -0.339                 &      -0.490                 &       0.332                 &      -1.437                 &      -0.094                 &       1.360                 \\
            &     (0.025)                 &     (0.054)                 &     (0.069)                 &     (0.063)                 &     (0.901)                 &     (0.550)                 &     (0.777)                 &     (0.227)                 &     (1.517)                 &     (1.780)                 &     (0.887)                 \\\addlinespace
$R*ICT_{c,t}$&       0.012                 &       0.004                 &      -0.017                 &       0.041                 &       0.021                 &      -0.129                 &       0.210                 &      -0.060                 &       0.038                 &       0.237                 &      -0.231                 \\
            &     (0.011)                 &     (0.021)                 &     (0.031)                 &     (0.031)                 &     (0.434)                 &     (0.300)                 &     (0.356)                 &     (0.108)                 &     (0.730)                 &     (0.814)                 &     (0.496)                 \\\addlinespace
$wL_{c,t}$&       0.506$^{\ast\ast\ast}$&       0.091                 &       1.011$^{\ast\ast}$    &       0.469$^{\ast\ast}$    &      -0.546$^{\ast\ast\ast}$&      -0.013                 &       0.223                 &      -0.756$^{\ast\ast\ast}$&       0.343                 &       1.443$^{\ast\ast}$    &      -1.774$^{\ast\ast\ast}$\\
            &     (0.114)                 &     (0.201)                 &     (0.347)                 &     (0.207)                 &     (0.173)                 &     (0.124)                 &     (0.174)                 &     (0.060)                 &     (0.415)                 &     (0.535)                 &     (0.227)                 \\\addlinespace
$rK_{c,t}$&       0.064                 &       0.057                 &       0.207                 &      -0.134                 &      -0.646$^{\ast\ast\ast}$&      -0.028                 &       0.158                 &      -0.776$^{\ast\ast\ast}$&       0.472                 &       1.266$^{\ast\ast\ast}$&      -1.744$^{\ast\ast\ast}$\\
            &     (0.089)                 &     (0.130)                 &     (0.201)                 &     (0.112)                 &     (0.168)                 &     (0.089)                 &     (0.157)                 &     (0.061)                 &     (0.296)                 &     (0.390)                 &     (0.245)                 \\\addlinespace
$pQ_{c,t}$&       0.198                 &       0.642$^{\ast}$        &      -0.538                 &       0.432                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.186)                 &     (0.308)                 &     (0.472)                 &     (0.260)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.002                 &      -0.004                 &       0.005                 &      -0.002                 &      -0.054$^{\ast}$        &      -0.046                 &       0.005                 &      -0.013                 &      -0.134                 &       0.129                 &       0.014                 \\
            &     (0.001)                 &     (0.003)                 &     (0.004)                 &     (0.003)                 &     (0.027)                 &     (0.030)                 &     (0.029)                 &     (0.007)                 &     (0.090)                 &     (0.089)                 &     (0.027)                 \\\addlinespace
$Services_{c,t}$&      -0.009                 &       0.016$^{\ast\ast\ast}$&      -0.018                 &      -0.018                 &      -0.068                 &       0.080                 &      -0.176                 &       0.029                 &       0.363                 &      -0.524                 &       0.138                 \\
            &     (0.006)                 &     (0.005)                 &     (0.011)                 &     (0.011)                 &     (0.098)                 &     (0.072)                 &     (0.123)                 &     (0.030)                 &     (0.258)                 &     (0.350)                 &     (0.144)                 \\\addlinespace
$HHI_{c,t}$&      -1.580$^{\ast}$        &       1.904$^{\ast\ast}$    &      -2.847                 &      -2.902$^{\ast}$        &     -25.186                 &      11.595                 &     -45.855                 &       9.074                 &      51.728                 &    -119.302                 &      60.402                 \\
            &     (0.760)                 &     (0.880)                 &     (2.066)                 &     (1.464)                 &    (19.558)                 &    (11.549)                 &    (26.317)                 &     (6.053)                 &    (50.548)                 &    (75.897)                 &    (37.084)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.000                 &      -0.002$^{\ast\ast}$    &       0.003                 &       0.001                 &       0.056$^{\ast\ast\ast}$&      -0.013                 &       0.047$^{\ast\ast}$    &       0.022$^{\ast\ast}$    &      -0.091$^{\ast\ast}$    &       0.091$^{\ast}$        &       0.003                 \\
            &     (0.001)                 &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.012)                 &     (0.009)                 &     (0.016)                 &     (0.008)                 &     (0.038)                 &     (0.046)                 &     (0.020)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.007                 &       0.032$^{\ast\ast\ast}$&      -0.026                 &       0.011                 &      -0.758$^{\ast\ast\ast}$&       0.054                 &      -0.502$^{\ast\ast}$    &      -0.310$^{\ast\ast}$    &       0.961$^{\ast}$        &      -0.871$^{\ast}$        &      -0.179                 \\
            &     (0.009)                 &     (0.009)                 &     (0.029)                 &     (0.021)                 &     (0.210)                 &     (0.139)                 &     (0.188)                 &     (0.116)                 &     (0.457)                 &     (0.452)                 &     (0.333)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.005$^{\ast\ast}$    &      -0.000                 &       0.009$^{\ast\ast}$    &       0.005                 &       0.131$^{\ast\ast}$    &       0.004                 &       0.111$^{\ast\ast}$    &       0.016                 &      -0.094$^{\ast\ast}$    &       0.199$^{\ast\ast\ast}$&      -0.103$^{\ast\ast}$    \\
            &     (0.002)                 &     (0.002)                 &     (0.003)                 &     (0.004)                 &     (0.053)                 &     (0.014)                 &     (0.038)                 &     (0.010)                 &     (0.039)                 &     (0.060)                 &     (0.044)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.007                 &       0.024$^{\ast}$        &       0.005                 &      -0.002                 &      -0.056                 &       0.040                 &      -0.040                 &      -0.055                 &       0.318                 &      -0.301                 &      -0.075                 \\
            &     (0.007)                 &     (0.011)                 &     (0.015)                 &     (0.013)                 &     (0.189)                 &     (0.098)                 &     (0.170)                 &     (0.044)                 &     (0.215)                 &     (0.357)                 &     (0.229)                 \\\addlinespace
$CTR_{c,t}$&       0.001                 &       0.005$^{\ast\ast}$    &       0.003                 &      -0.004$^{\ast}$        &       0.075                 &       0.054$^{\ast\ast}$    &       0.015                 &       0.006                 &       0.098                 &      -0.028                 &      -0.066                 \\
            &     (0.002)                 &     (0.002)                 &     (0.004)                 &     (0.002)                 &     (0.055)                 &     (0.023)                 &     (0.044)                 &     (0.015)                 &     (0.062)                 &     (0.091)                 &     (0.060)                 \\\addlinespace
$XRate_{c,t}$&       0.002                 &      -0.003                 &       0.020$^{\ast\ast\ast}$&      -0.007                 &       0.161$^{\ast}$        &       0.004                 &       0.164$^{\ast\ast\ast}$&      -0.007                 &      -0.223                 &       0.401$^{\ast\ast}$    &      -0.165$^{\ast\ast}$    \\
            &     (0.003)                 &     (0.003)                 &     (0.005)                 &     (0.005)                 &     (0.075)                 &     (0.060)                 &     (0.047)                 &     (0.014)                 &     (0.143)                 &     (0.143)                 &     (0.069)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &        .999                 &        .979                 &        .991                 &        .983                 &        .978                 &        .989                 &        .982                 &        .972                 \\
$N$      &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 \\


==> inputs/robustness/CTR_KPMG/Results2RICTint_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.018                 &       0.010                 &       0.002                 &      -0.057                 &      -0.160                 &       0.136                 &      -0.001                 &      -0.295                 &       0.538                 &       0.206                 &      -0.763                 \\
            &     (0.021)                 &     (0.033)                 &     (0.057)                 &     (0.035)                 &     (0.665)                 &     (0.487)                 &     (0.530)                 &     (0.246)                 &     (0.979)                 &     (1.001)                 &     (0.814)                 \\\addlinespace
$ICT_{c,t}$&       0.016                 &      -0.009                 &       0.010                 &       0.027                 &       0.374                 &      -0.094                 &       0.187                 &       0.280$^{\ast}$        &      -1.290                 &       0.579                 &       0.696                 \\
            &     (0.029)                 &     (0.049)                 &     (0.032)                 &     (0.056)                 &     (0.385)                 &     (0.559)                 &     (0.417)                 &     (0.142)                 &     (1.127)                 &     (0.871)                 &     (0.570)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.012                 &       0.008                 &       0.006                 &      -0.036                 &       0.161                 &      -0.049                 &       0.263                 &      -0.053                 &       0.349                 &      -0.107                 &      -0.251                 \\
            &     (0.021)                 &     (0.038)                 &     (0.035)                 &     (0.033)                 &     (0.565)                 &     (0.364)                 &     (0.610)                 &     (0.094)                 &     (0.658)                 &     (0.793)                 &     (0.456)                 \\\addlinespace
$wL_{c,t}$&       0.422$^{\ast\ast\ast}$&       0.358$^{\ast}$        &       0.588$^{\ast}$        &       0.372$^{\ast\ast\ast}$&      -0.632$^{\ast\ast}$    &       0.046                 &       0.103                 &      -0.782$^{\ast\ast\ast}$&       0.710$^{\ast}$        &       1.109$^{\ast}$        &      -1.806$^{\ast\ast\ast}$\\
            &     (0.076)                 &     (0.179)                 &     (0.279)                 &     (0.097)                 &     (0.219)                 &     (0.072)                 &     (0.245)                 &     (0.088)                 &     (0.342)                 &     (0.578)                 &     (0.349)                 \\\addlinespace
$rK_{c,t}$&       0.015                 &       0.233$^{\ast}$        &       0.140                 &      -0.241$^{\ast\ast}$    &      -0.719$^{\ast\ast\ast}$&       0.013                 &       0.058                 &      -0.789$^{\ast\ast\ast}$&       0.722$^{\ast\ast}$    &       1.012$^{\ast\ast}$    &      -1.728$^{\ast\ast\ast}$\\
            &     (0.057)                 &     (0.117)                 &     (0.126)                 &     (0.075)                 &     (0.164)                 &     (0.036)                 &     (0.184)                 &     (0.089)                 &     (0.253)                 &     (0.413)                 &     (0.309)                 \\\addlinespace
$pQ_{c,t}$&       0.232$^{\ast}$        &       0.128                 &       0.277                 &       0.244$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.121)                 &     (0.341)                 &     (0.329)                 &     (0.125)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.001                 &      -0.003                 &       0.001                 &       0.004$^{\ast}$        &      -0.065                 &      -0.043                 &      -0.014                 &      -0.008                 &      -0.080                 &       0.053                 &       0.024                 \\
            &     (0.001)                 &     (0.003)                 &     (0.004)                 &     (0.002)                 &     (0.054)                 &     (0.028)                 &     (0.029)                 &     (0.006)                 &     (0.060)                 &     (0.077)                 &     (0.050)                 \\\addlinespace
$Services_{c,t}$&      -0.005                 &       0.015$^{\ast\ast\ast}$&      -0.003                 &      -0.020$^{\ast\ast}$    &      -0.019                 &       0.064                 &      -0.014                 &      -0.069                 &       0.238                 &      -0.113                 &      -0.163                 \\
            &     (0.004)                 &     (0.003)                 &     (0.009)                 &     (0.008)                 &     (0.137)                 &     (0.039)                 &     (0.135)                 &     (0.048)                 &     (0.179)                 &     (0.256)                 &     (0.172)                 \\\addlinespace
$HHI_{c,t}$&      -1.604$^{\ast\ast}$    &       0.748                 &      -2.381                 &      -3.581$^{\ast\ast}$    &     -20.289                 &       4.725                 &     -22.330                 &      -2.684                 &      22.175                 &     -45.780                 &      17.390                 \\
            &     (0.576)                 &     (0.850)                 &     (1.618)                 &     (1.309)                 &    (13.480)                 &     (9.234)                 &    (13.544)                 &     (8.849)                 &    (25.596)                 &    (41.651)                 &    (32.746)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast}$        &       0.002                 &      -0.001                 &       0.040$^{\ast\ast}$    &      -0.004                 &       0.019                 &       0.025$^{\ast\ast\ast}$&      -0.041                 &       0.020                 &       0.024                 \\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.001)                 &     (0.014)                 &     (0.008)                 &     (0.015)                 &     (0.007)                 &     (0.028)                 &     (0.035)                 &     (0.017)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.019$^{\ast\ast}$    &       0.027                 &      -0.018                 &       0.040$^{\ast\ast}$    &      -0.298                 &       0.080                 &      -0.144                 &      -0.234                 &       0.564                 &      -0.247                 &      -0.319                 \\
            &     (0.006)                 &     (0.024)                 &     (0.035)                 &     (0.013)                 &     (0.253)                 &     (0.110)                 &     (0.185)                 &     (0.137)                 &     (0.384)                 &     (0.497)                 &     (0.345)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.002                 &       0.000                 &       0.005$^{\ast}$        &       0.001                 &       0.042                 &      -0.002                 &       0.047                 &      -0.003                 &      -0.042                 &       0.099$^{\ast}$        &      -0.070                 \\
            &     (0.001)                 &     (0.002)                 &     (0.003)                 &     (0.002)                 &     (0.034)                 &     (0.012)                 &     (0.027)                 &     (0.009)                 &     (0.030)                 &     (0.046)                 &     (0.043)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.002                 &       0.021                 &      -0.009                 &      -0.004                 &       0.049                 &       0.089                 &       0.041                 &      -0.081                 &       0.380                 &      -0.127                 &      -0.249                 \\
            &     (0.005)                 &     (0.013)                 &     (0.015)                 &     (0.009)                 &     (0.205)                 &     (0.090)                 &     (0.158)                 &     (0.052)                 &     (0.229)                 &     (0.258)                 &     (0.254)                 \\\addlinespace
$XRate_{c,t}$&       0.007                 &      -0.006                 &       0.010                 &       0.020$^{\ast\ast}$    &      -0.043                 &      -0.060                 &       0.015                 &       0.002                 &      -0.236                 &       0.248                 &      -0.021                 \\
            &     (0.006)                 &     (0.014)                 &     (0.011)                 &     (0.008)                 &     (0.200)                 &     (0.111)                 &     (0.215)                 &     (0.045)                 &     (0.232)                 &     (0.309)                 &     (0.181)                 \\\addlinespace
$CTR_{c,t}$&       0.004$^{\ast\ast}$    &       0.004                 &       0.012$^{\ast}$        &      -0.001                 &       0.231$^{\ast\ast}$    &       0.061                 &       0.123$^{\ast}$        &       0.047$^{\ast\ast}$    &      -0.037                 &       0.146                 &      -0.086                 \\
            &     (0.002)                 &     (0.007)                 &     (0.006)                 &     (0.002)                 &     (0.079)                 &     (0.039)                 &     (0.059)                 &     (0.019)                 &     (0.098)                 &     (0.118)                 &     (0.065)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .988                 &        .995                 &        .989                 &        .985                 &        .992                 &        .989                 &        .983                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/CTR_KPMG/Results2RICTint_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.053                 &      -0.061                 &       0.001                 &       0.039                 &       0.241                 &      -0.112                 &      -0.449                 &       0.802                 &      -0.529                 &      -1.326                 &       1.911                 \\
            &     (0.030)                 &     (0.036)                 &     (0.056)                 &     (0.059)                 &     (1.198)                 &     (0.886)                 &     (0.562)                 &     (0.581)                 &     (1.709)                 &     (0.990)                 &     (1.333)                 \\\addlinespace
$ICT_{c,t}$&      -0.073                 &      -0.102$^{\ast}$        &      -0.148                 &      -0.129                 &      -1.664                 &       1.558                 &      -2.081                 &      -1.141                 &       5.689                 &      -3.419                 &      -2.078                 \\
            &     (0.071)                 &     (0.046)                 &     (0.173)                 &     (0.109)                 &     (1.624)                 &     (0.862)                 &     (2.196)                 &     (0.679)                 &     (3.694)                 &     (4.545)                 &     (2.254)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.032                 &      -0.019                 &      -0.053                 &       0.031                 &      -1.479                 &      -0.833$^{\ast\ast}$    &      -0.806                 &       0.159                 &      -1.003                 &      -0.881                 &       1.911$^{\ast}$        \\
            &     (0.021)                 &     (0.011)                 &     (0.067)                 &     (0.034)                 &     (0.925)                 &     (0.274)                 &     (0.973)                 &     (0.229)                 &     (1.247)                 &     (1.603)                 &     (0.727)                 \\\addlinespace
$wL_{c,t}$&       0.501$^{\ast}$        &       0.559$^{\ast\ast}$    &       0.022                 &       0.869$^{\ast\ast\ast}$&      -0.509$^{\ast}$        &      -0.082                 &       0.122                 &      -0.548$^{\ast\ast\ast}$&       0.373                 &       0.739$^{\ast\ast}$    &      -1.197$^{\ast\ast\ast}$\\
            &     (0.193)                 &     (0.129)                 &     (0.413)                 &     (0.168)                 &     (0.226)                 &     (0.087)                 &     (0.156)                 &     (0.068)                 &     (0.195)                 &     (0.255)                 &     (0.218)                 \\\addlinespace
$rK_{c,t}$&       0.149                 &      -0.183                 &       0.395$^{\ast}$        &       0.196                 &      -0.473                 &      -0.114                 &       0.232                 &      -0.591$^{\ast\ast\ast}$&       0.327                 &       0.955$^{\ast\ast}$    &      -1.320$^{\ast\ast\ast}$\\
            &     (0.106)                 &     (0.131)                 &     (0.161)                 &     (0.135)                 &     (0.229)                 &     (0.085)                 &     (0.154)                 &     (0.050)                 &     (0.172)                 &     (0.224)                 &     (0.190)                 \\\addlinespace
$pQ_{c,t}$&       0.233                 &       0.254                 &       0.732                 &      -0.089                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.275)                 &     (0.248)                 &     (0.556)                 &     (0.305)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.003                 &      -0.001                 &      -0.013$^{\ast}$        &       0.005                 &      -0.229$^{\ast\ast\ast}$&      -0.077$^{\ast\ast}$    &      -0.138$^{\ast}$        &      -0.014                 &      -0.005                 &      -0.221                 &       0.200$^{\ast}$        \\
            &     (0.002)                 &     (0.002)                 &     (0.005)                 &     (0.006)                 &     (0.048)                 &     (0.020)                 &     (0.055)                 &     (0.026)                 &     (0.073)                 &     (0.128)                 &     (0.093)                 \\\addlinespace
$Services_{c,t}$&       0.007                 &      -0.002                 &       0.005                 &       0.014                 &       0.192                 &      -0.048                 &       0.141                 &       0.099                 &      -0.150                 &       0.031                 &       0.097                 \\
            &     (0.007)                 &     (0.008)                 &     (0.013)                 &     (0.009)                 &     (0.265)                 &     (0.109)                 &     (0.126)                 &     (0.083)                 &     (0.193)                 &     (0.189)                 &     (0.107)                 \\\addlinespace
$HHI_{c,t}$&      -1.525                 &      -2.531$^{\ast}$        &      -1.455                 &      -0.672                 &     -37.785                 &     -29.406                 &     -10.359                 &       1.980                 &     -57.172                 &      -4.554                 &      48.919$^{\ast}$        \\
            &     (1.220)                 &     (1.087)                 &     (2.014)                 &     (1.712)                 &    (43.344)                 &    (15.599)                 &    (24.832)                 &    (11.571)                 &    (26.997)                 &    (38.101)                 &    (22.124)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.002                 &      -0.003$^{\ast}$        &      -0.001                 &       0.001                 &      -0.096                 &      -0.037                 &      -0.038                 &      -0.022                 &      -0.043                 &       0.017                 &       0.020                 \\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.002)                 &     (0.051)                 &     (0.023)                 &     (0.040)                 &     (0.015)                 &     (0.039)                 &     (0.077)                 &     (0.049)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.028$^{\ast\ast}$    &       0.062$^{\ast\ast\ast}$&       0.036                 &      -0.049                 &       1.507$^{\ast\ast}$    &       0.801$^{\ast\ast\ast}$&       0.675                 &       0.031                 &       1.075                 &       0.367                 &      -1.302                 \\
            &     (0.008)                 &     (0.013)                 &     (0.038)                 &     (0.027)                 &     (0.461)                 &     (0.171)                 &     (0.453)                 &     (0.220)                 &     (0.577)                 &     (0.849)                 &     (0.626)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.015$^{\ast\ast}$    &      -0.001                 &       0.024$^{\ast\ast}$    &       0.014$^{\ast}$        &       0.391$^{\ast}$        &      -0.026                 &       0.377$^{\ast\ast}$    &       0.040                 &      -0.352$^{\ast\ast}$    &       0.599$^{\ast\ast}$    &      -0.263                 \\
            &     (0.004)                 &     (0.003)                 &     (0.006)                 &     (0.006)                 &     (0.149)                 &     (0.037)                 &     (0.126)                 &     (0.033)                 &     (0.120)                 &     (0.175)                 &     (0.136)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.012                 &       0.009                 &       0.020                 &      -0.007                 &       0.346                 &      -0.137                 &       0.455                 &       0.028                 &      -0.616                 &       0.829$^{\ast}$        &      -0.253                 \\
            &     (0.012)                 &     (0.012)                 &     (0.018)                 &     (0.018)                 &     (0.280)                 &     (0.110)                 &     (0.226)                 &     (0.094)                 &     (0.415)                 &     (0.362)                 &     (0.265)                 \\\addlinespace
$XRate_{c,t}$&      -0.010                 &      -0.024$^{\ast\ast}$    &       0.003                 &      -0.011                 &      -0.146                 &       0.052                 &      -0.105                 &      -0.093                 &       0.207                 &      -0.039                 &      -0.124                 \\
            &     (0.008)                 &     (0.007)                 &     (0.015)                 &     (0.013)                 &     (0.156)                 &     (0.115)                 &     (0.188)                 &     (0.073)                 &     (0.396)                 &     (0.394)                 &     (0.212)                 \\\addlinespace
$CTR_{c,t}$&       0.002                 &      -0.001                 &       0.006                 &       0.000                 &       0.120$^{\ast}$        &       0.018                 &       0.078                 &       0.024$^{\ast}$        &      -0.043                 &       0.095                 &      -0.043                 \\
            &     (0.002)                 &     (0.001)                 &     (0.004)                 &     (0.002)                 &     (0.055)                 &     (0.020)                 &     (0.045)                 &     (0.011)                 &     (0.072)                 &     (0.083)                 &     (0.040)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .995                 &        .998                 &        .996                 &        .992                 &        .998                 &        .996                 &        .994                 \\
$N$      &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 \\


==> inputs/robustness/CTR_KPMG/Results2RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.017                 &      -0.035                 &       0.035                 &      -0.040$^{\ast}$        &       0.109                 &      -0.313                 &       0.664                 &      -0.242                 &      -0.959                 &       1.846                 &      -0.924                 \\
            &     (0.012)                 &     (0.024)                 &     (0.052)                 &     (0.022)                 &     (0.603)                 &     (0.339)                 &     (0.499)                 &     (0.144)                 &     (1.002)                 &     (1.183)                 &     (0.665)                 \\\addlinespace
$ICT_{c,t}$&      -0.039                 &      -0.044                 &      -0.009                 &      -0.055                 &      -0.849                 &      -0.116                 &      -1.039                 &       0.305                 &      -0.291                 &      -1.442                 &       1.492                 \\
            &     (0.026)                 &     (0.039)                 &     (0.056)                 &     (0.061)                 &     (0.906)                 &     (0.581)                 &     (0.711)                 &     (0.217)                 &     (1.427)                 &     (1.538)                 &     (0.904)                 \\\addlinespace
$R*ICT_{c,t}$&       0.012                 &       0.012                 &      -0.001                 &       0.040                 &       0.157                 &      -0.242                 &       0.439                 &      -0.040                 &      -0.514                 &       0.836                 &      -0.252                 \\
            &     (0.012)                 &     (0.017)                 &     (0.032)                 &     (0.029)                 &     (0.507)                 &     (0.316)                 &     (0.470)                 &     (0.105)                 &     (0.841)                 &     (1.020)                 &     (0.549)                 \\\addlinespace
$wL_{c,t}$&       0.504$^{\ast\ast\ast}$&       0.083                 &       0.999$^{\ast\ast}$    &       0.467$^{\ast\ast}$    &      -0.541$^{\ast\ast\ast}$&      -0.018                 &       0.232                 &      -0.755$^{\ast\ast\ast}$&       0.320                 &       1.467$^{\ast\ast}$    &      -1.774$^{\ast\ast\ast}$\\
            &     (0.113)                 &     (0.201)                 &     (0.344)                 &     (0.206)                 &     (0.174)                 &     (0.125)                 &     (0.175)                 &     (0.059)                 &     (0.422)                 &     (0.542)                 &     (0.225)                 \\\addlinespace
$rK_{c,t}$&       0.062                 &       0.059                 &       0.215                 &      -0.137                 &      -0.639$^{\ast\ast\ast}$&      -0.035                 &       0.170                 &      -0.774$^{\ast\ast\ast}$&       0.439                 &       1.300$^{\ast\ast\ast}$&      -1.743$^{\ast\ast\ast}$\\
            &     (0.088)                 &     (0.133)                 &     (0.199)                 &     (0.107)                 &     (0.169)                 &     (0.090)                 &     (0.159)                 &     (0.060)                 &     (0.303)                 &     (0.400)                 &     (0.243)                 \\\addlinespace
$pQ_{c,t}$&       0.205                 &       0.652$^{\ast}$        &      -0.529                 &       0.440                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.184)                 &     (0.310)                 &     (0.472)                 &     (0.256)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.002                 &      -0.004                 &       0.005                 &      -0.002                 &      -0.054$^{\ast}$        &      -0.046                 &       0.005                 &      -0.013                 &      -0.135                 &       0.130                 &       0.014                 \\
            &     (0.001)                 &     (0.003)                 &     (0.004)                 &     (0.003)                 &     (0.027)                 &     (0.030)                 &     (0.028)                 &     (0.008)                 &     (0.092)                 &     (0.089)                 &     (0.027)                 \\\addlinespace
$Services_{c,t}$&      -0.009                 &       0.017$^{\ast\ast\ast}$&      -0.017                 &      -0.018                 &      -0.061                 &       0.075                 &      -0.166                 &       0.030                 &       0.337                 &      -0.496                 &       0.139                 \\
            &     (0.006)                 &     (0.005)                 &     (0.011)                 &     (0.011)                 &     (0.104)                 &     (0.070)                 &     (0.128)                 &     (0.030)                 &     (0.253)                 &     (0.350)                 &     (0.146)                 \\\addlinespace
$HHI_{c,t}$&      -1.603$^{\ast}$        &       1.883$^{\ast}$        &      -2.855                 &      -2.940$^{\ast}$        &     -25.520                 &      11.880                 &     -46.480$^{\ast}$        &       9.081                 &      52.987                 &    -120.853                 &      60.639                 \\
            &     (0.759)                 &     (0.892)                 &     (2.068)                 &     (1.455)                 &    (19.482)                 &    (11.633)                 &    (26.239)                 &     (6.067)                 &    (50.566)                 &    (76.131)                 &    (37.107)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001                 &      -0.002$^{\ast\ast}$    &       0.003                 &       0.001                 &       0.056$^{\ast\ast\ast}$&      -0.013                 &       0.046$^{\ast\ast}$    &       0.022$^{\ast\ast}$    &      -0.091$^{\ast\ast}$    &       0.091$^{\ast}$        &       0.003                 \\
            &     (0.001)                 &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.012)                 &     (0.009)                 &     (0.016)                 &     (0.008)                 &     (0.038)                 &     (0.046)                 &     (0.020)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.007                 &       0.032$^{\ast\ast\ast}$&      -0.027                 &       0.011                 &      -0.758$^{\ast\ast\ast}$&       0.054                 &      -0.502$^{\ast\ast}$    &      -0.310$^{\ast\ast}$    &       0.962$^{\ast\ast}$    &      -0.871$^{\ast}$        &      -0.180                 \\
            &     (0.009)                 &     (0.009)                 &     (0.029)                 &     (0.021)                 &     (0.208)                 &     (0.138)                 &     (0.187)                 &     (0.116)                 &     (0.420)                 &     (0.451)                 &     (0.335)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.005$^{\ast\ast}$    &      -0.000                 &       0.009$^{\ast\ast}$    &       0.005                 &       0.133$^{\ast\ast}$    &       0.003                 &       0.114$^{\ast\ast}$    &       0.016                 &      -0.100$^{\ast\ast}$    &       0.205$^{\ast\ast\ast}$&      -0.103$^{\ast\ast}$    \\
            &     (0.002)                 &     (0.002)                 &     (0.003)                 &     (0.004)                 &     (0.054)                 &     (0.015)                 &     (0.038)                 &     (0.010)                 &     (0.037)                 &     (0.060)                 &     (0.044)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.006                 &       0.024$^{\ast}$        &       0.005                 &      -0.003                 &      -0.052                 &       0.032                 &      -0.032                 &      -0.052                 &       0.283                 &      -0.273                 &      -0.068                 \\
            &     (0.007)                 &     (0.012)                 &     (0.016)                 &     (0.013)                 &     (0.198)                 &     (0.097)                 &     (0.178)                 &     (0.044)                 &     (0.238)                 &     (0.365)                 &     (0.228)                 \\\addlinespace
$XRate_{c,t}$&       0.002                 &      -0.005                 &       0.018$^{\ast\ast\ast}$&      -0.007                 &       0.134                 &       0.018                 &       0.123$^{\ast\ast}$    &      -0.007                 &      -0.149                 &       0.305$^{\ast}$        &      -0.148$^{\ast}$        \\
            &     (0.003)                 &     (0.004)                 &     (0.005)                 &     (0.005)                 &     (0.083)                 &     (0.066)                 &     (0.056)                 &     (0.015)                 &     (0.159)                 &     (0.153)                 &     (0.075)                 \\\addlinespace
$CTR_{c,t}$&       0.001                 &       0.005$^{\ast\ast}$    &       0.003                 &      -0.004$^{\ast}$        &       0.074                 &       0.055$^{\ast\ast}$    &       0.014                 &       0.005                 &       0.100                 &      -0.031                 &      -0.066                 \\
            &     (0.002)                 &     (0.002)                 &     (0.004)                 &     (0.002)                 &     (0.055)                 &     (0.023)                 &     (0.044)                 &     (0.015)                 &     (0.062)                 &     (0.093)                 &     (0.059)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &        .999                 &        .979                 &        .991                 &        .983                 &        .978                 &        .988                 &        .982                 &        .972                 \\
$N$      &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 \\


==> inputs/robustness/CTR_KPMG/Results2shortV1_RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.018                 &       0.010                 &       0.002                 &      -0.057                 &      -0.160                 &       0.136                 &      -0.001                 &      -0.295                 &       0.538                 &       0.206                 &      -0.763                 \\
            &     (0.021)                 &     (0.033)                 &     (0.057)                 &     (0.035)                 &     (0.665)                 &     (0.487)                 &     (0.530)                 &     (0.246)                 &     (0.979)                 &     (1.001)                 &     (0.814)                 \\\addlinespace
$ICT_{c,t}$&       0.016                 &      -0.009                 &       0.010                 &       0.027                 &       0.374                 &      -0.094                 &       0.187                 &       0.280$^{\ast}$        &      -1.290                 &       0.579                 &       0.696                 \\
            &     (0.029)                 &     (0.049)                 &     (0.032)                 &     (0.056)                 &     (0.385)                 &     (0.559)                 &     (0.417)                 &     (0.142)                 &     (1.127)                 &     (0.871)                 &     (0.570)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.012                 &       0.008                 &       0.006                 &      -0.036                 &       0.161                 &      -0.049                 &       0.263                 &      -0.053                 &       0.349                 &      -0.107                 &      -0.251                 \\
            &     (0.021)                 &     (0.038)                 &     (0.035)                 &     (0.033)                 &     (0.565)                 &     (0.364)                 &     (0.610)                 &     (0.094)                 &     (0.658)                 &     (0.793)                 &     (0.456)                 \\\addlinespace
$wL_{c,t}$&       0.422$^{\ast\ast\ast}$&       0.358$^{\ast}$        &       0.588$^{\ast}$        &       0.372$^{\ast\ast\ast}$&      -0.632$^{\ast\ast}$    &       0.046                 &       0.103                 &      -0.782$^{\ast\ast\ast}$&       0.710$^{\ast}$        &       1.109$^{\ast}$        &      -1.806$^{\ast\ast\ast}$\\
            &     (0.076)                 &     (0.179)                 &     (0.279)                 &     (0.097)                 &     (0.219)                 &     (0.072)                 &     (0.245)                 &     (0.088)                 &     (0.342)                 &     (0.578)                 &     (0.349)                 \\\addlinespace
$rK_{c,t}$&       0.015                 &       0.233$^{\ast}$        &       0.140                 &      -0.241$^{\ast\ast}$    &      -0.719$^{\ast\ast\ast}$&       0.013                 &       0.058                 &      -0.789$^{\ast\ast\ast}$&       0.722$^{\ast\ast}$    &       1.012$^{\ast\ast}$    &      -1.728$^{\ast\ast\ast}$\\
            &     (0.057)                 &     (0.117)                 &     (0.126)                 &     (0.075)                 &     (0.164)                 &     (0.036)                 &     (0.184)                 &     (0.089)                 &     (0.253)                 &     (0.413)                 &     (0.309)                 \\\addlinespace
$pQ_{c,t}$&       0.232$^{\ast}$        &       0.128                 &       0.277                 &       0.244$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.121)                 &     (0.341)                 &     (0.329)                 &     (0.125)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .988                 &        .995                 &        .989                 &        .985                 &        .992                 &        .989                 &        .983                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/CTR_KPMG/Results2shortV1_RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 2003-2007}}} \\\midrule
$R_{c,t}$ &      -0.053                 &      -0.061                 &       0.001                 &       0.039                 &       0.241                 &      -0.112                 &      -0.449                 &       0.802                 &      -0.529                 &      -1.326                 &       1.911                 \\
            &     (0.030)                 &     (0.036)                 &     (0.056)                 &     (0.059)                 &     (1.198)                 &     (0.886)                 &     (0.562)                 &     (0.581)                 &     (1.709)                 &     (0.990)                 &     (1.333)                 \\\addlinespace
$ICT_{c,t}$&      -0.073                 &      -0.102$^{\ast}$        &      -0.148                 &      -0.129                 &      -1.664                 &       1.558                 &      -2.081                 &      -1.141                 &       5.689                 &      -3.419                 &      -2.078                 \\
            &     (0.071)                 &     (0.046)                 &     (0.173)                 &     (0.109)                 &     (1.624)                 &     (0.862)                 &     (2.196)                 &     (0.679)                 &     (3.694)                 &     (4.545)                 &     (2.254)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.032                 &      -0.019                 &      -0.053                 &       0.031                 &      -1.479                 &      -0.833$^{\ast\ast}$    &      -0.806                 &       0.159                 &      -1.003                 &      -0.881                 &       1.911$^{\ast}$        \\
            &     (0.021)                 &     (0.011)                 &     (0.067)                 &     (0.034)                 &     (0.925)                 &     (0.274)                 &     (0.973)                 &     (0.229)                 &     (1.247)                 &     (1.603)                 &     (0.727)                 \\\addlinespace
$wL_{c,t}$&       0.501$^{\ast}$        &       0.559$^{\ast\ast}$    &       0.022                 &       0.869$^{\ast\ast\ast}$&      -0.509$^{\ast}$        &      -0.082                 &       0.122                 &      -0.548$^{\ast\ast\ast}$&       0.373                 &       0.739$^{\ast\ast}$    &      -1.197$^{\ast\ast\ast}$\\
            &     (0.193)                 &     (0.129)                 &     (0.413)                 &     (0.168)                 &     (0.226)                 &     (0.087)                 &     (0.156)                 &     (0.068)                 &     (0.195)                 &     (0.255)                 &     (0.218)                 \\\addlinespace
$rK_{c,t}$&       0.149                 &      -0.183                 &       0.395$^{\ast}$        &       0.196                 &      -0.473                 &      -0.114                 &       0.232                 &      -0.591$^{\ast\ast\ast}$&       0.327                 &       0.955$^{\ast\ast}$    &      -1.320$^{\ast\ast\ast}$\\
            &     (0.106)                 &     (0.131)                 &     (0.161)                 &     (0.135)                 &     (0.229)                 &     (0.085)                 &     (0.154)                 &     (0.050)                 &     (0.172)                 &     (0.224)                 &     (0.190)                 \\\addlinespace
$pQ_{c,t}$&       0.233                 &       0.254                 &       0.732                 &      -0.089                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.275)                 &     (0.248)                 &     (0.556)                 &     (0.305)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .995                 &        .998                 &        .996                 &        .992                 &        .998                 &        .996                 &        .994                 \\
$N$      &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 \\


==> inputs/robustness/CTR_KPMG/Results2shortV1_RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 2003-2016}}} \\\midrule
$R_{c,t}$ &      -0.017                 &      -0.035                 &       0.035                 &      -0.040$^{\ast}$        &       0.109                 &      -0.313                 &       0.664                 &      -0.242                 &      -0.959                 &       1.846                 &      -0.924                 \\
            &     (0.012)                 &     (0.024)                 &     (0.052)                 &     (0.022)                 &     (0.603)                 &     (0.339)                 &     (0.499)                 &     (0.144)                 &     (1.002)                 &     (1.183)                 &     (0.665)                 \\\addlinespace
$ICT_{c,t}$&      -0.039                 &      -0.044                 &      -0.009                 &      -0.055                 &      -0.849                 &      -0.116                 &      -1.039                 &       0.305                 &      -0.291                 &      -1.442                 &       1.492                 \\
            &     (0.026)                 &     (0.039)                 &     (0.056)                 &     (0.061)                 &     (0.906)                 &     (0.581)                 &     (0.711)                 &     (0.217)                 &     (1.427)                 &     (1.538)                 &     (0.904)                 \\\addlinespace
$R*ICT_{c,t}$&       0.012                 &       0.012                 &      -0.001                 &       0.040                 &       0.157                 &      -0.242                 &       0.439                 &      -0.040                 &      -0.514                 &       0.836                 &      -0.252                 \\
            &     (0.012)                 &     (0.017)                 &     (0.032)                 &     (0.029)                 &     (0.507)                 &     (0.316)                 &     (0.470)                 &     (0.105)                 &     (0.841)                 &     (1.020)                 &     (0.549)                 \\\addlinespace
$wL_{c,t}$&       0.504$^{\ast\ast\ast}$&       0.083                 &       0.999$^{\ast\ast}$    &       0.467$^{\ast\ast}$    &      -0.541$^{\ast\ast\ast}$&      -0.018                 &       0.232                 &      -0.755$^{\ast\ast\ast}$&       0.320                 &       1.467$^{\ast\ast}$    &      -1.774$^{\ast\ast\ast}$\\
            &     (0.113)                 &     (0.201)                 &     (0.344)                 &     (0.206)                 &     (0.174)                 &     (0.125)                 &     (0.175)                 &     (0.059)                 &     (0.422)                 &     (0.542)                 &     (0.225)                 \\\addlinespace
$rK_{c,t}$&       0.062                 &       0.059                 &       0.215                 &      -0.137                 &      -0.639$^{\ast\ast\ast}$&      -0.035                 &       0.170                 &      -0.774$^{\ast\ast\ast}$&       0.439                 &       1.300$^{\ast\ast\ast}$&      -1.743$^{\ast\ast\ast}$\\
            &     (0.088)                 &     (0.133)                 &     (0.199)                 &     (0.107)                 &     (0.169)                 &     (0.090)                 &     (0.159)                 &     (0.060)                 &     (0.303)                 &     (0.400)                 &     (0.243)                 \\\addlinespace
$pQ_{c,t}$&       0.205                 &       0.652$^{\ast}$        &      -0.529                 &       0.440                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.184)                 &     (0.310)                 &     (0.472)                 &     (0.256)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
%$R^{2}$  &          0.999                &          0.999                &        .999                 &        .999                 &        .979                 &        .991                 &        .983                 &        .978                 &        .988                 &        .982                 &        .972                 \\
$N$      &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 \\


==> inputs/robustness/CTR_KPMG/Results4RICTint_EUKLEMS_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.016                 &       0.028                 &      -0.017                 &      -0.016                 &       0.011$^{\ast\ast}$    &      -1.552$^{\ast\ast}$    &       0.003                 &       0.008$^{\ast}$        \\
            &     (0.028)                 &     (0.018)                 &     (0.025)                 &     (0.032)                 &     (0.004)                 &     (0.503)                 &     (0.006)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&      -0.001                 &       0.003                 &       0.046                 &       0.094                 &      -0.011$^{\ast}$        &       1.994                 &       0.001                 &       0.006                 \\
            &     (0.036)                 &     (0.031)                 &     (0.033)                 &     (0.062)                 &     (0.005)                 &     (1.273)                 &     (0.006)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.031                 &      -0.002                 &      -0.047$^{\ast}$        &      -0.039                 &       0.005                 &      -0.374                 &      -0.002                 &       0.008                 \\
            &     (0.025)                 &     (0.017)                 &     (0.024)                 &     (0.038)                 &     (0.003)                 &     (0.796)                 &     (0.003)                 &     (0.005)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .845                 &          0.999                &        .966                 &        .987                 &        .936                 &        .947                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/CTR_KPMG/Results4RICTint_EUKLEMS_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 2003-2007}}} \\\midrule
$R_{c,t}$ &      -0.339$^{\ast\ast}$    &      -0.054$^{\ast}$        &      -0.230$^{\ast\ast}$    &      -0.087                 &       0.020                 &      -4.130$^{\ast}$        &      -0.012$^{\ast}$        &       0.032                 \\
            &     (0.106)                 &     (0.023)                 &     (0.078)                 &     (0.042)                 &     (0.012)                 &     (1.600)                 &     (0.005)                 &     (0.042)                 \\\addlinespace
$ICT_{c,t}$&      -0.102                 &      -0.042                 &       0.030                 &      -0.131                 &      -0.047$^{\ast\ast}$    &       8.756$^{\ast}$        &       0.010                 &       0.028                 \\
            &     (0.152)                 &     (0.030)                 &     (0.085)                 &     (0.105)                 &     (0.013)                 &     (3.218)                 &     (0.012)                 &     (0.036)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.039                 &      -0.034$^{\ast\ast}$    &      -0.060                 &      -0.006                 &       0.010$^{\ast}$        &      -1.538$^{\ast}$        &      -0.003                 &      -0.008                 \\
            &     (0.053)                 &     (0.010)                 &     (0.038)                 &     (0.042)                 &     (0.004)                 &     (0.658)                 &     (0.005)                 &     (0.012)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .937                 &          0.999                &        .991                 &        .995                 &        .975                 &        .958                 \\
$N$      &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 \\


==> inputs/robustness/CTR_KPMG/Results4RICTint_EUKLEMS_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 2003-2016}}} \\\midrule
$R_{c,t}$ &      -0.089$^{\ast\ast}$    &       0.022                 &      -0.095$^{\ast\ast}$    &      -0.018                 &       0.008$^{\ast\ast}$    &      -1.126$^{\ast\ast\ast}$&       0.017$^{\ast}$        &       0.036$^{\ast\ast}$    \\
            &     (0.037)                 &     (0.017)                 &     (0.040)                 &     (0.026)                 &     (0.003)                 &     (0.366)                 &     (0.008)                 &     (0.016)                 \\\addlinespace
$ICT_{c,t}$&      -0.067                 &      -0.006                 &      -0.049                 &       0.064                 &      -0.016$^{\ast\ast}$    &       4.934$^{\ast\ast\ast}$&       0.016                 &       0.060$^{\ast\ast}$    \\
            &     (0.065)                 &     (0.040)                 &     (0.072)                 &     (0.080)                 &     (0.006)                 &     (0.821)                 &     (0.017)                 &     (0.026)                 \\\addlinespace
$R*ICT_{c,t}$&       0.021                 &      -0.002                 &       0.013                 &      -0.042                 &       0.007$^{\ast\ast}$    &      -1.799$^{\ast\ast\ast}$&      -0.006                 &      -0.024$^{\ast}$        \\
            &     (0.035)                 &     (0.015)                 &     (0.039)                 &     (0.040)                 &     (0.003)                 &     (0.430)                 &     (0.008)                 &     (0.013)                 \\\midrule
$R^{2}$  &        .998                 &        .999                 &        .835                 &        .999                 &         .95                 &        .982                 &        .835                 &        .783                 \\
$N$      &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 \\


==> inputs/robustness/CTR_KPMG/Results4RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.033                 &       0.034                 &      -0.021                 &      -0.007                 &       0.012$^{\ast\ast}$    &      -1.730$^{\ast\ast\ast}$&       0.004                 &       0.008$^{\ast}$        \\
            &     (0.028)                 &     (0.021)                 &     (0.025)                 &     (0.024)                 &     (0.004)                 &     (0.505)                 &     (0.006)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.011                 &       0.009                 &       0.046                 &       0.100$^{\ast}$        &      -0.011$^{\ast\ast}$    &       2.052                 &      -0.000                 &       0.006                 \\
            &     (0.019)                 &     (0.037)                 &     (0.039)                 &     (0.045)                 &     (0.004)                 &     (1.162)                 &     (0.006)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.033$^{\ast\ast}$    &      -0.009                 &      -0.047$^{\ast}$        &      -0.036                 &       0.005$^{\ast}$        &      -0.407                 &      -0.001                 &       0.009                 \\
            &     (0.013)                 &     (0.025)                 &     (0.025)                 &     (0.033)                 &     (0.003)                 &     (0.723)                 &     (0.003)                 &     (0.005)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &         .85                 &          0.999                &        .969                 &        .988                 &        .936                 &        .948                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/CTR_KPMG/Results4RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 2003-2007}}} \\\midrule
$R_{c,t}$ &      -0.275$^{\ast\ast}$    &      -0.123$^{\ast\ast}$    &      -0.222$^{\ast\ast}$    &      -0.091$^{\ast}$        &       0.019                 &      -4.158$^{\ast}$        &      -0.013$^{\ast}$        &       0.033                 \\
            &     (0.095)                 &     (0.041)                 &     (0.073)                 &     (0.037)                 &     (0.011)                 &     (1.531)                 &     (0.006)                 &     (0.042)                 \\\addlinespace
$ICT_{c,t}$&      -0.102                 &      -0.071                 &      -0.005                 &      -0.139                 &      -0.044$^{\ast\ast}$    &       8.827$^{\ast\ast}$    &       0.007                 &       0.022                 \\
            &     (0.158)                 &     (0.042)                 &     (0.109)                 &     (0.091)                 &     (0.013)                 &     (3.086)                 &     (0.010)                 &     (0.036)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.060                 &      -0.005                 &      -0.055                 &       0.004                 &       0.009                 &      -1.477$^{\ast}$        &      -0.002                 &      -0.007                 \\
            &     (0.055)                 &     (0.008)                 &     (0.039)                 &     (0.037)                 &     (0.004)                 &     (0.535)                 &     (0.005)                 &     (0.013)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .939                 &          0.999                &        .991                 &        .995                 &        .975                 &        .958                 \\
$N$      &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 \\


==> inputs/robustness/CTR_KPMG/Results4RICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 2003-2016}}} \\\midrule
$R_{c,t}$ &      -0.091$^{\ast}$        &       0.014                 &      -0.105$^{\ast\ast}$    &      -0.005                 &       0.009$^{\ast\ast}$    &      -1.151$^{\ast\ast\ast}$&       0.018$^{\ast}$        &       0.037$^{\ast\ast}$    \\
            &     (0.043)                 &     (0.019)                 &     (0.039)                 &     (0.023)                 &     (0.003)                 &     (0.342)                 &     (0.009)                 &     (0.016)                 \\\addlinespace
$ICT_{c,t}$&      -0.036                 &       0.003                 &      -0.047                 &       0.091                 &      -0.018$^{\ast\ast\ast}$&       4.974$^{\ast\ast\ast}$&       0.014                 &       0.057$^{\ast}$        \\
            &     (0.072)                 &     (0.043)                 &     (0.075)                 &     (0.069)                 &     (0.005)                 &     (0.962)                 &     (0.017)                 &     (0.027)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.007                 &      -0.001                 &       0.006                 &      -0.048                 &       0.008$^{\ast\ast}$    &      -1.697$^{\ast\ast\ast}$&      -0.005                 &      -0.021                 \\
            &     (0.036)                 &     (0.019)                 &     (0.039)                 &     (0.037)                 &     (0.003)                 &     (0.474)                 &     (0.008)                 &     (0.013)                 \\\midrule
$R^{2}$  &        .998                 &        .999                 &        .846                 &        .999                 &        .951                 &        .982                 &        .836                 &        .781                 \\
$N$      &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 \\


==> inputs/robustness/CTR_KPMG/Results4shortRICTint_ct_All_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.033                 &       0.034                 &      -0.021                 &      -0.007                 &      -1.730$^{\ast\ast\ast}$&       0.008$^{\ast}$        \\
            &     (0.028)                 &     (0.021)                 &     (0.025)                 &     (0.024)                 &     (0.505)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.011                 &       0.009                 &       0.046                 &       0.100$^{\ast}$        &       2.052                 &       0.006                 \\
            &     (0.019)                 &     (0.037)                 &     (0.039)                 &     (0.045)                 &     (1.162)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.033$^{\ast\ast}$    &      -0.009                 &      -0.047$^{\ast}$        &      -0.036                 &      -0.407                 &       0.009                 \\
            &     (0.013)                 &     (0.025)                 &     (0.025)                 &     (0.033)                 &     (0.723)                 &     (0.005)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &         .85                 &          0.999                &        .988                 &        .948                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/CTR_KPMG/Results4shortRICTint_ct_All_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 2003-2007}}} \\\midrule
$R_{c,t}$ &      -0.275$^{\ast\ast}$    &      -0.123$^{\ast\ast}$    &      -0.222$^{\ast\ast}$    &      -0.091$^{\ast}$        &      -4.158$^{\ast}$        &       0.033                 \\
            &     (0.095)                 &     (0.041)                 &     (0.073)                 &     (0.037)                 &     (1.531)                 &     (0.042)                 \\\addlinespace
$ICT_{c,t}$&      -0.102                 &      -0.071                 &      -0.005                 &      -0.139                 &       8.827$^{\ast\ast}$    &       0.022                 \\
            &     (0.158)                 &     (0.042)                 &     (0.109)                 &     (0.091)                 &     (3.086)                 &     (0.036)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.060                 &      -0.005                 &      -0.055                 &       0.004                 &      -1.477$^{\ast}$        &      -0.007                 \\
            &     (0.055)                 &     (0.008)                 &     (0.039)                 &     (0.037)                 &     (0.535)                 &     (0.013)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .939                 &          0.999                &        .995                 &        .958                 \\
$N$      &          95                 &          95                 &          95                 &          95                 &          95                 &          95                 \\


==> inputs/robustness/CTR_KPMG/Results4shortRICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $Services_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 2003-2016}}} \\\midrule
$R_{c,t}$ &      -0.091$^{\ast}$        &       0.014                 &      -0.105$^{\ast\ast}$    &      -0.005                 &      -1.151$^{\ast\ast\ast}$&       0.037$^{\ast\ast}$    \\
            &     (0.043)                 &     (0.019)                 &     (0.039)                 &     (0.023)                 &     (0.342)                 &     (0.016)                 \\\addlinespace
$ICT_{c,t}$&      -0.036                 &       0.003                 &      -0.047                 &       0.091                 &       4.974$^{\ast\ast\ast}$&       0.057$^{\ast}$        \\
            &     (0.072)                 &     (0.043)                 &     (0.075)                 &     (0.069)                 &     (0.962)                 &     (0.027)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.007                 &      -0.001                 &       0.006                 &      -0.048                 &      -1.697$^{\ast\ast\ast}$&      -0.021                 \\
            &     (0.036)                 &     (0.019)                 &     (0.039)                 &     (0.037)                 &     (0.474)                 &     (0.013)                 \\\midrule
%$R^{2}$  &        .998                 &        .999                 &        .846                 &        .999                 &        .982                 &        .781                 \\
$N$      &         266                 &         266                 &         266                 &         266                 &         266                 &         266                 \\


==> inputs/robustness/CTR_KPMG/Results5RICTint_EUKLEMS_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.010                 &      -0.032                 &      -0.012                 &       0.007                 &       0.065$^{\ast\ast}$    &      -0.027$^{\ast}$        &       0.019                 &      -0.005                 \\
            &     (0.034)                 &     (0.046)                 &     (0.026)                 &     (0.028)                 &     (0.023)                 &     (0.013)                 &     (0.022)                 &     (0.011)                 \\\addlinespace
$ICT_{c,t}$&       0.035                 &       0.140$^{\ast}$        &       0.081$^{\ast}$        &       0.060                 &       0.031                 &       0.023                 &       0.021                 &       0.008                 \\
            &     (0.040)                 &     (0.066)                 &     (0.042)                 &     (0.060)                 &     (0.030)                 &     (0.027)                 &     (0.015)                 &     (0.008)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.033                 &      -0.074                 &      -0.055                 &      -0.052                 &      -0.009                 &      -0.029                 &      -0.010                 &       0.004                 \\
            &     (0.031)                 &     (0.042)                 &     (0.031)                 &     (0.037)                 &     (0.021)                 &     (0.017)                 &     (0.012)                 &     (0.008)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &          0.999                &          0.999                &          0.999                &        .891                 &          0.999                &        .991                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         135                 &         135                 &         135                 &         135                 \\


==> inputs/robustness/CTR_KPMG/Results5RICTint_EUKLEMS_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 2003-2007}}} \\\midrule
$R_{c,t}$ &      -0.486$^{\ast\ast}$    &      -0.240$^{\ast}$        &      -0.396$^{\ast\ast}$    &      -0.330$^{\ast}$        &      -0.122                 &      -0.309$^{\ast\ast}$    &       0.005                 &      -0.029$^{\ast}$        \\
            &     (0.155)                 &     (0.092)                 &     (0.119)                 &     (0.120)                 &     (0.081)                 &     (0.090)                 &     (0.094)                 &     (0.014)                 \\\addlinespace
$ICT_{c,t}$&      -0.137                 &      -0.129                 &      -0.137                 &      -0.130                 &      -0.009                 &      -0.052                 &       0.019                 &      -0.056                 \\
            &     (0.190)                 &     (0.168)                 &     (0.177)                 &     (0.180)                 &     (0.093)                 &     (0.105)                 &     (0.141)                 &     (0.047)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.043                 &      -0.025                 &      -0.028                 &      -0.038                 &      -0.022                 &      -0.060                 &      -0.031                 &       0.008                 \\
            &     (0.065)                 &     (0.061)                 &     (0.062)                 &     (0.058)                 &     (0.049)                 &     (0.041)                 &     (0.056)                 &     (0.017)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &          0.999                &          0.999                &          0.999                &        .939                 &          0.999                &        .996                 \\
$N$      &          95                 &          95                 &          95                 &          95                 &          75                 &          75                 &          75                 &          75                 \\


==> inputs/robustness/CTR_KPMG/Results5RICTint_EUKLEMS_ct_All_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 2003-2016}}} \\\midrule
$R_{c,t}$ &      -0.046                 &      -0.063$^{\ast}$        &      -0.058$^{\ast}$        &      -0.041                 &       0.088$^{\ast\ast\ast}$&      -0.073$^{\ast\ast}$    &       0.054$^{\ast}$        &      -0.002                 \\
            &     (0.036)                 &     (0.031)                 &     (0.029)                 &     (0.031)                 &     (0.025)                 &     (0.029)                 &     (0.031)                 &     (0.008)                 \\\addlinespace
$ICT_{c,t}$&      -0.063                 &       0.011                 &      -0.033                 &      -0.057                 &      -0.025                 &      -0.048                 &      -0.022                 &      -0.002                 \\
            &     (0.100)                 &     (0.051)                 &     (0.079)                 &     (0.089)                 &     (0.059)                 &     (0.052)                 &     (0.038)                 &     (0.010)                 \\\addlinespace
$R*ICT_{c,t}$&       0.010                 &      -0.014                 &      -0.003                 &       0.006                 &       0.004                 &       0.022                 &       0.002                 &       0.001                 \\
            &     (0.045)                 &     (0.030)                 &     (0.038)                 &     (0.043)                 &     (0.029)                 &     (0.030)                 &     (0.024)                 &     (0.003)                 \\\midrule
$R^{2}$  &        .999                 &        .998                 &        .999                 &        .999                 &          0.999                &        .884                 &        .999                 &        .985                 \\
$N$      &         266                 &         266                 &         266                 &         266                 &         210                 &         210                 &         210                 &         210                 \\


==> inputs/robustness/CTR_KPMG/Results5RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.008                 &      -0.031                 &      -0.013                 &       0.005                 &       0.063$^{\ast\ast}$    &      -0.027$^{\ast}$        &       0.019                 &      -0.004                 \\
            &     (0.033)                 &     (0.046)                 &     (0.026)                 &     (0.028)                 &     (0.023)                 &     (0.013)                 &     (0.022)                 &     (0.011)                 \\\addlinespace
$ICT_{c,t}$&       0.048                 &       0.128$^{\ast}$        &       0.084$^{\ast}$        &       0.070                 &       0.043                 &       0.023                 &       0.023                 &       0.020$^{\ast\ast\ast}$\\
            &     (0.039)                 &     (0.062)                 &     (0.040)                 &     (0.058)                 &     (0.024)                 &     (0.027)                 &     (0.014)                 &     (0.003)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.040                 &      -0.065                 &      -0.055                 &      -0.056                 &      -0.016                 &      -0.029                 &      -0.011                 &      -0.002                 \\
            &     (0.035)                 &     (0.038)                 &     (0.031)                 &     (0.039)                 &     (0.024)                 &     (0.017)                 &     (0.012)                 &     (0.009)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &          0.999                &          0.999                &          0.999                &        .891                 &          0.999                &        .978                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         135                 &         135                 &         135                 &         135                 \\


==> inputs/robustness/CTR_KPMG/Results5RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 2003-2007}}} \\\midrule
$R_{c,t}$ &      -0.482$^{\ast\ast}$    &      -0.238$^{\ast}$        &      -0.393$^{\ast\ast}$    &      -0.328$^{\ast\ast}$    &      -0.122                 &      -0.308$^{\ast\ast}$    &       0.007                 &      -0.037                 \\
            &     (0.153)                 &     (0.091)                 &     (0.116)                 &     (0.118)                 &     (0.081)                 &     (0.089)                 &     (0.093)                 &     (0.026)                 \\\addlinespace
$ICT_{c,t}$&      -0.165                 &      -0.152                 &      -0.163                 &      -0.146                 &      -0.007                 &      -0.054                 &       0.009                 &      -0.135$^{\ast}$        \\
            &     (0.181)                 &     (0.155)                 &     (0.164)                 &     (0.168)                 &     (0.081)                 &     (0.111)                 &     (0.132)                 &     (0.051)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.031                 &      -0.014                 &      -0.017                 &      -0.029                 &      -0.021                 &      -0.056                 &      -0.025                 &       0.018                 \\
            &     (0.059)                 &     (0.055)                 &     (0.056)                 &     (0.052)                 &     (0.046)                 &     (0.039)                 &     (0.053)                 &     (0.016)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &          0.999                &          0.999                &          0.999                &        .938                 &          0.999                &        .985                 \\
$N$      &          95                 &          95                 &          95                 &          95                 &          75                 &          75                 &          75                 &          75                 \\


==> inputs/robustness/CTR_KPMG/Results5RICTint_ct_All_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 2003-2016}}} \\\midrule
$R_{c,t}$ &      -0.050                 &      -0.065$^{\ast}$        &      -0.062$^{\ast}$        &      -0.044                 &       0.083$^{\ast\ast\ast}$&      -0.074$^{\ast\ast}$    &       0.052                 &      -0.001                 \\
            &     (0.038)                 &     (0.032)                 &     (0.030)                 &     (0.033)                 &     (0.026)                 &     (0.029)                 &     (0.031)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t}$&      -0.025                 &       0.031                 &      -0.001                 &      -0.020                 &       0.007                 &      -0.043                 &      -0.008                 &       0.006                 \\
            &     (0.102)                 &     (0.051)                 &     (0.080)                 &     (0.091)                 &     (0.057)                 &     (0.051)                 &     (0.039)                 &     (0.019)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.009                 &      -0.023                 &      -0.018                 &      -0.012                 &      -0.013                 &       0.018                 &      -0.005                 &      -0.001                 \\
            &     (0.048)                 &     (0.031)                 &     (0.041)                 &     (0.046)                 &     (0.031)                 &     (0.029)                 &     (0.025)                 &     (0.005)                 \\\midrule
%$R^{2}$  &        .999                 &        .998                 &        .999                 &        .999                 &          0.999                &        .884                 &        .999                 &        .953                 \\
$N$      &         266                 &         266                 &         266                 &         266                 &         210                 &         210                 &         210                 &         210                 \\


==> inputs/robustness/ETR_Eurostat/Results1RICTint_EUKLEMS_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.005                 &       0.009                 &       0.029                 &      -0.022                 &       0.551                 &       0.332                 &       0.255                 &      -0.036                 &       0.337                 &       0.404                 &      -0.718                 \\
            &     (0.016)                 &     (0.023)                 &     (0.048)                 &     (0.026)                 &     (0.650)                 &     (0.327)                 &     (0.394)                 &     (0.330)                 &     (0.753)                 &     (1.057)                 &     (0.834)                 \\\addlinespace
$ICT_{c,t}$&      -0.011                 &       0.021                 &       0.013                 &      -0.048                 &      -0.735                 &      -0.288                 &       0.505                 &      -0.952                 &      -0.520                 &       2.363                 &      -1.877                 \\
            &     (0.028)                 &     (0.067)                 &     (0.034)                 &     (0.061)                 &     (0.626)                 &     (0.477)                 &     (0.355)                 &     (0.611)                 &     (1.073)                 &     (1.317)                 &     (1.116)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.002                 &      -0.006                 &       0.002                 &      -0.009                 &       0.257                 &       0.017                 &       0.104                 &       0.136                 &       0.323                 &      -0.567                 &       0.197                 \\
            &     (0.020)                 &     (0.034)                 &     (0.031)                 &     (0.034)                 &     (0.718)                 &     (0.306)                 &     (0.467)                 &     (0.367)                 &     (0.572)                 &     (0.681)                 &     (0.528)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .985                 &        .994                 &         .99                 &         .95                 &        .991                 &        .988                 &        .968                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/ETR_Eurostat/Results1RICTint_EUKLEMS_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 2006-2007}}} \\\midrule
$R_{c,t}$ &      -0.148                 &       0.169                 &      -0.393                 &       0.212                 &      -1.007                 &      -1.126                 &      -3.040                 &       3.159                 &      -1.732                 &      -7.885                 &       9.254                 \\
            &     (0.062)                 &     (0.073)                 &     (0.191)                 &     (0.255)                 &     (0.989)                 &     (1.011)                 &     (2.211)                 &     (1.677)                 &     (2.674)                 &     (5.719)                 &     (4.976)                 \\\addlinespace
$ICT_{c,t}$&      -0.863                 &      -1.293$^{\ast}$        &      -0.715                 &      -0.948                 &     -21.971                 &      -7.578                 &      -6.431                 &      -7.961                 &      -5.631                 &       6.458                 &      -3.999                 \\
            &     (0.238)                 &     (0.154)                 &     (0.663)                 &     (0.698)                 &     (5.903)                 &     (3.426)                 &     (8.190)                 &     (6.412)                 &     (9.277)                 &    (20.249)                 &    (19.462)                 \\\addlinespace
$R*ICT_{c,t}$&       0.127                 &       0.346$^{\ast}$        &      -0.030                 &       0.244                 &       2.161                 &       1.633                 &      -1.653                 &       2.181                 &       3.635                 &      -6.369                 &       3.347                 \\
            &     (0.068)                 &     (0.049)                 &     (0.206)                 &     (0.230)                 &     (1.408)                 &     (1.102)                 &     (2.476)                 &     (1.925)                 &     (2.756)                 &     (6.449)                 &     (6.206)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &        .999                 &        .995                 &          0.999                &        .999                 &        .996                 \\
$N$      &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 \\


==> inputs/robustness/ETR_Eurostat/Results1RICTint_EUKLEMS_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 2006-2016}}} \\\midrule
$R_{c,t}$ &       0.010                 &      -0.021                 &       0.056                 &      -0.005                 &       0.686                 &      -0.085                 &       0.617                 &       0.154                 &      -1.054                 &       1.408                 &      -0.356                 \\
            &     (0.009)                 &     (0.030)                 &     (0.064)                 &     (0.019)                 &     (0.503)                 &     (0.341)                 &     (0.511)                 &     (0.251)                 &     (1.083)                 &     (1.495)                 &     (0.853)                 \\\addlinespace
$ICT_{c,t}$&      -0.031                 &       0.014                 &      -0.002                 &      -0.079                 &      -1.502$^{\ast\ast}$    &      -0.149                 &      -0.174                 &      -1.179                 &       0.397                 &       1.592                 &      -2.169                 \\
            &     (0.023)                 &     (0.060)                 &     (0.052)                 &     (0.063)                 &     (0.600)                 &     (0.472)                 &     (0.634)                 &     (0.696)                 &     (1.224)                 &     (2.062)                 &     (1.510)                 \\\addlinespace
$R*ICT_{c,t}$&       0.009                 &      -0.015                 &       0.010                 &       0.038                 &       0.590                 &      -0.307                 &       0.309                 &       0.588                 &      -1.038                 &      -0.214                 &       1.258                 \\
            &     (0.013)                 &     (0.021)                 &     (0.032)                 &     (0.038)                 &     (0.424)                 &     (0.283)                 &     (0.401)                 &     (0.418)                 &     (0.757)                 &     (1.082)                 &     (0.979)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &        .999                 &        .979                 &        .993                 &        .985                 &        .932                 &        .988                 &        .982                 &        .955                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/ETR_Eurostat/Results1RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.006                 &       0.013                 &       0.033                 &      -0.023                 &       0.582                 &       0.314                 &       0.309                 &      -0.041                 &       0.284                 &       0.496                 &      -0.757                 \\
            &     (0.017)                 &     (0.020)                 &     (0.052)                 &     (0.027)                 &     (0.647)                 &     (0.332)                 &     (0.429)                 &     (0.335)                 &     (0.779)                 &     (1.125)                 &     (0.859)                 \\\addlinespace
$ICT_{c,t}$&      -0.015                 &      -0.005                 &      -0.012                 &      -0.041                 &      -0.911                 &      -0.182                 &       0.158                 &      -0.887                 &      -0.221                 &       1.760                 &      -1.575                 \\
            &     (0.030)                 &     (0.048)                 &     (0.032)                 &     (0.062)                 &     (0.682)                 &     (0.476)                 &     (0.370)                 &     (0.611)                 &     (0.921)                 &     (1.127)                 &     (1.105)                 \\\addlinespace
$R*ICT_{c,t}$&       0.000                 &       0.009                 &       0.016                 &      -0.013                 &       0.336                 &      -0.046                 &       0.294                 &       0.088                 &       0.144                 &      -0.206                 &       0.013                 \\
            &     (0.021)                 &     (0.026)                 &     (0.039)                 &     (0.035)                 &     (0.757)                 &     (0.317)                 &     (0.593)                 &     (0.370)                 &     (0.542)                 &     (0.759)                 &     (0.599)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .985                 &        .994                 &         .99                 &         .95                 &        .991                 &        .988                 &        .968                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/ETR_Eurostat/Results1RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 2006-2007}}} \\\midrule
$R_{c,t}$ &      -0.157                 &       0.136                 &      -0.410                 &       0.226                 &      -0.824                 &      -1.136                 &      -3.342                 &       3.654                 &      -2.008                 &      -8.762                 &      10.468                 \\
            &     (0.056)                 &     (0.095)                 &     (0.168)                 &     (0.255)                 &     (1.140)                 &     (1.027)                 &     (2.295)                 &     (1.734)                 &     (2.783)                 &     (5.745)                 &     (5.076)                 \\\addlinespace
$ICT_{c,t}$&      -1.772                 &      -1.600                 &      -1.380                 &      -2.587                 &     -31.601                 &      -9.570                 &      -2.047                 &     -19.984                 &      -1.939                 &      26.188                 &     -29.429                 \\
            &     (0.341)                 &     (0.443)                 &     (1.079)                 &     (1.343)                 &    (12.556)                 &     (6.256)                 &    (15.185)                 &    (12.986)                 &    (19.822)                 &    (35.241)                 &    (37.088)                 \\\addlinespace
$R*ICT_{c,t}$&       0.256                 &       0.356                 &       0.057                 &       0.505                 &       3.067                 &       1.690                 &      -2.740                 &       4.116                 &       2.727                 &      -9.776                 &       7.925                 \\
            &     (0.071)                 &     (0.082)                 &     (0.238)                 &     (0.259)                 &     (2.150)                 &     (1.289)                 &     (3.211)                 &     (2.503)                 &     (3.800)                 &     (7.878)                 &     (7.441)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &        .999                 &        .995                 &          0.999                &        .999                 &        .996                 \\
$N$      &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 \\


==> inputs/robustness/ETR_Eurostat/Results1RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 2006-2016}}} \\\midrule
$R_{c,t}$ &       0.011                 &      -0.018                 &       0.061                 &      -0.005                 &       0.700                 &      -0.116                 &       0.669                 &       0.147                 &      -1.165                 &       1.545                 &      -0.383                 \\
            &     (0.009)                 &     (0.029)                 &     (0.067)                 &     (0.020)                 &     (0.495)                 &     (0.344)                 &     (0.531)                 &     (0.254)                 &     (1.108)                 &     (1.574)                 &     (0.875)                 \\\addlinespace
$ICT_{c,t}$&      -0.036                 &      -0.011                 &      -0.038                 &      -0.077                 &      -1.706$^{\ast\ast}$    &       0.076                 &      -0.600                 &      -1.181                 &       1.258                 &       0.602                 &      -2.054                 \\
            &     (0.025)                 &     (0.032)                 &     (0.045)                 &     (0.063)                 &     (0.665)                 &     (0.477)                 &     (0.647)                 &     (0.668)                 &     (1.194)                 &     (1.964)                 &     (1.459)                 \\\addlinespace
$R*ICT_{c,t}$&       0.011                 &      -0.003                 &       0.028                 &       0.036                 &       0.637                 &      -0.427                 &       0.507                 &       0.557                 &      -1.463                 &       0.316                 &       1.149                 \\
            &     (0.014)                 &     (0.010)                 &     (0.041)                 &     (0.038)                 &     (0.467)                 &     (0.296)                 &     (0.578)                 &     (0.389)                 &     (0.866)                 &     (1.303)                 &     (0.987)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &        .999                 &        .979                 &        .993                 &        .985                 &        .932                 &        .988                 &        .982                 &        .955                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/ETR_Eurostat/Results2RICTint_EUKLEMS_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.011                 &       0.012                 &       0.017                 &      -0.058                 &       0.227                 &       0.272                 &       0.183                 &      -0.228                 &       0.543                 &       0.420                 &      -0.951                 \\
            &     (0.021)                 &     (0.027)                 &     (0.048)                 &     (0.033)                 &     (0.609)                 &     (0.431)                 &     (0.406)                 &     (0.235)                 &     (0.886)                 &     (0.782)                 &     (0.656)                 \\\addlinespace
$ICT_{c,t}$&       0.023                 &       0.017                 &       0.040                 &       0.023                 &       0.613                 &      -0.222                 &       0.545                 &       0.291$^{\ast\ast}$    &      -1.714                 &       1.118                 &       0.575                 \\
            &     (0.031)                 &     (0.061)                 &     (0.043)                 &     (0.058)                 &     (0.413)                 &     (0.602)                 &     (0.424)                 &     (0.099)                 &     (1.336)                 &     (1.194)                 &     (0.519)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.017                 &      -0.007                 &      -0.012                 &      -0.036                 &      -0.085                 &      -0.014                 &       0.074                 &      -0.145                 &       0.600                 &      -0.342                 &      -0.311                 \\
            &     (0.022)                 &     (0.038)                 &     (0.033)                 &     (0.033)                 &     (0.537)                 &     (0.360)                 &     (0.506)                 &     (0.090)                 &     (0.656)                 &     (0.755)                 &     (0.418)                 \\\addlinespace
$wL_{c,t}$&       0.406$^{\ast\ast\ast}$&       0.349                 &       0.552$^{\ast}$        &       0.372$^{\ast\ast\ast}$&      -0.658$^{\ast\ast\ast}$&       0.044                 &       0.087                 &      -0.789$^{\ast\ast\ast}$&       0.722$^{\ast}$        &       1.093$^{\ast}$        &      -1.805$^{\ast\ast\ast}$\\
            &     (0.070)                 &     (0.189)                 &     (0.271)                 &     (0.098)                 &     (0.179)                 &     (0.075)                 &     (0.216)                 &     (0.086)                 &     (0.332)                 &     (0.546)                 &     (0.337)                 \\\addlinespace
$rK_{c,t}$&       0.019                 &       0.231$^{\ast}$        &       0.149                 &      -0.243$^{\ast\ast}$    &      -0.715$^{\ast\ast\ast}$&       0.020                 &       0.056                 &      -0.791$^{\ast\ast\ast}$&       0.734$^{\ast\ast}$    &       1.012$^{\ast\ast}$    &      -1.741$^{\ast\ast\ast}$\\
            &     (0.055)                 &     (0.111)                 &     (0.109)                 &     (0.076)                 &     (0.138)                 &     (0.037)                 &     (0.162)                 &     (0.090)                 &     (0.247)                 &     (0.377)                 &     (0.298)                 \\\addlinespace
$pQ_{c,t}$&       0.214$^{\ast}$        &       0.097                 &       0.222                 &       0.249                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.105)                 &     (0.344)                 &     (0.281)                 &     (0.137)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.001                 &      -0.003                 &       0.001                 &       0.004$^{\ast\ast}$    &      -0.077                 &      -0.046                 &      -0.018                 &      -0.012                 &      -0.078                 &       0.051                 &       0.023                 \\
            &     (0.001)                 &     (0.003)                 &     (0.005)                 &     (0.002)                 &     (0.059)                 &     (0.030)                 &     (0.032)                 &     (0.008)                 &     (0.064)                 &     (0.085)                 &     (0.051)                 \\\addlinespace
$Services_{c,t}$&      -0.004                 &       0.016$^{\ast\ast\ast}$&      -0.000                 &      -0.020$^{\ast\ast}$    &       0.088                 &       0.097                 &       0.007                 &      -0.016                 &       0.238                 &      -0.123                 &      -0.120                 \\
            &     (0.004)                 &     (0.004)                 &     (0.010)                 &     (0.008)                 &     (0.126)                 &     (0.055)                 &     (0.120)                 &     (0.042)                 &     (0.207)                 &     (0.257)                 &     (0.146)                 \\\addlinespace
$HHI_{c,t}$&      -1.492$^{\ast\ast}$    &       1.008                 &      -2.119                 &      -3.500$^{\ast\ast}$    &      -8.188                 &       7.748                 &     -22.015                 &       6.079                 &      21.270                 &     -52.266                 &      30.231                 \\
            &     (0.574)                 &     (1.091)                 &     (1.894)                 &     (1.302)                 &    (14.832)                 &    (11.319)                 &    (12.254)                 &     (8.755)                 &    (28.940)                 &    (42.694)                 &    (34.878)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast}$        &       0.001                 &      -0.001                 &       0.041$^{\ast\ast}$    &      -0.004                 &       0.019                 &       0.026$^{\ast\ast\ast}$&      -0.041                 &       0.018                 &       0.026$^{\ast}$        \\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.001)                 &     (0.014)                 &     (0.010)                 &     (0.013)                 &     (0.008)                 &     (0.028)                 &     (0.032)                 &     (0.014)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.017$^{\ast\ast}$    &       0.025                 &      -0.022                 &       0.040$^{\ast\ast\ast}$&      -0.558$^{\ast}$        &       0.013                 &      -0.223                 &      -0.348$^{\ast\ast}$    &       0.599$^{\ast}$        &      -0.277                 &      -0.389                 \\
            &     (0.006)                 &     (0.017)                 &     (0.034)                 &     (0.012)                 &     (0.287)                 &     (0.110)                 &     (0.173)                 &     (0.141)                 &     (0.281)                 &     (0.404)                 &     (0.356)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003$^{\ast}$        &       0.001                 &       0.006$^{\ast}$        &       0.001                 &       0.072$^{\ast}$        &       0.007                 &       0.057$^{\ast}$        &       0.008                 &      -0.044                 &       0.105$^{\ast\ast}$    &      -0.068                 \\
            &     (0.001)                 &     (0.002)                 &     (0.003)                 &     (0.002)                 &     (0.036)                 &     (0.011)                 &     (0.028)                 &     (0.013)                 &     (0.028)                 &     (0.042)                 &     (0.042)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.002                 &       0.021$^{\ast}$        &      -0.009                 &      -0.004                 &       0.044                 &       0.094                 &       0.013                 &      -0.063                 &       0.401                 &      -0.186                 &      -0.197                 \\
            &     (0.005)                 &     (0.011)                 &     (0.017)                 &     (0.010)                 &     (0.200)                 &     (0.096)                 &     (0.155)                 &     (0.041)                 &     (0.233)                 &     (0.285)                 &     (0.249)                 \\\addlinespace
$ETR_{c,t}$&       0.004$^{\ast}$        &       0.003                 &       0.011$^{\ast}$        &      -0.001                 &       0.156$^{\ast}$        &       0.038                 &       0.124$^{\ast\ast}$    &      -0.006                 &      -0.037                 &       0.189$^{\ast}$        &      -0.163$^{\ast}$        \\
            &     (0.002)                 &     (0.004)                 &     (0.005)                 &     (0.002)                 &     (0.081)                 &     (0.039)                 &     (0.054)                 &     (0.021)                 &     (0.051)                 &     (0.093)                 &     (0.086)                 \\\addlinespace
$XRate_{c,t}$&       0.007                 &      -0.003                 &       0.013                 &       0.020$^{\ast\ast}$    &       0.006                 &      -0.063                 &       0.049                 &       0.020                 &      -0.274                 &       0.289                 &      -0.015                 \\
            &     (0.006)                 &     (0.011)                 &     (0.010)                 &     (0.008)                 &     (0.205)                 &     (0.100)                 &     (0.198)                 &     (0.048)                 &     (0.215)                 &     (0.299)                 &     (0.174)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .988                 &        .994                 &         .99                 &        .984                 &        .992                 &        .989                 &        .984                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/ETR_Eurostat/Results2RICTint_EUKLEMS_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.070                 &       0.148                 &      -0.114                 &       0.280                 &      -0.533                 &      -0.475                 &      -1.925                 &       1.868                 &      -0.389                 &      -4.458                 &       4.299                 \\
            &     (0.081)                 &     (0.067)                 &     (0.165)                 &     (0.334)                 &     (0.977)                 &     (0.875)                 &     (1.388)                 &     (0.413)                 &     (2.717)                 &     (3.223)                 &     (1.757)                 \\\addlinespace
$ICT_{c,t}$&      -0.845                 &      -1.195                 &      -1.458                 &      -0.399                 &     -25.247                 &     -12.085                 &     -14.371                 &       1.210                 &     -14.959                 &     -17.930                 &      31.018                 \\
            &     (0.257)                 &     (0.226)                 &     (0.590)                 &     (1.077)                 &     (6.532)                 &     (2.810)                 &     (8.327)                 &     (1.889)                 &     (9.804)                 &    (18.219)                 &    (10.496)                 \\\addlinespace
$R*ICT_{c,t}$&       0.113                 &       0.346$^{\ast}$        &      -0.044                 &       0.209                 &       2.407                 &       2.037                 &       0.094                 &       0.277                 &       4.591                 &      -1.096                 &      -3.072                 \\
            &     (0.059)                 &     (0.051)                 &     (0.144)                 &     (0.227)                 &     (1.457)                 &     (0.874)                 &     (1.774)                 &     (0.555)                 &     (2.572)                 &     (4.170)                 &     (2.707)                 \\\addlinespace
$wL_{c,t}$&       0.489                 &      -0.258                 &       2.717                 &      -0.213                 &      -0.025                 &       0.012                 &       0.770                 &      -0.807$^{\ast\ast}$    &       0.114                 &       2.299                 &      -2.468$^{\ast}$        \\
            &     (0.244)                 &     (0.274)                 &     (0.775)                 &     (1.305)                 &     (0.090)                 &     (0.110)                 &     (0.141)                 &     (0.050)                 &     (0.337)                 &     (0.416)                 &     (0.219)                 \\\addlinespace
$rK_{c,t}$&       0.223                 &      -0.005                 &       0.356                 &       0.487                 &      -0.153                 &      -0.148                 &       0.755                 &      -0.760$^{\ast\ast}$    &      -0.186                 &       2.229                 &      -2.071$^{\ast}$        \\
            &     (0.142)                 &     (0.106)                 &     (0.361)                 &     (0.682)                 &     (0.098)                 &     (0.117)                 &     (0.157)                 &     (0.056)                 &     (0.355)                 &     (0.396)                 &     (0.234)                 \\\addlinespace
$pQ_{c,t}$&       0.289                 &       1.888                 &      -3.318                 &       1.177                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.410)                 &     (0.406)                 &     (1.334)                 &     (2.252)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &       0.003                 &       0.003                 &      -0.002                 &      -0.039                 &       0.049                 &      -0.075                 &      -0.013                 &       0.193                 &      -0.168                 &      -0.056                 \\
            &     (0.003)                 &     (0.003)                 &     (0.007)                 &     (0.013)                 &     (0.053)                 &     (0.048)                 &     (0.071)                 &     (0.023)                 &     (0.145)                 &     (0.172)                 &     (0.095)                 \\\addlinespace
$Services_{c,t}$&       0.012                 &       0.021                 &      -0.006                 &       0.018                 &       0.451                 &       0.198                 &       0.049                 &       0.204                 &       0.078                 &      -0.411                 &       0.390                 \\
            &     (0.006)                 &     (0.005)                 &     (0.014)                 &     (0.022)                 &     (0.120)                 &     (0.082)                 &     (0.147)                 &     (0.054)                 &     (0.225)                 &     (0.342)                 &     (0.253)                 \\\addlinespace
$HHI_{c,t}$&       1.887                 &       9.422                 &      -9.666                 &       4.485                 &     106.696                 &      30.648                 &       4.798                 &      71.250$^{\ast}$        &     -19.160                 &    -162.688                 &     211.696                 \\
            &     (1.762)                 &     (2.247)                 &     (5.387)                 &     (9.192)                 &    (18.864)                 &    (26.958)                 &    (34.465)                 &    (10.156)                 &    (89.830)                 &   (124.015)                 &    (50.327)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.011$^{\ast}$        &       0.006                 &       0.002                 &      -0.078                 &      -0.118                 &       0.068                 &      -0.028                 &      -0.224                 &       0.221                 &      -0.009                 \\
            &     (0.003)                 &     (0.001)                 &     (0.004)                 &     (0.010)                 &     (0.056)                 &     (0.023)                 &     (0.076)                 &     (0.015)                 &     (0.090)                 &     (0.166)                 &     (0.088)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.058                 &       0.325$^{\ast}$        &      -0.218                 &       0.080                 &       3.059                 &       2.015                 &      -0.056                 &       1.100                 &       2.962                 &      -3.447                 &       1.130                 \\
            &     (0.035)                 &     (0.030)                 &     (0.090)                 &     (0.166)                 &     (0.518)                 &     (0.592)                 &     (0.859)                 &     (0.208)                 &     (1.974)                 &     (2.489)                 &     (0.884)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.009                 &      -0.042$^{\ast}$        &       0.061                 &      -0.011                 &       0.139                 &      -0.147                 &       0.482                 &      -0.196                 &      -0.551                 &       1.234                 &      -0.716                 \\
            &     (0.007)                 &     (0.006)                 &     (0.015)                 &     (0.030)                 &     (0.125)                 &     (0.076)                 &     (0.165)                 &     (0.046)                 &     (0.240)                 &     (0.369)                 &     (0.227)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.017                 &       0.012                 &      -0.004                 &       0.008                 &       0.709                 &      -0.063                 &       0.354                 &       0.418                 &      -0.862                 &      -0.343                 &       1.482                 \\
            &     (0.013)                 &     (0.015)                 &     (0.036)                 &     (0.066)                 &     (0.189)                 &     (0.209)                 &     (0.304)                 &     (0.090)                 &     (0.686)                 &     (0.953)                 &     (0.442)                 \\\addlinespace
$ETR_{c,t}$&      -0.010                 &       0.003                 &      -0.027                 &       0.002                 &      -0.266                 &       0.006                 &      -0.333                 &       0.060                 &       0.200                 &      -0.598                 &       0.390                 \\
            &     (0.002)                 &     (0.002)                 &     (0.006)                 &     (0.012)                 &     (0.043)                 &     (0.038)                 &     (0.055)                 &     (0.016)                 &     (0.117)                 &     (0.136)                 &     (0.063)                 \\\addlinespace
$XRate_{c,t}$&      -0.096                 &      -0.122                 &      -0.174                 &      -0.018                 &      -2.933                 &      -1.414                 &      -1.678                 &       0.160                 &      -1.626                 &      -1.857                 &       3.208                 \\
            &     (0.026)                 &     (0.020)                 &     (0.055)                 &     (0.109)                 &     (0.678)                 &     (0.276)                 &     (0.866)                 &     (0.176)                 &     (1.004)                 &     (1.831)                 &     (0.996)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                \\
$N$      &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 \\


==> inputs/robustness/ETR_Eurostat/Results2RICTint_EUKLEMS_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.007                 &      -0.016                 &       0.027                 &      -0.035                 &       0.207                 &      -0.122                 &       0.475                 &      -0.145                 &      -0.573                 &       1.376                 &      -0.823                 \\
            &     (0.009)                 &     (0.025)                 &     (0.048)                 &     (0.023)                 &     (0.546)                 &     (0.335)                 &     (0.462)                 &     (0.173)                 &     (0.984)                 &     (1.081)                 &     (0.628)                 \\\addlinespace
$ICT_{c,t}$&      -0.000                 &       0.004                 &       0.050                 &      -0.023                 &      -0.031                 &      -0.093                 &      -0.164                 &       0.226$^{\ast\ast\ast}$&      -0.922                 &       0.046                 &       0.701                 \\
            &     (0.024)                 &     (0.049)                 &     (0.062)                 &     (0.065)                 &     (0.595)                 &     (0.516)                 &     (0.693)                 &     (0.070)                 &     (1.485)                 &     (1.554)                 &     (0.559)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.005                 &      -0.014                 &      -0.016                 &       0.017                 &      -0.031                 &      -0.326                 &       0.341                 &      -0.046                 &      -0.494                 &       0.578                 &      -0.077                 \\
            &     (0.014)                 &     (0.017)                 &     (0.031)                 &     (0.041)                 &     (0.359)                 &     (0.294)                 &     (0.444)                 &     (0.068)                 &     (0.825)                 &     (0.918)                 &     (0.386)                 \\\addlinespace
$wL_{c,t}$&       0.387$^{\ast\ast\ast}$&       0.140                 &       0.835$^{\ast\ast}$    &       0.299                 &      -0.552$^{\ast\ast\ast}$&       0.014                 &       0.255                 &      -0.820$^{\ast\ast\ast}$&       0.401                 &       1.573$^{\ast\ast\ast}$&      -1.945$^{\ast\ast\ast}$\\
            &     (0.095)                 &     (0.205)                 &     (0.346)                 &     (0.194)                 &     (0.153)                 &     (0.107)                 &     (0.153)                 &     (0.052)                 &     (0.412)                 &     (0.468)                 &     (0.157)                 \\\addlinespace
$rK_{c,t}$&      -0.006                 &       0.154                 &       0.093                 &      -0.245$^{\ast\ast}$    &      -0.654$^{\ast\ast\ast}$&      -0.003                 &       0.161                 &      -0.812$^{\ast\ast\ast}$&       0.526                 &       1.321$^{\ast\ast\ast}$&      -1.831$^{\ast\ast\ast}$\\
            &     (0.079)                 &     (0.130)                 &     (0.129)                 &     (0.104)                 &     (0.150)                 &     (0.063)                 &     (0.142)                 &     (0.062)                 &     (0.299)                 &     (0.337)                 &     (0.183)                 \\\addlinespace
$pQ_{c,t}$&       0.263                 &       0.517                 &      -0.246                 &       0.396                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.158)                 &     (0.351)                 &     (0.448)                 &     (0.276)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.005                 &       0.005                 &       0.001                 &      -0.073                 &      -0.060                 &       0.002                 &      -0.015$^{\ast}$        &      -0.156                 &       0.140                 &       0.016                 \\
            &     (0.002)                 &     (0.004)                 &     (0.005)                 &     (0.003)                 &     (0.044)                 &     (0.035)                 &     (0.030)                 &     (0.007)                 &     (0.098)                 &     (0.093)                 &     (0.040)                 \\\addlinespace
$Services_{c,t}$&      -0.011$^{\ast\ast}$    &       0.019$^{\ast\ast\ast}$&      -0.020                 &      -0.022$^{\ast\ast}$    &      -0.109                 &       0.107                 &      -0.241$^{\ast}$        &       0.025                 &       0.472                 &      -0.655$^{\ast}$        &       0.174                 \\
            &     (0.004)                 &     (0.006)                 &     (0.012)                 &     (0.009)                 &     (0.130)                 &     (0.077)                 &     (0.121)                 &     (0.044)                 &     (0.275)                 &     (0.321)                 &     (0.152)                 \\\addlinespace
$HHI_{c,t}$&      -2.239$^{\ast\ast\ast}$&       1.749$^{\ast}$        &      -3.736$^{\ast}$        &      -3.812$^{\ast\ast}$    &     -31.018                 &      14.883                 &     -53.702$^{\ast\ast}$    &       7.801                 &      66.382                 &    -133.044$^{\ast}$        &      63.158$^{\ast}$        \\
            &     (0.523)                 &     (0.861)                 &     (1.990)                 &     (1.354)                 &    (21.287)                 &    (12.662)                 &    (21.242)                 &     (8.403)                 &    (50.329)                 &    (64.302)                 &    (31.524)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast}$        &       0.001                 &      -0.001                 &       0.049$^{\ast\ast\ast}$&      -0.011                 &       0.034$^{\ast\ast}$    &       0.026$^{\ast\ast\ast}$&      -0.075$^{\ast}$        &       0.058                 &       0.019                 \\
            &     (0.001)                 &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.013)                 &     (0.009)                 &     (0.015)                 &     (0.008)                 &     (0.038)                 &     (0.040)                 &     (0.014)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.017$^{\ast\ast}$    &       0.020$^{\ast\ast}$    &      -0.014                 &       0.036$^{\ast\ast}$    &      -0.652$^{\ast\ast}$    &       0.003                 &      -0.249                 &      -0.407$^{\ast\ast}$    &       0.663$^{\ast\ast\ast}$&      -0.245                 &      -0.493                 \\
            &     (0.007)                 &     (0.009)                 &     (0.031)                 &     (0.015)                 &     (0.237)                 &     (0.099)                 &     (0.154)                 &     (0.140)                 &     (0.205)                 &     (0.344)                 &     (0.360)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.004$^{\ast\ast}$    &       0.000                 &       0.007$^{\ast\ast}$    &       0.003                 &       0.108$^{\ast\ast}$    &       0.011                 &       0.082$^{\ast\ast}$    &       0.016                 &      -0.055                 &       0.138$^{\ast\ast}$    &      -0.081$^{\ast}$        \\
            &     (0.002)                 &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.044)                 &     (0.013)                 &     (0.033)                 &     (0.011)                 &     (0.047)                 &     (0.050)                 &     (0.041)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.002                 &       0.024$^{\ast}$        &      -0.002                 &      -0.007                 &       0.026                 &       0.127                 &      -0.011                 &      -0.090$^{\ast}$        &       0.487$^{\ast}$        &      -0.277                 &      -0.210                 \\
            &     (0.006)                 &     (0.013)                 &     (0.019)                 &     (0.011)                 &     (0.229)                 &     (0.080)                 &     (0.181)                 &     (0.049)                 &     (0.235)                 &     (0.355)                 &     (0.238)                 \\\addlinespace
$ETR_{c,t}$&       0.003$^{\ast}$        &       0.003                 &       0.012$^{\ast\ast}$    &      -0.003                 &       0.136                 &       0.036                 &       0.120$^{\ast}$        &      -0.020                 &      -0.035                 &       0.215$^{\ast\ast}$    &      -0.198$^{\ast\ast}$    \\
            &     (0.002)                 &     (0.002)                 &     (0.005)                 &     (0.002)                 &     (0.078)                 &     (0.024)                 &     (0.056)                 &     (0.019)                 &     (0.044)                 &     (0.093)                 &     (0.082)                 \\\addlinespace
$XRate_{c,t}$&       0.006                 &       0.004                 &       0.017$^{\ast\ast}$    &      -0.000                 &       0.122                 &       0.073                 &       0.063                 &      -0.014                 &       0.049                 &       0.141                 &      -0.187$^{\ast}$        \\
            &     (0.004)                 &     (0.003)                 &     (0.005)                 &     (0.010)                 &     (0.113)                 &     (0.076)                 &     (0.112)                 &     (0.025)                 &     (0.194)                 &     (0.217)                 &     (0.095)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .982                 &        .993                 &        .985                 &        .982                 &        .989                 &        .985                 &        .979                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/ETR_Eurostat/Results2RICTint_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.010                 &       0.017                 &       0.022                 &      -0.059                 &       0.281                 &       0.251                 &       0.253                 &      -0.223                 &       0.461                 &       0.526                 &      -0.976                 \\
            &     (0.022)                 &     (0.024)                 &     (0.051)                 &     (0.033)                 &     (0.618)                 &     (0.459)                 &     (0.432)                 &     (0.236)                 &     (0.915)                 &     (0.812)                 &     (0.655)                 \\\addlinespace
$ICT_{c,t}$&       0.018                 &      -0.007                 &       0.016                 &       0.026                 &       0.305                 &      -0.112                 &       0.157                 &       0.260$^{\ast\ast\ast}$&      -1.280                 &       0.550                 &       0.705                 \\
            &     (0.032)                 &     (0.052)                 &     (0.035)                 &     (0.057)                 &     (0.478)                 &     (0.584)                 &     (0.473)                 &     (0.056)                 &     (1.107)                 &     (0.878)                 &     (0.527)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.014                 &       0.005                 &       0.001                 &      -0.037                 &       0.075                 &      -0.075                 &       0.276                 &      -0.126                 &       0.345                 &      -0.030                 &      -0.369                 \\
            &     (0.022)                 &     (0.034)                 &     (0.037)                 &     (0.033)                 &     (0.623)                 &     (0.363)                 &     (0.628)                 &     (0.093)                 &     (0.605)                 &     (0.772)                 &     (0.450)                 \\\addlinespace
$wL_{c,t}$&       0.405$^{\ast\ast\ast}$&       0.340                 &       0.544$^{\ast}$        &       0.374$^{\ast\ast\ast}$&      -0.650$^{\ast\ast\ast}$&       0.041                 &       0.096                 &      -0.788$^{\ast\ast\ast}$&       0.712$^{\ast}$        &       1.104$^{\ast}$        &      -1.807$^{\ast\ast\ast}$\\
            &     (0.069)                 &     (0.188)                 &     (0.265)                 &     (0.097)                 &     (0.182)                 &     (0.076)                 &     (0.222)                 &     (0.085)                 &     (0.339)                 &     (0.558)                 &     (0.337)                 \\\addlinespace
$rK_{c,t}$&       0.022                 &       0.239$^{\ast}$        &       0.158                 &      -0.243$^{\ast\ast}$    &      -0.704$^{\ast\ast\ast}$&       0.016                 &       0.070                 &      -0.790$^{\ast\ast\ast}$&       0.718$^{\ast\ast}$    &       1.030$^{\ast\ast}$    &      -1.743$^{\ast\ast\ast}$\\
            &     (0.055)                 &     (0.118)                 &     (0.114)                 &     (0.073)                 &     (0.143)                 &     (0.037)                 &     (0.169)                 &     (0.088)                 &     (0.249)                 &     (0.391)                 &     (0.297)                 \\\addlinespace
$pQ_{c,t}$&       0.213$^{\ast}$        &       0.107                 &       0.228                 &       0.245$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.104)                 &     (0.345)                 &     (0.278)                 &     (0.130)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.001                 &      -0.003                 &       0.001                 &       0.004$^{\ast\ast}$    &      -0.076                 &      -0.046                 &      -0.018                 &      -0.012                 &      -0.078                 &       0.051                 &       0.023                 \\
            &     (0.001)                 &     (0.004)                 &     (0.004)                 &     (0.002)                 &     (0.058)                 &     (0.030)                 &     (0.032)                 &     (0.008)                 &     (0.063)                 &     (0.086)                 &     (0.051)                 \\\addlinespace
$Services_{c,t}$&      -0.003                 &       0.017$^{\ast\ast\ast}$&       0.000                 &      -0.020$^{\ast\ast}$    &       0.093                 &       0.096                 &       0.013                 &      -0.015                 &       0.231                 &      -0.115                 &      -0.121                 \\
            &     (0.004)                 &     (0.004)                 &     (0.010)                 &     (0.008)                 &     (0.128)                 &     (0.054)                 &     (0.121)                 &     (0.042)                 &     (0.209)                 &     (0.255)                 &     (0.147)                 \\\addlinespace
$HHI_{c,t}$&      -1.495$^{\ast\ast}$    &       0.959                 &      -2.165                 &      -3.485$^{\ast\ast}$    &      -9.118                 &       8.083                 &     -23.212$^{\ast}$        &       6.010                 &      22.479                 &     -53.927                 &      30.678                 \\
            &     (0.581)                 &     (1.071)                 &     (1.885)                 &     (1.305)                 &    (14.731)                 &    (11.543)                 &    (12.337)                 &     (8.701)                 &    (29.795)                 &    (43.342)                 &    (34.744)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast}$        &       0.001                 &      -0.001                 &       0.041$^{\ast\ast}$    &      -0.004                 &       0.019                 &       0.026$^{\ast\ast\ast}$&      -0.041                 &       0.018                 &       0.026$^{\ast}$        \\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.001)                 &     (0.014)                 &     (0.010)                 &     (0.013)                 &     (0.008)                 &     (0.028)                 &     (0.032)                 &     (0.014)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.017$^{\ast\ast}$    &       0.024                 &      -0.022                 &       0.040$^{\ast\ast\ast}$&      -0.550$^{\ast}$        &       0.010                 &      -0.213                 &      -0.346$^{\ast\ast}$    &       0.585$^{\ast}$        &      -0.262                 &      -0.390                 \\
            &     (0.006)                 &     (0.018)                 &     (0.034)                 &     (0.011)                 &     (0.287)                 &     (0.107)                 &     (0.162)                 &     (0.141)                 &     (0.269)                 &     (0.401)                 &     (0.353)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003$^{\ast}$        &       0.001                 &       0.006$^{\ast}$        &       0.001                 &       0.073$^{\ast}$        &       0.006                 &       0.059$^{\ast}$        &       0.008                 &      -0.045                 &       0.107$^{\ast\ast}$    &      -0.068                 \\
            &     (0.001)                 &     (0.002)                 &     (0.003)                 &     (0.002)                 &     (0.036)                 &     (0.011)                 &     (0.028)                 &     (0.013)                 &     (0.028)                 &     (0.042)                 &     (0.042)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.002                 &       0.021                 &      -0.009                 &      -0.004                 &       0.052                 &       0.091                 &       0.022                 &      -0.061                 &       0.386                 &      -0.172                 &      -0.196                 \\
            &     (0.005)                 &     (0.011)                 &     (0.017)                 &     (0.009)                 &     (0.203)                 &     (0.094)                 &     (0.159)                 &     (0.041)                 &     (0.237)                 &     (0.291)                 &     (0.254)                 \\\addlinespace
$XRate_{c,t}$&       0.007                 &      -0.005                 &       0.011                 &       0.020$^{\ast\ast}$    &      -0.018                 &      -0.053                 &       0.017                 &       0.018                 &      -0.237                 &       0.238                 &      -0.000                 \\
            &     (0.006)                 &     (0.012)                 &     (0.011)                 &     (0.009)                 &     (0.223)                 &     (0.104)                 &     (0.220)                 &     (0.050)                 &     (0.212)                 &     (0.298)                 &     (0.178)                 \\\addlinespace
$ETR_{c,t}$&       0.004$^{\ast}$        &       0.003                 &       0.011$^{\ast}$        &      -0.001                 &       0.156$^{\ast}$        &       0.038                 &       0.124$^{\ast}$        &      -0.006                 &      -0.037                 &       0.189$^{\ast}$        &      -0.162$^{\ast}$        \\
            &     (0.002)                 &     (0.004)                 &     (0.005)                 &     (0.002)                 &     (0.080)                 &     (0.039)                 &     (0.054)                 &     (0.021)                 &     (0.051)                 &     (0.093)                 &     (0.086)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .988                 &        .994                 &         .99                 &        .984                 &        .992                 &        .989                 &        .984                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/ETR_Eurostat/Results2RICTint_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.130                 &       0.091                 &      -0.212                 &       0.241                 &      -0.653                 &      -0.652                 &      -1.990                 &       1.988                 &      -0.882                 &      -4.258                 &       4.623                 \\
            &     (0.077)                 &     (0.087)                 &     (0.190)                 &     (0.341)                 &     (1.362)                 &     (0.868)                 &     (1.728)                 &     (0.421)                 &     (2.690)                 &     (3.608)                 &     (2.115)                 \\\addlinespace
$ICT_{c,t}$&      -1.777                 &      -1.453                 &      -1.905                 &      -2.026                 &     -32.988                 &     -13.633                 &     -19.156                 &      -0.199                 &     -11.824                 &     -28.743                 &      37.544                 \\
            &     (0.374)                 &     (0.627)                 &     (1.281)                 &     (1.668)                 &    (15.777)                 &     (5.174)                 &    (18.371)                 &     (3.157)                 &    (18.784)                 &    (36.950)                 &    (21.266)                 \\\addlinespace
$R*ICT_{c,t}$&       0.242                 &       0.369                 &      -0.011                 &       0.461                 &       3.152                 &       1.988                 &       0.597                 &       0.567                 &       3.611                 &       0.448                 &      -3.467                 \\
            &     (0.068)                 &     (0.097)                 &     (0.225)                 &     (0.283)                 &     (2.760)                 &     (1.092)                 &     (3.229)                 &     (0.682)                 &     (3.582)                 &     (6.787)                 &     (4.054)                 \\\addlinespace
$wL_{c,t}$&       0.257                 &      -0.548                 &       2.317                 &      -0.332                 &      -0.002                 &       0.011                 &       0.784                 &      -0.797$^{\ast\ast}$    &       0.084                 &       2.344                 &      -2.479$^{\ast}$        \\
            &     (0.159)                 &     (0.410)                 &     (0.976)                 &     (1.187)                 &     (0.187)                 &     (0.117)                 &     (0.210)                 &     (0.055)                 &     (0.339)                 &     (0.507)                 &     (0.338)                 \\\addlinespace
$rK_{c,t}$&       0.058                 &      -0.058                 &       0.291                 &       0.189                 &      -0.048                 &      -0.110                 &       0.823                 &      -0.761$^{\ast\ast}$    &      -0.170                 &       2.341                 &      -2.190                 \\
            &     (0.126)                 &     (0.198)                 &     (0.424)                 &     (0.633)                 &     (0.211)                 &     (0.122)                 &     (0.230)                 &     (0.058)                 &     (0.342)                 &     (0.502)                 &     (0.357)                 \\\addlinespace
$pQ_{c,t}$&       0.683                 &       2.303                 &      -2.801                 &       1.531                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.279)                 &     (0.667)                 &     (1.689)                 &     (2.142)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.001                 &       0.002                 &       0.001                 &       0.004                 &      -0.059                 &       0.031                 &      -0.086                 &      -0.004                 &       0.153                 &      -0.164                 &      -0.019                 \\
            &     (0.002)                 &     (0.004)                 &     (0.008)                 &     (0.011)                 &     (0.088)                 &     (0.049)                 &     (0.098)                 &     (0.023)                 &     (0.141)                 &     (0.205)                 &     (0.131)                 \\\addlinespace
$Services_{c,t}$&       0.009                 &       0.024                 &      -0.002                 &       0.008                 &       0.535                 &       0.247                 &       0.099                 &       0.189                 &       0.160                 &      -0.373                 &       0.272                 \\
            &     (0.006)                 &     (0.006)                 &     (0.014)                 &     (0.019)                 &     (0.128)                 &     (0.081)                 &     (0.149)                 &     (0.049)                 &     (0.222)                 &     (0.335)                 &     (0.242)                 \\\addlinespace
$HHI_{c,t}$&       3.890                 &      11.662                 &      -5.720                 &       5.183                 &     157.071                 &      50.836                 &      37.749                 &      68.485$^{\ast}$        &      -3.095                 &    -115.108                 &     151.384                 \\
            &     (0.876)                 &     (3.166)                 &     (6.610)                 &     (7.433)                 &    (42.720)                 &    (32.530)                 &    (41.817)                 &    (10.407)                 &    (88.895)                 &   (119.139)                 &    (70.229)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.003                 &      -0.009                 &       0.012                 &       0.003                 &       0.004                 &      -0.085                 &       0.122                 &      -0.033                 &      -0.195                 &       0.298                 &      -0.109                 \\
            &     (0.002)                 &     (0.002)                 &     (0.005)                 &     (0.008)                 &     (0.092)                 &     (0.028)                 &     (0.090)                 &     (0.016)                 &     (0.068)                 &     (0.175)                 &     (0.131)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.064                 &       0.326$^{\ast}$        &      -0.227                 &       0.101                 &       2.715                 &       1.799                 &      -0.248                 &       1.163                 &       2.579                 &      -3.566                 &       1.624                 \\
            &     (0.035)                 &     (0.043)                 &     (0.110)                 &     (0.171)                 &     (0.642)                 &     (0.707)                 &     (0.810)                 &     (0.204)                 &     (2.071)                 &     (2.308)                 &     (0.957)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.007                 &      -0.042                 &       0.062                 &      -0.017                 &       0.153                 &      -0.125                 &       0.487                 &      -0.208                 &      -0.490                 &       1.208                 &      -0.752                 \\
            &     (0.007)                 &     (0.009)                 &     (0.019)                 &     (0.031)                 &     (0.189)                 &     (0.087)                 &     (0.212)                 &     (0.047)                 &     (0.259)                 &     (0.441)                 &     (0.287)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.040                 &       0.033                 &       0.036                 &       0.022                 &       1.160                 &       0.127                 &       0.648                 &       0.385                 &      -0.685                 &       0.061                 &       0.928                 \\
            &     (0.007)                 &     (0.022)                 &     (0.045)                 &     (0.053)                 &     (0.369)                 &     (0.236)                 &     (0.352)                 &     (0.083)                 &     (0.628)                 &     (0.885)                 &     (0.581)                 \\\addlinespace
$XRate_{c,t}$&      -0.184                 &      -0.139                 &      -0.214                 &      -0.174                 &      -3.514                 &      -1.482                 &      -2.058                 &       0.025                 &      -1.215                 &      -2.795                 &       3.640                 \\
            &     (0.038)                 &     (0.063)                 &     (0.123)                 &     (0.169)                 &     (1.538)                 &     (0.512)                 &     (1.766)                 &     (0.282)                 &     (1.832)                 &     (3.512)                 &     (1.986)                 \\\addlinespace
$ETR_{c,t}$&      -0.020                 &      -0.001                 &      -0.036                 &      -0.012                 &      -0.368                 &      -0.023                 &      -0.400                 &       0.055                 &       0.208                 &      -0.721                 &       0.495                 \\
            &     (0.003)                 &     (0.006)                 &     (0.013)                 &     (0.017)                 &     (0.134)                 &     (0.057)                 &     (0.139)                 &     (0.024)                 &     (0.163)                 &     (0.273)                 &     (0.175)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &        .999                 \\
$N$      &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 \\


==> inputs/robustness/ETR_Eurostat/Results2RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.006                 &      -0.013                 &       0.032                 &      -0.036                 &       0.247                 &      -0.159                 &       0.540                 &      -0.135                 &      -0.729                 &       1.527                 &      -0.818                 \\
            &     (0.009)                 &     (0.025)                 &     (0.051)                 &     (0.023)                 &     (0.548)                 &     (0.336)                 &     (0.483)                 &     (0.170)                 &     (1.020)                 &     (1.138)                 &     (0.603)                 \\\addlinespace
$ICT_{c,t}$&      -0.003                 &      -0.020                 &       0.018                 &      -0.022                 &      -0.322                 &       0.146                 &      -0.635                 &       0.168$^{\ast\ast}$    &       0.078                 &      -0.991                 &       0.722                 \\
            &     (0.025)                 &     (0.025)                 &     (0.043)                 &     (0.064)                 &     (0.628)                 &     (0.509)                 &     (0.740)                 &     (0.057)                 &     (1.394)                 &     (1.523)                 &     (0.500)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.003                 &      -0.002                 &       0.001                 &       0.017                 &       0.098                 &      -0.449                 &       0.559                 &      -0.012                 &      -1.016                 &       1.082                 &      -0.060                 \\
            &     (0.014)                 &     (0.009)                 &     (0.034)                 &     (0.039)                 &     (0.487)                 &     (0.300)                 &     (0.604)                 &     (0.067)                 &     (0.964)                 &     (1.140)                 &     (0.416)                 \\\addlinespace
$wL_{c,t}$&       0.386$^{\ast\ast\ast}$&       0.131                 &       0.826$^{\ast\ast}$    &       0.298                 &      -0.546$^{\ast\ast\ast}$&       0.008                 &       0.265                 &      -0.818$^{\ast\ast\ast}$&       0.377                 &       1.595$^{\ast\ast\ast}$&      -1.945$^{\ast\ast\ast}$\\
            &     (0.095)                 &     (0.206)                 &     (0.342)                 &     (0.194)                 &     (0.155)                 &     (0.106)                 &     (0.157)                 &     (0.051)                 &     (0.417)                 &     (0.477)                 &     (0.156)                 \\\addlinespace
$rK_{c,t}$&      -0.006                 &       0.159                 &       0.103                 &      -0.247$^{\ast\ast}$    &      -0.646$^{\ast\ast\ast}$&      -0.010                 &       0.174                 &      -0.810$^{\ast\ast\ast}$&       0.496                 &       1.352$^{\ast\ast\ast}$&      -1.830$^{\ast\ast\ast}$\\
            &     (0.079)                 &     (0.134)                 &     (0.132)                 &     (0.101)                 &     (0.153)                 &     (0.062)                 &     (0.148)                 &     (0.061)                 &     (0.303)                 &     (0.350)                 &     (0.182)                 \\\addlinespace
$pQ_{c,t}$&       0.265                 &       0.528                 &      -0.237                 &       0.401                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.157)                 &     (0.352)                 &     (0.446)                 &     (0.274)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.000                 &      -0.005                 &       0.005                 &       0.001                 &      -0.072                 &      -0.060                 &       0.003                 &      -0.015$^{\ast}$        &      -0.158                 &       0.142                 &       0.016                 \\
            &     (0.002)                 &     (0.004)                 &     (0.005)                 &     (0.003)                 &     (0.043)                 &     (0.034)                 &     (0.029)                 &     (0.007)                 &     (0.098)                 &     (0.093)                 &     (0.040)                 \\\addlinespace
$Services_{c,t}$&      -0.011$^{\ast\ast}$    &       0.019$^{\ast\ast\ast}$&      -0.019                 &      -0.023$^{\ast\ast}$    &      -0.104                 &       0.103                 &      -0.234$^{\ast}$        &       0.027                 &       0.456                 &      -0.640$^{\ast}$        &       0.174                 \\
            &     (0.004)                 &     (0.006)                 &     (0.012)                 &     (0.009)                 &     (0.133)                 &     (0.076)                 &     (0.124)                 &     (0.045)                 &     (0.266)                 &     (0.320)                 &     (0.155)                 \\\addlinespace
$HHI_{c,t}$&      -2.244$^{\ast\ast\ast}$&       1.716$^{\ast}$        &      -3.764$^{\ast}$        &      -3.828$^{\ast\ast}$    &     -31.582                 &      15.468                 &     -54.769$^{\ast\ast}$    &       7.719                 &      68.551                 &    -135.375$^{\ast}$        &      63.282$^{\ast}$        \\
            &     (0.524)                 &     (0.856)                 &     (1.982)                 &     (1.354)                 &    (21.053)                 &    (12.587)                 &    (21.255)                 &     (8.382)                 &    (50.792)                 &    (64.781)                 &    (31.537)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002                 &       0.002                 &      -0.001                 &       0.049$^{\ast\ast\ast}$&      -0.011                 &       0.034$^{\ast\ast}$    &       0.026$^{\ast\ast\ast}$&      -0.075$^{\ast}$        &       0.058                 &       0.019                 \\
            &     (0.001)                 &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.013)                 &     (0.009)                 &     (0.015)                 &     (0.008)                 &     (0.038)                 &     (0.040)                 &     (0.015)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.017$^{\ast\ast}$    &       0.019$^{\ast}$        &      -0.014                 &       0.036$^{\ast\ast}$    &      -0.648$^{\ast\ast}$    &      -0.001                 &      -0.243                 &      -0.405$^{\ast\ast}$    &       0.646$^{\ast\ast\ast}$&      -0.230                 &      -0.492                 \\
            &     (0.007)                 &     (0.009)                 &     (0.030)                 &     (0.015)                 &     (0.237)                 &     (0.098)                 &     (0.155)                 &     (0.139)                 &     (0.198)                 &     (0.340)                 &     (0.358)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.004$^{\ast\ast}$    &       0.000                 &       0.007$^{\ast\ast}$    &       0.003                 &       0.110$^{\ast\ast}$    &       0.010                 &       0.084$^{\ast\ast}$    &       0.016                 &      -0.059                 &       0.142$^{\ast\ast}$    &      -0.081$^{\ast}$        \\
            &     (0.002)                 &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.045)                 &     (0.012)                 &     (0.035)                 &     (0.010)                 &     (0.044)                 &     (0.051)                 &     (0.041)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.002                 &       0.024                 &      -0.002                 &      -0.007                 &       0.030                 &       0.122                 &      -0.003                 &      -0.088$^{\ast}$        &       0.463$^{\ast}$        &      -0.258                 &      -0.207                 \\
            &     (0.006)                 &     (0.013)                 &     (0.019)                 &     (0.011)                 &     (0.248)                 &     (0.082)                 &     (0.190)                 &     (0.048)                 &     (0.247)                 &     (0.350)                 &     (0.240)                 \\\addlinespace
$XRate_{c,t}$&       0.005                 &       0.002                 &       0.014$^{\ast}$        &      -0.000                 &       0.100                 &       0.093                 &       0.027                 &      -0.020                 &       0.137                 &       0.055                 &      -0.188$^{\ast}$        \\
            &     (0.004)                 &     (0.003)                 &     (0.006)                 &     (0.010)                 &     (0.126)                 &     (0.078)                 &     (0.141)                 &     (0.026)                 &     (0.224)                 &     (0.253)                 &     (0.100)                 \\\addlinespace
$ETR_{c,t}$&       0.003$^{\ast}$        &       0.003                 &       0.012$^{\ast\ast}$    &      -0.003                 &       0.136                 &       0.036                 &       0.120$^{\ast}$        &      -0.020                 &      -0.035                 &       0.214$^{\ast\ast}$    &      -0.198$^{\ast\ast}$    \\
            &     (0.002)                 &     (0.002)                 &     (0.005)                 &     (0.002)                 &     (0.076)                 &     (0.023)                 &     (0.055)                 &     (0.019)                 &     (0.045)                 &     (0.094)                 &     (0.082)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .982                 &        .993                 &        .985                 &        .982                 &        .989                 &        .985                 &        .979                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/ETR_Eurostat/Results2shortV1_RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.010                 &       0.017                 &       0.022                 &      -0.059                 &       0.281                 &       0.251                 &       0.253                 &      -0.223                 &       0.461                 &       0.526                 &      -0.976                 \\
            &     (0.022)                 &     (0.024)                 &     (0.051)                 &     (0.033)                 &     (0.618)                 &     (0.459)                 &     (0.432)                 &     (0.236)                 &     (0.915)                 &     (0.812)                 &     (0.655)                 \\\addlinespace
$ICT_{c,t}$&       0.018                 &      -0.007                 &       0.016                 &       0.026                 &       0.305                 &      -0.112                 &       0.157                 &       0.260$^{\ast\ast\ast}$&      -1.280                 &       0.550                 &       0.705                 \\
            &     (0.032)                 &     (0.052)                 &     (0.035)                 &     (0.057)                 &     (0.478)                 &     (0.584)                 &     (0.473)                 &     (0.056)                 &     (1.107)                 &     (0.878)                 &     (0.527)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.014                 &       0.005                 &       0.001                 &      -0.037                 &       0.075                 &      -0.075                 &       0.276                 &      -0.126                 &       0.345                 &      -0.030                 &      -0.369                 \\
            &     (0.022)                 &     (0.034)                 &     (0.037)                 &     (0.033)                 &     (0.623)                 &     (0.363)                 &     (0.628)                 &     (0.093)                 &     (0.605)                 &     (0.772)                 &     (0.450)                 \\\addlinespace
$wL_{c,t}$&       0.405$^{\ast\ast\ast}$&       0.340                 &       0.544$^{\ast}$        &       0.374$^{\ast\ast\ast}$&      -0.650$^{\ast\ast\ast}$&       0.041                 &       0.096                 &      -0.788$^{\ast\ast\ast}$&       0.712$^{\ast}$        &       1.104$^{\ast}$        &      -1.807$^{\ast\ast\ast}$\\
            &     (0.069)                 &     (0.188)                 &     (0.265)                 &     (0.097)                 &     (0.182)                 &     (0.076)                 &     (0.222)                 &     (0.085)                 &     (0.339)                 &     (0.558)                 &     (0.337)                 \\\addlinespace
$rK_{c,t}$&       0.022                 &       0.239$^{\ast}$        &       0.158                 &      -0.243$^{\ast\ast}$    &      -0.704$^{\ast\ast\ast}$&       0.016                 &       0.070                 &      -0.790$^{\ast\ast\ast}$&       0.718$^{\ast\ast}$    &       1.030$^{\ast\ast}$    &      -1.743$^{\ast\ast\ast}$\\
            &     (0.055)                 &     (0.118)                 &     (0.114)                 &     (0.073)                 &     (0.143)                 &     (0.037)                 &     (0.169)                 &     (0.088)                 &     (0.249)                 &     (0.391)                 &     (0.297)                 \\\addlinespace
$pQ_{c,t}$&       0.213$^{\ast}$        &       0.107                 &       0.228                 &       0.245$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.104)                 &     (0.345)                 &     (0.278)                 &     (0.130)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .988                 &        .994                 &         .99                 &        .984                 &        .992                 &        .989                 &        .984                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/ETR_Eurostat/Results2shortV1_RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 2006-2007}}} \\\midrule
$R_{c,t}$ &      -0.130                 &       0.091                 &      -0.212                 &       0.241                 &      -0.653                 &      -0.652                 &      -1.990                 &       1.988                 &      -0.882                 &      -4.258                 &       4.623                 \\
            &     (0.077)                 &     (0.087)                 &     (0.190)                 &     (0.341)                 &     (1.362)                 &     (0.868)                 &     (1.728)                 &     (0.421)                 &     (2.690)                 &     (3.608)                 &     (2.115)                 \\\addlinespace
$ICT_{c,t}$&      -1.777                 &      -1.453                 &      -1.905                 &      -2.026                 &     -32.988                 &     -13.633                 &     -19.156                 &      -0.199                 &     -11.824                 &     -28.743                 &      37.544                 \\
            &     (0.374)                 &     (0.627)                 &     (1.281)                 &     (1.668)                 &    (15.777)                 &     (5.174)                 &    (18.371)                 &     (3.157)                 &    (18.784)                 &    (36.950)                 &    (21.266)                 \\\addlinespace
$R*ICT_{c,t}$&       0.242                 &       0.369                 &      -0.011                 &       0.461                 &       3.152                 &       1.988                 &       0.597                 &       0.567                 &       3.611                 &       0.448                 &      -3.467                 \\
            &     (0.068)                 &     (0.097)                 &     (0.225)                 &     (0.283)                 &     (2.760)                 &     (1.092)                 &     (3.229)                 &     (0.682)                 &     (3.582)                 &     (6.787)                 &     (4.054)                 \\\addlinespace
$wL_{c,t}$&       0.257                 &      -0.548                 &       2.317                 &      -0.332                 &      -0.002                 &       0.011                 &       0.784                 &      -0.797$^{\ast\ast}$    &       0.084                 &       2.344                 &      -2.479$^{\ast}$        \\
            &     (0.159)                 &     (0.410)                 &     (0.976)                 &     (1.187)                 &     (0.187)                 &     (0.117)                 &     (0.210)                 &     (0.055)                 &     (0.339)                 &     (0.507)                 &     (0.338)                 \\\addlinespace
$rK_{c,t}$&       0.058                 &      -0.058                 &       0.291                 &       0.189                 &      -0.048                 &      -0.110                 &       0.823                 &      -0.761$^{\ast\ast}$    &      -0.170                 &       2.341                 &      -2.190                 \\
            &     (0.126)                 &     (0.198)                 &     (0.424)                 &     (0.633)                 &     (0.211)                 &     (0.122)                 &     (0.230)                 &     (0.058)                 &     (0.342)                 &     (0.502)                 &     (0.357)                 \\\addlinespace
$pQ_{c,t}$&       0.683                 &       2.303                 &      -2.801                 &       1.531                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.279)                 &     (0.667)                 &     (1.689)                 &     (2.142)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &        .999                 \\
$N$      &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 \\


==> inputs/robustness/ETR_Eurostat/Results2shortV1_RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 2006-2016}}} \\\midrule
$R_{c,t}$ &      -0.006                 &      -0.013                 &       0.032                 &      -0.036                 &       0.247                 &      -0.159                 &       0.540                 &      -0.135                 &      -0.729                 &       1.527                 &      -0.818                 \\
            &     (0.009)                 &     (0.025)                 &     (0.051)                 &     (0.023)                 &     (0.548)                 &     (0.336)                 &     (0.483)                 &     (0.170)                 &     (1.020)                 &     (1.138)                 &     (0.603)                 \\\addlinespace
$ICT_{c,t}$&      -0.003                 &      -0.020                 &       0.018                 &      -0.022                 &      -0.322                 &       0.146                 &      -0.635                 &       0.168$^{\ast\ast}$    &       0.078                 &      -0.991                 &       0.722                 \\
            &     (0.025)                 &     (0.025)                 &     (0.043)                 &     (0.064)                 &     (0.628)                 &     (0.509)                 &     (0.740)                 &     (0.057)                 &     (1.394)                 &     (1.523)                 &     (0.500)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.003                 &      -0.002                 &       0.001                 &       0.017                 &       0.098                 &      -0.449                 &       0.559                 &      -0.012                 &      -1.016                 &       1.082                 &      -0.060                 \\
            &     (0.014)                 &     (0.009)                 &     (0.034)                 &     (0.039)                 &     (0.487)                 &     (0.300)                 &     (0.604)                 &     (0.067)                 &     (0.964)                 &     (1.140)                 &     (0.416)                 \\\addlinespace
$wL_{c,t}$&       0.386$^{\ast\ast\ast}$&       0.131                 &       0.826$^{\ast\ast}$    &       0.298                 &      -0.546$^{\ast\ast\ast}$&       0.008                 &       0.265                 &      -0.818$^{\ast\ast\ast}$&       0.377                 &       1.595$^{\ast\ast\ast}$&      -1.945$^{\ast\ast\ast}$\\
            &     (0.095)                 &     (0.206)                 &     (0.342)                 &     (0.194)                 &     (0.155)                 &     (0.106)                 &     (0.157)                 &     (0.051)                 &     (0.417)                 &     (0.477)                 &     (0.156)                 \\\addlinespace
$rK_{c,t}$&      -0.006                 &       0.159                 &       0.103                 &      -0.247$^{\ast\ast}$    &      -0.646$^{\ast\ast\ast}$&      -0.010                 &       0.174                 &      -0.810$^{\ast\ast\ast}$&       0.496                 &       1.352$^{\ast\ast\ast}$&      -1.830$^{\ast\ast\ast}$\\
            &     (0.079)                 &     (0.134)                 &     (0.132)                 &     (0.101)                 &     (0.153)                 &     (0.062)                 &     (0.148)                 &     (0.061)                 &     (0.303)                 &     (0.350)                 &     (0.182)                 \\\addlinespace
$pQ_{c,t}$&       0.265                 &       0.528                 &      -0.237                 &       0.401                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.157)                 &     (0.352)                 &     (0.446)                 &     (0.274)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
%$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .982                 &        .993                 &        .985                 &        .982                 &        .989                 &        .985                 &        .979                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/ETR_Eurostat/Results4RICTint_EUKLEMS_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.025                 &       0.020                 &      -0.032                 &      -0.013                 &       0.013$^{\ast\ast}$    &      -1.481$^{\ast\ast}$    &       0.004                 &       0.009$^{\ast}$        \\
            &     (0.026)                 &     (0.015)                 &     (0.024)                 &     (0.031)                 &     (0.004)                 &     (0.538)                 &     (0.005)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&      -0.007                 &      -0.001                 &       0.037                 &       0.097                 &      -0.010$^{\ast}$        &       1.924                 &       0.001                 &       0.006                 \\
            &     (0.036)                 &     (0.032)                 &     (0.032)                 &     (0.064)                 &     (0.005)                 &     (1.328)                 &     (0.007)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.027                 &       0.002                 &      -0.041                 &      -0.040                 &       0.004                 &      -0.475                 &      -0.002                 &       0.007                 \\
            &     (0.025)                 &     (0.015)                 &     (0.025)                 &     (0.038)                 &     (0.003)                 &     (0.806)                 &     (0.003)                 &     (0.006)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .838                 &          0.999                &        .967                 &        .987                 &        .936                 &        .947                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/ETR_Eurostat/Results4RICTint_EUKLEMS_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 2006-2007}}} \\\midrule
$R_{c,t}$ &      -0.644                 &      -0.035                 &      -0.650                 &      -0.025                 &       0.001                 &       5.013                 &       0.031                 &       0.190                 \\
            &     (0.188)                 &     (0.022)                 &     (0.155)                 &     (0.046)                 &     (0.006)                 &     (2.593)                 &     (0.013)                 &     (0.106)                 \\\addlinespace
$ICT_{c,t}$&       0.294                 &      -0.104                 &      -0.417                 &       0.023                 &       0.048                 &     -32.489                 &      -0.103                 &       0.360                 \\
            &     (0.533)                 &     (0.183)                 &     (0.505)                 &     (0.459)                 &     (0.051)                 &    (14.294)                 &     (0.063)                 &     (0.279)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.107                 &      -0.014                 &       0.114                 &      -0.087                 &      -0.016                 &       9.210                 &       0.029                 &      -0.039                 \\
            &     (0.116)                 &     (0.039)                 &     (0.101)                 &     (0.099)                 &     (0.011)                 &     (2.803)                 &     (0.016)                 &     (0.059)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .993                 &          0.999                &          0.999                &        .999                 &        .998                 &        .989                 \\
$N$      &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 \\


==> inputs/robustness/ETR_Eurostat/Results4RICTint_EUKLEMS_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 2006-2016}}} \\\midrule
$R_{c,t}$ &      -0.040                 &       0.022                 &      -0.043                 &      -0.021                 &       0.008$^{\ast}$        &      -1.122$^{\ast\ast}$    &       0.013                 &       0.027                 \\
            &     (0.026)                 &     (0.020)                 &     (0.030)                 &     (0.033)                 &     (0.004)                 &     (0.482)                 &     (0.008)                 &     (0.016)                 \\\addlinespace
$ICT_{c,t}$&       0.003                 &       0.007                 &       0.024                 &       0.109                 &      -0.012$^{\ast}$        &       3.360$^{\ast\ast\ast}$&       0.007                 &       0.034                 \\
            &     (0.036)                 &     (0.038)                 &     (0.049)                 &     (0.079)                 &     (0.006)                 &     (1.054)                 &     (0.011)                 &     (0.023)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.022                 &      -0.006                 &      -0.031                 &      -0.066                 &       0.005                 &      -1.007                 &      -0.002                 &      -0.008                 \\
            &     (0.023)                 &     (0.017)                 &     (0.027)                 &     (0.050)                 &     (0.004)                 &     (0.641)                 &     (0.005)                 &     (0.012)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .809                 &        .999                 &        .956                 &        .984                 &        .876                 &         .78                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/ETR_Eurostat/Results4RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.033                 &       0.019                 &      -0.036                 &      -0.005                 &       0.014$^{\ast\ast}$    &      -1.612$^{\ast\ast}$    &       0.004                 &       0.009$^{\ast}$        \\
            &     (0.027)                 &     (0.019)                 &     (0.023)                 &     (0.023)                 &     (0.004)                 &     (0.550)                 &     (0.005)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.008                 &       0.005                 &       0.038                 &       0.103$^{\ast\ast}$    &      -0.010$^{\ast\ast}$    &       1.990                 &      -0.000                 &       0.006                 \\
            &     (0.020)                 &     (0.037)                 &     (0.038)                 &     (0.044)                 &     (0.004)                 &     (1.181)                 &     (0.006)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.035$^{\ast}$        &      -0.002                 &      -0.044                 &      -0.035                 &       0.005$^{\ast}$        &      -0.535                 &      -0.001                 &       0.008                 \\
            &     (0.015)                 &     (0.023)                 &     (0.026)                 &     (0.032)                 &     (0.003)                 &     (0.704)                 &     (0.003)                 &     (0.005)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .846                 &          0.999                &        .971                 &        .988                 &        .936                 &        .948                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/ETR_Eurostat/Results4RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 2006-2007}}} \\\midrule
$R_{c,t}$ &      -0.600                 &      -0.036                 &      -0.619                 &      -0.018                 &      -0.000                 &       5.246                 &       0.033                 &       0.169                 \\
            &     (0.196)                 &     (0.031)                 &     (0.148)                 &     (0.049)                 &     (0.004)                 &     (2.788)                 &     (0.013)                 &     (0.100)                 \\\addlinespace
$ICT_{c,t}$&       0.004                 &      -0.584                 &      -1.016                 &      -0.348                 &       0.126                 &     -47.101                 &      -0.174                 &       0.763                 \\
            &     (0.906)                 &     (0.262)                 &     (0.697)                 &     (0.465)                 &     (0.035)                 &    (20.932)                 &     (0.091)                 &     (0.395)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.124                 &       0.090                 &       0.192                 &      -0.036                 &      -0.028                 &      10.816                 &       0.038                 &      -0.084                 \\
            &     (0.154)                 &     (0.055)                 &     (0.125)                 &     (0.087)                 &     (0.007)                 &     (3.456)                 &     (0.018)                 &     (0.071)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .993                 &          0.999                &          0.999                &        .999                 &        .998                 &         .99                 \\
$N$      &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 \\


==> inputs/robustness/ETR_Eurostat/Results4RICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 2006-2016}}} \\\midrule
$R_{c,t}$ &      -0.046                 &       0.016                 &      -0.051                 &      -0.006                 &       0.010$^{\ast\ast}$    &      -1.255$^{\ast\ast}$    &       0.014                 &       0.028                 \\
            &     (0.027)                 &     (0.022)                 &     (0.028)                 &     (0.025)                 &     (0.004)                 &     (0.475)                 &     (0.008)                 &     (0.016)                 \\\addlinespace
$ICT_{c,t}$&       0.026                 &       0.015                 &       0.024                 &       0.130$^{\ast}$        &      -0.013$^{\ast\ast}$    &       3.418$^{\ast\ast}$    &       0.005                 &       0.031                 \\
            &     (0.032)                 &     (0.042)                 &     (0.050)                 &     (0.064)                 &     (0.005)                 &     (1.121)                 &     (0.011)                 &     (0.022)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.041$^{\ast\ast}$    &      -0.007                 &      -0.035                 &      -0.065                 &       0.006$^{\ast}$        &      -1.013                 &      -0.000                 &      -0.005                 \\
            &     (0.017)                 &     (0.022)                 &     (0.027)                 &     (0.041)                 &     (0.003)                 &     (0.574)                 &     (0.005)                 &     (0.010)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &        .825                 &          0.999                &        .961                 &        .984                 &        .876                 &         .78                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/ETR_Eurostat/Results4shortRICTint_ct_All_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.033                 &       0.019                 &      -0.036                 &      -0.005                 &      -1.612$^{\ast\ast}$    &       0.009$^{\ast}$        \\
            &     (0.027)                 &     (0.019)                 &     (0.023)                 &     (0.023)                 &     (0.550)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.008                 &       0.005                 &       0.038                 &       0.103$^{\ast\ast}$    &       1.990                 &       0.006                 \\
            &     (0.020)                 &     (0.037)                 &     (0.038)                 &     (0.044)                 &     (1.181)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.035$^{\ast}$        &      -0.002                 &      -0.044                 &      -0.035                 &      -0.535                 &       0.008                 \\
            &     (0.015)                 &     (0.023)                 &     (0.026)                 &     (0.032)                 &     (0.704)                 &     (0.005)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .846                 &          0.999                &        .988                 &        .948                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/ETR_Eurostat/Results4shortRICTint_ct_All_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 2006-2007}}} \\\midrule
$R_{c,t}$ &      -0.600                 &      -0.036                 &      -0.619                 &      -0.018                 &       5.246                 &       0.169                 \\
            &     (0.196)                 &     (0.031)                 &     (0.148)                 &     (0.049)                 &     (2.788)                 &     (0.100)                 \\\addlinespace
$ICT_{c,t}$&       0.004                 &      -0.584                 &      -1.016                 &      -0.348                 &     -47.101                 &       0.763                 \\
            &     (0.906)                 &     (0.262)                 &     (0.697)                 &     (0.465)                 &    (20.932)                 &     (0.395)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.124                 &       0.090                 &       0.192                 &      -0.036                 &      10.816                 &      -0.084                 \\
            &     (0.154)                 &     (0.055)                 &     (0.125)                 &     (0.087)                 &     (3.456)                 &     (0.071)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .993                 &          0.999                &        .999                 &         .99                 \\
$N$      &          38                 &          38                 &          38                 &          38                 &          38                 &          38                 \\


==> inputs/robustness/ETR_Eurostat/Results4shortRICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $Services_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 2006-2016}}} \\\midrule
$R_{c,t}$ &      -0.046                 &       0.016                 &      -0.051                 &      -0.006                 &      -1.255$^{\ast\ast}$    &       0.028                 \\
            &     (0.027)                 &     (0.022)                 &     (0.028)                 &     (0.025)                 &     (0.475)                 &     (0.016)                 \\\addlinespace
$ICT_{c,t}$&       0.026                 &       0.015                 &       0.024                 &       0.130$^{\ast}$        &       3.418$^{\ast\ast}$    &       0.031                 \\
            &     (0.032)                 &     (0.042)                 &     (0.050)                 &     (0.064)                 &     (1.121)                 &     (0.022)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.041$^{\ast\ast}$    &      -0.007                 &      -0.035                 &      -0.065                 &      -1.013                 &      -0.005                 \\
            &     (0.017)                 &     (0.022)                 &     (0.027)                 &     (0.041)                 &     (0.574)                 &     (0.010)                 \\\midrule
%$R^{2}$  &        .999                 &        .999                 &        .825                 &          0.999                &        .984                 &         .78                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/ETR_Eurostat/Results5RICTint_EUKLEMS_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.005                 &      -0.036                 &      -0.023                 &      -0.004                 &       0.071$^{\ast\ast\ast}$&      -0.034$^{\ast\ast}$    &       0.030                 &      -0.003                 \\
            &     (0.032)                 &     (0.040)                 &     (0.023)                 &     (0.025)                 &     (0.019)                 &     (0.012)                 &     (0.022)                 &     (0.010)                 \\\addlinespace
$ICT_{c,t}$&       0.031                 &       0.139$^{\ast}$        &       0.077$^{\ast}$        &       0.057                 &       0.038                 &       0.024                 &       0.020                 &       0.008                 \\
            &     (0.039)                 &     (0.066)                 &     (0.040)                 &     (0.058)                 &     (0.025)                 &     (0.023)                 &     (0.018)                 &     (0.008)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.024                 &      -0.071                 &      -0.048                 &      -0.044                 &      -0.006                 &      -0.028                 &      -0.012                 &       0.004                 \\
            &     (0.028)                 &     (0.043)                 &     (0.029)                 &     (0.034)                 &     (0.015)                 &     (0.015)                 &     (0.013)                 &     (0.008)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &          0.999                &          0.999                &          0.999                &        .886                 &          0.999                &        .991                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         135                 &         135                 &         135                 &         135                 \\


==> inputs/robustness/ETR_Eurostat/Results5RICTint_EUKLEMS_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 2006-2007}}} \\\midrule
$R_{c,t}$ &      -0.805                 &      -0.680                 &      -0.748                 &      -0.498                 &      -0.289                 &      -0.504                 &      -0.281                 &      -0.109                 \\
            &     (0.275)                 &     (0.170)                 &     (0.214)                 &     (0.176)                 &     (0.140)                 &     (0.184)                 &     (0.150)                 &     (0.033)                 \\\addlinespace
$ICT_{c,t}$&       0.668                 &      -0.797                 &       0.004                 &       0.015                 &       0.749                 &       0.137                 &       0.026                 &       0.177                 \\
            &     (0.856)                 &     (0.948)                 &     (0.832)                 &     (0.698)                 &     (0.349)                 &     (0.490)                 &     (0.297)                 &     (0.131)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.161                 &      -0.031                 &      -0.077                 &      -0.061                 &      -0.173                 &      -0.075                 &       0.020                 &      -0.049                 \\
            &     (0.154)                 &     (0.167)                 &     (0.144)                 &     (0.129)                 &     (0.085)                 &     (0.113)                 &     (0.058)                 &     (0.034)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &        .975                 &          0.999                &          0.999                \\
$N$      &          38                 &          38                 &          38                 &          38                 &          30                 &          30                 &          30                 &          30                 \\


==> inputs/robustness/ETR_Eurostat/Results5RICTint_EUKLEMS_ct_All_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 2006-2016}}} \\\midrule
$R_{c,t}$ &      -0.011                 &      -0.063$^{\ast}$        &      -0.038$^{\ast}$        &      -0.024                 &       0.077$^{\ast\ast\ast}$&      -0.051$^{\ast\ast\ast}$&       0.035                 &      -0.005                 \\
            &     (0.022)                 &     (0.029)                 &     (0.021)                 &     (0.024)                 &     (0.018)                 &     (0.015)                 &     (0.024)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t}$&       0.046                 &       0.102                 &       0.070                 &       0.048                 &       0.041                 &       0.015                 &       0.016                 &       0.009                 \\
            &     (0.052)                 &     (0.059)                 &     (0.046)                 &     (0.064)                 &     (0.035)                 &     (0.021)                 &     (0.023)                 &     (0.005)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.046                 &      -0.057                 &      -0.056$^{\ast}$        &      -0.053                 &      -0.027                 &      -0.023$^{\ast}$        &      -0.018                 &      -0.004                 \\
            &     (0.029)                 &     (0.037)                 &     (0.029)                 &     (0.035)                 &     (0.024)                 &     (0.012)                 &     (0.018)                 &     (0.006)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &        .999                 &        .999                 &          0.999                &        .896                 &          0.999                &         .99                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         165                 &         165                 &         165                 &         165                 \\


==> inputs/robustness/ETR_Eurostat/Results5RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.008                 &      -0.035                 &      -0.024                 &      -0.006                 &       0.069$^{\ast\ast\ast}$&      -0.034$^{\ast\ast}$    &       0.030                 &      -0.003                 \\
            &     (0.031)                 &     (0.040)                 &     (0.023)                 &     (0.025)                 &     (0.020)                 &     (0.012)                 &     (0.022)                 &     (0.010)                 \\\addlinespace
$ICT_{c,t}$&       0.046                 &       0.127$^{\ast}$        &       0.082$^{\ast}$        &       0.069                 &       0.050$^{\ast\ast}$    &       0.025                 &       0.021                 &       0.022$^{\ast\ast\ast}$\\
            &     (0.035)                 &     (0.062)                 &     (0.038)                 &     (0.054)                 &     (0.019)                 &     (0.023)                 &     (0.017)                 &     (0.003)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.031                 &      -0.063                 &      -0.050                 &      -0.050                 &      -0.012                 &      -0.028                 &      -0.012                 &      -0.001                 \\
            &     (0.032)                 &     (0.039)                 &     (0.030)                 &     (0.036)                 &     (0.020)                 &     (0.015)                 &     (0.013)                 &     (0.010)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &          0.999                &          0.999                &          0.999                &        .886                 &          0.999                &        .979                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         135                 &         135                 &         135                 &         135                 \\


==> inputs/robustness/ETR_Eurostat/Results5RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 2006-2007}}} \\\midrule
$R_{c,t}$ &      -0.787                 &      -0.629                 &      -0.717                 &      -0.475                 &      -0.295                 &      -0.507                 &      -0.282                 &      -0.115                 \\
            &     (0.290)                 &     (0.168)                 &     (0.219)                 &     (0.181)                 &     (0.156)                 &     (0.181)                 &     (0.150)                 &     (0.043)                 \\\addlinespace
$ICT_{c,t}$&      -0.026                 &      -2.421                 &      -1.044                 &      -0.775                 &       1.087                 &      -0.910                 &      -0.263                 &       0.882                 \\
            &     (1.376)                 &     (1.015)                 &     (1.129)                 &     (0.901)                 &     (0.745)                 &     (0.775)                 &     (0.588)                 &     (0.371)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.042                 &       0.190                 &       0.078                 &       0.054                 &      -0.219                 &       0.120                 &       0.073                 &      -0.179                 \\
            &     (0.213)                 &     (0.145)                 &     (0.165)                 &     (0.135)                 &     (0.138)                 &     (0.134)                 &     (0.097)                 &     (0.074)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &        .977                 &          0.999                &        .999                 \\
$N$      &          38                 &          38                 &          38                 &          38                 &          30                 &          30                 &          30                 &          30                 \\


==> inputs/robustness/ETR_Eurostat/Results5RICTint_ct_All_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 2006-2016}}} \\\midrule
$R_{c,t}$ &      -0.013                 &      -0.062$^{\ast}$        &      -0.039$^{\ast}$        &      -0.026                 &       0.074$^{\ast\ast\ast}$&      -0.051$^{\ast\ast\ast}$&       0.035                 &       0.001                 \\
            &     (0.022)                 &     (0.029)                 &     (0.021)                 &     (0.025)                 &     (0.019)                 &     (0.015)                 &     (0.024)                 &     (0.007)                 \\\addlinespace
$ICT_{c,t}$&       0.069                 &       0.102$^{\ast}$        &       0.084$^{\ast}$        &       0.069                 &       0.063$^{\ast}$        &       0.015                 &       0.020                 &       0.026$^{\ast\ast\ast}$\\
            &     (0.048)                 &     (0.055)                 &     (0.044)                 &     (0.061)                 &     (0.032)                 &     (0.022)                 &     (0.024)                 &     (0.002)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.056$^{\ast}$        &      -0.054                 &      -0.061$^{\ast}$        &      -0.061                 &      -0.038                 &      -0.022                 &      -0.019                 &      -0.006                 \\
            &     (0.030)                 &     (0.033)                 &     (0.028)                 &     (0.036)                 &     (0.026)                 &     (0.013)                 &     (0.018)                 &     (0.006)                 \\\midrule
%$R^{2}$  &        .999                 &        .999                 &        .999                 &        .999                 &          0.999                &        .896                 &          0.999                &        .976                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         165                 &         165                 &         165                 &         165                 \\


==> inputs/robustness/IV/Results1RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.007                 &       0.015                 &       0.030                 &      -0.019                 &       0.615                 &       0.346                 &       0.260                 &       0.009                 &       0.365                 &       0.348                 &      -0.689                 \\
            &     (0.015)                 &     (0.024)                 &     (0.052)                 &     (0.019)                 &     (0.612)                 &     (0.284)                 &     (0.429)                 &     (0.266)                 &     (0.824)                 &     (1.051)                 &     (0.670)                 \\\addlinespace
$ICT_{c,t}$&      -0.039                 &      -0.030                 &      -0.036                 &      -0.067                 &      -1.914$^{\ast}$        &      -0.578                 &      -0.022                 &      -1.313$^{\ast\ast}$    &      -0.522                 &       2.098                 &      -1.694                 \\
            &     (0.027)                 &     (0.050)                 &     (0.060)                 &     (0.050)                 &     (1.059)                 &     (0.518)                 &     (0.729)                 &     (0.548)                 &     (1.221)                 &     (1.406)                 &     (1.265)                 \\\addlinespace
$R*ICT_{c,t}$&       0.005                 &       0.018                 &       0.010                 &      -0.004                 &       0.599                 &       0.082                 &       0.230                 &       0.286                 &       0.407                 &      -0.632                 &       0.208                 \\
            &     (0.016)                 &     (0.030)                 &     (0.035)                 &     (0.030)                 &     (0.715)                 &     (0.295)                 &     (0.526)                 &     (0.326)                 &     (0.742)                 &     (0.812)                 &     (0.735)                 \\\midrule
Under-F     &        75.5                 &        75.5                 &        75.5                 &        75.5                 &        79.9                 &        79.9                 &        79.9                 &        79.9                 &        79.9                 &        79.9                 &        79.9                 \\
Under-p     &        .908                 &        .908                 &        .908                 &        .908                 &        .831                 &        .831                 &        .831                 &        .831                 &        .831                 &        .831                 &        .831                 \\
Weak-CD F   &        1.13                 &        1.13                 &        1.13                 &        1.13                 &        1.16                 &        1.16                 &        1.16                 &        1.16                 &        1.16                 &        1.16                 &        1.16                 \\
Weak-KP rk F&        8.91                 &        8.91                 &        8.91                 &        8.91                 &        8.39                 &        8.39                 &        8.39                 &        8.39                 &        8.39                 &        8.39                 &        8.39                 \\
Over-Hansen J&        95.8                 &         102                 &         103                 &        94.8                 &        97.4                 &         104                 &         109                 &         100                 &        89.1                 &         106                 &         109                 \\
Over-Hansen J p&        .373                 &        .218                 &        .196                 &        .401                 &         .33                 &        .191                 &        .113                 &        .262                 &        .567                 &        .148                 &        .111                 \\
$R^{2}$  &        .806                 &        .724                 &        .412                 &        .536                 &        .449                 &        .293                 &        .189                 &          .5                 &        .231                 &        .117                 &         .28                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/IV/Results1RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.054$^{\ast\ast\ast}$&      -0.149$^{\ast\ast\ast}$&      -0.100$^{\ast\ast\ast}$&      -0.007                 &      -0.504                 &      -0.203                 &      -0.580$^{\ast\ast}$    &       0.279$^{\ast}$        &      -0.177                 &      -1.472$^{\ast\ast\ast}$&       0.967$^{\ast\ast}$    \\
            &     (0.015)                 &     (0.050)                 &     (0.027)                 &     (0.017)                 &     (0.412)                 &     (0.186)                 &     (0.291)                 &     (0.159)                 &     (0.499)                 &     (0.537)                 &     (0.389)                 \\\addlinespace
$ICT_{c,t}$&      -0.006                 &      -0.154                 &      -0.072                 &       0.003                 &       1.036                 &       0.938$^{\ast\ast\ast}$&      -0.520                 &       0.618$^{\ast\ast}$    &       1.562$^{\ast\ast}$    &      -2.280$^{\ast\ast}$    &       0.508                 \\
            &     (0.025)                 &     (0.103)                 &     (0.046)                 &     (0.027)                 &     (0.827)                 &     (0.315)                 &     (0.623)                 &     (0.271)                 &     (0.791)                 &     (1.054)                 &     (0.570)                 \\\addlinespace
$R*ICT_{c,t}$&       0.001                 &       0.055                 &       0.008                 &       0.001                 &      -0.777                 &      -0.204                 &      -0.244                 &      -0.330$^{\ast\ast}$    &       0.193                 &       0.247                 &      -0.173                 \\
            &     (0.015)                 &     (0.040)                 &     (0.024)                 &     (0.016)                 &     (0.477)                 &     (0.199)                 &     (0.342)                 &     (0.150)                 &     (0.409)                 &     (0.553)                 &     (0.360)                 \\\midrule
Under-F     &         111                 &         111                 &         111                 &         111                 &         118                 &         118                 &         118                 &         118                 &         118                 &         118                 &         118                 \\
Under-p     &       .0968                 &       .0968                 &       .0968                 &       .0968                 &       .0392                 &       .0392                 &       .0392                 &       .0392                 &       .0392                 &       .0392                 &       .0392                 \\
Weak-CD F   &        4.44                 &        4.44                 &        4.44                 &        4.44                 &        4.09                 &        4.09                 &        4.09                 &        4.09                 &        4.09                 &        4.09                 &        4.09                 \\
Weak-KP rk F&        9.03                 &        9.03                 &        9.03                 &        9.03                 &        8.46                 &        8.46                 &        8.46                 &        8.46                 &        8.46                 &        8.46                 &        8.46                 \\
Over-Hansen J&         110                 &          95                 &         105                 &         112                 &         127                 &         108                 &         111                 &         112                 &         119                 &         101                 &         124                 \\
Over-Hansen J p&       .0998                 &        .394                 &        .164                 &       .0749                 &      .00938                 &        .117                 &       .0838                 &        .078                 &       .0298                 &        .248                 &       .0142                 \\
$R^{2}$  &        .928                 &        .574                 &        .836                 &        .898                 &        .245                 &        .261                 &        .243                 &        .213                 &        .336                 &         .28                 &          .2                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/IV/Results1RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.025$^{\ast\ast\ast}$&      -0.055$^{\ast\ast\ast}$&       0.030                 &      -0.024$^{\ast\ast}$    &       0.265                 &      -0.335$^{\ast\ast\ast}$&       0.603$^{\ast\ast\ast}$&      -0.003                 &      -1.284$^{\ast\ast\ast}$&       1.422$^{\ast\ast\ast}$&      -0.324                 \\
            &     (0.008)                 &     (0.013)                 &     (0.022)                 &     (0.012)                 &     (0.263)                 &     (0.126)                 &     (0.212)                 &     (0.122)                 &     (0.351)                 &     (0.467)                 &     (0.358)                 \\\addlinespace
$ICT_{c,t}$&      -0.071$^{\ast\ast}$    &      -0.156$^{\ast}$        &      -0.106$^{\ast\ast}$    &      -0.057                 &      -1.459$^{\ast}$        &      -0.076                 &      -1.258$^{\ast\ast}$    &      -0.125                 &       1.177                 &      -1.592                 &       0.607                 \\
            &     (0.030)                 &     (0.094)                 &     (0.050)                 &     (0.037)                 &     (0.883)                 &     (0.411)                 &     (0.570)                 &     (0.346)                 &     (0.949)                 &     (1.209)                 &     (0.769)                 \\\addlinespace
$R*ICT_{c,t}$&       0.028$^{\ast\ast}$    &       0.052                 &       0.039                 &       0.044$^{\ast\ast\ast}$&       0.284                 &      -0.166                 &       0.236                 &       0.213                 &      -0.863$^{\ast}$        &       0.449                 &       0.304                 \\
            &     (0.014)                 &     (0.037)                 &     (0.024)                 &     (0.017)                 &     (0.414)                 &     (0.196)                 &     (0.266)                 &     (0.162)                 &     (0.440)                 &     (0.563)                 &     (0.390)                 \\\midrule
Under-F     &         131                 &         131                 &         131                 &         131                 &         139                 &         139                 &         139                 &         139                 &         139                 &         139                 &         139                 \\
Under-p     &      .00604                 &      .00604                 &      .00604                 &      .00604                 &      .00148                 &      .00148                 &      .00148                 &      .00148                 &      .00148                 &      .00148                 &      .00148                 \\
Weak-CD F   &        3.23                 &        3.23                 &        3.23                 &        3.23                 &        3.24                 &        3.24                 &        3.24                 &        3.24                 &        3.24                 &        3.24                 &        3.24                 \\
Weak-KP rk F&        2.15                 &        2.15                 &        2.15                 &        2.15                 &        2.23                 &        2.23                 &        2.23                 &        2.23                 &        2.23                 &        2.23                 &        2.23                 \\
Over-Hansen J&         165                 &         113                 &         164                 &         159                 &         168                 &         150                 &         163                 &         162                 &         166                 &         151                 &         175                 \\
Over-Hansen J p&    5.09e-06                 &       .0658                 &    5.78e-06                 &    .0000199                 &    2.18e-06                 &     .000124                 &    6.94e-06                 &    8.32e-06                 &    3.68e-06                 &     .000094                 &    3.74e-07                 \\
$R^{2}$  &        .915                 &        .696                 &         .66                 &        .846                 &        .373                 &        .189                 &        .233                 &        .435                 &        .342                 &        .114                 &        .172                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/IV/Results2RICTint_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.010                 &       0.019                 &       0.018                 &      -0.057$^{\ast\ast\ast}$&       0.234                 &       0.273                 &       0.190                 &      -0.229                 &       0.598                 &       0.414                 &      -0.996$^{\ast}$        \\
            &     (0.015)                 &     (0.024)                 &     (0.049)                 &     (0.021)                 &     (0.509)                 &     (0.280)                 &     (0.419)                 &     (0.153)                 &     (0.765)                 &     (0.890)                 &     (0.556)                 \\\addlinespace
$ICT_{c,t}$&      -0.001                 &      -0.028                 &      -0.012                 &       0.010                 &      -0.130                 &      -0.386                 &      -0.016                 &       0.272                 &      -1.828$^{\ast}$        &       0.414                 &       1.297                 \\
            &     (0.029)                 &     (0.051)                 &     (0.063)                 &     (0.045)                 &     (0.969)                 &     (0.478)                 &     (0.791)                 &     (0.214)                 &     (1.044)                 &     (1.199)                 &     (0.911)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.011                 &       0.013                 &      -0.002                 &      -0.030                 &       0.070                 &      -0.010                 &       0.193                 &      -0.113                 &       0.705                 &      -0.297                 &      -0.432                 \\
            &     (0.018)                 &     (0.032)                 &     (0.036)                 &     (0.029)                 &     (0.617)                 &     (0.278)                 &     (0.553)                 &     (0.124)                 &     (0.650)                 &     (0.769)                 &     (0.553)                 \\\addlinespace
$wL_{c,t}$&       0.396$^{\ast\ast\ast}$&       0.331$^{\ast}$        &       0.529$^{\ast\ast\ast}$&       0.369$^{\ast\ast\ast}$&      -0.652$^{\ast\ast\ast}$&       0.045                 &       0.091                 &      -0.788$^{\ast\ast\ast}$&       0.723$^{\ast\ast}$    &       1.099$^{\ast\ast\ast}$&      -1.806$^{\ast\ast\ast}$\\
            &     (0.070)                 &     (0.174)                 &     (0.178)                 &     (0.141)                 &     (0.180)                 &     (0.101)                 &     (0.137)                 &     (0.091)                 &     (0.326)                 &     (0.368)                 &     (0.241)                 \\\addlinespace
$rK_{c,t}$&       0.022                 &       0.238$^{\ast}$        &       0.153                 &      -0.236$^{\ast\ast\ast}$&      -0.707$^{\ast\ast\ast}$&       0.022                 &       0.061                 &      -0.790$^{\ast\ast\ast}$&       0.735$^{\ast\ast\ast}$&       1.021$^{\ast\ast\ast}$&      -1.744$^{\ast\ast\ast}$\\
            &     (0.049)                 &     (0.134)                 &     (0.141)                 &     (0.079)                 &     (0.146)                 &     (0.082)                 &     (0.106)                 &     (0.081)                 &     (0.266)                 &     (0.271)                 &     (0.219)                 \\\addlinespace
$pQ_{c,t}$&       0.213$^{\ast}$        &       0.112                 &       0.216                 &       0.254                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.120)                 &     (0.298)                 &     (0.310)                 &     (0.183)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.000                 &      -0.003                 &       0.000                 &       0.004$^{\ast\ast\ast}$&      -0.084$^{\ast\ast}$    &      -0.048$^{\ast\ast}$    &      -0.024                 &      -0.012                 &      -0.075                 &       0.041                 &       0.030                 \\
            &     (0.001)                 &     (0.002)                 &     (0.003)                 &     (0.002)                 &     (0.036)                 &     (0.023)                 &     (0.030)                 &     (0.011)                 &     (0.073)                 &     (0.078)                 &     (0.043)                 \\\addlinespace
$Services_{c,t}$&      -0.000                 &       0.020$^{\ast\ast\ast}$&       0.009                 &      -0.020$^{\ast\ast\ast}$&       0.222                 &       0.130$^{\ast}$        &       0.113                 &      -0.021                 &       0.206                 &       0.040                 &      -0.258$^{\ast}$        \\
            &     (0.003)                 &     (0.006)                 &     (0.011)                 &     (0.006)                 &     (0.137)                 &     (0.066)                 &     (0.114)                 &     (0.047)                 &     (0.210)                 &     (0.261)                 &     (0.154)                 \\\addlinespace
$HHI_{c,t}$&      -0.873                 &       1.469                 &      -0.408                 &      -3.697$^{\ast\ast\ast}$&      16.366                 &      13.639                 &      -2.420                 &       5.147                 &      14.525                 &     -22.570                 &       5.055                 \\
            &     (0.574)                 &     (1.018)                 &     (2.263)                 &     (0.952)                 &    (21.226)                 &    (11.903)                 &    (19.741)                 &     (7.032)                 &    (40.771)                 &    (49.668)                 &    (26.006)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast\ast}$    &       0.001                 &      -0.001                 &       0.045$^{\ast\ast\ast}$&      -0.003                 &       0.022$^{\ast\ast}$    &       0.026$^{\ast\ast\ast}$&      -0.041$^{\ast\ast}$    &       0.023                 &       0.022$^{\ast}$        \\
            &     (0.000)                 &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.011)                 &     (0.005)                 &     (0.009)                 &     (0.004)                 &     (0.019)                 &     (0.022)                 &     (0.011)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.012$^{\ast\ast}$    &       0.020$^{\ast}$        &      -0.036                 &       0.041$^{\ast\ast\ast}$&      -0.782$^{\ast\ast\ast}$&      -0.045                 &      -0.401$^{\ast\ast\ast}$&      -0.335$^{\ast\ast\ast}$&       0.656$^{\ast\ast\ast}$&      -0.557$^{\ast\ast}$    &      -0.147                 \\
            &     (0.006)                 &     (0.010)                 &     (0.022)                 &     (0.008)                 &     (0.191)                 &     (0.075)                 &     (0.132)                 &     (0.071)                 &     (0.205)                 &     (0.272)                 &     (0.197)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003$^{\ast\ast\ast}$&       0.001                 &       0.008$^{\ast\ast\ast}$&       0.001                 &       0.093$^{\ast\ast}$    &       0.012                 &       0.074$^{\ast\ast\ast}$&       0.007                 &      -0.048$^{\ast}$        &       0.130$^{\ast\ast\ast}$&      -0.090$^{\ast\ast\ast}$\\
            &     (0.001)                 &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.040)                 &     (0.010)                 &     (0.026)                 &     (0.015)                 &     (0.029)                 &     (0.038)                 &     (0.028)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.005                 &       0.023$^{\ast\ast\ast}$&      -0.002                 &      -0.004                 &       0.144                 &       0.115                 &       0.092                 &      -0.063                 &       0.373$^{\ast\ast\ast}$&      -0.070                 &      -0.289                 \\
            &     (0.005)                 &     (0.008)                 &     (0.017)                 &     (0.006)                 &     (0.198)                 &     (0.072)                 &     (0.135)                 &     (0.041)                 &     (0.139)                 &     (0.255)                 &     (0.185)                 \\\addlinespace
$XRate_{c,t}$&       0.007                 &      -0.007                 &       0.012                 &       0.020$^{\ast\ast\ast}$&      -0.013                 &      -0.060                 &       0.033                 &       0.014                 &      -0.311                 &       0.305                 &       0.010                 \\
            &     (0.006)                 &     (0.010)                 &     (0.010)                 &     (0.007)                 &     (0.200)                 &     (0.089)                 &     (0.182)                 &     (0.046)                 &     (0.217)                 &     (0.262)                 &     (0.176)                 \\\midrule
Under-F     &        73.1                 &        73.1                 &        73.1                 &        73.1                 &        81.7                 &        81.7                 &        81.7                 &        81.7                 &        81.7                 &        81.7                 &        81.7                 \\
Under-p     &        .937                 &        .937                 &        .937                 &        .937                 &        .793                 &        .793                 &        .793                 &        .793                 &        .793                 &        .793                 &        .793                 \\
Weak-CD F   &        1.26                 &        1.26                 &        1.26                 &        1.26                 &        1.32                 &        1.32                 &        1.32                 &        1.32                 &        1.32                 &        1.32                 &        1.32                 \\
Weak-KP rk F&        17.6                 &        17.6                 &        17.6                 &        17.6                 &        20.3                 &        20.3                 &        20.3                 &        20.3                 &        20.3                 &        20.3                 &        20.3                 \\
Over-Hansen J&        96.5                 &         105                 &        99.8                 &         100                 &         104                 &         105                 &         107                 &          97                 &          90                 &        96.3                 &        93.5                 \\
Over-Hansen J p&        .354                 &        .165                 &         .27                 &        .268                 &        .187                 &        .168                 &        .138                 &        .341                 &        .539                 &        .358                 &        .437                 \\
$R^{2}$  &        .847                 &        .744                 &        .435                 &        .645                 &        .542                 &          .3                 &        .192                 &        .847                 &        .298                 &        .204                 &        .622                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/IV/Results2RICTint_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.030$^{\ast}$        &      -0.084$^{\ast\ast}$    &      -0.086$^{\ast\ast\ast}$&       0.025                 &      -0.391                 &      -0.173                 &      -0.527$^{\ast}$        &       0.310$^{\ast\ast\ast}$&      -0.165                 &      -1.435$^{\ast\ast}$    &       0.982$^{\ast\ast\ast}$\\
            &     (0.016)                 &     (0.038)                 &     (0.029)                 &     (0.019)                 &     (0.331)                 &     (0.159)                 &     (0.295)                 &     (0.102)                 &     (0.470)                 &     (0.565)                 &     (0.335)                 \\\addlinespace
$ICT_{c,t}$&      -0.032                 &      -0.161$^{\ast}$        &      -0.107$^{\ast\ast}$    &       0.011                 &      -0.745                 &       0.304                 &      -1.216$^{\ast}$        &       0.167                 &       0.945                 &      -2.475$^{\ast\ast}$    &       0.896                 \\
            &     (0.025)                 &     (0.085)                 &     (0.051)                 &     (0.027)                 &     (0.780)                 &     (0.370)                 &     (0.673)                 &     (0.171)                 &     (0.909)                 &     (1.179)                 &     (0.664)                 \\\addlinespace
$R*ICT_{c,t}$&       0.001                 &       0.034                 &       0.013                 &      -0.012                 &       0.021                 &       0.049                 &      -0.059                 &       0.031                 &       0.311                 &       0.046                 &       0.103                 \\
            &     (0.013)                 &     (0.030)                 &     (0.025)                 &     (0.014)                 &     (0.442)                 &     (0.198)                 &     (0.351)                 &     (0.092)                 &     (0.423)                 &     (0.581)                 &     (0.359)                 \\\addlinespace
$wL_{c,t}$&       0.575$^{\ast\ast\ast}$&       1.370$^{\ast\ast\ast}$&       0.408$^{\ast\ast}$    &       0.618$^{\ast\ast\ast}$&      -0.594$^{\ast\ast\ast}$&      -0.132                 &       0.052                 &      -0.514$^{\ast\ast\ast}$&       0.180                 &       0.574$^{\ast\ast\ast}$&      -0.934$^{\ast\ast\ast}$\\
            &     (0.146)                 &     (0.453)                 &     (0.195)                 &     (0.148)                 &     (0.148)                 &     (0.091)                 &     (0.108)                 &     (0.059)                 &     (0.186)                 &     (0.220)                 &     (0.181)                 \\\addlinespace
$rK_{c,t}$&      -0.010                 &       0.284                 &      -0.093                 &       0.190$^{\ast\ast}$    &      -0.894$^{\ast\ast\ast}$&      -0.251$^{\ast\ast\ast}$&      -0.094                 &      -0.548$^{\ast\ast\ast}$&       0.030                 &       0.465$^{\ast\ast}$    &      -0.746$^{\ast\ast\ast}$\\
            &     (0.082)                 &     (0.258)                 &     (0.129)                 &     (0.090)                 &     (0.146)                 &     (0.088)                 &     (0.101)                 &     (0.055)                 &     (0.176)                 &     (0.203)                 &     (0.175)                 \\\addlinespace
$pQ_{c,t}$&       0.436$^{\ast\ast}$    &      -0.662                 &       0.646$^{\ast\ast}$    &       0.239                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.201)                 &     (0.652)                 &     (0.284)                 &     (0.211)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.007$^{\ast\ast}$    &      -0.001                 &       0.004$^{\ast\ast}$    &       0.009                 &      -0.062$^{\ast\ast}$    &       0.016                 &       0.055$^{\ast\ast\ast}$&      -0.158$^{\ast\ast}$    &      -0.033                 &       0.172$^{\ast\ast\ast}$\\
            &     (0.002)                 &     (0.004)                 &     (0.003)                 &     (0.002)                 &     (0.039)                 &     (0.025)                 &     (0.030)                 &     (0.017)                 &     (0.061)                 &     (0.059)                 &     (0.057)                 \\\addlinespace
$Services_{c,t}$&       0.001                 &      -0.025                 &      -0.014$^{\ast}$        &      -0.001                 &      -0.060                 &       0.151$^{\ast\ast}$    &      -0.204$^{\ast\ast\ast}$&      -0.007                 &       0.570$^{\ast\ast\ast}$&      -0.545$^{\ast\ast\ast}$&      -0.045                 \\
            &     (0.004)                 &     (0.021)                 &     (0.007)                 &     (0.005)                 &     (0.101)                 &     (0.064)                 &     (0.076)                 &     (0.032)                 &     (0.130)                 &     (0.156)                 &     (0.110)                 \\\addlinespace
$HHI_{c,t}$&      -1.110$^{\ast}$        &      -1.873                 &      -2.916$^{\ast\ast\ast}$&      -1.852$^{\ast\ast}$    &     -44.560$^{\ast\ast}$    &      15.266                 &     -42.472$^{\ast\ast\ast}$&     -17.353$^{\ast\ast\ast}$&      89.960$^{\ast\ast\ast}$&     -66.832$^{\ast\ast\ast}$&      -8.603                 \\
            &     (0.643)                 &     (2.304)                 &     (1.114)                 &     (0.788)                 &    (17.280)                 &    (10.888)                 &    (11.942)                 &     (5.830)                 &    (21.731)                 &    (24.851)                 &    (21.370)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001                 &       0.004$^{\ast\ast\ast}$&       0.002$^{\ast\ast}$    &      -0.000                 &       0.031$^{\ast\ast}$    &       0.014$^{\ast}$        &       0.011                 &       0.006                 &       0.010                 &       0.001                 &      -0.025                 \\
            &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.001)                 &     (0.013)                 &     (0.007)                 &     (0.011)                 &     (0.005)                 &     (0.016)                 &     (0.025)                 &     (0.020)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.004                 &      -0.006                 &       0.003                 &      -0.007                 &       0.165                 &      -0.076                 &       0.212$^{\ast\ast}$    &       0.028                 &      -0.154                 &       0.487$^{\ast}$        &       0.233                 \\
            &     (0.006)                 &     (0.009)                 &     (0.011)                 &     (0.005)                 &     (0.144)                 &     (0.093)                 &     (0.101)                 &     (0.045)                 &     (0.189)                 &     (0.260)                 &     (0.186)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.004$^{\ast\ast}$    &      -0.005                 &       0.006$^{\ast}$        &       0.000                 &       0.135$^{\ast\ast\ast}$&       0.020                 &       0.098$^{\ast\ast}$    &       0.017$^{\ast}$        &      -0.025                 &       0.092                 &      -0.080$^{\ast}$        \\
            &     (0.002)                 &     (0.005)                 &     (0.004)                 &     (0.002)                 &     (0.046)                 &     (0.025)                 &     (0.045)                 &     (0.010)                 &     (0.062)                 &     (0.081)                 &     (0.048)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.005                 &      -0.018                 &       0.012                 &      -0.018$^{\ast\ast\ast}$&      -0.029                 &       0.047                 &       0.031                 &      -0.107$^{\ast\ast}$    &      -0.080                 &       0.299                 &      -0.364$^{\ast}$        \\
            &     (0.005)                 &     (0.013)                 &     (0.009)                 &     (0.007)                 &     (0.142)                 &     (0.081)                 &     (0.112)                 &     (0.044)                 &     (0.174)                 &     (0.210)                 &     (0.187)                 \\\addlinespace
$XRate_{c,t}$&      -0.005$^{\ast\ast\ast}$&      -0.007                 &      -0.010$^{\ast\ast\ast}$&      -0.005$^{\ast\ast\ast}$&      -0.112$^{\ast\ast}$    &       0.005                 &      -0.109$^{\ast\ast}$    &      -0.009                 &       0.156$^{\ast\ast\ast}$&      -0.193$^{\ast\ast}$    &       0.089$^{\ast}$        \\
            &     (0.002)                 &     (0.005)                 &     (0.004)                 &     (0.002)                 &     (0.050)                 &     (0.020)                 &     (0.045)                 &     (0.011)                 &     (0.056)                 &     (0.079)                 &     (0.047)                 \\\midrule
Under-F     &         123                 &         123                 &         123                 &         123                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 \\
Under-p     &       .0213                 &       .0213                 &       .0213                 &       .0213                 &       .0185                 &       .0185                 &       .0185                 &       .0185                 &       .0185                 &       .0185                 &       .0185                 \\
Weak-CD F   &        3.76                 &        3.76                 &        3.76                 &        3.76                 &        4.65                 &        4.65                 &        4.65                 &        4.65                 &        4.65                 &        4.65                 &        4.65                 \\
Weak-KP rk F&        9.87                 &        9.87                 &        9.87                 &        9.87                 &        9.23                 &        9.23                 &        9.23                 &        9.23                 &        9.23                 &        9.23                 &        9.23                 \\
Over-Hansen J&         117                 &        85.6                 &         115                 &         108                 &         119                 &         108                 &         113                 &         123                 &         124                 &         108                 &         122                 \\
Over-Hansen J p&        .039                 &        .667                 &       .0505                 &        .128                 &       .0306                 &        .118                 &       .0678                 &       .0162                 &       .0155                 &        .123                 &       .0204                 \\
$R^{2}$  &        .946                 &         .62                 &        .845                 &        .912                 &        .468                 &        .352                 &        .291                 &        .623                 &        .356                 &        .308                 &        .325                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/IV/Results2RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.017$^{\ast\ast}$    &      -0.047$^{\ast\ast\ast}$&       0.039$^{\ast}$        &      -0.015                 &       0.157                 &      -0.338$^{\ast\ast\ast}$&       0.591$^{\ast\ast\ast}$&      -0.096                 &      -1.186$^{\ast\ast\ast}$&       1.482$^{\ast\ast\ast}$&      -0.499$^{\ast}$        \\
            &     (0.007)                 &     (0.013)                 &     (0.022)                 &     (0.011)                 &     (0.234)                 &     (0.123)                 &     (0.207)                 &     (0.068)                 &     (0.342)                 &     (0.455)                 &     (0.274)                 \\\addlinespace
$ICT_{c,t}$&      -0.072$^{\ast\ast\ast}$&      -0.125$^{\ast}$        &      -0.113$^{\ast\ast}$    &      -0.071$^{\ast\ast}$    &      -1.756$^{\ast\ast\ast}$&      -0.347                 &      -1.647$^{\ast\ast\ast}$&       0.239                 &       0.729                 &      -2.477$^{\ast}$        &       1.869$^{\ast\ast}$    \\
            &     (0.020)                 &     (0.075)                 &     (0.050)                 &     (0.031)                 &     (0.670)                 &     (0.369)                 &     (0.608)                 &     (0.212)                 &     (0.989)                 &     (1.278)                 &     (0.722)                 \\\addlinespace
$R*ICT_{c,t}$&       0.026$^{\ast\ast\ast}$&       0.035                 &       0.036                 &       0.047$^{\ast\ast\ast}$&       0.408                 &      -0.031                 &       0.405                 &       0.034                 &      -0.591                 &       0.817                 &      -0.299                 \\
            &     (0.009)                 &     (0.028)                 &     (0.023)                 &     (0.014)                 &     (0.319)                 &     (0.177)                 &     (0.276)                 &     (0.098)                 &     (0.458)                 &     (0.576)                 &     (0.348)                 \\\addlinespace
$wL_{c,t}$&       0.599$^{\ast\ast\ast}$&       0.721$^{\ast\ast\ast}$&       0.711$^{\ast\ast\ast}$&       0.615$^{\ast\ast\ast}$&      -0.452$^{\ast\ast\ast}$&       0.065                 &       0.117                 &      -0.634$^{\ast\ast\ast}$&       0.582$^{\ast\ast\ast}$&       0.789$^{\ast\ast\ast}$&      -1.407$^{\ast\ast\ast}$\\
            &     (0.089)                 &     (0.249)                 &     (0.157)                 &     (0.132)                 &     (0.108)                 &     (0.074)                 &     (0.096)                 &     (0.047)                 &     (0.199)                 &     (0.260)                 &     (0.141)                 \\\addlinespace
$rK_{c,t}$&       0.096$^{\ast}$        &       0.241                 &       0.154                 &       0.056                 &      -0.651$^{\ast\ast\ast}$&      -0.014                 &       0.023                 &      -0.660$^{\ast\ast\ast}$&       0.518$^{\ast\ast\ast}$&       0.716$^{\ast\ast\ast}$&      -1.326$^{\ast\ast\ast}$\\
            &     (0.053)                 &     (0.149)                 &     (0.103)                 &     (0.070)                 &     (0.097)                 &     (0.067)                 &     (0.082)                 &     (0.041)                 &     (0.186)                 &     (0.225)                 &     (0.126)                 \\\addlinespace
$pQ_{c,t}$&       0.202                 &      -0.058                 &       0.070                 &       0.261                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.136)                 &     (0.353)                 &     (0.225)                 &     (0.185)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.003                 &       0.006$^{\ast\ast\ast}$&      -0.002$^{\ast}$        &       0.005                 &      -0.030$^{\ast}$        &       0.040$^{\ast\ast}$    &      -0.005                 &      -0.107$^{\ast\ast}$    &       0.136$^{\ast\ast\ast}$&      -0.007                 \\
            &     (0.001)                 &     (0.002)                 &     (0.002)                 &     (0.001)                 &     (0.027)                 &     (0.017)                 &     (0.019)                 &     (0.009)                 &     (0.047)                 &     (0.051)                 &     (0.028)                 \\\addlinespace
$Services_{c,t}$&      -0.003                 &       0.011                 &      -0.012$^{\ast\ast}$    &      -0.015$^{\ast\ast\ast}$&      -0.005                 &       0.147$^{\ast\ast\ast}$&      -0.099$^{\ast}$        &      -0.053$^{\ast}$        &       0.488$^{\ast\ast\ast}$&      -0.310$^{\ast\ast}$    &      -0.193$^{\ast\ast\ast}$\\
            &     (0.002)                 &     (0.009)                 &     (0.005)                 &     (0.004)                 &     (0.064)                 &     (0.042)                 &     (0.051)                 &     (0.029)                 &     (0.110)                 &     (0.136)                 &     (0.069)                 \\\addlinespace
$HHI_{c,t}$&      -0.876$^{\ast\ast}$    &       2.309$^{\ast\ast}$    &      -3.476$^{\ast\ast\ast}$&      -2.798$^{\ast\ast\ast}$&     -12.749                 &      25.013$^{\ast\ast\ast}$&     -26.577$^{\ast\ast\ast}$&     -11.185$^{\ast\ast}$    &      89.593$^{\ast\ast\ast}$&     -71.822$^{\ast\ast\ast}$&     -16.892                 \\
            &     (0.369)                 &     (1.142)                 &     (0.889)                 &     (0.519)                 &    (10.616)                 &     (7.225)                 &     (8.536)                 &     (4.471)                 &    (18.760)                 &    (24.369)                 &    (13.211)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.002$^{\ast\ast\ast}$&      -0.000                 &       0.004$^{\ast\ast\ast}$&       0.002$^{\ast\ast\ast}$&       0.050$^{\ast\ast\ast}$&      -0.005                 &       0.036$^{\ast\ast\ast}$&       0.019$^{\ast\ast\ast}$&      -0.063$^{\ast\ast\ast}$&       0.060$^{\ast\ast\ast}$&      -0.006                 \\
            &     (0.000)                 &     (0.001)                 &     (0.001)                 &     (0.000)                 &     (0.008)                 &     (0.005)                 &     (0.006)                 &     (0.004)                 &     (0.013)                 &     (0.017)                 &     (0.011)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.008$^{\ast}$        &       0.006                 &      -0.022$^{\ast\ast}$    &      -0.012$^{\ast\ast}$    &      -0.323$^{\ast\ast\ast}$&      -0.043                 &      -0.175$^{\ast\ast}$    &      -0.105$^{\ast\ast}$    &       0.314$^{\ast\ast}$    &      -0.282                 &       0.208                 \\
            &     (0.005)                 &     (0.007)                 &     (0.010)                 &     (0.005)                 &     (0.104)                 &     (0.062)                 &     (0.087)                 &     (0.047)                 &     (0.158)                 &     (0.234)                 &     (0.155)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.005$^{\ast\ast\ast}$&      -0.002                 &       0.004$^{\ast}$        &       0.006$^{\ast\ast\ast}$&       0.118$^{\ast\ast\ast}$&       0.012                 &       0.073$^{\ast\ast\ast}$&       0.032$^{\ast\ast}$    &      -0.031                 &       0.052                 &      -0.035                 \\
            &     (0.001)                 &     (0.002)                 &     (0.002)                 &     (0.002)                 &     (0.031)                 &     (0.015)                 &     (0.025)                 &     (0.013)                 &     (0.042)                 &     (0.057)                 &     (0.032)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.007$^{\ast}$        &       0.008                 &       0.003                 &      -0.004                 &       0.007                 &       0.006                 &       0.059                 &      -0.058$^{\ast}$        &       0.014                 &       0.037                 &      -0.188                 \\
            &     (0.004)                 &     (0.010)                 &     (0.011)                 &     (0.006)                 &     (0.103)                 &     (0.057)                 &     (0.091)                 &     (0.032)                 &     (0.158)                 &     (0.203)                 &     (0.122)                 \\\addlinespace
$XRate_{c,t}$&      -0.005$^{\ast\ast\ast}$&      -0.006                 &      -0.004                 &      -0.009$^{\ast\ast\ast}$&      -0.096$^{\ast\ast}$    &      -0.021                 &      -0.068$^{\ast}$        &      -0.007                 &       0.069                 &      -0.073                 &       0.062                 \\
            &     (0.001)                 &     (0.004)                 &     (0.003)                 &     (0.002)                 &     (0.043)                 &     (0.022)                 &     (0.040)                 &     (0.013)                 &     (0.057)                 &     (0.085)                 &     (0.049)                 \\\midrule
Under-F     &         125                 &         125                 &         125                 &         125                 &         123                 &         123                 &         123                 &         123                 &         123                 &         123                 &         123                 \\
Under-p     &       .0142                 &       .0142                 &       .0142                 &       .0142                 &       .0213                 &       .0213                 &       .0213                 &       .0213                 &       .0213                 &       .0213                 &       .0213                 \\
Weak-CD F   &        3.27                 &        3.27                 &        3.27                 &        3.27                 &        3.05                 &        3.05                 &        3.05                 &        3.05                 &        3.05                 &        3.05                 &        3.05                 \\
Weak-KP rk F&        2.06                 &        2.06                 &        2.06                 &        2.06                 &        2.21                 &        2.21                 &        2.21                 &        2.21                 &        2.21                 &        2.21                 &        2.21                 \\
Over-Hansen J&         164                 &         123                 &         165                 &         169                 &         165                 &         167                 &         162                 &         153                 &         154                 &         150                 &         155                 \\
Over-Hansen J p&    5.55e-06                 &       .0163                 &    4.94e-06                 &    1.77e-06                 &    4.69e-06                 &    2.84e-06                 &    8.50e-06                 &    .0000728                 &    .0000515                 &     .000122                 &    .0000435                 \\
$R^{2}$  &        .938                 &        .716                 &        .681                 &         .87                 &        .499                 &        .224                 &        .256                 &        .764                 &        .369                 &        .157                 &         .41                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/IV/Results2shortV1_RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.010                 &       0.019                 &       0.018                 &      -0.057$^{\ast\ast\ast}$&       0.234                 &       0.273                 &       0.190                 &      -0.229                 &       0.598                 &       0.414                 &      -0.996$^{\ast}$        \\
            &     (0.015)                 &     (0.024)                 &     (0.049)                 &     (0.021)                 &     (0.509)                 &     (0.280)                 &     (0.419)                 &     (0.153)                 &     (0.765)                 &     (0.890)                 &     (0.556)                 \\\addlinespace
$ICT_{c,t}$&      -0.001                 &      -0.028                 &      -0.012                 &       0.010                 &      -0.130                 &      -0.386                 &      -0.016                 &       0.272                 &      -1.828$^{\ast}$        &       0.414                 &       1.297                 \\
            &     (0.029)                 &     (0.051)                 &     (0.063)                 &     (0.045)                 &     (0.969)                 &     (0.478)                 &     (0.791)                 &     (0.214)                 &     (1.044)                 &     (1.199)                 &     (0.911)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.011                 &       0.013                 &      -0.002                 &      -0.030                 &       0.070                 &      -0.010                 &       0.193                 &      -0.113                 &       0.705                 &      -0.297                 &      -0.432                 \\
            &     (0.018)                 &     (0.032)                 &     (0.036)                 &     (0.029)                 &     (0.617)                 &     (0.278)                 &     (0.553)                 &     (0.124)                 &     (0.650)                 &     (0.769)                 &     (0.553)                 \\\addlinespace
$wL_{c,t}$&       0.396$^{\ast\ast\ast}$&       0.331$^{\ast}$        &       0.529$^{\ast\ast\ast}$&       0.369$^{\ast\ast\ast}$&      -0.652$^{\ast\ast\ast}$&       0.045                 &       0.091                 &      -0.788$^{\ast\ast\ast}$&       0.723$^{\ast\ast}$    &       1.099$^{\ast\ast\ast}$&      -1.806$^{\ast\ast\ast}$\\
            &     (0.070)                 &     (0.174)                 &     (0.178)                 &     (0.141)                 &     (0.180)                 &     (0.101)                 &     (0.137)                 &     (0.091)                 &     (0.326)                 &     (0.368)                 &     (0.241)                 \\\addlinespace
$rK_{c,t}$&       0.022                 &       0.238$^{\ast}$        &       0.153                 &      -0.236$^{\ast\ast\ast}$&      -0.707$^{\ast\ast\ast}$&       0.022                 &       0.061                 &      -0.790$^{\ast\ast\ast}$&       0.735$^{\ast\ast\ast}$&       1.021$^{\ast\ast\ast}$&      -1.744$^{\ast\ast\ast}$\\
            &     (0.049)                 &     (0.134)                 &     (0.141)                 &     (0.079)                 &     (0.146)                 &     (0.082)                 &     (0.106)                 &     (0.081)                 &     (0.266)                 &     (0.271)                 &     (0.219)                 \\\addlinespace
$pQ_{c,t}$&       0.213$^{\ast}$        &       0.112                 &       0.216                 &       0.254                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.120)                 &     (0.298)                 &     (0.310)                 &     (0.183)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
Under-F     &        73.1                 &        73.1                 &        73.1                 &        73.1                 &        81.7                 &        81.7                 &        81.7                 &        81.7                 &        81.7                 &        81.7                 &        81.7                 \\
Under-p     &        .937                 &        .937                 &        .937                 &        .937                 &        .793                 &        .793                 &        .793                 &        .793                 &        .793                 &        .793                 &        .793                 \\
Weak-CD F   &        1.26                 &        1.26                 &        1.26                 &        1.26                 &        1.32                 &        1.32                 &        1.32                 &        1.32                 &        1.32                 &        1.32                 &        1.32                 \\
Weak-KP rk F&        17.6                 &        17.6                 &        17.6                 &        17.6                 &        20.3                 &        20.3                 &        20.3                 &        20.3                 &        20.3                 &        20.3                 &        20.3                 \\
Over-Hansen J&        96.5                 &         105                 &        99.8                 &         100                 &         104                 &         105                 &         107                 &          97                 &          90                 &        96.3                 &        93.5                 \\
Over-Hansen J p&        .354                 &        .165                 &         .27                 &        .268                 &        .187                 &        .168                 &        .138                 &        .341                 &        .539                 &        .358                 &        .437                 \\
$R^{2}$  &        .847                 &        .744                 &        .435                 &        .645                 &        .542                 &          .3                 &        .192                 &        .847                 &        .298                 &        .204                 &        .622                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/IV/Results2shortV1_RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.030$^{\ast}$        &      -0.084$^{\ast\ast}$    &      -0.086$^{\ast\ast\ast}$&       0.025                 &      -0.391                 &      -0.173                 &      -0.527$^{\ast}$        &       0.310$^{\ast\ast\ast}$&      -0.165                 &      -1.435$^{\ast\ast}$    &       0.982$^{\ast\ast\ast}$\\
            &     (0.016)                 &     (0.038)                 &     (0.029)                 &     (0.019)                 &     (0.331)                 &     (0.159)                 &     (0.295)                 &     (0.102)                 &     (0.470)                 &     (0.565)                 &     (0.335)                 \\\addlinespace
$ICT_{c,t}$&      -0.032                 &      -0.161$^{\ast}$        &      -0.107$^{\ast\ast}$    &       0.011                 &      -0.745                 &       0.304                 &      -1.216$^{\ast}$        &       0.167                 &       0.945                 &      -2.475$^{\ast\ast}$    &       0.896                 \\
            &     (0.025)                 &     (0.085)                 &     (0.051)                 &     (0.027)                 &     (0.780)                 &     (0.370)                 &     (0.673)                 &     (0.171)                 &     (0.909)                 &     (1.179)                 &     (0.664)                 \\\addlinespace
$R*ICT_{c,t}$&       0.001                 &       0.034                 &       0.013                 &      -0.012                 &       0.021                 &       0.049                 &      -0.059                 &       0.031                 &       0.311                 &       0.046                 &       0.103                 \\
            &     (0.013)                 &     (0.030)                 &     (0.025)                 &     (0.014)                 &     (0.442)                 &     (0.198)                 &     (0.351)                 &     (0.092)                 &     (0.423)                 &     (0.581)                 &     (0.359)                 \\\addlinespace
$wL_{c,t}$&       0.575$^{\ast\ast\ast}$&       1.370$^{\ast\ast\ast}$&       0.408$^{\ast\ast}$    &       0.618$^{\ast\ast\ast}$&      -0.594$^{\ast\ast\ast}$&      -0.132                 &       0.052                 &      -0.514$^{\ast\ast\ast}$&       0.180                 &       0.574$^{\ast\ast\ast}$&      -0.934$^{\ast\ast\ast}$\\
            &     (0.146)                 &     (0.453)                 &     (0.195)                 &     (0.148)                 &     (0.148)                 &     (0.091)                 &     (0.108)                 &     (0.059)                 &     (0.186)                 &     (0.220)                 &     (0.181)                 \\\addlinespace
$rK_{c,t}$&      -0.010                 &       0.284                 &      -0.093                 &       0.190$^{\ast\ast}$    &      -0.894$^{\ast\ast\ast}$&      -0.251$^{\ast\ast\ast}$&      -0.094                 &      -0.548$^{\ast\ast\ast}$&       0.030                 &       0.465$^{\ast\ast}$    &      -0.746$^{\ast\ast\ast}$\\
            &     (0.082)                 &     (0.258)                 &     (0.129)                 &     (0.090)                 &     (0.146)                 &     (0.088)                 &     (0.101)                 &     (0.055)                 &     (0.176)                 &     (0.203)                 &     (0.175)                 \\\addlinespace
$pQ_{c,t}$&       0.436$^{\ast\ast}$    &      -0.662                 &       0.646$^{\ast\ast}$    &       0.239                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.201)                 &     (0.652)                 &     (0.284)                 &     (0.211)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
Under-F     &         123                 &         123                 &         123                 &         123                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 &         124                 \\
Under-p     &       .0213                 &       .0213                 &       .0213                 &       .0213                 &       .0185                 &       .0185                 &       .0185                 &       .0185                 &       .0185                 &       .0185                 &       .0185                 \\
Weak-CD F   &        3.76                 &        3.76                 &        3.76                 &        3.76                 &        4.65                 &        4.65                 &        4.65                 &        4.65                 &        4.65                 &        4.65                 &        4.65                 \\
Weak-KP rk F&        9.87                 &        9.87                 &        9.87                 &        9.87                 &        9.23                 &        9.23                 &        9.23                 &        9.23                 &        9.23                 &        9.23                 &        9.23                 \\
Over-Hansen J&         117                 &        85.6                 &         115                 &         108                 &         119                 &         108                 &         113                 &         123                 &         124                 &         108                 &         122                 \\
Over-Hansen J p&        .039                 &        .667                 &       .0505                 &        .128                 &       .0306                 &        .118                 &       .0678                 &       .0162                 &       .0155                 &        .123                 &       .0204                 \\
$R^{2}$  &        .946                 &         .62                 &        .845                 &        .912                 &        .468                 &        .352                 &        .291                 &        .623                 &        .356                 &        .308                 &        .325                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/IV/Results2shortV1_RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.017$^{\ast\ast}$    &      -0.047$^{\ast\ast\ast}$&       0.039$^{\ast}$        &      -0.015                 &       0.157                 &      -0.338$^{\ast\ast\ast}$&       0.591$^{\ast\ast\ast}$&      -0.096                 &      -1.186$^{\ast\ast\ast}$&       1.482$^{\ast\ast\ast}$&      -0.499$^{\ast}$        \\
            &     (0.007)                 &     (0.013)                 &     (0.022)                 &     (0.011)                 &     (0.234)                 &     (0.123)                 &     (0.207)                 &     (0.068)                 &     (0.342)                 &     (0.455)                 &     (0.274)                 \\\addlinespace
$ICT_{c,t}$&      -0.072$^{\ast\ast\ast}$&      -0.125$^{\ast}$        &      -0.113$^{\ast\ast}$    &      -0.071$^{\ast\ast}$    &      -1.756$^{\ast\ast\ast}$&      -0.347                 &      -1.647$^{\ast\ast\ast}$&       0.239                 &       0.729                 &      -2.477$^{\ast}$        &       1.869$^{\ast\ast}$    \\
            &     (0.020)                 &     (0.075)                 &     (0.050)                 &     (0.031)                 &     (0.670)                 &     (0.369)                 &     (0.608)                 &     (0.212)                 &     (0.989)                 &     (1.278)                 &     (0.722)                 \\\addlinespace
$R*ICT_{c,t}$&       0.026$^{\ast\ast\ast}$&       0.035                 &       0.036                 &       0.047$^{\ast\ast\ast}$&       0.408                 &      -0.031                 &       0.405                 &       0.034                 &      -0.591                 &       0.817                 &      -0.299                 \\
            &     (0.009)                 &     (0.028)                 &     (0.023)                 &     (0.014)                 &     (0.319)                 &     (0.177)                 &     (0.276)                 &     (0.098)                 &     (0.458)                 &     (0.576)                 &     (0.348)                 \\\addlinespace
$wL_{c,t}$&       0.599$^{\ast\ast\ast}$&       0.721$^{\ast\ast\ast}$&       0.711$^{\ast\ast\ast}$&       0.615$^{\ast\ast\ast}$&      -0.452$^{\ast\ast\ast}$&       0.065                 &       0.117                 &      -0.634$^{\ast\ast\ast}$&       0.582$^{\ast\ast\ast}$&       0.789$^{\ast\ast\ast}$&      -1.407$^{\ast\ast\ast}$\\
            &     (0.089)                 &     (0.249)                 &     (0.157)                 &     (0.132)                 &     (0.108)                 &     (0.074)                 &     (0.096)                 &     (0.047)                 &     (0.199)                 &     (0.260)                 &     (0.141)                 \\\addlinespace
$rK_{c,t}$&       0.096$^{\ast}$        &       0.241                 &       0.154                 &       0.056                 &      -0.651$^{\ast\ast\ast}$&      -0.014                 &       0.023                 &      -0.660$^{\ast\ast\ast}$&       0.518$^{\ast\ast\ast}$&       0.716$^{\ast\ast\ast}$&      -1.326$^{\ast\ast\ast}$\\
            &     (0.053)                 &     (0.149)                 &     (0.103)                 &     (0.070)                 &     (0.097)                 &     (0.067)                 &     (0.082)                 &     (0.041)                 &     (0.186)                 &     (0.225)                 &     (0.126)                 \\\addlinespace
$pQ_{c,t}$&       0.202                 &      -0.058                 &       0.070                 &       0.261                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.136)                 &     (0.353)                 &     (0.225)                 &     (0.185)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
Under-F     &         125                 &         125                 &         125                 &         125                 &         123                 &         123                 &         123                 &         123                 &         123                 &         123                 &         123                 \\
Under-p     &       .0142                 &       .0142                 &       .0142                 &       .0142                 &       .0213                 &       .0213                 &       .0213                 &       .0213                 &       .0213                 &       .0213                 &       .0213                 \\
Weak-CD F   &        3.27                 &        3.27                 &        3.27                 &        3.27                 &        3.05                 &        3.05                 &        3.05                 &        3.05                 &        3.05                 &        3.05                 &        3.05                 \\
Weak-KP rk F&        2.06                 &        2.06                 &        2.06                 &        2.06                 &        2.21                 &        2.21                 &        2.21                 &        2.21                 &        2.21                 &        2.21                 &        2.21                 \\
Over-Hansen J&         164                 &         123                 &         165                 &         169                 &         165                 &         167                 &         162                 &         153                 &         154                 &         150                 &         155                 \\
Over-Hansen J p&    5.55e-06                 &       .0163                 &    4.94e-06                 &    1.77e-06                 &    4.69e-06                 &    2.84e-06                 &    8.50e-06                 &    .0000728                 &    .0000515                 &     .000122                 &    .0000435                 \\
%$R^{2}$  &        .938                 &        .716                 &        .681                 &         .87                 &        .499                 &        .224                 &        .256                 &        .764                 &        .369                 &        .157                 &         .41                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/IV/Results4RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.040$^{\ast\ast}$    &       0.020                 &      -0.037$^{\ast\ast}$    &      -0.011                 &       0.014$^{\ast\ast\ast}$&      -1.687$^{\ast\ast\ast}$&       0.004                 &       0.008$^{\ast}$        \\
            &     (0.019)                 &     (0.014)                 &     (0.018)                 &     (0.021)                 &     (0.004)                 &     (0.522)                 &     (0.004)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.052                 &       0.011                 &       0.038                 &       0.122$^{\ast\ast\ast}$&      -0.015$^{\ast\ast}$    &       3.100$^{\ast\ast\ast}$&      -0.002                 &       0.012                 \\
            &     (0.040)                 &     (0.043)                 &     (0.042)                 &     (0.046)                 &     (0.006)                 &     (1.139)                 &     (0.007)                 &     (0.010)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.051$^{\ast\ast}$    &      -0.002                 &      -0.034                 &      -0.051$^{\ast}$        &       0.005                 &      -0.840                 &      -0.000                 &       0.004                 \\
            &     (0.024)                 &     (0.023)                 &     (0.023)                 &     (0.029)                 &     (0.003)                 &     (0.609)                 &     (0.004)                 &     (0.006)                 \\\midrule
Under-F     &        85.7                 &        85.7                 &        85.7                 &        85.7                 &        85.7                 &        85.7                 &        85.7                 &        85.7                 \\
Under-p     &        .692                 &        .692                 &        .692                 &        .692                 &        .692                 &        .692                 &        .692                 &        .692                 \\
Weak-CD F   &        1.21                 &        1.21                 &        1.21                 &        1.21                 &        1.21                 &        1.21                 &        1.21                 &        1.21                 \\
Weak-KP rk F&        7.34                 &        7.34                 &        7.34                 &        7.34                 &        7.34                 &        7.34                 &        7.34                 &        7.34                 \\
Over-Hansen J&        93.5                 &          95                 &         108                 &         105                 &         106                 &          95                 &        90.2                 &          99                 \\
Over-Hansen J p&        .436                 &        .396                 &        .126                 &        .161                 &        .157                 &        .396                 &        .535                 &        .289                 \\
$R^{2}$  &        .534                 &        .556                 &        .488                 &         .62                 &        .571                 &        .587                 &        .109                 &        .331                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/IV/Results4RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.138$^{\ast\ast\ast}$&      -0.030$^{\ast\ast}$    &      -0.064$^{\ast\ast\ast}$&      -0.061$^{\ast\ast\ast}$&       0.003                 &      -1.865$^{\ast\ast\ast}$&      -0.006                 &       0.016$^{\ast\ast}$    \\
            &     (0.021)                 &     (0.014)                 &     (0.020)                 &     (0.012)                 &     (0.002)                 &     (0.340)                 &     (0.004)                 &     (0.007)                 \\\addlinespace
$ICT_{c,t}$&       0.294$^{\ast\ast\ast}$&      -0.146$^{\ast\ast\ast}$&       0.145$^{\ast\ast\ast}$&      -0.059$^{\ast\ast\ast}$&       0.017$^{\ast\ast\ast}$&      -2.582$^{\ast\ast\ast}$&      -0.010                 &       0.019                 \\
            &     (0.040)                 &     (0.019)                 &     (0.030)                 &     (0.022)                 &     (0.004)                 &     (0.743)                 &     (0.010)                 &     (0.012)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.131$^{\ast\ast\ast}$&       0.040$^{\ast\ast\ast}$&      -0.068$^{\ast\ast\ast}$&       0.024$^{\ast\ast}$    &      -0.010$^{\ast\ast\ast}$&       1.353$^{\ast\ast\ast}$&       0.001                 &      -0.005                 \\
            &     (0.021)                 &     (0.010)                 &     (0.015)                 &     (0.012)                 &     (0.002)                 &     (0.411)                 &     (0.005)                 &     (0.007)                 \\\midrule
Under-F     &         108                 &         108                 &         108                 &         108                 &         108                 &         108                 &         108                 &         108                 \\
Under-p     &        .135                 &        .135                 &        .135                 &        .135                 &        .135                 &        .135                 &        .135                 &        .135                 \\
Weak-CD F   &        4.08                 &        4.08                 &        4.08                 &        4.08                 &        4.08                 &        4.08                 &        4.08                 &        4.08                 \\
Weak-KP rk F&        7.12                 &        7.12                 &        7.12                 &        7.12                 &        7.12                 &        7.12                 &        7.12                 &        7.12                 \\
Over-Hansen J&         120                 &         111                 &         117                 &         117                 &         119                 &        94.3                 &        87.1                 &         120                 \\
Over-Hansen J p&       .0266                 &       .0851                 &       .0392                 &       .0386                 &       .0297                 &        .413                 &        .624                 &       .0248                 \\
$R^{2}$  &        .733                 &        .634                 &        .535                 &        .655                 &        .305                 &        .375                 &        .416                 &        .263                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/IV/Results4RICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.141$^{\ast\ast\ast}$&       0.007                 &      -0.084$^{\ast\ast\ast}$&      -0.046$^{\ast\ast\ast}$&       0.001                 &      -0.690$^{\ast\ast}$    &       0.006$^{\ast}$        &       0.038$^{\ast\ast\ast}$\\
            &     (0.020)                 &     (0.009)                 &     (0.016)                 &     (0.014)                 &     (0.002)                 &     (0.270)                 &     (0.003)                 &     (0.006)                 \\\addlinespace
$ICT_{c,t}$&       0.167$^{\ast\ast}$    &      -0.104$^{\ast\ast\ast}$&       0.037                 &      -0.000                 &       0.005                 &      -0.107                 &      -0.007                 &       0.063$^{\ast\ast\ast}$\\
            &     (0.085)                 &     (0.030)                 &     (0.045)                 &     (0.053)                 &     (0.007)                 &     (1.039)                 &     (0.011)                 &     (0.014)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.079$^{\ast}$        &       0.041$^{\ast\ast\ast}$&      -0.012                 &      -0.007                 &      -0.003                 &       0.617                 &       0.006                 &      -0.018$^{\ast\ast}$    \\
            &     (0.042)                 &     (0.014)                 &     (0.021)                 &     (0.025)                 &     (0.004)                 &     (0.517)                 &     (0.006)                 &     (0.007)                 \\\midrule
Under-F     &         138                 &         138                 &         138                 &         138                 &         138                 &         138                 &         138                 &         138                 \\
Under-p     &      .00176                 &      .00176                 &      .00176                 &      .00176                 &      .00176                 &      .00176                 &      .00176                 &      .00176                 \\
Weak-CD F   &        3.25                 &        3.25                 &        3.25                 &        3.25                 &        3.25                 &        3.25                 &        3.25                 &        3.25                 \\
Weak-KP rk F&        2.32                 &        2.32                 &        2.32                 &        2.32                 &        2.32                 &        2.32                 &        2.32                 &        2.32                 \\
Over-Hansen J&         160                 &         147                 &         159                 &         171                 &         176                 &         150                 &         150                 &         130                 \\
Over-Hansen J p&    .0000152                 &     .000232                 &    .0000192                 &    1.09e-06                 &    3.60e-07                 &     .000138                 &     .000119                 &      .00535                 \\
$R^{2}$  &        .628                 &         .43                 &        .541                 &        .476                 &        .252                 &        .507                 &        .147                 &        .278                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/IV/Results4shortRICTint_ct_All_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.040$^{\ast\ast}$    &       0.020                 &      -0.037$^{\ast\ast}$    &      -0.011                 &      -1.687$^{\ast\ast\ast}$&       0.008$^{\ast}$        \\
            &     (0.019)                 &     (0.014)                 &     (0.018)                 &     (0.021)                 &     (0.522)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.052                 &       0.011                 &       0.038                 &       0.122$^{\ast\ast\ast}$&       3.100$^{\ast\ast\ast}$&       0.012                 \\
            &     (0.040)                 &     (0.043)                 &     (0.042)                 &     (0.046)                 &     (1.139)                 &     (0.010)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.051$^{\ast\ast}$    &      -0.002                 &      -0.034                 &      -0.051$^{\ast}$        &      -0.840                 &       0.004                 \\
            &     (0.024)                 &     (0.023)                 &     (0.023)                 &     (0.029)                 &     (0.609)                 &     (0.006)                 \\\midrule
Under-F     &        85.7                 &        85.7                 &        85.7                 &        85.7                 &        85.7                 &        85.7                 \\
Under-p     &        .692                 &        .692                 &        .692                 &        .692                 &        .692                 &        .692                 \\
Weak-CD F   &        1.21                 &        1.21                 &        1.21                 &        1.21                 &        1.21                 &        1.21                 \\
Weak-KP rk F&        7.34                 &        7.34                 &        7.34                 &        7.34                 &        7.34                 &        7.34                 \\
Over-Hansen J&        93.5                 &          95                 &         108                 &         105                 &          95                 &          99                 \\
Over-Hansen J p&        .436                 &        .396                 &        .126                 &        .161                 &        .396                 &        .289                 \\
$R^{2}$  &        .534                 &        .556                 &        .488                 &         .62                 &        .587                 &        .331                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/IV/Results4shortRICTint_ct_All_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.138$^{\ast\ast\ast}$&      -0.030$^{\ast\ast}$    &      -0.064$^{\ast\ast\ast}$&      -0.061$^{\ast\ast\ast}$&      -1.865$^{\ast\ast\ast}$&       0.016$^{\ast\ast}$    \\
            &     (0.021)                 &     (0.014)                 &     (0.020)                 &     (0.012)                 &     (0.340)                 &     (0.007)                 \\\addlinespace
$ICT_{c,t}$&       0.294$^{\ast\ast\ast}$&      -0.146$^{\ast\ast\ast}$&       0.145$^{\ast\ast\ast}$&      -0.059$^{\ast\ast\ast}$&      -2.582$^{\ast\ast\ast}$&       0.019                 \\
            &     (0.040)                 &     (0.019)                 &     (0.030)                 &     (0.022)                 &     (0.743)                 &     (0.012)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.131$^{\ast\ast\ast}$&       0.040$^{\ast\ast\ast}$&      -0.068$^{\ast\ast\ast}$&       0.024$^{\ast\ast}$    &       1.353$^{\ast\ast\ast}$&      -0.005                 \\
            &     (0.021)                 &     (0.010)                 &     (0.015)                 &     (0.012)                 &     (0.411)                 &     (0.007)                 \\\midrule
Under-F     &         108                 &         108                 &         108                 &         108                 &         108                 &         108                 \\
Under-p     &        .135                 &        .135                 &        .135                 &        .135                 &        .135                 &        .135                 \\
Weak-CD F   &        4.08                 &        4.08                 &        4.08                 &        4.08                 &        4.08                 &        4.08                 \\
Weak-KP rk F&        7.12                 &        7.12                 &        7.12                 &        7.12                 &        7.12                 &        7.12                 \\
Over-Hansen J&         120                 &         111                 &         117                 &         117                 &        94.3                 &         120                 \\
Over-Hansen J p&       .0266                 &       .0851                 &       .0392                 &       .0386                 &        .413                 &       .0248                 \\
$R^{2}$  &        .733                 &        .634                 &        .535                 &        .655                 &        .375                 &        .263                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/IV/Results4shortRICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $Services_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.141$^{\ast\ast\ast}$&       0.007                 &      -0.084$^{\ast\ast\ast}$&      -0.046$^{\ast\ast\ast}$&      -0.690$^{\ast\ast}$    &       0.038$^{\ast\ast\ast}$\\
            &     (0.020)                 &     (0.009)                 &     (0.016)                 &     (0.014)                 &     (0.270)                 &     (0.006)                 \\\addlinespace
$ICT_{c,t}$&       0.167$^{\ast\ast}$    &      -0.104$^{\ast\ast\ast}$&       0.037                 &      -0.000                 &      -0.107                 &       0.063$^{\ast\ast\ast}$\\
            &     (0.085)                 &     (0.030)                 &     (0.045)                 &     (0.053)                 &     (1.039)                 &     (0.014)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.079$^{\ast}$        &       0.041$^{\ast\ast\ast}$&      -0.012                 &      -0.007                 &       0.617                 &      -0.018$^{\ast\ast}$    \\
            &     (0.042)                 &     (0.014)                 &     (0.021)                 &     (0.025)                 &     (0.517)                 &     (0.007)                 \\\midrule
Under-F     &         138                 &         138                 &         138                 &         138                 &         138                 &         138                 \\
Under-p     &      .00176                 &      .00176                 &      .00176                 &      .00176                 &      .00176                 &      .00176                 \\
Weak-CD F   &        3.25                 &        3.25                 &        3.25                 &        3.25                 &        3.25                 &        3.25                 \\
Weak-KP rk F&        2.32                 &        2.32                 &        2.32                 &        2.32                 &        2.32                 &        2.32                 \\
Over-Hansen J&         160                 &         147                 &         159                 &         171                 &         150                 &         130                 \\
Over-Hansen J p&    .0000152                 &     .000232                 &    .0000192                 &    1.09e-06                 &     .000138                 &      .00535                 \\
%$R^{2}$  &        .628                 &         .43                 &        .541                 &        .476                 &        .507                 &        .278                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/IV/Results5RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.011                 &      -0.043                 &      -0.031                 &      -0.008                 &       0.052$^{\ast\ast}$    &      -0.034$^{\ast\ast}$    &       0.024                 &      -0.006                 \\
            &     (0.028)                 &     (0.044)                 &     (0.023)                 &     (0.022)                 &     (0.026)                 &     (0.015)                 &     (0.022)                 &     (0.010)                 \\\addlinespace
$ICT_{c,t}$&       0.098                 &       0.118$^{\ast}$        &       0.108$^{\ast}$        &       0.077                 &       0.058                 &       0.030                 &      -0.003                 &       0.031                 \\
            &     (0.064)                 &     (0.064)                 &     (0.057)                 &     (0.055)                 &     (0.061)                 &     (0.035)                 &     (0.044)                 &     (0.022)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.055                 &      -0.062                 &      -0.064$^{\ast}$        &      -0.056$^{\ast}$        &      -0.040                 &      -0.031                 &      -0.008                 &      -0.009                 \\
            &     (0.038)                 &     (0.044)                 &     (0.034)                 &     (0.032)                 &     (0.044)                 &     (0.023)                 &     (0.030)                 &     (0.017)                 \\\midrule
Under-F     &        91.6                 &        91.6                 &        91.6                 &        91.6                 &        76.8                 &        76.8                 &        76.8                 &        76.8                 \\
Under-p     &        .521                 &        .521                 &        .521                 &        .521                 &        .888                 &        .888                 &        .888                 &        .888                 \\
Weak-CD F   &        1.26                 &        1.26                 &        1.26                 &        1.26                 &        1.18                 &        1.18                 &        1.18                 &        1.18                 \\
Weak-KP rk F&        7.68                 &        7.68                 &        7.68                 &        7.68                 &         129                 &         129                 &         129                 &         129                 \\
Over-Hansen J&         101                 &         103                 &         110                 &         114                 &                          &                          &                          &                          \\
Over-Hansen J p&        .244                 &        .194                 &       .0971                 &       .0569                 &                             &                             &                             &                             \\
$R^{2}$  &        .539                 &        .618                 &        .677                 &        .716                 &        .728                 &         .45                 &        .428                 &        .322                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         135                 &         135                 &         135                 &         135                 \\


==> inputs/robustness/IV/Results5RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.179$^{\ast\ast\ast}$&      -0.136$^{\ast\ast\ast}$&      -0.168$^{\ast\ast\ast}$&      -0.116$^{\ast\ast\ast}$&      -0.061$^{\ast\ast\ast}$&      -0.116$^{\ast\ast\ast}$&      -0.019$^{\ast}$        &       0.009                 \\
            &     (0.026)                 &     (0.027)                 &     (0.024)                 &     (0.026)                 &     (0.011)                 &     (0.015)                 &     (0.011)                 &     (0.008)                 \\\addlinespace
$ICT_{c,t}$&       0.111$^{\ast\ast}$    &      -0.043                 &       0.046                 &       0.092$^{\ast}$        &       0.015                 &       0.003                 &       0.141$^{\ast\ast\ast}$&      -0.098$^{\ast\ast\ast}$\\
            &     (0.049)                 &     (0.056)                 &     (0.051)                 &     (0.051)                 &     (0.021)                 &     (0.038)                 &     (0.023)                 &     (0.021)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.061$^{\ast\ast}$    &      -0.037                 &      -0.047$^{\ast}$        &      -0.078$^{\ast\ast\ast}$&      -0.008                 &      -0.006                 &      -0.057$^{\ast\ast\ast}$&       0.061$^{\ast\ast\ast}$\\
            &     (0.025)                 &     (0.028)                 &     (0.025)                 &     (0.025)                 &     (0.012)                 &     (0.021)                 &     (0.014)                 &     (0.012)                 \\\midrule
Under-F     &         103                 &         103                 &         103                 &         103                 &         107                 &         107                 &         107                 &         107                 \\
Under-p     &        .218                 &        .218                 &        .218                 &        .218                 &        .155                 &        .155                 &        .155                 &        .155                 \\
Weak-CD F   &        4.19                 &        4.19                 &        4.19                 &        4.19                 &        6.46                 &        6.46                 &        6.46                 &        6.46                 \\
Weak-KP rk F&        6.95                 &        6.95                 &        6.95                 &        6.95                 &        18.6                 &        18.6                 &        18.6                 &        18.6                 \\
Over-Hansen J&         119                 &         124                 &         125                 &         121                 &        99.8                 &        92.1                 &         108                 &         106                 \\
Over-Hansen J p&       .0321                 &       .0157                 &       .0126                 &       .0219                 &        .272                 &        .479                 &        .117                 &        .145                 \\
$R^{2}$  &        .636                 &        .512                 &        .617                 &        .583                 &        .602                 &        .638                 &        .739                 &        .532                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         174                 &         174                 &         174                 &         174                 \\


==> inputs/robustness/IV/Results5RICTint_ct_All_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.131$^{\ast\ast\ast}$&      -0.133$^{\ast\ast\ast}$&      -0.137$^{\ast\ast\ast}$&      -0.114$^{\ast\ast\ast}$&       0.010                 &      -0.106$^{\ast\ast\ast}$&      -0.013                 &      -0.001                 \\
            &     (0.022)                 &     (0.023)                 &     (0.021)                 &     (0.021)                 &     (0.015)                 &     (0.015)                 &     (0.015)                 &     (0.007)                 \\\addlinespace
$ICT_{c,t}$&       0.051                 &      -0.080                 &      -0.002                 &       0.029                 &       0.041                 &      -0.035                 &       0.115$^{\ast\ast\ast}$&      -0.066$^{\ast\ast\ast}$\\
            &     (0.076)                 &     (0.081)                 &     (0.072)                 &     (0.072)                 &     (0.036)                 &     (0.038)                 &     (0.043)                 &     (0.021)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.029                 &       0.025                 &      -0.008                 &      -0.030                 &      -0.026                 &       0.026                 &      -0.065$^{\ast\ast}$    &       0.038$^{\ast\ast\ast}$\\
            &     (0.039)                 &     (0.037)                 &     (0.036)                 &     (0.036)                 &     (0.023)                 &     (0.021)                 &     (0.026)                 &     (0.012)                 \\\midrule
Under-F     &         139                 &         139                 &         139                 &         139                 &         117                 &         117                 &         117                 &         117                 \\
Under-p     &      .00142                 &      .00142                 &      .00142                 &      .00142                 &       .0468                 &       .0468                 &       .0468                 &       .0468                 \\
Weak-CD F   &        3.21                 &        3.21                 &        3.21                 &        3.21                 &        3.65                 &        3.65                 &        3.65                 &        3.65                 \\
Weak-KP rk F&        2.23                 &        2.23                 &        2.23                 &        2.23                 &        2.89                 &        2.89                 &        2.89                 &        2.89                 \\
Over-Hansen J&         166                 &         160                 &         169                 &         162                 &         153                 &         137                 &         170                 &         151                 \\
Over-Hansen J p&    3.49e-06                 &    .0000134                 &    1.90e-06                 &    9.64e-06                 &    .0000695                 &      .00156                 &    1.32e-06                 &     .000112                 \\
%$R^{2}$  &        .527                 &        .409                 &        .496                 &        .523                 &        .579                 &        .589                 &        .642                 &        .368                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         309                 &         309                 &         309                 &         309                 \\


==> inputs/robustness/IVlags/Results1RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.004                 &       0.008                 &       0.051                 &      -0.031                 &       0.392                 &       0.117                 &       0.426                 &      -0.152                 &      -0.073                 &       1.012                 &      -0.895                 \\
            &     (0.017)                 &     (0.027)                 &     (0.057)                 &     (0.024)                 &     (0.651)                 &     (0.298)                 &     (0.447)                 &     (0.313)                 &     (0.916)                 &     (1.137)                 &     (0.723)                 \\\addlinespace
$ICT_{c,t}$&      -0.019                 &      -0.014                 &       0.005                 &      -0.031                 &      -0.475                 &      -0.312                 &       0.438                 &      -0.601                 &      -1.222                 &       2.349                 &      -1.254                 \\
            &     (0.037)                 &     (0.060)                 &     (0.066)                 &     (0.067)                 &     (1.366)                 &     (0.639)                 &     (0.895)                 &     (0.699)                 &     (1.445)                 &     (1.601)                 &     (1.443)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.004                 &       0.011                 &       0.004                 &      -0.023                 &      -0.099                 &      -0.142                 &       0.139                 &      -0.095                 &       0.466                 &      -0.396                 &      -0.063                 \\
            &     (0.021)                 &     (0.037)                 &     (0.040)                 &     (0.036)                 &     (0.854)                 &     (0.314)                 &     (0.545)                 &     (0.393)                 &     (0.778)                 &     (0.815)                 &     (0.766)                 \\\midrule
Under-F     &        11.6                 &        11.6                 &        11.6                 &        11.6                 &        11.3                 &        11.3                 &        11.3                 &        11.3                 &        11.3                 &        11.3                 &        11.3                 \\
Under-p     &       .0202                 &       .0202                 &       .0202                 &       .0202                 &       .0234                 &       .0234                 &       .0234                 &       .0234                 &       .0234                 &       .0234                 &       .0234                 \\
Weak-CD F   &        17.3                 &        17.3                 &        17.3                 &        17.3                 &        17.5                 &        17.5                 &        17.5                 &        17.5                 &        17.5                 &        17.5                 &        17.5                 \\
Weak-KP rk F&        20.3                 &        20.3                 &        20.3                 &        20.3                 &        22.5                 &        22.5                 &        22.5                 &        22.5                 &        22.5                 &        22.5                 &        22.5                 \\
Over-Hansen J&        7.42                 &        4.76                 &        2.78                 &         7.6                 &        2.61                 &        7.41                 &        3.45                 &        3.72                 &        2.33                 &        3.78                 &        7.73                 \\
Over-Hansen J p&       .0596                 &         .19                 &        .427                 &        .055                 &        .456                 &       .0599                 &        .327                 &        .294                 &        .507                 &        .287                 &       .0519                 \\
$R^{2}$  &        .807                 &        .724                 &        .409                 &        .537                 &        .451                 &         .29                 &        .184                 &        .502                 &        .222                 &        .109                 &         .28                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/IVlags/Results1RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.072$^{\ast\ast\ast}$&      -0.109$^{\ast\ast}$    &      -0.148$^{\ast\ast\ast}$&      -0.022                 &      -0.886$^{\ast}$        &      -0.101                 &      -0.931$^{\ast\ast}$    &       0.147                 &       0.223                 &      -2.407$^{\ast\ast\ast}$&       1.022$^{\ast\ast}$    \\
            &     (0.018)                 &     (0.043)                 &     (0.036)                 &     (0.016)                 &     (0.473)                 &     (0.240)                 &     (0.366)                 &     (0.135)                 &     (0.560)                 &     (0.679)                 &     (0.461)                 \\\addlinespace
$ICT_{c,t}$&      -0.019                 &      -0.015                 &      -0.105$^{\ast\ast}$    &      -0.040                 &       1.063                 &       1.458$^{\ast\ast}$    &      -0.512                 &       0.117                 &       2.590$^{\ast\ast\ast}$&      -3.130$^{\ast\ast\ast}$&      -0.409                 \\
            &     (0.030)                 &     (0.084)                 &     (0.052)                 &     (0.030)                 &     (1.086)                 &     (0.582)                 &     (0.736)                 &     (0.318)                 &     (0.993)                 &     (1.179)                 &     (0.925)                 \\\addlinespace
$R*ICT_{c,t}$&       0.013                 &       0.002                 &       0.031                 &       0.025                 &      -0.651                 &      -0.377                 &      -0.211                 &      -0.062                 &      -0.258                 &       0.718                 &       0.209                 \\
            &     (0.017)                 &     (0.030)                 &     (0.028)                 &     (0.016)                 &     (0.582)                 &     (0.242)                 &     (0.403)                 &     (0.143)                 &     (0.423)                 &     (0.633)                 &     (0.421)                 \\\midrule
Under-F     &          49                 &          49                 &          49                 &          49                 &        43.3                 &        43.3                 &        43.3                 &        43.3                 &        43.3                 &        43.3                 &        43.3                 \\
Under-p     &    5.95e-10                 &    5.95e-10                 &    5.95e-10                 &    5.95e-10                 &    9.15e-09                 &    9.15e-09                 &    9.15e-09                 &    9.15e-09                 &    9.15e-09                 &    9.15e-09                 &    9.15e-09                 \\
Weak-CD F   &        36.9                 &        36.9                 &        36.9                 &        36.9                 &        40.8                 &        40.8                 &        40.8                 &        40.8                 &        40.8                 &        40.8                 &        40.8                 \\
Weak-KP rk F&          21                 &          21                 &          21                 &          21                 &          24                 &          24                 &          24                 &          24                 &          24                 &          24                 &          24                 \\
Over-Hansen J&        3.02                 &        4.66                 &        2.04                 &        .979                 &        1.38                 &        3.15                 &        .665                 &        4.02                 &        4.85                 &        .534                 &         2.2                 \\
Over-Hansen J p&        .389                 &        .199                 &        .564                 &        .806                 &        .711                 &        .369                 &        .881                 &        .259                 &        .183                 &        .911                 &        .533                 \\
$R^{2}$  &        .928                 &        .565                 &        .835                 &        .896                 &         .25                 &        .247                 &        .247                 &        .206                 &        .328                 &        .275                 &        .197                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/IVlags/Results1RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.035$^{\ast\ast\ast}$&      -0.056$^{\ast\ast\ast}$&      -0.014                 &      -0.025$^{\ast\ast}$    &       0.042                 &      -0.260$^{\ast\ast}$    &       0.262                 &       0.040                 &      -0.865$^{\ast\ast\ast}$&       0.487                 &      -0.000                 \\
            &     (0.010)                 &     (0.013)                 &     (0.023)                 &     (0.011)                 &     (0.263)                 &     (0.115)                 &     (0.224)                 &     (0.108)                 &     (0.333)                 &     (0.483)                 &     (0.309)                 \\\addlinespace
$ICT_{c,t}$&      -0.037$^{\ast}$        &       0.000                 &      -0.132$^{\ast\ast\ast}$&      -0.034                 &      -0.794                 &       0.947$^{\ast}$        &      -1.606$^{\ast\ast\ast}$&      -0.135                 &       3.097$^{\ast\ast\ast}$&      -3.297$^{\ast\ast\ast}$&       0.318                 \\
            &     (0.022)                 &     (0.072)                 &     (0.040)                 &     (0.025)                 &     (0.655)                 &     (0.572)                 &     (0.436)                 &     (0.274)                 &     (1.192)                 &     (0.996)                 &     (0.729)                 \\\addlinespace
$R*ICT_{c,t}$&       0.017                 &      -0.015                 &       0.059$^{\ast\ast\ast}$&       0.033$^{\ast\ast\ast}$&       0.130                 &      -0.599$^{\ast\ast}$    &       0.523$^{\ast\ast}$    &       0.205                 &      -1.724$^{\ast\ast\ast}$&       1.372$^{\ast\ast\ast}$&       0.345                 \\
            &     (0.011)                 &     (0.029)                 &     (0.019)                 &     (0.012)                 &     (0.332)                 &     (0.244)                 &     (0.224)                 &     (0.130)                 &     (0.494)                 &     (0.475)                 &     (0.342)                 \\\midrule
Under-F     &        16.7                 &        16.7                 &        16.7                 &        16.7                 &        16.2                 &        16.2                 &        16.2                 &        16.2                 &        16.2                 &        16.2                 &        16.2                 \\
Under-p     &      .00221                 &      .00221                 &      .00221                 &      .00221                 &      .00276                 &      .00276                 &      .00276                 &      .00276                 &      .00276                 &      .00276                 &      .00276                 \\
Weak-CD F   &        97.8                 &        97.8                 &        97.8                 &        97.8                 &        98.8                 &        98.8                 &        98.8                 &        98.8                 &        98.8                 &        98.8                 &        98.8                 \\
Weak-KP rk F&        10.7                 &        10.7                 &        10.7                 &        10.7                 &        10.6                 &        10.6                 &        10.6                 &        10.6                 &        10.6                 &        10.6                 &        10.6                 \\
Over-Hansen J&        7.82                 &        .928                 &        4.98                 &        8.55                 &        4.22                 &        2.37                 &         2.6                 &        3.63                 &         .39                 &        1.21                 &        2.12                 \\
Over-Hansen J p&       .0498                 &        .819                 &        .173                 &       .0358                 &        .239                 &        .499                 &        .457                 &        .304                 &        .942                 &         .75                 &        .548                 \\
$R^{2}$  &        .915                 &        .696                 &        .661                 &        .846                 &        .376                 &        .176                 &        .244                 &        .436                 &        .338                 &         .12                 &        .175                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/IVlags/Results2RICTint_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.016                 &       0.007                 &       0.034                 &      -0.069$^{\ast\ast\ast}$&       0.110                 &       0.033                 &       0.364                 &      -0.287                 &       0.038                 &       0.985                 &      -0.985$^{\ast}$        \\
            &     (0.016)                 &     (0.026)                 &     (0.051)                 &     (0.024)                 &     (0.513)                 &     (0.294)                 &     (0.423)                 &     (0.173)                 &     (0.829)                 &     (0.942)                 &     (0.561)                 \\\addlinespace
$ICT_{c,t}$&       0.020                 &      -0.011                 &       0.039                 &       0.043                 &       0.808                 &      -0.218                 &       0.442                 &       0.585$^{\ast\ast}$    &      -2.337                 &       1.139                 &       1.070                 \\
            &     (0.043)                 &     (0.062)                 &     (0.076)                 &     (0.068)                 &     (1.200)                 &     (0.683)                 &     (1.004)                 &     (0.275)                 &     (1.490)                 &     (1.645)                 &     (0.962)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.022                 &       0.002                 &      -0.015                 &      -0.047                 &      -0.298                 &      -0.181                 &       0.142                 &      -0.259                 &       0.602                 &      -0.247                 &      -0.350                 \\
            &     (0.024)                 &     (0.037)                 &     (0.042)                 &     (0.038)                 &     (0.711)                 &     (0.323)                 &     (0.583)                 &     (0.159)                 &     (0.728)                 &     (0.861)                 &     (0.563)                 \\\addlinespace
$wL_{c,t}$&       0.405$^{\ast\ast\ast}$&       0.342$^{\ast}$        &       0.540$^{\ast\ast\ast}$&       0.384$^{\ast\ast\ast}$&      -0.681$^{\ast\ast\ast}$&       0.060                 &       0.054                 &      -0.795$^{\ast\ast\ast}$&       0.795$^{\ast\ast}$    &       1.015$^{\ast\ast\ast}$&      -1.797$^{\ast\ast\ast}$\\
            &     (0.070)                 &     (0.178)                 &     (0.180)                 &     (0.139)                 &     (0.185)                 &     (0.101)                 &     (0.134)                 &     (0.092)                 &     (0.317)                 &     (0.345)                 &     (0.241)                 \\\addlinespace
$rK_{c,t}$&       0.015                 &       0.229$^{\ast}$        &       0.143                 &      -0.248$^{\ast\ast\ast}$&      -0.746$^{\ast\ast\ast}$&       0.029                 &       0.026                 &      -0.801$^{\ast\ast\ast}$&       0.795$^{\ast\ast\ast}$&       0.948$^{\ast\ast\ast}$&      -1.734$^{\ast\ast\ast}$\\
            &     (0.050)                 &     (0.136)                 &     (0.144)                 &     (0.081)                 &     (0.155)                 &     (0.086)                 &     (0.109)                 &     (0.082)                 &     (0.273)                 &     (0.260)                 &     (0.219)                 \\\addlinespace
$pQ_{c,t}$&       0.202                 &       0.102                 &       0.202                 &       0.236                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.122)                 &     (0.302)                 &     (0.304)                 &     (0.183)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.000                 &      -0.003                 &       0.001                 &       0.004$^{\ast\ast\ast}$&      -0.086$^{\ast\ast}$    &      -0.050$^{\ast\ast}$    &      -0.023                 &      -0.013                 &      -0.080                 &       0.045                 &       0.030                 \\
            &     (0.001)                 &     (0.002)                 &     (0.003)                 &     (0.002)                 &     (0.037)                 &     (0.024)                 &     (0.029)                 &     (0.011)                 &     (0.074)                 &     (0.078)                 &     (0.043)                 \\\addlinespace
$Services_{c,t}$&      -0.000                 &       0.020$^{\ast\ast\ast}$&       0.007                 &      -0.021$^{\ast\ast\ast}$&       0.206                 &       0.129$^{\ast}$        &       0.103                 &      -0.025                 &       0.220                 &       0.022                 &      -0.254                 \\
            &     (0.003)                 &     (0.006)                 &     (0.012)                 &     (0.006)                 &     (0.137)                 &     (0.068)                 &     (0.116)                 &     (0.047)                 &     (0.217)                 &     (0.270)                 &     (0.154)                 \\\addlinespace
$HHI_{c,t}$&      -0.805                 &       1.614                 &      -0.582                 &      -3.553$^{\ast\ast\ast}$&      19.847                 &      15.637                 &      -2.055                 &       6.265                 &      16.609                 &     -23.991                 &       4.356                 \\
            &     (0.564)                 &     (1.033)                 &     (2.228)                 &     (0.949)                 &    (21.407)                 &    (12.118)                 &    (19.615)                 &     (7.058)                 &    (40.341)                 &    (48.249)                 &    (26.100)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast\ast\ast}$&       0.001                 &      -0.001                 &       0.045$^{\ast\ast\ast}$&      -0.004                 &       0.023$^{\ast\ast}$    &       0.026$^{\ast\ast\ast}$&      -0.043$^{\ast\ast}$    &       0.025                 &       0.022$^{\ast}$        \\
            &     (0.000)                 &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.011)                 &     (0.005)                 &     (0.009)                 &     (0.004)                 &     (0.020)                 &     (0.023)                 &     (0.011)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.013$^{\ast\ast}$    &       0.021$^{\ast\ast}$    &      -0.037$^{\ast}$        &       0.042$^{\ast\ast\ast}$&      -0.801$^{\ast\ast\ast}$&      -0.030                 &      -0.430$^{\ast\ast\ast}$&      -0.341$^{\ast\ast\ast}$&       0.719$^{\ast\ast\ast}$&      -0.627$^{\ast\ast}$    &      -0.140                 \\
            &     (0.006)                 &     (0.010)                 &     (0.022)                 &     (0.009)                 &     (0.192)                 &     (0.077)                 &     (0.132)                 &     (0.072)                 &     (0.213)                 &     (0.274)                 &     (0.195)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003$^{\ast\ast\ast}$&       0.001                 &       0.008$^{\ast\ast\ast}$&       0.000                 &       0.090$^{\ast\ast}$    &       0.008                 &       0.076$^{\ast\ast\ast}$&       0.006                 &      -0.055$^{\ast}$        &       0.137$^{\ast\ast\ast}$&      -0.090$^{\ast\ast\ast}$\\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.001)                 &     (0.041)                 &     (0.010)                 &     (0.026)                 &     (0.015)                 &     (0.031)                 &     (0.040)                 &     (0.029)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.005                 &       0.024$^{\ast\ast\ast}$&      -0.005                 &      -0.004                 &       0.131                 &       0.132$^{\ast}$        &       0.065                 &      -0.067                 &       0.437$^{\ast\ast\ast}$&      -0.141                 &      -0.284                 \\
            &     (0.005)                 &     (0.008)                 &     (0.017)                 &     (0.006)                 &     (0.196)                 &     (0.070)                 &     (0.137)                 &     (0.041)                 &     (0.146)                 &     (0.258)                 &     (0.184)                 \\\addlinespace
$XRate_{c,t}$&       0.009                 &      -0.004                 &       0.010                 &       0.023$^{\ast\ast\ast}$&       0.027                 &       0.006                 &      -0.017                 &       0.038                 &      -0.164                 &       0.151                 &       0.005                 \\
            &     (0.006)                 &     (0.011)                 &     (0.011)                 &     (0.008)                 &     (0.212)                 &     (0.091)                 &     (0.178)                 &     (0.049)                 &     (0.202)                 &     (0.252)                 &     (0.179)                 \\\midrule
Under-F     &        11.3                 &        11.3                 &        11.3                 &        11.3                 &        11.1                 &        11.1                 &        11.1                 &        11.1                 &        11.1                 &        11.1                 &        11.1                 \\
Under-p     &        .023                 &        .023                 &        .023                 &        .023                 &       .0251                 &       .0251                 &       .0251                 &       .0251                 &       .0251                 &       .0251                 &       .0251                 \\
Weak-CD F   &        15.5                 &        15.5                 &        15.5                 &        15.5                 &        15.4                 &        15.4                 &        15.4                 &        15.4                 &        15.4                 &        15.4                 &        15.4                 \\
Weak-KP rk F&        16.3                 &        16.3                 &        16.3                 &        16.3                 &        16.8                 &        16.8                 &        16.8                 &        16.8                 &        16.8                 &        16.8                 &        16.8                 \\
Over-Hansen J&        7.18                 &        4.42                 &        2.93                 &        6.55                 &        4.51                 &        7.33                 &        3.54                 &        1.76                 &        2.41                 &        1.75                 &        4.31                 \\
Over-Hansen J p&       .0665                 &         .22                 &        .403                 &       .0877                 &        .212                 &        .062                 &        .315                 &        .623                 &        .491                 &        .625                 &         .23                 \\
$R^{2}$  &        .848                 &        .744                 &        .433                 &        .645                 &        .541                 &        .295                 &        .187                 &        .845                 &        .288                 &        .197                 &        .623                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/IVlags/Results2RICTint_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.053$^{\ast\ast\ast}$&      -0.037                 &      -0.144$^{\ast\ast\ast}$&       0.001                 &      -0.513                 &      -0.000                 &      -0.935$^{\ast\ast}$    &       0.422$^{\ast\ast\ast}$&       0.170                 &      -2.698$^{\ast\ast\ast}$&       1.471$^{\ast\ast\ast}$\\
            &     (0.019)                 &     (0.039)                 &     (0.040)                 &     (0.018)                 &     (0.444)                 &     (0.213)                 &     (0.376)                 &     (0.113)                 &     (0.552)                 &     (0.696)                 &     (0.414)                 \\\addlinespace
$ICT_{c,t}$&      -0.061$^{\ast\ast}$    &      -0.010                 &      -0.156$^{\ast\ast\ast}$&      -0.058$^{\ast}$        &      -0.025                 &       1.068                 &      -1.236                 &       0.144                 &       1.943$^{\ast}$        &      -4.097$^{\ast\ast\ast}$&       0.842                 \\
            &     (0.031)                 &     (0.076)                 &     (0.058)                 &     (0.035)                 &     (1.180)                 &     (0.693)                 &     (0.796)                 &     (0.223)                 &     (1.155)                 &     (1.320)                 &     (0.922)                 \\\addlinespace
$R*ICT_{c,t}$&       0.020                 &      -0.027                 &       0.046                 &       0.022                 &      -0.189                 &      -0.225                 &       0.002                 &       0.034                 &      -0.091                 &       0.895                 &       0.010                 \\
            &     (0.016)                 &     (0.033)                 &     (0.031)                 &     (0.015)                 &     (0.580)                 &     (0.265)                 &     (0.420)                 &     (0.108)                 &     (0.474)                 &     (0.672)                 &     (0.455)                 \\\addlinespace
$wL_{c,t}$&       0.490$^{\ast\ast\ast}$&       1.473$^{\ast\ast\ast}$&       0.210                 &       0.542$^{\ast\ast\ast}$&      -0.621$^{\ast\ast\ast}$&      -0.158$^{\ast}$        &       0.052                 &      -0.515$^{\ast\ast\ast}$&       0.151                 &       0.602$^{\ast\ast\ast}$&      -0.923$^{\ast\ast\ast}$\\
            &     (0.149)                 &     (0.503)                 &     (0.210)                 &     (0.148)                 &     (0.150)                 &     (0.088)                 &     (0.111)                 &     (0.058)                 &     (0.185)                 &     (0.222)                 &     (0.178)                 \\\addlinespace
$rK_{c,t}$&      -0.068                 &       0.502                 &      -0.213                 &       0.086                 &      -0.887$^{\ast\ast\ast}$&      -0.249$^{\ast\ast\ast}$&      -0.086                 &      -0.552$^{\ast\ast\ast}$&       0.033                 &       0.461$^{\ast\ast}$    &      -0.751$^{\ast\ast\ast}$\\
            &     (0.084)                 &     (0.337)                 &     (0.138)                 &     (0.097)                 &     (0.151)                 &     (0.092)                 &     (0.104)                 &     (0.053)                 &     (0.181)                 &     (0.208)                 &     (0.173)                 \\\addlinespace
$pQ_{c,t}$&       0.558$^{\ast\ast\ast}$&      -0.949                 &       0.906$^{\ast\ast\ast}$&       0.401$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.203)                 &     (0.770)                 &     (0.298)                 &     (0.213)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.002                 &      -0.006$^{\ast}$        &      -0.003                 &       0.003                 &       0.004                 &      -0.059$^{\ast\ast}$    &       0.004                 &       0.058$^{\ast\ast\ast}$&      -0.149$^{\ast\ast}$    &      -0.070                 &       0.187$^{\ast\ast\ast}$\\
            &     (0.002)                 &     (0.004)                 &     (0.003)                 &     (0.002)                 &     (0.040)                 &     (0.025)                 &     (0.031)                 &     (0.017)                 &     (0.061)                 &     (0.063)                 &     (0.058)                 \\\addlinespace
$Services_{c,t}$&       0.001                 &      -0.022                 &      -0.016$^{\ast\ast}$    &      -0.002                 &      -0.051                 &       0.186$^{\ast\ast\ast}$&      -0.238$^{\ast\ast\ast}$&       0.002                 &       0.623$^{\ast\ast\ast}$&      -0.688$^{\ast\ast\ast}$&      -0.007                 \\
            &     (0.004)                 &     (0.021)                 &     (0.008)                 &     (0.005)                 &     (0.105)                 &     (0.071)                 &     (0.081)                 &     (0.031)                 &     (0.144)                 &     (0.170)                 &     (0.105)                 \\\addlinespace
$HHI_{c,t}$&      -0.811                 &      -3.003                 &      -2.395$^{\ast\ast}$    &      -1.272                 &     -49.016$^{\ast\ast\ast}$&      12.585                 &     -45.205$^{\ast\ast\ast}$&     -16.396$^{\ast\ast\ast}$&      87.064$^{\ast\ast\ast}$&     -66.572$^{\ast\ast}$    &      -5.172                 \\
            &     (0.675)                 &     (2.721)                 &     (1.157)                 &     (0.847)                 &    (17.803)                 &    (11.406)                 &    (12.344)                 &     (5.610)                 &    (22.332)                 &    (26.119)                 &    (21.503)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001$^{\ast\ast}$    &       0.003$^{\ast\ast}$    &       0.003$^{\ast\ast\ast}$&       0.000                 &       0.033$^{\ast\ast}$    &       0.012                 &       0.017                 &       0.005                 &       0.005                 &       0.023                 &      -0.033$^{\ast}$        \\
            &     (0.001)                 &     (0.001)                 &     (0.001)                 &     (0.001)                 &     (0.014)                 &     (0.008)                 &     (0.011)                 &     (0.005)                 &     (0.017)                 &     (0.025)                 &     (0.019)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.005                 &      -0.007                 &       0.001                 &      -0.007                 &       0.138                 &      -0.089                 &       0.193$^{\ast\ast}$    &       0.034                 &      -0.166                 &       0.470$^{\ast\ast}$    &       0.259                 \\
            &     (0.006)                 &     (0.010)                 &     (0.010)                 &     (0.005)                 &     (0.147)                 &     (0.101)                 &     (0.091)                 &     (0.042)                 &     (0.202)                 &     (0.218)                 &     (0.176)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.004$^{\ast\ast}$    &      -0.006                 &       0.007$^{\ast}$        &       0.000                 &       0.138$^{\ast\ast\ast}$&       0.022                 &       0.100$^{\ast\ast}$    &       0.017                 &      -0.023                 &       0.093                 &      -0.083$^{\ast}$        \\
            &     (0.002)                 &     (0.005)                 &     (0.004)                 &     (0.002)                 &     (0.047)                 &     (0.026)                 &     (0.046)                 &     (0.010)                 &     (0.064)                 &     (0.085)                 &     (0.048)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.004                 &      -0.012                 &       0.014                 &      -0.020$^{\ast\ast\ast}$&       0.001                 &       0.103                 &      -0.005                 &      -0.097$^{\ast\ast}$    &      -0.001                 &       0.124                 &      -0.332$^{\ast}$        \\
            &     (0.005)                 &     (0.012)                 &     (0.009)                 &     (0.007)                 &     (0.146)                 &     (0.089)                 &     (0.120)                 &     (0.044)                 &     (0.190)                 &     (0.228)                 &     (0.188)                 \\\addlinespace
$XRate_{c,t}$&      -0.005$^{\ast\ast\ast}$&      -0.003                 &      -0.011$^{\ast\ast\ast}$&      -0.006$^{\ast\ast\ast}$&      -0.091                 &       0.032                 &      -0.117$^{\ast\ast}$    &      -0.007                 &       0.192$^{\ast\ast\ast}$&      -0.263$^{\ast\ast\ast}$&       0.095$^{\ast}$        \\
            &     (0.002)                 &     (0.004)                 &     (0.004)                 &     (0.002)                 &     (0.063)                 &     (0.033)                 &     (0.049)                 &     (0.012)                 &     (0.065)                 &     (0.084)                 &     (0.053)                 \\\midrule
Under-F     &        55.7                 &        55.7                 &        55.7                 &        55.7                 &        42.5                 &        42.5                 &        42.5                 &        42.5                 &        42.5                 &        42.5                 &        42.5                 \\
Under-p     &    2.29e-11                 &    2.29e-11                 &    2.29e-11                 &    2.29e-11                 &    1.34e-08                 &    1.34e-08                 &    1.34e-08                 &    1.34e-08                 &    1.34e-08                 &    1.34e-08                 &    1.34e-08                 \\
Weak-CD F   &        28.5                 &        28.5                 &        28.5                 &        28.5                 &        37.2                 &        37.2                 &        37.2                 &        37.2                 &        37.2                 &        37.2                 &        37.2                 \\
Weak-KP rk F&          14                 &          14                 &          14                 &          14                 &        20.1                 &        20.1                 &        20.1                 &        20.1                 &        20.1                 &        20.1                 &        20.1                 \\
Over-Hansen J&        4.72                 &        2.98                 &        2.94                 &        3.55                 &        3.04                 &        4.48                 &        1.08                 &        1.68                 &        4.94                 &        .814                 &        1.87                 \\
Over-Hansen J p&        .193                 &        .395                 &        .401                 &        .314                 &        .386                 &        .214                 &        .783                 &        .642                 &        .176                 &        .846                 &        .599                 \\
$R^{2}$  &        .945                 &        .608                 &        .842                 &         .91                 &        .463                 &        .329                 &        .295                 &        .623                 &        .349                 &        .295                 &        .327                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/IVlags/Results2RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.025$^{\ast\ast\ast}$&      -0.041$^{\ast\ast\ast}$&      -0.003                 &      -0.015                 &      -0.008                 &      -0.276$^{\ast\ast}$    &       0.235                 &       0.033                 &      -0.872$^{\ast\ast\ast}$&       0.457                 &       0.020                 \\
            &     (0.008)                 &     (0.012)                 &     (0.023)                 &     (0.010)                 &     (0.230)                 &     (0.111)                 &     (0.226)                 &     (0.071)                 &     (0.319)                 &     (0.506)                 &     (0.272)                 \\\addlinespace
$ICT_{c,t}$&      -0.073$^{\ast\ast\ast}$&      -0.019                 &      -0.173$^{\ast\ast\ast}$&      -0.077$^{\ast\ast\ast}$&      -1.256$^{\ast}$        &       0.656                 &      -2.168$^{\ast\ast\ast}$&       0.257                 &       2.559$^{\ast\ast}$    &      -4.492$^{\ast\ast\ast}$&       1.798$^{\ast\ast\ast}$\\
            &     (0.017)                 &     (0.066)                 &     (0.041)                 &     (0.028)                 &     (0.716)                 &     (0.583)                 &     (0.504)                 &     (0.206)                 &     (1.115)                 &     (1.278)                 &     (0.623)                 \\\addlinespace
$R*ICT_{c,t}$&       0.027$^{\ast\ast\ast}$&      -0.012                 &       0.072$^{\ast\ast\ast}$&       0.046$^{\ast\ast\ast}$&       0.243                 &      -0.492$^{\ast\ast}$    &       0.739$^{\ast\ast\ast}$&      -0.004                 &      -1.476$^{\ast\ast\ast}$&       1.893$^{\ast\ast\ast}$&      -0.337                 \\
            &     (0.008)                 &     (0.025)                 &     (0.019)                 &     (0.012)                 &     (0.325)                 &     (0.240)                 &     (0.248)                 &     (0.094)                 &     (0.474)                 &     (0.566)                 &     (0.298)                 \\\addlinespace
$wL_{c,t}$&       0.587$^{\ast\ast\ast}$&       0.715$^{\ast\ast\ast}$&       0.644$^{\ast\ast\ast}$&       0.627$^{\ast\ast\ast}$&      -0.470$^{\ast\ast\ast}$&       0.028                 &       0.137                 &      -0.635$^{\ast\ast\ast}$&       0.513$^{\ast\ast\ast}$&       0.868$^{\ast\ast\ast}$&      -1.407$^{\ast\ast\ast}$\\
            &     (0.088)                 &     (0.246)                 &     (0.149)                 &     (0.132)                 &     (0.105)                 &     (0.070)                 &     (0.094)                 &     (0.048)                 &     (0.193)                 &     (0.251)                 &     (0.142)                 \\\addlinespace
$rK_{c,t}$&       0.087$^{\ast}$        &       0.286$^{\ast}$        &       0.081                 &       0.057                 &      -0.663$^{\ast\ast\ast}$&      -0.035                 &       0.031                 &      -0.660$^{\ast\ast\ast}$&       0.482$^{\ast\ast\ast}$&       0.749$^{\ast\ast\ast}$&      -1.320$^{\ast\ast\ast}$\\
            &     (0.052)                 &     (0.158)                 &     (0.101)                 &     (0.069)                 &     (0.096)                 &     (0.064)                 &     (0.081)                 &     (0.042)                 &     (0.181)                 &     (0.217)                 &     (0.128)                 \\\addlinespace
$pQ_{c,t}$&       0.214                 &      -0.085                 &       0.160                 &       0.248                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.136)                 &     (0.363)                 &     (0.220)                 &     (0.183)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.003$^{\ast}$        &       0.005$^{\ast\ast\ast}$&      -0.002$^{\ast}$        &       0.003                 &      -0.034$^{\ast}$        &       0.041$^{\ast\ast}$    &      -0.004                 &      -0.114$^{\ast\ast}$    &       0.143$^{\ast\ast\ast}$&      -0.006                 \\
            &     (0.001)                 &     (0.002)                 &     (0.002)                 &     (0.001)                 &     (0.027)                 &     (0.018)                 &     (0.019)                 &     (0.010)                 &     (0.046)                 &     (0.048)                 &     (0.028)                 \\\addlinespace
$Services_{c,t}$&      -0.004                 &       0.011                 &      -0.014$^{\ast\ast\ast}$&      -0.015$^{\ast\ast\ast}$&      -0.018                 &       0.159$^{\ast\ast\ast}$&      -0.135$^{\ast\ast}$    &      -0.041                 &       0.526$^{\ast\ast\ast}$&      -0.406$^{\ast\ast\ast}$&      -0.154$^{\ast\ast}$    \\
            &     (0.002)                 &     (0.009)                 &     (0.005)                 &     (0.004)                 &     (0.064)                 &     (0.044)                 &     (0.054)                 &     (0.029)                 &     (0.114)                 &     (0.143)                 &     (0.068)                 \\\addlinespace
$HHI_{c,t}$&      -0.842$^{\ast\ast}$    &       2.124$^{\ast}$        &      -3.252$^{\ast\ast\ast}$&      -2.758$^{\ast\ast\ast}$&     -13.378                 &      25.014$^{\ast\ast\ast}$&     -27.500$^{\ast\ast\ast}$&     -10.892$^{\ast\ast}$    &      90.048$^{\ast\ast\ast}$&     -73.367$^{\ast\ast\ast}$&     -16.158                 \\
            &     (0.371)                 &     (1.177)                 &     (0.910)                 &     (0.520)                 &    (10.465)                 &     (7.261)                 &     (8.596)                 &     (4.490)                 &    (18.854)                 &    (24.729)                 &    (13.226)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.002$^{\ast\ast\ast}$&       0.000                 &       0.003$^{\ast\ast\ast}$&       0.002$^{\ast\ast\ast}$&       0.051$^{\ast\ast\ast}$&      -0.004                 &       0.036$^{\ast\ast\ast}$&       0.019$^{\ast\ast\ast}$&      -0.061$^{\ast\ast\ast}$&       0.058$^{\ast\ast\ast}$&      -0.005                 \\
            &     (0.000)                 &     (0.001)                 &     (0.001)                 &     (0.000)                 &     (0.007)                 &     (0.005)                 &     (0.006)                 &     (0.004)                 &     (0.012)                 &     (0.016)                 &     (0.011)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.008$^{\ast}$        &       0.002                 &      -0.018$^{\ast\ast}$    &      -0.012$^{\ast\ast}$    &      -0.331$^{\ast\ast\ast}$&      -0.062                 &      -0.161$^{\ast\ast}$    &      -0.108$^{\ast\ast}$    &       0.275$^{\ast}$        &      -0.225                 &       0.197                 \\
            &     (0.004)                 &     (0.007)                 &     (0.009)                 &     (0.005)                 &     (0.102)                 &     (0.064)                 &     (0.079)                 &     (0.048)                 &     (0.156)                 &     (0.215)                 &     (0.153)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.005$^{\ast\ast\ast}$&      -0.002                 &       0.004$^{\ast}$        &       0.006$^{\ast\ast\ast}$&       0.116$^{\ast\ast\ast}$&       0.012                 &       0.071$^{\ast\ast\ast}$&       0.033$^{\ast\ast\ast}$&      -0.030                 &       0.046                 &      -0.031                 \\
            &     (0.001)                 &     (0.002)                 &     (0.002)                 &     (0.002)                 &     (0.031)                 &     (0.016)                 &     (0.026)                 &     (0.013)                 &     (0.045)                 &     (0.059)                 &     (0.031)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.007$^{\ast}$        &       0.011                 &       0.003                 &      -0.004                 &       0.015                 &       0.047                 &       0.016                 &      -0.047                 &       0.105                 &      -0.117                 &      -0.148                 \\
            &     (0.004)                 &     (0.010)                 &     (0.011)                 &     (0.006)                 &     (0.104)                 &     (0.058)                 &     (0.091)                 &     (0.032)                 &     (0.158)                 &     (0.210)                 &     (0.121)                 \\\addlinespace
$XRate_{c,t}$&      -0.005$^{\ast\ast\ast}$&      -0.000                 &      -0.007$^{\ast\ast}$    &      -0.009$^{\ast\ast\ast}$&      -0.071                 &       0.031                 &      -0.096$^{\ast\ast\ast}$&      -0.005                 &       0.166$^{\ast\ast}$    &      -0.188$^{\ast\ast}$    &       0.064                 \\
            &     (0.001)                 &     (0.004)                 &     (0.003)                 &     (0.002)                 &     (0.047)                 &     (0.035)                 &     (0.036)                 &     (0.013)                 &     (0.070)                 &     (0.087)                 &     (0.046)                 \\\midrule
Under-F     &        20.3                 &        20.3                 &        20.3                 &        20.3                 &          21                 &          21                 &          21                 &          21                 &          21                 &          21                 &          21                 \\
Under-p     &     .000433                 &     .000433                 &     .000433                 &     .000433                 &     .000322                 &     .000322                 &     .000322                 &     .000322                 &     .000322                 &     .000322                 &     .000322                 \\
Weak-CD F   &        91.5                 &        91.5                 &        91.5                 &        91.5                 &        89.2                 &        89.2                 &        89.2                 &        89.2                 &        89.2                 &        89.2                 &        89.2                 \\
Weak-KP rk F&        9.65                 &        9.65                 &        9.65                 &        9.65                 &        9.75                 &        9.75                 &        9.75                 &        9.75                 &        9.75                 &        9.75                 &        9.75                 \\
Over-Hansen J&        8.91                 &        .606                 &        4.07                 &        5.06                 &        2.64                 &         1.7                 &        2.48                 &        4.36                 &        .156                 &        2.12                 &        3.89                 \\
Over-Hansen J p&       .0305                 &        .895                 &        .255                 &        .167                 &        .451                 &        .637                 &         .48                 &        .225                 &        .984                 &        .547                 &        .273                 \\
$R^{2}$  &        .938                 &        .715                 &        .682                 &        .871                 &        .501                 &        .214                 &        .264                 &        .763                 &        .366                 &        .155                 &        .411                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/IVlags/Results2shortV1_RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.013                 &       0.016                 &       0.038                 &      -0.071$^{\ast\ast\ast}$&       0.226                 &       0.090                 &       0.406                 &      -0.270                 &       0.120                 &       0.964                 &      -1.080$^{\ast}$        \\
            &     (0.017)                 &     (0.027)                 &     (0.052)                 &     (0.024)                 &     (0.531)                 &     (0.300)                 &     (0.431)                 &     (0.169)                 &     (0.823)                 &     (0.942)                 &     (0.569)                 \\\addlinespace
$ICT_{c,t}$&       0.018                 &      -0.014                 &       0.030                 &       0.042                 &       0.764                 &      -0.193                 &       0.371                 &       0.586$^{\ast\ast}$    &      -2.235                 &       0.998                 &       1.089                 \\
            &     (0.044)                 &     (0.061)                 &     (0.075)                 &     (0.070)                 &     (1.186)                 &     (0.675)                 &     (0.951)                 &     (0.269)                 &     (1.438)                 &     (1.575)                 &     (0.947)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.022                 &       0.002                 &      -0.014                 &      -0.047                 &      -0.309                 &      -0.191                 &       0.139                 &      -0.257                 &       0.585                 &      -0.247                 &      -0.330                 \\
            &     (0.024)                 &     (0.037)                 &     (0.041)                 &     (0.038)                 &     (0.703)                 &     (0.322)                 &     (0.573)                 &     (0.157)                 &     (0.723)                 &     (0.852)                 &     (0.558)                 \\\addlinespace
$wL_{c,t}$&       0.403$^{\ast\ast\ast}$&       0.336$^{\ast}$        &       0.535$^{\ast\ast\ast}$&       0.385$^{\ast\ast\ast}$&      -0.683$^{\ast\ast\ast}$&       0.056                 &       0.057                 &      -0.796$^{\ast\ast\ast}$&       0.785$^{\ast\ast}$    &       1.026$^{\ast\ast\ast}$&      -1.795$^{\ast\ast\ast}$\\
            &     (0.071)                 &     (0.174)                 &     (0.180)                 &     (0.137)                 &     (0.185)                 &     (0.101)                 &     (0.134)                 &     (0.092)                 &     (0.315)                 &     (0.345)                 &     (0.240)                 \\\addlinespace
$rK_{c,t}$&       0.019                 &       0.238$^{\ast}$        &       0.152                 &      -0.249$^{\ast\ast\ast}$&      -0.743$^{\ast\ast\ast}$&       0.027                 &       0.032                 &      -0.801$^{\ast\ast\ast}$&       0.788$^{\ast\ast\ast}$&       0.961$^{\ast\ast\ast}$&      -1.736$^{\ast\ast\ast}$\\
            &     (0.049)                 &     (0.136)                 &     (0.145)                 &     (0.081)                 &     (0.154)                 &     (0.085)                 &     (0.108)                 &     (0.082)                 &     (0.269)                 &     (0.257)                 &     (0.218)                 \\\addlinespace
$pQ_{c,t}$&       0.202$^{\ast}$        &       0.102                 &       0.202                 &       0.236                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.121)                 &     (0.297)                 &     (0.303)                 &     (0.182)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
Under-F     &        11.6                 &        11.6                 &        11.6                 &        11.6                 &        11.1                 &        11.1                 &        11.1                 &        11.1                 &        11.1                 &        11.1                 &        11.1                 \\
Under-p     &        .115                 &        .115                 &        .115                 &        .115                 &        .132                 &        .132                 &        .132                 &        .132                 &        .132                 &        .132                 &        .132                 \\
Weak-CD F   &        10.3                 &        10.3                 &        10.3                 &        10.3                 &        10.3                 &        10.3                 &        10.3                 &        10.3                 &        10.3                 &        10.3                 &        10.3                 \\
Weak-KP rk F&        15.7                 &        15.7                 &        15.7                 &        15.7                 &        16.3                 &        16.3                 &        16.3                 &        16.3                 &        16.3                 &        16.3                 &        16.3                 \\
Over-Hansen J&        8.77                 &        8.08                 &         7.9                 &        8.28                 &        6.97                 &        8.79                 &        9.52                 &        3.09                 &           4                 &         6.9                 &        6.14                 \\
Over-Hansen J p&        .187                 &        .232                 &        .245                 &        .218                 &        .323                 &        .186                 &        .146                 &        .798                 &        .677                 &         .33                 &        .407                 \\
$R^{2}$  &        .848                 &        .744                 &        .433                 &        .644                 &        .541                 &        .298                 &        .188                 &        .845                 &         .29                 &        .199                 &        .623                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/IVlags/Results2shortV1_RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.052$^{\ast\ast\ast}$&      -0.045                 &      -0.137$^{\ast\ast\ast}$&       0.006                 &      -0.568                 &      -0.085                 &      -0.905$^{\ast\ast}$    &       0.422$^{\ast\ast\ast}$&      -0.034                 &      -2.568$^{\ast\ast\ast}$&       1.470$^{\ast\ast\ast}$\\
            &     (0.019)                 &     (0.039)                 &     (0.039)                 &     (0.019)                 &     (0.426)                 &     (0.208)                 &     (0.366)                 &     (0.109)                 &     (0.558)                 &     (0.683)                 &     (0.398)                 \\\addlinespace
$ICT_{c,t}$&      -0.050$^{\ast}$        &      -0.023                 &      -0.143$^{\ast\ast\ast}$&      -0.039                 &      -0.179                 &       0.933                 &      -1.244                 &       0.132                 &       1.755$^{\ast}$        &      -3.850$^{\ast\ast\ast}$&       0.794                 \\
            &     (0.030)                 &     (0.064)                 &     (0.055)                 &     (0.031)                 &     (1.069)                 &     (0.595)                 &     (0.759)                 &     (0.206)                 &     (1.044)                 &     (1.245)                 &     (0.848)                 \\\addlinespace
$R*ICT_{c,t}$&       0.015                 &      -0.018                 &       0.040                 &       0.013                 &      -0.118                 &      -0.160                 &       0.004                 &       0.038                 &       0.013                 &       0.782                 &       0.030                 \\
            &     (0.016)                 &     (0.027)                 &     (0.029)                 &     (0.014)                 &     (0.549)                 &     (0.245)                 &     (0.403)                 &     (0.101)                 &     (0.449)                 &     (0.639)                 &     (0.433)                 \\\addlinespace
$wL_{c,t}$&       0.495$^{\ast\ast\ast}$&       1.444$^{\ast\ast\ast}$&       0.232                 &       0.559$^{\ast\ast\ast}$&      -0.618$^{\ast\ast\ast}$&      -0.155$^{\ast}$        &       0.052                 &      -0.515$^{\ast\ast\ast}$&       0.155                 &       0.597$^{\ast\ast\ast}$&      -0.922$^{\ast\ast\ast}$\\
            &     (0.151)                 &     (0.501)                 &     (0.207)                 &     (0.149)                 &     (0.149)                 &     (0.088)                 &     (0.110)                 &     (0.058)                 &     (0.184)                 &     (0.221)                 &     (0.178)                 \\\addlinespace
$rK_{c,t}$&      -0.053                 &       0.479                 &      -0.190                 &       0.113                 &      -0.889$^{\ast\ast\ast}$&      -0.250$^{\ast\ast\ast}$&      -0.087                 &      -0.552$^{\ast\ast\ast}$&       0.034                 &       0.462$^{\ast\ast}$    &      -0.751$^{\ast\ast\ast}$\\
            &     (0.085)                 &     (0.321)                 &     (0.133)                 &     (0.095)                 &     (0.150)                 &     (0.090)                 &     (0.104)                 &     (0.053)                 &     (0.179)                 &     (0.206)                 &     (0.173)                 \\\addlinespace
$pQ_{c,t}$&       0.540$^{\ast\ast\ast}$&      -0.902                 &       0.868$^{\ast\ast\ast}$&       0.362$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.206)                 &     (0.753)                 &     (0.292)                 &     (0.214)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
Under-F     &        61.5                 &        61.5                 &        61.5                 &        61.5                 &        50.9                 &        50.9                 &        50.9                 &        50.9                 &        50.9                 &        50.9                 &        50.9                 \\
Under-p     &    7.40e-11                 &    7.40e-11                 &    7.40e-11                 &    7.40e-11                 &    9.62e-09                 &    9.62e-09                 &    9.62e-09                 &    9.62e-09                 &    9.62e-09                 &    9.62e-09                 &    9.62e-09                 \\
Weak-CD F   &          24                 &          24                 &          24                 &          24                 &        31.2                 &        31.2                 &        31.2                 &        31.2                 &        31.2                 &        31.2                 &        31.2                 \\
Weak-KP rk F&        14.4                 &        14.4                 &        14.4                 &        14.4                 &        15.9                 &        15.9                 &        15.9                 &        15.9                 &        15.9                 &        15.9                 &        15.9                 \\
Over-Hansen J&        6.72                 &        8.22                 &        4.86                 &        9.16                 &        4.69                 &        9.68                 &        2.09                 &        2.29                 &        11.7                 &        4.69                 &         2.1                 \\
Over-Hansen J p&        .347                 &        .222                 &        .562                 &        .165                 &        .584                 &        .139                 &        .911                 &        .891                 &       .0692                 &        .585                 &        .911                 \\
$R^{2}$  &        .946                 &         .61                 &        .843                 &        .911                 &        .466                 &        .337                 &        .296                 &        .623                 &        .352                 &        .301                 &        .326                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/IVlags/Results2shortV1_RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.025$^{\ast\ast\ast}$&      -0.041$^{\ast\ast\ast}$&      -0.003                 &      -0.014                 &       0.003                 &      -0.275$^{\ast\ast}$    &       0.243                 &       0.035                 &      -0.884$^{\ast\ast\ast}$&       0.460                 &       0.017                 \\
            &     (0.008)                 &     (0.012)                 &     (0.023)                 &     (0.010)                 &     (0.229)                 &     (0.111)                 &     (0.227)                 &     (0.070)                 &     (0.320)                 &     (0.505)                 &     (0.272)                 \\\addlinespace
$ICT_{c,t}$&      -0.074$^{\ast\ast\ast}$&      -0.018                 &      -0.181$^{\ast\ast\ast}$&      -0.073$^{\ast\ast\ast}$&      -1.407$^{\ast\ast}$    &       0.650                 &      -2.318$^{\ast\ast\ast}$&       0.261                 &       2.691$^{\ast\ast}$    &      -4.695$^{\ast\ast\ast}$&       1.892$^{\ast\ast\ast}$\\
            &     (0.017)                 &     (0.062)                 &     (0.041)                 &     (0.028)                 &     (0.701)                 &     (0.547)                 &     (0.522)                 &     (0.198)                 &     (1.064)                 &     (1.243)                 &     (0.619)                 \\\addlinespace
$R*ICT_{c,t}$&       0.027$^{\ast\ast\ast}$&      -0.013                 &       0.075$^{\ast\ast\ast}$&       0.044$^{\ast\ast\ast}$&       0.310                 &      -0.489$^{\ast\ast}$    &       0.805$^{\ast\ast\ast}$&      -0.006                 &      -1.535$^{\ast\ast\ast}$&       1.984$^{\ast\ast\ast}$&      -0.380                 \\
            &     (0.008)                 &     (0.024)                 &     (0.019)                 &     (0.012)                 &     (0.318)                 &     (0.226)                 &     (0.255)                 &     (0.092)                 &     (0.456)                 &     (0.556)                 &     (0.299)                 \\\addlinespace
$wL_{c,t}$&       0.588$^{\ast\ast\ast}$&       0.715$^{\ast\ast\ast}$&       0.645$^{\ast\ast\ast}$&       0.626$^{\ast\ast\ast}$&      -0.465$^{\ast\ast\ast}$&       0.028                 &       0.142                 &      -0.635$^{\ast\ast\ast}$&       0.508$^{\ast\ast\ast}$&       0.875$^{\ast\ast\ast}$&      -1.411$^{\ast\ast\ast}$\\
            &     (0.088)                 &     (0.246)                 &     (0.149)                 &     (0.132)                 &     (0.105)                 &     (0.070)                 &     (0.094)                 &     (0.048)                 &     (0.194)                 &     (0.251)                 &     (0.142)                 \\\addlinespace
$rK_{c,t}$&       0.086                 &       0.286$^{\ast}$        &       0.079                 &       0.059                 &      -0.660$^{\ast\ast\ast}$&      -0.034                 &       0.035                 &      -0.660$^{\ast\ast\ast}$&       0.479$^{\ast\ast\ast}$&       0.753$^{\ast\ast\ast}$&      -1.322$^{\ast\ast\ast}$\\
            &     (0.053)                 &     (0.159)                 &     (0.102)                 &     (0.069)                 &     (0.096)                 &     (0.064)                 &     (0.081)                 &     (0.042)                 &     (0.182)                 &     (0.217)                 &     (0.128)                 \\\addlinespace
$pQ_{c,t}$&       0.214                 &      -0.085                 &       0.162                 &       0.247                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.136)                 &     (0.363)                 &     (0.220)                 &     (0.184)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
Under-F     &        30.9                 &        30.9                 &        30.9                 &        30.9                 &        30.6                 &        30.6                 &        30.6                 &        30.6                 &        30.6                 &        30.6                 &        30.6                 \\
Under-p     &    .0000647                 &    .0000647                 &    .0000647                 &    .0000647                 &    .0000723                 &    .0000723                 &    .0000723                 &    .0000723                 &    .0000723                 &    .0000723                 &    .0000723                 \\
Weak-CD F   &        65.8                 &        65.8                 &        65.8                 &        65.8                 &        64.2                 &        64.2                 &        64.2                 &        64.2                 &        64.2                 &        64.2                 &        64.2                 \\
Weak-KP rk F&        17.5                 &        17.5                 &        17.5                 &        17.5                 &        17.3                 &        17.3                 &        17.3                 &        17.3                 &        17.3                 &        17.3                 &        17.3                 \\
Over-Hansen J&          12                 &        2.01                 &         5.8                 &        9.77                 &        4.09                 &        2.24                 &         4.5                 &        7.01                 &        2.29                 &        4.08                 &        5.27                 \\
Over-Hansen J p&       .0611                 &        .919                 &        .446                 &        .135                 &        .665                 &        .896                 &         .61                 &        .319                 &        .891                 &        .666                 &        .509                 \\
%$R^{2}$  &        .938                 &        .714                 &        .681                 &        .871                 &        .502                 &        .215                 &        .262                 &        .763                 &        .365                 &        .153                 &        .411                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/IVlags/Results3RICTint_cit_All_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{i,c,t}$&      -0.037                 &       0.020$^{\ast}$        &      -0.057$^{\ast\ast\ast}$&      -0.039                 &      -0.005$^{\ast}$        &      -0.022                 \\
            &     (0.023)                 &     (0.010)                 &     (0.019)                 &     (0.064)                 &     (0.003)                 &     (0.018)                 \\\addlinespace
$ICT_{i,c,t}$&      -0.028                 &       0.015                 &      -0.043$^{\ast}$        &      -0.058                 &      -0.015$^{\ast\ast}$    &      -0.041                 \\
            &     (0.023)                 &     (0.011)                 &     (0.022)                 &     (0.068)                 &     (0.006)                 &     (0.050)                 \\\addlinespace
$R*ICT_{i,c,t}$&      -0.015$^{\ast}$        &       0.001                 &      -0.016$^{\ast\ast}$    &       0.041$^{\ast\ast}$    &      -0.004$^{\ast\ast}$    &       0.013                 \\
            &     (0.008)                 &     (0.003)                 &     (0.007)                 &     (0.020)                 &     (0.001)                 &     (0.009)                 \\\midrule
Under-F     &        46.8                 &        46.8                 &        46.8                 &        46.8                 &        46.8                 &        46.8                 \\
Under-p     &    6.05e-08                 &    6.05e-08                 &    6.05e-08                 &    6.15e-08                 &    6.13e-08                 &    6.13e-08                 \\
Weak-CD F   &         309                 &         309                 &         309                 &         305                 &         302                 &         302                 \\
Weak-KP rk F&        24.8                 &        24.8                 &        24.8                 &        24.7                 &        24.8                 &        24.8                 \\
Over-Hansen J&        5.41                 &        13.8                 &        7.36                 &          12                 &        12.2                 &        2.69                 \\
Over-Hansen J p&        .493                 &       .0324                 &        .289                 &       .0625                 &        .057                 &        .847                 \\
$R^{2}$  &      .00916                 &       .0017                 &       .0177                 &      .00194                 &      .00246                 &       .0071                 \\
$N$      &        2070                 &        2070                 &        2070                 &        2052                 &        2025                 &        2025                 \\


==> inputs/robustness/IVlags/Results3RICTint_cit_All_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{i,c,t}$&       0.003                 &       0.016$^{\ast\ast\ast}$&      -0.013                 &       0.007                 &       0.001                 &       0.027$^{\ast\ast}$    \\
            &     (0.016)                 &     (0.005)                 &     (0.015)                 &     (0.035)                 &     (0.003)                 &     (0.012)                 \\\addlinespace
$ICT_{i,c,t}$&       0.029$^{\ast\ast\ast}$&       0.005                 &       0.025$^{\ast\ast\ast}$&       0.002                 &       0.003                 &       0.027$^{\ast\ast\ast}$\\
            &     (0.006)                 &     (0.004)                 &     (0.006)                 &     (0.016)                 &     (0.005)                 &     (0.009)                 \\\addlinespace
$R*ICT_{i,c,t}$&       0.003                 &       0.001                 &       0.002                 &      -0.004                 &      -0.000                 &       0.007$^{\ast\ast}$    \\
            &     (0.003)                 &     (0.001)                 &     (0.003)                 &     (0.009)                 &     (0.001)                 &     (0.003)                 \\\midrule
Under-F     &         117                 &         117                 &         117                 &         115                 &         117                 &         117                 \\
Under-p     &    3.80e-22                 &    3.80e-22                 &    3.80e-22                 &    7.48e-22                 &    2.98e-22                 &    2.98e-22                 \\
Weak-CD F   &         904                 &         904                 &         904                 &         890                 &         890                 &         890                 \\
Weak-KP rk F&        64.5                 &        64.5                 &        64.5                 &        63.7                 &        64.7                 &        64.7                 \\
Over-Hansen J&        6.08                 &        6.06                 &        10.9                 &        2.35                 &        9.53                 &        6.98                 \\
Over-Hansen J p&        .415                 &        .417                 &       .0921                 &        .884                 &        .146                 &        .322                 \\
$R^{2}$  &      .00713                 &      .00209                 &      .00912                 &    .0000155                 &   -.0000941                 &       .0139                 \\
$N$      &        2827                 &        2827                 &        2827                 &        2790                 &        2777                 &        2777                 \\


==> inputs/robustness/IVlags/Results3RICTint_cit_All_95t16.tex <==
& ln $wL_{i,c,t}$ & ln $w_{i,c,t}$ & ln $L_{i,c,t}$ & ln $rK_{i,c,t}$ & ln $r_{i,c,t}$ & ln $K_{i,c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{i,c,t}$&      -0.026$^{\ast}$        &       0.029$^{\ast\ast\ast}$&      -0.055$^{\ast\ast\ast}$&      -0.055$^{\ast\ast}$    &      -0.010$^{\ast\ast\ast}$&       0.015                 \\
            &     (0.014)                 &     (0.005)                 &     (0.013)                 &     (0.025)                 &     (0.003)                 &     (0.012)                 \\\addlinespace
$ICT_{i,c,t}$&       0.021$^{\ast\ast\ast}$&       0.005$^{\ast\ast}$    &       0.017$^{\ast\ast\ast}$&       0.028$^{\ast\ast\ast}$&      -0.001                 &       0.027$^{\ast\ast\ast}$\\
            &     (0.004)                 &     (0.002)                 &     (0.004)                 &     (0.011)                 &     (0.003)                 &     (0.007)                 \\\addlinespace
$R*ICT_{i,c,t}$&      -0.006$^{\ast\ast\ast}$&       0.005$^{\ast\ast\ast}$&      -0.012$^{\ast\ast\ast}$&       0.004                 &      -0.004$^{\ast\ast\ast}$&       0.007$^{\ast\ast}$    \\
            &     (0.002)                 &     (0.001)                 &     (0.002)                 &     (0.006)                 &     (0.001)                 &     (0.003)                 \\\midrule
Under-F     &         166                 &         166                 &         166                 &         167                 &         166                 &         166                 \\
Under-p     &    1.43e-32                 &    1.43e-32                 &    1.43e-32                 &    1.24e-32                 &    1.41e-32                 &    1.41e-32                 \\
Weak-CD F   &        2314                 &        2314                 &        2314                 &        2288                 &        2274                 &        2274                 \\
Weak-KP rk F&         159                 &         159                 &         159                 &         158                 &         159                 &         159                 \\
Over-Hansen J&        4.62                 &         7.7                 &        3.53                 &        6.99                 &         4.3                 &        7.28                 \\
Over-Hansen J p&        .594                 &        .261                 &         .74                 &        .322                 &        .637                 &        .296                 \\
%$R^{2}$  &      .00929                 &      .00612                 &       .0211                 &      .00202                 &      .00475                 &       .0105                 \\
$N$      &        4898                 &        4898                 &        4898                 &        4843                 &        4803                 &        4803                 \\


==> inputs/robustness/IVlags/Results4RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.045$^{\ast\ast}$    &       0.017                 &      -0.047$^{\ast\ast}$    &      -0.010                 &       0.016$^{\ast\ast\ast}$&      -1.911$^{\ast\ast\ast}$&       0.006                 &       0.013$^{\ast\ast\ast}$\\
            &     (0.019)                 &     (0.017)                 &     (0.020)                 &     (0.022)                 &     (0.004)                 &     (0.581)                 &     (0.004)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.000                 &       0.004                 &       0.007                 &       0.118$^{\ast}$        &      -0.007                 &       1.614                 &       0.007                 &       0.001                 \\
            &     (0.040)                 &     (0.050)                 &     (0.057)                 &     (0.068)                 &     (0.007)                 &     (1.292)                 &     (0.007)                 &     (0.009)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.034                 &       0.001                 &      -0.022                 &      -0.055                 &       0.002                 &      -0.199                 &      -0.004                 &       0.013$^{\ast\ast\ast}$\\
            &     (0.021)                 &     (0.025)                 &     (0.026)                 &     (0.038)                 &     (0.004)                 &     (0.706)                 &     (0.004)                 &     (0.005)                 \\\midrule
Under-F     &        11.4                 &        11.4                 &        11.4                 &        11.4                 &        11.4                 &        11.4                 &        11.4                 &        11.4                 \\
Under-p     &       .0221                 &       .0221                 &       .0221                 &       .0221                 &       .0221                 &       .0221                 &       .0221                 &       .0221                 \\
Weak-CD F   &          18                 &          18                 &          18                 &          18                 &          18                 &          18                 &          18                 &          18                 \\
Weak-KP rk F&        23.9                 &        23.9                 &        23.9                 &        23.9                 &        23.9                 &        23.9                 &        23.9                 &        23.9                 \\
Over-Hansen J&         3.7                 &           5                 &        13.1                 &        5.07                 &        3.23                 &        3.07                 &        6.48                 &        5.19                 \\
Over-Hansen J p&        .295                 &        .172                 &      .00436                 &        .167                 &        .357                 &        .381                 &       .0905                 &        .159                 \\
$R^{2}$  &        .535                 &        .556                 &        .482                 &        .619                 &        .568                 &        .588                 &        .101                 &        .329                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/IVlags/Results4RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.162$^{\ast\ast\ast}$&      -0.059$^{\ast\ast\ast}$&      -0.110$^{\ast\ast\ast}$&      -0.083$^{\ast\ast\ast}$&       0.000                 &      -1.369$^{\ast\ast\ast}$&      -0.011$^{\ast\ast}$    &       0.012$^{\ast}$        \\
            &     (0.027)                 &     (0.014)                 &     (0.019)                 &     (0.017)                 &     (0.003)                 &     (0.347)                 &     (0.004)                 &     (0.007)                 \\\addlinespace
$ICT_{c,t}$&       0.328$^{\ast\ast\ast}$&      -0.176$^{\ast\ast\ast}$&       0.137$^{\ast\ast\ast}$&      -0.058$^{\ast\ast}$    &       0.016$^{\ast\ast\ast}$&      -2.818$^{\ast\ast\ast}$&      -0.001                 &       0.029$^{\ast\ast}$    \\
            &     (0.039)                 &     (0.028)                 &     (0.038)                 &     (0.025)                 &     (0.005)                 &     (0.765)                 &     (0.008)                 &     (0.014)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.153$^{\ast\ast\ast}$&       0.059$^{\ast\ast\ast}$&      -0.061$^{\ast\ast\ast}$&       0.025$^{\ast}$        &      -0.008$^{\ast\ast\ast}$&       1.341$^{\ast\ast\ast}$&      -0.004                 &      -0.011                 \\
            &     (0.023)                 &     (0.015)                 &     (0.019)                 &     (0.013)                 &     (0.002)                 &     (0.421)                 &     (0.004)                 &     (0.007)                 \\\midrule
Under-F     &        31.6                 &        31.6                 &        31.6                 &        31.6                 &        31.6                 &        31.6                 &        31.6                 &        31.6                 \\
Under-p     &    2.35e-06                 &    2.35e-06                 &    2.35e-06                 &    2.35e-06                 &    2.35e-06                 &    2.35e-06                 &    2.35e-06                 &    2.35e-06                 \\
Weak-CD F   &        46.9                 &        46.9                 &        46.9                 &        46.9                 &        46.9                 &        46.9                 &        46.9                 &        46.9                 \\
Weak-KP rk F&        32.7                 &        32.7                 &        32.7                 &        32.7                 &        32.7                 &        32.7                 &        32.7                 &        32.7                 \\
Over-Hansen J&        4.39                 &        4.39                 &        3.08                 &        3.68                 &        3.76                 &        6.15                 &        .715                 &        1.62                 \\
Over-Hansen J p&        .223                 &        .223                 &        .379                 &        .298                 &        .288                 &        .104                 &         .87                 &        .655                 \\
$R^{2}$  &        .732                 &        .624                 &        .533                 &        .651                 &        .303                 &        .376                 &        .417                 &        .263                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/IVlags/Results4RICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.156$^{\ast\ast\ast}$&      -0.014                 &      -0.097$^{\ast\ast\ast}$&      -0.074$^{\ast\ast\ast}$&       0.001                 &      -0.818$^{\ast\ast\ast}$&      -0.001                 &       0.031$^{\ast\ast\ast}$\\
            &     (0.022)                 &     (0.009)                 &     (0.015)                 &     (0.015)                 &     (0.002)                 &     (0.230)                 &     (0.003)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.235$^{\ast\ast\ast}$&      -0.140$^{\ast\ast\ast}$&       0.089$^{\ast\ast}$    &      -0.030                 &       0.003                 &      -0.681                 &      -0.001                 &       0.041$^{\ast\ast\ast}$\\
            &     (0.079)                 &     (0.023)                 &     (0.037)                 &     (0.038)                 &     (0.006)                 &     (0.764)                 &     (0.007)                 &     (0.009)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.106$^{\ast\ast}$    &       0.056$^{\ast\ast\ast}$&      -0.036$^{\ast\ast}$    &       0.007                 &      -0.002                 &       0.766$^{\ast}$        &       0.002                 &      -0.009$^{\ast\ast}$    \\
            &     (0.043)                 &     (0.012)                 &     (0.018)                 &     (0.020)                 &     (0.003)                 &     (0.403)                 &     (0.003)                 &     (0.004)                 \\\midrule
Under-F     &        15.8                 &        15.8                 &        15.8                 &        15.8                 &        15.8                 &        15.8                 &        15.8                 &        15.8                 \\
Under-p     &      .00335                 &      .00335                 &      .00335                 &      .00335                 &      .00335                 &      .00335                 &      .00335                 &      .00335                 \\
Weak-CD F   &        96.9                 &        96.9                 &        96.9                 &        96.9                 &        96.9                 &        96.9                 &        96.9                 &        96.9                 \\
Weak-KP rk F&        9.35                 &        9.35                 &        9.35                 &        9.35                 &        9.35                 &        9.35                 &        9.35                 &        9.35                 \\
Over-Hansen J&        13.4                 &        9.15                 &         2.6                 &        8.84                 &        11.2                 &        12.1                 &        7.08                 &        2.13                 \\
Over-Hansen J p&      .00387                 &       .0273                 &        .457                 &       .0315                 &       .0109                 &      .00716                 &       .0695                 &        .547                 \\
$R^{2}$  &        .624                 &        .421                 &        .542                 &        .472                 &        .254                 &        .505                 &        .151                 &        .292                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/IVlags/Results4shortRICTint_ct_All_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.047$^{\ast\ast}$    &       0.016                 &      -0.044$^{\ast\ast}$    &      -0.014                 &      -1.842$^{\ast\ast\ast}$&       0.013$^{\ast\ast\ast}$\\
            &     (0.019)                 &     (0.016)                 &     (0.019)                 &     (0.022)                 &     (0.586)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.000                 &       0.004                 &       0.009                 &       0.113$^{\ast}$        &       1.790                 &      -0.000                 \\
            &     (0.038)                 &     (0.049)                 &     (0.056)                 &     (0.068)                 &     (1.306)                 &     (0.008)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.033                 &       0.001                 &      -0.023                 &      -0.053                 &      -0.227                 &       0.013$^{\ast\ast\ast}$\\
            &     (0.021)                 &     (0.025)                 &     (0.025)                 &     (0.038)                 &     (0.714)                 &     (0.005)                 \\\midrule
Under-F     &        12.3                 &        12.3                 &        12.3                 &        12.3                 &        12.3                 &        12.3                 \\
Under-p     &       .0924                 &       .0924                 &       .0924                 &       .0924                 &       .0924                 &       .0924                 \\
Weak-CD F   &        12.1                 &        12.1                 &        12.1                 &        12.1                 &        12.1                 &        12.1                 \\
Weak-KP rk F&        22.1                 &        22.1                 &        22.1                 &        22.1                 &        22.1                 &        22.1                 \\
Over-Hansen J&        4.95                 &        7.63                 &        13.9                 &        6.24                 &        5.29                 &         6.5                 \\
Over-Hansen J p&         .55                 &        .267                 &       .0312                 &        .397                 &        .507                 &         .37                 \\
$R^{2}$  &        .535                 &        .556                 &        .483                 &        .619                 &        .589                 &        .329                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/IVlags/Results4shortRICTint_ct_All_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.163$^{\ast\ast\ast}$&      -0.060$^{\ast\ast\ast}$&      -0.109$^{\ast\ast\ast}$&      -0.085$^{\ast\ast\ast}$&      -1.384$^{\ast\ast\ast}$&       0.009                 \\
            &     (0.027)                 &     (0.013)                 &     (0.019)                 &     (0.017)                 &     (0.345)                 &     (0.007)                 \\\addlinespace
$ICT_{c,t}$&       0.330$^{\ast\ast\ast}$&      -0.172$^{\ast\ast\ast}$&       0.149$^{\ast\ast\ast}$&      -0.055$^{\ast\ast}$    &      -2.873$^{\ast\ast\ast}$&       0.023$^{\ast}$        \\
            &     (0.037)                 &     (0.027)                 &     (0.038)                 &     (0.023)                 &     (0.729)                 &     (0.013)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.154$^{\ast\ast\ast}$&       0.057$^{\ast\ast\ast}$&      -0.066$^{\ast\ast\ast}$&       0.024$^{\ast\ast}$    &       1.355$^{\ast\ast\ast}$&      -0.008                 \\
            &     (0.022)                 &     (0.014)                 &     (0.019)                 &     (0.012)                 &     (0.400)                 &     (0.007)                 \\\midrule
Under-F     &        45.4                 &        45.4                 &        45.4                 &        45.4                 &        45.4                 &        45.4                 \\
Under-p     &    1.14e-07                 &    1.14e-07                 &    1.14e-07                 &    1.14e-07                 &    1.14e-07                 &    1.14e-07                 \\
Weak-CD F   &        39.4                 &        39.4                 &        39.4                 &        39.4                 &        39.4                 &        39.4                 \\
Weak-KP rk F&        25.1                 &        25.1                 &        25.1                 &        25.1                 &        25.1                 &        25.1                 \\
Over-Hansen J&        5.53                 &        5.77                 &        7.24                 &        7.21                 &        10.2                 &        4.96                 \\
Over-Hansen J p&        .478                 &        .449                 &        .299                 &        .302                 &        .117                 &        .549                 \\
$R^{2}$  &        .731                 &        .625                 &        .533                 &         .65                 &        .375                 &        .265                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/IVlags/Results4shortRICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $Services_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.155$^{\ast\ast\ast}$&      -0.014                 &      -0.096$^{\ast\ast\ast}$&      -0.076$^{\ast\ast\ast}$&      -0.842$^{\ast\ast\ast}$&       0.030$^{\ast\ast\ast}$\\
            &     (0.022)                 &     (0.009)                 &     (0.015)                 &     (0.015)                 &     (0.234)                 &     (0.004)                 \\\addlinespace
$ICT_{c,t}$&       0.234$^{\ast\ast\ast}$&      -0.139$^{\ast\ast\ast}$&       0.090$^{\ast\ast}$    &      -0.025                 &      -0.771                 &       0.039$^{\ast\ast\ast}$\\
            &     (0.078)                 &     (0.023)                 &     (0.036)                 &     (0.038)                 &     (0.750)                 &     (0.009)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.105$^{\ast\ast}$    &       0.056$^{\ast\ast\ast}$&      -0.037$^{\ast\ast}$    &       0.005                 &       0.802$^{\ast\ast}$    &      -0.008$^{\ast}$        \\
            &     (0.043)                 &     (0.012)                 &     (0.017)                 &     (0.020)                 &     (0.401)                 &     (0.004)                 \\\midrule
Under-F     &        26.4                 &        26.4                 &        26.4                 &        26.4                 &        26.4                 &        26.4                 \\
Under-p     &      .00043                 &      .00043                 &      .00043                 &      .00043                 &      .00043                 &      .00043                 \\
Weak-CD F   &          69                 &          69                 &          69                 &          69                 &          69                 &          69                 \\
Weak-KP rk F&        17.9                 &        17.9                 &        17.9                 &        17.9                 &        17.9                 &        17.9                 \\
Over-Hansen J&        15.4                 &        15.6                 &        3.98                 &        21.3                 &        23.7                 &        8.37                 \\
Over-Hansen J p&       .0174                 &       .0158                 &        .679                 &      .00163                 &     .000604                 &        .212                 \\
%$R^{2}$  &        .624                 &        .421                 &        .542                 &        .472                 &        .504                 &        .292                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/IVlags/Results5RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.020                 &      -0.027                 &      -0.030                 &      -0.016                 &       0.061$^{\ast\ast\ast}$&      -0.033$^{\ast\ast\ast}$&       0.019                 &       0.001                 \\
            &     (0.031)                 &     (0.043)                 &     (0.024)                 &     (0.023)                 &     (0.020)                 &     (0.011)                 &     (0.017)                 &     (0.008)                 \\\addlinespace
$ICT_{c,t}$&       0.011                 &       0.147$^{\ast}$        &       0.071                 &       0.068                 &       0.037                 &       0.018                 &       0.016                 &       0.013                 \\
            &     (0.085)                 &     (0.082)                 &     (0.079)                 &     (0.077)                 &     (0.043)                 &     (0.030)                 &     (0.028)                 &     (0.017)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.024                 &      -0.071                 &      -0.051                 &      -0.062                 &      -0.026                 &      -0.023                 &      -0.024                 &       0.002                 \\
            &     (0.042)                 &     (0.054)                 &     (0.041)                 &     (0.038)                 &     (0.025)                 &     (0.015)                 &     (0.017)                 &     (0.010)                 \\\midrule
Under-F     &        11.2                 &        11.2                 &        11.2                 &        11.2                 &        10.3                 &        10.3                 &        10.3                 &        10.3                 \\
Under-p     &       .0244                 &       .0244                 &       .0244                 &       .0244                 &       .0363                 &       .0363                 &       .0363                 &       .0363                 \\
Weak-CD F   &          18                 &          18                 &          18                 &          18                 &        12.4                 &        12.4                 &        12.4                 &        12.4                 \\
Weak-KP rk F&        24.4                 &        24.4                 &        24.4                 &        24.4                 &        22.3                 &        22.3                 &        22.3                 &        22.3                 \\
Over-Hansen J&        3.25                 &        1.14                 &        3.86                 &         5.8                 &        7.47                 &        10.5                 &        6.39                 &        4.78                 \\
Over-Hansen J p&        .355                 &        .767                 &        .277                 &        .122                 &       .0585                 &       .0149                 &        .094                 &        .189                 \\
$R^{2}$  &        .538                 &        .618                 &        .677                 &        .714                 &        .736                 &        .465                 &        .464                 &        .333                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         135                 &         135                 &         135                 &         135                 \\


==> inputs/robustness/IVlags/Results5RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.229$^{\ast\ast\ast}$&      -0.201$^{\ast\ast\ast}$&      -0.222$^{\ast\ast\ast}$&      -0.175$^{\ast\ast\ast}$&      -0.070$^{\ast\ast\ast}$&      -0.116$^{\ast\ast\ast}$&      -0.022$^{\ast}$        &       0.010                 \\
            &     (0.029)                 &     (0.036)                 &     (0.030)                 &     (0.029)                 &     (0.012)                 &     (0.018)                 &     (0.012)                 &     (0.010)                 \\\addlinespace
$ICT_{c,t}$&       0.118$^{\ast\ast}$    &      -0.049                 &       0.050                 &       0.094                 &       0.009                 &       0.033                 &       0.157$^{\ast\ast\ast}$&      -0.092$^{\ast\ast\ast}$\\
            &     (0.058)                 &     (0.065)                 &     (0.059)                 &     (0.060)                 &     (0.025)                 &     (0.042)                 &     (0.023)                 &     (0.024)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.068$^{\ast\ast}$    &      -0.037                 &      -0.053$^{\ast}$        &      -0.082$^{\ast\ast\ast}$&      -0.007                 &      -0.028                 &      -0.070$^{\ast\ast\ast}$&       0.059$^{\ast\ast\ast}$\\
            &     (0.030)                 &     (0.033)                 &     (0.030)                 &     (0.030)                 &     (0.015)                 &     (0.023)                 &     (0.015)                 &     (0.013)                 \\\midrule
Under-F     &        32.2                 &        32.2                 &        32.2                 &        32.2                 &        33.7                 &        33.7                 &        33.7                 &        33.7                 \\
Under-p     &    1.77e-06                 &    1.77e-06                 &    1.77e-06                 &    1.77e-06                 &    8.42e-07                 &    8.42e-07                 &    8.42e-07                 &    8.42e-07                 \\
Weak-CD F   &        49.6                 &        49.6                 &        49.6                 &        49.6                 &          35                 &          35                 &          35                 &          35                 \\
Weak-KP rk F&        38.3                 &        38.3                 &        38.3                 &        38.3                 &        30.4                 &        30.4                 &        30.4                 &        30.4                 \\
Over-Hansen J&        6.38                 &        4.51                 &        5.18                 &        4.79                 &        5.54                 &        2.04                 &         3.7                 &         4.5                 \\
Over-Hansen J p&       .0943                 &        .211                 &        .159                 &        .188                 &        .136                 &        .564                 &        .296                 &        .213                 \\
$R^{2}$  &        .632                 &        .503                 &        .611                 &        .578                 &          .6                 &        .637                 &        .738                 &        .532                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         174                 &         174                 &         174                 &         174                 \\


==> inputs/robustness/IVlags/Results5RICTint_ct_All_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.167$^{\ast\ast\ast}$&      -0.168$^{\ast\ast\ast}$&      -0.175$^{\ast\ast\ast}$&      -0.148$^{\ast\ast\ast}$&      -0.017                 &      -0.111$^{\ast\ast\ast}$&      -0.025$^{\ast}$        &      -0.001                 \\
            &     (0.023)                 &     (0.028)                 &     (0.024)                 &     (0.022)                 &     (0.014)                 &     (0.016)                 &     (0.013)                 &     (0.007)                 \\\addlinespace
$ICT_{c,t}$&       0.088                 &      -0.115                 &       0.007                 &       0.016                 &       0.031                 &       0.002                 &       0.127$^{\ast\ast\ast}$&      -0.054$^{\ast\ast}$    \\
            &     (0.074)                 &     (0.070)                 &     (0.069)                 &     (0.072)                 &     (0.032)                 &     (0.042)                 &     (0.036)                 &     (0.025)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.044                 &       0.028                 &      -0.016                 &      -0.027                 &      -0.022                 &       0.004                 &      -0.068$^{\ast\ast\ast}$&       0.032$^{\ast\ast}$    \\
            &     (0.041)                 &     (0.034)                 &     (0.037)                 &     (0.038)                 &     (0.022)                 &     (0.023)                 &     (0.024)                 &     (0.013)                 \\\midrule
Under-F     &        15.8                 &        15.8                 &        15.8                 &        15.8                 &          19                 &          19                 &          19                 &          19                 \\
Under-p     &      .00337                 &      .00337                 &      .00337                 &      .00337                 &       .0008                 &       .0008                 &       .0008                 &       .0008                 \\
Weak-CD F   &        97.2                 &        97.2                 &        97.2                 &        97.2                 &          72                 &          72                 &          72                 &          72                 \\
Weak-KP rk F&        9.42                 &        9.42                 &        9.42                 &        9.42                 &        9.21                 &        9.21                 &        9.21                 &        9.21                 \\
Over-Hansen J&        17.7                 &        15.8                 &          18                 &        18.6                 &        20.7                 &        10.8                 &        16.6                 &        3.52                 \\
Over-Hansen J p&     .000513                 &      .00123                 &      .00044                 &     .000324                 &     .000123                 &       .0127                 &     .000862                 &        .318                 \\
%$R^{2}$  &        .521                 &        .403                 &        .489                 &        .517                 &        .571                 &        .589                 &        .638                 &        .372                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         309                 &         309                 &         309                 &         309                 \\


==> inputs/robustness/TaxProgressiveness/Results2RICTint_EUKLEMS_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.011                 &       0.009                 &       0.018                 &      -0.055                 &       0.182                 &       0.236                 &       0.171                 &      -0.226                 &       0.489                 &       0.451                 &      -0.920                 \\
            &     (0.022)                 &     (0.027)                 &     (0.058)                 &     (0.030)                 &     (0.789)                 &     (0.465)                 &     (0.565)                 &     (0.240)                 &     (0.780)                 &     (0.997)                 &     (0.801)                 \\\addlinespace
$ICT_{c,t}$&       0.027                 &       0.013                 &       0.056                 &       0.026                 &       0.668$^{\ast}$        &      -0.269                 &       0.649$^{\ast}$        &       0.287$^{\ast\ast}$    &      -1.887                 &       1.397                 &       0.476                 \\
            &     (0.033)                 &     (0.062)                 &     (0.042)                 &     (0.056)                 &     (0.352)                 &     (0.670)                 &     (0.310)                 &     (0.104)                 &     (1.330)                 &     (1.112)                 &     (0.635)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.019                 &      -0.017                 &      -0.013                 &      -0.030                 &      -0.227                 &      -0.125                 &       0.039                 &      -0.141                 &       0.429                 &      -0.242                 &      -0.216                 \\
            &     (0.024)                 &     (0.035)                 &     (0.036)                 &     (0.034)                 &     (0.613)                 &     (0.418)                 &     (0.524)                 &     (0.103)                 &     (0.524)                 &     (0.732)                 &     (0.588)                 \\\addlinespace
$wL_{c,t}$&       0.400$^{\ast\ast\ast}$&       0.353$^{\ast}$        &       0.530                 &       0.368$^{\ast\ast\ast}$&      -0.614$^{\ast\ast}$    &       0.005                 &       0.172                 &      -0.792$^{\ast\ast\ast}$&       0.580                 &       1.320$^{\ast}$        &      -1.885$^{\ast\ast\ast}$\\
            &     (0.085)                 &     (0.181)                 &     (0.291)                 &     (0.092)                 &     (0.190)                 &     (0.064)                 &     (0.238)                 &     (0.082)                 &     (0.373)                 &     (0.592)                 &     (0.332)                 \\\addlinespace
$rK_{c,t}$&       0.017                 &       0.225                 &       0.146                 &      -0.240$^{\ast\ast}$    &      -0.680$^{\ast\ast\ast}$&      -0.016                 &       0.129                 &      -0.794$^{\ast\ast\ast}$&       0.607$^{\ast}$        &       1.212$^{\ast\ast}$    &      -1.808$^{\ast\ast\ast}$\\
            &     (0.067)                 &     (0.122)                 &     (0.172)                 &     (0.072)                 &     (0.158)                 &     (0.043)                 &     (0.190)                 &     (0.087)                 &     (0.298)                 &     (0.446)                 &     (0.304)                 \\\addlinespace
$pQ_{c,t}$&       0.219                 &       0.075                 &       0.249                 &       0.266$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.138)                 &     (0.326)                 &     (0.345)                 &     (0.127)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.000                 &      -0.003                 &       0.000                 &       0.004$^{\ast\ast}$    &      -0.082                 &      -0.049                 &      -0.021                 &      -0.012                 &      -0.082                 &       0.051                 &       0.028                 \\
            &     (0.001)                 &     (0.003)                 &     (0.004)                 &     (0.002)                 &     (0.067)                 &     (0.031)                 &     (0.035)                 &     (0.007)                 &     (0.059)                 &     (0.084)                 &     (0.056)                 \\\addlinespace
$Services_{c,t}$&       0.000                 &       0.018$^{\ast\ast}$    &       0.011                 &      -0.020$^{\ast\ast}$    &       0.214                 &       0.128$^{\ast}$        &       0.108                 &      -0.021                 &       0.206                 &       0.033                 &      -0.252                 \\
            &     (0.005)                 &     (0.006)                 &     (0.012)                 &     (0.008)                 &     (0.185)                 &     (0.068)                 &     (0.145)                 &     (0.046)                 &     (0.223)                 &     (0.270)                 &     (0.147)                 \\\addlinespace
$HHI_{c,t}$&      -0.568                 &       1.283                 &       0.727                 &      -3.433$^{\ast\ast}$    &      21.543                 &      11.839                 &       4.915                 &       4.789                 &       5.550                 &      -4.734                 &      -3.019                 \\
            &     (0.557)                 &     (0.984)                 &     (1.627)                 &     (1.234)                 &    (22.088)                 &    (12.163)                 &    (15.181)                 &     (9.764)                 &    (28.211)                 &    (38.514)                 &    (32.725)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast\ast}$    &       0.001                 &      -0.001                 &       0.044$^{\ast\ast}$    &      -0.003                 &       0.021                 &       0.026$^{\ast\ast\ast}$&      -0.040                 &       0.020                 &       0.023                 \\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.001)                 &     (0.015)                 &     (0.009)                 &     (0.013)                 &     (0.007)                 &     (0.023)                 &     (0.027)                 &     (0.015)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.015$^{\ast}$        &       0.017$^{\ast}$        &      -0.025                 &       0.044$^{\ast\ast\ast}$&      -0.707$^{\ast}$        &      -0.112                 &      -0.251                 &      -0.344$^{\ast\ast}$    &       0.398$^{\ast}$        &      -0.143                 &      -0.296                 \\
            &     (0.008)                 &     (0.008)                 &     (0.032)                 &     (0.011)                 &     (0.326)                 &     (0.112)                 &     (0.196)                 &     (0.136)                 &     (0.207)                 &     (0.379)                 &     (0.405)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003$^{\ast}$        &       0.002                 &       0.006                 &       0.000                 &       0.082                 &       0.017                 &       0.057                 &       0.008                 &      -0.024                 &       0.088                 &      -0.073                 \\
            &     (0.001)                 &     (0.002)                 &     (0.003)                 &     (0.002)                 &     (0.049)                 &     (0.018)                 &     (0.036)                 &     (0.011)                 &     (0.038)                 &     (0.058)                 &     (0.045)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.005                 &       0.022$^{\ast}$        &      -0.000                 &      -0.004                 &       0.147                 &       0.099                 &       0.115                 &      -0.067                 &       0.324                 &       0.009                 &      -0.318                 \\
            &     (0.006)                 &     (0.011)                 &     (0.018)                 &     (0.009)                 &     (0.209)                 &     (0.089)                 &     (0.174)                 &     (0.049)                 &     (0.280)                 &     (0.301)                 &     (0.249)                 \\\addlinespace
$Gini^{w}_{c,t}$&      -0.537                 &       0.528                 &      -2.051                 &      -0.507                 &     -12.162                 &       7.944                 &     -20.840                 &       0.735                 &      32.091                 &     -53.621$^{\ast}$        &      20.293                 \\
            &     (0.392)                 &     (0.719)                 &     (1.460)                 &     (0.337)                 &    (13.472)                 &     (8.613)                 &    (12.652)                 &     (3.204)                 &    (19.997)                 &    (28.792)                 &    (19.304)                 \\\addlinespace
$XRate_{c,t}$&       0.007                 &      -0.000                 &       0.009                 &       0.018$^{\ast}$        &       0.020                 &      -0.031                 &       0.031                 &       0.020                 &      -0.202                 &       0.206                 &      -0.010                 \\
            &     (0.007)                 &     (0.010)                 &     (0.014)                 &     (0.008)                 &     (0.252)                 &     (0.118)                 &     (0.228)                 &     (0.052)                 &     (0.199)                 &     (0.324)                 &     (0.210)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .986                 &        .994                 &        .989                 &        .984                 &        .992                 &         .99                 &        .983                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/TaxProgressiveness/Results2RICTint_EUKLEMS_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.040$^{\ast}$        &      -0.074                 &      -0.108$^{\ast\ast\ast}$&       0.019                 &      -0.698                 &      -0.219                 &      -0.852$^{\ast\ast}$    &       0.373$^{\ast\ast}$    &      -0.102                 &      -2.037$^{\ast\ast}$    &       1.340$^{\ast\ast}$    \\
            &     (0.020)                 &     (0.051)                 &     (0.030)                 &     (0.031)                 &     (0.393)                 &     (0.193)                 &     (0.382)                 &     (0.133)                 &     (0.482)                 &     (0.783)                 &     (0.479)                 \\\addlinespace
$ICT_{c,t}$&      -0.033                 &      -0.077                 &      -0.085$^{\ast}$        &      -0.011                 &      -0.519                 &       0.411                 &      -1.042$^{\ast}$        &       0.112                 &       1.051                 &      -2.221$^{\ast}$        &       0.549                 \\
            &     (0.019)                 &     (0.068)                 &     (0.041)                 &     (0.021)                 &     (0.539)                 &     (0.395)                 &     (0.503)                 &     (0.143)                 &     (0.844)                 &     (1.051)                 &     (0.744)                 \\\addlinespace
$R*ICT_{c,t}$&       0.010                 &       0.019                 &       0.023                 &       0.001                 &       0.013                 &      -0.002                 &      -0.027                 &       0.043                 &       0.198                 &       0.198                 &       0.117                 \\
            &     (0.016)                 &     (0.029)                 &     (0.030)                 &     (0.016)                 &     (0.527)                 &     (0.255)                 &     (0.378)                 &     (0.085)                 &     (0.408)                 &     (0.634)                 &     (0.567)                 \\\addlinespace
$wL_{c,t}$&       0.454$^{\ast}$        &       1.166$^{\ast\ast}$    &       0.168                 &       0.617$^{\ast\ast\ast}$&      -0.596$^{\ast\ast}$    &      -0.149                 &       0.069                 &      -0.516$^{\ast\ast\ast}$&       0.144                 &       0.600$^{\ast}$        &      -0.921$^{\ast\ast\ast}$\\
            &     (0.220)                 &     (0.516)                 &     (0.300)                 &     (0.177)                 &     (0.228)                 &     (0.140)                 &     (0.161)                 &     (0.088)                 &     (0.264)                 &     (0.303)                 &     (0.287)                 \\\addlinespace
$rK_{c,t}$&      -0.062                 &       0.287                 &      -0.177                 &       0.166                 &      -0.878$^{\ast\ast\ast}$&      -0.252                 &      -0.073                 &      -0.553$^{\ast\ast\ast}$&       0.021                 &       0.497$^{\ast}$        &      -0.764$^{\ast\ast}$    \\
            &     (0.125)                 &     (0.375)                 &     (0.146)                 &     (0.124)                 &     (0.242)                 &     (0.142)                 &     (0.159)                 &     (0.069)                 &     (0.262)                 &     (0.265)                 &     (0.292)                 \\\addlinespace
$pQ_{c,t}$&       0.626$^{\ast}$        &      -0.395                 &       0.997$^{\ast\ast}$    &       0.257                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.307)                 &     (0.827)                 &     (0.364)                 &     (0.292)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.006                 &      -0.001                 &       0.004                 &       0.013                 &      -0.054                 &       0.013                 &       0.054$^{\ast}$        &      -0.137                 &      -0.040                 &       0.157$^{\ast}$        \\
            &     (0.002)                 &     (0.004)                 &     (0.003)                 &     (0.003)                 &     (0.045)                 &     (0.036)                 &     (0.037)                 &     (0.026)                 &     (0.092)                 &     (0.081)                 &     (0.082)                 \\\addlinespace
$Services_{c,t}$&       0.001                 &      -0.023                 &      -0.014                 &      -0.001                 &      -0.118                 &       0.131                 &      -0.255$^{\ast}$        &       0.005                 &       0.543$^{\ast\ast}$    &      -0.643$^{\ast\ast}$    &       0.045                 \\
            &     (0.003)                 &     (0.029)                 &     (0.009)                 &     (0.005)                 &     (0.142)                 &     (0.105)                 &     (0.130)                 &     (0.032)                 &     (0.208)                 &     (0.277)                 &     (0.143)                 \\\addlinespace
$HHI_{c,t}$&      -1.195                 &      -2.788                 &      -3.268$^{\ast\ast\ast}$&      -1.606                 &     -54.320                 &       9.264                 &     -48.355$^{\ast\ast}$    &     -15.229$^{\ast}$        &      79.681$^{\ast\ast}$    &     -77.106$^{\ast\ast}$    &       8.416                 \\
            &     (0.680)                 &     (3.200)                 &     (0.900)                 &     (0.939)                 &    (30.764)                 &    (20.456)                 &    (17.037)                 &     (7.222)                 &    (33.259)                 &    (25.627)                 &    (34.445)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001                 &       0.005$^{\ast}$        &       0.003$^{\ast\ast}$    &      -0.000                 &       0.042$^{\ast}$        &       0.019                 &       0.018                 &       0.004                 &       0.019                 &       0.016                 &      -0.042                 \\
            &     (0.001)                 &     (0.003)                 &     (0.002)                 &     (0.001)                 &     (0.021)                 &     (0.012)                 &     (0.018)                 &     (0.008)                 &     (0.026)                 &     (0.037)                 &     (0.033)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.005                 &      -0.010                 &      -0.000                 &      -0.007                 &       0.144                 &      -0.084                 &       0.196                 &       0.033                 &      -0.161                 &       0.459                 &       0.261                 \\
            &     (0.007)                 &     (0.012)                 &     (0.009)                 &     (0.004)                 &     (0.179)                 &     (0.134)                 &     (0.113)                 &     (0.065)                 &     (0.301)                 &     (0.279)                 &     (0.273)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003                 &      -0.006                 &       0.006                 &       0.000                 &       0.131                 &       0.018                 &       0.095                 &       0.018                 &      -0.030                 &       0.085                 &      -0.071                 \\
            &     (0.003)                 &     (0.006)                 &     (0.006)                 &     (0.002)                 &     (0.079)                 &     (0.034)                 &     (0.073)                 &     (0.013)                 &     (0.084)                 &     (0.127)                 &     (0.069)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.008                 &      -0.022                 &       0.008                 &      -0.018$^{\ast}$        &      -0.068                 &       0.038                 &      -0.009                 &      -0.097                 &      -0.086                 &       0.230                 &      -0.311                 \\
            &     (0.008)                 &     (0.013)                 &     (0.014)                 &     (0.009)                 &     (0.189)                 &     (0.116)                 &     (0.161)                 &     (0.071)                 &     (0.254)                 &     (0.327)                 &     (0.283)                 \\\addlinespace
$Gini^{w}_{c,t}$&      -0.275$^{\ast\ast}$    &      -0.683$^{\ast}$        &      -0.552$^{\ast}$        &       0.063                 &      -4.170                 &      -3.206                 &      -1.796                 &       0.831                 &      -6.484                 &      -3.617                 &       8.131$^{\ast}$        \\
            &     (0.117)                 &     (0.314)                 &     (0.299)                 &     (0.204)                 &     (3.602)                 &     (2.205)                 &     (3.607)                 &     (1.094)                 &     (4.423)                 &     (7.292)                 &     (4.507)                 \\\addlinespace
$XRate_{c,t}$&      -0.004$^{\ast\ast}$    &      -0.003                 &      -0.007$^{\ast\ast}$    &      -0.005$^{\ast\ast}$    &      -0.107$^{\ast\ast}$    &       0.002                 &      -0.099$^{\ast\ast}$    &      -0.010                 &       0.148$^{\ast}$        &      -0.172$^{\ast\ast}$    &       0.082                 \\
            &     (0.002)                 &     (0.006)                 &     (0.003)                 &     (0.002)                 &     (0.046)                 &     (0.034)                 &     (0.036)                 &     (0.011)                 &     (0.078)                 &     (0.068)                 &     (0.048)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .982                 &        .988                 &        .984                 &        .973                 &         .99                 &        .986                 &         .97                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/TaxProgressiveness/Results2RICTint_EUKLEMS_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.016                 &      -0.041$^{\ast}$        &       0.014                 &      -0.008                 &      -0.021                 &      -0.319                 &       0.297                 &       0.000                 &      -0.973                 &       0.762                 &      -0.126                 \\
            &     (0.010)                 &     (0.020)                 &     (0.041)                 &     (0.020)                 &     (0.443)                 &     (0.241)                 &     (0.364)                 &     (0.127)                 &     (0.640)                 &     (0.913)                 &     (0.550)                 \\\addlinespace
$ICT_{c,t}$&      -0.049$^{\ast\ast\ast}$&      -0.052                 &      -0.099$^{\ast\ast}$    &      -0.036$^{\ast}$        &      -1.284$^{\ast\ast}$    &       0.076                 &      -1.572$^{\ast\ast}$    &       0.212                 &       1.053                 &      -2.365$^{\ast\ast}$    &       1.347$^{\ast\ast}$    \\
            &     (0.011)                 &     (0.067)                 &     (0.036)                 &     (0.021)                 &     (0.467)                 &     (0.342)                 &     (0.606)                 &     (0.156)                 &     (0.901)                 &     (1.098)                 &     (0.613)                 \\\addlinespace
$R*ICT_{c,t}$&       0.019$^{\ast\ast\ast}$&       0.007                 &       0.042$^{\ast\ast}$    &       0.029$^{\ast\ast\ast}$&       0.346                 &      -0.218                 &       0.547$^{\ast\ast}$    &       0.017                 &      -0.828$^{\ast\ast}$    &       0.999$^{\ast\ast}$    &      -0.187                 \\
            &     (0.005)                 &     (0.023)                 &     (0.016)                 &     (0.010)                 &     (0.261)                 &     (0.154)                 &     (0.259)                 &     (0.073)                 &     (0.359)                 &     (0.428)                 &     (0.281)                 \\\addlinespace
$wL_{c,t}$&       0.581$^{\ast\ast\ast}$&       0.713$^{\ast}$        &       0.658$^{\ast\ast}$    &       0.597$^{\ast\ast\ast}$&      -0.447$^{\ast\ast}$    &       0.049                 &       0.133                 &      -0.629$^{\ast\ast\ast}$&       0.548$^{\ast\ast}$    &       0.817$^{\ast\ast}$    &      -1.399$^{\ast\ast\ast}$\\
            &     (0.167)                 &     (0.359)                 &     (0.273)                 &     (0.152)                 &     (0.161)                 &     (0.112)                 &     (0.135)                 &     (0.095)                 &     (0.243)                 &     (0.375)                 &     (0.254)                 \\\addlinespace
$rK_{c,t}$&       0.089                 &       0.268                 &       0.116                 &       0.050                 &      -0.646$^{\ast\ast\ast}$&      -0.023                 &       0.033                 &      -0.657$^{\ast\ast\ast}$&       0.498$^{\ast\ast}$    &       0.727$^{\ast\ast}$    &      -1.319$^{\ast\ast\ast}$\\
            &     (0.089)                 &     (0.270)                 &     (0.159)                 &     (0.089)                 &     (0.138)                 &     (0.088)                 &     (0.107)                 &     (0.074)                 &     (0.178)                 &     (0.259)                 &     (0.217)                 \\\addlinespace
$pQ_{c,t}$&       0.224                 &      -0.069                 &       0.131                 &       0.285                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.249)                 &     (0.589)                 &     (0.365)                 &     (0.230)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.003                 &       0.006                 &      -0.002                 &       0.010                 &      -0.031                 &       0.039                 &       0.002                 &      -0.117                 &       0.135                 &       0.002                 \\
            &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.002)                 &     (0.039)                 &     (0.026)                 &     (0.029)                 &     (0.014)                 &     (0.078)                 &     (0.087)                 &     (0.041)                 \\\addlinespace
$Services_{c,t}$&      -0.003                 &       0.011                 &      -0.014                 &      -0.014$^{\ast}$        &      -0.030                 &       0.151$^{\ast}$        &      -0.135                 &      -0.046                 &       0.517$^{\ast\ast}$    &      -0.379                 &      -0.164                 \\
            &     (0.004)                 &     (0.014)                 &     (0.010)                 &     (0.007)                 &     (0.092)                 &     (0.081)                 &     (0.099)                 &     (0.041)                 &     (0.235)                 &     (0.272)                 &     (0.109)                 \\\addlinespace
$HHI_{c,t}$&      -0.901                 &       2.158                 &      -3.412                 &      -2.814$^{\ast\ast\ast}$&     -14.469                 &      24.880$^{\ast}$        &     -27.992                 &     -11.358                 &      90.809$^{\ast\ast}$    &     -73.689                 &     -16.310                 \\
            &     (0.581)                 &     (1.791)                 &     (2.096)                 &     (0.838)                 &    (17.999)                 &    (13.683)                 &    (19.079)                 &     (7.994)                 &    (43.087)                 &    (58.783)                 &    (24.745)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.002$^{\ast\ast\ast}$&       0.000                 &       0.004$^{\ast\ast}$    &       0.002$^{\ast\ast\ast}$&       0.052$^{\ast\ast\ast}$&      -0.005                 &       0.038$^{\ast\ast\ast}$&       0.019$^{\ast\ast\ast}$&      -0.064$^{\ast\ast}$    &       0.061                 &      -0.006                 \\
            &     (0.000)                 &     (0.001)                 &     (0.001)                 &     (0.001)                 &     (0.012)                 &     (0.008)                 &     (0.013)                 &     (0.004)                 &     (0.025)                 &     (0.036)                 &     (0.014)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.009                 &       0.003                 &      -0.021                 &      -0.013$^{\ast\ast}$    &      -0.332$^{\ast}$        &      -0.052                 &      -0.172                 &      -0.108$^{\ast\ast}$    &       0.304                 &      -0.267                 &       0.207                 \\
            &     (0.007)                 &     (0.009)                 &     (0.015)                 &     (0.006)                 &     (0.189)                 &     (0.090)                 &     (0.155)                 &     (0.046)                 &     (0.262)                 &     (0.391)                 &     (0.161)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.005$^{\ast\ast\ast}$&      -0.002                 &       0.004                 &       0.005$^{\ast\ast}$    &       0.114$^{\ast\ast\ast}$&       0.012                 &       0.070$^{\ast}$        &       0.032$^{\ast\ast\ast}$&      -0.027                 &       0.046                 &      -0.033                 \\
            &     (0.001)                 &     (0.004)                 &     (0.004)                 &     (0.002)                 &     (0.028)                 &     (0.019)                 &     (0.036)                 &     (0.010)                 &     (0.067)                 &     (0.084)                 &     (0.040)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.007                 &       0.010                 &       0.004                 &      -0.005                 &      -0.009                 &       0.022                 &       0.039                 &      -0.070                 &       0.071                 &      -0.022                 &      -0.194                 \\
            &     (0.005)                 &     (0.009)                 &     (0.015)                 &     (0.006)                 &     (0.193)                 &     (0.103)                 &     (0.160)                 &     (0.058)                 &     (0.282)                 &     (0.340)                 &     (0.226)                 \\\addlinespace
$Gini^{w}_{c,t}$&      -0.121                 &      -0.039                 &      -0.093                 &      -0.227                 &      -1.701                 &      -0.136                 &       0.110                 &      -1.675                 &       2.191                 &       0.147                 &      -1.891                 \\
            &     (0.079)                 &     (0.139)                 &     (0.138)                 &     (0.132)                 &     (2.972)                 &     (1.489)                 &     (1.733)                 &     (1.382)                 &     (3.346)                 &     (3.259)                 &     (3.640)                 \\\addlinespace
$XRate_{c,t}$&      -0.004$^{\ast\ast\ast}$&      -0.001                 &      -0.003                 &      -0.007$^{\ast\ast\ast}$&      -0.067$^{\ast}$        &       0.000                 &      -0.055                 &      -0.011                 &       0.084                 &      -0.061                 &       0.029                 \\
            &     (0.001)                 &     (0.005)                 &     (0.002)                 &     (0.002)                 &     (0.034)                 &     (0.027)                 &     (0.034)                 &     (0.010)                 &     (0.065)                 &     (0.076)                 &     (0.032)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &        .999                 &        .973                 &        .985                 &        .975                 &        .961                 &        .983                 &        .972                 &        .957                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/TaxProgressiveness/Results2RICTint_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.010                 &       0.013                 &       0.023                 &      -0.056                 &       0.236                 &       0.216                 &       0.242                 &      -0.221                 &       0.408                 &       0.557                 &      -0.946                 \\
            &     (0.022)                 &     (0.025)                 &     (0.060)                 &     (0.030)                 &     (0.794)                 &     (0.481)                 &     (0.585)                 &     (0.240)                 &     (0.807)                 &     (1.017)                 &     (0.798)                 \\\addlinespace
$ICT_{c,t}$&       0.022                 &      -0.011                 &       0.031                 &       0.030                 &       0.349                 &      -0.164                 &       0.256                 &       0.257$^{\ast\ast\ast}$&      -1.459                 &       0.828                 &       0.615                 \\
            &     (0.034)                 &     (0.052)                 &     (0.032)                 &     (0.055)                 &     (0.469)                 &     (0.672)                 &     (0.342)                 &     (0.056)                 &     (1.075)                 &     (0.791)                 &     (0.653)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.016                 &      -0.005                 &       0.001                 &      -0.031                 &      -0.065                 &      -0.186                 &       0.243                 &      -0.122                 &       0.173                 &       0.074                 &      -0.278                 \\
            &     (0.024)                 &     (0.027)                 &     (0.042)                 &     (0.033)                 &     (0.703)                 &     (0.431)                 &     (0.657)                 &     (0.104)                 &     (0.526)                 &     (0.818)                 &     (0.605)                 \\\addlinespace
$wL_{c,t}$&       0.399$^{\ast\ast\ast}$&       0.344$^{\ast}$        &       0.522                 &       0.370$^{\ast\ast\ast}$&      -0.608$^{\ast\ast}$    &       0.003                 &       0.180                 &      -0.791$^{\ast\ast\ast}$&       0.571                 &       1.331$^{\ast}$        &      -1.886$^{\ast\ast\ast}$\\
            &     (0.085)                 &     (0.180)                 &     (0.288)                 &     (0.090)                 &     (0.194)                 &     (0.065)                 &     (0.244)                 &     (0.081)                 &     (0.379)                 &     (0.603)                 &     (0.332)                 \\\addlinespace
$rK_{c,t}$&       0.020                 &       0.232                 &       0.157                 &      -0.239$^{\ast\ast\ast}$&      -0.669$^{\ast\ast\ast}$&      -0.019                 &       0.142                 &      -0.792$^{\ast\ast\ast}$&       0.591$^{\ast}$        &       1.231$^{\ast\ast}$    &      -1.811$^{\ast\ast\ast}$\\
            &     (0.068)                 &     (0.127)                 &     (0.178)                 &     (0.069)                 &     (0.164)                 &     (0.046)                 &     (0.198)                 &     (0.085)                 &     (0.301)                 &     (0.459)                 &     (0.304)                 \\\addlinespace
$pQ_{c,t}$&       0.217                 &       0.085                 &       0.253                 &       0.261$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.137)                 &     (0.325)                 &     (0.348)                 &     (0.120)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.000                 &      -0.003                 &       0.000                 &       0.004$^{\ast\ast}$    &      -0.082                 &      -0.050                 &      -0.020                 &      -0.012                 &      -0.082                 &       0.051                 &       0.028                 \\
            &     (0.001)                 &     (0.003)                 &     (0.004)                 &     (0.002)                 &     (0.064)                 &     (0.031)                 &     (0.035)                 &     (0.007)                 &     (0.059)                 &     (0.083)                 &     (0.055)                 \\\addlinespace
$Services_{c,t}$&       0.000                 &       0.019$^{\ast\ast}$    &       0.011                 &      -0.020$^{\ast\ast}$    &       0.220                 &       0.126$^{\ast}$        &       0.114                 &      -0.020                 &       0.198                 &       0.041                 &      -0.253                 \\
            &     (0.005)                 &     (0.006)                 &     (0.012)                 &     (0.008)                 &     (0.187)                 &     (0.067)                 &     (0.147)                 &     (0.047)                 &     (0.223)                 &     (0.271)                 &     (0.148)                 \\\addlinespace
$HHI_{c,t}$&      -0.571                 &       1.222                 &       0.677                 &      -3.414$^{\ast\ast}$    &      20.495                 &      12.182                 &       3.589                 &       4.724                 &       6.745                 &      -6.478                 &      -2.492                 \\
            &     (0.563)                 &     (0.936)                 &     (1.637)                 &     (1.234)                 &    (22.114)                 &    (12.660)                 &    (15.151)                 &     (9.745)                 &    (29.095)                 &    (39.240)                 &    (32.568)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast\ast}$    &       0.001                 &      -0.001                 &       0.044$^{\ast\ast}$    &      -0.003                 &       0.021                 &       0.026$^{\ast\ast\ast}$&      -0.040                 &       0.020                 &       0.023                 \\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.001)                 &     (0.014)                 &     (0.009)                 &     (0.012)                 &     (0.007)                 &     (0.022)                 &     (0.027)                 &     (0.015)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.015$^{\ast}$        &       0.017$^{\ast}$        &      -0.025                 &       0.044$^{\ast\ast\ast}$&      -0.700$^{\ast}$        &      -0.115                 &      -0.243                 &      -0.342$^{\ast\ast}$    &       0.385                 &      -0.129                 &      -0.297                 \\
            &     (0.008)                 &     (0.007)                 &     (0.032)                 &     (0.011)                 &     (0.330)                 &     (0.114)                 &     (0.196)                 &     (0.136)                 &     (0.208)                 &     (0.376)                 &     (0.401)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003$^{\ast}$        &       0.002                 &       0.006                 &       0.000                 &       0.083                 &       0.017                 &       0.059                 &       0.008                 &      -0.026                 &       0.090                 &      -0.073                 \\
            &     (0.001)                 &     (0.002)                 &     (0.003)                 &     (0.002)                 &     (0.048)                 &     (0.018)                 &     (0.036)                 &     (0.011)                 &     (0.038)                 &     (0.056)                 &     (0.045)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.005                 &       0.022$^{\ast}$        &       0.000                 &      -0.004                 &       0.154                 &       0.096                 &       0.124                 &      -0.066                 &       0.307                 &       0.024                 &      -0.317                 \\
            &     (0.006)                 &     (0.012)                 &     (0.018)                 &     (0.009)                 &     (0.204)                 &     (0.088)                 &     (0.170)                 &     (0.049)                 &     (0.279)                 &     (0.305)                 &     (0.254)                 \\\addlinespace
$XRate_{c,t}$&       0.006                 &      -0.002                 &       0.007                 &       0.018$^{\ast}$        &      -0.003                 &      -0.022                 &       0.000                 &       0.018                 &      -0.166                 &       0.157                 &       0.005                 \\
            &     (0.008)                 &     (0.009)                 &     (0.016)                 &     (0.008)                 &     (0.269)                 &     (0.126)                 &     (0.251)                 &     (0.053)                 &     (0.204)                 &     (0.335)                 &     (0.213)                 \\\addlinespace
$Gini^{w}_{c,t}$&      -0.534                 &       0.546                 &      -2.035                 &      -0.512                 &     -11.923                 &       7.904                 &     -20.568                 &       0.741                 &      31.981                 &     -53.367$^{\ast}$        &      20.169                 \\
            &     (0.391)                 &     (0.700)                 &     (1.449)                 &     (0.338)                 &    (13.351)                 &     (8.440)                 &    (12.519)                 &     (3.255)                 &    (20.372)                 &    (28.630)                 &    (19.228)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .986                 &        .994                 &        .989                 &        .984                 &        .992                 &         .99                 &        .983                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/TaxProgressiveness/Results2RICTint_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.040$^{\ast}$        &      -0.077                 &      -0.107$^{\ast\ast\ast}$&       0.019                 &      -0.693$^{\ast}$        &      -0.231                 &      -0.835$^{\ast}$        &       0.372$^{\ast\ast}$    &      -0.119                 &      -1.993$^{\ast\ast}$    &       1.335$^{\ast\ast}$    \\
            &     (0.020)                 &     (0.049)                 &     (0.030)                 &     (0.032)                 &     (0.385)                 &     (0.185)                 &     (0.384)                 &     (0.133)                 &     (0.471)                 &     (0.789)                 &     (0.470)                 \\\addlinespace
$ICT_{c,t}$&      -0.042                 &      -0.162                 &      -0.109$^{\ast}$        &      -0.008                 &      -0.750                 &       0.356                 &      -1.223                 &       0.117                 &       1.133                 &      -2.522$^{\ast}$        &       0.664                 \\
            &     (0.025)                 &     (0.124)                 &     (0.052)                 &     (0.027)                 &     (0.684)                 &     (0.465)                 &     (0.702)                 &     (0.173)                 &     (0.999)                 &     (1.381)                 &     (0.951)                 \\\addlinespace
$R*ICT_{c,t}$&       0.012                 &       0.047                 &       0.028                 &      -0.001                 &       0.075                 &       0.047                 &      -0.029                 &       0.056                 &       0.242                 &       0.163                 &       0.123                 \\
            &     (0.017)                 &     (0.044)                 &     (0.031)                 &     (0.018)                 &     (0.559)                 &     (0.259)                 &     (0.411)                 &     (0.092)                 &     (0.409)                 &     (0.679)                 &     (0.603)                 \\\addlinespace
$wL_{c,t}$&       0.445$^{\ast}$        &       1.155$^{\ast\ast}$    &       0.140                 &       0.613$^{\ast\ast\ast}$&      -0.602$^{\ast\ast}$    &      -0.140                 &       0.052                 &      -0.514$^{\ast\ast\ast}$&       0.165                 &       0.566$^{\ast}$        &      -0.913$^{\ast\ast\ast}$\\
            &     (0.220)                 &     (0.484)                 &     (0.297)                 &     (0.179)                 &     (0.225)                 &     (0.140)                 &     (0.157)                 &     (0.087)                 &     (0.265)                 &     (0.302)                 &     (0.284)                 \\\addlinespace
$rK_{c,t}$&      -0.068                 &       0.200                 &      -0.194                 &       0.170                 &      -0.887$^{\ast\ast\ast}$&      -0.249                 &      -0.086                 &      -0.552$^{\ast\ast\ast}$&       0.034                 &       0.474$^{\ast}$        &      -0.758$^{\ast\ast}$    \\
            &     (0.128)                 &     (0.319)                 &     (0.149)                 &     (0.127)                 &     (0.242)                 &     (0.143)                 &     (0.156)                 &     (0.069)                 &     (0.263)                 &     (0.266)                 &     (0.294)                 \\\addlinespace
$pQ_{c,t}$&       0.641$^{\ast}$        &      -0.292                 &       1.044$^{\ast\ast}$    &       0.255                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.310)                 &     (0.739)                 &     (0.365)                 &     (0.297)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.006                 &      -0.001                 &       0.004                 &       0.013                 &      -0.054                 &       0.013                 &       0.054$^{\ast}$        &      -0.137                 &      -0.038                 &       0.157$^{\ast}$        \\
            &     (0.002)                 &     (0.004)                 &     (0.003)                 &     (0.003)                 &     (0.045)                 &     (0.036)                 &     (0.037)                 &     (0.026)                 &     (0.091)                 &     (0.082)                 &     (0.083)                 \\\addlinespace
$Services_{c,t}$&       0.002                 &      -0.023                 &      -0.013                 &      -0.001                 &      -0.116                 &       0.124                 &      -0.244$^{\ast}$        &       0.004                 &       0.529$^{\ast\ast}$    &      -0.619$^{\ast\ast}$    &       0.040                 \\
            &     (0.003)                 &     (0.027)                 &     (0.009)                 &     (0.005)                 &     (0.143)                 &     (0.104)                 &     (0.133)                 &     (0.031)                 &     (0.208)                 &     (0.279)                 &     (0.144)                 \\\addlinespace
$HHI_{c,t}$&      -1.141                 &      -2.182                 &      -3.120$^{\ast\ast\ast}$&      -1.632                 &     -53.009                 &       9.721                 &     -47.469$^{\ast\ast}$    &     -15.260$^{\ast}$        &      79.200$^{\ast\ast}$    &     -76.069$^{\ast\ast}$    &       7.733                 \\
            &     (0.686)                 &     (2.773)                 &     (0.898)                 &     (0.948)                 &    (31.000)                 &    (20.654)                 &    (17.061)                 &     (7.347)                 &    (33.558)                 &    (25.963)                 &    (35.039)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001                 &       0.005$^{\ast}$        &       0.003$^{\ast\ast}$    &      -0.000                 &       0.042$^{\ast}$        &       0.020                 &       0.018                 &       0.004                 &       0.019                 &       0.015                 &      -0.042                 \\
            &     (0.001)                 &     (0.003)                 &     (0.002)                 &     (0.001)                 &     (0.021)                 &     (0.012)                 &     (0.018)                 &     (0.008)                 &     (0.026)                 &     (0.038)                 &     (0.033)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.006                 &      -0.009                 &      -0.001                 &      -0.007                 &       0.149                 &      -0.081                 &       0.197                 &       0.033                 &      -0.160                 &       0.459                 &       0.260                 \\
            &     (0.007)                 &     (0.011)                 &     (0.009)                 &     (0.004)                 &     (0.178)                 &     (0.131)                 &     (0.113)                 &     (0.065)                 &     (0.300)                 &     (0.285)                 &     (0.273)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003                 &      -0.006                 &       0.006                 &       0.000                 &       0.131                 &       0.016                 &       0.097                 &       0.018                 &      -0.033                 &       0.090                 &      -0.072                 \\
            &     (0.003)                 &     (0.006)                 &     (0.006)                 &     (0.002)                 &     (0.080)                 &     (0.033)                 &     (0.074)                 &     (0.013)                 &     (0.084)                 &     (0.129)                 &     (0.070)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.008                 &      -0.026                 &       0.008                 &      -0.017$^{\ast}$        &      -0.073                 &       0.031                 &      -0.006                 &      -0.098                 &      -0.095                 &       0.236                 &      -0.311                 \\
            &     (0.008)                 &     (0.015)                 &     (0.014)                 &     (0.009)                 &     (0.192)                 &     (0.117)                 &     (0.162)                 &     (0.071)                 &     (0.255)                 &     (0.330)                 &     (0.283)                 \\\addlinespace
$XRate_{c,t}$&      -0.005$^{\ast\ast}$    &      -0.007                 &      -0.009$^{\ast\ast}$    &      -0.005$^{\ast\ast}$    &      -0.119$^{\ast\ast}$    &       0.005                 &      -0.116$^{\ast\ast}$    &      -0.009                 &       0.160$^{\ast}$        &      -0.205$^{\ast\ast}$    &       0.091$^{\ast\ast}$    \\
            &     (0.002)                 &     (0.006)                 &     (0.003)                 &     (0.002)                 &     (0.047)                 &     (0.033)                 &     (0.044)                 &     (0.011)                 &     (0.081)                 &     (0.082)                 &     (0.040)                 \\\addlinespace
$Gini^{w}_{c,t}$&      -0.276$^{\ast\ast}$    &      -0.667$^{\ast}$        &      -0.560$^{\ast}$        &       0.061                 &      -4.085                 &      -3.125                 &      -1.788                 &       0.828                 &      -6.421                 &      -3.643                 &       8.095                 \\
            &     (0.118)                 &     (0.313)                 &     (0.300)                 &     (0.204)                 &     (3.691)                 &     (2.275)                 &     (3.607)                 &     (1.095)                 &     (4.514)                 &     (7.436)                 &     (4.566)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .982                 &        .988                 &        .984                 &        .973                 &         .99                 &        .986                 &         .97                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/TaxProgressiveness/Results2RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.016                 &      -0.039$^{\ast}$        &       0.016                 &      -0.007                 &      -0.001                 &      -0.320                 &       0.319                 &       0.000                 &      -0.996                 &       0.798                 &      -0.140                 \\
            &     (0.010)                 &     (0.019)                 &     (0.041)                 &     (0.020)                 &     (0.439)                 &     (0.237)                 &     (0.362)                 &     (0.126)                 &     (0.634)                 &     (0.910)                 &     (0.543)                 \\\addlinespace
$ICT_{c,t}$&      -0.057$^{\ast\ast\ast}$&      -0.092                 &      -0.118$^{\ast\ast\ast}$&      -0.039                 &      -1.559$^{\ast\ast}$    &       0.026                 &      -1.797$^{\ast\ast\ast}$&       0.213                 &       1.209                 &      -2.698$^{\ast\ast}$    &       1.526$^{\ast\ast}$    \\
            &     (0.013)                 &     (0.098)                 &     (0.038)                 &     (0.025)                 &     (0.553)                 &     (0.368)                 &     (0.622)                 &     (0.174)                 &     (0.936)                 &     (1.083)                 &     (0.671)                 \\\addlinespace
$R*ICT_{c,t}$&       0.021$^{\ast\ast\ast}$&       0.022                 &       0.047$^{\ast\ast}$    &       0.030$^{\ast\ast}$    &       0.416                 &      -0.200                 &       0.590$^{\ast\ast}$    &       0.026                 &      -0.876$^{\ast\ast}$    &       1.068$^{\ast\ast}$    &      -0.210                 \\
            &     (0.006)                 &     (0.034)                 &     (0.017)                 &     (0.012)                 &     (0.295)                 &     (0.153)                 &     (0.268)                 &     (0.080)                 &     (0.365)                 &     (0.422)                 &     (0.302)                 \\\addlinespace
$wL_{c,t}$&       0.575$^{\ast\ast\ast}$&       0.718$^{\ast}$        &       0.647$^{\ast\ast}$    &       0.592$^{\ast\ast\ast}$&      -0.454$^{\ast\ast\ast}$&       0.052                 &       0.122                 &      -0.627$^{\ast\ast\ast}$&       0.555$^{\ast\ast}$    &       0.799$^{\ast\ast}$    &      -1.388$^{\ast\ast\ast}$\\
            &     (0.167)                 &     (0.357)                 &     (0.274)                 &     (0.151)                 &     (0.157)                 &     (0.111)                 &     (0.135)                 &     (0.094)                 &     (0.245)                 &     (0.380)                 &     (0.253)                 \\\addlinespace
$rK_{c,t}$&       0.087                 &       0.259                 &       0.111                 &       0.050                 &      -0.652$^{\ast\ast\ast}$&      -0.022                 &       0.025                 &      -0.655$^{\ast\ast\ast}$&       0.503$^{\ast\ast}$    &       0.715$^{\ast\ast}$    &      -1.311$^{\ast\ast\ast}$\\
            &     (0.089)                 &     (0.261)                 &     (0.160)                 &     (0.089)                 &     (0.137)                 &     (0.088)                 &     (0.107)                 &     (0.074)                 &     (0.180)                 &     (0.265)                 &     (0.217)                 \\\addlinespace
$pQ_{c,t}$&       0.233                 &      -0.062                 &       0.149                 &       0.290                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.249)                 &     (0.577)                 &     (0.368)                 &     (0.231)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.003                 &       0.006                 &      -0.002                 &       0.010                 &      -0.031                 &       0.038                 &       0.002                 &      -0.117                 &       0.135                 &       0.002                 \\
            &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.002)                 &     (0.039)                 &     (0.026)                 &     (0.029)                 &     (0.014)                 &     (0.077)                 &     (0.087)                 &     (0.041)                 \\\addlinespace
$Services_{c,t}$&      -0.003                 &       0.011                 &      -0.014                 &      -0.014$^{\ast}$        &      -0.026                 &       0.151$^{\ast}$        &      -0.129                 &      -0.047                 &       0.513$^{\ast\ast}$    &      -0.371                 &      -0.169                 \\
            &     (0.004)                 &     (0.014)                 &     (0.010)                 &     (0.007)                 &     (0.092)                 &     (0.080)                 &     (0.099)                 &     (0.041)                 &     (0.235)                 &     (0.273)                 &     (0.109)                 \\\addlinespace
$HHI_{c,t}$&      -0.903                 &       2.201                 &      -3.412                 &      -2.824$^{\ast\ast\ast}$&     -14.113                 &      24.969$^{\ast}$        &     -27.662                 &     -11.420                 &      90.799$^{\ast\ast}$    &     -73.283                 &     -16.685                 \\
            &     (0.582)                 &     (1.763)                 &     (2.088)                 &     (0.843)                 &    (17.909)                 &    (13.689)                 &    (19.071)                 &     (7.985)                 &    (43.113)                 &    (58.868)                 &    (24.721)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.002$^{\ast\ast\ast}$&       0.000                 &       0.004$^{\ast\ast}$    &       0.002$^{\ast\ast\ast}$&       0.052$^{\ast\ast\ast}$&      -0.005                 &       0.038$^{\ast\ast\ast}$&       0.019$^{\ast\ast\ast}$&      -0.064$^{\ast\ast}$    &       0.061                 &      -0.006                 \\
            &     (0.000)                 &     (0.001)                 &     (0.001)                 &     (0.001)                 &     (0.012)                 &     (0.008)                 &     (0.013)                 &     (0.004)                 &     (0.025)                 &     (0.036)                 &     (0.014)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.009                 &       0.004                 &      -0.021                 &      -0.013$^{\ast\ast}$    &      -0.329                 &      -0.050                 &      -0.171                 &      -0.108$^{\ast\ast}$    &       0.305                 &      -0.266                 &       0.206                 \\
            &     (0.007)                 &     (0.008)                 &     (0.015)                 &     (0.006)                 &     (0.191)                 &     (0.090)                 &     (0.156)                 &     (0.046)                 &     (0.262)                 &     (0.392)                 &     (0.160)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.005$^{\ast\ast\ast}$&      -0.002                 &       0.004                 &       0.005$^{\ast\ast}$    &       0.114$^{\ast\ast\ast}$&       0.012                 &       0.071$^{\ast}$        &       0.031$^{\ast\ast\ast}$&      -0.027                 &       0.047                 &      -0.034                 \\
            &     (0.001)                 &     (0.004)                 &     (0.004)                 &     (0.002)                 &     (0.028)                 &     (0.019)                 &     (0.036)                 &     (0.010)                 &     (0.067)                 &     (0.084)                 &     (0.040)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.007                 &       0.009                 &       0.003                 &      -0.005                 &      -0.012                 &       0.020                 &       0.039                 &      -0.071                 &       0.070                 &      -0.021                 &      -0.194                 \\
            &     (0.005)                 &     (0.009)                 &     (0.015)                 &     (0.006)                 &     (0.193)                 &     (0.103)                 &     (0.159)                 &     (0.059)                 &     (0.283)                 &     (0.339)                 &     (0.227)                 \\\addlinespace
$XRate_{c,t}$&      -0.004$^{\ast\ast\ast}$&      -0.004                 &      -0.004                 &      -0.007$^{\ast\ast\ast}$&      -0.087$^{\ast\ast}$    &      -0.002                 &      -0.075$^{\ast}$        &      -0.010                 &       0.098                 &      -0.090                 &       0.045                 \\
            &     (0.001)                 &     (0.006)                 &     (0.003)                 &     (0.002)                 &     (0.035)                 &     (0.028)                 &     (0.037)                 &     (0.011)                 &     (0.068)                 &     (0.080)                 &     (0.034)                 \\\addlinespace
$Gini^{w}_{c,t}$&      -0.123                 &      -0.018                 &      -0.095                 &      -0.231$^{\ast}$        &      -1.661                 &      -0.089                 &       0.080                 &      -1.653                 &       2.233                 &       0.087                 &      -1.862                 \\
            &     (0.080)                 &     (0.146)                 &     (0.145)                 &     (0.132)                 &     (2.991)                 &     (1.480)                 &     (1.773)                 &     (1.370)                 &     (3.329)                 &     (3.287)                 &     (3.623)                 \\\midrule
%$R^{2}$  &          0.999                &        .998                 &        .999                 &        .999                 &        .973                 &        .985                 &        .975                 &        .961                 &        .983                 &        .972                 &        .957                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/TaxProgressiveness/Results2shortV1_RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.010                 &       0.013                 &       0.023                 &      -0.056                 &       0.236                 &       0.216                 &       0.242                 &      -0.221                 &       0.408                 &       0.557                 &      -0.946                 \\
            &     (0.022)                 &     (0.025)                 &     (0.060)                 &     (0.030)                 &     (0.794)                 &     (0.481)                 &     (0.585)                 &     (0.240)                 &     (0.807)                 &     (1.017)                 &     (0.798)                 \\\addlinespace
$ICT_{c,t}$&       0.022                 &      -0.011                 &       0.031                 &       0.030                 &       0.349                 &      -0.164                 &       0.256                 &       0.257$^{\ast\ast\ast}$&      -1.459                 &       0.828                 &       0.615                 \\
            &     (0.034)                 &     (0.052)                 &     (0.032)                 &     (0.055)                 &     (0.469)                 &     (0.672)                 &     (0.342)                 &     (0.056)                 &     (1.075)                 &     (0.791)                 &     (0.653)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.016                 &      -0.005                 &       0.001                 &      -0.031                 &      -0.065                 &      -0.186                 &       0.243                 &      -0.122                 &       0.173                 &       0.074                 &      -0.278                 \\
            &     (0.024)                 &     (0.027)                 &     (0.042)                 &     (0.033)                 &     (0.703)                 &     (0.431)                 &     (0.657)                 &     (0.104)                 &     (0.526)                 &     (0.818)                 &     (0.605)                 \\\addlinespace
$wL_{c,t}$&       0.399$^{\ast\ast\ast}$&       0.344$^{\ast}$        &       0.522                 &       0.370$^{\ast\ast\ast}$&      -0.608$^{\ast\ast}$    &       0.003                 &       0.180                 &      -0.791$^{\ast\ast\ast}$&       0.571                 &       1.331$^{\ast}$        &      -1.886$^{\ast\ast\ast}$\\
            &     (0.085)                 &     (0.180)                 &     (0.288)                 &     (0.090)                 &     (0.194)                 &     (0.065)                 &     (0.244)                 &     (0.081)                 &     (0.379)                 &     (0.603)                 &     (0.332)                 \\\addlinespace
$rK_{c,t}$&       0.020                 &       0.232                 &       0.157                 &      -0.239$^{\ast\ast\ast}$&      -0.669$^{\ast\ast\ast}$&      -0.019                 &       0.142                 &      -0.792$^{\ast\ast\ast}$&       0.591$^{\ast}$        &       1.231$^{\ast\ast}$    &      -1.811$^{\ast\ast\ast}$\\
            &     (0.068)                 &     (0.127)                 &     (0.178)                 &     (0.069)                 &     (0.164)                 &     (0.046)                 &     (0.198)                 &     (0.085)                 &     (0.301)                 &     (0.459)                 &     (0.304)                 \\\addlinespace
$pQ_{c,t}$&       0.217                 &       0.085                 &       0.253                 &       0.261$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.137)                 &     (0.325)                 &     (0.348)                 &     (0.120)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .986                 &        .994                 &        .989                 &        .984                 &        .992                 &         .99                 &        .983                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/TaxProgressiveness/Results2shortV1_RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.040$^{\ast}$        &      -0.077                 &      -0.107$^{\ast\ast\ast}$&       0.019                 &      -0.693$^{\ast}$        &      -0.231                 &      -0.835$^{\ast}$        &       0.372$^{\ast\ast}$    &      -0.119                 &      -1.993$^{\ast\ast}$    &       1.335$^{\ast\ast}$    \\
            &     (0.020)                 &     (0.049)                 &     (0.030)                 &     (0.032)                 &     (0.385)                 &     (0.185)                 &     (0.384)                 &     (0.133)                 &     (0.471)                 &     (0.789)                 &     (0.470)                 \\\addlinespace
$ICT_{c,t}$&      -0.042                 &      -0.162                 &      -0.109$^{\ast}$        &      -0.008                 &      -0.750                 &       0.356                 &      -1.223                 &       0.117                 &       1.133                 &      -2.522$^{\ast}$        &       0.664                 \\
            &     (0.025)                 &     (0.124)                 &     (0.052)                 &     (0.027)                 &     (0.684)                 &     (0.465)                 &     (0.702)                 &     (0.173)                 &     (0.999)                 &     (1.381)                 &     (0.951)                 \\\addlinespace
$R*ICT_{c,t}$&       0.012                 &       0.047                 &       0.028                 &      -0.001                 &       0.075                 &       0.047                 &      -0.029                 &       0.056                 &       0.242                 &       0.163                 &       0.123                 \\
            &     (0.017)                 &     (0.044)                 &     (0.031)                 &     (0.018)                 &     (0.559)                 &     (0.259)                 &     (0.411)                 &     (0.092)                 &     (0.409)                 &     (0.679)                 &     (0.603)                 \\\addlinespace
$wL_{c,t}$&       0.445$^{\ast}$        &       1.155$^{\ast\ast}$    &       0.140                 &       0.613$^{\ast\ast\ast}$&      -0.602$^{\ast\ast}$    &      -0.140                 &       0.052                 &      -0.514$^{\ast\ast\ast}$&       0.165                 &       0.566$^{\ast}$        &      -0.913$^{\ast\ast\ast}$\\
            &     (0.220)                 &     (0.484)                 &     (0.297)                 &     (0.179)                 &     (0.225)                 &     (0.140)                 &     (0.157)                 &     (0.087)                 &     (0.265)                 &     (0.302)                 &     (0.284)                 \\\addlinespace
$rK_{c,t}$&      -0.068                 &       0.200                 &      -0.194                 &       0.170                 &      -0.887$^{\ast\ast\ast}$&      -0.249                 &      -0.086                 &      -0.552$^{\ast\ast\ast}$&       0.034                 &       0.474$^{\ast}$        &      -0.758$^{\ast\ast}$    \\
            &     (0.128)                 &     (0.319)                 &     (0.149)                 &     (0.127)                 &     (0.242)                 &     (0.143)                 &     (0.156)                 &     (0.069)                 &     (0.263)                 &     (0.266)                 &     (0.294)                 \\\addlinespace
$pQ_{c,t}$&       0.641$^{\ast}$        &      -0.292                 &       1.044$^{\ast\ast}$    &       0.255                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.310)                 &     (0.739)                 &     (0.365)                 &     (0.297)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .982                 &        .988                 &        .984                 &        .973                 &         .99                 &        .986                 &         .97                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/TaxProgressiveness/Results2shortV1_RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.016                 &      -0.039$^{\ast}$        &       0.016                 &      -0.007                 &      -0.001                 &      -0.320                 &       0.319                 &       0.000                 &      -0.996                 &       0.798                 &      -0.140                 \\
            &     (0.010)                 &     (0.019)                 &     (0.041)                 &     (0.020)                 &     (0.439)                 &     (0.237)                 &     (0.362)                 &     (0.126)                 &     (0.634)                 &     (0.910)                 &     (0.543)                 \\\addlinespace
$ICT_{c,t}$&      -0.057$^{\ast\ast\ast}$&      -0.092                 &      -0.118$^{\ast\ast\ast}$&      -0.039                 &      -1.559$^{\ast\ast}$    &       0.026                 &      -1.797$^{\ast\ast\ast}$&       0.213                 &       1.209                 &      -2.698$^{\ast\ast}$    &       1.526$^{\ast\ast}$    \\
            &     (0.013)                 &     (0.098)                 &     (0.038)                 &     (0.025)                 &     (0.553)                 &     (0.368)                 &     (0.622)                 &     (0.174)                 &     (0.936)                 &     (1.083)                 &     (0.671)                 \\\addlinespace
$R*ICT_{c,t}$&       0.021$^{\ast\ast\ast}$&       0.022                 &       0.047$^{\ast\ast}$    &       0.030$^{\ast\ast}$    &       0.416                 &      -0.200                 &       0.590$^{\ast\ast}$    &       0.026                 &      -0.876$^{\ast\ast}$    &       1.068$^{\ast\ast}$    &      -0.210                 \\
            &     (0.006)                 &     (0.034)                 &     (0.017)                 &     (0.012)                 &     (0.295)                 &     (0.153)                 &     (0.268)                 &     (0.080)                 &     (0.365)                 &     (0.422)                 &     (0.302)                 \\\addlinespace
$wL_{c,t}$&       0.575$^{\ast\ast\ast}$&       0.718$^{\ast}$        &       0.647$^{\ast\ast}$    &       0.592$^{\ast\ast\ast}$&      -0.454$^{\ast\ast\ast}$&       0.052                 &       0.122                 &      -0.627$^{\ast\ast\ast}$&       0.555$^{\ast\ast}$    &       0.799$^{\ast\ast}$    &      -1.388$^{\ast\ast\ast}$\\
            &     (0.167)                 &     (0.357)                 &     (0.274)                 &     (0.151)                 &     (0.157)                 &     (0.111)                 &     (0.135)                 &     (0.094)                 &     (0.245)                 &     (0.380)                 &     (0.253)                 \\\addlinespace
$rK_{c,t}$&       0.087                 &       0.259                 &       0.111                 &       0.050                 &      -0.652$^{\ast\ast\ast}$&      -0.022                 &       0.025                 &      -0.655$^{\ast\ast\ast}$&       0.503$^{\ast\ast}$    &       0.715$^{\ast\ast}$    &      -1.311$^{\ast\ast\ast}$\\
            &     (0.089)                 &     (0.261)                 &     (0.160)                 &     (0.089)                 &     (0.137)                 &     (0.088)                 &     (0.107)                 &     (0.074)                 &     (0.180)                 &     (0.265)                 &     (0.217)                 \\\addlinespace
$pQ_{c,t}$&       0.233                 &      -0.062                 &       0.149                 &       0.290                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.249)                 &     (0.577)                 &     (0.368)                 &     (0.231)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &        .999                 &        .973                 &        .985                 &        .975                 &        .961                 &        .983                 &        .972                 &        .957                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/Tk_alt/Results2RICTint_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.021                 &       0.015                 &       0.030                 &      -0.058                 &       0.023                 &       0.233                 &       0.010                 &      -0.220                 &       0.479                 &      -0.015                 &      -0.901                 \\
            &     (0.015)                 &     (0.025)                 &     (0.076)                 &     (0.034)                 &     (0.522)                 &     (0.405)                 &     (0.245)                 &     (0.238)                 &     (0.925)                 &     (0.496)                 &     (0.776)                 \\\addlinespace
$ICT_{c,t}$&       0.010                 &      -0.007                 &       0.018                 &       0.026                 &       0.233                 &      -0.118                 &       0.090                 &       0.261$^{\ast\ast\ast}$&      -1.274                 &       0.238                 &       0.731                 \\
            &     (0.049)                 &     (0.050)                 &     (0.062)                 &     (0.056)                 &     (0.696)                 &     (0.623)                 &     (0.208)                 &     (0.058)                 &     (1.056)                 &     (0.632)                 &     (0.657)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.027                 &      -0.000                 &      -0.056                 &      -0.035                 &      -0.442                 &      -0.131                 &      -0.195                 &      -0.117                 &       0.399                 &      -0.642                 &      -0.135                 \\
            &     (0.029)                 &     (0.031)                 &     (0.068)                 &     (0.033)                 &     (0.559)                 &     (0.376)                 &     (0.260)                 &     (0.095)                 &     (0.595)                 &     (0.568)                 &     (0.535)                 \\\addlinespace
$wL_{c,t}$&       0.387$^{\ast\ast\ast}$&       0.339                 &       0.997$^{\ast}$        &       0.375$^{\ast\ast\ast}$&      -0.654$^{\ast\ast\ast}$&       0.039                 &       0.095                 &      -0.788$^{\ast\ast\ast}$&       0.715$^{\ast}$        &       0.627$^{\ast}$        &      -1.795$^{\ast\ast\ast}$\\
            &     (0.053)                 &     (0.193)                 &     (0.463)                 &     (0.094)                 &     (0.096)                 &     (0.070)                 &     (0.120)                 &     (0.085)                 &     (0.342)                 &     (0.335)                 &     (0.343)                 \\\addlinespace
$rK_{c,t}$&      -0.038                 &       0.235                 &       0.400                 &      -0.242$^{\ast\ast}$    &      -0.715$^{\ast\ast\ast}$&       0.013                 &       0.061                 &      -0.789$^{\ast\ast\ast}$&       0.722$^{\ast\ast}$    &       0.539$^{\ast}$        &      -1.728$^{\ast\ast\ast}$\\
            &     (0.049)                 &     (0.130)                 &     (0.280)                 &     (0.075)                 &     (0.062)                 &     (0.032)                 &     (0.088)                 &     (0.089)                 &     (0.253)                 &     (0.242)                 &     (0.306)                 \\\addlinespace
$pQ_{c,t}$&       0.293$^{\ast\ast}$    &       0.099                 &      -0.093                 &       0.248$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.098)                 &     (0.351)                 &     (0.462)                 &     (0.128)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.001                 &      -0.003                 &       0.001                 &       0.004$^{\ast\ast}$    &      -0.058                 &      -0.048                 &       0.002                 &      -0.012                 &      -0.077                 &       0.048                 &       0.031                 \\
            &     (0.002)                 &     (0.003)                 &     (0.006)                 &     (0.002)                 &     (0.059)                 &     (0.032)                 &     (0.023)                 &     (0.007)                 &     (0.063)                 &     (0.062)                 &     (0.049)                 \\\addlinespace
$Services_{c,t}$&      -0.003                 &       0.019$^{\ast\ast}$    &       0.019                 &      -0.021$^{\ast\ast}$    &       0.146                 &       0.127$^{\ast}$        &       0.040                 &      -0.020                 &       0.200                 &       0.018                 &      -0.252                 \\
            &     (0.004)                 &     (0.007)                 &     (0.011)                 &     (0.008)                 &     (0.112)                 &     (0.066)                 &     (0.058)                 &     (0.047)                 &     (0.234)                 &     (0.155)                 &     (0.161)                 \\\addlinespace
$HHI_{c,t}$&      -1.236$^{\ast}$        &       1.508                 &       0.348                 &      -3.682$^{\ast\ast}$    &      20.727                 &      14.520                 &       1.263                 &       4.943                 &      16.206                 &      -6.102                 &       3.475                 \\
            &     (0.656)                 &     (1.067)                 &     (2.394)                 &     (1.346)                 &    (14.891)                 &    (13.039)                 &     (6.916)                 &     (9.459)                 &    (36.421)                 &    (23.935)                 &    (34.892)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001$^{\ast}$        &      -0.002$^{\ast}$        &       0.002                 &      -0.001                 &       0.027$^{\ast\ast}$    &      -0.003                 &       0.004                 &       0.026$^{\ast\ast\ast}$&      -0.042                 &      -0.009                 &       0.022                 \\
            &     (0.000)                 &     (0.001)                 &     (0.004)                 &     (0.001)                 &     (0.009)                 &     (0.008)                 &     (0.006)                 &     (0.007)                 &     (0.027)                 &     (0.017)                 &     (0.015)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.020$^{\ast\ast\ast}$&       0.020$^{\ast}$        &      -0.055                 &       0.041$^{\ast\ast\ast}$&      -0.484$^{\ast\ast}$    &      -0.051                 &      -0.097                 &      -0.336$^{\ast\ast}$    &       0.644$^{\ast\ast}$    &       0.045                 &      -0.133                 \\
            &     (0.005)                 &     (0.010)                 &     (0.058)                 &     (0.011)                 &     (0.197)                 &     (0.075)                 &     (0.113)                 &     (0.130)                 &     (0.231)                 &     (0.329)                 &     (0.325)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.002                 &       0.001                 &       0.015$^{\ast}$        &       0.001                 &       0.062                 &       0.011                 &       0.044$^{\ast\ast}$    &       0.007                 &      -0.050                 &       0.100$^{\ast\ast}$    &      -0.088$^{\ast}$        \\
            &     (0.002)                 &     (0.001)                 &     (0.006)                 &     (0.002)                 &     (0.042)                 &     (0.013)                 &     (0.019)                 &     (0.012)                 &     (0.030)                 &     (0.042)                 &     (0.041)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.007                 &       0.023$^{\ast}$        &       0.013                 &      -0.004                 &       0.171                 &       0.111                 &       0.125                 &      -0.064                 &       0.366                 &       0.283                 &      -0.280                 \\
            &     (0.005)                 &     (0.012)                 &     (0.030)                 &     (0.009)                 &     (0.154)                 &     (0.092)                 &     (0.082)                 &     (0.045)                 &     (0.224)                 &     (0.232)                 &     (0.258)                 \\\addlinespace
$XRate_{c,t}$&       0.010                 &      -0.004                 &       0.023                 &       0.020$^{\ast\ast}$    &       0.057                 &      -0.042                 &       0.082                 &       0.017                 &      -0.247                 &       0.239                 &      -0.046                 \\
            &     (0.008)                 &     (0.011)                 &     (0.025)                 &     (0.008)                 &     (0.185)                 &     (0.108)                 &     (0.101)                 &     (0.050)                 &     (0.205)                 &     (0.222)                 &     (0.197)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .998                 &          0.999                &        .988                 &        .994                 &        .959                 &        .984                 &        .992                 &        .967                 &        .982                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/Tk_alt/Results2RICTint_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.023                 &      -0.078                 &      -0.123$^{\ast}$        &       0.020                 &      -0.156                 &      -0.223                 &      -0.303                 &       0.370$^{\ast\ast}$    &      -0.104                 &      -0.798                 &       1.315$^{\ast\ast}$    \\
            &     (0.025)                 &     (0.049)                 &     (0.061)                 &     (0.032)                 &     (0.315)                 &     (0.185)                 &     (0.207)                 &     (0.132)                 &     (0.480)                 &     (0.521)                 &     (0.459)                 \\\addlinespace
$ICT_{c,t}$&      -0.027                 &      -0.163                 &      -0.176                 &      -0.008                 &      -0.109                 &       0.275                 &      -0.522                 &       0.138                 &       0.967                 &      -1.136                 &       0.873                 \\
            &     (0.030)                 &     (0.123)                 &     (0.120)                 &     (0.028)                 &     (0.611)                 &     (0.468)                 &     (0.453)                 &     (0.187)                 &     (1.024)                 &     (1.109)                 &     (0.997)                 \\\addlinespace
$R*ICT_{c,t}$&       0.006                 &       0.036                 &       0.024                 &       0.000                 &       0.083                 &       0.053                 &      -0.024                 &       0.054                 &       0.254                 &      -0.161                 &       0.107                 \\
            &     (0.017)                 &     (0.045)                 &     (0.063)                 &     (0.016)                 &     (0.405)                 &     (0.267)                 &     (0.249)                 &     (0.092)                 &     (0.423)                 &     (0.584)                 &     (0.624)                 \\\addlinespace
$wL_{c,t}$&       0.537$^{\ast\ast}$    &       1.383$^{\ast\ast}$    &       0.132                 &       0.593$^{\ast\ast\ast}$&      -0.645$^{\ast\ast}$    &      -0.129                 &       0.002                 &      -0.517$^{\ast\ast\ast}$&       0.187                 &       0.129                 &      -0.940$^{\ast\ast\ast}$\\
            &     (0.234)                 &     (0.495)                 &     (0.403)                 &     (0.137)                 &     (0.234)                 &     (0.138)                 &     (0.123)                 &     (0.088)                 &     (0.262)                 &     (0.341)                 &     (0.287)                 \\\addlinespace
$rK_{c,t}$&      -0.027                 &       0.288                 &      -0.292                 &       0.162                 &      -0.850$^{\ast\ast\ast}$&      -0.249$^{\ast}$        &      -0.049                 &      -0.552$^{\ast\ast\ast}$&       0.033                 &       0.084                 &      -0.757$^{\ast\ast}$    \\
            &     (0.149)                 &     (0.343)                 &     (0.315)                 &     (0.110)                 &     (0.233)                 &     (0.138)                 &     (0.122)                 &     (0.070)                 &     (0.258)                 &     (0.322)                 &     (0.286)                 \\\addlinespace
$pQ_{c,t}$&       0.509                 &      -0.671                 &       1.081$^{\ast}$        &       0.290                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.354)                 &     (0.801)                 &     (0.529)                 &     (0.213)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.007                 &       0.005                 &       0.004                 &       0.001                 &      -0.063                 &       0.008                 &       0.056$^{\ast}$        &      -0.155                 &      -0.011                 &       0.180$^{\ast}$        \\
            &     (0.003)                 &     (0.004)                 &     (0.011)                 &     (0.003)                 &     (0.055)                 &     (0.038)                 &     (0.037)                 &     (0.027)                 &     (0.092)                 &     (0.089)                 &     (0.089)                 \\\addlinespace
$Services_{c,t}$&       0.003                 &      -0.024                 &      -0.040$^{\ast}$        &      -0.001                 &      -0.030                 &       0.146                 &      -0.174$^{\ast}$        &      -0.002                 &       0.574$^{\ast\ast}$    &      -0.487$^{\ast\ast}$    &      -0.016                 \\
            &     (0.005)                 &     (0.028)                 &     (0.022)                 &     (0.005)                 &     (0.148)                 &     (0.104)                 &     (0.080)                 &     (0.028)                 &     (0.200)                 &     (0.208)                 &     (0.140)                 \\\addlinespace
$HHI_{c,t}$&      -0.346                 &      -1.847                 &      -1.250                 &      -1.663                 &     -18.405                 &      14.996                 &     -16.743                 &     -16.658$^{\ast}$        &      90.039$^{\ast\ast}$    &     -20.624                 &      -5.931                 \\
            &     (0.808)                 &     (2.807)                 &     (3.030)                 &     (0.960)                 &    (30.447)                 &    (20.870)                 &    (13.087)                 &     (7.923)                 &    (33.816)                 &    (30.048)                 &    (39.046)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.000                 &       0.004$^{\ast}$        &      -0.002                 &      -0.000                 &       0.005                 &       0.015                 &      -0.016                 &       0.006                 &       0.008                 &      -0.058$^{\ast}$        &      -0.029                 \\
            &     (0.001)                 &     (0.002)                 &     (0.003)                 &     (0.001)                 &     (0.020)                 &     (0.011)                 &     (0.013)                 &     (0.008)                 &     (0.025)                 &     (0.030)                 &     (0.031)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.004                 &      -0.006                 &       0.021                 &      -0.007$^{\ast}$        &       0.104                 &      -0.077                 &       0.150                 &       0.032                 &      -0.152                 &       0.403                 &       0.250                 \\
            &     (0.010)                 &     (0.012)                 &     (0.022)                 &     (0.004)                 &     (0.190)                 &     (0.134)                 &     (0.117)                 &     (0.066)                 &     (0.308)                 &     (0.285)                 &     (0.279)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.004                 &      -0.005                 &       0.019$^{\ast}$        &       0.000                 &       0.112$^{\ast}$        &       0.020                 &       0.075$^{\ast}$        &       0.017                 &      -0.026                 &       0.131                 &      -0.081                 \\
            &     (0.003)                 &     (0.006)                 &     (0.010)                 &     (0.002)                 &     (0.054)                 &     (0.033)                 &     (0.040)                 &     (0.012)                 &     (0.081)                 &     (0.093)                 &     (0.068)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.007                 &      -0.019                 &       0.034                 &      -0.018$^{\ast}$        &      -0.011                 &       0.039                 &       0.050                 &      -0.100                 &      -0.080                 &       0.291                 &      -0.330                 \\
            &     (0.009)                 &     (0.011)                 &     (0.034)                 &     (0.009)                 &     (0.213)                 &     (0.125)                 &     (0.125)                 &     (0.069)                 &     (0.261)                 &     (0.296)                 &     (0.300)                 \\\addlinespace
$XRate_{c,t}$&      -0.004$^{\ast\ast}$    &      -0.007                 &      -0.005                 &      -0.005$^{\ast\ast}$    &      -0.062                 &       0.003                 &      -0.057$^{\ast\ast}$    &      -0.008                 &       0.156$^{\ast}$        &      -0.107$^{\ast\ast}$    &       0.095$^{\ast\ast}$    \\
            &     (0.001)                 &     (0.006)                 &     (0.007)                 &     (0.002)                 &     (0.044)                 &     (0.033)                 &     (0.022)                 &     (0.011)                 &     (0.080)                 &     (0.049)                 &     (0.037)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .996                 &          0.999                &        .968                 &        .988                 &        .905                 &        .972                 &         .99                 &        .938                 &        .969                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/Tk_alt/Results2RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.031$^{\ast\ast}$    &      -0.039$^{\ast}$        &       0.002                 &      -0.014                 &      -0.406                 &      -0.323                 &      -0.028                 &      -0.055                 &      -0.922                 &      -0.043                 &      -0.202                 \\
            &     (0.013)                 &     (0.019)                 &     (0.046)                 &     (0.021)                 &     (0.332)                 &     (0.226)                 &     (0.166)                 &     (0.127)                 &     (0.598)                 &     (0.393)                 &     (0.515)                 \\\addlinespace
$ICT_{c,t}$&      -0.047$^{\ast\ast\ast}$&      -0.093                 &      -0.150                 &      -0.047$^{\ast}$        &      -0.487                 &       0.022                 &      -0.661$^{\ast}$        &       0.152                 &       1.291                 &      -1.164                 &       1.457$^{\ast\ast}$    \\
            &     (0.015)                 &     (0.095)                 &     (0.088)                 &     (0.024)                 &     (0.378)                 &     (0.353)                 &     (0.347)                 &     (0.165)                 &     (0.903)                 &     (0.919)                 &     (0.608)                 \\\addlinespace
$R*ICT_{c,t}$&       0.014$^{\ast}$        &       0.022                 &       0.049                 &       0.031$^{\ast\ast}$    &       0.059                 &      -0.199                 &       0.219                 &       0.040                 &      -0.893$^{\ast\ast}$    &       0.346                 &      -0.196                 \\
            &     (0.008)                 &     (0.034)                 &     (0.050)                 &     (0.012)                 &     (0.175)                 &     (0.153)                 &     (0.195)                 &     (0.077)                 &     (0.363)                 &     (0.533)                 &     (0.291)                 \\\addlinespace
$wL_{c,t}$&       0.573$^{\ast\ast\ast}$&       0.721$^{\ast}$        &       0.580                 &       0.626$^{\ast\ast\ast}$&      -0.582$^{\ast\ast\ast}$&       0.051                 &      -0.003                 &      -0.630$^{\ast\ast\ast}$&       0.560$^{\ast\ast}$    &       0.146                 &      -1.392$^{\ast\ast\ast}$\\
            &     (0.185)                 &     (0.345)                 &     (0.348)                 &     (0.150)                 &     (0.146)                 &     (0.111)                 &     (0.085)                 &     (0.094)                 &     (0.245)                 &     (0.265)                 &     (0.253)                 \\\addlinespace
$rK_{c,t}$&       0.091                 &       0.260                 &       0.234                 &       0.069                 &      -0.694$^{\ast\ast\ast}$&      -0.022                 &      -0.014                 &      -0.659$^{\ast\ast\ast}$&       0.508$^{\ast\ast}$    &       0.182                 &      -1.315$^{\ast\ast\ast}$\\
            &     (0.095)                 &     (0.256)                 &     (0.242)                 &     (0.091)                 &     (0.124)                 &     (0.088)                 &     (0.075)                 &     (0.073)                 &     (0.178)                 &     (0.211)                 &     (0.216)                 \\\addlinespace
$pQ_{c,t}$&       0.251                 &      -0.066                 &       0.212                 &       0.238                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.278)                 &     (0.561)                 &     (0.614)                 &     (0.220)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.003$^{\ast}$        &      -0.003                 &       0.004                 &      -0.002                 &      -0.030                 &      -0.031                 &       0.004                 &      -0.004                 &      -0.109                 &       0.022                 &      -0.004                 \\
            &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.002)                 &     (0.045)                 &     (0.026)                 &     (0.014)                 &     (0.016)                 &     (0.076)                 &     (0.034)                 &     (0.040)                 \\\addlinespace
$Services_{c,t}$&      -0.002                 &       0.011                 &      -0.006                 &      -0.015$^{\ast\ast}$    &       0.066                 &       0.151$^{\ast}$        &      -0.037                 &      -0.047                 &       0.513$^{\ast\ast}$    &      -0.092                 &      -0.169                 \\
            &     (0.005)                 &     (0.013)                 &     (0.008)                 &     (0.007)                 &     (0.087)                 &     (0.080)                 &     (0.032)                 &     (0.042)                 &     (0.235)                 &     (0.105)                 &     (0.111)                 \\\addlinespace
$HHI_{c,t}$&      -0.387                 &       2.203                 &       0.026                 &      -2.793$^{\ast\ast\ast}$&      12.276                 &      24.999$^{\ast}$        &      -1.860                 &     -10.863                 &      90.046$^{\ast\ast}$    &       1.651                 &     -16.057                 \\
            &     (0.858)                 &     (1.771)                 &     (1.738)                 &     (0.840)                 &    (18.947)                 &    (13.563)                 &     (6.698)                 &     (7.968)                 &    (42.454)                 &    (17.602)                 &    (24.486)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001                 &       0.000                 &       0.001                 &       0.002$^{\ast\ast\ast}$&       0.013                 &      -0.005                 &      -0.000                 &       0.018$^{\ast\ast\ast}$&      -0.062$^{\ast\ast}$    &      -0.022                 &      -0.007                 \\
            &     (0.001)                 &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.012)                 &     (0.007)                 &     (0.008)                 &     (0.004)                 &     (0.024)                 &     (0.019)                 &     (0.012)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.005                 &       0.004                 &      -0.010                 &      -0.012$^{\ast}$        &      -0.169                 &      -0.050                 &      -0.016                 &      -0.103$^{\ast\ast}$    &       0.298                 &       0.088                 &       0.211                 \\
            &     (0.008)                 &     (0.008)                 &     (0.021)                 &     (0.006)                 &     (0.161)                 &     (0.091)                 &     (0.104)                 &     (0.044)                 &     (0.257)                 &     (0.237)                 &     (0.156)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.006$^{\ast\ast\ast}$&      -0.002                 &       0.014$^{\ast\ast}$    &       0.006$^{\ast\ast}$    &       0.099$^{\ast\ast\ast}$&       0.012                 &       0.054$^{\ast\ast}$    &       0.033$^{\ast\ast\ast}$&      -0.029                 &       0.100$^{\ast}$        &      -0.032                 \\
            &     (0.002)                 &     (0.004)                 &     (0.005)                 &     (0.002)                 &     (0.029)                 &     (0.019)                 &     (0.023)                 &     (0.011)                 &     (0.065)                 &     (0.055)                 &     (0.040)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.007                 &       0.009                 &       0.023                 &      -0.003                 &       0.062                 &       0.020                 &       0.101                 &      -0.060                 &       0.055                 &       0.306                 &      -0.182                 \\
            &     (0.007)                 &     (0.009)                 &     (0.022)                 &     (0.006)                 &     (0.178)                 &     (0.106)                 &     (0.080)                 &     (0.062)                 &     (0.274)                 &     (0.191)                 &     (0.221)                 \\\addlinespace
$XRate_{c,t}$&      -0.005$^{\ast\ast\ast}$&      -0.004                 &      -0.006                 &      -0.008$^{\ast\ast\ast}$&      -0.053                 &      -0.002                 &      -0.038                 &      -0.012                 &       0.101                 &      -0.070                 &       0.042                 \\
            &     (0.001)                 &     (0.006)                 &     (0.006)                 &     (0.002)                 &     (0.036)                 &     (0.028)                 &     (0.023)                 &     (0.011)                 &     (0.067)                 &     (0.061)                 &     (0.034)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .996                 &        .999                 &        .965                 &        .985                 &        .887                 &         .96                 &        .983                 &        .916                 &        .956                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/Tk_alt/Results2shortV1_RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.021                 &       0.015                 &       0.030                 &      -0.058                 &       0.023                 &       0.233                 &       0.010                 &      -0.220                 &       0.479                 &      -0.015                 &      -0.901                 \\
            &     (0.015)                 &     (0.025)                 &     (0.076)                 &     (0.034)                 &     (0.522)                 &     (0.405)                 &     (0.245)                 &     (0.238)                 &     (0.925)                 &     (0.496)                 &     (0.776)                 \\\addlinespace
$ICT_{c,t}$&       0.010                 &      -0.007                 &       0.018                 &       0.026                 &       0.233                 &      -0.118                 &       0.090                 &       0.261$^{\ast\ast\ast}$&      -1.274                 &       0.238                 &       0.731                 \\
            &     (0.049)                 &     (0.050)                 &     (0.062)                 &     (0.056)                 &     (0.696)                 &     (0.623)                 &     (0.208)                 &     (0.058)                 &     (1.056)                 &     (0.632)                 &     (0.657)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.027                 &      -0.000                 &      -0.056                 &      -0.035                 &      -0.442                 &      -0.131                 &      -0.195                 &      -0.117                 &       0.399                 &      -0.642                 &      -0.135                 \\
            &     (0.029)                 &     (0.031)                 &     (0.068)                 &     (0.033)                 &     (0.559)                 &     (0.376)                 &     (0.260)                 &     (0.095)                 &     (0.595)                 &     (0.568)                 &     (0.535)                 \\\addlinespace
$wL_{c,t}$&       0.387$^{\ast\ast\ast}$&       0.339                 &       0.997$^{\ast}$        &       0.375$^{\ast\ast\ast}$&      -0.654$^{\ast\ast\ast}$&       0.039                 &       0.095                 &      -0.788$^{\ast\ast\ast}$&       0.715$^{\ast}$        &       0.627$^{\ast}$        &      -1.795$^{\ast\ast\ast}$\\
            &     (0.053)                 &     (0.193)                 &     (0.463)                 &     (0.094)                 &     (0.096)                 &     (0.070)                 &     (0.120)                 &     (0.085)                 &     (0.342)                 &     (0.335)                 &     (0.343)                 \\\addlinespace
$rK_{c,t}$&      -0.038                 &       0.235                 &       0.400                 &      -0.242$^{\ast\ast}$    &      -0.715$^{\ast\ast\ast}$&       0.013                 &       0.061                 &      -0.789$^{\ast\ast\ast}$&       0.722$^{\ast\ast}$    &       0.539$^{\ast}$        &      -1.728$^{\ast\ast\ast}$\\
            &     (0.049)                 &     (0.130)                 &     (0.280)                 &     (0.075)                 &     (0.062)                 &     (0.032)                 &     (0.088)                 &     (0.089)                 &     (0.253)                 &     (0.242)                 &     (0.306)                 \\\addlinespace
$pQ_{c,t}$&       0.293$^{\ast\ast}$    &       0.099                 &      -0.093                 &       0.248$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.098)                 &     (0.351)                 &     (0.462)                 &     (0.128)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
%$R^{2}$  &          0.999                &          0.999                &        .998                 &          0.999                &        .988                 &        .994                 &        .959                 &        .984                 &        .992                 &        .967                 &        .982                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/Tk_alt/Results2shortV1_RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.023                 &      -0.078                 &      -0.123$^{\ast}$        &       0.020                 &      -0.156                 &      -0.223                 &      -0.303                 &       0.370$^{\ast\ast}$    &      -0.104                 &      -0.798                 &       1.315$^{\ast\ast}$    \\
            &     (0.025)                 &     (0.049)                 &     (0.061)                 &     (0.032)                 &     (0.315)                 &     (0.185)                 &     (0.207)                 &     (0.132)                 &     (0.480)                 &     (0.521)                 &     (0.459)                 \\\addlinespace
$ICT_{c,t}$&      -0.027                 &      -0.163                 &      -0.176                 &      -0.008                 &      -0.109                 &       0.275                 &      -0.522                 &       0.138                 &       0.967                 &      -1.136                 &       0.873                 \\
            &     (0.030)                 &     (0.123)                 &     (0.120)                 &     (0.028)                 &     (0.611)                 &     (0.468)                 &     (0.453)                 &     (0.187)                 &     (1.024)                 &     (1.109)                 &     (0.997)                 \\\addlinespace
$R*ICT_{c,t}$&       0.006                 &       0.036                 &       0.024                 &       0.000                 &       0.083                 &       0.053                 &      -0.024                 &       0.054                 &       0.254                 &      -0.161                 &       0.107                 \\
            &     (0.017)                 &     (0.045)                 &     (0.063)                 &     (0.016)                 &     (0.405)                 &     (0.267)                 &     (0.249)                 &     (0.092)                 &     (0.423)                 &     (0.584)                 &     (0.624)                 \\\addlinespace
$wL_{c,t}$&       0.537$^{\ast\ast}$    &       1.383$^{\ast\ast}$    &       0.132                 &       0.593$^{\ast\ast\ast}$&      -0.645$^{\ast\ast}$    &      -0.129                 &       0.002                 &      -0.517$^{\ast\ast\ast}$&       0.187                 &       0.129                 &      -0.940$^{\ast\ast\ast}$\\
            &     (0.234)                 &     (0.495)                 &     (0.403)                 &     (0.137)                 &     (0.234)                 &     (0.138)                 &     (0.123)                 &     (0.088)                 &     (0.262)                 &     (0.341)                 &     (0.287)                 \\\addlinespace
$rK_{c,t}$&      -0.027                 &       0.288                 &      -0.292                 &       0.162                 &      -0.850$^{\ast\ast\ast}$&      -0.249$^{\ast}$        &      -0.049                 &      -0.552$^{\ast\ast\ast}$&       0.033                 &       0.084                 &      -0.757$^{\ast\ast}$    \\
            &     (0.149)                 &     (0.343)                 &     (0.315)                 &     (0.110)                 &     (0.233)                 &     (0.138)                 &     (0.122)                 &     (0.070)                 &     (0.258)                 &     (0.322)                 &     (0.286)                 \\\addlinespace
$pQ_{c,t}$&       0.509                 &      -0.671                 &       1.081$^{\ast}$        &       0.290                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.354)                 &     (0.801)                 &     (0.529)                 &     (0.213)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
%$R^{2}$  &          0.999                &        .998                 &        .996                 &          0.999                &        .968                 &        .988                 &        .905                 &        .972                 &         .99                 &        .938                 &        .969                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/Tk_alt/Results2shortV1_RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.031$^{\ast\ast}$    &      -0.039$^{\ast}$        &       0.002                 &      -0.014                 &      -0.406                 &      -0.323                 &      -0.028                 &      -0.055                 &      -0.922                 &      -0.043                 &      -0.202                 \\
            &     (0.013)                 &     (0.019)                 &     (0.046)                 &     (0.021)                 &     (0.332)                 &     (0.226)                 &     (0.166)                 &     (0.127)                 &     (0.598)                 &     (0.393)                 &     (0.515)                 \\\addlinespace
$ICT_{c,t}$&      -0.047$^{\ast\ast\ast}$&      -0.093                 &      -0.150                 &      -0.047$^{\ast}$        &      -0.487                 &       0.022                 &      -0.661$^{\ast}$        &       0.152                 &       1.291                 &      -1.164                 &       1.457$^{\ast\ast}$    \\
            &     (0.015)                 &     (0.095)                 &     (0.088)                 &     (0.024)                 &     (0.378)                 &     (0.353)                 &     (0.347)                 &     (0.165)                 &     (0.903)                 &     (0.919)                 &     (0.608)                 \\\addlinespace
$R*ICT_{c,t}$&       0.014$^{\ast}$        &       0.022                 &       0.049                 &       0.031$^{\ast\ast}$    &       0.059                 &      -0.199                 &       0.219                 &       0.040                 &      -0.893$^{\ast\ast}$    &       0.346                 &      -0.196                 \\
            &     (0.008)                 &     (0.034)                 &     (0.050)                 &     (0.012)                 &     (0.175)                 &     (0.153)                 &     (0.195)                 &     (0.077)                 &     (0.363)                 &     (0.533)                 &     (0.291)                 \\\addlinespace
$wL_{c,t}$&       0.573$^{\ast\ast\ast}$&       0.721$^{\ast}$        &       0.580                 &       0.626$^{\ast\ast\ast}$&      -0.582$^{\ast\ast\ast}$&       0.051                 &      -0.003                 &      -0.630$^{\ast\ast\ast}$&       0.560$^{\ast\ast}$    &       0.146                 &      -1.392$^{\ast\ast\ast}$\\
            &     (0.185)                 &     (0.345)                 &     (0.348)                 &     (0.150)                 &     (0.146)                 &     (0.111)                 &     (0.085)                 &     (0.094)                 &     (0.245)                 &     (0.265)                 &     (0.253)                 \\\addlinespace
$rK_{c,t}$&       0.091                 &       0.260                 &       0.234                 &       0.069                 &      -0.694$^{\ast\ast\ast}$&      -0.022                 &      -0.014                 &      -0.659$^{\ast\ast\ast}$&       0.508$^{\ast\ast}$    &       0.182                 &      -1.315$^{\ast\ast\ast}$\\
            &     (0.095)                 &     (0.256)                 &     (0.242)                 &     (0.091)                 &     (0.124)                 &     (0.088)                 &     (0.075)                 &     (0.073)                 &     (0.178)                 &     (0.211)                 &     (0.216)                 \\\addlinespace
$pQ_{c,t}$&       0.251                 &      -0.066                 &       0.212                 &       0.238                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.278)                 &     (0.561)                 &     (0.614)                 &     (0.220)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
%$R^{2}$  &          0.999                &        .998                 &        .996                 &        .999                 &        .965                 &        .985                 &        .887                 &         .96                 &        .983                 &        .916                 &        .956                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/Trade_OECD/Results1RICTint_EUKLEMS_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.004                 &       0.005                 &       0.027                 &      -0.021                 &       0.436                 &       0.277                 &       0.236                 &      -0.077                 &       0.232                 &       0.524                 &      -0.728                 \\
            &     (0.020)                 &     (0.021)                 &     (0.056)                 &     (0.028)                 &     (0.803)                 &     (0.353)                 &     (0.522)                 &     (0.342)                 &     (0.800)                 &     (1.152)                 &     (0.961)                 \\\addlinespace
$ICT_{c,t}$&      -0.008                 &       0.008                 &       0.037                 &      -0.044                 &      -0.860                 &      -0.354                 &       0.530$^{\ast}$        &      -1.036$^{\ast}$        &      -0.586                 &       2.581$^{\ast\ast}$    &      -2.002$^{\ast\ast}$    \\
            &     (0.035)                 &     (0.060)                 &     (0.044)                 &     (0.065)                 &     (0.737)                 &     (0.469)                 &     (0.251)                 &     (0.541)                 &     (1.089)                 &     (0.820)                 &     (0.742)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.013                 &      -0.003                 &      -0.042                 &      -0.011                 &       0.156                 &       0.055                 &      -0.172                 &       0.273                 &       0.530                 &      -1.281$^{\ast\ast}$    &       0.683$^{\ast}$        \\
            &     (0.022)                 &     (0.031)                 &     (0.029)                 &     (0.035)                 &     (0.768)                 &     (0.283)                 &     (0.416)                 &     (0.357)                 &     (0.462)                 &     (0.487)                 &     (0.363)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .984                 &        .995                 &        .989                 &        .953                 &        .992                 &        .989                 &        .967                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/Trade_OECD/Results1RICTint_EUKLEMS_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.067$^{\ast\ast}$    &      -0.132$^{\ast}$        &      -0.129$^{\ast\ast\ast}$&      -0.008                 &      -0.929                 &      -0.281                 &      -0.895$^{\ast\ast}$    &       0.247                 &      -0.073                 &      -1.965$^{\ast\ast}$    &       1.193$^{\ast\ast}$    \\
            &     (0.022)                 &     (0.068)                 &     (0.037)                 &     (0.030)                 &     (0.674)                 &     (0.281)                 &     (0.392)                 &     (0.239)                 &     (0.519)                 &     (0.662)                 &     (0.515)                 \\\addlinespace
$ICT_{c,t}$&      -0.002                 &      -0.034                 &      -0.059                 &      -0.001                 &       0.555                 &       0.811$^{\ast\ast}$    &      -0.552                 &       0.297                 &       1.600$^{\ast\ast}$    &      -2.010$^{\ast}$        &       0.110                 \\
            &     (0.020)                 &     (0.081)                 &     (0.043)                 &     (0.020)                 &     (0.586)                 &     (0.292)                 &     (0.464)                 &     (0.194)                 &     (0.667)                 &     (0.939)                 &     (0.547)                 \\\addlinespace
$R*ICT_{c,t}$&       0.001                 &       0.007                 &       0.010                 &       0.007                 &      -0.515                 &      -0.197                 &      -0.172                 &      -0.146                 &      -0.019                 &       0.300                 &       0.057                 \\
            &     (0.018)                 &     (0.035)                 &     (0.033)                 &     (0.014)                 &     (0.596)                 &     (0.260)                 &     (0.393)                 &     (0.129)                 &     (0.355)                 &     (0.639)                 &     (0.565)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .975                 &        .987                 &        .983                 &        .943                 &         .99                 &        .985                 &        .964                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/Trade_OECD/Results1RICTint_EUKLEMS_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.023                 &      -0.051$^{\ast\ast}$    &       0.015                 &      -0.024                 &       0.137                 &      -0.267                 &       0.392                 &       0.012                 &      -0.915                 &       0.821                 &      -0.164                 \\
            &     (0.014)                 &     (0.023)                 &     (0.043)                 &     (0.017)                 &     (0.438)                 &     (0.208)                 &     (0.349)                 &     (0.188)                 &     (0.639)                 &     (0.879)                 &     (0.548)                 \\\addlinespace
$ICT_{c,t}$&      -0.032$^{\ast\ast\ast}$&      -0.039                 &      -0.076$^{\ast\ast}$    &      -0.022                 &      -1.049$^{\ast\ast\ast}$&       0.288                 &      -1.227$^{\ast\ast}$    &      -0.110                 &       1.531                 &      -1.661                 &       0.323                 \\
            &     (0.011)                 &     (0.076)                 &     (0.028)                 &     (0.016)                 &     (0.358)                 &     (0.355)                 &     (0.493)                 &     (0.137)                 &     (0.963)                 &     (1.012)                 &     (0.476)                 \\\addlinespace
$R*ICT_{c,t}$&       0.013                 &       0.005                 &       0.031$^{\ast\ast}$    &       0.026$^{\ast\ast}$    &       0.242                 &      -0.319$^{\ast}$        &       0.363$^{\ast}$        &       0.198$^{\ast}$        &      -1.052$^{\ast\ast\ast}$&       0.579                 &       0.379                 \\
            &     (0.008)                 &     (0.027)                 &     (0.014)                 &     (0.010)                 &     (0.211)                 &     (0.162)                 &     (0.187)                 &     (0.102)                 &     (0.299)                 &     (0.394)                 &     (0.304)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .998                 &        .999                 &        .968                 &        .985                 &        .975                 &        .906                 &        .982                 &        .972                 &        .942                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/Trade_OECD/Results1RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.004                 &       0.009                 &       0.030                 &      -0.022                 &       0.472                 &       0.263                 &       0.286                 &      -0.077                 &       0.178                 &       0.600                 &      -0.753                 \\
            &     (0.020)                 &     (0.018)                 &     (0.058)                 &     (0.028)                 &     (0.801)                 &     (0.355)                 &     (0.547)                 &     (0.346)                 &     (0.820)                 &     (1.212)                 &     (0.981)                 \\\addlinespace
$ICT_{c,t}$&      -0.011                 &      -0.017                 &       0.018                 &      -0.036                 &      -1.071                 &      -0.265                 &       0.199                 &      -1.006                 &      -0.272                 &       2.047$^{\ast\ast\ast}$&      -1.770$^{\ast\ast}$    \\
            &     (0.037)                 &     (0.042)                 &     (0.039)                 &     (0.065)                 &     (0.769)                 &     (0.466)                 &     (0.236)                 &     (0.547)                 &     (0.914)                 &     (0.514)                 &     (0.746)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.011                 &       0.011                 &      -0.031                 &      -0.015                 &       0.254                 &      -0.000                 &       0.008                 &       0.246                 &       0.344                 &      -0.961$^{\ast}$        &       0.541                 \\
            &     (0.022)                 &     (0.021)                 &     (0.027)                 &     (0.036)                 &     (0.800)                 &     (0.292)                 &     (0.511)                 &     (0.365)                 &     (0.412)                 &     (0.456)                 &     (0.400)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .984                 &        .995                 &        .989                 &        .953                 &        .992                 &        .988                 &        .967                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/Trade_OECD/Results1RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.067$^{\ast\ast\ast}$&      -0.135$^{\ast}$        &      -0.127$^{\ast\ast\ast}$&      -0.008                 &      -0.949                 &      -0.302                 &      -0.890$^{\ast\ast}$    &       0.243                 &      -0.102                 &      -1.927$^{\ast\ast}$    &       1.200$^{\ast\ast}$    \\
            &     (0.022)                 &     (0.065)                 &     (0.036)                 &     (0.030)                 &     (0.652)                 &     (0.273)                 &     (0.384)                 &     (0.243)                 &     (0.512)                 &     (0.648)                 &     (0.517)                 \\\addlinespace
$ICT_{c,t}$&      -0.005                 &      -0.103                 &      -0.076                 &      -0.001                 &       0.669                 &       0.903$^{\ast\ast}$    &      -0.648                 &       0.415$^{\ast}$        &       1.838$^{\ast\ast}$    &      -2.406$^{\ast}$        &       0.254                 \\
            &     (0.024)                 &     (0.138)                 &     (0.053)                 &     (0.025)                 &     (0.722)                 &     (0.351)                 &     (0.644)                 &     (0.223)                 &     (0.809)                 &     (1.254)                 &     (0.690)                 \\\addlinespace
$R*ICT_{c,t}$&       0.002                 &       0.032                 &       0.013                 &       0.007                 &      -0.539                 &      -0.181                 &      -0.180                 &      -0.178                 &       0.004                 &       0.319                 &       0.005                 \\
            &     (0.019)                 &     (0.050)                 &     (0.035)                 &     (0.015)                 &     (0.641)                 &     (0.272)                 &     (0.433)                 &     (0.134)                 &     (0.348)                 &     (0.684)                 &     (0.612)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .975                 &        .987                 &        .983                 &        .943                 &         .99                 &        .985                 &        .964                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/Trade_OECD/Results1RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.022                 &      -0.048$^{\ast\ast}$    &       0.017                 &      -0.024                 &       0.150                 &      -0.270                 &       0.405                 &       0.015                 &      -0.938                 &       0.842                 &      -0.166                 \\
            &     (0.014)                 &     (0.022)                 &     (0.043)                 &     (0.017)                 &     (0.438)                 &     (0.206)                 &     (0.346)                 &     (0.188)                 &     (0.632)                 &     (0.875)                 &     (0.542)                 \\\addlinespace
$ICT_{c,t}$&      -0.040$^{\ast\ast\ast}$&      -0.079                 &      -0.094$^{\ast\ast\ast}$&      -0.027                 &      -1.234$^{\ast\ast\ast}$&       0.281                 &      -1.401$^{\ast\ast}$    &      -0.114                 &       1.733                 &      -1.922$^{\ast}$        &       0.428                 \\
            &     (0.011)                 &     (0.108)                 &     (0.031)                 &     (0.018)                 &     (0.421)                 &     (0.375)                 &     (0.517)                 &     (0.186)                 &     (1.027)                 &     (1.042)                 &     (0.591)                 \\\addlinespace
$R*ICT_{c,t}$&       0.015$^{\ast\ast}$    &       0.021                 &       0.037$^{\ast\ast}$    &       0.028$^{\ast\ast}$    &       0.285                 &      -0.311$^{\ast}$        &       0.395$^{\ast}$        &       0.201                 &      -1.105$^{\ast\ast\ast}$&       0.637                 &       0.358                 \\
            &     (0.007)                 &     (0.038)                 &     (0.015)                 &     (0.011)                 &     (0.229)                 &     (0.157)                 &     (0.195)                 &     (0.123)                 &     (0.313)                 &     (0.399)                 &     (0.354)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .998                 &        .999                 &        .968                 &        .985                 &        .975                 &        .906                 &        .982                 &        .972                 &        .942                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/Trade_OECD/Results2RICTint_EUKLEMS_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.013                 &       0.009                 &       0.015                 &      -0.057$^{\ast}$        &       0.096                 &       0.185                 &       0.175                 &      -0.264                 &       0.350                 &       0.597                 &      -0.923                 \\
            &     (0.022)                 &     (0.024)                 &     (0.060)                 &     (0.030)                 &     (0.779)                 &     (0.385)                 &     (0.526)                 &     (0.232)                 &     (0.878)                 &     (0.920)                 &     (0.776)                 \\\addlinespace
$ICT_{c,t}$&       0.026                 &       0.003                 &       0.066                 &       0.028                 &       0.567$^{\ast}$        &      -0.300                 &       0.606$^{\ast}$        &       0.261                 &      -1.880                 &       1.340                 &       0.548                 \\
            &     (0.036)                 &     (0.054)                 &     (0.052)                 &     (0.061)                 &     (0.297)                 &     (0.580)                 &     (0.264)                 &     (0.143)                 &     (1.069)                 &     (0.907)                 &     (0.636)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.025                 &      -0.002                 &      -0.053                 &      -0.036                 &      -0.263                 &       0.030                 &      -0.199                 &      -0.094                 &       0.889$^{\ast\ast}$    &      -0.942                 &      -0.019                 \\
            &     (0.023)                 &     (0.031)                 &     (0.036)                 &     (0.036)                 &     (0.515)                 &     (0.326)                 &     (0.436)                 &     (0.094)                 &     (0.379)                 &     (0.557)                 &     (0.483)                 \\\addlinespace
$wL_{c,t}$&       0.435$^{\ast\ast\ast}$&       0.208                 &       0.649                 &       0.492$^{\ast\ast\ast}$&      -0.636$^{\ast\ast}$    &       0.097                 &       0.030                 &      -0.763$^{\ast\ast\ast}$&       0.865$^{\ast\ast}$    &       0.890$^{\ast}$        &      -1.761$^{\ast\ast\ast}$\\
            &     (0.100)                 &     (0.267)                 &     (0.423)                 &     (0.144)                 &     (0.228)                 &     (0.093)                 &     (0.205)                 &     (0.093)                 &     (0.312)                 &     (0.430)                 &     (0.328)                 \\\addlinespace
$rK_{c,t}$&       0.030                 &       0.157                 &       0.193                 &      -0.184$^{\ast\ast}$    &      -0.705$^{\ast\ast\ast}$&       0.059                 &       0.007                 &      -0.772$^{\ast\ast\ast}$&       0.843$^{\ast\ast}$    &       0.851$^{\ast\ast}$    &      -1.701$^{\ast\ast\ast}$\\
            &     (0.072)                 &     (0.124)                 &     (0.230)                 &     (0.071)                 &     (0.177)                 &     (0.076)                 &     (0.158)                 &     (0.092)                 &     (0.294)                 &     (0.326)                 &     (0.291)                 \\\addlinespace
$pQ_{c,t}$&       0.124                 &       0.464                 &      -0.218                 &      -0.008                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.190)                 &     (0.475)                 &     (0.722)                 &     (0.208)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.001                 &      -0.004                 &       0.002                 &       0.005$^{\ast\ast\ast}$&      -0.089                 &      -0.054                 &      -0.020                 &      -0.015$^{\ast}$        &      -0.094                 &       0.064                 &       0.028                 \\
            &     (0.001)                 &     (0.003)                 &     (0.004)                 &     (0.001)                 &     (0.055)                 &     (0.030)                 &     (0.030)                 &     (0.007)                 &     (0.055)                 &     (0.064)                 &     (0.053)                 \\\addlinespace
$Services_{c,t}$&      -0.001                 &       0.020$^{\ast}$        &       0.010                 &      -0.023$^{\ast\ast}$    &       0.189                 &       0.082                 &       0.148                 &      -0.041                 &       0.096                 &       0.181                 &      -0.277                 \\
            &     (0.005)                 &     (0.009)                 &     (0.013)                 &     (0.010)                 &     (0.194)                 &     (0.076)                 &     (0.161)                 &     (0.047)                 &     (0.232)                 &     (0.284)                 &     (0.184)                 \\\addlinespace
$HHI_{c,t}$&      -0.599                 &       0.343                 &       2.622                 &      -3.546$^{\ast}$        &       3.754                 &      -7.745                 &      17.121                 &      -5.622                 &     -42.836                 &      55.907                 &     -10.408                 \\
            &     (0.827)                 &     (1.929)                 &     (2.713)                 &     (1.878)                 &    (34.771)                 &    (16.761)                 &    (28.425)                 &    (11.141)                 &    (48.239)                 &    (54.461)                 &    (40.483)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast}$        &       0.001                 &      -0.001                 &       0.041$^{\ast\ast}$    &      -0.006                 &       0.023                 &       0.024$^{\ast\ast\ast}$&      -0.052                 &       0.035                 &       0.020                 \\
            &     (0.001)                 &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.015)                 &     (0.007)                 &     (0.016)                 &     (0.006)                 &     (0.032)                 &     (0.036)                 &     (0.018)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.014$^{\ast}$        &       0.012                 &      -0.023                 &       0.045$^{\ast\ast\ast}$&      -0.784$^{\ast\ast}$    &      -0.016                 &      -0.446$^{\ast\ast}$    &      -0.322$^{\ast\ast}$    &       0.743$^{\ast\ast}$    &      -0.688                 &      -0.112                 \\
            &     (0.007)                 &     (0.009)                 &     (0.026)                 &     (0.012)                 &     (0.276)                 &     (0.079)                 &     (0.178)                 &     (0.120)                 &     (0.252)                 &     (0.381)                 &     (0.321)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003$^{\ast}$        &       0.001                 &       0.008$^{\ast}$        &       0.001                 &       0.093$^{\ast\ast}$    &       0.014                 &       0.071$^{\ast}$        &       0.009                 &      -0.041                 &       0.118$^{\ast}$        &      -0.086$^{\ast}$        \\
            &     (0.001)                 &     (0.002)                 &     (0.004)                 &     (0.002)                 &     (0.039)                 &     (0.011)                 &     (0.036)                 &     (0.009)                 &     (0.042)                 &     (0.058)                 &     (0.044)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.004                 &       0.025$^{\ast}$        &      -0.007                 &      -0.005                 &       0.172                 &       0.155                 &       0.055                 &      -0.037                 &       0.530$^{\ast}$        &      -0.264                 &      -0.249                 \\
            &     (0.006)                 &     (0.012)                 &     (0.021)                 &     (0.009)                 &     (0.183)                 &     (0.087)                 &     (0.142)                 &     (0.058)                 &     (0.242)                 &     (0.341)                 &     (0.236)                 \\\addlinespace
$Imports^{\%GDP}_{c,t}$&       0.002                 &      -0.007$^{\ast}$        &       0.010                 &       0.004                 &      -0.042                 &      -0.029                 &       0.011                 &      -0.024                 &      -0.121                 &       0.138                 &      -0.027                 \\
            &     (0.002)                 &     (0.003)                 &     (0.010)                 &     (0.002)                 &     (0.036)                 &     (0.028)                 &     (0.044)                 &     (0.018)                 &     (0.096)                 &     (0.117)                 &     (0.069)                 \\\addlinespace
$Exports^{\%GDP}_{c,t}$&      -0.002                 &       0.007$^{\ast\ast}$    &      -0.012                 &      -0.003                 &       0.057                 &       0.061$^{\ast\ast}$    &      -0.041                 &       0.037                 &       0.196                 &      -0.242                 &       0.044                 \\
            &     (0.003)                 &     (0.003)                 &     (0.011)                 &     (0.004)                 &     (0.073)                 &     (0.025)                 &     (0.069)                 &     (0.024)                 &     (0.127)                 &     (0.166)                 &     (0.078)                 \\\addlinespace
$XRate_{c,t}$&       0.008                 &      -0.001                 &       0.017                 &       0.018$^{\ast}$        &       0.054                 &      -0.062                 &       0.099                 &       0.017                 &      -0.293$^{\ast}$        &       0.365                 &      -0.065                 \\
            &     (0.007)                 &     (0.010)                 &     (0.013)                 &     (0.008)                 &     (0.222)                 &     (0.085)                 &     (0.195)                 &     (0.043)                 &     (0.131)                 &     (0.260)                 &     (0.186)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .986                 &        .995                 &        .989                 &        .985                 &        .992                 &        .989                 &        .982                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/Trade_OECD/Results2RICTint_EUKLEMS_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.041$^{\ast}$        &      -0.066                 &      -0.111$^{\ast\ast\ast}$&       0.020                 &      -0.688                 &      -0.209                 &      -0.854$^{\ast\ast}$    &       0.374$^{\ast\ast}$    &      -0.050                 &      -2.053$^{\ast\ast}$    &       1.329$^{\ast\ast}$    \\
            &     (0.021)                 &     (0.050)                 &     (0.033)                 &     (0.032)                 &     (0.388)                 &     (0.190)                 &     (0.382)                 &     (0.131)                 &     (0.488)                 &     (0.765)                 &     (0.455)                 \\\addlinespace
$ICT_{c,t}$&      -0.032                 &      -0.075                 &      -0.086$^{\ast}$        &      -0.011                 &      -0.600                 &       0.355                 &      -1.084$^{\ast}$        &       0.129                 &       0.982                 &      -2.325$^{\ast}$        &       0.712                 \\
            &     (0.022)                 &     (0.069)                 &     (0.045)                 &     (0.022)                 &     (0.566)                 &     (0.405)                 &     (0.569)                 &     (0.160)                 &     (0.871)                 &     (1.188)                 &     (0.819)                 \\\addlinespace
$R*ICT_{c,t}$&       0.005                 &       0.003                 &       0.015                 &       0.002                 &       0.003                 &      -0.026                 &      -0.037                 &       0.066                 &       0.102                 &       0.212                 &       0.175                 \\
            &     (0.017)                 &     (0.030)                 &     (0.030)                 &     (0.015)                 &     (0.548)                 &     (0.273)                 &     (0.387)                 &     (0.098)                 &     (0.436)                 &     (0.668)                 &     (0.617)                 \\\addlinespace
$wL_{c,t}$&       0.553$^{\ast\ast}$    &       1.375$^{\ast\ast}$    &       0.370                 &       0.592$^{\ast\ast\ast}$&      -0.561$^{\ast\ast}$    &      -0.108                 &       0.100                 &      -0.553$^{\ast\ast\ast}$&       0.242                 &       0.640$^{\ast}$        &      -1.048$^{\ast\ast\ast}$\\
            &     (0.208)                 &     (0.507)                 &     (0.308)                 &     (0.136)                 &     (0.199)                 &     (0.134)                 &     (0.161)                 &     (0.071)                 &     (0.238)                 &     (0.322)                 &     (0.279)                 \\\addlinespace
$rK_{c,t}$&      -0.039                 &       0.202                 &      -0.079                 &       0.149                 &      -0.863$^{\ast\ast\ast}$&      -0.231                 &      -0.052                 &      -0.579$^{\ast\ast\ast}$&       0.060                 &       0.528$^{\ast}$        &      -0.841$^{\ast\ast}$    \\
            &     (0.130)                 &     (0.298)                 &     (0.165)                 &     (0.113)                 &     (0.218)                 &     (0.139)                 &     (0.153)                 &     (0.056)                 &     (0.258)                 &     (0.272)                 &     (0.285)                 \\\addlinespace
$pQ_{c,t}$&       0.475                 &      -0.542                 &       0.630                 &       0.309                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.298)                 &     (0.748)                 &     (0.427)                 &     (0.213)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.000                 &      -0.000                 &      -0.002                 &       0.004                 &       0.015                 &      -0.041                 &       0.024                 &       0.033                 &      -0.093                 &      -0.037                 &       0.112                 \\
            &     (0.002)                 &     (0.005)                 &     (0.004)                 &     (0.003)                 &     (0.046)                 &     (0.040)                 &     (0.037)                 &     (0.027)                 &     (0.099)                 &     (0.081)                 &     (0.088)                 \\\addlinespace
$Services_{c,t}$&      -0.000                 &      -0.029                 &      -0.016$^{\ast}$        &      -0.001                 &      -0.099                 &       0.137                 &      -0.248$^{\ast}$        &       0.012                 &       0.523$^{\ast\ast}$    &      -0.610$^{\ast\ast}$    &       0.027                 \\
            &     (0.004)                 &     (0.031)                 &     (0.009)                 &     (0.005)                 &     (0.144)                 &     (0.099)                 &     (0.116)                 &     (0.033)                 &     (0.179)                 &     (0.249)                 &     (0.130)                 \\\addlinespace
$HHI_{c,t}$&      -0.815                 &      -3.790                 &      -2.302                 &      -1.813$^{\ast}$        &     -44.222                 &      17.670                 &     -37.918$^{\ast\ast}$    &     -23.974$^{\ast}$        &      82.333$^{\ast\ast\ast}$&     -53.053                 &     -25.774                 \\
            &     (0.645)                 &     (4.483)                 &     (2.054)                 &     (0.913)                 &    (26.156)                 &    (16.126)                 &    (14.648)                 &    (11.832)                 &    (25.772)                 &    (39.131)                 &    (36.458)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001                 &       0.004                 &       0.002                 &      -0.000                 &       0.034                 &       0.013                 &       0.014                 &       0.007                 &       0.003                 &       0.010                 &      -0.026                 \\
            &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.001)                 &     (0.019)                 &     (0.013)                 &     (0.015)                 &     (0.008)                 &     (0.027)                 &     (0.032)                 &     (0.033)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.005                 &      -0.011                 &       0.002                 &      -0.007                 &       0.141                 &      -0.093                 &       0.187                 &       0.047                 &      -0.185                 &       0.451                 &       0.295                 \\
            &     (0.008)                 &     (0.012)                 &     (0.010)                 &     (0.004)                 &     (0.176)                 &     (0.135)                 &     (0.109)                 &     (0.067)                 &     (0.313)                 &     (0.284)                 &     (0.269)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.004                 &      -0.003                 &       0.006                 &       0.000                 &       0.137                 &       0.024                 &       0.097                 &       0.016                 &      -0.007                 &       0.085                 &      -0.085                 \\
            &     (0.003)                 &     (0.005)                 &     (0.006)                 &     (0.002)                 &     (0.083)                 &     (0.033)                 &     (0.078)                 &     (0.010)                 &     (0.082)                 &     (0.130)                 &     (0.087)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.003                 &      -0.001                 &       0.014                 &      -0.018$^{\ast}$        &      -0.051                 &       0.063                 &      -0.012                 &      -0.102                 &       0.043                 &       0.187                 &      -0.342                 \\
            &     (0.008)                 &     (0.011)                 &     (0.016)                 &     (0.009)                 &     (0.235)                 &     (0.136)                 &     (0.206)                 &     (0.064)                 &     (0.305)                 &     (0.396)                 &     (0.297)                 \\\addlinespace
$Imports^{\%GDP}_{c,t}$&      -0.002                 &      -0.018                 &       0.001                 &      -0.001                 &      -0.018                 &      -0.032                 &      -0.010                 &       0.024                 &      -0.136                 &       0.023                 &       0.070                 \\
            &     (0.003)                 &     (0.011)                 &     (0.006)                 &     (0.003)                 &     (0.075)                 &     (0.034)                 &     (0.061)                 &     (0.030)                 &     (0.093)                 &     (0.093)                 &     (0.067)                 \\\addlinespace
$Exports^{\%GDP}_{c,t}$&       0.000                 &       0.012                 &      -0.002                 &       0.001                 &      -0.001                 &       0.005                 &      -0.014                 &       0.008                 &       0.073                 &      -0.052                 &       0.022                 \\
            &     (0.002)                 &     (0.010)                 &     (0.007)                 &     (0.003)                 &     (0.068)                 &     (0.037)                 &     (0.060)                 &     (0.027)                 &     (0.087)                 &     (0.113)                 &     (0.090)                 \\\addlinespace
$XRate_{c,t}$&      -0.004$^{\ast\ast}$    &      -0.002                 &      -0.009$^{\ast\ast}$    &      -0.005$^{\ast\ast}$    &      -0.110$^{\ast}$        &      -0.001                 &      -0.106$^{\ast\ast}$    &      -0.003                 &       0.151                 &      -0.187$^{\ast\ast}$    &       0.101                 \\
            &     (0.002)                 &     (0.007)                 &     (0.004)                 &     (0.002)                 &     (0.052)                 &     (0.037)                 &     (0.045)                 &     (0.011)                 &     (0.088)                 &     (0.080)                 &     (0.057)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .982                 &        .988                 &        .984                 &        .975                 &         .99                 &        .986                 &         .97                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/Trade_OECD/Results2RICTint_EUKLEMS_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.018$^{\ast}$        &      -0.041$^{\ast}$        &       0.023                 &      -0.021                 &      -0.016                 &      -0.296                 &       0.358                 &      -0.078                 &      -0.874                 &       0.876                 &      -0.293                 \\
            &     (0.009)                 &     (0.020)                 &     (0.042)                 &     (0.017)                 &     (0.381)                 &     (0.200)                 &     (0.346)                 &     (0.123)                 &     (0.610)                 &     (0.902)                 &     (0.454)                 \\\addlinespace
$ICT_{c,t}$&      -0.053$^{\ast\ast\ast}$&      -0.052                 &      -0.096$^{\ast\ast}$    &      -0.049$^{\ast\ast\ast}$&      -1.264$^{\ast\ast\ast}$&       0.127                 &      -1.513$^{\ast\ast\ast}$&       0.123                 &       1.171                 &      -2.233$^{\ast\ast}$    &       1.147$^{\ast\ast}$    \\
            &     (0.010)                 &     (0.065)                 &     (0.035)                 &     (0.017)                 &     (0.382)                 &     (0.338)                 &     (0.525)                 &     (0.119)                 &     (0.904)                 &     (0.981)                 &     (0.413)                 \\\addlinespace
$R*ICT_{c,t}$&       0.019$^{\ast\ast\ast}$&       0.007                 &       0.036$^{\ast\ast}$    &       0.034$^{\ast\ast\ast}$&       0.266                 &      -0.264                 &       0.467$^{\ast\ast}$    &       0.063                 &      -0.885$^{\ast\ast}$    &       0.839$^{\ast\ast}$    &      -0.017                 \\
            &     (0.005)                 &     (0.022)                 &     (0.016)                 &     (0.009)                 &     (0.215)                 &     (0.154)                 &     (0.209)                 &     (0.063)                 &     (0.398)                 &     (0.372)                 &     (0.236)                 \\\addlinespace
$wL_{c,t}$&       0.560$^{\ast\ast\ast}$&       0.736$^{\ast}$        &       0.688$^{\ast\ast}$    &       0.552$^{\ast\ast\ast}$&      -0.448$^{\ast\ast\ast}$&       0.039                 &       0.141                 &      -0.629$^{\ast\ast\ast}$&       0.544$^{\ast\ast}$    &       0.822$^{\ast\ast}$    &      -1.399$^{\ast\ast\ast}$\\
            &     (0.159)                 &     (0.351)                 &     (0.303)                 &     (0.107)                 &     (0.150)                 &     (0.106)                 &     (0.111)                 &     (0.086)                 &     (0.227)                 &     (0.342)                 &     (0.214)                 \\\addlinespace
$rK_{c,t}$&       0.066                 &       0.290                 &       0.159                 &      -0.019                 &      -0.639$^{\ast\ast\ast}$&      -0.024                 &       0.046                 &      -0.662$^{\ast\ast\ast}$&       0.503$^{\ast\ast\ast}$&       0.747$^{\ast\ast\ast}$&      -1.337$^{\ast\ast\ast}$\\
            &     (0.095)                 &     (0.275)                 &     (0.184)                 &     (0.073)                 &     (0.128)                 &     (0.083)                 &     (0.090)                 &     (0.068)                 &     (0.164)                 &     (0.242)                 &     (0.191)                 \\\addlinespace
$pQ_{c,t}$&       0.284                 &      -0.107                 &       0.111                 &       0.379$^{\ast\ast}$    &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.248)                 &     (0.603)                 &     (0.445)                 &     (0.155)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.003                 &       0.005$^{\ast}$        &      -0.001                 &       0.001                 &      -0.039                 &       0.040                 &      -0.000                 &      -0.115                 &       0.132                 &       0.004                 \\
            &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.002)                 &     (0.045)                 &     (0.028)                 &     (0.027)                 &     (0.014)                 &     (0.071)                 &     (0.078)                 &     (0.036)                 \\\addlinespace
$Services_{c,t}$&      -0.002                 &       0.011                 &      -0.013                 &      -0.014$^{\ast\ast}$    &      -0.005                 &       0.162$^{\ast}$        &      -0.112                 &      -0.055                 &       0.527$^{\ast\ast}$    &      -0.334                 &      -0.207$^{\ast}$        \\
            &     (0.004)                 &     (0.014)                 &     (0.011)                 &     (0.006)                 &     (0.093)                 &     (0.079)                 &     (0.106)                 &     (0.041)                 &     (0.236)                 &     (0.287)                 &     (0.101)                 \\\addlinespace
$HHI_{c,t}$&      -0.416                 &       2.453                 &      -1.393                 &      -3.771$^{\ast\ast\ast}$&      15.803                 &      40.343$^{\ast\ast}$    &      -2.580                 &     -21.960$^{\ast\ast}$    &     103.829$^{\ast\ast}$    &     -22.236                 &     -66.549$^{\ast\ast\ast}$\\
            &     (0.538)                 &     (1.869)                 &     (1.986)                 &     (1.034)                 &    (22.125)                 &    (14.712)                 &    (20.226)                 &     (9.149)                 &    (46.577)                 &    (58.572)                 &    (23.010)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001$^{\ast\ast\ast}$&       0.000                 &       0.004$^{\ast\ast}$    &       0.002$^{\ast\ast\ast}$&       0.049$^{\ast\ast\ast}$&      -0.005                 &       0.035$^{\ast\ast}$    &       0.018$^{\ast\ast\ast}$&      -0.063$^{\ast\ast}$    &       0.057                 &      -0.004                 \\
            &     (0.000)                 &     (0.001)                 &     (0.001)                 &     (0.001)                 &     (0.013)                 &     (0.008)                 &     (0.013)                 &     (0.004)                 &     (0.025)                 &     (0.036)                 &     (0.012)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.009                 &       0.004                 &      -0.019                 &      -0.014$^{\ast\ast}$    &      -0.279                 &      -0.021                 &      -0.134                 &      -0.123$^{\ast\ast}$    &       0.324                 &      -0.185                 &       0.127                 \\
            &     (0.007)                 &     (0.009)                 &     (0.015)                 &     (0.005)                 &     (0.188)                 &     (0.090)                 &     (0.152)                 &     (0.046)                 &     (0.237)                 &     (0.386)                 &     (0.142)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.005$^{\ast\ast\ast}$&      -0.002                 &       0.004                 &       0.006$^{\ast\ast}$    &       0.113$^{\ast\ast\ast}$&       0.012                 &       0.068                 &       0.034$^{\ast\ast}$    &      -0.029                 &       0.042                 &      -0.028                 \\
            &     (0.001)                 &     (0.004)                 &     (0.004)                 &     (0.002)                 &     (0.035)                 &     (0.019)                 &     (0.041)                 &     (0.012)                 &     (0.061)                 &     (0.092)                 &     (0.049)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.008                 &       0.010                 &       0.002                 &      -0.001                 &       0.047                 &       0.034                 &       0.084                 &      -0.071                 &       0.068                 &       0.057                 &      -0.251                 \\
            &     (0.005)                 &     (0.010)                 &     (0.015)                 &     (0.007)                 &     (0.189)                 &     (0.102)                 &     (0.164)                 &     (0.064)                 &     (0.292)                 &     (0.347)                 &     (0.193)                 \\\addlinespace
$Imports^{\%GDP}_{c,t}$&      -0.002                 &       0.001                 &       0.001                 &      -0.005$^{\ast}$        &       0.005                 &       0.026                 &      -0.010                 &      -0.011                 &       0.020                 &       0.004                 &      -0.022                 \\
            &     (0.002)                 &     (0.002)                 &     (0.005)                 &     (0.002)                 &     (0.054)                 &     (0.022)                 &     (0.053)                 &     (0.014)                 &     (0.066)                 &     (0.091)                 &     (0.046)                 \\\addlinespace
$Exports^{\%GDP}_{c,t}$&       0.000                 &      -0.001                 &      -0.005                 &       0.005$^{\ast\ast}$    &      -0.064                 &      -0.048$^{\ast}$        &      -0.046                 &       0.030$^{\ast\ast}$    &      -0.041                 &      -0.108                 &       0.119$^{\ast\ast\ast}$\\
            &     (0.001)                 &     (0.002)                 &     (0.005)                 &     (0.002)                 &     (0.053)                 &     (0.025)                 &     (0.045)                 &     (0.013)                 &     (0.069)                 &     (0.087)                 &     (0.034)                 \\\addlinespace
$XRate_{c,t}$&      -0.004$^{\ast\ast\ast}$&      -0.002                 &      -0.004                 &      -0.006$^{\ast\ast\ast}$&      -0.090$^{\ast\ast\ast}$&      -0.009                 &      -0.075$^{\ast\ast}$    &      -0.005                 &       0.078                 &      -0.098                 &       0.063$^{\ast\ast}$    \\
            &     (0.001)                 &     (0.005)                 &     (0.003)                 &     (0.002)                 &     (0.031)                 &     (0.029)                 &     (0.027)                 &     (0.011)                 &     (0.064)                 &     (0.070)                 &     (0.029)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &        .999                 &        .974                 &        .986                 &        .976                 &        .962                 &        .983                 &        .973                 &         .96                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/Trade_OECD/Results2RICTint_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.012                 &       0.014                 &       0.019                 &      -0.058$^{\ast}$        &       0.150                 &       0.168                 &       0.241                 &      -0.258                 &       0.274                 &       0.693                 &      -0.947                 \\
            &     (0.022)                 &     (0.022)                 &     (0.063)                 &     (0.030)                 &     (0.787)                 &     (0.386)                 &     (0.548)                 &     (0.233)                 &     (0.903)                 &     (0.966)                 &     (0.776)                 \\\addlinespace
$ICT_{c,t}$&       0.022                 &      -0.022                 &       0.046                 &       0.031                 &       0.247                 &      -0.213                 &       0.231                 &       0.229$^{\ast\ast}$    &      -1.469$^{\ast}$        &       0.799                 &       0.689                 \\
            &     (0.036)                 &     (0.042)                 &     (0.042)                 &     (0.059)                 &     (0.422)                 &     (0.552)                 &     (0.297)                 &     (0.091)                 &     (0.771)                 &     (0.479)                 &     (0.641)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.023                 &       0.012                 &      -0.042                 &      -0.037                 &      -0.099                 &      -0.021                 &      -0.004                 &      -0.074                 &       0.647$^{\ast}$        &      -0.645                 &      -0.082                 \\
            &     (0.023)                 &     (0.025)                 &     (0.033)                 &     (0.036)                 &     (0.593)                 &     (0.321)                 &     (0.544)                 &     (0.090)                 &     (0.293)                 &     (0.534)                 &     (0.489)                 \\\addlinespace
$wL_{c,t}$&       0.433$^{\ast\ast\ast}$&       0.197                 &       0.642                 &       0.494$^{\ast\ast\ast}$&      -0.628$^{\ast\ast}$    &       0.095                 &       0.039                 &      -0.762$^{\ast\ast\ast}$&       0.857$^{\ast\ast}$    &       0.902$^{\ast}$        &      -1.764$^{\ast\ast\ast}$\\
            &     (0.100)                 &     (0.267)                 &     (0.418)                 &     (0.143)                 &     (0.232)                 &     (0.092)                 &     (0.209)                 &     (0.092)                 &     (0.313)                 &     (0.439)                 &     (0.329)                 \\\addlinespace
$rK_{c,t}$&       0.033                 &       0.163                 &       0.202                 &      -0.183$^{\ast\ast}$    &      -0.694$^{\ast\ast\ast}$&       0.056                 &       0.021                 &      -0.770$^{\ast\ast\ast}$&       0.829$^{\ast\ast}$    &       0.870$^{\ast\ast}$    &      -1.705$^{\ast\ast\ast}$\\
            &     (0.072)                 &     (0.125)                 &     (0.235)                 &     (0.069)                 &     (0.183)                 &     (0.075)                 &     (0.164)                 &     (0.091)                 &     (0.293)                 &     (0.336)                 &     (0.292)                 \\\addlinespace
$pQ_{c,t}$&       0.124                 &       0.482                 &      -0.211                 &      -0.013                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.189)                 &     (0.474)                 &     (0.719)                 &     (0.205)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.001                 &      -0.004                 &       0.002                 &       0.005$^{\ast\ast\ast}$&      -0.089                 &      -0.054                 &      -0.019                 &      -0.015$^{\ast}$        &      -0.094                 &       0.064                 &       0.027                 \\
            &     (0.001)                 &     (0.002)                 &     (0.004)                 &     (0.001)                 &     (0.053)                 &     (0.030)                 &     (0.031)                 &     (0.007)                 &     (0.054)                 &     (0.065)                 &     (0.052)                 \\\addlinespace
$Services_{c,t}$&      -0.001                 &       0.020$^{\ast}$        &       0.011                 &      -0.023$^{\ast\ast}$    &       0.193                 &       0.081                 &       0.153                 &      -0.040                 &       0.088                 &       0.188                 &      -0.276                 \\
            &     (0.005)                 &     (0.009)                 &     (0.013)                 &     (0.010)                 &     (0.196)                 &     (0.075)                 &     (0.163)                 &     (0.047)                 &     (0.235)                 &     (0.287)                 &     (0.185)                 \\\addlinespace
$HHI_{c,t}$&      -0.599                 &       0.238                 &       2.578                 &      -3.518$^{\ast}$        &       2.585                 &      -7.504                 &      15.706                 &      -5.617                 &     -41.965                 &      54.074                 &      -9.381                 \\
            &     (0.831)                 &     (1.998)                 &     (2.746)                 &     (1.884)                 &    (34.614)                 &    (16.779)                 &    (28.147)                 &    (11.123)                 &    (49.692)                 &    (54.626)                 &    (40.365)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast}$        &       0.001                 &      -0.001                 &       0.041$^{\ast\ast}$    &      -0.006                 &       0.023                 &       0.024$^{\ast\ast\ast}$&      -0.052                 &       0.035                 &       0.019                 \\
            &     (0.001)                 &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.015)                 &     (0.007)                 &     (0.016)                 &     (0.006)                 &     (0.031)                 &     (0.036)                 &     (0.018)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.014$^{\ast}$        &       0.012                 &      -0.023                 &       0.046$^{\ast\ast\ast}$&      -0.776$^{\ast\ast}$    &      -0.019                 &      -0.436$^{\ast\ast}$    &      -0.321$^{\ast\ast}$    &       0.729$^{\ast\ast}$    &      -0.673                 &      -0.114                 \\
            &     (0.007)                 &     (0.009)                 &     (0.026)                 &     (0.012)                 &     (0.276)                 &     (0.078)                 &     (0.178)                 &     (0.120)                 &     (0.244)                 &     (0.370)                 &     (0.320)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003$^{\ast\ast}$    &       0.001                 &       0.008$^{\ast}$        &       0.001                 &       0.094$^{\ast\ast}$    &       0.014                 &       0.072$^{\ast}$        &       0.009                 &      -0.042                 &       0.120$^{\ast}$        &      -0.087$^{\ast}$        \\
            &     (0.001)                 &     (0.002)                 &     (0.004)                 &     (0.002)                 &     (0.038)                 &     (0.011)                 &     (0.036)                 &     (0.009)                 &     (0.042)                 &     (0.058)                 &     (0.044)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.004                 &       0.025$^{\ast}$        &      -0.006                 &      -0.005                 &       0.180                 &       0.151                 &       0.064                 &      -0.035                 &       0.514$^{\ast}$        &      -0.250                 &      -0.246                 \\
            &     (0.006)                 &     (0.012)                 &     (0.020)                 &     (0.009)                 &     (0.178)                 &     (0.087)                 &     (0.144)                 &     (0.058)                 &     (0.253)                 &     (0.339)                 &     (0.240)                 \\\addlinespace
$XRate_{c,t}$&       0.008                 &      -0.003                 &       0.015                 &       0.018$^{\ast}$        &       0.030                 &      -0.055                 &       0.069                 &       0.015                 &      -0.260$^{\ast}$        &       0.317                 &      -0.049                 \\
            &     (0.007)                 &     (0.010)                 &     (0.013)                 &     (0.008)                 &     (0.239)                 &     (0.088)                 &     (0.214)                 &     (0.044)                 &     (0.125)                 &     (0.258)                 &     (0.186)                 \\\addlinespace
$Imports^{\%GDP}_{c,t}$&       0.002                 &      -0.007$^{\ast}$        &       0.009                 &       0.004                 &      -0.042                 &      -0.029                 &       0.011                 &      -0.024                 &      -0.120                 &       0.138                 &      -0.028                 \\
            &     (0.002)                 &     (0.003)                 &     (0.010)                 &     (0.002)                 &     (0.037)                 &     (0.028)                 &     (0.044)                 &     (0.018)                 &     (0.096)                 &     (0.117)                 &     (0.070)                 \\\addlinespace
$Exports^{\%GDP}_{c,t}$&      -0.002                 &       0.007$^{\ast\ast}$    &      -0.012                 &      -0.003                 &       0.058                 &       0.061$^{\ast\ast}$    &      -0.040                 &       0.037                 &       0.195                 &      -0.241                 &       0.044                 \\
            &     (0.003)                 &     (0.003)                 &     (0.011)                 &     (0.004)                 &     (0.074)                 &     (0.025)                 &     (0.070)                 &     (0.024)                 &     (0.128)                 &     (0.166)                 &     (0.078)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .986                 &        .995                 &        .989                 &        .985                 &        .992                 &        .989                 &        .982                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/Trade_OECD/Results2RICTint_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.040$^{\ast}$        &      -0.068                 &      -0.110$^{\ast\ast\ast}$&       0.020                 &      -0.683                 &      -0.220                 &      -0.836$^{\ast\ast}$    &       0.372$^{\ast\ast}$    &      -0.067                 &      -2.006$^{\ast\ast}$    &       1.321$^{\ast\ast}$    \\
            &     (0.021)                 &     (0.049)                 &     (0.033)                 &     (0.032)                 &     (0.384)                 &     (0.183)                 &     (0.381)                 &     (0.131)                 &     (0.478)                 &     (0.750)                 &     (0.447)                 \\\addlinespace
$ICT_{c,t}$&      -0.040                 &      -0.155                 &      -0.108$^{\ast}$        &      -0.008                 &      -0.838                 &       0.311                 &      -1.257                 &       0.109                 &       1.106                 &      -2.633                 &       0.789                 \\
            &     (0.028)                 &     (0.121)                 &     (0.057)                 &     (0.028)                 &     (0.727)                 &     (0.477)                 &     (0.778)                 &     (0.197)                 &     (1.018)                 &     (1.544)                 &     (1.064)                 \\\addlinespace
$R*ICT_{c,t}$&       0.006                 &       0.028                 &       0.018                 &       0.000                 &       0.061                 &       0.012                 &      -0.043                 &       0.093                 &       0.110                 &       0.176                 &       0.216                 \\
            &     (0.018)                 &     (0.040)                 &     (0.032)                 &     (0.017)                 &     (0.586)                 &     (0.284)                 &     (0.421)                 &     (0.106)                 &     (0.443)                 &     (0.711)                 &     (0.668)                 \\\addlinespace
$wL_{c,t}$&       0.543$^{\ast\ast}$    &       1.354$^{\ast\ast}$    &       0.342                 &       0.589$^{\ast\ast\ast}$&      -0.571$^{\ast\ast}$    &      -0.099                 &       0.079                 &      -0.551$^{\ast\ast\ast}$&       0.265                 &       0.598$^{\ast}$        &      -1.035$^{\ast\ast\ast}$\\
            &     (0.208)                 &     (0.466)                 &     (0.303)                 &     (0.140)                 &     (0.196)                 &     (0.133)                 &     (0.155)                 &     (0.071)                 &     (0.238)                 &     (0.320)                 &     (0.279)                 \\\addlinespace
$rK_{c,t}$&      -0.045                 &       0.114                 &      -0.096                 &       0.153                 &      -0.874$^{\ast\ast\ast}$&      -0.227                 &      -0.068                 &      -0.579$^{\ast\ast\ast}$&       0.076                 &       0.499$^{\ast}$        &      -0.832$^{\ast\ast}$    \\
            &     (0.133)                 &     (0.248)                 &     (0.163)                 &     (0.116)                 &     (0.217)                 &     (0.139)                 &     (0.149)                 &     (0.056)                 &     (0.260)                 &     (0.273)                 &     (0.289)                 \\\addlinespace
$pQ_{c,t}$&       0.492                 &      -0.425                 &       0.678                 &       0.307                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.302)                 &     (0.656)                 &     (0.419)                 &     (0.221)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.000                 &      -0.000                 &      -0.002                 &       0.004                 &       0.014                 &      -0.041                 &       0.021                 &       0.033                 &      -0.090                 &      -0.040                 &       0.114                 \\
            &     (0.002)                 &     (0.005)                 &     (0.004)                 &     (0.003)                 &     (0.043)                 &     (0.041)                 &     (0.037)                 &     (0.027)                 &     (0.100)                 &     (0.081)                 &     (0.088)                 \\\addlinespace
$Services_{c,t}$&       0.000                 &      -0.028                 &      -0.015                 &      -0.001                 &      -0.095                 &       0.130                 &      -0.235$^{\ast}$        &       0.010                 &       0.510$^{\ast\ast}$    &      -0.582$^{\ast\ast}$    &       0.017                 \\
            &     (0.004)                 &     (0.029)                 &     (0.009)                 &     (0.005)                 &     (0.145)                 &     (0.098)                 &     (0.118)                 &     (0.033)                 &     (0.177)                 &     (0.252)                 &     (0.129)                 \\\addlinespace
$HHI_{c,t}$&      -0.797                 &      -3.341                 &      -2.237                 &      -1.844$^{\ast}$        &     -43.233                 &      18.272                 &     -37.764$^{\ast\ast}$    &     -23.740$^{\ast}$        &      82.205$^{\ast\ast\ast}$&     -53.537                 &     -25.672                 \\
            &     (0.639)                 &     (4.059)                 &     (2.036)                 &     (0.916)                 &    (26.259)                 &    (16.166)                 &    (14.351)                 &    (11.889)                 &    (25.705)                 &    (38.658)                 &    (36.698)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001                 &       0.004                 &       0.002                 &      -0.000                 &       0.034                 &       0.013                 &       0.014                 &       0.007                 &       0.003                 &       0.009                 &      -0.025                 \\
            &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.001)                 &     (0.019)                 &     (0.012)                 &     (0.015)                 &     (0.009)                 &     (0.027)                 &     (0.033)                 &     (0.033)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.005                 &      -0.010                 &       0.002                 &      -0.007$^{\ast}$        &       0.146                 &      -0.091                 &       0.190                 &       0.047                 &      -0.186                 &       0.454                 &       0.294                 \\
            &     (0.008)                 &     (0.011)                 &     (0.010)                 &     (0.004)                 &     (0.173)                 &     (0.132)                 &     (0.110)                 &     (0.068)                 &     (0.313)                 &     (0.289)                 &     (0.269)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.004                 &      -0.003                 &       0.007                 &       0.000                 &       0.137                 &       0.023                 &       0.099                 &       0.015                 &      -0.010                 &       0.089                 &      -0.087                 \\
            &     (0.003)                 &     (0.005)                 &     (0.006)                 &     (0.002)                 &     (0.084)                 &     (0.033)                 &     (0.079)                 &     (0.010)                 &     (0.082)                 &     (0.130)                 &     (0.088)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.003                 &      -0.005                 &       0.013                 &      -0.018$^{\ast}$        &      -0.057                 &       0.056                 &      -0.009                 &      -0.104                 &       0.037                 &       0.194                 &      -0.344                 \\
            &     (0.008)                 &     (0.010)                 &     (0.016)                 &     (0.009)                 &     (0.239)                 &     (0.137)                 &     (0.208)                 &     (0.063)                 &     (0.303)                 &     (0.397)                 &     (0.296)                 \\\addlinespace
$XRate_{c,t}$&      -0.005$^{\ast\ast}$    &      -0.005                 &      -0.010$^{\ast\ast}$    &      -0.005$^{\ast\ast}$    &      -0.123$^{\ast\ast}$    &       0.001                 &      -0.122$^{\ast\ast}$    &      -0.003                 &       0.163$^{\ast}$        &      -0.220$^{\ast\ast}$    &       0.110$^{\ast\ast}$    \\
            &     (0.002)                 &     (0.006)                 &     (0.004)                 &     (0.002)                 &     (0.053)                 &     (0.036)                 &     (0.053)                 &     (0.011)                 &     (0.088)                 &     (0.097)                 &     (0.049)                 \\\addlinespace
$Imports^{\%GDP}_{c,t}$&      -0.002                 &      -0.018                 &       0.001                 &      -0.001                 &      -0.015                 &      -0.032                 &      -0.007                 &       0.024                 &      -0.139                 &       0.027                 &       0.069                 \\
            &     (0.003)                 &     (0.011)                 &     (0.006)                 &     (0.003)                 &     (0.075)                 &     (0.034)                 &     (0.062)                 &     (0.030)                 &     (0.093)                 &     (0.096)                 &     (0.068)                 \\\addlinespace
$Exports^{\%GDP}_{c,t}$&       0.000                 &       0.012                 &      -0.002                 &       0.001                 &      -0.001                 &       0.005                 &      -0.013                 &       0.008                 &       0.073                 &      -0.050                 &       0.021                 \\
            &     (0.002)                 &     (0.010)                 &     (0.007)                 &     (0.003)                 &     (0.068)                 &     (0.038)                 &     (0.059)                 &     (0.027)                 &     (0.087)                 &     (0.112)                 &     (0.089)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .982                 &        .988                 &        .984                 &        .974                 &         .99                 &        .986                 &         .97                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/Trade_OECD/Results2RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.017$^{\ast}$        &      -0.038$^{\ast}$        &       0.024                 &      -0.020                 &       0.000                 &      -0.298                 &       0.372                 &      -0.075                 &      -0.897                 &       0.899                 &      -0.296                 \\
            &     (0.010)                 &     (0.019)                 &     (0.042)                 &     (0.017)                 &     (0.379)                 &     (0.198)                 &     (0.341)                 &     (0.122)                 &     (0.604)                 &     (0.897)                 &     (0.448)                 \\\addlinespace
$ICT_{c,t}$&      -0.060$^{\ast\ast\ast}$&      -0.091                 &      -0.113$^{\ast\ast\ast}$&      -0.054$^{\ast\ast}$    &      -1.490$^{\ast\ast\ast}$&       0.101                 &      -1.690$^{\ast\ast\ast}$&       0.098                 &       1.362                 &      -2.471$^{\ast\ast}$    &       1.227$^{\ast\ast}$    \\
            &     (0.011)                 &     (0.095)                 &     (0.038)                 &     (0.019)                 &     (0.456)                 &     (0.354)                 &     (0.539)                 &     (0.131)                 &     (0.947)                 &     (0.984)                 &     (0.454)                 \\\addlinespace
$R*ICT_{c,t}$&       0.020$^{\ast\ast\ast}$&       0.021                 &       0.040$^{\ast\ast}$    &       0.035$^{\ast\ast\ast}$&       0.317                 &      -0.255                 &       0.491$^{\ast\ast}$    &       0.081                 &      -0.946$^{\ast\ast}$    &       0.871$^{\ast\ast}$    &      -0.003                 \\
            &     (0.005)                 &     (0.034)                 &     (0.017)                 &     (0.010)                 &     (0.242)                 &     (0.152)                 &     (0.213)                 &     (0.067)                 &     (0.410)                 &     (0.364)                 &     (0.254)                 \\\addlinespace
$wL_{c,t}$&       0.554$^{\ast\ast\ast}$&       0.736$^{\ast\ast}$    &       0.677$^{\ast\ast}$    &       0.546$^{\ast\ast\ast}$&      -0.457$^{\ast\ast\ast}$&       0.042                 &       0.128                 &      -0.626$^{\ast\ast\ast}$&       0.553$^{\ast\ast}$    &       0.801$^{\ast\ast}$    &      -1.387$^{\ast\ast\ast}$\\
            &     (0.158)                 &     (0.348)                 &     (0.304)                 &     (0.107)                 &     (0.147)                 &     (0.106)                 &     (0.113)                 &     (0.086)                 &     (0.229)                 &     (0.350)                 &     (0.214)                 \\\addlinespace
$rK_{c,t}$&       0.064                 &       0.278                 &       0.155                 &      -0.019                 &      -0.646$^{\ast\ast\ast}$&      -0.022                 &       0.036                 &      -0.660$^{\ast\ast\ast}$&       0.509$^{\ast\ast\ast}$&       0.732$^{\ast\ast\ast}$&      -1.328$^{\ast\ast\ast}$\\
            &     (0.095)                 &     (0.265)                 &     (0.184)                 &     (0.074)                 &     (0.126)                 &     (0.083)                 &     (0.091)                 &     (0.068)                 &     (0.166)                 &     (0.249)                 &     (0.191)                 \\\addlinespace
$pQ_{c,t}$&       0.292                 &      -0.093                 &       0.127                 &       0.384$^{\ast\ast}$    &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.248)                 &     (0.589)                 &     (0.446)                 &     (0.156)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &      -0.003                 &       0.005$^{\ast}$        &      -0.001                 &       0.000                 &      -0.039                 &       0.039                 &      -0.000                 &      -0.114                 &       0.131                 &       0.005                 \\
            &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.002)                 &     (0.045)                 &     (0.027)                 &     (0.027)                 &     (0.014)                 &     (0.071)                 &     (0.078)                 &     (0.037)                 \\\addlinespace
$Services_{c,t}$&      -0.002                 &       0.011                 &      -0.012                 &      -0.014$^{\ast\ast}$    &      -0.001                 &       0.161$^{\ast}$        &      -0.107                 &      -0.055                 &       0.524$^{\ast\ast}$    &      -0.327                 &      -0.210$^{\ast}$        \\
            &     (0.004)                 &     (0.014)                 &     (0.011)                 &     (0.006)                 &     (0.093)                 &     (0.078)                 &     (0.106)                 &     (0.041)                 &     (0.235)                 &     (0.287)                 &     (0.101)                 \\\addlinespace
$HHI_{c,t}$&      -0.433                 &       2.449                 &      -1.428                 &      -3.792$^{\ast\ast\ast}$&      15.645                 &      40.383$^{\ast\ast}$    &      -2.741                 &     -21.997$^{\ast\ast}$    &     104.190$^{\ast\ast}$    &     -22.533                 &     -66.533$^{\ast\ast\ast}$\\
            &     (0.540)                 &     (1.883)                 &     (1.975)                 &     (1.041)                 &    (22.087)                 &    (14.718)                 &    (20.198)                 &     (9.127)                 &    (46.604)                 &    (58.539)                 &    (22.957)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001$^{\ast\ast\ast}$&       0.000                 &       0.004$^{\ast\ast}$    &       0.002$^{\ast\ast\ast}$&       0.049$^{\ast\ast\ast}$&      -0.005                 &       0.035$^{\ast\ast}$    &       0.018$^{\ast\ast\ast}$&      -0.063$^{\ast\ast}$    &       0.057                 &      -0.004                 \\
            &     (0.000)                 &     (0.001)                 &     (0.001)                 &     (0.001)                 &     (0.013)                 &     (0.008)                 &     (0.013)                 &     (0.004)                 &     (0.025)                 &     (0.036)                 &     (0.012)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.009                 &       0.004                 &      -0.020                 &      -0.014$^{\ast\ast}$    &      -0.277                 &      -0.020                 &      -0.134                 &      -0.123$^{\ast\ast}$    &       0.325                 &      -0.186                 &       0.127                 \\
            &     (0.007)                 &     (0.009)                 &     (0.015)                 &     (0.006)                 &     (0.190)                 &     (0.090)                 &     (0.153)                 &     (0.046)                 &     (0.236)                 &     (0.387)                 &     (0.141)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.005$^{\ast\ast\ast}$&      -0.002                 &       0.004                 &       0.006$^{\ast\ast}$    &       0.114$^{\ast\ast\ast}$&       0.012                 &       0.068                 &       0.034$^{\ast\ast}$    &      -0.030                 &       0.043                 &      -0.029                 \\
            &     (0.001)                 &     (0.004)                 &     (0.004)                 &     (0.002)                 &     (0.035)                 &     (0.019)                 &     (0.041)                 &     (0.012)                 &     (0.060)                 &     (0.092)                 &     (0.050)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.008                 &       0.009                 &       0.002                 &      -0.001                 &       0.044                 &       0.032                 &       0.084                 &      -0.072                 &       0.068                 &       0.059                 &      -0.252                 \\
            &     (0.005)                 &     (0.010)                 &     (0.015)                 &     (0.007)                 &     (0.189)                 &     (0.102)                 &     (0.163)                 &     (0.064)                 &     (0.291)                 &     (0.346)                 &     (0.194)                 \\\addlinespace
$XRate_{c,t}$&      -0.005$^{\ast\ast\ast}$&      -0.004                 &      -0.006$^{\ast}$        &      -0.007$^{\ast\ast\ast}$&      -0.107$^{\ast\ast\ast}$&      -0.010                 &      -0.091$^{\ast\ast\ast}$&      -0.006                 &       0.093                 &      -0.121                 &       0.072$^{\ast\ast}$    \\
            &     (0.001)                 &     (0.006)                 &     (0.003)                 &     (0.002)                 &     (0.032)                 &     (0.029)                 &     (0.030)                 &     (0.011)                 &     (0.066)                 &     (0.074)                 &     (0.030)                 \\\addlinespace
$Imports^{\%GDP}_{c,t}$&      -0.002                 &       0.001                 &       0.001                 &      -0.005$^{\ast}$        &       0.006                 &       0.025                 &      -0.008                 &      -0.012                 &       0.019                 &       0.007                 &      -0.024                 \\
            &     (0.002)                 &     (0.002)                 &     (0.005)                 &     (0.002)                 &     (0.054)                 &     (0.022)                 &     (0.053)                 &     (0.014)                 &     (0.066)                 &     (0.092)                 &     (0.047)                 \\\addlinespace
$Exports^{\%GDP}_{c,t}$&       0.000                 &      -0.001                 &      -0.005                 &       0.005$^{\ast\ast}$    &      -0.064                 &      -0.048$^{\ast}$        &      -0.046                 &       0.030$^{\ast\ast}$    &      -0.041                 &      -0.109                 &       0.119$^{\ast\ast\ast}$\\
            &     (0.001)                 &     (0.002)                 &     (0.005)                 &     (0.002)                 &     (0.053)                 &     (0.025)                 &     (0.045)                 &     (0.013)                 &     (0.069)                 &     (0.087)                 &     (0.034)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &        .999                 &        .974                 &        .986                 &        .976                 &        .962                 &        .983                 &        .973                 &         .96                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/Trade_OECD/Results2shortV1_RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.012                 &       0.014                 &       0.019                 &      -0.058$^{\ast}$        &       0.150                 &       0.168                 &       0.241                 &      -0.258                 &       0.274                 &       0.693                 &      -0.947                 \\
            &     (0.022)                 &     (0.022)                 &     (0.063)                 &     (0.030)                 &     (0.787)                 &     (0.386)                 &     (0.548)                 &     (0.233)                 &     (0.903)                 &     (0.966)                 &     (0.776)                 \\\addlinespace
$ICT_{c,t}$&       0.022                 &      -0.022                 &       0.046                 &       0.031                 &       0.247                 &      -0.213                 &       0.231                 &       0.229$^{\ast\ast}$    &      -1.469$^{\ast}$        &       0.799                 &       0.689                 \\
            &     (0.036)                 &     (0.042)                 &     (0.042)                 &     (0.059)                 &     (0.422)                 &     (0.552)                 &     (0.297)                 &     (0.091)                 &     (0.771)                 &     (0.479)                 &     (0.641)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.023                 &       0.012                 &      -0.042                 &      -0.037                 &      -0.099                 &      -0.021                 &      -0.004                 &      -0.074                 &       0.647$^{\ast}$        &      -0.645                 &      -0.082                 \\
            &     (0.023)                 &     (0.025)                 &     (0.033)                 &     (0.036)                 &     (0.593)                 &     (0.321)                 &     (0.544)                 &     (0.090)                 &     (0.293)                 &     (0.534)                 &     (0.489)                 \\\addlinespace
$wL_{c,t}$&       0.433$^{\ast\ast\ast}$&       0.197                 &       0.642                 &       0.494$^{\ast\ast\ast}$&      -0.628$^{\ast\ast}$    &       0.095                 &       0.039                 &      -0.762$^{\ast\ast\ast}$&       0.857$^{\ast\ast}$    &       0.902$^{\ast}$        &      -1.764$^{\ast\ast\ast}$\\
            &     (0.100)                 &     (0.267)                 &     (0.418)                 &     (0.143)                 &     (0.232)                 &     (0.092)                 &     (0.209)                 &     (0.092)                 &     (0.313)                 &     (0.439)                 &     (0.329)                 \\\addlinespace
$rK_{c,t}$&       0.033                 &       0.163                 &       0.202                 &      -0.183$^{\ast\ast}$    &      -0.694$^{\ast\ast\ast}$&       0.056                 &       0.021                 &      -0.770$^{\ast\ast\ast}$&       0.829$^{\ast\ast}$    &       0.870$^{\ast\ast}$    &      -1.705$^{\ast\ast\ast}$\\
            &     (0.072)                 &     (0.125)                 &     (0.235)                 &     (0.069)                 &     (0.183)                 &     (0.075)                 &     (0.164)                 &     (0.091)                 &     (0.293)                 &     (0.336)                 &     (0.292)                 \\\addlinespace
$pQ_{c,t}$&       0.124                 &       0.482                 &      -0.211                 &      -0.013                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.189)                 &     (0.474)                 &     (0.719)                 &     (0.205)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .986                 &        .995                 &        .989                 &        .985                 &        .992                 &        .989                 &        .982                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/Trade_OECD/Results2shortV1_RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.040$^{\ast}$        &      -0.068                 &      -0.110$^{\ast\ast\ast}$&       0.020                 &      -0.683                 &      -0.220                 &      -0.836$^{\ast\ast}$    &       0.372$^{\ast\ast}$    &      -0.067                 &      -2.006$^{\ast\ast}$    &       1.321$^{\ast\ast}$    \\
            &     (0.021)                 &     (0.049)                 &     (0.033)                 &     (0.032)                 &     (0.384)                 &     (0.183)                 &     (0.381)                 &     (0.131)                 &     (0.478)                 &     (0.750)                 &     (0.447)                 \\\addlinespace
$ICT_{c,t}$&      -0.040                 &      -0.155                 &      -0.108$^{\ast}$        &      -0.008                 &      -0.838                 &       0.311                 &      -1.257                 &       0.109                 &       1.106                 &      -2.633                 &       0.789                 \\
            &     (0.028)                 &     (0.121)                 &     (0.057)                 &     (0.028)                 &     (0.727)                 &     (0.477)                 &     (0.778)                 &     (0.197)                 &     (1.018)                 &     (1.544)                 &     (1.064)                 \\\addlinespace
$R*ICT_{c,t}$&       0.006                 &       0.028                 &       0.018                 &       0.000                 &       0.061                 &       0.012                 &      -0.043                 &       0.093                 &       0.110                 &       0.176                 &       0.216                 \\
            &     (0.018)                 &     (0.040)                 &     (0.032)                 &     (0.017)                 &     (0.586)                 &     (0.284)                 &     (0.421)                 &     (0.106)                 &     (0.443)                 &     (0.711)                 &     (0.668)                 \\\addlinespace
$wL_{c,t}$&       0.543$^{\ast\ast}$    &       1.354$^{\ast\ast}$    &       0.342                 &       0.589$^{\ast\ast\ast}$&      -0.571$^{\ast\ast}$    &      -0.099                 &       0.079                 &      -0.551$^{\ast\ast\ast}$&       0.265                 &       0.598$^{\ast}$        &      -1.035$^{\ast\ast\ast}$\\
            &     (0.208)                 &     (0.466)                 &     (0.303)                 &     (0.140)                 &     (0.196)                 &     (0.133)                 &     (0.155)                 &     (0.071)                 &     (0.238)                 &     (0.320)                 &     (0.279)                 \\\addlinespace
$rK_{c,t}$&      -0.045                 &       0.114                 &      -0.096                 &       0.153                 &      -0.874$^{\ast\ast\ast}$&      -0.227                 &      -0.068                 &      -0.579$^{\ast\ast\ast}$&       0.076                 &       0.499$^{\ast}$        &      -0.832$^{\ast\ast}$    \\
            &     (0.133)                 &     (0.248)                 &     (0.163)                 &     (0.116)                 &     (0.217)                 &     (0.139)                 &     (0.149)                 &     (0.056)                 &     (0.260)                 &     (0.273)                 &     (0.289)                 \\\addlinespace
$pQ_{c,t}$&       0.492                 &      -0.425                 &       0.678                 &       0.307                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.302)                 &     (0.656)                 &     (0.419)                 &     (0.221)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .982                 &        .988                 &        .984                 &        .974                 &         .99                 &        .986                 &         .97                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/Trade_OECD/Results2shortV1_RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.017$^{\ast}$        &      -0.038$^{\ast}$        &       0.024                 &      -0.020                 &       0.000                 &      -0.298                 &       0.372                 &      -0.075                 &      -0.897                 &       0.899                 &      -0.296                 \\
            &     (0.010)                 &     (0.019)                 &     (0.042)                 &     (0.017)                 &     (0.379)                 &     (0.198)                 &     (0.341)                 &     (0.122)                 &     (0.604)                 &     (0.897)                 &     (0.448)                 \\\addlinespace
$ICT_{c,t}$&      -0.060$^{\ast\ast\ast}$&      -0.091                 &      -0.113$^{\ast\ast\ast}$&      -0.054$^{\ast\ast}$    &      -1.490$^{\ast\ast\ast}$&       0.101                 &      -1.690$^{\ast\ast\ast}$&       0.098                 &       1.362                 &      -2.471$^{\ast\ast}$    &       1.227$^{\ast\ast}$    \\
            &     (0.011)                 &     (0.095)                 &     (0.038)                 &     (0.019)                 &     (0.456)                 &     (0.354)                 &     (0.539)                 &     (0.131)                 &     (0.947)                 &     (0.984)                 &     (0.454)                 \\\addlinespace
$R*ICT_{c,t}$&       0.020$^{\ast\ast\ast}$&       0.021                 &       0.040$^{\ast\ast}$    &       0.035$^{\ast\ast\ast}$&       0.317                 &      -0.255                 &       0.491$^{\ast\ast}$    &       0.081                 &      -0.946$^{\ast\ast}$    &       0.871$^{\ast\ast}$    &      -0.003                 \\
            &     (0.005)                 &     (0.034)                 &     (0.017)                 &     (0.010)                 &     (0.242)                 &     (0.152)                 &     (0.213)                 &     (0.067)                 &     (0.410)                 &     (0.364)                 &     (0.254)                 \\\addlinespace
$wL_{c,t}$&       0.554$^{\ast\ast\ast}$&       0.736$^{\ast\ast}$    &       0.677$^{\ast\ast}$    &       0.546$^{\ast\ast\ast}$&      -0.457$^{\ast\ast\ast}$&       0.042                 &       0.128                 &      -0.626$^{\ast\ast\ast}$&       0.553$^{\ast\ast}$    &       0.801$^{\ast\ast}$    &      -1.387$^{\ast\ast\ast}$\\
            &     (0.158)                 &     (0.348)                 &     (0.304)                 &     (0.107)                 &     (0.147)                 &     (0.106)                 &     (0.113)                 &     (0.086)                 &     (0.229)                 &     (0.350)                 &     (0.214)                 \\\addlinespace
$rK_{c,t}$&       0.064                 &       0.278                 &       0.155                 &      -0.019                 &      -0.646$^{\ast\ast\ast}$&      -0.022                 &       0.036                 &      -0.660$^{\ast\ast\ast}$&       0.509$^{\ast\ast\ast}$&       0.732$^{\ast\ast\ast}$&      -1.328$^{\ast\ast\ast}$\\
            &     (0.095)                 &     (0.265)                 &     (0.184)                 &     (0.074)                 &     (0.126)                 &     (0.083)                 &     (0.091)                 &     (0.068)                 &     (0.166)                 &     (0.249)                 &     (0.191)                 \\\addlinespace
$pQ_{c,t}$&       0.292                 &      -0.093                 &       0.127                 &       0.384$^{\ast\ast}$    &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.248)                 &     (0.589)                 &     (0.446)                 &     (0.156)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
%$R^{2}$  &          0.999                &        .998                 &        .999                 &        .999                 &        .974                 &        .986                 &        .976                 &        .962                 &        .983                 &        .973                 &         .96                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/Trade_OECD/Results4RICTint_EUKLEMS_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.008                 &       0.041$^{\ast}$        &      -0.009                 &      -0.026                 &       0.005                 &      -0.606                 &       0.003                 &       0.004                 \\
            &     (0.026)                 &     (0.018)                 &     (0.026)                 &     (0.033)                 &     (0.003)                 &     (0.543)                 &     (0.005)                 &     (0.005)                 \\\addlinespace
$ICT_{c,t}$&      -0.011                 &      -0.009                 &       0.033                 &       0.097                 &      -0.007                 &       1.608                 &       0.000                 &       0.008                 \\
            &     (0.031)                 &     (0.027)                 &     (0.041)                 &     (0.054)                 &     (0.004)                 &     (1.296)                 &     (0.006)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.026                 &       0.003                 &      -0.040                 &      -0.034                 &       0.005$^{\ast}$        &      -0.617                 &      -0.001                 &       0.009$^{\ast\ast}$    \\
            &     (0.024)                 &     (0.013)                 &     (0.023)                 &     (0.032)                 &     (0.002)                 &     (0.770)                 &     (0.002)                 &     (0.004)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .849                 &          0.999                &        .984                 &         .99                 &         .94                 &        .951                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/Trade_OECD/Results4RICTint_EUKLEMS_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.161$^{\ast\ast\ast}$&      -0.013                 &      -0.078$^{\ast\ast\ast}$&      -0.068$^{\ast\ast}$    &       0.003                 &      -1.445$^{\ast\ast}$    &      -0.006                 &       0.015                 \\
            &     (0.032)                 &     (0.019)                 &     (0.025)                 &     (0.028)                 &     (0.002)                 &     (0.497)                 &     (0.008)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t}$&       0.259$^{\ast\ast\ast}$&      -0.088$^{\ast\ast\ast}$&       0.150$^{\ast\ast\ast}$&      -0.048$^{\ast\ast}$    &       0.009$^{\ast\ast\ast}$&      -1.344$^{\ast}$        &       0.011                 &       0.034$^{\ast\ast}$    \\
            &     (0.039)                 &     (0.024)                 &     (0.038)                 &     (0.019)                 &     (0.002)                 &     (0.708)                 &     (0.009)                 &     (0.015)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.141$^{\ast\ast\ast}$&       0.023                 &      -0.082$^{\ast\ast\ast}$&       0.017                 &      -0.005$^{\ast\ast\ast}$&       0.671                 &      -0.010                 &      -0.017                 \\
            &     (0.031)                 &     (0.013)                 &     (0.022)                 &     (0.013)                 &     (0.001)                 &     (0.441)                 &     (0.007)                 &     (0.011)                 \\\midrule
$R^{2}$  &        .998                 &        .999                 &        .931                 &          0.999                &        .983                 &        .984                 &        .795                 &        .887                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/Trade_OECD/Results4RICTint_EUKLEMS_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.137$^{\ast\ast\ast}$&       0.003                 &      -0.075$^{\ast\ast}$    &      -0.083$^{\ast\ast}$    &       0.000                 &      -0.773$^{\ast\ast}$    &       0.003                 &       0.035$^{\ast\ast\ast}$\\
            &     (0.024)                 &     (0.014)                 &     (0.032)                 &     (0.031)                 &     (0.002)                 &     (0.269)                 &     (0.006)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t}$&       0.157$^{\ast\ast\ast}$&      -0.084$^{\ast\ast}$    &       0.086$^{\ast\ast}$    &      -0.033                 &      -0.003                 &       0.415                 &      -0.002                 &       0.036$^{\ast\ast\ast}$\\
            &     (0.043)                 &     (0.035)                 &     (0.036)                 &     (0.054)                 &     (0.003)                 &     (0.820)                 &     (0.007)                 &     (0.012)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.059$^{\ast\ast\ast}$&       0.027$^{\ast}$        &      -0.041$^{\ast\ast}$    &       0.011                 &       0.002                 &       0.164                 &       0.003                 &      -0.010                 \\
            &     (0.014)                 &     (0.014)                 &     (0.018)                 &     (0.024)                 &     (0.001)                 &     (0.398)                 &     (0.004)                 &     (0.006)                 \\\midrule
$R^{2}$  &        .996                 &        .999                 &        .913                 &        .999                 &        .967                 &        .976                 &        .732                 &        .784                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/Trade_OECD/Results4RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.026                 &       0.045$^{\ast}$        &      -0.014                 &      -0.009                 &       0.006$^{\ast}$        &      -0.820                 &       0.004                 &       0.005                 \\
            &     (0.029)                 &     (0.022)                 &     (0.026)                 &     (0.024)                 &     (0.003)                 &     (0.526)                 &     (0.005)                 &     (0.006)                 \\\addlinespace
$ICT_{c,t}$&       0.008                 &      -0.005                 &       0.038                 &       0.095$^{\ast\ast}$    &      -0.009$^{\ast\ast}$    &       1.797                 &      -0.002                 &       0.007                 \\
            &     (0.020)                 &     (0.029)                 &     (0.042)                 &     (0.036)                 &     (0.004)                 &     (1.189)                 &     (0.005)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.033$^{\ast}$        &       0.000                 &      -0.042$^{\ast}$        &      -0.029                 &       0.006$^{\ast\ast}$    &      -0.662                 &       0.000                 &       0.010$^{\ast\ast}$    \\
            &     (0.015)                 &     (0.018)                 &     (0.022)                 &     (0.028)                 &     (0.003)                 &     (0.711)                 &     (0.002)                 &     (0.004)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &         .85                 &          0.999                &        .984                 &         .99                 &         .94                 &        .952                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/Trade_OECD/Results4RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.145$^{\ast\ast\ast}$&      -0.041$^{\ast}$        &      -0.083$^{\ast\ast\ast}$&      -0.065$^{\ast\ast}$    &       0.002                 &      -1.436$^{\ast\ast}$    &      -0.008                 &       0.013                 \\
            &     (0.038)                 &     (0.019)                 &     (0.025)                 &     (0.025)                 &     (0.002)                 &     (0.510)                 &     (0.008)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t}$&       0.303$^{\ast\ast\ast}$&      -0.129$^{\ast\ast\ast}$&       0.170$^{\ast\ast\ast}$&      -0.053$^{\ast\ast}$    &       0.010$^{\ast\ast\ast}$&      -1.510                 &       0.004                 &       0.034$^{\ast}$        \\
            &     (0.052)                 &     (0.017)                 &     (0.045)                 &     (0.023)                 &     (0.002)                 &     (0.905)                 &     (0.011)                 &     (0.018)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.141$^{\ast\ast\ast}$&       0.032$^{\ast\ast\ast}$&      -0.082$^{\ast\ast\ast}$&       0.019                 &      -0.005$^{\ast\ast\ast}$&       0.674                 &      -0.008                 &      -0.016                 \\
            &     (0.033)                 &     (0.009)                 &     (0.025)                 &     (0.014)                 &     (0.001)                 &     (0.491)                 &     (0.006)                 &     (0.011)                 \\\midrule
$R^{2}$  &        .998                 &        .999                 &         .93                 &          0.999                &        .982                 &        .984                 &        .797                 &        .888                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/Trade_OECD/Results4RICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.141$^{\ast\ast\ast}$&      -0.003                 &      -0.082$^{\ast\ast}$    &      -0.067$^{\ast\ast\ast}$&       0.001                 &      -0.799$^{\ast\ast}$    &       0.001                 &       0.034$^{\ast\ast\ast}$\\
            &     (0.023)                 &     (0.017)                 &     (0.031)                 &     (0.020)                 &     (0.002)                 &     (0.278)                 &     (0.005)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t}$&       0.155$^{\ast\ast\ast}$&      -0.090$^{\ast\ast}$    &       0.085$^{\ast}$        &      -0.018                 &      -0.003                 &       0.648                 &      -0.005                 &       0.040$^{\ast\ast\ast}$\\
            &     (0.049)                 &     (0.042)                 &     (0.042)                 &     (0.057)                 &     (0.003)                 &     (0.989)                 &     (0.009)                 &     (0.013)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.060$^{\ast\ast\ast}$&       0.032$^{\ast}$        &      -0.040$^{\ast}$        &       0.010                 &       0.002                 &       0.085                 &       0.004                 &      -0.011                 \\
            &     (0.015)                 &     (0.018)                 &     (0.019)                 &     (0.025)                 &     (0.001)                 &     (0.427)                 &     (0.005)                 &     (0.007)                 \\\midrule
$R^{2}$  &        .996                 &        .999                 &        .915                 &        .999                 &        .967                 &        .976                 &        .727                 &        .783                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/Trade_OECD/Results4shortRICTint_ct_All_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.026                 &       0.045$^{\ast}$        &      -0.014                 &      -0.009                 &      -0.820                 &       0.005                 \\
            &     (0.029)                 &     (0.022)                 &     (0.026)                 &     (0.024)                 &     (0.526)                 &     (0.006)                 \\\addlinespace
$ICT_{c,t}$&       0.008                 &      -0.005                 &       0.038                 &       0.095$^{\ast\ast}$    &       1.797                 &       0.007                 \\
            &     (0.020)                 &     (0.029)                 &     (0.042)                 &     (0.036)                 &     (1.189)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.033$^{\ast}$        &       0.000                 &      -0.042$^{\ast}$        &      -0.029                 &      -0.662                 &       0.010$^{\ast\ast}$    \\
            &     (0.015)                 &     (0.018)                 &     (0.022)                 &     (0.028)                 &     (0.711)                 &     (0.004)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &         .85                 &          0.999                &         .99                 &        .952                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/Trade_OECD/Results4shortRICTint_ct_All_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.145$^{\ast\ast\ast}$&      -0.041$^{\ast}$        &      -0.083$^{\ast\ast\ast}$&      -0.065$^{\ast\ast}$    &      -1.436$^{\ast\ast}$    &       0.013                 \\
            &     (0.038)                 &     (0.019)                 &     (0.025)                 &     (0.025)                 &     (0.510)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t}$&       0.303$^{\ast\ast\ast}$&      -0.129$^{\ast\ast\ast}$&       0.170$^{\ast\ast\ast}$&      -0.053$^{\ast\ast}$    &      -1.510                 &       0.034$^{\ast}$        \\
            &     (0.052)                 &     (0.017)                 &     (0.045)                 &     (0.023)                 &     (0.905)                 &     (0.018)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.141$^{\ast\ast\ast}$&       0.032$^{\ast\ast\ast}$&      -0.082$^{\ast\ast\ast}$&       0.019                 &       0.674                 &      -0.016                 \\
            &     (0.033)                 &     (0.009)                 &     (0.025)                 &     (0.014)                 &     (0.491)                 &     (0.011)                 \\\midrule
$R^{2}$  &        .998                 &        .999                 &         .93                 &          0.999                &        .984                 &        .888                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         224                 &         224                 \\


==> inputs/robustness/Trade_OECD/Results4shortRICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $Services_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.141$^{\ast\ast\ast}$&      -0.003                 &      -0.082$^{\ast\ast}$    &      -0.067$^{\ast\ast\ast}$&      -0.799$^{\ast\ast}$    &       0.034$^{\ast\ast\ast}$\\
            &     (0.023)                 &     (0.017)                 &     (0.031)                 &     (0.020)                 &     (0.278)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t}$&       0.155$^{\ast\ast\ast}$&      -0.090$^{\ast\ast}$    &       0.085$^{\ast}$        &      -0.018                 &       0.648                 &       0.040$^{\ast\ast\ast}$\\
            &     (0.049)                 &     (0.042)                 &     (0.042)                 &     (0.057)                 &     (0.989)                 &     (0.013)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.060$^{\ast\ast\ast}$&       0.032$^{\ast}$        &      -0.040$^{\ast}$        &       0.010                 &       0.085                 &      -0.011                 \\
            &     (0.015)                 &     (0.018)                 &     (0.019)                 &     (0.025)                 &     (0.427)                 &     (0.007)                 \\\midrule
%$R^{2}$  &        .996                 &        .999                 &        .915                 &        .999                 &        .976                 &        .783                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         395                 &         395                 \\


==> inputs/robustness/Trade_OECD/Results5RICTint_EUKLEMS_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.036                 &      -0.057                 &      -0.011                 &       0.006                 &       0.066$^{\ast\ast\ast}$&      -0.019                 &      -0.002                 &      -0.003                 \\
            &     (0.035)                 &     (0.062)                 &     (0.033)                 &     (0.024)                 &     (0.017)                 &     (0.016)                 &     (0.017)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t}$&       0.010                 &       0.145$^{\ast}$        &       0.069                 &       0.046                 &       0.023                 &       0.021                 &       0.026$^{\ast}$        &       0.009                 \\
            &     (0.040)                 &     (0.064)                 &     (0.040)                 &     (0.042)                 &     (0.015)                 &     (0.023)                 &     (0.012)                 &     (0.009)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.027                 &      -0.061                 &      -0.044                 &      -0.036                 &      -0.003                 &      -0.025                 &      -0.010                 &       0.000                 \\
            &     (0.026)                 &     (0.034)                 &     (0.026)                 &     (0.024)                 &     (0.015)                 &     (0.014)                 &     (0.011)                 &     (0.007)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &          0.999                &          0.999                &          0.999                &        .898                 &          0.999                &        .994                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         135                 &         135                 &         135                 &         135                 \\


==> inputs/robustness/Trade_OECD/Results5RICTint_EUKLEMS_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.194$^{\ast\ast\ast}$&      -0.144$^{\ast\ast\ast}$&      -0.179$^{\ast\ast\ast}$&      -0.134$^{\ast\ast\ast}$&      -0.060$^{\ast\ast\ast}$&      -0.112$^{\ast\ast\ast}$&      -0.017                 &      -0.011                 \\
            &     (0.042)                 &     (0.042)                 &     (0.038)                 &     (0.038)                 &     (0.013)                 &     (0.023)                 &     (0.012)                 &     (0.010)                 \\\addlinespace
$ICT_{c,t}$&       0.108$^{\ast\ast\ast}$&      -0.031                 &       0.050                 &       0.081$^{\ast\ast}$    &       0.009                 &       0.019                 &       0.102$^{\ast\ast\ast}$&      -0.014                 \\
            &     (0.027)                 &     (0.044)                 &     (0.031)                 &     (0.034)                 &     (0.014)                 &     (0.029)                 &     (0.023)                 &     (0.016)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.072$^{\ast\ast\ast}$&      -0.042                 &      -0.056$^{\ast\ast}$    &      -0.081$^{\ast\ast}$    &      -0.006                 &      -0.021                 &      -0.047$^{\ast\ast}$    &       0.019$^{\ast}$        \\
            &     (0.022)                 &     (0.026)                 &     (0.022)                 &     (0.027)                 &     (0.017)                 &     (0.020)                 &     (0.020)                 &     (0.010)                 \\\midrule
$R^{2}$  &        .999                 &        .998                 &        .999                 &        .999                 &          0.999                &        .948                 &        .999                 &        .977                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         174                 &         174                 &         174                 &         174                 \\


==> inputs/robustness/Trade_OECD/Results5RICTint_EUKLEMS_ct_All_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.141$^{\ast\ast\ast}$&      -0.153$^{\ast\ast\ast}$&      -0.154$^{\ast\ast\ast}$&      -0.128$^{\ast\ast\ast}$&      -0.005                 &      -0.112$^{\ast\ast\ast}$&      -0.027$^{\ast}$        &      -0.019$^{\ast\ast}$    \\
            &     (0.030)                 &     (0.036)                 &     (0.031)                 &     (0.029)                 &     (0.020)                 &     (0.024)                 &     (0.014)                 &     (0.008)                 \\\addlinespace
$ICT_{c,t}$&       0.049                 &      -0.073$^{\ast}$        &      -0.002                 &      -0.002                 &       0.012                 &      -0.021                 &       0.071$^{\ast\ast}$    &      -0.008                 \\
            &     (0.044)                 &     (0.041)                 &     (0.041)                 &     (0.036)                 &     (0.024)                 &     (0.038)                 &     (0.024)                 &     (0.019)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.020                 &       0.023                 &      -0.002                 &      -0.008                 &      -0.002                 &       0.020                 &      -0.035$^{\ast\ast}$    &       0.008                 \\
            &     (0.026)                 &     (0.025)                 &     (0.024)                 &     (0.023)                 &     (0.016)                 &     (0.019)                 &     (0.013)                 &     (0.008)                 \\\midrule
$R^{2}$  &        .998                 &        .997                 &        .998                 &        .998                 &        .999                 &        .925                 &        .999                 &        .959                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         309                 &         309                 &         309                 &         309                 \\


==> inputs/robustness/Trade_OECD/Results5RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.034                 &      -0.056                 &      -0.012                 &       0.005                 &       0.065$^{\ast\ast\ast}$&      -0.019                 &      -0.002                 &       0.002                 \\
            &     (0.035)                 &     (0.062)                 &     (0.033)                 &     (0.024)                 &     (0.017)                 &     (0.016)                 &     (0.017)                 &     (0.008)                 \\\addlinespace
$ICT_{c,t}$&       0.023                 &       0.131$^{\ast}$        &       0.071$^{\ast}$        &       0.052                 &       0.029$^{\ast}$        &       0.021                 &       0.023$^{\ast}$        &       0.020$^{\ast\ast}$    \\
            &     (0.039)                 &     (0.058)                 &     (0.038)                 &     (0.041)                 &     (0.013)                 &     (0.022)                 &     (0.012)                 &     (0.006)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.033                 &      -0.052                 &      -0.044                 &      -0.038                 &      -0.006                 &      -0.025                 &      -0.009                 &      -0.006                 \\
            &     (0.030)                 &     (0.031)                 &     (0.026)                 &     (0.025)                 &     (0.015)                 &     (0.013)                 &     (0.010)                 &     (0.009)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &          0.999                &          0.999                &          0.999                &        .898                 &          0.999                &        .982                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         135                 &         135                 &         135                 &         135                 \\


==> inputs/robustness/Trade_OECD/Results5RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.197$^{\ast\ast\ast}$&      -0.145$^{\ast\ast\ast}$&      -0.181$^{\ast\ast\ast}$&      -0.136$^{\ast\ast\ast}$&      -0.060$^{\ast\ast\ast}$&      -0.113$^{\ast\ast\ast}$&      -0.018                 &       0.009                 \\
            &     (0.042)                 &     (0.042)                 &     (0.038)                 &     (0.038)                 &     (0.013)                 &     (0.022)                 &     (0.013)                 &     (0.012)                 \\\addlinespace
$ICT_{c,t}$&       0.132$^{\ast\ast\ast}$&      -0.042                 &       0.060                 &       0.100$^{\ast}$        &       0.014                 &       0.026                 &       0.127$^{\ast\ast\ast}$&      -0.081$^{\ast\ast\ast}$\\
            &     (0.039)                 &     (0.055)                 &     (0.043)                 &     (0.047)                 &     (0.016)                 &     (0.037)                 &     (0.030)                 &     (0.024)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.077$^{\ast\ast}$    &      -0.044                 &      -0.060$^{\ast\ast}$    &      -0.087$^{\ast\ast}$    &      -0.008                 &      -0.023                 &      -0.048$^{\ast\ast}$    &       0.050$^{\ast\ast\ast}$\\
            &     (0.026)                 &     (0.029)                 &     (0.027)                 &     (0.031)                 &     (0.017)                 &     (0.021)                 &     (0.021)                 &     (0.011)                 \\\midrule
$R^{2}$  &        .999                 &        .998                 &        .999                 &        .999                 &          0.999                &        .948                 &        .999                 &        .935                 \\
$N$      &         224                 &         224                 &         224                 &         224                 &         174                 &         174                 &         174                 &         174                 \\


==> inputs/robustness/Trade_OECD/Results5RICTint_ct_All_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.142$^{\ast\ast\ast}$&      -0.153$^{\ast\ast\ast}$&      -0.155$^{\ast\ast\ast}$&      -0.129$^{\ast\ast\ast}$&      -0.006                 &      -0.112$^{\ast\ast\ast}$&      -0.028$^{\ast}$        &      -0.005                 \\
            &     (0.030)                 &     (0.036)                 &     (0.031)                 &     (0.029)                 &     (0.020)                 &     (0.024)                 &     (0.014)                 &     (0.013)                 \\\addlinespace
$ICT_{c,t}$&       0.057                 &      -0.079                 &       0.000                 &       0.002                 &       0.019                 &      -0.026                 &       0.081$^{\ast\ast}$    &      -0.047                 \\
            &     (0.049)                 &     (0.048)                 &     (0.046)                 &     (0.040)                 &     (0.028)                 &     (0.044)                 &     (0.029)                 &     (0.030)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.021                 &       0.023                 &      -0.003                 &      -0.009                 &      -0.005                 &       0.022                 &      -0.037$^{\ast\ast}$    &       0.026$^{\ast\ast}$    \\
            &     (0.027)                 &     (0.026)                 &     (0.025)                 &     (0.024)                 &     (0.017)                 &     (0.021)                 &     (0.014)                 &     (0.012)                 \\\midrule
%$R^{2}$  &        .998                 &        .997                 &        .998                 &        .998                 &        .999                 &        .925                 &        .999                 &        .871                 \\
$N$      &         395                 &         395                 &         395                 &         395                 &         309                 &         309                 &         309                 &         309                 \\


==> inputs/robustness/lagged_controls/Results1RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t-1}$&       0.015                 &       0.003                 &       0.062                 &      -0.003                 &       0.462                 &       0.060                 &       0.459                 &      -0.057                 &      -0.577                 &       1.339                 &      -0.653                 \\
            &     (0.014)                 &     (0.017)                 &     (0.050)                 &     (0.021)                 &     (0.535)                 &     (0.228)                 &     (0.421)                 &     (0.295)                 &     (0.708)                 &     (1.099)                 &     (0.785)                 \\\addlinespace
$ICT_{c,t-1}$&      -0.000                 &       0.000                 &      -0.005                 &       0.001                 &      -0.058                 &       0.035$^{\ast}$        &      -0.075$^{\ast}$        &      -0.018                 &       0.144$^{\ast\ast}$    &      -0.136                 &      -0.005                 \\
            &     (0.001)                 &     (0.003)                 &     (0.006)                 &     (0.001)                 &     (0.046)                 &     (0.016)                 &     (0.039)                 &     (0.012)                 &     (0.060)                 &     (0.095)                 &     (0.041)                 \\\addlinespace
$R*ICT_{c,t-1}$&       0.000                 &       0.000                 &       0.004                 &      -0.001                 &       0.080                 &      -0.011                 &       0.071$^{\ast}$        &       0.019                 &      -0.098                 &       0.097                 &      -0.001                 \\
            &     (0.001)                 &     (0.003)                 &     (0.006)                 &     (0.001)                 &     (0.054)                 &     (0.021)                 &     (0.037)                 &     (0.018)                 &     (0.059)                 &     (0.097)                 &     (0.048)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .983                 &        .994                 &        .989                 &        .947                 &        .992                 &        .988                 &        .965                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/lagged_controls/Results1RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t-1}$&      -0.068$^{\ast\ast\ast}$&      -0.129$^{\ast\ast}$    &      -0.113$^{\ast\ast\ast}$&      -0.023                 &      -0.949                 &      -0.252                 &      -0.772$^{\ast\ast}$    &       0.075                 &       0.127                 &      -1.448$^{\ast\ast\ast}$&       0.842                 \\
            &     (0.020)                 &     (0.057)                 &     (0.030)                 &     (0.034)                 &     (0.529)                 &     (0.203)                 &     (0.310)                 &     (0.248)                 &     (0.587)                 &     (0.431)                 &     (0.523)                 \\\addlinespace
$ICT_{c,t-1}$&       0.005                 &       0.056$^{\ast\ast\ast}$&       0.015$^{\ast\ast}$    &      -0.005                 &       0.188                 &       0.017                 &       0.238$^{\ast\ast}$    &      -0.067                 &      -0.122                 &       0.347$^{\ast\ast}$    &      -0.233                 \\
            &     (0.004)                 &     (0.014)                 &     (0.007)                 &     (0.006)                 &     (0.159)                 &     (0.072)                 &     (0.096)                 &     (0.048)                 &     (0.120)                 &     (0.133)                 &     (0.152)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.006                 &      -0.032                 &      -0.040$^{\ast\ast}$    &       0.018                 &      -0.611                 &       0.060                 &      -0.783$^{\ast\ast}$    &       0.112                 &       0.744$^{\ast\ast}$    &      -1.179$^{\ast\ast\ast}$&       0.515                 \\
            &     (0.012)                 &     (0.044)                 &     (0.017)                 &     (0.014)                 &     (0.438)                 &     (0.204)                 &     (0.255)                 &     (0.120)                 &     (0.294)                 &     (0.332)                 &     (0.368)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .977                 &        .988                 &        .985                 &        .943                 &        .991                 &        .988                 &        .966                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/lagged_controls/Results1RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t-1}$&      -0.040$^{\ast\ast}$    &      -0.080$^{\ast\ast\ast}$&      -0.001                 &      -0.032                 &      -0.123                 &      -0.361                 &       0.268                 &      -0.030                 &      -1.019                 &       0.893                 &      -0.048                 \\
            &     (0.017)                 &     (0.026)                 &     (0.042)                 &     (0.023)                 &     (0.524)                 &     (0.244)                 &     (0.390)                 &     (0.214)                 &     (0.700)                 &     (0.931)                 &     (0.623)                 \\\addlinespace
$ICT_{c,t-1}$&       0.001                 &       0.062$^{\ast\ast\ast}$&      -0.009                 &      -0.008$^{\ast\ast}$    &      -0.021                 &       0.156$^{\ast\ast\ast}$&      -0.070                 &      -0.106$^{\ast\ast}$    &       0.492$^{\ast\ast\ast}$&      -0.254                 &      -0.237$^{\ast\ast}$    \\
            &     (0.003)                 &     (0.005)                 &     (0.009)                 &     (0.003)                 &     (0.124)                 &     (0.035)                 &     (0.106)                 &     (0.039)                 &     (0.137)                 &     (0.211)                 &     (0.084)                 \\\addlinespace
$R*ICT_{c,t-1}$&       0.000                 &      -0.044$^{\ast\ast\ast}$&       0.006                 &       0.027$^{\ast\ast\ast}$&      -0.252                 &      -0.339$^{\ast\ast\ast}$&      -0.164                 &       0.252$^{\ast\ast}$    &      -0.784$^{\ast}$        &       0.030                 &       0.753$^{\ast\ast}$    \\
            &     (0.010)                 &     (0.011)                 &     (0.027)                 &     (0.008)                 &     (0.432)                 &     (0.094)                 &     (0.403)                 &     (0.099)                 &     (0.395)                 &     (0.653)                 &     (0.295)                 \\\midrule
$R^{2}$  &          0.999                &        .999                 &        .999                 &        .999                 &        .967                 &        .986                 &        .975                 &        .906                 &        .983                 &        .973                 &        .938                 \\
$N$      &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 \\


==> inputs/robustness/lagged_controls/Results2RICTint_ct_All_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t-1}$&       0.002                 &       0.002                 &       0.052                 &      -0.027                 &       0.288                 &      -0.010                 &       0.434                 &      -0.136                 &      -0.572                 &       1.354                 &      -0.677                 \\
            &     (0.015)                 &     (0.020)                 &     (0.053)                 &     (0.026)                 &     (0.486)                 &     (0.185)                 &     (0.408)                 &     (0.184)                 &     (0.782)                 &     (0.855)                 &     (0.571)                 \\\addlinespace
$ICT_{c,t-1}$&       0.001                 &       0.000                 &      -0.004                 &       0.002                 &      -0.039                 &       0.038$^{\ast\ast}$    &      -0.074$^{\ast}$        &      -0.003                 &       0.134$^{\ast}$        &      -0.152                 &       0.021                 \\
            &     (0.001)                 &     (0.005)                 &     (0.006)                 &     (0.001)                 &     (0.039)                 &     (0.013)                 &     (0.040)                 &     (0.012)                 &     (0.065)                 &     (0.086)                 &     (0.042)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.000                 &       0.001                 &       0.003                 &      -0.003                 &       0.052                 &      -0.016                 &       0.070                 &      -0.003                 &      -0.082                 &       0.120                 &      -0.040                 \\
            &     (0.001)                 &     (0.005)                 &     (0.005)                 &     (0.002)                 &     (0.041)                 &     (0.017)                 &     (0.039)                 &     (0.014)                 &     (0.068)                 &     (0.081)                 &     (0.049)                 \\\addlinespace
$wL_{c,t}$&       0.393$^{\ast\ast\ast}$&       0.366$^{\ast}$        &       0.461$^{\ast}$        &       0.367$^{\ast}$        &      -0.655$^{\ast\ast}$    &       0.031                 &       0.095                 &      -0.781$^{\ast\ast\ast}$&       0.714$^{\ast}$        &       1.043$^{\ast}$        &      -1.758$^{\ast\ast\ast}$\\
            &     (0.083)                 &     (0.187)                 &     (0.210)                 &     (0.165)                 &     (0.201)                 &     (0.082)                 &     (0.237)                 &     (0.074)                 &     (0.352)                 &     (0.559)                 &     (0.325)                 \\\addlinespace
$rK_{c,t}$&       0.018                 &       0.235                 &       0.126                 &      -0.236$^{\ast\ast\ast}$&      -0.708$^{\ast\ast\ast}$&      -0.006                 &       0.077                 &      -0.779$^{\ast\ast\ast}$&       0.678$^{\ast\ast}$    &       0.995$^{\ast\ast}$    &      -1.676$^{\ast\ast\ast}$\\
            &     (0.062)                 &     (0.146)                 &     (0.138)                 &     (0.061)                 &     (0.167)                 &     (0.052)                 &     (0.191)                 &     (0.079)                 &     (0.280)                 &     (0.408)                 &     (0.288)                 \\\addlinespace
$pQ_{c,t}$&       0.218                 &       0.058                 &       0.328                 &       0.269                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.121)                 &     (0.355)                 &     (0.267)                 &     (0.205)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&       0.001                 &      -0.003                 &       0.001                 &       0.005$^{\ast}$        &      -0.081                 &      -0.050                 &      -0.020                 &      -0.011                 &      -0.084                 &       0.046                 &       0.034                 \\
            &     (0.001)                 &     (0.003)                 &     (0.004)                 &     (0.002)                 &     (0.057)                 &     (0.032)                 &     (0.031)                 &     (0.007)                 &     (0.067)                 &     (0.076)                 &     (0.048)                 \\\addlinespace
$Services_{c,t}$&      -0.001                 &       0.020$^{\ast\ast}$    &       0.010                 &      -0.023$^{\ast\ast}$    &       0.234                 &       0.124$^{\ast}$        &       0.133                 &      -0.023                 &       0.172                 &       0.075                 &      -0.258                 \\
            &     (0.005)                 &     (0.007)                 &     (0.013)                 &     (0.008)                 &     (0.194)                 &     (0.062)                 &     (0.154)                 &     (0.055)                 &     (0.241)                 &     (0.289)                 &     (0.175)                 \\\addlinespace
$HHI_{c,t}$&      -0.965                 &       1.660                 &      -0.423                 &      -4.158$^{\ast\ast}$    &      16.634                 &      18.345                 &      -4.260                 &       2.549                 &      25.182                 &     -19.871                 &      -7.209                 \\
            &     (0.733)                 &     (0.973)                 &     (2.149)                 &     (1.339)                 &    (24.431)                 &    (13.125)                 &    (16.460)                 &     (9.091)                 &    (34.532)                 &    (43.677)                 &    (32.686)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.001                 &      -0.002$^{\ast}$        &       0.002                 &      -0.001                 &       0.044$^{\ast\ast}$    &      -0.005                 &       0.023                 &       0.027$^{\ast\ast\ast}$&      -0.048                 &       0.029                 &       0.022                 \\
            &     (0.001)                 &     (0.001)                 &     (0.003)                 &     (0.001)                 &     (0.015)                 &     (0.007)                 &     (0.015)                 &     (0.007)                 &     (0.030)                 &     (0.038)                 &     (0.015)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.012                 &       0.022$^{\ast\ast}$    &      -0.039                 &       0.040$^{\ast\ast\ast}$&      -0.797$^{\ast\ast}$    &      -0.014                 &      -0.446$^{\ast\ast}$    &      -0.337$^{\ast\ast}$    &       0.733$^{\ast\ast\ast}$&      -0.646                 &      -0.143                 \\
            &     (0.009)                 &     (0.009)                 &     (0.038)                 &     (0.010)                 &     (0.276)                 &     (0.082)                 &     (0.172)                 &     (0.123)                 &     (0.208)                 &     (0.387)                 &     (0.289)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003$^{\ast\ast}$    &       0.001                 &       0.008$^{\ast}$        &       0.001                 &       0.094$^{\ast}$        &       0.010                 &       0.075$^{\ast\ast}$    &       0.009                 &      -0.058                 &       0.134$^{\ast\ast}$    &      -0.083$^{\ast}$        \\
            &     (0.001)                 &     (0.001)                 &     (0.004)                 &     (0.002)                 &     (0.042)                 &     (0.009)                 &     (0.030)                 &     (0.009)                 &     (0.033)                 &     (0.050)                 &     (0.037)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.004                 &       0.025$^{\ast}$        &      -0.008                 &      -0.007                 &       0.132                 &       0.142                 &       0.055                 &      -0.065                 &       0.454$^{\ast}$        &      -0.163                 &      -0.288                 \\
            &     (0.006)                 &     (0.013)                 &     (0.016)                 &     (0.010)                 &     (0.216)                 &     (0.101)                 &     (0.138)                 &     (0.049)                 &     (0.206)                 &     (0.238)                 &     (0.232)                 \\\addlinespace
$XRate_{c,t}$&       0.002                 &      -0.003                 &       0.002                 &       0.008$^{\ast\ast}$    &      -0.037                 &      -0.040                 &       0.014                 &      -0.011                 &       0.002                 &      -0.014                 &      -0.011                 \\
            &     (0.004)                 &     (0.011)                 &     (0.009)                 &     (0.003)                 &     (0.110)                 &     (0.041)                 &     (0.077)                 &     (0.025)                 &     (0.080)                 &     (0.146)                 &     (0.101)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .986                 &        .995                 &        .989                 &        .984                 &        .992                 &        .989                 &        .982                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/lagged_controls/Results2RICTint_ct_All_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t-1}$&      -0.051$^{\ast\ast}$    &      -0.088$^{\ast}$        &      -0.103$^{\ast\ast\ast}$&       0.000                 &      -0.726$^{\ast}$        &      -0.190                 &      -0.767$^{\ast\ast}$    &       0.231                 &       0.106                 &      -1.632$^{\ast\ast}$    &       1.086$^{\ast\ast}$    \\
            &     (0.020)                 &     (0.046)                 &     (0.029)                 &     (0.031)                 &     (0.388)                 &     (0.171)                 &     (0.319)                 &     (0.163)                 &     (0.565)                 &     (0.569)                 &     (0.417)                 \\\addlinespace
$ICT_{c,t-1}$&       0.007                 &       0.059$^{\ast\ast\ast}$&       0.017$^{\ast\ast}$    &      -0.004                 &       0.245                 &       0.047                 &       0.275$^{\ast\ast}$    &      -0.077$^{\ast\ast}$    &      -0.069                 &       0.395$^{\ast\ast}$    &      -0.322$^{\ast\ast}$    \\
            &     (0.005)                 &     (0.013)                 &     (0.007)                 &     (0.005)                 &     (0.137)                 &     (0.064)                 &     (0.100)                 &     (0.030)                 &     (0.120)                 &     (0.130)                 &     (0.141)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.017                 &      -0.049                 &      -0.047$^{\ast\ast}$    &       0.008                 &      -0.666                 &       0.009                 &      -0.875$^{\ast\ast\ast}$&       0.200$^{\ast\ast}$    &       0.604$^{\ast}$        &      -1.374$^{\ast\ast\ast}$&       0.838$^{\ast\ast}$    \\
            &     (0.012)                 &     (0.038)                 &     (0.017)                 &     (0.013)                 &     (0.395)                 &     (0.178)                 &     (0.278)                 &     (0.072)                 &     (0.290)                 &     (0.360)                 &     (0.358)                 \\\addlinespace
$wL_{c,t}$&       0.503$^{\ast\ast}$    &       1.020$^{\ast\ast}$    &       0.321                 &       0.578$^{\ast\ast\ast}$&      -0.592$^{\ast\ast}$    &      -0.135                 &       0.063                 &      -0.521$^{\ast\ast\ast}$&       0.180                 &       0.695$^{\ast\ast}$    &      -0.978$^{\ast\ast\ast}$\\
            &     (0.182)                 &     (0.377)                 &     (0.288)                 &     (0.087)                 &     (0.240)                 &     (0.125)                 &     (0.166)                 &     (0.096)                 &     (0.245)                 &     (0.294)                 &     (0.297)                 \\\addlinespace
$rK_{c,t}$&      -0.047                 &       0.229                 &      -0.100                 &       0.142                 &      -0.894$^{\ast\ast\ast}$&      -0.266$^{\ast}$        &      -0.064                 &      -0.564$^{\ast\ast\ast}$&       0.016                 &       0.626$^{\ast\ast}$    &      -0.801$^{\ast\ast}$    \\
            &     (0.117)                 &     (0.343)                 &     (0.148)                 &     (0.085)                 &     (0.249)                 &     (0.126)                 &     (0.167)                 &     (0.072)                 &     (0.236)                 &     (0.269)                 &     (0.288)                 \\\addlinespace
$pQ_{c,t}$&       0.491$^{\ast}$        &      -0.331                 &       0.673                 &       0.310$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.271)                 &     (0.702)                 &     (0.392)                 &     (0.165)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.002                 &      -0.010$^{\ast}$        &      -0.004                 &       0.003                 &      -0.024                 &      -0.067                 &      -0.011                 &       0.053                 &      -0.154                 &      -0.083                 &       0.197$^{\ast}$        \\
            &     (0.002)                 &     (0.005)                 &     (0.003)                 &     (0.002)                 &     (0.042)                 &     (0.041)                 &     (0.027)                 &     (0.030)                 &     (0.099)                 &     (0.079)                 &     (0.093)                 \\\addlinespace
$Services_{c,t}$&      -0.000                 &      -0.009                 &      -0.016$^{\ast}$        &      -0.002                 &      -0.051                 &       0.154$^{\ast}$        &      -0.203$^{\ast}$        &      -0.002                 &       0.586$^{\ast\ast\ast}$&      -0.598$^{\ast\ast}$    &      -0.017                 \\
            &     (0.004)                 &     (0.022)                 &     (0.008)                 &     (0.006)                 &     (0.113)                 &     (0.084)                 &     (0.095)                 &     (0.027)                 &     (0.184)                 &     (0.210)                 &     (0.132)                 \\\addlinespace
$HHI_{c,t}$&      -1.148                 &      -1.382                 &      -3.522$^{\ast\ast\ast}$&      -1.375                 &     -41.111                 &      18.332                 &     -49.240$^{\ast\ast}$    &     -10.203                 &      93.559$^{\ast\ast}$    &     -94.704$^{\ast\ast\ast}$&       9.444                 \\
            &     (0.642)                 &     (2.723)                 &     (1.114)                 &     (1.001)                 &    (28.250)                 &    (21.354)                 &    (17.962)                 &     (7.318)                 &    (40.509)                 &    (29.104)                 &    (36.654)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001                 &       0.002                 &       0.002                 &       0.000                 &       0.025                 &       0.007                 &       0.012                 &       0.005                 &      -0.006                 &       0.013                 &      -0.027                 \\
            &     (0.001)                 &     (0.002)                 &     (0.001)                 &     (0.001)                 &     (0.019)                 &     (0.013)                 &     (0.014)                 &     (0.009)                 &     (0.033)                 &     (0.028)                 &     (0.031)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.001                 &      -0.004                 &       0.004                 &      -0.007                 &       0.266                 &       0.007                 &       0.219$^{\ast}$        &       0.041                 &      -0.039                 &       0.405                 &       0.171                 \\
            &     (0.007)                 &     (0.014)                 &     (0.007)                 &     (0.006)                 &     (0.177)                 &     (0.153)                 &     (0.110)                 &     (0.079)                 &     (0.382)                 &     (0.236)                 &     (0.288)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.006$^{\ast}$        &      -0.002                 &       0.013$^{\ast\ast}$    &       0.001                 &       0.208$^{\ast\ast\ast}$&       0.022                 &       0.170$^{\ast\ast}$    &       0.016                 &      -0.086                 &       0.222$^{\ast\ast}$    &      -0.145$^{\ast\ast}$    \\
            &     (0.003)                 &     (0.006)                 &     (0.005)                 &     (0.003)                 &     (0.065)                 &     (0.035)                 &     (0.062)                 &     (0.016)                 &     (0.098)                 &     (0.100)                 &     (0.064)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.000                 &      -0.001                 &       0.020$^{\ast}$        &      -0.016$^{\ast}$        &      -0.028                 &       0.026                 &       0.038                 &      -0.092                 &      -0.115                 &       0.269                 &      -0.300                 \\
            &     (0.007)                 &     (0.008)                 &     (0.010)                 &     (0.008)                 &     (0.211)                 &     (0.131)                 &     (0.154)                 &     (0.062)                 &     (0.266)                 &     (0.274)                 &     (0.302)                 \\\addlinespace
$XRate_{c,t}$&      -0.001                 &       0.002                 &      -0.001                 &      -0.004                 &      -0.031                 &      -0.006                 &      -0.010                 &      -0.015$^{\ast}$        &       0.069                 &      -0.017                 &       0.015                 \\
            &     (0.002)                 &     (0.006)                 &     (0.002)                 &     (0.002)                 &     (0.047)                 &     (0.039)                 &     (0.037)                 &     (0.008)                 &     (0.085)                 &     (0.079)                 &     (0.054)                 \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .985                 &         .99                 &        .986                 &        .973                 &        .991                 &        .988                 &        .972                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/lagged_controls/Results2RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t-1}$&      -0.032$^{\ast\ast}$    &      -0.071$^{\ast\ast\ast}$&       0.009                 &      -0.023                 &      -0.260                 &      -0.397                 &       0.225                 &      -0.088                 &      -1.005                 &       0.900                 &      -0.097                 \\
            &     (0.013)                 &     (0.023)                 &     (0.042)                 &     (0.023)                 &     (0.498)                 &     (0.244)                 &     (0.388)                 &     (0.132)                 &     (0.678)                 &     (0.891)                 &     (0.513)                 \\\addlinespace
$ICT_{c,t-1}$&       0.001                 &       0.062$^{\ast\ast\ast}$&      -0.008                 &      -0.007$^{\ast\ast}$    &       0.070                 &       0.170$^{\ast\ast\ast}$&      -0.060                 &      -0.040                 &       0.455$^{\ast\ast\ast}$&      -0.318                 &      -0.124                 \\
            &     (0.003)                 &     (0.005)                 &     (0.009)                 &     (0.003)                 &     (0.103)                 &     (0.035)                 &     (0.108)                 &     (0.028)                 &     (0.138)                 &     (0.218)                 &     (0.098)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.006                 &      -0.048$^{\ast\ast\ast}$&      -0.000                 &       0.021$^{\ast\ast}$    &      -0.405                 &      -0.368$^{\ast\ast\ast}$&      -0.191                 &       0.154$^{\ast}$        &      -0.735$^{\ast}$        &       0.109                 &       0.603                 \\
            &     (0.010)                 &     (0.010)                 &     (0.026)                 &     (0.008)                 &     (0.389)                 &     (0.086)                 &     (0.413)                 &     (0.075)                 &     (0.377)                 &     (0.681)                 &     (0.350)                 \\\addlinespace
$wL_{c,t}$&       0.582$^{\ast\ast\ast}$&       0.495$^{\ast}$        &       0.683$^{\ast\ast}$    &       0.643$^{\ast\ast\ast}$&      -0.488$^{\ast\ast\ast}$&       0.028                 &       0.130                 &      -0.645$^{\ast\ast\ast}$&       0.491$^{\ast}$        &       0.968$^{\ast\ast}$    &      -1.451$^{\ast\ast\ast}$\\
            &     (0.155)                 &     (0.244)                 &     (0.292)                 &     (0.153)                 &     (0.165)                 &     (0.113)                 &     (0.140)                 &     (0.091)                 &     (0.271)                 &     (0.367)                 &     (0.262)                 \\\addlinespace
$rK_{c,t}$&       0.089                 &       0.161                 &       0.131                 &       0.054                 &      -0.679$^{\ast\ast\ast}$&      -0.041                 &       0.037                 &      -0.675$^{\ast\ast\ast}$&       0.458$^{\ast\ast}$    &       0.868$^{\ast\ast\ast}$&      -1.368$^{\ast\ast\ast}$\\
            &     (0.083)                 &     (0.190)                 &     (0.162)                 &     (0.095)                 &     (0.145)                 &     (0.090)                 &     (0.112)                 &     (0.071)                 &     (0.195)                 &     (0.232)                 &     (0.227)                 \\\addlinespace
$pQ_{c,t}$&       0.197                 &       0.177                 &       0.086                 &       0.225                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.229)                 &     (0.414)                 &     (0.397)                 &     (0.219)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.002$^{\ast}$        &      -0.004                 &       0.005                 &      -0.003                 &      -0.006                 &      -0.030                 &       0.029                 &      -0.005                 &      -0.105                 &       0.124                 &      -0.002                 \\
            &     (0.001)                 &     (0.003)                 &     (0.003)                 &     (0.002)                 &     (0.032)                 &     (0.026)                 &     (0.026)                 &     (0.015)                 &     (0.078)                 &     (0.084)                 &     (0.036)                 \\\addlinespace
$Services_{c,t}$&      -0.005                 &       0.018$^{\ast}$        &      -0.016                 &      -0.017$^{\ast\ast}$    &      -0.006                 &       0.171$^{\ast\ast}$    &      -0.141                 &      -0.036                 &       0.565$^{\ast\ast}$    &      -0.460$^{\ast}$        &      -0.136                 \\
            &     (0.004)                 &     (0.009)                 &     (0.010)                 &     (0.007)                 &     (0.077)                 &     (0.077)                 &     (0.094)                 &     (0.042)                 &     (0.245)                 &     (0.263)                 &     (0.117)                 \\\addlinespace
$HHI_{c,t}$&      -0.872                 &       3.116$^{\ast\ast}$    &      -3.700                 &      -2.805$^{\ast\ast\ast}$&      -7.331                 &      28.141$^{\ast}$        &     -28.952                 &      -6.520                 &      95.670$^{\ast\ast}$    &     -91.345                 &      -7.366                 \\
            &     (0.571)                 &     (1.317)                 &     (2.161)                 &     (0.910)                 &    (16.516)                 &    (13.850)                 &    (19.326)                 &     (7.087)                 &    (45.283)                 &    (58.328)                 &    (25.214)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.001$^{\ast\ast\ast}$&      -0.001                 &       0.004$^{\ast\ast\ast}$&       0.002$^{\ast\ast\ast}$&       0.050$^{\ast\ast\ast}$&      -0.009                 &       0.041$^{\ast\ast\ast}$&       0.018$^{\ast\ast\ast}$&      -0.076$^{\ast\ast\ast}$&       0.076$^{\ast\ast}$    &      -0.006                 \\
            &     (0.000)                 &     (0.001)                 &     (0.001)                 &     (0.001)                 &     (0.011)                 &     (0.006)                 &     (0.012)                 &     (0.004)                 &     (0.024)                 &     (0.035)                 &     (0.012)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&      -0.006                 &       0.010                 &      -0.021                 &      -0.012$^{\ast}$        &      -0.335                 &      -0.016                 &      -0.200                 &      -0.119$^{\ast\ast}$    &       0.377                 &      -0.340                 &       0.143                 \\
            &     (0.006)                 &     (0.007)                 &     (0.013)                 &     (0.007)                 &     (0.199)                 &     (0.088)                 &     (0.142)                 &     (0.044)                 &     (0.261)                 &     (0.314)                 &     (0.146)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.006$^{\ast\ast\ast}$&      -0.001                 &       0.006                 &       0.006$^{\ast\ast}$    &       0.138$^{\ast\ast\ast}$&       0.017                 &       0.089$^{\ast\ast}$    &       0.031$^{\ast\ast\ast}$&      -0.039                 &       0.086                 &      -0.055                 \\
            &     (0.002)                 &     (0.003)                 &     (0.004)                 &     (0.002)                 &     (0.035)                 &     (0.016)                 &     (0.035)                 &     (0.011)                 &     (0.059)                 &     (0.078)                 &     (0.039)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.009                 &       0.022$^{\ast\ast}$    &       0.006                 &      -0.004                 &       0.071                 &       0.034                 &       0.089                 &      -0.052                 &       0.051                 &      -0.008                 &      -0.181                 \\
            &     (0.006)                 &     (0.008)                 &     (0.013)                 &     (0.007)                 &     (0.191)                 &     (0.101)                 &     (0.155)                 &     (0.053)                 &     (0.261)                 &     (0.315)                 &     (0.233)                 \\\addlinespace
$XRate_{c,t}$&      -0.001                 &       0.006$^{\ast\ast}$    &       0.002                 &      -0.005$^{\ast\ast\ast}$&       0.013                 &       0.015                 &       0.020                 &      -0.022$^{\ast}$        &       0.066                 &       0.030                 &      -0.053                 \\
            &     (0.001)                 &     (0.003)                 &     (0.002)                 &     (0.002)                 &     (0.038)                 &     (0.023)                 &     (0.021)                 &     (0.011)                 &     (0.054)                 &     (0.056)                 &     (0.033)                 \\\midrule
$R^{2}$  &          0.999                &        .999                 &        .999                 &        .999                 &        .973                 &        .986                 &        .976                 &        .962                 &        .984                 &        .975                 &        .957                 \\
$N$      &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 \\


==> inputs/robustness/lagged_controls/Results2shortV1_RICTint_ct_All_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t-1}$&       0.002                 &       0.002                 &       0.052                 &      -0.027                 &       0.288                 &      -0.010                 &       0.434                 &      -0.136                 &      -0.572                 &       1.354                 &      -0.677                 \\
            &     (0.015)                 &     (0.020)                 &     (0.053)                 &     (0.026)                 &     (0.486)                 &     (0.185)                 &     (0.408)                 &     (0.184)                 &     (0.782)                 &     (0.855)                 &     (0.571)                 \\\addlinespace
$ICT_{c,t-1}$&       0.001                 &       0.000                 &      -0.004                 &       0.002                 &      -0.039                 &       0.038$^{\ast\ast}$    &      -0.074$^{\ast}$        &      -0.003                 &       0.134$^{\ast}$        &      -0.152                 &       0.021                 \\
            &     (0.001)                 &     (0.005)                 &     (0.006)                 &     (0.001)                 &     (0.039)                 &     (0.013)                 &     (0.040)                 &     (0.012)                 &     (0.065)                 &     (0.086)                 &     (0.042)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.000                 &       0.001                 &       0.003                 &      -0.003                 &       0.052                 &      -0.016                 &       0.070                 &      -0.003                 &      -0.082                 &       0.120                 &      -0.040                 \\
            &     (0.001)                 &     (0.005)                 &     (0.005)                 &     (0.002)                 &     (0.041)                 &     (0.017)                 &     (0.039)                 &     (0.014)                 &     (0.068)                 &     (0.081)                 &     (0.049)                 \\\addlinespace
$wL_{c,t}$&       0.393$^{\ast\ast\ast}$&       0.366$^{\ast}$        &       0.461$^{\ast}$        &       0.367$^{\ast}$        &      -0.655$^{\ast\ast}$    &       0.031                 &       0.095                 &      -0.781$^{\ast\ast\ast}$&       0.714$^{\ast}$        &       1.043$^{\ast}$        &      -1.758$^{\ast\ast\ast}$\\
            &     (0.083)                 &     (0.187)                 &     (0.210)                 &     (0.165)                 &     (0.201)                 &     (0.082)                 &     (0.237)                 &     (0.074)                 &     (0.352)                 &     (0.559)                 &     (0.325)                 \\\addlinespace
$rK_{c,t}$&       0.018                 &       0.235                 &       0.126                 &      -0.236$^{\ast\ast\ast}$&      -0.708$^{\ast\ast\ast}$&      -0.006                 &       0.077                 &      -0.779$^{\ast\ast\ast}$&       0.678$^{\ast\ast}$    &       0.995$^{\ast\ast}$    &      -1.676$^{\ast\ast\ast}$\\
            &     (0.062)                 &     (0.146)                 &     (0.138)                 &     (0.061)                 &     (0.167)                 &     (0.052)                 &     (0.191)                 &     (0.079)                 &     (0.280)                 &     (0.408)                 &     (0.288)                 \\\addlinespace
$pQ_{c,t}$&       0.218                 &       0.058                 &       0.328                 &       0.269                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.121)                 &     (0.355)                 &     (0.267)                 &     (0.205)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &          0.999                &        .986                 &        .995                 &        .989                 &        .984                 &        .992                 &        .989                 &        .982                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/lagged_controls/Results2shortV1_RICTint_ct_All_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t-1}$&      -0.051$^{\ast\ast}$    &      -0.088$^{\ast}$        &      -0.103$^{\ast\ast\ast}$&       0.000                 &      -0.726$^{\ast}$        &      -0.190                 &      -0.767$^{\ast\ast}$    &       0.231                 &       0.106                 &      -1.632$^{\ast\ast}$    &       1.086$^{\ast\ast}$    \\
            &     (0.020)                 &     (0.046)                 &     (0.029)                 &     (0.031)                 &     (0.388)                 &     (0.171)                 &     (0.319)                 &     (0.163)                 &     (0.565)                 &     (0.569)                 &     (0.417)                 \\\addlinespace
$ICT_{c,t-1}$&       0.007                 &       0.059$^{\ast\ast\ast}$&       0.017$^{\ast\ast}$    &      -0.004                 &       0.245                 &       0.047                 &       0.275$^{\ast\ast}$    &      -0.077$^{\ast\ast}$    &      -0.069                 &       0.395$^{\ast\ast}$    &      -0.322$^{\ast\ast}$    \\
            &     (0.005)                 &     (0.013)                 &     (0.007)                 &     (0.005)                 &     (0.137)                 &     (0.064)                 &     (0.100)                 &     (0.030)                 &     (0.120)                 &     (0.130)                 &     (0.141)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.017                 &      -0.049                 &      -0.047$^{\ast\ast}$    &       0.008                 &      -0.666                 &       0.009                 &      -0.875$^{\ast\ast\ast}$&       0.200$^{\ast\ast}$    &       0.604$^{\ast}$        &      -1.374$^{\ast\ast\ast}$&       0.838$^{\ast\ast}$    \\
            &     (0.012)                 &     (0.038)                 &     (0.017)                 &     (0.013)                 &     (0.395)                 &     (0.178)                 &     (0.278)                 &     (0.072)                 &     (0.290)                 &     (0.360)                 &     (0.358)                 \\\addlinespace
$wL_{c,t}$&       0.503$^{\ast\ast}$    &       1.020$^{\ast\ast}$    &       0.321                 &       0.578$^{\ast\ast\ast}$&      -0.592$^{\ast\ast}$    &      -0.135                 &       0.063                 &      -0.521$^{\ast\ast\ast}$&       0.180                 &       0.695$^{\ast\ast}$    &      -0.978$^{\ast\ast\ast}$\\
            &     (0.182)                 &     (0.377)                 &     (0.288)                 &     (0.087)                 &     (0.240)                 &     (0.125)                 &     (0.166)                 &     (0.096)                 &     (0.245)                 &     (0.294)                 &     (0.297)                 \\\addlinespace
$rK_{c,t}$&      -0.047                 &       0.229                 &      -0.100                 &       0.142                 &      -0.894$^{\ast\ast\ast}$&      -0.266$^{\ast}$        &      -0.064                 &      -0.564$^{\ast\ast\ast}$&       0.016                 &       0.626$^{\ast\ast}$    &      -0.801$^{\ast\ast}$    \\
            &     (0.117)                 &     (0.343)                 &     (0.148)                 &     (0.085)                 &     (0.249)                 &     (0.126)                 &     (0.167)                 &     (0.072)                 &     (0.236)                 &     (0.269)                 &     (0.288)                 \\\addlinespace
$pQ_{c,t}$&       0.491$^{\ast}$        &      -0.331                 &       0.673                 &       0.310$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.271)                 &     (0.702)                 &     (0.392)                 &     (0.165)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &        .998                 &        .999                 &          0.999                &        .985                 &         .99                 &        .986                 &        .973                 &        .991                 &        .988                 &        .972                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/lagged_controls/Results2shortV1_RICTint_ct_All_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t-1}$&      -0.032$^{\ast\ast}$    &      -0.071$^{\ast\ast\ast}$&       0.009                 &      -0.023                 &      -0.260                 &      -0.397                 &       0.225                 &      -0.088                 &      -1.005                 &       0.900                 &      -0.097                 \\
            &     (0.013)                 &     (0.023)                 &     (0.042)                 &     (0.023)                 &     (0.498)                 &     (0.244)                 &     (0.388)                 &     (0.132)                 &     (0.678)                 &     (0.891)                 &     (0.513)                 \\\addlinespace
$ICT_{c,t-1}$&       0.001                 &       0.062$^{\ast\ast\ast}$&      -0.008                 &      -0.007$^{\ast\ast}$    &       0.070                 &       0.170$^{\ast\ast\ast}$&      -0.060                 &      -0.040                 &       0.455$^{\ast\ast\ast}$&      -0.318                 &      -0.124                 \\
            &     (0.003)                 &     (0.005)                 &     (0.009)                 &     (0.003)                 &     (0.103)                 &     (0.035)                 &     (0.108)                 &     (0.028)                 &     (0.138)                 &     (0.218)                 &     (0.098)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.006                 &      -0.048$^{\ast\ast\ast}$&      -0.000                 &       0.021$^{\ast\ast}$    &      -0.405                 &      -0.368$^{\ast\ast\ast}$&      -0.191                 &       0.154$^{\ast}$        &      -0.735$^{\ast}$        &       0.109                 &       0.603                 \\
            &     (0.010)                 &     (0.010)                 &     (0.026)                 &     (0.008)                 &     (0.389)                 &     (0.086)                 &     (0.413)                 &     (0.075)                 &     (0.377)                 &     (0.681)                 &     (0.350)                 \\\addlinespace
$wL_{c,t}$&       0.582$^{\ast\ast\ast}$&       0.495$^{\ast}$        &       0.683$^{\ast\ast}$    &       0.643$^{\ast\ast\ast}$&      -0.488$^{\ast\ast\ast}$&       0.028                 &       0.130                 &      -0.645$^{\ast\ast\ast}$&       0.491$^{\ast}$        &       0.968$^{\ast\ast}$    &      -1.451$^{\ast\ast\ast}$\\
            &     (0.155)                 &     (0.244)                 &     (0.292)                 &     (0.153)                 &     (0.165)                 &     (0.113)                 &     (0.140)                 &     (0.091)                 &     (0.271)                 &     (0.367)                 &     (0.262)                 \\\addlinespace
$rK_{c,t}$&       0.089                 &       0.161                 &       0.131                 &       0.054                 &      -0.679$^{\ast\ast\ast}$&      -0.041                 &       0.037                 &      -0.675$^{\ast\ast\ast}$&       0.458$^{\ast\ast}$    &       0.868$^{\ast\ast\ast}$&      -1.368$^{\ast\ast\ast}$\\
            &     (0.083)                 &     (0.190)                 &     (0.162)                 &     (0.095)                 &     (0.145)                 &     (0.090)                 &     (0.112)                 &     (0.071)                 &     (0.195)                 &     (0.232)                 &     (0.227)                 \\\addlinespace
$pQ_{c,t}$&       0.197                 &       0.177                 &       0.086                 &       0.225                 &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.229)                 &     (0.414)                 &     (0.397)                 &     (0.219)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
%$R^{2}$  &          0.999                &        .999                 &        .999                 &        .999                 &        .973                 &        .986                 &        .976                 &        .962                 &        .984                 &        .975                 &        .957                 \\
$N$      &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 \\


==> inputs/robustness/lagged_controls/Results3RICTint_cit_All_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{i,c,t-1}$&       0.000                 &      -0.002$^{\ast\ast}$    &       0.002                 &      -0.002                 &       0.001$^{\ast\ast\ast}$&      -0.001                 \\
            &     (0.001)                 &     (0.001)                 &     (0.001)                 &     (0.005)                 &     (0.000)                 &     (0.001)                 \\\addlinespace
$ICT_{i,c,t-1}$&       0.000                 &      -0.000                 &       0.000                 &      -0.001$^{\ast}$        &       0.000$^{\ast\ast\ast}$&       0.000                 \\
            &     (0.000)                 &     (0.000)                 &     (0.000)                 &     (0.001)                 &     (0.000)                 &     (0.000)                 \\\addlinespace
$R*ICT_{i,c,t-1}$&       0.000$^{\ast\ast}$    &      -0.000$^{\ast\ast\ast}$&       0.000$^{\ast\ast\ast}$&       0.000                 &       0.000$^{\ast}$        &      -0.000                 \\
            &     (0.000)                 &     (0.000)                 &     (0.000)                 &     (0.000)                 &     (0.000)                 &     (0.000)                 \\\midrule
$R^{2}$  &        .999                 &        .998                 &        .998                 &        .985                 &        .918                 &        .999                 \\
$N$      &        2070                 &        2070                 &        2070                 &        2052                 &        2025                 &        2025                 \\


==> inputs/robustness/lagged_controls/Results3RICTint_cit_All_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{i,c,t-1}$&      -0.008                 &       0.013                 &      -0.021                 &      -0.047                 &      -0.002                 &       0.017                 \\
            &     (0.025)                 &     (0.007)                 &     (0.025)                 &     (0.046)                 &     (0.005)                 &     (0.019)                 \\\addlinespace
$ICT_{i,c,t-1}$&       0.025$^{\ast\ast}$    &       0.004                 &       0.021$^{\ast}$        &      -0.010                 &       0.002                 &       0.029                 \\
            &     (0.011)                 &     (0.006)                 &     (0.011)                 &     (0.033)                 &     (0.011)                 &     (0.017)                 \\\addlinespace
$R*ICT_{i,c,t-1}$&       0.003                 &       0.000                 &       0.003                 &      -0.018                 &      -0.001                 &       0.006                 \\
            &     (0.005)                 &     (0.002)                 &     (0.005)                 &     (0.019)                 &     (0.003)                 &     (0.008)                 \\\midrule
$R^{2}$  &        .998                 &        .997                 &        .997                 &        .977                 &        .944                 &        .998                 \\
$N$      &        2598                 &        2598                 &        2598                 &        2567                 &        2553                 &        2553                 \\


==> inputs/robustness/lagged_controls/Results3RICTint_cit_All_95t16.tex <==
& ln $wL_{i,c,t}$ & ln $w_{i,c,t}$ & ln $L_{i,c,t}$ & ln $rK_{i,c,t}$ & ln $r_{i,c,t}$ & ln $K_{i,c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{i,c,t-1}$&      -0.031                 &       0.028$^{\ast\ast}$    &      -0.058$^{\ast\ast}$    &      -0.090$^{\ast}$        &      -0.012$^{\ast}$        &       0.008                 \\
            &     (0.030)                 &     (0.010)                 &     (0.027)                 &     (0.047)                 &     (0.007)                 &     (0.028)                 \\\addlinespace
$ICT_{i,c,t-1}$&       0.019                 &       0.005                 &       0.014                 &       0.023                 &      -0.000                 &       0.026                 \\
            &     (0.012)                 &     (0.005)                 &     (0.013)                 &     (0.027)                 &     (0.010)                 &     (0.023)                 \\\addlinespace
$R*ICT_{i,c,t-1}$&      -0.007                 &       0.005$^{\ast}$        &      -0.013$^{\ast\ast}$    &      -0.001                 &      -0.004$^{\ast}$        &       0.007                 \\
            &     (0.006)                 &     (0.003)                 &     (0.006)                 &     (0.012)                 &     (0.002)                 &     (0.008)                 \\\midrule
%$R^{2}$  &        .997                 &        .996                 &        .995                 &        .972                 &        .927                 &        .997                 \\
$N$      &        4668                 &        4668                 &        4668                 &        4619                 &        4578                 &        4578                 \\


==> inputs/robustness/lagged_controls/Results4RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t-1}$&      -0.015                 &       0.024                 &      -0.012                 &      -0.005                 &       0.008                 &      -1.289                 &       0.005                 &       0.001                 \\
            &     (0.019)                 &     (0.022)                 &     (0.027)                 &     (0.020)                 &     (0.006)                 &     (0.744)                 &     (0.004)                 &     (0.003)                 \\\addlinespace
$ICT_{c,t-1}$&       0.001                 &       0.001                 &       0.004$^{\ast}$        &       0.004                 &      -0.001                 &       0.080                 &      -0.000                 &       0.000$^{\ast}$        \\
            &     (0.001)                 &     (0.001)                 &     (0.002)                 &     (0.002)                 &     (0.000)                 &     (0.048)                 &     (0.000)                 &     (0.000)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.001                 &      -0.001                 &      -0.005$^{\ast\ast}$    &      -0.003                 &       0.001$^{\ast}$        &      -0.161$^{\ast\ast\ast}$&       0.000                 &      -0.001                 \\
            &     (0.002)                 &     (0.001)                 &     (0.002)                 &     (0.003)                 &     (0.000)                 &     (0.047)                 &     (0.000)                 &     (0.000)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .821                 &          0.999                &        .965                 &        .987                 &        .936                 &        .942                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/lagged_controls/Results4RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t-1}$&      -0.121$^{\ast\ast\ast}$&      -0.041$^{\ast\ast}$    &      -0.058$^{\ast}$        &      -0.063$^{\ast\ast}$    &       0.004                 &      -1.766$^{\ast\ast\ast}$&      -0.007                 &       0.010                 \\
            &     (0.032)                 &     (0.018)                 &     (0.032)                 &     (0.025)                 &     (0.003)                 &     (0.443)                 &     (0.006)                 &     (0.011)                 \\\addlinespace
$ICT_{c,t-1}$&       0.015                 &       0.010$^{\ast}$        &       0.008                 &       0.009                 &       0.001                 &      -0.166                 &       0.002$^{\ast}$        &      -0.001                 \\
            &     (0.013)                 &     (0.005)                 &     (0.009)                 &     (0.005)                 &     (0.001)                 &     (0.187)                 &     (0.001)                 &     (0.003)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.025                 &      -0.024$^{\ast}$        &      -0.016                 &      -0.008                 &      -0.002                 &       0.340                 &      -0.006                 &       0.000                 \\
            &     (0.036)                 &     (0.013)                 &     (0.024)                 &     (0.014)                 &     (0.003)                 &     (0.574)                 &     (0.004)                 &     (0.008)                 \\\midrule
$R^{2}$  &        .998                 &        .999                 &         .92                 &          0.999                &        .958                 &        .981                 &        .775                 &        .879                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/lagged_controls/Results4RICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t-1}$&      -0.124$^{\ast\ast\ast}$&      -0.012                 &      -0.072$^{\ast\ast}$    &      -0.065$^{\ast\ast\ast}$&       0.003                 &      -0.962$^{\ast\ast\ast}$&       0.001                 &       0.033$^{\ast\ast\ast}$\\
            &     (0.027)                 &     (0.014)                 &     (0.032)                 &     (0.022)                 &     (0.003)                 &     (0.313)                 &     (0.004)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t-1}$&       0.014$^{\ast\ast}$    &       0.005                 &       0.004                 &       0.014$^{\ast\ast}$    &      -0.000                 &      -0.303$^{\ast\ast}$    &      -0.001                 &      -0.006$^{\ast\ast}$    \\
            &     (0.006)                 &     (0.004)                 &     (0.006)                 &     (0.006)                 &     (0.001)                 &     (0.123)                 &     (0.001)                 &     (0.003)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.012                 &      -0.007                 &      -0.004                 &      -0.014                 &      -0.001                 &       0.708$^{\ast}$        &       0.002                 &       0.013$^{\ast}$        \\
            &     (0.017)                 &     (0.009)                 &     (0.016)                 &     (0.021)                 &     (0.003)                 &     (0.361)                 &     (0.003)                 &     (0.007)                 \\\midrule
$R^{2}$  &        .996                 &        .999                 &        .901                 &        .999                 &        .922                 &        .974                 &        .708                 &        .749                 \\
$N$      &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 \\


==> inputs/robustness/lagged_controls/Results4shortRICTint_ct_All_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t-1}$&      -0.015                 &       0.024                 &      -0.012                 &      -0.005                 &      -1.289                 &       0.001                 \\
            &     (0.019)                 &     (0.022)                 &     (0.027)                 &     (0.020)                 &     (0.744)                 &     (0.003)                 \\\addlinespace
$ICT_{c,t-1}$&       0.001                 &       0.001                 &       0.004$^{\ast}$        &       0.004                 &       0.080                 &       0.000$^{\ast}$        \\
            &     (0.001)                 &     (0.001)                 &     (0.002)                 &     (0.002)                 &     (0.048)                 &     (0.000)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.001                 &      -0.001                 &      -0.005$^{\ast\ast}$    &      -0.003                 &      -0.161$^{\ast\ast\ast}$&      -0.001                 \\
            &     (0.002)                 &     (0.001)                 &     (0.002)                 &     (0.003)                 &     (0.047)                 &     (0.000)                 \\\midrule
$R^{2}$  &        .999                 &          0.999                &        .821                 &          0.999                &        .987                 &        .942                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         171                 &         171                 \\


==> inputs/robustness/lagged_controls/Results4shortRICTint_ct_All_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t-1}$&      -0.121$^{\ast\ast\ast}$&      -0.041$^{\ast\ast}$    &      -0.058$^{\ast}$        &      -0.063$^{\ast\ast}$    &      -1.766$^{\ast\ast\ast}$&       0.010                 \\
            &     (0.032)                 &     (0.018)                 &     (0.032)                 &     (0.025)                 &     (0.443)                 &     (0.011)                 \\\addlinespace
$ICT_{c,t-1}$&       0.015                 &       0.010$^{\ast}$        &       0.008                 &       0.009                 &      -0.166                 &      -0.001                 \\
            &     (0.013)                 &     (0.005)                 &     (0.009)                 &     (0.005)                 &     (0.187)                 &     (0.003)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.025                 &      -0.024$^{\ast}$        &      -0.016                 &      -0.008                 &       0.340                 &       0.000                 \\
            &     (0.036)                 &     (0.013)                 &     (0.024)                 &     (0.014)                 &     (0.574)                 &     (0.008)                 \\\midrule
$R^{2}$  &        .998                 &        .999                 &         .92                 &          0.999                &        .981                 &        .879                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         209                 &         209                 \\


==> inputs/robustness/lagged_controls/Results4shortRICTint_ct_All_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $Services_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t-1}$&      -0.124$^{\ast\ast\ast}$&      -0.012                 &      -0.072$^{\ast\ast}$    &      -0.065$^{\ast\ast\ast}$&      -0.962$^{\ast\ast\ast}$&       0.033$^{\ast\ast\ast}$\\
            &     (0.027)                 &     (0.014)                 &     (0.032)                 &     (0.022)                 &     (0.313)                 &     (0.009)                 \\\addlinespace
$ICT_{c,t-1}$&       0.014$^{\ast\ast}$    &       0.005                 &       0.004                 &       0.014$^{\ast\ast}$    &      -0.303$^{\ast\ast}$    &      -0.006$^{\ast\ast}$    \\
            &     (0.006)                 &     (0.004)                 &     (0.006)                 &     (0.006)                 &     (0.123)                 &     (0.003)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.012                 &      -0.007                 &      -0.004                 &      -0.014                 &       0.708$^{\ast}$        &       0.013$^{\ast}$        \\
            &     (0.017)                 &     (0.009)                 &     (0.016)                 &     (0.021)                 &     (0.361)                 &     (0.007)                 \\\midrule
%$R^{2}$  &        .996                 &        .999                 &        .901                 &        .999                 &        .974                 &        .749                 \\
$N$      &         380                 &         380                 &         380                 &         380                 &         380                 &         380                 \\


==> inputs/robustness/lagged_controls/Results5RICTint_ct_All_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t-1}$&       0.013                 &      -0.015                 &      -0.001                 &       0.007                 &       0.046$^{\ast}$        &      -0.010                 &       0.007                 &      -0.001                 \\
            &     (0.020)                 &     (0.032)                 &     (0.024)                 &     (0.019)                 &     (0.024)                 &     (0.012)                 &     (0.027)                 &     (0.007)                 \\\addlinespace
$ICT_{c,t-1}$&       0.004$^{\ast}$        &       0.002                 &       0.004$^{\ast}$        &       0.003                 &       0.000                 &       0.002$^{\ast\ast}$    &      -0.001                 &       0.001$^{\ast}$        \\
            &     (0.002)                 &     (0.002)                 &     (0.002)                 &     (0.002)                 &     (0.001)                 &     (0.001)                 &     (0.001)                 &     (0.000)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.005$^{\ast}$        &      -0.001                 &      -0.004                 &      -0.002                 &       0.001                 &      -0.002$^{\ast\ast}$    &       0.002                 &      -0.001$^{\ast\ast}$    \\
            &     (0.002)                 &     (0.002)                 &     (0.002)                 &     (0.002)                 &     (0.002)                 &     (0.001)                 &     (0.001)                 &     (0.000)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &          0.999                &          0.999                &          0.999                &        .866                 &          0.999                &        .977                 \\
$N$      &         171                 &         171                 &         171                 &         171                 &         135                 &         135                 &         135                 &         135                 \\


==> inputs/robustness/lagged_controls/Results5RICTint_ct_All_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t-1}$&      -0.173$^{\ast\ast\ast}$&      -0.139$^{\ast\ast\ast}$&      -0.164$^{\ast\ast\ast}$&      -0.123$^{\ast\ast\ast}$&      -0.062$^{\ast\ast\ast}$&      -0.112$^{\ast\ast\ast}$&      -0.028$^{\ast}$        &      -0.003                 \\
            &     (0.034)                 &     (0.039)                 &     (0.034)                 &     (0.035)                 &     (0.014)                 &     (0.024)                 &     (0.015)                 &     (0.018)                 \\\addlinespace
$ICT_{c,t-1}$&       0.019                 &       0.037$^{\ast\ast\ast}$&       0.025$^{\ast\ast}$    &       0.026$^{\ast\ast}$    &       0.005                 &       0.004                 &       0.001                 &      -0.011                 \\
            &     (0.011)                 &     (0.010)                 &     (0.011)                 &     (0.012)                 &     (0.006)                 &     (0.005)                 &     (0.009)                 &     (0.007)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.033                 &      -0.074$^{\ast\ast}$    &      -0.046                 &      -0.058$^{\ast}$        &      -0.004                 &      -0.002                 &       0.001                 &       0.035                 \\
            &     (0.028)                 &     (0.027)                 &     (0.027)                 &     (0.030)                 &     (0.017)                 &     (0.014)                 &     (0.024)                 &     (0.021)                 \\\midrule
$R^{2}$  &        .999                 &        .998                 &        .999                 &        .999                 &          0.999                &        .954                 &        .999                 &        .917                 \\
$N$      &         209                 &         209                 &         209                 &         209                 &         161                 &         161                 &         161                 &         161                 \\


==> inputs/robustness/lagged_controls/Results5RICTint_ct_All_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t-1}$&      -0.141$^{\ast\ast\ast}$&      -0.143$^{\ast\ast\ast}$&      -0.149$^{\ast\ast\ast}$&      -0.123$^{\ast\ast\ast}$&      -0.007                 &      -0.116$^{\ast\ast\ast}$&      -0.018                 &      -0.019                 \\
            &     (0.029)                 &     (0.037)                 &     (0.032)                 &     (0.030)                 &     (0.021)                 &     (0.032)                 &     (0.017)                 &     (0.018)                 \\\addlinespace
$ICT_{c,t-1}$&       0.016$^{\ast\ast}$    &       0.026$^{\ast\ast}$    &       0.021$^{\ast\ast}$    &       0.021$^{\ast\ast}$    &       0.007                 &       0.002                 &       0.005                 &      -0.000                 \\
            &     (0.007)                 &     (0.011)                 &     (0.008)                 &     (0.008)                 &     (0.008)                 &     (0.004)                 &     (0.006)                 &     (0.004)                 \\\addlinespace
$R*ICT_{c,t-1}$&      -0.014                 &      -0.037                 &      -0.025                 &      -0.033                 &      -0.010                 &       0.010                 &      -0.011                 &       0.009                 \\
            &     (0.023)                 &     (0.029)                 &     (0.025)                 &     (0.025)                 &     (0.023)                 &     (0.012)                 &     (0.019)                 &     (0.010)                 \\\midrule
%$R^{2}$  &        .998                 &        .996                 &        .998                 &        .998                 &        .999                 &        .927                 &        .998                 &        .877                 \\
$N$      &         380                 &         380                 &         380                 &         380                 &         296                 &         296                 &         296                 &         296                 \\


==> inputs/south_95_16/Results1RICTint_ct_South_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax} \\\midrule & $ln T_{c,t}$ & $ln T^l_{c,t}$ & $ln T^k_{c,t}$ & $ln T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.158                 &      -0.173                 &       0.020                 &      -0.272                 &      -5.660$^{\ast\ast}$    &      -2.091                 &      -0.575                 &      -2.994                 &      -2.005                 &       3.854                 &      -5.622                 \\
            &     (0.068)                 &     (0.126)                 &     (0.105)                 &     (0.132)                 &     (1.758)                 &     (1.250)                 &     (0.990)                 &     (1.281)                 &     (3.209)                 &     (2.798)                 &     (3.480)                 \\\addlinespace
$ICT_{c,t}$&      -0.032                 &      -0.084$^{\ast}$        &      -0.006                 &      -0.022                 &      -0.708                 &      -0.719$^{\ast\ast}$    &       0.120                 &      -0.109                 &      -1.770$^{\ast\ast}$    &       1.216                 &       0.158                 \\
            &     (0.018)                 &     (0.028)                 &     (0.045)                 &     (0.032)                 &     (0.302)                 &     (0.148)                 &     (0.290)                 &     (0.239)                 &     (0.454)                 &     (0.703)                 &     (0.946)                 \\\addlinespace
$R*ICT_{c,t}$&       0.011                 &       0.020                 &      -0.054                 &       0.076                 &       0.773                 &       0.376                 &      -0.420                 &       0.817$^{\ast}$        &       0.270                 &      -2.347$^{\ast\ast}$    &       2.533$^{\ast}$        \\
            &     (0.032)                 &     (0.037)                 &     (0.055)                 &     (0.040)                 &     (0.426)                 &     (0.353)                 &     (0.182)                 &     (0.291)                 &     (0.762)                 &     (0.677)                 &     (0.877)                 \\\midrule
$R^{2}$  &          0.999                &        .999                 &        .999                 &        .999                 &        .971                 &        .967                 &        .972                 &        .959                 &        .955                 &        .935                 &        .971                 \\
$N$      &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 \\


==> inputs/south_95_16/Results2RICTint_ct_South_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.089                 &      -0.021                 &      -0.083                 &      -0.119                 &      -2.639                 &      -0.113                 &      -1.396                 &      -1.130                 &       0.936                 &      -1.106                 &      -0.403                 \\
            &     (0.067)                 &     (0.053)                 &     (0.133)                 &     (0.166)                 &     (1.458)                 &     (0.454)                 &     (1.262)                 &     (0.553)                 &     (1.185)                 &     (3.073)                 &     (2.338)                 \\\addlinespace
$ICT_{c,t}$&      -0.012                 &      -0.021                 &       0.027                 &      -0.045                 &      -0.476                 &      -0.412                 &       0.032                 &      -0.096                 &      -1.057$^{\ast}$        &       0.827                 &       0.230                 \\
            &     (0.018)                 &     (0.035)                 &     (0.045)                 &     (0.027)                 &     (0.370)                 &     (0.240)                 &     (0.254)                 &     (0.146)                 &     (0.404)                 &     (0.582)                 &     (0.770)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.017                 &      -0.044                 &      -0.015                 &       0.016                 &      -0.231                 &      -0.523                 &      -0.108                 &       0.400                 &      -1.465$^{\ast}$        &      -0.686                 &       1.309                 \\
            &     (0.035)                 &     (0.032)                 &     (0.081)                 &     (0.048)                 &     (0.564)                 &     (0.277)                 &     (0.599)                 &     (0.173)                 &     (0.518)                 &     (0.989)                 &     (0.943)                 \\\addlinespace
$wL_{c,t}$&       0.474                 &       1.449$^{\ast\ast}$    &       0.816                 &      -0.577                 &      -0.522                 &       0.204                 &       0.054                 &      -0.780$^{\ast\ast\ast}$&       1.207$^{\ast\ast\ast}$&       0.830                 &      -2.059$^{\ast\ast}$    \\
            &     (0.228)                 &     (0.404)                 &     (0.509)                 &     (0.271)                 &     (0.370)                 &     (0.127)                 &     (0.270)                 &     (0.113)                 &     (0.193)                 &     (0.444)                 &     (0.468)                 \\\addlinespace
$rK_{c,t}$&       0.032                 &       0.291                 &       0.798                 &      -0.833$^{\ast\ast}$    &      -0.726$^{\ast}$        &      -0.031                 &       0.126                 &      -0.821$^{\ast\ast\ast}$&       0.691$^{\ast\ast}$    &       1.169$^{\ast\ast}$    &      -2.196$^{\ast\ast}$    \\
            &     (0.134)                 &     (0.163)                 &     (0.373)                 &     (0.212)                 &     (0.236)                 &     (0.068)                 &     (0.190)                 &     (0.124)                 &     (0.207)                 &     (0.340)                 &     (0.447)                 \\\addlinespace
$pQ_{c,t}$&       0.371                 &      -0.715                 &      -0.531                 &       2.045$^{\ast\ast\ast}$&                             &                             &                             &                             &                             &                             &                             \\
            &     (0.362)                 &     (0.526)                 &     (0.928)                 &     (0.284)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.001                 &       0.006$^{\ast}$        &      -0.013                 &       0.006                 &      -0.061                 &       0.089$^{\ast\ast}$    &      -0.129                 &      -0.022                 &       0.295$^{\ast}$        &      -0.314$^{\ast}$        &       0.075                 \\
            &     (0.002)                 &     (0.002)                 &     (0.007)                 &     (0.004)                 &     (0.088)                 &     (0.026)                 &     (0.063)                 &     (0.028)                 &     (0.099)                 &     (0.121)                 &     (0.113)                 \\\addlinespace
$Services_{c,t}$&      -0.004                 &      -0.017                 &      -0.032                 &       0.038$^{\ast}$        &      -0.480                 &      -0.057                 &      -0.212                 &      -0.211$^{\ast\ast}$    &       0.268                 &      -0.312                 &      -0.260                 \\
            &     (0.008)                 &     (0.013)                 &     (0.023)                 &     (0.015)                 &     (0.273)                 &     (0.122)                 &     (0.180)                 &     (0.050)                 &     (0.254)                 &     (0.277)                 &     (0.252)                 \\\addlinespace
$HHI_{c,t}$&      -0.676                 &      -2.176                 &      -0.745                 &       1.953                 &     -68.953                 &     -33.946                 &      -4.902                 &     -30.105                 &     -56.626                 &       3.487                 &     -47.370                 \\
            &     (2.259)                 &     (3.393)                 &     (4.358)                 &     (3.691)                 &    (61.669)                 &    (37.106)                 &    (62.160)                 &    (25.849)                 &    (70.218)                 &    (97.698)                 &   (124.679)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&       0.000                 &       0.000                 &      -0.000                 &       0.001                 &       0.017                 &       0.007                 &      -0.012                 &       0.022$^{\ast\ast}$    &      -0.011                 &      -0.043                 &       0.042                 \\
            &     (0.002)                 &     (0.001)                 &     (0.004)                 &     (0.001)                 &     (0.030)                 &     (0.016)                 &     (0.020)                 &     (0.005)                 &     (0.024)                 &     (0.036)                 &     (0.038)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.015                 &       0.026$^{\ast\ast}$    &      -0.007                 &       0.020                 &       0.196                 &       0.374$^{\ast}$        &       0.157                 &      -0.334$^{\ast}$        &       1.037$^{\ast\ast\ast}$&       0.241                 &      -0.709                 \\
            &     (0.011)                 &     (0.008)                 &     (0.027)                 &     (0.014)                 &     (0.291)                 &     (0.119)                 &     (0.112)                 &     (0.118)                 &     (0.132)                 &     (0.212)                 &     (0.344)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.009                 &       0.002                 &       0.019                 &       0.007                 &       0.195                 &       0.009                 &       0.210$^{\ast}$        &      -0.024                 &      -0.184$^{\ast}$        &       0.400$^{\ast}$        &      -0.284                 \\
            &     (0.007)                 &     (0.004)                 &     (0.009)                 &     (0.009)                 &     (0.123)                 &     (0.042)                 &     (0.089)                 &     (0.030)                 &     (0.075)                 &     (0.132)                 &     (0.162)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.009                 &       0.011                 &       0.021                 &      -0.008                 &       0.221                 &       0.193                 &       0.373                 &      -0.345$^{\ast\ast}$    &       0.377                 &       0.835                 &      -1.038                 \\
            &     (0.009)                 &     (0.014)                 &     (0.024)                 &     (0.023)                 &     (0.469)                 &     (0.185)                 &     (0.305)                 &     (0.099)                 &     (0.217)                 &     (0.550)                 &     (0.474)                 \\\addlinespace
$XRate_{c,t}$&       0.419                 &      -0.144                 &       1.882                 &      -0.328                 &       6.553                 &      -2.304                 &      16.370                 &      -7.514                 &      -6.859                 &      58.045$^{\ast\ast}$    &     -33.208                 \\
            &     (0.541)                 &     (0.819)                 &     (0.971)                 &     (0.239)                 &    (18.145)                 &     (8.853)                 &    (10.138)                 &     (4.234)                 &    (11.312)                 &    (14.966)                 &    (21.609)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &        .999                 &        .976                 &        .978                 &        .973                 &        .986                 &        .973                 &        .948                 &        .984                 \\
$N$      &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 \\


==> inputs/south_95_16/Results2shortEXCGDPV1_RICTint_ct_South_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{8}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.089                 &      -0.021                 &      -0.083                 &      -0.119                 &       0.936                 &      -1.106                 &      -0.403                 \\
            &     (0.067)                 &     (0.053)                 &     (0.133)                 &     (0.166)                 &     (1.185)                 &     (3.073)                 &     (2.338)                 \\\addlinespace
$ICT_{c,t}$&      -0.012                 &      -0.021                 &       0.027                 &      -0.045                 &      -1.057$^{\ast}$        &       0.827                 &       0.230                 \\
            &     (0.018)                 &     (0.035)                 &     (0.045)                 &     (0.027)                 &     (0.404)                 &     (0.582)                 &     (0.770)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.017                 &      -0.044                 &      -0.015                 &       0.016                 &      -1.465$^{\ast}$        &      -0.686                 &       1.309                 \\
            &     (0.035)                 &     (0.032)                 &     (0.081)                 &     (0.048)                 &     (0.518)                 &     (0.989)                 &     (0.943)                 \\\addlinespace
$wL_{c,t}$&       0.474                 &       1.449$^{\ast\ast}$    &       0.816                 &      -0.577                 &       1.207$^{\ast\ast\ast}$&       0.830                 &      -2.059$^{\ast\ast}$    \\
            &     (0.228)                 &     (0.404)                 &     (0.509)                 &     (0.271)                 &     (0.193)                 &     (0.444)                 &     (0.468)                 \\\addlinespace
$rK_{c,t}$&       0.032                 &       0.291                 &       0.798                 &      -0.833$^{\ast\ast}$    &       0.691$^{\ast\ast}$    &       1.169$^{\ast\ast}$    &      -2.196$^{\ast\ast}$    \\
            &     (0.134)                 &     (0.163)                 &     (0.373)                 &     (0.212)                 &     (0.207)                 &     (0.340)                 &     (0.447)                 \\\addlinespace
$pQ_{c,t}$&       0.371                 &      -0.715                 &      -0.531                 &       2.045$^{\ast\ast\ast}$&                             &                             &                             \\
            &     (0.362)                 &     (0.526)                 &     (0.928)                 &     (0.284)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &        .999                 &        .973                 &        .948                 &        .984                 \\
$N$      &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 \\


==> inputs/south_95_16/Results2shortEXCGDPV2_RICTint_ct_South_95t16.tex <==
& $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{4}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &       0.936                 &      -1.106                 &      -0.403                 \\
            &     (1.185)                 &     (3.073)                 &     (2.338)                 \\\addlinespace
$ICT_{c,t}$&      -1.057$^{\ast}$        &       0.827                 &       0.230                 \\
            &     (0.404)                 &     (0.582)                 &     (0.770)                 \\\addlinespace
$R*ICT_{c,t}$&      -1.465$^{\ast}$        &      -0.686                 &       1.309                 \\
            &     (0.518)                 &     (0.989)                 &     (0.943)                 \\\addlinespace
$wL_{c,t}$&       1.207$^{\ast\ast\ast}$&       0.830                 &      -2.059$^{\ast\ast}$    \\
            &     (0.193)                 &     (0.444)                 &     (0.468)                 \\\addlinespace
$rK_{c,t}$&       0.691$^{\ast\ast}$    &       1.169$^{\ast\ast}$    &      -2.196$^{\ast\ast}$    \\
            &     (0.207)                 &     (0.340)                 &     (0.447)                 \\\midrule
$R^{2}$  &        .973                 &        .948                 &        .984                 \\
$N$      &          83                 &          83                 &          83                 \\


==> inputs/south_95_16/Results2shortV1_RICTint_ct_South_95t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency} &\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{12}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.089                 &      -0.021                 &      -0.083                 &      -0.119                 &      -2.639                 &      -0.113                 &      -1.396                 &      -1.130                 &       0.936                 &      -1.106                 &      -0.403                 \\
            &     (0.067)                 &     (0.053)                 &     (0.133)                 &     (0.166)                 &     (1.458)                 &     (0.454)                 &     (1.262)                 &     (0.553)                 &     (1.185)                 &     (3.073)                 &     (2.338)                 \\\addlinespace
$ICT_{c,t}$&      -0.012                 &      -0.021                 &       0.027                 &      -0.045                 &      -0.476                 &      -0.412                 &       0.032                 &      -0.096                 &      -1.057$^{\ast}$        &       0.827                 &       0.230                 \\
            &     (0.018)                 &     (0.035)                 &     (0.045)                 &     (0.027)                 &     (0.370)                 &     (0.240)                 &     (0.254)                 &     (0.146)                 &     (0.404)                 &     (0.582)                 &     (0.770)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.017                 &      -0.044                 &      -0.015                 &       0.016                 &      -0.231                 &      -0.523                 &      -0.108                 &       0.400                 &      -1.465$^{\ast}$        &      -0.686                 &       1.309                 \\
            &     (0.035)                 &     (0.032)                 &     (0.081)                 &     (0.048)                 &     (0.564)                 &     (0.277)                 &     (0.599)                 &     (0.173)                 &     (0.518)                 &     (0.989)                 &     (0.943)                 \\\addlinespace
$wL_{c,t}$&       0.474                 &       1.449$^{\ast\ast}$    &       0.816                 &      -0.577                 &      -0.522                 &       0.204                 &       0.054                 &      -0.780$^{\ast\ast\ast}$&       1.207$^{\ast\ast\ast}$&       0.830                 &      -2.059$^{\ast\ast}$    \\
            &     (0.228)                 &     (0.404)                 &     (0.509)                 &     (0.271)                 &     (0.370)                 &     (0.127)                 &     (0.270)                 &     (0.113)                 &     (0.193)                 &     (0.444)                 &     (0.468)                 \\\addlinespace
$rK_{c,t}$&       0.032                 &       0.291                 &       0.798                 &      -0.833$^{\ast\ast}$    &      -0.726$^{\ast}$        &      -0.031                 &       0.126                 &      -0.821$^{\ast\ast\ast}$&       0.691$^{\ast\ast}$    &       1.169$^{\ast\ast}$    &      -2.196$^{\ast\ast}$    \\
            &     (0.134)                 &     (0.163)                 &     (0.373)                 &     (0.212)                 &     (0.236)                 &     (0.068)                 &     (0.190)                 &     (0.124)                 &     (0.207)                 &     (0.340)                 &     (0.447)                 \\\addlinespace
$pQ_{c,t}$&       0.371                 &      -0.715                 &      -0.531                 &       2.045$^{\ast\ast\ast}$&                             &                             &                             &                             &                             &                             &                             \\
            &     (0.362)                 &     (0.526)                 &     (0.928)                 &     (0.284)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .999                 &        .999                 &        .976                 &        .978                 &        .973                 &        .986                 &        .973                 &        .948                 &        .984                 \\
$N$      &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 \\


==> inputs/south_95_16/Results2shortV2_RICTint_ct_South_95t16.tex <==
&\multicolumn{4}{c}{Taxes as \% of GDP} &\multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule \multicolumn{8}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -2.639                 &      -0.113                 &      -1.396                 &      -1.130                 &       0.936                 &      -1.106                 &      -0.403                 \\
            &     (1.458)                 &     (0.454)                 &     (1.262)                 &     (0.553)                 &     (1.185)                 &     (3.073)                 &     (2.338)                 \\\addlinespace
$ICT_{c,t}$&      -0.476                 &      -0.412                 &       0.032                 &      -0.096                 &      -1.057$^{\ast}$        &       0.827                 &       0.230                 \\
            &     (0.370)                 &     (0.240)                 &     (0.254)                 &     (0.146)                 &     (0.404)                 &     (0.582)                 &     (0.770)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.231                 &      -0.523                 &      -0.108                 &       0.400                 &      -1.465$^{\ast}$        &      -0.686                 &       1.309                 \\
            &     (0.564)                 &     (0.277)                 &     (0.599)                 &     (0.173)                 &     (0.518)                 &     (0.989)                 &     (0.943)                 \\\addlinespace
$wL_{c,t}$&      -0.522                 &       0.204                 &       0.054                 &      -0.780$^{\ast\ast\ast}$&       1.207$^{\ast\ast\ast}$&       0.830                 &      -2.059$^{\ast\ast}$    \\
            &     (0.370)                 &     (0.127)                 &     (0.270)                 &     (0.113)                 &     (0.193)                 &     (0.444)                 &     (0.468)                 \\\addlinespace
$rK_{c,t}$&      -0.726$^{\ast}$        &      -0.031                 &       0.126                 &      -0.821$^{\ast\ast\ast}$&       0.691$^{\ast\ast}$    &       1.169$^{\ast\ast}$    &      -2.196$^{\ast\ast}$    \\
            &     (0.236)                 &     (0.068)                 &     (0.190)                 &     (0.124)                 &     (0.207)                 &     (0.340)                 &     (0.447)                 \\\midrule
$R^{2}$  &        .976                 &        .978                 &        .973                 &        .986                 &        .973                 &        .948                 &        .984                 \\
$N$      &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 \\


==> inputs/south_95_16/Results3RICTint_cit_South_95t16.tex <==
& ln $wL_{i,c,t}$ & ln $w_{i,c,t}$ & ln $L_{i,c,t}$ & ln $rK_{i,c,t}$ & ln $r_{i,c,t}$ & ln $K_{i,c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{i,c,t}$&      -0.017                 &       0.079$^{\ast}$        &      -0.096                 &      -0.239                 &      -0.033$^{\ast\ast\ast}$&      -0.036                 \\
            &     (0.072)                 &     (0.041)                 &     (0.073)                 &     (0.186)                 &     (0.010)                 &     (0.052)                 \\\addlinespace
$ICT_{i,c,t}$&       0.068$^{\ast\ast\ast}$&       0.035                 &       0.033                 &      -0.065                 &       0.011$^{\ast\ast}$    &       0.020                 \\
            &     (0.016)                 &     (0.024)                 &     (0.022)                 &     (0.064)                 &     (0.005)                 &     (0.012)                 \\\addlinespace
$R*ICT_{i,c,t}$&       0.023                 &       0.014                 &       0.010                 &       0.067                 &       0.015$^{\ast\ast\ast}$&      -0.050$^{\ast\ast}$    \\
            &     (0.024)                 &     (0.012)                 &     (0.024)                 &     (0.062)                 &     (0.005)                 &     (0.020)                 \\\midrule
$R^{2}$  &        .996                 &        .967                 &        .995                 &        .952                 &        .987                 &        .997                 \\
$N$      &         981                 &         981                 &         981                 &         959                 &         981                 &         981                 \\


==> inputs/south_95_16/Results4RICTint_ct_South_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $HHI_{c,t}$ & $Services_{c,t}$ & $Gini^{L}_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.163                 &      -0.034                 &       0.018                 &      -0.084$^{\ast\ast}$    &       0.017$^{\ast}$        &      -3.596$^{\ast}$        &      -0.012                 &      -0.021                 \\
            &     (0.083)                 &     (0.040)                 &     (0.061)                 &     (0.019)                 &     (0.005)                 &     (1.304)                 &     (0.010)                 &     (0.030)                 \\\addlinespace
$ICT_{c,t}$&       0.030                 &       0.043$^{\ast\ast}$    &      -0.044$^{\ast}$        &       0.099$^{\ast\ast\ast}$&       0.001                 &       0.712                 &      -0.000                 &       0.002                 \\
            &     (0.015)                 &     (0.013)                 &     (0.017)                 &     (0.006)                 &     (0.001)                 &     (0.355)                 &     (0.004)                 &     (0.005)                 \\\addlinespace
$R*ICT_{c,t}$&       0.034                 &      -0.064$^{\ast\ast}$    &      -0.031$^{\ast}$        &      -0.031$^{\ast\ast\ast}$&      -0.008$^{\ast\ast}$    &       0.944$^{\ast}$        &      -0.011                 &       0.010                 \\
            &     (0.017)                 &     (0.014)                 &     (0.010)                 &     (0.005)                 &     (0.002)                 &     (0.401)                 &     (0.006)                 &     (0.007)                 \\\midrule
$R^{2}$  &        .997                 &          0.999                &        .982                 &          0.999                &        .987                 &        .995                 &        .953                 &        .926                 \\
$N$      &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 \\


==> inputs/south_95_16/Results4shortRICTint_ct_South_95t16.tex <==
& ln $w_{c,t}$ & ln $L_{c,t}$ & ln $r_{c,t}$ & ln $K_{c,t}$ & $Services_{c,t}$ & $Gini^{w}_{c,t}$ \\\midrule \multicolumn{7}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.163                 &      -0.034                 &       0.018                 &      -0.084$^{\ast\ast}$    &      -3.596$^{\ast}$        &      -0.021                 \\
            &     (0.083)                 &     (0.040)                 &     (0.061)                 &     (0.019)                 &     (1.304)                 &     (0.030)                 \\\addlinespace
$ICT_{c,t}$&       0.030                 &       0.043$^{\ast\ast}$    &      -0.044$^{\ast}$        &       0.099$^{\ast\ast\ast}$&       0.712                 &       0.002                 \\
            &     (0.015)                 &     (0.013)                 &     (0.017)                 &     (0.006)                 &     (0.355)                 &     (0.005)                 \\\addlinespace
$R*ICT_{c,t}$&       0.034                 &      -0.064$^{\ast\ast}$    &      -0.031$^{\ast}$        &      -0.031$^{\ast\ast\ast}$&       0.944$^{\ast}$        &       0.010                 \\
            &     (0.017)                 &     (0.014)                 &     (0.010)                 &     (0.005)                 &     (0.401)                 &     (0.007)                 \\\midrule
$R^{2}$  &        .997                 &          0.999                &        .982                 &          0.999                &        .995                 &        .926                 \\
$N$      &          83                 &          83                 &          83                 &          83                 &          83                 &          83                 \\


==> inputs/south_95_16/Results5RICTint_ct_South_95t16.tex <==
& ln $wL_{c,t}$ & ln $rK_{c,t}$ & ln $(wL+rK)_{c,t}$ & ln $pQ_{c,t}$ & ln $Q_{c,t}$ & ln $p_{c,t}$ & ln $LProd_{c,t}$ & ln $TFP_{c,t}$ \\\midrule \multicolumn{9}{l}{\textbf{\emph{Panel A: full period 1995-2016}}} \\\midrule
$R_{c,t}$ &      -0.193                 &       0.176$^{\ast\ast}$    &      -0.055                 &       0.010                 &      -0.008                 &      -0.036                 &       0.039                 &       0.056                 \\
            &     (0.140)                 &     (0.040)                 &     (0.082)                 &     (0.045)                 &     (0.041)                 &     (0.041)                 &     (0.022)                 &     (0.021)                 \\\addlinespace
$ICT_{c,t}$&       0.055                 &       0.092$^{\ast\ast}$    &       0.070$^{\ast\ast}$    &       0.097$^{\ast\ast\ast}$&       0.092                 &       0.084$^{\ast\ast}$    &       0.027                 &      -0.006                 \\
            &     (0.023)                 &     (0.021)                 &     (0.013)                 &     (0.015)                 &     (0.053)                 &     (0.019)                 &     (0.033)                 &     (0.016)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.017                 &      -0.162$^{\ast\ast}$    &      -0.071$^{\ast}$        &      -0.103$^{\ast\ast\ast}$&      -0.078$^{\ast}$        &       0.009                 &      -0.021                 &      -0.016                 \\
            &     (0.038)                 &     (0.030)                 &     (0.023)                 &     (0.014)                 &     (0.018)                 &     (0.014)                 &     (0.016)                 &     (0.009)                 \\\midrule
$R^{2}$  &        .999                 &        .999                 &        .999                 &          0.999                &          0.999                &        .998                 &        .999                 &        .994                 \\
$N$      &          83                 &          83                 &          83                 &          83                 &          61                 &          61                 &          61                 &          61                 \\


==> inputs/south_subperiod/Results1RICTint_ct_South_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.329$^{\ast}$        &      -0.152                 &      -0.546                 &      -0.194                 &     -11.876$^{\ast\ast}$    &      -1.525                 &      -7.294$^{\ast}$        &      -3.057                 &       6.052                 &      -9.334                 &       4.973                 \\
            &     (0.139)                 &     (0.117)                 &     (0.384)                 &     (0.267)                 &     (3.600)                 &     (1.220)                 &     (2.476)                 &     (1.657)                 &     (3.201)                 &     (4.689)                 &     (6.883)                 \\\addlinespace
$ICT_{c,t}$&       0.039                 &      -0.006                 &       0.046                 &       0.091$^{\ast\ast}$    &       1.605                 &       0.025                 &       0.735                 &       0.845$^{\ast\ast}$    &      -2.092$^{\ast}$        &      -0.063                 &       1.298                 \\
            &     (0.031)                 &     (0.024)                 &     (0.076)                 &     (0.028)                 &     (0.893)                 &     (0.198)                 &     (0.796)                 &     (0.228)                 &     (0.881)                 &     (1.872)                 &     (1.178)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.066$^{\ast}$        &      -0.094$^{\ast}$        &      -0.084                 &      -0.004                 &      -1.393                 &      -0.727                 &      -0.705                 &       0.039                 &      -0.550                 &      -0.199                 &       1.862                 \\
            &     (0.021)                 &     (0.039)                 &     (0.047)                 &     (0.058)                 &     (0.703)                 &     (0.346)                 &     (0.465)                 &     (0.494)                 &     (1.159)                 &     (1.370)                 &     (2.353)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .992                 &        .994                 &         .99                 &        .993                 &        .986                 &        .974                 &        .993                 \\
$N$      &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 \\


==> inputs/south_subperiod/Results1RICTint_ct_South_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.428$^{\ast\ast}$    &      -0.388                 &      -0.784                 &      -0.182                 &     -12.186$^{\ast\ast}$    &      -2.540                 &      -8.536$^{\ast}$        &      -1.111                 &       3.842                 &     -11.378                 &       8.483                 \\
            &     (0.125)                 &     (0.245)                 &     (0.380)                 &     (0.242)                 &     (3.262)                 &     (2.450)                 &     (2.830)                 &     (2.351)                 &     (3.875)                 &     (7.832)                 &     (8.293)                 \\\addlinespace
$ICT_{c,t}$&      -0.140                 &      -0.236$^{\ast\ast}$    &      -0.280                 &       0.098                 &      -5.795$^{\ast}$        &      -3.293$^{\ast\ast}$    &      -3.255                 &       0.753                 &      -4.770$^{\ast\ast}$    &      -5.327                 &       7.326                 \\
            &     (0.077)                 &     (0.066)                 &     (0.155)                 &     (0.091)                 &     (2.388)                 &     (1.021)                 &     (1.796)                 &     (1.118)                 &     (1.385)                 &     (4.020)                 &     (3.980)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.013                 &      -0.071                 &       0.023                 &      -0.034                 &       1.345$^{\ast}$        &      -0.057                 &       1.199$^{\ast}$        &       0.203                 &      -1.695                 &       1.470                 &      -0.860                 \\
            &     (0.030)                 &     (0.045)                 &     (0.060)                 &     (0.038)                 &     (0.423)                 &     (0.436)                 &     (0.493)                 &     (0.444)                 &     (0.789)                 &     (1.588)                 &     (1.445)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .981                 &        .976                 &         .99                 &        .975                 &        .981                 &        .981                 &        .992                 \\
$N$      &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 \\


==> inputs/south_subperiod/Results2RICTint_ct_South_08t16.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.384                 &      -0.332$^{\ast}$        &      -0.773                 &       0.062                 &     -10.053$^{\ast}$        &      -1.729                 &      -7.012                 &      -1.312                 &       3.044                 &     -10.847                 &       9.006                 \\
            &     (0.181)                 &     (0.130)                 &     (0.419)                 &     (0.185)                 &     (3.567)                 &     (0.982)                 &     (3.203)                 &     (0.992)                 &     (2.594)                 &     (6.833)                 &     (5.686)                 \\\addlinespace
$ICT_{c,t}$&       0.051                 &       0.039                 &       0.079                 &       0.047                 &       0.967                 &       0.238                 &       0.572                 &       0.157                 &      -0.634                 &       0.393                 &      -0.536                 \\
            &     (0.048)                 &     (0.022)                 &     (0.095)                 &     (0.049)                 &     (1.198)                 &     (0.213)                 &     (1.010)                 &     (0.137)                 &     (0.755)                 &     (2.124)                 &     (0.919)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.053                 &      -0.041                 &      -0.048                 &      -0.054                 &      -1.513                 &      -0.467                 &      -0.835                 &      -0.210                 &       0.350                 &      -0.226                 &       0.865                 \\
            &     (0.038)                 &     (0.031)                 &     (0.079)                 &     (0.038)                 &     (0.715)                 &     (0.274)                 &     (0.588)                 &     (0.154)                 &     (0.931)                 &     (1.509)                 &     (0.824)                 \\\addlinespace
$wL_{c,t}$&       0.351                 &       0.605                 &       2.436                 &      -2.242$^{\ast}$        &      -0.958                 &       0.042                 &      -0.119                 &      -0.882$^{\ast\ast\ast}$&       1.396                 &       0.829                 &      -1.927                 \\
            &     (0.485)                 &     (0.397)                 &     (1.097)                 &     (0.830)                 &     (0.656)                 &     (0.208)                 &     (0.629)                 &     (0.126)                 &     (0.771)                 &     (1.287)                 &     (1.010)                 \\\addlinespace
$rK_{c,t}$&       0.267                 &       0.867$^{\ast}$        &       1.109$^{\ast\ast}$    &      -1.243$^{\ast\ast}$    &      -1.066                 &       0.170                 &      -0.188                 &      -1.048$^{\ast\ast\ast}$&       1.903$^{\ast}$        &       0.859                 &      -2.508$^{\ast\ast}$    \\
            &     (0.169)                 &     (0.308)                 &     (0.256)                 &     (0.368)                 &     (0.666)                 &     (0.117)                 &     (0.627)                 &     (0.072)                 &     (0.688)                 &     (1.270)                 &     (0.728)                 \\\addlinespace
$pQ_{c,t}$&       0.398                 &       0.008                 &      -2.175                 &       3.413$^{\ast\ast}$    &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.601)                 &     (0.311)                 &     (1.465)                 &     (0.977)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.002                 &      -0.012                 &       0.006                 &       0.005                 &      -0.109                 &      -0.081                 &      -0.016                 &      -0.012                 &      -0.175                 &       0.080                 &       0.102                 \\
            &     (0.005)                 &     (0.006)                 &     (0.014)                 &     (0.007)                 &     (0.161)                 &     (0.069)                 &     (0.099)                 &     (0.040)                 &     (0.091)                 &     (0.127)                 &     (0.237)                 \\\addlinespace
$Services_{c,t}$&      -0.006                 &      -0.011                 &      -0.034                 &       0.025                 &      -0.167                 &      -0.129                 &      -0.038                 &       0.000                 &      -0.289                 &      -0.201                 &       0.350                 \\
            &     (0.017)                 &     (0.015)                 &     (0.034)                 &     (0.024)                 &     (0.271)                 &     (0.088)                 &     (0.263)                 &     (0.081)                 &     (0.297)                 &     (0.505)                 &     (0.424)                 \\\addlinespace
$HHI_{c,t}$&      -4.953$^{\ast}$        &      -5.104                 &      -2.218                 &      -7.507$^{\ast\ast\ast}$&     -31.593                 &     -47.814$^{\ast}$        &       6.422                 &       9.798                 &    -150.883                 &      -4.442                 &     100.503                 \\
            &     (1.729)                 &     (2.725)                 &     (5.155)                 &     (1.202)                 &    (71.039)                 &    (16.303)                 &    (76.111)                 &    (13.611)                 &   (118.158)                 &   (154.686)                 &    (52.185)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.000                 &      -0.000                 &       0.000                 &      -0.003$^{\ast}$        &      -0.017                 &      -0.017                 &      -0.024                 &       0.024$^{\ast\ast}$    &      -0.049$^{\ast}$        &      -0.053                 &       0.105                 \\
            &     (0.001)                 &     (0.002)                 &     (0.002)                 &     (0.001)                 &     (0.039)                 &     (0.013)                 &     (0.027)                 &     (0.004)                 &     (0.018)                 &     (0.047)                 &     (0.047)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.000                 &      -0.031                 &      -0.021                 &       0.072$^{\ast}$        &      -0.283                 &       0.003                 &       0.167                 &      -0.452$^{\ast\ast}$    &       0.437                 &       0.659                 &      -1.002                 \\
            &     (0.006)                 &     (0.022)                 &     (0.032)                 &     (0.029)                 &     (0.204)                 &     (0.125)                 &     (0.193)                 &     (0.094)                 &     (0.300)                 &     (0.483)                 &     (0.427)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.003                 &       0.003                 &       0.005                 &      -0.000                 &       0.023                 &       0.013                 &       0.029                 &      -0.019                 &       0.020                 &       0.044                 &      -0.108                 \\
            &     (0.002)                 &     (0.003)                 &     (0.005)                 &     (0.003)                 &     (0.056)                 &     (0.020)                 &     (0.059)                 &     (0.018)                 &     (0.064)                 &     (0.159)                 &     (0.085)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&      -0.011                 &      -0.023                 &      -0.027                 &       0.015                 &      -0.037                 &      -0.132                 &       0.125                 &      -0.030                 &      -0.398                 &      -0.108                 &       0.289                 \\
            &     (0.009)                 &     (0.018)                 &     (0.033)                 &     (0.022)                 &     (0.136)                 &     (0.124)                 &     (0.220)                 &     (0.075)                 &     (0.367)                 &     (0.689)                 &     (0.312)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .994                 &        .995                 &         .99                 &        .999                 &        .993                 &        .975                 &        .996                 \\
$N$      &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 \\


==> inputs/south_subperiod/Results2RICTint_ct_South_95t07.tex <==
&\multicolumn{4}{c}{Taxes in ln of nat. currency}& \multicolumn{4}{c}{Taxes as \% of GDP}& \multicolumn{3}{c}{Taxes as \% of total tax}\\\midrule & ln $T_{c,t}$ & ln $T^l_{c,t}$ & ln $T^k_{c,t}$ & ln$T^y_{c,t}$ & $T_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ & $T^l_{c,t}$ & $T^k_{c,t}$ & $T^y_{c,t}$ \\\midrule 
$R_{c,t}$ &      -0.388$^{\ast\ast}$    &      -0.259                 &      -0.565$^{\ast}$        &      -0.385$^{\ast}$        &     -10.997$^{\ast\ast}$    &      -1.285                 &      -7.763$^{\ast\ast}$    &      -1.949$^{\ast\ast}$    &       6.488$^{\ast\ast}$    &      -9.874                 &       5.615                 \\
            &     (0.111)                 &     (0.119)                 &     (0.201)                 &     (0.123)                 &     (3.270)                 &     (1.477)                 &     (2.375)                 &     (0.587)                 &     (1.157)                 &     (4.882)                 &     (4.968)                 \\\addlinespace
$ICT_{c,t}$&      -0.102                 &      -0.115                 &      -0.131                 &      -0.046                 &      -5.088                 &      -1.759                 &      -1.620                 &      -1.709$^{\ast\ast}$    &      -0.710                 &      -0.848                 &       0.456                 \\
            &     (0.090)                 &     (0.101)                 &     (0.200)                 &     (0.080)                 &     (2.961)                 &     (0.975)                 &     (2.275)                 &     (0.412)                 &     (0.657)                 &     (4.096)                 &     (3.753)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.015                 &      -0.076                 &       0.120$^{\ast\ast}$    &      -0.115$^{\ast}$        &       1.376$^{\ast}$        &      -0.163                 &       1.013$^{\ast}$        &       0.525$^{\ast\ast}$    &      -2.062$^{\ast\ast\ast}$&       0.881                 &      -0.030                 \\
            &     (0.034)                 &     (0.050)                 &     (0.036)                 &     (0.041)                 &     (0.553)                 &     (0.270)                 &     (0.421)                 &     (0.141)                 &     (0.324)                 &     (1.002)                 &     (0.913)                 \\\addlinespace
$wL_{c,t}$&       0.132                 &       0.412                 &       2.065$^{\ast}$        &      -1.803$^{\ast\ast}$    &      -0.542                 &      -0.092                 &       0.365                 &      -0.815$^{\ast\ast}$    &       0.311                 &       1.501$^{\ast}$        &      -1.843$^{\ast}$        \\
            &     (0.370)                 &     (0.542)                 &     (0.761)                 &     (0.456)                 &     (0.388)                 &     (0.190)                 &     (0.270)                 &     (0.153)                 &     (0.263)                 &     (0.535)                 &     (0.641)                 \\\addlinespace
$rK_{c,t}$&      -0.166                 &      -0.556$^{\ast}$        &       0.610                 &      -0.439$^{\ast}$        &      -0.938$^{\ast}$        &      -0.439$^{\ast\ast}$    &       0.213                 &      -0.713$^{\ast\ast}$    &      -0.346                 &       1.323$^{\ast\ast}$    &      -1.353$^{\ast}$        \\
            &     (0.176)                 &     (0.176)                 &     (0.431)                 &     (0.144)                 &     (0.306)                 &     (0.121)                 &     (0.212)                 &     (0.127)                 &     (0.207)                 &     (0.401)                 &     (0.471)                 \\\addlinespace
$pQ_{c,t}$&       0.260                 &       0.109                 &      -1.056                 &       0.923$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.555)                 &     (0.623)                 &     (1.547)                 &     (0.333)                 &                             &                             &                             &                             &                             &                             &                             \\\addlinespace
$GDPgrowth_{c,t}$&      -0.003                 &       0.004                 &      -0.018$^{\ast}$        &       0.006                 &      -0.174                 &       0.023                 &      -0.167                 &      -0.029                 &       0.242$^{\ast}$        &      -0.343                 &       0.159                 \\
            &     (0.006)                 &     (0.007)                 &     (0.007)                 &     (0.008)                 &     (0.097)                 &     (0.035)                 &     (0.094)                 &     (0.084)                 &     (0.100)                 &     (0.222)                 &     (0.256)                 \\\addlinespace
$Services_{c,t}$&      -0.004                 &       0.015                 &      -0.099$^{\ast}$        &       0.060$^{\ast\ast}$    &      -0.529                 &       0.027                 &      -0.706$^{\ast}$        &       0.149                 &       0.642                 &      -1.386$^{\ast}$        &       1.077$^{\ast}$        \\
            &     (0.014)                 &     (0.021)                 &     (0.039)                 &     (0.015)                 &     (0.502)                 &     (0.221)                 &     (0.270)                 &     (0.110)                 &     (0.283)                 &     (0.503)                 &     (0.417)                 \\\addlinespace
$HHI_{c,t}$&     -10.445                 &      -6.114                 &     -30.324$^{\ast\ast}$    &       3.208                 &    -348.658$^{\ast}$        &     -68.918                 &    -293.377$^{\ast\ast}$    &      13.637                 &     124.267$^{\ast}$        &    -613.334$^{\ast\ast}$    &     396.704$^{\ast\ast}$    \\
            &     (4.584)                 &     (4.367)                 &     (7.599)                 &     (3.817)                 &   (146.418)                 &    (50.586)                 &    (79.913)                 &    (32.846)                 &    (49.023)                 &   (121.922)                 &    (95.655)                 \\\addlinespace
$Debt^{\%GDP}_{c,t}$&      -0.008                 &      -0.008                 &      -0.003                 &      -0.016$^{\ast\ast}$    &      -0.109                 &      -0.015                 &      -0.078                 &      -0.015                 &       0.050                 &      -0.146                 &       0.048                 \\
            &     (0.005)                 &     (0.005)                 &     (0.007)                 &     (0.005)                 &     (0.064)                 &     (0.022)                 &     (0.051)                 &     (0.011)                 &     (0.030)                 &     (0.103)                 &     (0.090)                 \\\addlinespace
$Interest^{\%GDP}_{c,t}$&       0.003                 &       0.017                 &      -0.031                 &       0.013                 &       0.037                 &       0.209                 &      -0.133                 &      -0.039                 &       0.675                 &      -0.371                 &       0.708                 \\
            &     (0.013)                 &     (0.015)                 &     (0.027)                 &     (0.014)                 &     (0.472)                 &     (0.155)                 &     (0.319)                 &     (0.107)                 &     (0.310)                 &     (0.663)                 &     (0.465)                 \\\addlinespace
$Lending^{\%GDP}_{c,t}$&       0.016                 &       0.011                 &       0.025                 &       0.011                 &       0.444                 &       0.096                 &       0.352$^{\ast}$        &      -0.004                 &      -0.114                 &       0.654$^{\ast}$        &      -0.367                 \\
            &     (0.008)                 &     (0.011)                 &     (0.013)                 &     (0.007)                 &     (0.248)                 &     (0.118)                 &     (0.134)                 &     (0.056)                 &     (0.119)                 &     (0.206)                 &     (0.218)                 \\\addlinespace
$GovInv^{\%GDP}_{c,t}$&       0.012                 &       0.034                 &      -0.035                 &       0.019                 &       0.203                 &       0.361                 &      -0.066                 &      -0.092                 &       0.959$^{\ast}$        &      -0.048                 &      -0.131                 \\
            &     (0.017)                 &     (0.027)                 &     (0.037)                 &     (0.018)                 &     (0.605)                 &     (0.291)                 &     (0.272)                 &     (0.145)                 &     (0.343)                 &     (0.576)                 &     (0.545)                 \\\addlinespace
$XRate_{c,t}$&       0.840                 &       0.028                 &       2.373$^{\ast\ast}$    &       0.564                 &      10.241                 &      -7.190                 &      22.429$^{\ast\ast}$    &      -4.998                 &     -25.622$^{\ast}$        &      73.655$^{\ast\ast\ast}$&     -33.538$^{\ast}$        \\
            &     (0.487)                 &     (0.515)                 &     (0.735)                 &     (0.500)                 &    (13.471)                 &     (6.928)                 &     (5.940)                 &     (3.275)                 &    (10.534)                 &     (9.454)                 &    (11.738)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .986                 &        .988                 &        .991                 &         .99                 &        .989                 &        .986                 &        .995                 \\
$N$      &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 \\


==> inputs/south_subperiod/Results2shortEXCGDPV1_RICTint_ct_South_08t16.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.384                 &      -0.332$^{\ast}$        &      -0.773                 &       0.062                 &       3.044                 &     -10.847                 &       9.006                 \\
            &     (0.181)                 &     (0.130)                 &     (0.419)                 &     (0.185)                 &     (2.594)                 &     (6.833)                 &     (5.686)                 \\\addlinespace
$ICT_{c,t}$&       0.051                 &       0.039                 &       0.079                 &       0.047                 &      -0.634                 &       0.393                 &      -0.536                 \\
            &     (0.048)                 &     (0.022)                 &     (0.095)                 &     (0.049)                 &     (0.755)                 &     (2.124)                 &     (0.919)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.053                 &      -0.041                 &      -0.048                 &      -0.054                 &       0.350                 &      -0.226                 &       0.865                 \\
            &     (0.038)                 &     (0.031)                 &     (0.079)                 &     (0.038)                 &     (0.931)                 &     (1.509)                 &     (0.824)                 \\\addlinespace
$wL_{c,t}$&       0.351                 &       0.605                 &       2.436                 &      -2.242$^{\ast}$        &       1.396                 &       0.829                 &      -1.927                 \\
            &     (0.485)                 &     (0.397)                 &     (1.097)                 &     (0.830)                 &     (0.771)                 &     (1.287)                 &     (1.010)                 \\\addlinespace
$rK_{c,t}$&       0.267                 &       0.867$^{\ast}$        &       1.109$^{\ast\ast}$    &      -1.243$^{\ast\ast}$    &       1.903$^{\ast}$        &       0.859                 &      -2.508$^{\ast\ast}$    \\
            &     (0.169)                 &     (0.308)                 &     (0.256)                 &     (0.368)                 &     (0.688)                 &     (1.270)                 &     (0.728)                 \\\addlinespace
$pQ_{c,t}$&       0.398                 &       0.008                 &      -2.175                 &       3.413$^{\ast\ast}$    &                             &                             &                             \\
            &     (0.601)                 &     (0.311)                 &     (1.465)                 &     (0.977)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .993                 &        .975                 &        .996                 \\
$N$      &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 \\


==> inputs/south_subperiod/Results2shortEXCGDPV1_RICTint_ct_South_95t07.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.388$^{\ast\ast}$    &      -0.259                 &      -0.565$^{\ast}$        &      -0.385$^{\ast}$        &       6.488$^{\ast\ast}$    &      -9.874                 &       5.615                 \\
            &     (0.111)                 &     (0.119)                 &     (0.201)                 &     (0.123)                 &     (1.157)                 &     (4.882)                 &     (4.968)                 \\\addlinespace
$ICT_{c,t}$&      -0.102                 &      -0.115                 &      -0.131                 &      -0.046                 &      -0.710                 &      -0.848                 &       0.456                 \\
            &     (0.090)                 &     (0.101)                 &     (0.200)                 &     (0.080)                 &     (0.657)                 &     (4.096)                 &     (3.753)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.015                 &      -0.076                 &       0.120$^{\ast\ast}$    &      -0.115$^{\ast}$        &      -2.062$^{\ast\ast\ast}$&       0.881                 &      -0.030                 \\
            &     (0.034)                 &     (0.050)                 &     (0.036)                 &     (0.041)                 &     (0.324)                 &     (1.002)                 &     (0.913)                 \\\addlinespace
$wL_{c,t}$&       0.132                 &       0.412                 &       2.065$^{\ast}$        &      -1.803$^{\ast\ast}$    &       0.311                 &       1.501$^{\ast}$        &      -1.843$^{\ast}$        \\
            &     (0.370)                 &     (0.542)                 &     (0.761)                 &     (0.456)                 &     (0.263)                 &     (0.535)                 &     (0.641)                 \\\addlinespace
$rK_{c,t}$&      -0.166                 &      -0.556$^{\ast}$        &       0.610                 &      -0.439$^{\ast}$        &      -0.346                 &       1.323$^{\ast\ast}$    &      -1.353$^{\ast}$        \\
            &     (0.176)                 &     (0.176)                 &     (0.431)                 &     (0.144)                 &     (0.207)                 &     (0.401)                 &     (0.471)                 \\\addlinespace
$pQ_{c,t}$&       0.260                 &       0.109                 &      -1.056                 &       0.923$^{\ast}$        &                             &                             &                             \\
            &     (0.555)                 &     (0.623)                 &     (1.547)                 &     (0.333)                 &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .989                 &        .986                 &        .995                 \\
$N$      &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 \\


==> inputs/south_subperiod/Results2shortEXCGDPV2_RICTint_ct_South_08t16.tex <==
\multicolumn{4}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       3.044                 &     -10.847                 &       9.006                 \\
            &     (2.594)                 &     (6.833)                 &     (5.686)                 \\\addlinespace
$ICT_{c,t}$&      -0.634                 &       0.393                 &      -0.536                 \\
            &     (0.755)                 &     (2.124)                 &     (0.919)                 \\\addlinespace
$R*ICT_{c,t}$&       0.350                 &      -0.226                 &       0.865                 \\
            &     (0.931)                 &     (1.509)                 &     (0.824)                 \\\addlinespace
$wL_{c,t}$&       1.396                 &       0.829                 &      -1.927                 \\
            &     (0.771)                 &     (1.287)                 &     (1.010)                 \\\addlinespace
$rK_{c,t}$&       1.903$^{\ast}$        &       0.859                 &      -2.508$^{\ast\ast}$    \\
            &     (0.688)                 &     (1.270)                 &     (0.728)                 \\\midrule
$R^{2}$  &        .993                 &        .975                 &        .996                 \\
$N$      &          36                 &          36                 &          36                 \\


==> inputs/south_subperiod/Results2shortEXCGDPV2_RICTint_ct_South_95t07.tex <==
\multicolumn{4}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &       6.488$^{\ast\ast}$    &      -9.874                 &       5.615                 \\
            &     (1.157)                 &     (4.882)                 &     (4.968)                 \\\addlinespace
$ICT_{c,t}$&      -0.710                 &      -0.848                 &       0.456                 \\
            &     (0.657)                 &     (4.096)                 &     (3.753)                 \\\addlinespace
$R*ICT_{c,t}$&      -2.062$^{\ast\ast\ast}$&       0.881                 &      -0.030                 \\
            &     (0.324)                 &     (1.002)                 &     (0.913)                 \\\addlinespace
$wL_{c,t}$&       0.311                 &       1.501$^{\ast}$        &      -1.843$^{\ast}$        \\
            &     (0.263)                 &     (0.535)                 &     (0.641)                 \\\addlinespace
$rK_{c,t}$&      -0.346                 &       1.323$^{\ast\ast}$    &      -1.353$^{\ast}$        \\
            &     (0.207)                 &     (0.401)                 &     (0.471)                 \\\midrule
$R^{2}$  &        .989                 &        .986                 &        .995                 \\
$N$      &          47                 &          47                 &          47                 \\


==> inputs/south_subperiod/Results2shortV1_RICTint_ct_South_08t16.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &      -0.384                 &      -0.332$^{\ast}$        &      -0.773                 &       0.062                 &     -10.053$^{\ast}$        &      -1.729                 &      -7.012                 &      -1.312                 &       3.044                 &     -10.847                 &       9.006                 \\
            &     (0.181)                 &     (0.130)                 &     (0.419)                 &     (0.185)                 &     (3.567)                 &     (0.982)                 &     (3.203)                 &     (0.992)                 &     (2.594)                 &     (6.833)                 &     (5.686)                 \\\addlinespace
$ICT_{c,t}$&       0.051                 &       0.039                 &       0.079                 &       0.047                 &       0.967                 &       0.238                 &       0.572                 &       0.157                 &      -0.634                 &       0.393                 &      -0.536                 \\
            &     (0.048)                 &     (0.022)                 &     (0.095)                 &     (0.049)                 &     (1.198)                 &     (0.213)                 &     (1.010)                 &     (0.137)                 &     (0.755)                 &     (2.124)                 &     (0.919)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.053                 &      -0.041                 &      -0.048                 &      -0.054                 &      -1.513                 &      -0.467                 &      -0.835                 &      -0.210                 &       0.350                 &      -0.226                 &       0.865                 \\
            &     (0.038)                 &     (0.031)                 &     (0.079)                 &     (0.038)                 &     (0.715)                 &     (0.274)                 &     (0.588)                 &     (0.154)                 &     (0.931)                 &     (1.509)                 &     (0.824)                 \\\addlinespace
$wL_{c,t}$&       0.351                 &       0.605                 &       2.436                 &      -2.242$^{\ast}$        &      -0.958                 &       0.042                 &      -0.119                 &      -0.882$^{\ast\ast\ast}$&       1.396                 &       0.829                 &      -1.927                 \\
            &     (0.485)                 &     (0.397)                 &     (1.097)                 &     (0.830)                 &     (0.656)                 &     (0.208)                 &     (0.629)                 &     (0.126)                 &     (0.771)                 &     (1.287)                 &     (1.010)                 \\\addlinespace
$rK_{c,t}$&       0.267                 &       0.867$^{\ast}$        &       1.109$^{\ast\ast}$    &      -1.243$^{\ast\ast}$    &      -1.066                 &       0.170                 &      -0.188                 &      -1.048$^{\ast\ast\ast}$&       1.903$^{\ast}$        &       0.859                 &      -2.508$^{\ast\ast}$    \\
            &     (0.169)                 &     (0.308)                 &     (0.256)                 &     (0.368)                 &     (0.666)                 &     (0.117)                 &     (0.627)                 &     (0.072)                 &     (0.688)                 &     (1.270)                 &     (0.728)                 \\\addlinespace
$pQ_{c,t}$&       0.398                 &       0.008                 &      -2.175                 &       3.413$^{\ast\ast}$    &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.601)                 &     (0.311)                 &     (1.465)                 &     (0.977)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .994                 &        .995                 &         .99                 &        .999                 &        .993                 &        .975                 &        .996                 \\
$N$      &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 \\


==> inputs/south_subperiod/Results2shortV1_RICTint_ct_South_95t07.tex <==
\multicolumn{12}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.388$^{\ast\ast}$    &      -0.259                 &      -0.565$^{\ast}$        &      -0.385$^{\ast}$        &     -10.997$^{\ast\ast}$    &      -1.285                 &      -7.763$^{\ast\ast}$    &      -1.949$^{\ast\ast}$    &       6.488$^{\ast\ast}$    &      -9.874                 &       5.615                 \\
            &     (0.111)                 &     (0.119)                 &     (0.201)                 &     (0.123)                 &     (3.270)                 &     (1.477)                 &     (2.375)                 &     (0.587)                 &     (1.157)                 &     (4.882)                 &     (4.968)                 \\\addlinespace
$ICT_{c,t}$&      -0.102                 &      -0.115                 &      -0.131                 &      -0.046                 &      -5.088                 &      -1.759                 &      -1.620                 &      -1.709$^{\ast\ast}$    &      -0.710                 &      -0.848                 &       0.456                 \\
            &     (0.090)                 &     (0.101)                 &     (0.200)                 &     (0.080)                 &     (2.961)                 &     (0.975)                 &     (2.275)                 &     (0.412)                 &     (0.657)                 &     (4.096)                 &     (3.753)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.015                 &      -0.076                 &       0.120$^{\ast\ast}$    &      -0.115$^{\ast}$        &       1.376$^{\ast}$        &      -0.163                 &       1.013$^{\ast}$        &       0.525$^{\ast\ast}$    &      -2.062$^{\ast\ast\ast}$&       0.881                 &      -0.030                 \\
            &     (0.034)                 &     (0.050)                 &     (0.036)                 &     (0.041)                 &     (0.553)                 &     (0.270)                 &     (0.421)                 &     (0.141)                 &     (0.324)                 &     (1.002)                 &     (0.913)                 \\\addlinespace
$wL_{c,t}$&       0.132                 &       0.412                 &       2.065$^{\ast}$        &      -1.803$^{\ast\ast}$    &      -0.542                 &      -0.092                 &       0.365                 &      -0.815$^{\ast\ast}$    &       0.311                 &       1.501$^{\ast}$        &      -1.843$^{\ast}$        \\
            &     (0.370)                 &     (0.542)                 &     (0.761)                 &     (0.456)                 &     (0.388)                 &     (0.190)                 &     (0.270)                 &     (0.153)                 &     (0.263)                 &     (0.535)                 &     (0.641)                 \\\addlinespace
$rK_{c,t}$&      -0.166                 &      -0.556$^{\ast}$        &       0.610                 &      -0.439$^{\ast}$        &      -0.938$^{\ast}$        &      -0.439$^{\ast\ast}$    &       0.213                 &      -0.713$^{\ast\ast}$    &      -0.346                 &       1.323$^{\ast\ast}$    &      -1.353$^{\ast}$        \\
            &     (0.176)                 &     (0.176)                 &     (0.431)                 &     (0.144)                 &     (0.306)                 &     (0.121)                 &     (0.212)                 &     (0.127)                 &     (0.207)                 &     (0.401)                 &     (0.471)                 \\\addlinespace
$pQ_{c,t}$&       0.260                 &       0.109                 &      -1.056                 &       0.923$^{\ast}$        &                             &                             &                             &                             &                             &                             &                             \\
            &     (0.555)                 &     (0.623)                 &     (1.547)                 &     (0.333)                 &                             &                             &                             &                             &                             &                             &                             \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &        .986                 &        .988                 &        .991                 &         .99                 &        .989                 &        .986                 &        .995                 \\
$N$      &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 \\


==> inputs/south_subperiod/Results2shortV2_RICTint_ct_South_08t16.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &     -10.053$^{\ast}$        &      -1.729                 &      -7.012                 &      -1.312                 &       3.044                 &     -10.847                 &       9.006                 \\
            &     (3.567)                 &     (0.982)                 &     (3.203)                 &     (0.992)                 &     (2.594)                 &     (6.833)                 &     (5.686)                 \\\addlinespace
$ICT_{c,t}$&       0.967                 &       0.238                 &       0.572                 &       0.157                 &      -0.634                 &       0.393                 &      -0.536                 \\
            &     (1.198)                 &     (0.213)                 &     (1.010)                 &     (0.137)                 &     (0.755)                 &     (2.124)                 &     (0.919)                 \\\addlinespace
$R*ICT_{c,t}$&      -1.513                 &      -0.467                 &      -0.835                 &      -0.210                 &       0.350                 &      -0.226                 &       0.865                 \\
            &     (0.715)                 &     (0.274)                 &     (0.588)                 &     (0.154)                 &     (0.931)                 &     (1.509)                 &     (0.824)                 \\\addlinespace
$wL_{c,t}$&      -0.958                 &       0.042                 &      -0.119                 &      -0.882$^{\ast\ast\ast}$&       1.396                 &       0.829                 &      -1.927                 \\
            &     (0.656)                 &     (0.208)                 &     (0.629)                 &     (0.126)                 &     (0.771)                 &     (1.287)                 &     (1.010)                 \\\addlinespace
$rK_{c,t}$&      -1.066                 &       0.170                 &      -0.188                 &      -1.048$^{\ast\ast\ast}$&       1.903$^{\ast}$        &       0.859                 &      -2.508$^{\ast\ast}$    \\
            &     (0.666)                 &     (0.117)                 &     (0.627)                 &     (0.072)                 &     (0.688)                 &     (1.270)                 &     (0.728)                 \\\midrule
$R^{2}$  &        .994                 &        .995                 &         .99                 &        .999                 &        .993                 &        .975                 &        .996                 \\
$N$      &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 \\


==> inputs/south_subperiod/Results2shortV2_RICTint_ct_South_95t07.tex <==
\multicolumn{8}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &     -10.997$^{\ast\ast}$    &      -1.285                 &      -7.763$^{\ast\ast}$    &      -1.949$^{\ast\ast}$    &       6.488$^{\ast\ast}$    &      -9.874                 &       5.615                 \\
            &     (3.270)                 &     (1.477)                 &     (2.375)                 &     (0.587)                 &     (1.157)                 &     (4.882)                 &     (4.968)                 \\\addlinespace
$ICT_{c,t}$&      -5.088                 &      -1.759                 &      -1.620                 &      -1.709$^{\ast\ast}$    &      -0.710                 &      -0.848                 &       0.456                 \\
            &     (2.961)                 &     (0.975)                 &     (2.275)                 &     (0.412)                 &     (0.657)                 &     (4.096)                 &     (3.753)                 \\\addlinespace
$R*ICT_{c,t}$&       1.376$^{\ast}$        &      -0.163                 &       1.013$^{\ast}$        &       0.525$^{\ast\ast}$    &      -2.062$^{\ast\ast\ast}$&       0.881                 &      -0.030                 \\
            &     (0.553)                 &     (0.270)                 &     (0.421)                 &     (0.141)                 &     (0.324)                 &     (1.002)                 &     (0.913)                 \\\addlinespace
$wL_{c,t}$&      -0.542                 &      -0.092                 &       0.365                 &      -0.815$^{\ast\ast}$    &       0.311                 &       1.501$^{\ast}$        &      -1.843$^{\ast}$        \\
            &     (0.388)                 &     (0.190)                 &     (0.270)                 &     (0.153)                 &     (0.263)                 &     (0.535)                 &     (0.641)                 \\\addlinespace
$rK_{c,t}$&      -0.938$^{\ast}$        &      -0.439$^{\ast\ast}$    &       0.213                 &      -0.713$^{\ast\ast}$    &      -0.346                 &       1.323$^{\ast\ast}$    &      -1.353$^{\ast}$        \\
            &     (0.306)                 &     (0.121)                 &     (0.212)                 &     (0.127)                 &     (0.207)                 &     (0.401)                 &     (0.471)                 \\\midrule
$R^{2}$  &        .986                 &        .988                 &        .991                 &         .99                 &        .989                 &        .986                 &        .995                 \\
$N$      &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 \\


==> inputs/south_subperiod/Results3RICTint_cit_South_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{i,c,t}$&      -0.068                 &       0.184                 &      -0.252                 &      -0.710                 &      -0.055                 &      -0.052                 \\
            &     (0.159)                 &     (0.131)                 &     (0.151)                 &     (0.547)                 &     (0.035)                 &     (0.084)                 \\\addlinespace
$ICT_{i,c,t}$&       0.084$^{\ast\ast}$    &       0.048                 &       0.036                 &       0.114                 &       0.029$^{\ast\ast}$    &       0.036                 \\
            &     (0.029)                 &     (0.029)                 &     (0.033)                 &     (0.097)                 &     (0.013)                 &     (0.023)                 \\\addlinespace
$R*ICT_{i,c,t}$&       0.099$^{\ast}$        &       0.007                 &       0.092                 &       0.202                 &       0.025$^{\ast}$        &      -0.103$^{\ast\ast}$    \\
            &     (0.053)                 &     (0.031)                 &     (0.052)                 &     (0.140)                 &     (0.011)                 &     (0.041)                 \\\midrule
$R^{2}$  &        .998                 &        .972                 &        .998                 &        .978                 &        .874                 &        .999                 \\
$N$      &         405                 &         405                 &         405                 &         396                 &         405                 &         405                 \\


==> inputs/south_subperiod/Results3RICTint_cit_South_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{i,c,t}$&       0.026                 &       0.052$^{\ast\ast}$    &      -0.026                 &      -0.085$^{\ast}$        &      -0.007                 &      -0.003                 \\
            &     (0.020)                 &     (0.022)                 &     (0.023)                 &     (0.046)                 &     (0.006)                 &     (0.029)                 \\\addlinespace
$ICT_{i,c,t}$&       0.090$^{\ast}$        &       0.097                 &      -0.007                 &      -0.378                 &      -0.009                 &       0.054                 \\
            &     (0.042)                 &     (0.062)                 &     (0.045)                 &     (0.232)                 &     (0.008)                 &     (0.036)                 \\\addlinespace
$R*ICT_{i,c,t}$&      -0.013                 &      -0.017$^{\ast\ast}$    &       0.005                 &      -0.048$^{\ast}$        &       0.004$^{\ast}$        &      -0.017$^{\ast}$        \\
            &     (0.009)                 &     (0.007)                 &     (0.007)                 &     (0.025)                 &     (0.002)                 &     (0.009)                 \\\midrule
$R^{2}$  &        .998                 &         .97                 &        .998                 &        .959                 &        .992                 &        .999                 \\
$N$      &         576                 &         576                 &         576                 &         563                 &         576                 &         576                 \\


==> inputs/south_subperiod/Results4RICTint_ct_South_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.262$^{\ast\ast\ast}$&       0.112                 &       0.309$^{\ast}$        &       0.101$^{\ast}$        &      -0.006                 &       0.011                 &      -0.007                 &       0.017                 \\
            &     (0.041)                 &     (0.050)                 &     (0.105)                 &     (0.042)                 &     (0.007)                 &     (2.620)                 &     (0.011)                 &     (0.033)                 \\\addlinespace
$ICT_{c,t}$&       0.006                 &      -0.050                 &      -0.110$^{\ast\ast}$    &       0.031$^{\ast}$        &      -0.003                 &       1.791$^{\ast}$        &      -0.003                 &       0.005                 \\
            &     (0.011)                 &     (0.032)                 &     (0.033)                 &     (0.012)                 &     (0.001)                 &     (0.643)                 &     (0.004)                 &     (0.008)                 \\\addlinespace
$R*ICT_{c,t}$&       0.022                 &       0.015                 &      -0.004                 &       0.019                 &      -0.004                 &       0.394                 &      -0.008$^{\ast}$        &       0.010                 \\
            &     (0.012)                 &     (0.027)                 &     (0.034)                 &     (0.009)                 &     (0.004)                 &     (0.684)                 &     (0.003)                 &     (0.008)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .946                 &          0.999                &         .99                 &        .996                 &        .992                 &        .976                 \\
$N$      &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 \\


==> inputs/south_subperiod/Results4RICTint_ct_South_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.181$^{\ast}$        &      -0.053                 &      -0.054                 &      -0.111$^{\ast\ast}$    &      -0.011                 &      -0.455                 &       0.018                 &      -0.118                 \\
            &     (0.058)                 &     (0.057)                 &     (0.090)                 &     (0.031)                 &     (0.007)                 &     (2.112)                 &     (0.021)                 &     (0.080)                 \\\addlinespace
$ICT_{c,t}$&      -0.018                 &      -0.015                 &      -0.000                 &       0.045$^{\ast\ast\ast}$&      -0.018$^{\ast\ast}$    &       2.840                 &      -0.010                 &      -0.082                 \\
            &     (0.046)                 &     (0.030)                 &     (0.061)                 &     (0.007)                 &     (0.005)                 &     (1.340)                 &     (0.011)                 &     (0.037)                 \\\addlinespace
$R*ICT_{c,t}$&       0.014                 &      -0.048$^{\ast}$        &      -0.012                 &      -0.019$^{\ast}$        &      -0.001                 &       0.353                 &      -0.017$^{\ast}$        &       0.018                 \\
            &     (0.016)                 &     (0.018)                 &     (0.030)                 &     (0.007)                 &     (0.001)                 &     (0.359)                 &     (0.006)                 &     (0.017)                 \\\midrule
$R^{2}$  &        .998                 &          0.999                &        .989                 &          0.999                &        .997                 &        .997                 &        .976                 &        .945                 \\
$N$      &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 \\


==> inputs/south_subperiod/Results4shortRICTint_ct_South_08t16.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.262$^{\ast\ast\ast}$&       0.112                 &       0.309$^{\ast}$        &       0.101$^{\ast}$        &       0.011                 &       0.017                 \\
            &     (0.041)                 &     (0.050)                 &     (0.105)                 &     (0.042)                 &     (2.620)                 &     (0.033)                 \\\addlinespace
$ICT_{c,t}$&       0.006                 &      -0.050                 &      -0.110$^{\ast\ast}$    &       0.031$^{\ast}$        &       1.791$^{\ast}$        &       0.005                 \\
            &     (0.011)                 &     (0.032)                 &     (0.033)                 &     (0.012)                 &     (0.643)                 &     (0.008)                 \\\addlinespace
$R*ICT_{c,t}$&       0.022                 &       0.015                 &      -0.004                 &       0.019                 &       0.394                 &       0.010                 \\
            &     (0.012)                 &     (0.027)                 &     (0.034)                 &     (0.009)                 &     (0.684)                 &     (0.008)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &        .946                 &          0.999                &        .996                 &        .976                 \\
$N$      &          36                 &          36                 &          36                 &          36                 &          36                 &          36                 \\


==> inputs/south_subperiod/Results4shortRICTint_ct_South_95t07.tex <==
\multicolumn{7}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.181$^{\ast}$        &      -0.053                 &      -0.054                 &      -0.111$^{\ast\ast}$    &      -0.455                 &      -0.118                 \\
            &     (0.058)                 &     (0.057)                 &     (0.090)                 &     (0.031)                 &     (2.112)                 &     (0.080)                 \\\addlinespace
$ICT_{c,t}$&      -0.018                 &      -0.015                 &      -0.000                 &       0.045$^{\ast\ast\ast}$&       2.840                 &      -0.082                 \\
            &     (0.046)                 &     (0.030)                 &     (0.061)                 &     (0.007)                 &     (1.340)                 &     (0.037)                 \\\addlinespace
$R*ICT_{c,t}$&       0.014                 &      -0.048$^{\ast}$        &      -0.012                 &      -0.019$^{\ast}$        &       0.353                 &       0.018                 \\
            &     (0.016)                 &     (0.018)                 &     (0.030)                 &     (0.007)                 &     (0.359)                 &     (0.017)                 \\\midrule
$R^{2}$  &        .998                 &          0.999                &        .989                 &          0.999                &        .997                 &        .945                 \\
$N$      &          47                 &          47                 &          47                 &          47                 &          47                 &          47                 \\


==> inputs/south_subperiod/Results5RICTint_ct_South_08t16.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel C: sub-period 2008-2016}}} \\\midrule
$R_{c,t}$ &       0.292$^{\ast}$        &       0.366$^{\ast}$        &       0.315$^{\ast\ast}$    &       0.303$^{\ast}$        &       0.340$^{\ast\ast}$    &       0.123                 &       0.121                 &       0.066$^{\ast}$        \\
            &     (0.110)                 &     (0.122)                 &     (0.084)                 &     (0.098)                 &     (0.059)                 &     (0.070)                 &     (0.063)                 &     (0.018)                 \\\addlinespace
$ICT_{c,t}$&      -0.029                 &      -0.058                 &      -0.040                 &      -0.051                 &      -0.113$^{\ast}$        &       0.076                 &      -0.028                 &      -0.017                 \\
            &     (0.035)                 &     (0.033)                 &     (0.020)                 &     (0.026)                 &     (0.029)                 &     (0.032)                 &     (0.024)                 &     (0.017)                 \\\addlinespace
$R*ICT_{c,t}$&       0.036                 &      -0.071                 &      -0.005                 &       0.012                 &      -0.022                 &       0.003                 &      -0.006                 &       0.002                 \\
            &     (0.037)                 &     (0.035)                 &     (0.023)                 &     (0.028)                 &     (0.016)                 &     (0.013)                 &     (0.017)                 &     (0.009)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &         .97                 &          0.999                &        .997                 \\
$N$      &          36                 &          36                 &          36                 &          36                 &          27                 &          27                 &          27                 &          27                 \\


==> inputs/south_subperiod/Results5RICTint_ct_South_95t07.tex <==
\multicolumn{9}{l}{\textbf{\emph{Panel B: sub-period 1995-2007}}} \\\midrule
$R_{c,t}$ &      -0.275$^{\ast\ast\ast}$&       0.129                 &      -0.122$^{\ast}$        &      -0.130$^{\ast}$        &      -0.242                 &       0.045                 &      -0.122                 &      -0.013                 \\
            &     (0.038)                 &     (0.141)                 &     (0.039)                 &     (0.051)                 &     (0.170)                 &     (0.087)                 &     (0.208)                 &     (0.079)                 \\\addlinespace
$ICT_{c,t}$&      -0.073                 &       0.297$^{\ast\ast}$    &       0.064                 &       0.078$^{\ast\ast}$    &       0.060$^{\ast}$        &       0.022                 &       0.033                 &      -0.048$^{\ast}$        \\
            &     (0.050)                 &     (0.063)                 &     (0.043)                 &     (0.024)                 &     (0.017)                 &     (0.013)                 &     (0.029)                 &     (0.014)                 \\\addlinespace
$R*ICT_{c,t}$&      -0.035$^{\ast}$        &      -0.075                 &      -0.050$^{\ast\ast}$    &      -0.047$^{\ast\ast}$    &       0.002                 &      -0.040                 &       0.042                 &      -0.009                 \\
            &     (0.013)                 &     (0.036)                 &     (0.014)                 &     (0.012)                 &     (0.064)                 &     (0.034)                 &     (0.081)                 &     (0.029)                 \\\midrule
$R^{2}$  &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &          0.999                &        .999                 \\
$N$      &          47                 &          47                 &          47                 &          47                 &          34                 &          34                 &          34                 &          34                 \\


==> robustness_endogenous_automation.tex <==
\FloatBarrier
\newpage
\section{Robustness: Coping with endogenous automation}
\label{SM:diffusion_endogeneity}
As explained in Sec. \ref{sec:empirical_approach_ai_data}, one major concern to the robustness of our results arises from potential endogeneity of AT diffusion. 
Ideally, we would like to measure the pure impact of technological progress in ATs as exogenous driver of AT diffusion to see how technological change affects the economy and public revenues. But we can only observe patterns of AT adoption which can endogenously dependent on economic dynamics. 

To cope with these concerns, we use three different types of robustness checks relying on lagged data and IVs. Here, we present the results of these robustness checks. 

In Sec. \ref{SM:robustness_lagged_controls}, we used robot- and ICT-intensity from $t-1$ instead of contemporaneous diffusion measures as explanatory variable. 
In Sec. \ref{SM:lagged_iv}, we used an IV approach. In particular, deeper lags from $t-1$, $t-2$ and $t-3$ are used as explanatory variables on the first stage to instrument contemporaneous AT diffusion. Below the tables with the results, we report statistics to test for under-, weak- and over-identification of the IV approach. The estimates of the coefficients of this approach are consistent with the results presented in the main text. 

Another IV approach is shown in Sec. \ref{SM:robustness_IV}. Here, we used robot and ICT products imports by all countries in the world except $c$ as in instrument for robot and ICT diffusion in country $c$.  This approach is inspired by \citet{blanas2019afraid} and follows the idea that AT imports to other countries should be driven by technological advances in ATs, but are entirely exogenous from the economic dynamics in country $c$. 
Again, we obtain qualitatively consistent point estimates for the coefficients, but the validity tests indicate a weak explanatory power at the first stage. 

Summing up, the lag-based and both IV approaches to cope with the endogeneity of AT diffusion measures support our analysis qualitatively, but the trade-based IV approach suffers from the weakness of instruments.\footnote{We have also experimented with alternative external IV approaches to construct Bartik-style instruments, but we ran into similar issues in terms of the validity of our instruments.} 

%The external IV for Robots (ICT) is constructed using information on imports of Robots (ICT goods) to produce the following country-level measures. For each country c in our dataset, I find all of its trade partners p based on the imports of Robots (ICT goods). Then, for each partner p I compute their exports of Robots (ICT goods) to all countries in the world other than c (or to all other non-sample countries). Then, for each country c I sum across all of its trade partners' p exports mentioned above using as weights base-year import values of country c from country p relative to country c's total imports of Robots (ICT goods). The idea with this instrument is to capture the surge in use of Robots (ICT goods) that can be seen as exogenous, i.e. not related to domestic demand, tax differences and other confounding factors. For more details on the instrument, see the discussion in the thread below. 
%Note that for Robots we have only one product code, and thus construct one external instrument (IVR). For ICT we have 48 products, and thus construct 48 external instruments (IVICT1toIVICT48). In the estimations I use the first lag of all of those and their interactions thereof, i.e. lag1 IVR with each of the lags from IVICT1toIVICT48. 

%Results 1) and 2) have both country-year and country-industry-year regressions, while results in 3) have only the country-year regressions. I did not produce results for the regional splits, but it is very easy to do so if needed. I have also uploaded the new code in Dropbox (I did not upload the BACI trade data used to construct the IV since they are over a 1GB, but let me know if you want me to).

\subsection{Using lagged ($t-1$) measures of ATs as controls}
\label{SM:robustness_lagged_controls}
\FloatBarrier
\subsubsection{Taxation and automation}

    \begin{table}[H]
    \caption{Taxation and automation}
    {\centering
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results2shortV1_RICTint_ct_All_95t16}
\midrule
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results2shortV1_RICTint_ct_All_95t07}
\midrule
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results2shortV1_RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}} \\ 
    \label{tab:regr_pre_tax_robots_lagged_controls} \scriptsize
      Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results of aggregate flows of tax revenues on different automation measures for 19 European countries during the period 2006-2016. All regressions use country level data and include: GDP growth, gross output share of the service sector in total economy; Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors; government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; effective tax rate; and country ($c$) and year ($t$) fixed effects. All regressions in Panel A also include the ln of gross-output value ($pQ$).
    \end{table}

\FloatBarrier
\newpage

\subsubsection{Taxation and economic production}

	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production for the period 2006-2016}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results2RICTint_ct_All_95t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2006-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); effective tax rate ($ETR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	\subsubsection{The replacement effect}

			\begin{table}[H]
    {\centering 
    \caption{The replacement effect}
    \label{tab:regr_replacement_lag}
    \begin{adjustbox}{width=0.6\textwidth}\begin{tabular}{l|ccc|ccc}
    \toprule \addlinespace
    
    \csname @@input\endcsname{inputs/robustness/lagged_controls/Results3RICTint_cit_All_95t16}
    \bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results3RICTint_cit_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results3RICTint_cit_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to test the replacement effect for 19 European countries during the period 1995-2016. All regressions use industry level data for the subset of industries susceptible to automation, defined as industries were the use of industrial robots is prevalent (see Appendix Table~\ref{appendix:data}). All regressions include: country industry ($ci$); country year ($ct$); and industry year ($it$) fixed effects. All regressions are weighted by the base-sample-year share of each industry’s number of hours worked to country-wide hours worked. Standard errors are clustered both at the country-industry and year level.
    \end{table}
    
 


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production for the period 1995-2007}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/lagged_controls/Results2RICTint_ct_All_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2006-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); effective tax rate ($ETR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production after 2008}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results2RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); effective tax rate ($ETR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

\FloatBarrier	
\newpage
\subsubsection{The reinstatement effect}

		\begin{table}[!h]
    {\centering 
    \caption{The reinstatement effect}
    \label{tab:regr_reinstatement_lagged_controls_Eurostat}
    \begin{adjustbox}{width=0.9\textwidth}\begin{tabular}{l|cccccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/lagged_controls/Results4shortRICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results4shortRICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results4shortRICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the reinstatement effect for 19 European countries during the period 2006-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); effective tax rate; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
\newpage
\subsubsection{The real-income effect}

	\begin{table}[!h]
    {\centering 
        \caption{The real income effect}
            \label{tab:regr_realincome_lagged_controls_Eurostat}

    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccccccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results5RICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results5RICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/lagged_controls/Results5RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ \noindent }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the real income effect for 19 European countries during the period 2006-2016. Labor productivity is measured as the share of gross-output volumes ($Q$) over the total number of hours worked. TFP is calculated as the residual from an OLS regression of gross-output volumes ($Q$) on a translog production function including capital volumes ($K$), total number of hours worked ($L$) and intermediate input volumes ($M$). All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; effective tax rate; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
\newpage


\subsection{Using deeper lags ($t-1$, $t-2$ , $t-3$) of AT measures as an IV}
\label{SM:lagged_iv}
\FloatBarrier
\subsubsection{Taxation and automation}

    \begin{table}[H]
    \caption{Taxation and automation}
    {\centering
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/IVlags/Results2shortV1_RICTint_ct_All_95t16}
\midrule
\csname @@input\endcsname{inputs/robustness/IVlags/Results2shortV1_RICTint_ct_All_95t07}
\midrule
\csname @@input\endcsname{inputs/robustness/IVlags/Results2shortV1_RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}} \\ 
    \label{tab:regr_pre_tax_robots_IVlags} \scriptsize
  Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results of aggregate flows of tax revenues on different automation measures for 19 European countries during the period 2003-2016. All regressions use country level data and include: GDP growth, gross output share of the service sector in total economy; Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors; government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; corporate tax rate; and country ($c$) and year ($t$) fixed effects. All regressions in Panel A also include the ln of gross-output value ($pQ$).
    \end{table}

\FloatBarrier
\newpage
\subsubsection{Taxation and economic production}

	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/IVlags/Results2RICTint_ct_All_95t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2003-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); corporate tax rate ($CTR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production for the period 2003-2007}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/IVlags/Results2RICTint_ct_All_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2003-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); corporate tax rate ($CTR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production after 2008}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/IVlags/Results2RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); corporate tax rate ($CTR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

\FloatBarrier	
\newpage
\subsubsection{The replacement effect}

			\begin{table}[H]
    {\centering 
    \caption{The replacement effect}
    \label{tab:regr_replacement_ivlag}
    \begin{adjustbox}{width=0.6\textwidth}\begin{tabular}{l|ccc|ccc}
    \toprule \addlinespace
    
    \csname @@input\endcsname{inputs/robustness/IVlags/Results3RICTint_cit_All_95t16}
    \bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IVlags/Results3RICTint_cit_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IVlags/Results3RICTint_cit_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to test the replacement effect for 19 European countries during the period 1995-2016. All regressions use industry level data for the subset of industries susceptible to automation, defined as industries were the use of industrial robots is prevalent (see Appendix Table~\ref{appendix:data}). All regressions include: country industry ($ci$); country year ($ct$); and industry year ($it$) fixed effects. All regressions are weighted by the base-sample-year share of each industry’s number of hours worked to country-wide hours worked. Standard errors are clustered both at the country-industry and year level.
    \end{table}
    
    
	

\subsubsection{The reinstatement effect}

		\begin{table}[!h]
    {\centering 
    \caption{The reinstatement effect}
    \label{tab:regr_reinstatement_IVlags}
    \begin{adjustbox}{width=0.9\textwidth}\begin{tabular}{l|cccccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/IVlags/Results4shortRICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IVlags/Results4shortRICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IVlags/Results4shortRICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the reinstatement effect for 19 European countries during the period 2003-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); corporate tax rate; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
\newpage
\subsubsection{The real-income effect}

	\begin{table}[!h]
    {\centering 
        \caption{The real income effect}
            \label{tab:regr_realincome_IVlags}

    \begin{adjustbox}{width=0.9\textwidth}\begin{tabular}{l|cccccccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/IVlags/Results5RICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IVlags/Results5RICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IVlags/Results5RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ \noindent }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the real income effect for 19 European countries during the period 2003-2016. Labor productivity is measured as the share of gross-output volumes ($Q$) over the total number of hours worked. TFP is calculated as the residual from an OLS regression of gross-output volumes ($Q$) on a translog production function including capital volumes ($K$), total number of hours worked ($L$) and intermediate input volumes ($M$). All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; corporate tax rate; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
%\newpage




\subsection{Using trade data on imports of robot and ICT products to construct external IVs for the AT measures}

%\clearpage
\label{SM:robustness_IV}
\FloatBarrier
\subsubsection{Taxation and automation}

    \begin{table}[H]
    \caption{Taxation and automation}
    {\centering
    \begin{adjustbox}{width=0.9\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/IV/Results2shortV1_RICTint_ct_All_95t16}
\midrule
\csname @@input\endcsname{inputs/robustness/IV/Results2shortV1_RICTint_ct_All_95t07}
\midrule
\csname @@input\endcsname{inputs/robustness/IV/Results2shortV1_RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    \label{tab:regr_pre_tax_robots_IV} \scriptsize
  Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results of aggregate flows of tax revenues on different automation measures for 19 European countries during the period 1995-2016. All regressions use country level data and include: GDP growth, gross output share of the service sector in total economy; Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors; government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; imports as \% of GDP; exports as \% of GDP; and country ($c$) and year ($t$) fixed effects. All regressions in Panel A also include the ln of gross-output value ($pQ$).
    \end{table}

\FloatBarrier
\newpage
\subsubsection{Taxation and economic production}

	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/IV/Results2RICTint_ct_All_95t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 1995-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); imports as \% of GDP ($Imports^{\%GDP}_{c,t}$); exports as \% of GDP ($Exports^{\%GDP}_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production before 2007}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/IV/Results2RICTint_ct_All_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 1995-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); imports as \% of GDP ($Imports^{\%GDP}_{c,t}$); exports as \% of GDP ($Exports^{\%GDP}_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production after 2008}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/IV/Results2RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); imports as \% of GDP ($Imports^{\%GDP}_{c,t}$); exports as \% of GDP ($Exports^{\%GDP}_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

\FloatBarrier	
\newpage
\subsubsection{The reinstatement effect}

		\begin{table}[!h]
    {\centering 
    \caption{The reinstatement effect}
    \label{tab:regr_reinstatement_IV}
    \begin{adjustbox}{width=\textwidth,totalheight=0.80\textheight,keepaspectratio}\begin{tabular}{l|cccccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/IV/Results4shortRICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IV/Results4shortRICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IV/Results4shortRICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the reinstatement effect for 19 European countries during the period 1995-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); imports as \% of GDP; exports as \% of GDP; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
\newpage
\subsubsection{The real-income effect}

	\begin{table}[!h]
    {\centering 
        \caption{The real income effect}
            \label{tab:regr_realincome_IV}

    \begin{adjustbox}{width=0.90\textwidth}\begin{tabular}{l|cccccccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/IV/Results5RICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IV/Results5RICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IV/Results5RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ \noindent }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the real income effect for 19 European countries during the period 1995-2016. Labor productivity is measured as the share of gross-output volumes ($Q$) over the total number of hours worked. TFP is calculated as the residual from an OLS regression of gross-output volumes ($Q$) on a translog production function including capital volumes ($K$), total number of hours worked ($L$) and intermediate input volumes ($M$). All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; imports as \% of GDP; exports as \% of GDP; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
\newpage

==> robustness_tax_trade_distribution.tex <==
\FloatBarrier
\newpage
\section{Robustness checks: Taxes, trade and income distribution}
\label{SM:robustness_taxes}

In this section, we provide the results of a series of robustness checks. 

First, we make sure that our results are not driven by changes in the tax system. Unfortunately, comprehensive data that covers the whole range of different taxes, that is consistent across our sample of countries and covers a reasonable number of years is not available. 
We are only able to proxy tax reforms using data on corporate taxation that cover a smaller period of time but all countries in our sample. We use two different data sources. 

In \ref{SM:robustness_KPMG}, we repeat all baseline country level regressions and include as an additional control the corporate tax rate ($CRT_{c,t}$) sourced from KPMG.\footnote{The data were sourced from the KPMG website: \url{https://home.kpmg/xx/en/home/services/tax/tax-tools-and-resources/tax-rates-online.html}} 
This data are only available between 2003-2016 and only the results for the period after 2008 are comparable with the baseline analysis.

Next, in \ref{SM:robustness_ETR_Eurostat} we repeat all baseline country level regressions and include as an additional control the effective tax rate ($ERT_{c,t}$) sourced from Eurostat.\footnote{This is the Effective Average Tax Rate (ETR) for large corporations in non-financial sector, computed at corporate level, for average asset composition and funding sources, using the Devereux/Griffith 
 methodology. The data are available in Eurostat: \url{https://ec.europa.eu/taxation_customs/business/economic-analysis-taxation/data-taxation_en}} 
The ETR variable is only available between 2006-2016 and again, only the results for the period after 2008 are comparable with the baseline analysis.
 
Another concern regarding the robustness of our results may arise from the impact of trade. In our baseline, we only controlled for the exchange rate which does not or only poorly vary across different European countries. To capture the country specific impact of trade, we repeat all baseline country level regressions and include as additional controls the countrylevel imports ($Imports^{\% GDP}_{c,t}$) and exports ($Exports^{\% GDP}_{c,t}$) as percentage of GDP sourced from the OECD National Accounts Database.\footnote{The data are available in OECD: \url{https://stats.oecd.org/viewhtml.aspx?datasetcode=NAAG\&lang=en\#}} 
The results are shown in Table \ref{SM:robustness_trade}. 
%Note that, similar to the baseline analysis, the additional variables are available for all years, i.e. 1995-2016.

\begin{comment}
To support the interpretation of our results, we examine the relationship between automation and income distribution and between income distribution and taxation. 

In \ref{SM:robustness_distribution} illustrate the distributional effect of AT diffusion. We rely on the same empirical specification used to estimate the reinstatement effects, but now our regressions are based on the following four left hand side variables: two Gini coefficients from the industry level distribution of hourly wage ($Gini^{w}_{c,t}$) and labor in terms of hours worked ($Gini^{L}_{c,t}$), respectively; and two dispersion measures computed as the 90/10 percentile ratio from the industry level distribution of hourly wage ($Dispersion^{w}_{c,t}$) and labor in terms of hours worked ($Dispersion^{L}_{c,t}$), respectively. To construct the measures we use the EUKLEMS dataset.
\end{comment}
Further, to explore the nexus between distribution and taxation, we examine the progressiveness of taxation (Table \ref{SM:robustness_progressive}). To do so, we rely on the same empirical specification used to understand the determinants of taxation, but now our regressions include as an additional control the Gini coefficient from the industry level distribution of labor in terms of hours worked ($Gini^{L}_{c,t}$) sourced from Eurostat.

Finally, we also test whether the attribution of capital taxes within the broad categories from OECD might affect our results. In particular we test whether the exclusion of the OECD tax category 1100 ``taxes on income, profits and capital gains of individuals'' from the taxes on capital $T^k$ changes the interpretation of our findings (assuming that these are neither capital nor labor taxes in the strict sense of their origin). The results are presented in \ref{SM:robustness_Tk} where we find similar results as in our baseline but the share of taxes as a percent of total taxes and GDP drops significantly due to this omission.


\subsection{Controlling for changes in corporate taxation using KPMG data}
\label{SM:robustness_KPMG}
\FloatBarrier
\subsubsection{Taxation and automation}

    \begin{table}[H]
    \caption{Taxation and automation}
    {
    \begin{adjustbox}{width=0.85\textwidth}
    \centering
    \begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results2shortV1_RICTint_ct_All_95t16}
\midrule
\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results2shortV1_RICTint_ct_All_95t07}
\midrule
\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results2shortV1_RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}} \\ 
    \label{tab:regr_pre_tax_robots_KPMG} \scriptsize
  Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results of aggregate flows of tax revenues on different automation measures for 19 European countries during the period 2003-2016. All regressions use country level data and include: GDP growth, gross output share of the service sector in total economy; Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors; government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; corporate tax rate; and country ($c$) and year ($t$) fixed effects. All regressions in Panel A also include the ln of gross-output value ($pQ$).
    \end{table}

\FloatBarrier
\newpage
\subsubsection{Taxation and economic production}

	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production for the period 2003-2016}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results2RICTint_ct_All_95t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2003-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); corporate tax rate ($CTR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production for the period 2003-2007}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results2RICTint_ct_All_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2003-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); corporate tax rate ($CTR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production after 2008}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results2RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); corporate tax rate ($CTR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

\FloatBarrier	
\newpage

\subsubsection{The reinstatement effect}

		\begin{table}[!h]
    {\centering 
    \caption{The reinstatement effect}
    \label{tab:regr_reinstatement_KPMG}
    \begin{adjustbox}{width=0.9\textwidth}\begin{tabular}{l|cccccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results4shortRICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results4shortRICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results4shortRICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the reinstatement effect for 19 European countries during the period 2003-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); corporate tax rate; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
\newpage
\subsubsection{The real-income effect}

	\begin{table}[!h]
    {\centering 
        \caption{The real income effect}
            \label{tab:regr_realincome_KPMG}

    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccccccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results5RICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results5RICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/CTR_KPMG/Results5RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ \noindent }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the real income effect for 19 European countries during the period 2003-2016. Labor productivity is measured as the share of gross-output volumes ($Q$) over the total number of hours worked. TFP is calculated as the residual from an OLS regression of gross-output volumes ($Q$) on a translog production function including capital volumes ($K$), total number of hours worked ($L$) and intermediate input volumes ($M$). All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; corporate tax rate; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
%\newpage



\subsection{Controlling for changes in corporate taxation using Eurostat data}
\label{SM:robustness_ETR_Eurostat}
\FloatBarrier
\subsubsection{Taxation and automation}

    \begin{table}[H]
    \caption{Taxation and automation}
    { \centering
    \begin{adjustbox}{width=0.9\textwidth}
    \centering
    \begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results2shortV1_RICTint_ct_All_95t16}
\midrule
\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results2shortV1_RICTint_ct_All_95t07}
\midrule
\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results2shortV1_RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    \label{tab:regr_pre_tax_robots_ETR} \scriptsize
      Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results of aggregate flows of tax revenues on different automation measures for 19 European countries during the period 2006-2016. All regressions use country level data and include: GDP growth, gross output share of the service sector in total economy; Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors; government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; effective tax rate; and country ($c$) and year ($t$) fixed effects. All regressions in Panel A also include the ln of gross-output value ($pQ$).
    \end{table}

\FloatBarrier
%\newpage

\subsubsection{Taxation and economic production}

	\begin{table}[!ht]
	{\centering 
    \caption{Taxation and the structure of economic production for the period 2006-2016}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results2RICTint_ct_All_95t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2006-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); effective tax rate ($ETR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production  for the period 2006-2007}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results2RICTint_ct_All_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2006-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); effective tax rate ($ETR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production after 2008}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results2RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); effective tax rate ($ETR_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

\FloatBarrier	
\newpage
\subsubsection{The reinstatement effect}

		\begin{table}[!h]
    {\centering 
    \caption{The reinstatement effect}
    \label{tab:regr_reinstatement_ETR_Eurostat}
    \begin{adjustbox}{width=0.8\textwidth}\begin{tabular}{l|cccccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results4shortRICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results4shortRICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results4shortRICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the reinstatement effect for 19 European countries during the period 2006-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); effective tax rate; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
\newpage
\subsubsection{The real-income effect}

	\begin{table}[!h]
    {\centering 
        \caption{The real income effect}
            \label{tab:regr_realincome_ETR_Eurostat}

    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccccccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results5RICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results5RICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/ETR_Eurostat/Results5RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ \noindent }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the real income effect for 19 European countries during the period 2006-2016. Labor productivity is measured as the share of gross-output volumes ($Q$) over the total number of hours worked. TFP is calculated as the residual from an OLS regression of gross-output volumes ($Q$) on a translog production function including capital volumes ($K$), total number of hours worked ($L$) and intermediate input volumes ($M$). All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; effective tax rate; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
%\newpage




\subsection{Controlling for trade}
\label{SM:robustness_trade}
\FloatBarrier
\subsubsection{Taxation and automation}

    \begin{table}[H]
    \caption{Taxation and automation}
    { \centering
    \begin{adjustbox}{width=0.85\textwidth}
    \centering
    \begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results2shortV1_RICTint_ct_All_95t16}
\midrule
\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results2shortV1_RICTint_ct_All_95t07}
\midrule
\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results2shortV1_RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    \label{tab:regr_pre_tax_robots_Trade} \scriptsize
  Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results of aggregate flows of tax revenues on different automation measures for 19 European countries during the period 1995-2016. All regressions use country level data and include: GDP growth, gross output share of the service sector in total economy; Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors; government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; imports as \% of GDP; exports as \% of GDP; and country ($c$) and year ($t$) fixed effects. All regressions in Panel A also include the ln of gross-output value ($pQ$).
    \end{table}

\FloatBarrier
\newpage
\subsubsection{Taxation and economic production}

	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results2RICTint_ct_All_95t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 1995-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); imports as \% of GDP ($Imports^{\%GDP}_{c,t}$); exports as \% of GDP ($Exports^{\%GDP}_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production before 2007}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results2RICTint_ct_All_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 1995-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); imports as \% of GDP ($Imports^{\%GDP}_{c,t}$); exports as \% of GDP ($Exports^{\%GDP}_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production after 2008}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results2RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); imports as \% of GDP ($Imports^{\%GDP}_{c,t}$); exports as \% of GDP ($Exports^{\%GDP}_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

\FloatBarrier	
\newpage
\subsubsection{The reinstatement effect}

		\begin{table}[!h]
    {\centering 
    \caption{The reinstatement effect}
    \label{tab:regr_reinstatement_trade}
    \begin{adjustbox}{width=0.8\textwidth}\begin{tabular}{l|cccccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results4shortRICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results4shortRICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results4shortRICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the reinstatement effect for 19 European countries during the period 1995-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); imports as \% of GDP; exports as \% of GDP; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
\newpage
\subsubsection{The real-income effect}

	\begin{table}[!h]
    {\centering 
        \caption{The real income effect}
            \label{tab:regr_realincome_trade}

    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccccccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results5RICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results5RICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/Trade_OECD/Results5RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ \noindent }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the real income effect for 19 European countries during the period 1995-2016. Labor productivity is measured as the share of gross-output volumes ($Q$) over the total number of hours worked. TFP is calculated as the residual from an OLS regression of gross-output volumes ($Q$) on a translog production function including capital volumes ($K$), total number of hours worked ($L$) and intermediate input volumes ($M$). All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; imports as \% of GDP; exports as \% of GDP; and country ($c$) and year ($t$) fixed effects.
    \end{table}

\FloatBarrier
\newpage
\begin{comment}
\subsection{Distributional effects of automation}
\label{SM:robustness_distribution}
\subsubsection{Whole Europe}
		\begin{table}[H]
    {\centering 
    \caption{The distributional impact}
    \label{tab:regr_reinstatement_distribution}
    %\begin{adjustbox}{width=0.9\textwidth}
    \begin{tabular}{l|ccccccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_All_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_All_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_All_08t16}
\bottomrule
    \end{tabular}
    %\end{adjustbox}
    \\}
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the reinstatement effect for 19 European countries during the period 1995-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); and country ($c$) and year ($t$) fixed effects. $Gini^{L}_{c,t}$ and $Gini^{w}_{c,t}$ are Gini indices from the industry level distribution of labor in terms of hours worked and hourly wage, respectively. $Dispersion^{L}_{c,t}$ and $Dispersion^{w}_{c,t}$ are dispersion measures computed as the 90/10 percentile ratio from the industry level distribution of labor in terms of hours worked and hourly wage, respectively.
    \end{table}



\FloatBarrier
\newpage

\subsubsection{Eastern Europe}
		\begin{table}[H]
    {\centering 
    \caption{The distributional impact}
    \label{tab:regr_reinstatement_distribution_east}
    %\begin{adjustbox}{width=0.9\textwidth}
    \begin{tabular}{l|ccccccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_East_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_East_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_East_08t16}
\bottomrule
    \end{tabular}%\end{adjustbox}
    \\ }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the reinstatement effect for Eastern European countries and the period from 1995-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); and country ($c$) and year ($t$) fixed effects. $Gini^{L}_{c,t}$ and $Gini^{w}_{c,t}$ are Gini indices from the industry level distribution of labor in terms of hours worked and hourly wage, respectively. $Dispersion^{L}_{c,t}$ and $Dispersion^{w}_{c,t}$ are dispersion measures computed as the 90/10 percentile ratio from the industry level distribution of labor in terms of hours worked and hourly wage, respectively.
    \end{table}



\FloatBarrier
\newpage

\subsubsection{Northern Europe}
		\begin{table}[H]
    {\centering 
    \caption{The distributional impact}
    \label{tab:regr_reinstatement_distribution_north}
    %\begin{adjustbox}{width=0.9\textwidth}
    \begin{tabular}{l|ccccccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_North_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_North_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_North_08t16}
\bottomrule
    \end{tabular}
    %\end{adjustbox}
    \\ }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the reinstatement effect for Northern European countries and the period from 1995-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); and country ($c$) and year ($t$) fixed effects. $Gini^{L}_{c,t}$ and $Gini^{w}_{c,t}$ are Gini indices from the industry level distribution of labor in terms of hours worked and hourly wage, respectively. $Dispersion^{L}_{c,t}$ and $Dispersion^{w}_{c,t}$ are dispersion measures computed as the 90/10 percentile ratio from the industry level distribution of labor in terms of hours worked and hourly wage, respectively.
    \end{table}



\FloatBarrier
\newpage

\subsubsection{Southern Europe}
		\begin{table}[H]
    {\centering 
    \caption{The distributional impact}
    \label{tab:regr_reinstatement_distribution_south}
    %\begin{adjustbox}{width=0.9\textwidth}
    \begin{tabular}{l|ccccccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_South_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_South_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/robustness/IncomeDist/Results4shortRICTint_ct_South_08t16}
\bottomrule
    \end{tabular}
    %\end{adjustbox}
    \\ }
    \scriptsize
    Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to test the reinstatement effect for Southern European countries and the period from 1995-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); and country ($c$) and year ($t$) fixed effects. $Gini^{L}_{c,t}$ and $Gini^{w}_{c,t}$ are Gini indices from the industry level distribution of labor in terms of hours worked and hourly wage, respectively. $Dispersion^{L}_{c,t}$ and $Dispersion^{w}_{c,t}$ are dispersion measures computed as the 90/10 percentile ratio from the industry level distribution of labor in terms of hours worked and hourly wage, respectively.
    \end{table}



\FloatBarrier
\newpage



\end{comment}
\subsection{The progressiveness of taxation}
\label{SM:robustness_progressive}

%\subsubsection{Whole Europe}
	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production}
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/TaxProgressiveness/Results2RICTint_ct_All_95t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 1995-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); Gini index from the industry level distribution of hourly wage ($Gini^{w}_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}
 
	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production before 2007}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/TaxProgressiveness/Results2RICTint_ct_All_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 1995-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); Gini index from the industry level distribution of hourly wage ($Gini^{w}_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

	


	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production after 2008}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/TaxProgressiveness/Results2RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); Gini index from the industry level distribution of hourly wage ($Gini^{w}_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

\FloatBarrier
\newpage



\subsection{Excluding OECD group 1100 ``taxes on income, profits and capital gains of individuals'' from capital taxes}
\label{SM:robustness_Tk}
\FloatBarrier
\subsubsection{Taxation and automation}

    \begin{table}[H]
    \caption{Taxation and automation}
    { \centering
    \begin{adjustbox}{width=0.85\textwidth}
    \centering
    \begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/Tk_alt/Results2shortV1_RICTint_ct_All_95t16}
\midrule
\csname @@input\endcsname{inputs/robustness/Tk_alt/Results2shortV1_RICTint_ct_All_95t07}
\midrule
\csname @@input\endcsname{inputs/robustness/Tk_alt/Results2shortV1_RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    \label{tab:regr_pre_tax_robots_Trade} \scriptsize
  Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results of aggregate flows of tax revenues on different automation measures for 19 European countries during the period 1995-2016. All regressions use country level data and include: GDP growth, gross output share of the service sector in total economy; Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors; government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; and country ($c$) and year ($t$) fixed effects. All regressions in Panel A also include the ln of gross-output value ($pQ$). Taxes on capital $T^k$ exclude the OECD tax category 1100 ``taxes on income, profits and capital gains of individuals''.
    \end{table}
    
    
	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production before 2007}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace

\csname @@input\endcsname{inputs/robustness/Tk_alt/Results2RICTint_ct_All_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 1995-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$);  and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP. Taxes on capital $T^k$ exclude the OECD tax category 1100 ``taxes on income, profits and capital gains of individuals''.
    \end{table}

	

	\begin{table}[!ht]
	{\centering 
     
    \caption{Taxation and the structure of economic production after 2008}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    
    \toprule \addlinespace
\csname @@input\endcsname{inputs/robustness/Tk_alt/Results2RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }

        \scriptsize
   Notes: $\ast$ \(p<0.05\), $\ast\ast$ \(p<0.01\), $\ast\ast\ast$ \(p<0.001\). Regression results to establish the link between tax aggregation and economic production for 19 European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$), share of gross output produced in service industries ($Services_{c,t}$); the Herfindahl-Hirschman Index computed based on the gross-output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP. Taxes on capital $T^k$ exclude the OECD tax category 1100 ``taxes on income, profits and capital gains of individuals''.
    \end{table}

    
\FloatBarrier
\newpage

==> suppl_material.tex <==
\appendix
\renewcommand{\appendixname}{Supplementary Material}
\renewcommand{\thesection}{SI.\arabic{section}} \setcounter{section}{0}
\renewcommand{\thefigure}{SI.\arabic{section}\arabic{figure}} \setcounter{figure}{0}
\renewcommand{\thetable}{SI.\arabic{section}\arabic{table}} \setcounter{table}{0}
\renewcommand{\theequation}{SI.\arabic{equation}} \setcounter{equation}{0}
%\part*{SUPPLEMENTARY MATERIAL --- ONLINE APPENDIX}
\section{Additional regression results}
\subsection{Prerequisites}
\subsubsection{Further determinants of taxation}
\label{appendix:add_results_determinants_taxation}
    Here, we briefly outline other determinants of taxation that are included in the regressions but not discussed in the main text. These regressors are motivated by the literature and taxation and cover GDP growth, the market share of services $Services_{c,t}$, public finance related indicators (debt, interest payments and deficit), measures for industrial concentration $HHI_{c,t}$, the exchange rate $XRate_{c,t}$ (i.e. US\$ per Euro) as proxy for trade and public investments $GovInvest^{\%GDP}_{c,t}$. 
    
	Labor taxes in absolute terms, in relation to GDP and as share in total taxation exhibit a positive correlation with the service share. 
	This pattern holds for the majority of sub-periods and regions. In other sub-samples, we additionally find a negative association of the services share with taxes on capital and goods. Northern Europe is an exception where we observe a weakly significant opposite relationship. 	

    High indebtedness and higher deficits are positively related to taxes in absolute terms and measured in percentage GDP. 
    %This relationship is reversed in some regions after the financial crisis 2008. 
    Net lending as percentage GDP is positively correlated with all taxes except from labor taxes which are negatively related to deficits. 
    
	We find a higher exchange rate $XRate_{c,t}$ to be negatively related to taxes on capital, goods and in total measured in absolute terms and as percentage of GDP. We also observe a higher exchange rate to be positively related to the relative tax contribution of labor at the cost of taxes on capital. This relationship is opposite in Southern European countries.\footnote{Note that the exchange rate varies across European countries only in the time dimension since the EU's Exchange Rate Mechanism aims to keep exchange rate fluctuations between the Euro and other European currencies flat (see also \url{https://stats.oecd.org/glossary/detail.asp?ID=3055}). Hence, $XRate_{c,t}$ captures the competitiveness of European countries on global markets but can not be interpreted as an indicator for within-European trade.}

	\begin{table}[H]
	{\centering 
     
    \caption{Taxation and the structure of production}
    
    \label{tab:regr_pre_tax_prod6}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/all_95_16/Results2RICTint_ct_All_95t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ } \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production for 19 European countries during the period 1995-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block (Taxes in ln of national currency), $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP. Standard errors are clustered both at the country and year level.
    \end{table}
\newpage

	\begin{table}[!hb]
	{\centering 
     
    \caption{Taxation and the structure of production before 2007 in whole Europe}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/all_subperiod/Results2RICTint_ct_All_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
        \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production  for 19 European countries during the period 1995-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}
\newpage
	\begin{table}[H]
	{\centering 
     
    \caption{Taxation and the structure of production after 2008 in whole Europe}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}

    \toprule \addlinespace
\csname @@input\endcsname{inputs/all_subperiod/Results2RICTint_ct_All_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    %%\label{tab:regr_pre_tax_prod6}
        \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production for 19 European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block, $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}

\FloatBarrier
\subsubsection{Taxation and automation by region and period}
\label{appendix:add_results_taxes_and_ai}
    \begin{table}[H]
    \caption{Taxation and automation in Eastern Europe}
    {\centering
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/east_95_16/Results2shortV1_RICTint_ct_East_95t16}
\midrule
\csname @@input\endcsname{inputs/east_subperiod/Results2shortV1_RICTint_ct_East_95t07}
\midrule
\csname @@input\endcsname{inputs/east_subperiod/Results2shortV1_RICTint_ct_East_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}} \\ 
    \label{tab:regr_pre_tax_robots_east} \scriptsize
  Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results of aggregate flows of tax revenues on different automation measures for Eastern European countries during the period 1995-2016. All regressions use country level data and include: GDP growth, gross output share of service industries; Herfindahl-Hirschman Index based on the gross output shares of macro-sectors; government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; and country ($c$) and year ($t$) fixed effects. All regressions for Taxes in ln of national currency also include the ln of gross output value ($pQ$). Standard errors are clustered both at the country and year level.
    \end{table}
    
    \begin{table}[H]
    \caption{Taxation and automation in Northern Europe}
    {\centering
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/north_95_16/Results2shortV1_RICTint_ct_North_95t16}
\midrule
\csname @@input\endcsname{inputs/north_subperiod/Results2shortV1_RICTint_ct_North_95t07}
\midrule
\csname @@input\endcsname{inputs/north_subperiod/Results2shortV1_RICTint_ct_North_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}} \\ 
    \label{tab:regr_pre_tax_robots_north} \scriptsize
  Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results of aggregate flows of tax revenues on different automation measures for Northern European countries during the period 1995-2016. All regressions use country level data and include: GDP growth, gross output share of service industries; Herfindahl-Hirschman Index based on the gross output shares of macro-sectors; government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; and country ($c$) and year ($t$) fixed effects. All regressions for Taxes in ln of national currency also include the ln of gross output value ($pQ$). Standard errors are clustered both at the country and year level.
    \end{table}
    
    \begin{table}[H]
    \caption{Taxation and automation in Southern Europe}
    {\centering
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/south_95_16/Results2shortV1_RICTint_ct_South_95t16}
\midrule
\csname @@input\endcsname{inputs/south_subperiod/Results2shortV1_RICTint_ct_South_95t07}
\midrule
\csname @@input\endcsname{inputs/south_subperiod/Results2shortV1_RICTint_ct_South_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}} \\ 
    \label{tab:regr_pre_tax_robots_south} \scriptsize
  Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results of aggregate flows of tax revenues on different automation measures for Southern European countries during the period 1995-2016. All regressions use country level data and include: GDP growth, gross output share of service industries; Herfindahl-Hirschman Index based on the gross output shares of macro-sectors; government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; and country ($c$) and year ($t$) fixed effects. All regressions for Taxes in ln of national currency also include the ln of gross output value ($pQ$). Standard errors are clustered both at the country and year level.
    \end{table}


\newpage
\subsubsection{Taxation, automation and the economy in different regions}
\label{appendix:add_results_taxes_and_the_economy}
To control for regional differences, we split the sample into Eastern, Northern and Southern Europe which differ by tax systems, their industrial structure and the extent to which countries were hit by the financial crisis.\footnote{Descriptive statistics and time series plots illustrating the regional peculiarities can be found in Appendix \ref{appendix:descr_stats} and \ref{appendix:key_vars_by_region}.} 

In Eastern Europe, we find that robot diffusion is negatively associated with taxes on labor and goods, but we do not observe any effects of ICT. The depth of automation is positively correlated with taxes on capital and goods and a shift from taxation of labor to capital. Until 2007, the effect of $R \ast ICT_{c,t}$ on capital taxation is opposite, i.e. negative. 

In Northern Europe, we observe a negative correlation between robot diffusion and the depth of automation and labor taxes. Until 2007, robot diffusion and automation depth exhibit a negative impact on total tax revenues and capital taxation and after 2008 on taxes on goods. 
Conversely, ICT diffusion is positively related to labor taxation at the expense of taxes on capital. 

In Southern Europe, we find robots to be negatively correlated with total tax revenues and taxes on goods measured as percentage GDP. Prior to 2007, we see a negative relationship between robots and labor taxation and after 2008 with capital taxation. 
ICTs exhibit a negative association with labor taxation and we observe an increasing share of goods taxation. 

While results for Eastern and Northern Europe align with the observations made for the full sample, the findings for Southern Europe are slightly different. We find ICT to coincide with capital accumulation and to be associated with more employment, while the effect of robots on employment and wages is negative before 2007 but positive afterwards.     
    
\FloatBarrier

	\begin{table}[H]
	{\centering 
    \caption{Taxation and the structure of production in Eastern Europe}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/east_95_16/Results2RICTint_ct_East_95t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    %\label{tab:regr_pre_tax_prod6}
        \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production for Eastern European countries during the period 1995-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block (Taxes in ln of national currency), $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}
%    \end{landscape}
	

	\begin{table}[H]
	{\centering 
     
    \caption{Taxation and the structure of production in Eastern Europe before 2007}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    %\begin{adjustbox}{width=\textwidth}\begin{tabular}{p{0.6cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/east_subperiod/Results2RICTint_ct_East_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    %\label{tab:regr_pre_tax_prod6}
        \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production for Eastern European countries during the period 1995-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block (Taxes in ln of national currency), $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}
%    \end{landscape}
	


	\begin{table}[H]
	{\centering 
     
    \caption{Taxation and the structure of production in Eastern Europe after 2008}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    %\begin{adjustbox}{width=\textwidth}\begin{tabular}{p{0.6cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/east_subperiod/Results2RICTint_ct_East_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    %%\label{tab:regr_pre_tax_prod6}
        \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production for Eastern European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block (Taxes in ln of national currency), $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}
%    \end{landscape}
	


\FloatBarrier

	\begin{table}[H]
	{\centering 
     
    \caption{Taxation and the structure of production in Northern Europe}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/north_95_16/Results2RICTint_ct_North_95t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    %\label{tab:regr_pre_tax_prod6}
        \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production for Northern European countries during the period 1995-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block (Taxes in ln of national currency), $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}
%    \end{landscape}
	

	\begin{table}[H]
	{\centering 
     
    \caption{Taxation and the structure of production in Northern Europe before 2007}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    %\begin{adjustbox}{width=\textwidth}\begin{tabular}{p{0.6cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}}
    \toprule \addlinespace
%\csname @@input\endcsname{inputs/north_subperiod/Results2_ct_North_95t07}
%\csname @@input\endcsname{inputs/north_subperiod/Results2ROB_ct_North_95t07}
%\csname @@input\endcsname{inputs/north_subperiod/Results2ICT_ct_North_95t07}
%\csname @@input\endcsname{inputs/north_subperiod/Results2RICT_ct_North_95t07}
\csname @@input\endcsname{inputs/north_subperiod/Results2RICTint_ct_North_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    %\label{tab:regr_pre_tax_prod6}
        \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production for Northern European countries during the period 1995-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block (Taxes in ln of national currency), $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}
%    \end{landscape}
	


	\begin{table}[H]
	{\centering 
     
    \caption{Taxation and the structure of production in Northern Europe after 2008}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/north_subperiod/Results2RICTint_ct_North_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    %\label{tab:regr_pre_tax_prod6}
        \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production for Northern European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block (Taxes in ln of national currency), $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP..
    \end{table}
%    \end{landscape}
	

\FloatBarrier

	\begin{table}[H]
	{\centering 
     
    \caption{Taxation and the structure of production in Southern Europe}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/south_95_16/Results2RICTint_ct_South_95t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    %\label{tab:regr_pre_tax_prod6}
        \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production for Southern European countries during the period 1995-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block (Taxes in ln of national currency), $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}
%    \end{landscape}
	

	\begin{table}[H]
	{\centering 
     
    \caption{Taxation and the structure of production in Southern Europe before 2007}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/south_subperiod/Results2RICTint_ct_South_95t07}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    %\label{tab:regr_pre_tax_prod6}
        \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production for Southern European countries during the period 1995-2007. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block (Taxes in ln of national currency), $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}
%    \end{landscape}
	


	\begin{table}[H]
	{\centering 
     
    \caption{Taxation and the structure of production in Southern Europe after 2008}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccc|cccc|ccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/south_subperiod/Results2RICTint_ct_South_08t16}
\bottomrule
    \end{tabular}\end{adjustbox} \\ }
    %\label{tab:regr_pre_tax_prod6}
        \scriptsize
   Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to examine the link between tax aggregation and economic production for Southern European countries during the period 2008-2016. All regressions use country level data and include: GDP growth ($GDPgrowth_{c,t}$); share of gross output produced in service industries ($Services_{c,t}$); Herfindahl-Hirschman Index based on the gross output shares of macro-sectors ($HHI_{c,t}$); government consolidated gross debt as \% of GDP ($Debt^{\%GDP}_{c,t}$); government interest payable as \% of GDP ($Interest^{\%GDP}_{c,t}$); net government lending/borrowing as \% of GDP ($Lending^{\%GDP}_{c,t}$); gross fixed capital formation as \% of GDP ($GovInv^{\%GDP}_{c,t}$); period average exchange rate ($XRate_{c,t}$); and country ($c$) and year ($t$) fixed effects. For the first block (Taxes in ln of national currency), $wL_{c,t}$, $rK_{c,t}$ and $pQ_{c,t}$ are expressed as the natural logarithm ($ln$) while for the last two blocks they are expressed as \% of GDP.
    \end{table}
%    \end{landscape}
	

\FloatBarrier

\subsection{The economic impact of automation by region}
\label{appendix:add_results_ai_and_the_economy}
\subsubsection{The replacement effect}
\label{appendix:replacement_country}
	
	\textcolor{red}{check these}
	
	In Eastern Europe, we find robots and the depth of automation to coincide with labor replacement reflected in lower employment. The effects on capital prices are ambiguous: ICT ($R \ast ICT_{i,c,t}$) exhibits negative (positive) correlations with $r_{i,c,t}$. These relationships are more prevalent before 2007. 
	
	In Northern Europe and after 2008, we observe a replacement effect reflected in a decreasing wage bill and labor demand induced by robots. During that period, we also observe that ICT diffusion is associated with lower labor demand. Prior to 2007, we observe almost no significant effects. We only find a positive correlation of robot diffusion and capital accumulation. 
	
	In Southern Europe, we do not observe any AT-induced replacement effect. ICT is positively correlated with the wage bill throughout all periods. While we do not find any effect of robots on labor demand, we see that robot diffusion is associated with increasing wages. 
	ICT and the depth of automation are both associated with increasing capital prices but decreasing capital stocks. 

			\begin{table}[H]
    {\centering 
    \caption{The replacement effect in Eastern Europe}
    %\label{tab:regr_replacement_east}
    \begin{adjustbox}{width=0.8\textwidth}\begin{tabular}{l|ccc|ccc}
    %\begin{adjustbox}{width=\textwidth}\begin{tabular}{p{0.6cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}}
    \toprule \addlinespace
    
    \csname @@input\endcsname{inputs/east_95_16/Results3RICTint_cit_East_95t16}

    \bottomrule \addlinespace
%\multicolumn{13}{l}{\emph{\underline{Sub-period from 1995 to 2007}}}\\ %\addlinespace
\csname @@input\endcsname{inputs/east_subperiod/Results3RICTint_cit_East_95t07}

\bottomrule \addlinespace
%\multicolumn{13}{l}{\emph{\underline{Sub-period from 1995 to 2007}}}\\ %\addlinespace
\csname @@input\endcsname{inputs/east_subperiod/Results3RICTint_cit_East_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to test the replacement effect for Eastern European countries during the period 1995-2016. All regressions use industry level data for the subset of industries susceptible to automation, defined as industries were the use of industrial robots is prevalent (see Appendix Table~\ref{appendix:data}). All regressions include: country industry ($ci$); country year ($ct$); and industry year ($it$) fixed effects. All regressions are weighted by the base-sample-year share of each industry’s number of hours worked to country-wide hours worked.
    \end{table}
\FloatBarrier
			\begin{table}[H]
    {\centering 
    \caption{The replacement effect in Northern Europe}
    %\label{tab:regr_replacement_north}
    \begin{adjustbox}{width=0.8\textwidth}\begin{tabular}{l|ccc|ccc}
    %\begin{adjustbox}{width=\textwidth}\begin{tabular}{p{0.6cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}}
    \toprule \addlinespace
    
    \csname @@input\endcsname{inputs/north_95_16/Results3RICTint_cit_North_95t16}

    \bottomrule \addlinespace
%\multicolumn{13}{l}{\emph{\underline{Sub-period from 1995 to 2007}}}\\ %\addlinespace
\csname @@input\endcsname{inputs/north_subperiod/Results3RICTint_cit_North_95t07}

\bottomrule \addlinespace
%\multicolumn{13}{l}{\emph{\underline{Sub-period from 1995 to 2007}}}\\ %\addlinespace
\csname @@input\endcsname{inputs/north_subperiod/Results3RICTint_cit_North_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to test the replacement effect for Northern European countries during the period 1995-2016. All regressions use industry level data for the subset of industries susceptible to automation, defined as industries were the use of industrial robots is prevalent (see Appendix Table~\ref{appendix:data}). All regressions include: country industry ($ci$); country year ($ct$); and industry year ($it$) fixed effects. All regressions are weighted by the base-sample-year share of each industry’s number of hours worked to country-wide hours worked.
    \end{table}
\FloatBarrier
			\begin{table}[H]
    {\centering 
    \caption{The replacement effect in Southern Europe}
    %\label{tab:regr_replacement_south}
    \begin{adjustbox}{width=0.8\textwidth}\begin{tabular}{l|ccc|ccc}
    %\begin{adjustbox}{width=\textwidth}\begin{tabular}{p{0.6cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}}
    \toprule \addlinespace
    
    \csname @@input\endcsname{inputs/south_95_16/Results3RICTint_cit_South_95t16}

    \bottomrule \addlinespace
%\multicolumn{13}{l}{\emph{\underline{Sub-period from 1995 to 2007}}}\\ %\addlinespace
\csname @@input\endcsname{inputs/south_subperiod/Results3RICTint_cit_South_95t07}

\bottomrule \addlinespace
%\multicolumn{13}{l}{\emph{\underline{Sub-period from 1995 to 2007}}}\\ %\addlinespace
\csname @@input\endcsname{inputs/south_subperiod/Results3RICTint_cit_South_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to test the replacement effect for Southern European countries during the period 1995-2016. All regressions use industry level data for the subset of industries susceptible to automation, defined as industries were the use of industrial robots is prevalent (see Appendix Table~\ref{appendix:data}). All regressions include: country industry ($ci$); country year ($ct$); and industry year ($it$) fixed effects. All regressions are weighted by the base-sample-year share of each industry’s number of hours worked to country-wide hours worked.
    \end{table}
\FloatBarrier

\subsubsection{The reinstatement effect}
\label{appendix:reinstatement_country}
In Eastern Europe, we find robots to exhibit a negative association with country level wages and capital prices, but a positive one with total employment. 
For ICT, we observe the opposite pattern, i.e. increasing wages and capital prices. Effects on factor demand for labor and capital are not significant. 
We find that robots are correlated with increasing wage inequality and ICT with a decreasing output share of services. 

In Northern Europe, we do not find any support for a robot induced reinstatement effect: The diffusion of robots exhibits a negative association with factor prices and quantities for both, capital and labor. We also find that robot diffusion is associated with a decline in services. 
For ICT diffusion, we find almost no significant effects. We only observe an increasing output share of services after 2008. 

		\begin{table}[H]
    {\centering 
    \caption{The reinstatement effect in Eastern Europe}
    %\label{tab:regr_reinstatement}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|ccccccc}
    %\begin{adjustbox}{width=\textwidth}\begin{tabular}{p{0.6cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}|p{.95cm}p{.95cm}p{.95cm}}
    \toprule \addlinespace

\csname @@input\endcsname{inputs/east_95_16/Results4shortRICTint_ct_East_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/east_subperiod/Results4shortRICTint_ct_East_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/east_subperiod/Results4shortRICTint_ct_East_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to test the reinstatement effect for Eastern European countries during the period 1995-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); and country ($c$) and year ($t$) fixed effects.
    
    \end{table}



\FloatBarrier

		\begin{table}[H]
    {\centering 
    \caption{The reinstatement effect in Northern Europe}
    %\label{tab:regr_reinstatement}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|ccccccc}
    \toprule \addlinespace

\csname @@input\endcsname{inputs/north_95_16/Results4shortRICTint_ct_North_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/north_subperiod/Results4shortRICTint_ct_North_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/north_subperiod/Results4shortRICTint_ct_North_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to test the reinstatement effect for Northern European countries during the period 1995-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); and country ($c$) and year ($t$) fixed effects.
    
    \end{table}



\FloatBarrier

		\begin{table}[H]
    {\centering 
    \caption{The reinstatement effect in Southern Europe}
    %\label{tab:regr_reinstatement}
    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|ccccccc}
    \toprule \addlinespace

\csname @@input\endcsname{inputs/south_95_16/Results4shortRICTint_ct_South_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/south_subperiod/Results4shortRICTint_ct_South_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/south_subperiod/Results4shortRICTint_ct_South_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ }
    \scriptsize
    Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to test the reinstatement effect for Southern European countries during the period 1995-2016. All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; value added TFP--calculated as the residual from an OLS regression of value-added volumes ($VA$) on a translog production function including capital volumes ($K$) and total number of hours worked ($L$); and country ($c$) and year ($t$) fixed effects.
    
    \end{table}



\FloatBarrier

\subsubsection{The real income effect}
\label{appendix:real_income_country}
For the subset of Eastern European countries, we find that robot diffusion is significantly negatively correlated with factor incomes, both capital and labor. We find a negative impact on prices, but observe an expansion of output. 
ICT exhibits only a weak negative correlation with prices and TFP, and prior to 20017, we also observe a negative association with capital income. 

In Norther Europe, we observe similar patterns, i.e. negative correlations between robot diffusion and factor revenues and output prices. For ICT and the depth of automation, we do not find any significant effects. 

The patterns in Southern Europe are different: After 2008, we find that robots are significantly positively related to labor and capital income and to output and sales. WE also observe a positive correlation with TFP.  
	
	\begin{table}[H]
    {\centering 
        \caption{The real income effect in Eastern Europe}
            %\label{tab:regr_realincome_east_9516}

    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccccccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/east_95_16/Results5RICTint_ct_East_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/east_subperiod/Results5RICTint_ct_East_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/east_subperiod/Results5RICTint_ct_East_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ \noindent }
    \scriptsize
    Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to test the real income effect for Eastern European countries during the period 1995-2016. Labor productivity is measured as the share of gross output volumes ($Q$) over the total number of hours worked. TFP is calculated as the residual from an OLS regression of gross output volumes ($Q$) on a translog production function including capital volumes ($K$), total number of hours worked ($L$) and intermediate input volumes ($M$). All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; and country ($c$) and year ($t$) fixed effects.
    \end{table}


\FloatBarrier
	\begin{table}[H]
    {\centering 
        \caption{The real income effect in Northern Europe}
            %\label{tab:regr_realincome_north_9516}

    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccccccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/north_95_16/Results5RICTint_ct_North_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/north_subperiod/Results5RICTint_ct_North_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/north_subperiod/Results5RICTint_ct_North_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ \noindent }
    \scriptsize
    Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to test the real income effect for Northern European countries during the period 1995-2016. Labor productivity is measured as the share of gross output volumes ($Q$) over the total number of hours worked. TFP is calculated as the residual from an OLS regression of gross output volumes ($Q$) on a translog production function including capital volumes ($K$), total number of hours worked ($L$) and intermediate input volumes ($M$). All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; and country ($c$) and year ($t$) fixed effects.
    \end{table}


\FloatBarrier

	\begin{table}
    {\centering 
        \caption{The real income effect in Southern Europe}
            %\label{tab:regr_realincome_south_9516}

    \begin{adjustbox}{width=\textwidth}\begin{tabular}{l|cccccccc}
    \toprule \addlinespace
\csname @@input\endcsname{inputs/south_95_16/Results5RICTint_ct_South_95t16}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/south_subperiod/Results5RICTint_ct_South_95t07}
\bottomrule \addlinespace
\csname @@input\endcsname{inputs/south_subperiod/Results5RICTint_ct_South_08t16}
\bottomrule
    \end{tabular}\end{adjustbox}\\ \noindent }
    \scriptsize
    Notes: \sym{*}\(p<0.05\), \sym{**}\(p<0.01\), \sym{***}\(p<0.001\). Regression results to test the real income effect for Southern European countries during the period 1995-2016. Labor productivity is measured as the share of gross output volumes ($Q$) over the total number of hours worked. TFP is calculated as the residual from an OLS regression of gross output volumes ($Q$) on a translog production function including capital volumes ($K$), total number of hours worked ($L$) and intermediate input volumes ($M$). All regressions include: GDP growth, government consolidated gross debt as \% of GDP; government interest payable as \% of GDP; net government lending/borrowing as \% of GDP; gross fixed capital formation as \% of GDP; period average exchange rate; and country ($c$) and year ($t$) fixed effects.
    \end{table}



\section{Analysis at the sub-national level}
\label{SM:firm_level}
The impact of automation is heterogeneous across firms, industries and regions. 
To analyze the impact of automation on aggregate taxation, we would ideally have data that provides a direct link between firm and industry level production accounts and tax payments. 
%that can be aggregated to see impact of automation on the revenue side of governments' budgets. 
But this data does not exist and granular data on firm or industry level tax payments draws only a partial picture: For example, at the firm level we have data on corporate taxes charged on profits and represent a part of aggregate taxes on capital. But we do not know how profits of individual firms or industries affect individual wealth levels and the demand for saving, investment in financial accounts and durable goods (e.g. housing) which all are subject to other kinds of taxation. 

We complement the macro level analysis with a region level approach using firm level data provided by \citet{BvD2020data} and analyze the nexus between regional patterns of automation, labor demand and corporate tax payments in NUTS2-regions. This analysis draws only a partial picture of economic reality, but illustrates that the impacts of automation are diverse at the granular level. For governments, this understanding is important because --- dependent on the country-specific structure of tax administration --- locally raised taxes can be decisive to ensure the financing of essential public infrastructure. 

\subsection{Empirical approach}
	\label{SM:empirical_local_analysis}
	%The impact of ATs is heterogeneous across firms and industries. In the analyses described above, we study its effect on the structure of economic production and taxation at the national level. 
    But as explained in Sec. \ref{sec:background_taxation}, tax revenues are collected at different levels of government administration (central, federal, local).  
    For governments it is also relevant to understand the impact of automation at the local level. 
    To analyze the local effects of automation, we would ideally use regional data on economic production, automation and taxation. Unfortunately, this data is not available in a format that is consistent with the country level analysis introduced above. 
    
    As an alternative, we use firm level data being aware that firm level evidence draws only a partial picture of the economic reality. 
    In particular, we rely on the proprietary firm level data set Amadeus, the European counterpart of ORBIS-Global, which is a product of \citet{BvD2020data} (BvDEP). The underlying data are firms' financial statements sourced from various national registries (e.g. statistical agencies) and standardized by BvDEP for cross-country comparability.\footnote{For more details over the standardization procedure, see the correspondence tables used for each country by \citet{BvD2020manual}. 
    For the initial data cleaning and preparation procedure we follow \cite{kalemli2015construct}. Specifically, we drop firms reporting consolidated accounts, i.e. C1 and C2 codes and, if duplicate, the rest is kept based on the presence of annual reports over local registry filling. We also use annual records over quarters and late calendar months over early months.}
    
    For the analysis, we rely on balance sheet information of firms in the European countries where the industry level information on robot- or ICT-intensity exist for the period 2008-2016. To cover the largest set of regions across EU possible, we examine the effects of robot- and ICT-intensity separately and, thus, rely on the maximal amount of information available across data sets. More precisely, the sample used to analyze the impact of ICT-intensity ($ICT_{i,c,t}$) covers the same set of countries and industries used in the country  and industry level analysis from above. The sample used to analyze the impact of robot-intensity ($R_{i,c,t}$) also includes the following set of countries: Croatia (HR); Hungary (HU); Ireland (IE); Poland (PL); Portugal (PT); and Romania (RO).
    
    For each firm in the data set we retain those reporting strictly positive firm-year values on the number of employees or taxes payed. The latter refers to income tax expenses of the reporting period plus any net deferred tax expenses/income between the current and the previous reporting period. Conclusions drawn from this analysis are limited to a rather specific category of fiscal taxes, i.e. corporate income taxes.
    
    Each firm's primary production activity is based on the NACE Rev.2 (ISIC Rev.4) 2-digit industry code used to merge with the industry level measures on robot- and ICT-intensity.
    The sample includes the same set of 15 industry groups covered in the industry level sample (see Appendix Table~\ref{tab:industry_codes} for a detailed description of the industry codes). Finally, we link firms to the location of economic activity trough the NUTS version 2016 regional classification codes which across the EU and UK cover 281 regions at NUTS 2 and 1348 regions at NUTS 3 level \citep{eurostat2020nuts}. The sample used in our analysis for the effects of robot (ICT) intensity covers 273 (227) NUTS 2 and 1314 (1127) NUTS 3 regions. For more details over the summary statistics of the firm level sample and variables considered, see Appendix Table~\ref{tab:descriptives_firm}.

    ORBIS-Global is widely accepted as one of the best available options in terms of the richness of balance sheet information and cross-country comparability at the expense of incomplete coverage for smaller-sized firms with simplified financial reporting obligations \citep{bajgar2020coverage,kalemli2015construct}. Thus, while a large number of micro firms remain unrecorded, the sample manages to cover around 60\% of economic activity in terms of employment, on average (see Appendix Table~\ref{tab:coverage_firm_L}).\footnote{For similar evidence see \citet{bormans2020link}.}
    
    However, it is still crucial to understand the representativeness of the firm level corporate income taxes relative to the economy wide capital and corporate income taxes. Even when we look at the country level sample, we find that corporate taxes on income, profits and capital gains (variable code 1200 in \citet{OECD2019} data set) represent only 22\% of total capital taxes $T^{k}$, on average across sample-countries (see Appendix Table~\ref{tab:coverage_firm_T}). When we focus on the firm level samples we see that, on average, they represent around 20\% of the economy-wide corporate taxes on income, profits and capital gains (see Appendix Table~\ref{tab:coverage_firm_T}). This gap is mainly driven by the fact that in the firm level samples we only observe firms in the limited sub-set of the 15 industry groupings used in the industry level analysis and not the whole economy. However, even if we observed firm level data for the whole economy the sample will remain underrepresented, in line with the results from above on the coverage on employment. Overall, while the firm level data is helpful in uncovering interesting underlying heterogeneity, any results will capture a very limited part of the aggregate effects.
    
    Using a regression analysis, we estimate the impact of robot $R_{i,c,t}$ and $ICT_{i,c,t}$ intensity on regional labor demand $L_{f,r,i,t}$ and corporate tax payment $T^{\pi}_{f,r,i,t}$. To illustrate the effects, we estimate for each country the following specification
    \begin{equation}
        Y_{f,r,t} \sim \beta^{x}_{r} \cdot \mathbbm{1}(r,i)_f \cdot X_{i,c,t} + \epsilon_{r,f,t}
    \end{equation}
    where $Y_{f,r,t} \in \{ T^{\pi}_{f,r,t}, L_{f,r,t} \}$, $X_{i,c,t} \in \{ R_{i,c,t}, ICT_{i,c,t}\}$ and $i \in I_c$. $\mathbbm{1}(r,i)_f$ is a firm-specific dummy variable that equals one if firm $f$ is located in region $r$ and with primary economic activity in industry $i$.\footnote{Since we drop firms reporting consolidated accounts, we account for any double counting that could possibly arise from subsidiary firms integrating their statements to the national of international headquarter. However, we cannot control for such a possibility for multi-plant firms, due to the absence of data at such granular level.} All regressions include firm and NUTS3-region-year FE and are weighted using the same weights as in the industry level analysis, i.e. base-sample-year share of each industry’s number of hours worked to country-wide hours worked. For the standard errors, we use multi-way clustering at the industry, region and year level.
    
    Note that we combine data from different levels of aggregation here. In particular, we merge industry-country level data on automation with firm level data where the location of the firm is observed. This way we are able to map the industry-country level to the region-level dimension. However, since we do not directly observe the allocation of robot and ICT-intensity across regions, our estimation strategy assumes that all industries within an country are equally exposed to automation independent of the regional identity. Using this estimation strategy, we capture within-industry technological change and induced reallocation across firms that might be regionally unequally distributed.%\footnote{\green{@A: Moreover, do we use weights in the end? This should be mentioned here. Some general remark, not sure whether we should act on this, but we should think about reasons for our decision: Above, we have included R and ICT simultaneously. Why don't we do this here? I would not re-do the analysis, but we should be able to provide arguments (if a reviewer is asking for this, at least I would ask for this).} \textcolor{red}{@K and P: We use the same industry level weights as in the industry level analysis. Concerning the reasoning on why we do not include it simultaneously, I briefly discuss it above in the data section. The general idea is that Robot intensity is available for an additional 5 countries and thus we want to explore most of regions available.} \green{K@A: My question was related to the question whether we use firm-specific weight capturing the weight of a firm within and industry and the weight of an industry within a country simultaneously. In my view, still the best approach content-wise, but I suggest to do this only, if any reviewer is complaining about this. The firm level analysis is too limited in many other regards such that I find it is not worth the effort to spend more time on this.}} 
    
    We illustrate the effects of ICT and robot adoption at the regional level drawing maps that show the estimated effect $\beta_{r}$ on corporate taxes and on local labor demand. Different color codes indicate the size and direction of the expected impact.
    
	
	\FloatBarrier

\subsection{Results}
\label{SM:results_local_analysis}
In the preceding analysis, we observed that the economic effects of automation can be heterogeneous across different groups of countries. This indicates that local conditions matter. Now, we explore regional heterogeneity at the sub-national level. 

In Fig. \ref{fig:ai_nuts2}, we show the regional effects of automation at the level of NUTS2 regions. The figures on top (Fig. \ref{fig:nuts2_LR} and \ref{fig:nuts2_LICT}) show the effects on local labor demand that is captured by the firms in our sample. The figures at the bottom illustrate the correlation between automation and corporate tax revenues (Fig. \ref{fig:nuts2_TR} and \ref{fig:nuts2_TICT}). On the left (right) hand side, we show the estimated effects of robot (ICT) adoption. The colors indicate the scale of the effect where green color indicates positive and red color negative estimated effects. 
Additional plots at the NUTS3 and at the country level aggregated from firm level data are available in the Appendix \ref{appendix:add_results_local_effects}. 

Visually, indicated by the similar coloring patterns comparing the map at the top with its analog at the bottom, it can be seen that in most regions the effects of automation on labor and taxation point into the same direction: When ATs exhibit a negative association with employment, we also observe a negative impact with corporate tax payments. Few exceptions at the local level exist where we find an opposite pattern of correlation. For example, in Alentejo (Portugal, PT18) and in Corse (France, FR83) the impact of robots on labor is negatively correlated with its impact on corporate taxes. In parts of Ireland and many regions of the UK, we observe generally a negative correlation between the effect of robots on tax revenues and on labor as indicated by opposite coloring codes for each NUTS regions, i.e. robots have a negative impact on labor but a positive impact on corporate tax payments and vice versa. 
% Note for interpretation: This could be due to distributional issues (for example, when robots come, many employment-intensive, but unproductive firms exit the market and high-profit-superstars with low employment grow) but it can be also due to design of fiscal policies. And many other explanations possible, recall industry level data and also cross-industry reallocation possible. 

We also observe that the impact of robots compared to ICT differs across regions and countries. For example, we observe robots to have a positive impact on labor and taxation in Italy, but we find a negative impact of ICT. The opposite pattern holds true for parts of Greece where ICT tends to exhibit a positive effect, but robots a negative one. 

Generally, we find that most regions in Spain, France and the Baltic countries to be the beneficiaries of automation: Both, robots and ICT diffusion, exhibit positive effects on regional labor demand and corporate taxation. The estimated effects draw a mixed picture of Germany and the UK: Some regions exhibit strong negative, others strong positive impacts. In Sweden and Finland, we find negative effects of robot diffusion on both, labor and taxes, and mixed effects of ICT. 

\begin{figure}
    {\centering
    
    \caption{Automation at the sub-national level (NUTS2 regions)}
    \label{fig:ai_nuts2}
    \begin{subfigure}[r]{0.49\textwidth}
    \subcaption{Labor \& robots}
     \label{fig:nuts2_LR}
     \includegraphics[width=\textwidth]{inputs/maps/NUTS2_lnL_R.pdf}
    \end{subfigure}
        \begin{subfigure}[r]{0.49\textwidth}
        \subcaption{Labor \& ICT}
         \label{fig:nuts2_LICT}
     \includegraphics[width=\textwidth]{inputs/maps/NUTS2_lnL_ICT.pdf}
    \end{subfigure}
    
    \begin{subfigure}[r]{0.49\textwidth}
    \subcaption{Taxes \& robots}
    \label{fig:nuts2_TR}
     \includegraphics[width=\textwidth]{inputs/maps/NUTS2_lnT_R.pdf}
    \end{subfigure}
    \begin{subfigure}[r]{0.49\textwidth}
    \subcaption{Taxes \& ICT}
    \label{fig:nuts2_TICT}
     \includegraphics[width=\textwidth]{inputs/maps/NUTS2_lnT_ICT.pdf}
     
    \end{subfigure}}
    \footnotesize
     \scriptsize
	    Source: Author's calculations based on ORBIS Global, IFR and EUKLEMS data sets.\\
	    Notes: Each map presents the point estimates from regressing for each country separately the ln of the firm level corporate income tax ($Taxes$) and number of employees ($L$), respectively, on the industry level robot ($R$) or $ICT$ intensity interacted with a full set of NUTS2 version 2016-regional dummies. All regressions include firm and NUTS3 version 2016-region-year fixed effects and are weighted using the same weights as in the industry level analysis, i.e. base-sample-year share of each industry’s number of hours worked to country-wide hours worked. The estimated effects are plotted with 2 shades of green and red for two groups of positive and negative values, respectively, with the darker colors representing stronger effects. Regions with no data are left blank. Panels (a) and (c) cover 273 NUTS2 regions, while panels (b) and (d) cover 227 NUTS2 regions.
\end{figure}


\FloatBarrier	

\subsection{Discussion and insights}
	Our analysis at the sub-national (NUTS2) level underlines the heterogeneity of impacts in two regards: (1) The linkage between economic outcomes, taxes to automation, and (2) the relationship between economic outcomes and tax payments differ across regions. Limited to corporate taxation in the period 2008-2016 and covering only a subset of industries and firms, we find that automation is positively correlated with employment in some regions, while negatively in others. 
	In most regions, we find a positive correlation between employment and taxes: Hence, when the net of the replacement and reinstatement effect is employment increasing, corporate tax payments tend to be higher. However, this relationship is reverse for some of the regions in our analysis. 
	Note that the sub-national analysis draws only a partial picture of the aggregate reality: Due to data limitations, we cover only corporate tax payments of a subset of firms drawn from a subset of industries. Corporate tax payments are a subset of capital taxes and represent only a fraction of total taxation. Hence, the results can not be extrapolated to the flows of aggregate taxation.
	%\footnote{\textcolor{red}{@A: Here it would be nice to have a number, i.e. (1) aggr. corporate taxes (covered by our data) over (1) $T^k$ and (2) $T^{total}$. You can use the average across countries, but if this is not too much effort, it would be also nice to see it country-wise which can be also an indicator how well our regional analysis represents a country.}}

\subsection{Additional information on firm level data}

\subsubsection{Data and descriptives}
		\begin{table}[H]
	 \caption{Representativeness of employment in ORBIS vs. EUKLEMS data}
        \label{tab:coverage_firm_L}
        {\centering
        %\begin{adjustbox}{width=\textwidth}
        \begin{tabular}{lccccc}
        \toprule
         \input{inputs/coverage/Coverage_sample_firm_L}
         \bottomrule
        \end{tabular}
        %\end{adjustbox}
        }\\
       \scriptsize
        Notes: Columns (1), (2) and (3) show the total number of employees in EUKLEMS, $R$-sample and $ICT$-sample, respectively, for each country in the last sample period, i.e. 2016.  $R$- and $ICT$-sample refer to the firm level ORBIS sample when robot- and ICT-density is reported, respectively. Columns (4) and (5) report the employment shares in \% covered by the firm level sample relative to the aggregate data in EUKLEMS, i.e. the ratio of (2) over (1) and (3) over (1), respectively. All samples cover the same 15 industry-groupings used in the analysis and discussed in detail in Appendix Table~\ref{tab:industry_codes}. 
    \end{table}
    
		\begin{table}[H]
	 \caption{Representativeness of corporate taxes in ORBIS firm level samples vs. OECD country level data.}
        \label{tab:coverage_firm_T}
        {\centering
        \begin{adjustbox}{width=0.8\textwidth}
        \begin{tabular}{lccccc}
        \toprule
         \input{inputs/coverage/Coverage_sample_firm_T}
         \bottomrule
        \end{tabular}
        \end{adjustbox}
        }\\
       \scriptsize
         Notes: Column (1) shows the total tax on capital $T^{k}$ in billions of national currency for each country in the last sample period, i.e. 2016. Column (2) is a sub-category of column (1) capturing corporate taxes on income, profits and capital gains $T^{k,corp}$ (with variable code 1200 in \citet{OECD2019} data set). Column (3) is the ratio of (1) over (2) in \%. Columns (4) and (5) capture the share of total taxes reported in the $R$- and $ICT$-sample used in the analysis, respectively, over (2) in \%. $R$- and $ICT$-sample refer to the firm level ORBIS sample when robot- and ICT-density is reported, respectively. The aggregate taxes cover the whole economy while the firm level samples cover the 15 industry-groupings discussed in detail in Appendix Table~\ref{tab:industry_codes}.  
    \end{table}


			    \begin{table}[H]
		            \caption{Summary statistics for firm level sample}
\label{tab:descriptives_firm}

	    \scriptsize
        {\centering
        \begin{adjustbox}{width=1\textwidth}
\begin{tabular}{lcccc}
\toprule
\csname @@input\endcsname{inputs/descriptives/Sumstat_firm}
\midrule
\csname @@input\endcsname{inputs/descriptives/Sumstat_firm_more}
\end{tabular}
\end{adjustbox}
}\\
\scriptsize
 Notes: $\dagger$ refers to values in thousands for the Mean, St.Dev., Min, Median, and Max. This table presents the summary statistics on the firm level corporate income tax ($T_{f,i,t}$) and number of employees ($L_{f,i,t}$) for 2 different samples. $R$- and $ICT$-sample refer to samples with non-missing values of industry level robot- and ICT-intensity, respectively. The $ICT$-sample covers the following 18 countries: AT; BE; CZ; DE; DK; EE; ES; FI; FR; GR; IT; LT; LV; NL; SE; SI; SK; and UK, while the $R$-sample covers 6 additional countries: HR; HU; IE; PL; PT; and RO. Both samples cover the same set of 15 industry groups included in the industry level analysis---for more details see Appendix Table~\ref{tab:industry_codes}.
\end{table}


\subsubsection{Additional results}
\label{appendix:add_results_local_effects}

\begin{figure}[H]
    {\centering
    \begin{subfigure}[r]{0.49\textwidth}
    
     \includegraphics[width=\linewidth]{inputs/maps/NUTS0_lnL_R.pdf}
     
     \subcaption{Labor \& robots}
    \end{subfigure}
        \begin{subfigure}[r]{0.49\textwidth}
     \includegraphics[width=\linewidth]{inputs/maps/NUTS0_lnL_ICT.pdf}
     
        \subcaption{Labor \& ICT}
    \end{subfigure}
    
    \begin{subfigure}[r]{0.49\textwidth}
     \includegraphics[width=\linewidth]{inputs/maps/NUTS0_lnT_R.pdf}
     
    \subcaption{Taxes \& robots}
    \end{subfigure}
    \begin{subfigure}[r]{0.49\textwidth}
     \includegraphics[width=\linewidth]{inputs/maps/NUTS0_lnT_ICT.pdf}
     
    \subcaption{Taxes \& ICT}
    \end{subfigure}
    \caption{automation at the national level (NUTS0 regions)}
    \label{fig:ai_nuts0}
    }
    \scriptsize
    Source: Author's calculations based on ORBIS Global, IFR and EUKLEMS data sets.\\
    Notes: Each map presents the point estimates from regressing for each country separately the ln of the firm level corporate income tax ($Taxes$) and number of employees ($L$), respectively, on the industry level robot ($R$) or $ICT$ intensity. All regressions include firm and NUTS3 version 2016-region-year fixed effects and are weighted using the same weights as in the industry level analysis, i.e. base-sample-year share of each industry’s number of hours worked to country-wide hours worked. The estimated effects are plotted with 2 shades of green and red for two groups of positive and negative values, respectively, with the darker colors representing stronger effects. Regions with no data are left blank.    
\end{figure}

%\begin{comment}

\begin{figure}
    {\centering
    \begin{subfigure}[r]{0.49\textwidth}
    
     \includegraphics[width=\linewidth]{inputs/maps/NUTS3_lnL_R.pdf}
     
     \subcaption{Labor \& robots}
    \end{subfigure}
        \begin{subfigure}[r]{0.49\textwidth}
     \includegraphics[width=\linewidth]{inputs/maps/NUTS3_lnL_ICT.pdf}
     
        \subcaption{Labor \& ICT}
    \end{subfigure}
    
    \begin{subfigure}[r]{0.49\textwidth}
     \includegraphics[width=\linewidth]{inputs/maps/NUTS3_lnT_R.pdf}
     
    \subcaption{Taxes \& robots}
    \end{subfigure}
    \begin{subfigure}[r]{0.49\textwidth}
     \includegraphics[width=\linewidth]{inputs/maps/NUTS3_lnT_ICT.pdf}
     
    \subcaption{Taxes \& ICT}
    \end{subfigure}
    \caption{automation at the sub-national level (NUTS3 regions)}
    \label{fig:ai_nuts3}
    }
    \scriptsize
    Source: Author's calculations based on ORBIS Global, IFR and EUKLEMS data sets.\\
    Notes: Each map presents the point estimates from regressing for each country separately the ln of the firm level corporate income tax ($Taxes$) and number of employees ($L$), respectively, on the industry level robot ($R$) or $ICT$ intensity interacted with a full set of NUTS3 version 2016-regional dummies. All regressions include firm and NUTS3 version 2016-region-year fixed effects and are weighted using the same weights as in the industry level analysis, i.e. base-sample-year share of each industry’s number of hours worked to country-wide hours worked. The estimated effects are plotted with 2 shades of green and red for two groups of positive and negative values, respectively, with the darker colors representing stronger effects. Regions with no data are left blank. Panels (a), (b), (c) and (d) cover 1310, 1119, 1314, and 1123 NUTS3 regions, respectively.
\end{figure}
    
%\end{comment}

\input{robustness_endogenous_automation}
\input{robustness_tax_trade_distribution}



